Representing Long-Range Context for Graph Neural Networks with Global Attention

Graph neural networks are powerful architectures for structured datasets. However, current methods struggle to represent long-range dependencies. Scaling the depth or width of GNNs is insufficient to broaden receptive fields as larger GNNs encounter optimization instabilities such as vanishing gradients and representation oversmoothing, while pooling-based approaches have yet to become as universally useful as in computer vision. In this work, we propose the use of Transformer-based self-attention to learn long-range pairwise relationships, with a novel "readout" mechanism to obtain a global graph embedding. Inspired by recent computer vision results that find position-invariant attention performant in learning long-range relationships, our method, which we call GraphTrans, applies a permutation-invariant Transformer module after a standard GNN module. This simple architecture leads to state-of-the-art results on several graph classification tasks, outperforming methods that explicitly encode graph structure. Our results suggest that purely-learning-based approaches without graph structure may be suitable for learning high-level, long-range relationships on graphs. Code for GraphTrans is available at https://github.com/ucbrise/graphtrans.

==> combined.tex <==
@inproceedings{Zhao2020PairNorm:,
 author = {Lingxiao Zhao and
Leman Akoglu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ZhaoA20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {PairNorm: Tackling Oversmoothing in GNNs},
 url = {https://openreview.net/forum?id=rkecl1rtwB},
 year = {2020}
}

@inproceedings{li2019deepgcns,
 author = {Guohao Li and
Matthias M{\"{u}}ller and
Ali K. Thabet and
Bernard Ghanem},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/Li0TG19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00936},
 pages = {9266--9275},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {DeepGCNs: Can GCNs Go As Deep As CNNs?},
 url = {https://doi.org/10.1109/ICCV.2019.00936},
 year = {2019}
}

@inproceedings{fernandes2018structured,
 author = {Patrick Fernandes and
Miltiadis Allamanis and
Marc Brockschmidt},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/FernandesAB19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Structured Neural Summarization},
 url = {https://openreview.net/forum?id=H1ersoRqtm},
 year = {2019}
}

@inproceedings{Bahdanau2015NeuralMT,
 author = {Dzmitry Bahdanau and
Kyunghyun Cho and
Yoshua Bengio},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/BahdanauCB14.bib},
 booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Fri, 29 Mar 2019 00:00:00 +0100},
 title = {Neural Machine Translation by Jointly Learning to Align and Translate},
 url = {http://arxiv.org/abs/1409.0473},
 year = {2015}
}

@inproceedings{corso2020pna,
 author = {Gabriele Corso and
Luca Cavalleri and
Dominique Beaini and
Pietro Li{\`{o}} and
Petar Velickovic},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/CorsoCBLV20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Principal Neighbourhood Aggregation for Graph Nets},
 url = {https://proceedings.neurips.cc/paper/2020/hash/99cad265a1768cc2dd013f0e740300ae-Abstract.html},
 year = {2020}
}

@inproceedings{vinyals2016order,
 author = {Oriol Vinyals and
Samy Bengio and
Manjunath Kudlur},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/VinyalsBK15.bib},
 booktitle = {4th International Conference on Learning Representations, {ICLR} 2016,
San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Order Matters: Sequence to sequence for sets},
 url = {http://arxiv.org/abs/1511.06391},
 year = {2016}
}

@inproceedings{zhang2018end,
 author = {Muhan Zhang and
Zhicheng Cui and
Marion Neumann and
Yixin Chen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/ZhangCNC18.bib},
 booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
(AAAI-18), the 30th innovative Applications of Artificial Intelligence
(IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
Artificial Intelligence (EAAI-18), New Orleans, Louisiana, USA, February
2-7, 2018},
 editor = {Sheila A. McIlraith and
Kilian Q. Weinberger},
 pages = {4438--4445},
 publisher = {{AAAI} Press},
 timestamp = {Mon, 22 Oct 2018 01:00:00 +0200},
 title = {An End-to-End Deep Learning Architecture for Graph Classification},
 url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/17146},
 year = {2018}
}

@inproceedings{Errica2020A,
 author = {Federico Errica and
Marco Podda and
Davide Bacciu and
Alessio Micheli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ErricaPBM20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {A Fair Comparison of Graph Neural Networks for Graph Classification},
 url = {https://openreview.net/forum?id=HygDF6NFPB},
 year = {2020}
}

@article{wale_comparison_2008,
 author = {Wale, Nikil and Watson, Ian A. and Karypis, George},
 doi = {10.1007/s10115-007-0103-5},
 issn = {0219-3116},
 journal = {Knowledge and Information Systems},
 number = {3},
 pages = {347--375},
 title = {Comparison of descriptor spaces for chemical compound retrieval and classification},
 url = {https://doi.org/10.1007/s10115-007-0103-5},
 volume = {14},
 year = {2008}
}

@inproceedings{hu2020ogb,
 author = {Weihua Hu and
Matthias Fey and
Marinka Zitnik and
Yuxiao Dong and
Hongyu Ren and
Bowen Liu and
Michele Catasta and
Jure Leskovec},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/HuFZDRLCL20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Open Graph Benchmark: Datasets for Machine Learning on Graphs},
 url = {https://proceedings.neurips.cc/paper/2020/hash/fb60d411a5c5b72b2e7d3527cfc84fd0-Abstract.html},
 year = {2020}
}

@article{tailor2021adaptive,
 author = {Tailor, Shyam A and Opolka, Felix L and Li{\`o}, Pietro and Lane, Nicholas D},
 journal = {ArXiv preprint},
 title = {Adaptive Filters and Aggregator Fusion for Efficient Graph Convolutions},
 url = {https://arxiv.org/abs/2104.01481},
 volume = {abs/2104.01481},
 year = {2021}
}

@inproceedings{Wu2020LiteTransformer,
 author = {Zhanghao Wu and
Zhijian Liu and
Ji Lin and
Yujun Lin and
Song Han},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/WuLLLH20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Tue, 22 Dec 2020 00:00:00 +0100},
 title = {Lite Transformer with Long-Short Range Attention},
 url = {https://openreview.net/forum?id=ByeMPlHKPH},
 year = {2020}
}

@inproceedings{Chen:2018vf,
 address = {Melbourne, Australia},
 author = {Chen, Mia Xu  and
Firat, Orhan  and
Bapna, Ankur  and
Johnson, Melvin  and
Macherey, Wolfgang  and
Foster, George  and
Jones, Llion  and
Schuster, Mike  and
Shazeer, Noam  and
Parmar, Niki  and
Vaswani, Ashish  and
Uszkoreit, Jakob  and
Kaiser, Lukasz  and
Chen, Zhifeng  and
Wu, Yonghui  and
Hughes, Macduff},
 booktitle = {Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
 doi = {10.18653/v1/P18-1008},
 pages = {76--86},
 publisher = {Association for Computational Linguistics},
 title = {The Best of Both Worlds: Combining Recent Advances in Neural Machine Translation},
 url = {https://aclanthology.org/P18-1008},
 year = {2018}
}

@inproceedings{Pereyra:2016regularizing,
 author = {Pereyra, Gabriel and Tucker, George and Chorowski, Jan and Kaiser, Lukasz and Hinton, Geoffrey},
 booktitle = {ICLR Workshop},
 title = {Regularizing Neural Networks by Penalizing Confident Output Distributions},
 year = {2017}
}

@inproceedings{Wu:2019payless,
 author = {Felix Wu and
Angela Fan and
Alexei Baevski and
Yann N. Dauphin and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/WuFBDA19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Pay Less Attention with Lightweight and Dynamic Convolutions},
 url = {https://openreview.net/forum?id=SkVhlh09tX},
 year = {2019}
}

@inproceedings{Sukhbaatar:2019adaptive,
 address = {Florence, Italy},
 author = {Sukhbaatar, Sainbayar  and
Grave, Edouard  and
Bojanowski, Piotr  and
Joulin, Armand},
 booktitle = {Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/P19-1032},
 pages = {331--335},
 publisher = {Association for Computational Linguistics},
 title = {Adaptive Attention Span in Transformers},
 url = {https://aclanthology.org/P19-1032},
 year = {2019}
}

@techreport{Tsarkov-CFQ:Task,
 arxivid = {2012.08266v1},
 author = {Tsarkov, Dmitry and Tihon, Tibor and Scales, Nathan and Momchev, Nikola and Sinopalnikov, Danila and Sch{\"{a}}rli, Nathanael},
 isbn = {2012.08266v1},
 title = {{*-CFQ: Analyzing the Scalability of Machine Learning on a Compositional Task}},
 url = {https://github.com/google-research/google-}
}

@article{Dwivedi2020AGraphs,
 author = {Dwivedi, Vijay Prakash and Bresson, Xavier},
 journal = {ArXiv preprint},
 title = {{A Generalization of Transformer Networks to Graphs}},
 url = {https://arxiv.org/abs/2012.09699},
 volume = {abs/2012.09699},
 year = {2020}
}

@inproceedings{Bunel2016AdaptiveCompilation,
 author = {Rudy Bunel and
Alban Desmaison and
Pawan Kumar Mudigonda and
Pushmeet Kohli and
Philip H. S. Torr},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/BunelDMKT16.bib},
 booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
on Neural Information Processing Systems 2016, December 5-10, 2016,
Barcelona, Spain},
 editor = {Daniel D. Lee and
Masashi Sugiyama and
Ulrike von Luxburg and
Isabelle Guyon and
Roman Garnett},
 pages = {1444--1452},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Adaptive Neural Compilation},
 url = {https://proceedings.neurips.cc/paper/2016/hash/f0adc8838f4bdedde4ec2cfad0515589-Abstract.html},
 year = {2016}
}

@inproceedings{Johnson2020AdaScaleTraining,
 author = {Tyler B. Johnson and
Pulkit Agrawal and
Haijie Gu and
Carlos Guestrin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/JohnsonAGG20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {4911--4920},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {AdaScale {SGD:} {A} User-Friendly Algorithm for Distributed Training},
 url = {http://proceedings.mlr.press/v119/johnson20a.html},
 volume = {119},
 year = {2020}
}

@inproceedings{DosovitskiyANSCALE,
 author = {Alexey Dosovitskiy and
Lucas Beyer and
Alexander Kolesnikov and
Dirk Weissenborn and
Xiaohua Zhai and
Thomas Unterthiner and
Mostafa Dehghani and
Matthias Minderer and
Georg Heigold and
Sylvain Gelly and
Jakob Uszkoreit and
Neil Houlsby},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/DosovitskiyB0WZ21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {An Image is Worth 16x16 Words: Transformers for Image Recognition
at Scale},
 url = {https://openreview.net/forum?id=YicbFdNTTy},
 year = {2021}
}

@techreport{Tanaka2021AutomaticLearning,
 arxivid = {2103.16063v1},
 author = {Tanaka, Masahiro and Taura, Kenjiro and Hanawa, Toshihiro and Torisawa, Kentaro},
 title = {{Automatic Graph Partitioning for Very Large-scale Deep Learning}},
 year = {2021}
}

@inproceedings{ZhouBERTExit,
 author = {Wangchunshu Zhou and
Canwen Xu and
Tao Ge and
Julian J. McAuley and
Ke Xu and
Furu Wei},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/ZhouXGM0W20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {{BERT} Loses Patience: Fast and Robust Inference with Early Exit},
 url = {https://proceedings.neurips.cc/paper/2020/hash/d4dd111a4fd973394238aca5c05bebe3-Abstract.html},
 year = {2020}
}

@inproceedings{IvanovBOOSTNETWORKS,
 author = {Sergei Ivanov and
Liudmila Prokhorenkova},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/0004P21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Boost then Convolve: Gradient Boosting Meets Graph Neural Networks},
 url = {https://openreview.net/forum?id=ebS5NUfoMKL},
 year = {2021}
}

@misc{RexfordClosingLoop,
 author = {Rexford, Jennifer},
 title = {{Closing the Network Control Loop}},
 url = {https://www.youtube.com/watch?v=XUxC8kXEYo0&feature=youtu.be&ab_channel=OpenNetworkingFoundation}
}

@article{Cappart2021CombinatorialNetworks,
 author = {Cappart, Quentin and Ch{\'{e}}telat, Didier and Khalil, Elias and Lodi, Andrea and Morris, Christopher and Veli{\v{c}}kovi{\'{c}}, Petar},
 journal = {ArXiv preprint},
 title = {{Combinatorial optimization and reasoning with graph neural networks}},
 url = {https://arxiv.org/abs/2102.09544},
 volume = {abs/2102.09544},
 year = {2021}
}

@inproceedings{Belilovsky2019DecoupledCNNs,
 author = {Eugene Belilovsky and
Michael Eickenberg and
Edouard Oyallon},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/BelilovskyEO20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {736--745},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Decoupled Greedy Learning of CNNs},
 url = {http://proceedings.mlr.press/v119/belilovsky20a.html},
 volume = {119},
 year = {2020}
}

@inproceedings{Jaderberg2016DecoupledGradients,
 author = {Max Jaderberg and
Wojciech Marian Czarnecki and
Simon Osindero and
Oriol Vinyals and
Alex Graves and
David Silver and
Koray Kavukcuoglu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/JaderbergCOVGSK17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {1627--1635},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Decoupled Neural Interfaces using Synthetic Gradients},
 url = {http://proceedings.mlr.press/v70/jaderberg17a.html},
 volume = {70},
 year = {2017}
}

@techreport{NarangDoApplications,
 arxivid = {2102.11972v1},
 author = {Narang, Sharan and Won, Hyung and Tay, Chung Yi and Fedus, William and Fevry, Thibault and Matena, Michael and Malkan, Karishma and Fiedel, Noah and Shazeer, Noam and Lan, Zhenzhong and Zhou, Yanqi and Li, Wei and Ding, Nan and Marcus, Jake and Roberts, Adam and Raffel, Colin},
 title = {{Do Transformer Modifications Transfer Across Implementations and Applications?}},
 url = {https://github.com/google-research/}
}

@techreport{NarayananEfficientClusters,
 arxivid = {2104.04473v1},
 author = {Narayanan, Deepak and Shoeybi, Mohammad and Casper, Jared and Legresley, Patrick and Patwary, Mostofa and Korthikanti, Vijay and Vainbrand, Dmitri and Kashinkunti, Prethvi and Bernauer, Julie and Catanzaro, Bryan and Phanishayee, Amar and Zaharia, Matei},
 isbn = {2104.04473v1},
 title = {{Efficient Large-Scale Language Model Training on GPU Clusters; Efficient Large-Scale Language Model Training on GPU Clusters}},
 url = {https://github.com/nvidia/megatron-lm;}
}

@techreport{CarionEnd-to-EndTransformers,
 arxivid = {2005.12872v3},
 author = {Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
 title = {{End-to-End Object Detection with Transformers}},
 url = {https://github.com/facebookresearch/detr.}
}

@inproceedings{Andor2019GivingComprehension,
 address = {Hong Kong, China},
 author = {Andor, Daniel  and
He, Luheng  and
Lee, Kenton  and
Pitler, Emily},
 booktitle = {Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)},
 doi = {10.18653/v1/D19-1609},
 pages = {5947--5952},
 publisher = {Association for Computational Linguistics},
 title = {Giving {BERT} a Calculator: Finding Operations and Arguments with Reading Comprehension},
 url = {https://aclanthology.org/D19-1609},
 year = {2019}
}

@inproceedings{BelilovskyGreedyImageNet,
 author = {Eugene Belilovsky and
Michael Eickenberg and
Edouard Oyallon},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/BelilovskyEO19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {583--593},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Greedy Layerwise Learning Can Scale To ImageNet},
 url = {http://proceedings.mlr.press/v97/belilovsky19a.html},
 volume = {97},
 year = {2019}
}

@article{Park2020HetPipe:Parallelism,
 author = {Park, Jay H. and Yun, Gyeongchan and Yi, Chang M. and Nguyen, Nguyen T. and Lee, Seungmin and Choi, Jaesik and Noh, Sam H. and Choi, Young-ri},
 journal = {ArXiv preprint},
 title = {{HetPipe: Enabling Large DNN Training on (Whimpy) Heterogeneous GPU Clusters through Integration of Pipelined Model Parallelism and Data Parallelism}},
 url = {https://arxiv.org/abs/2005.14038},
 volume = {abs/2005.14038},
 year = {2020}
}

@techreport{ZhongHierarchicalNetworks,
 arxivid = {2009.03717v1},
 author = {Zhong, Zhiqiang and Li, Cheng-Te and Pang, Jun},
 keywords = {Index Terms-Graph neural networks, hierarchical structure, network communities !, representation learning},
 title = {{Hierarchical Message-Passing Graph Neural Networks}},
 url = {https://github.com/}
}

@inproceedings{Brock2021High-PerformanceNormalization,
 author = {Andy Brock and
Soham De and
Samuel L. Smith and
Karen Simonyan},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/BrockDSS21.bib},
 booktitle = {Proceedings of the 38th International Conference on Machine Learning,
{ICML} 2021, 18-24 July 2021, Virtual Event},
 editor = {Marina Meila and
Tong Zhang},
 pages = {1059--1071},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 25 Aug 2021 01:00:00 +0200},
 title = {High-Performance Large-Scale Image Recognition Without Normalization},
 url = {http://proceedings.mlr.press/v139/brock21a.html},
 volume = {139},
 year = {2021}
}

@misc{HowResearch,
 title = {{How to write a great research paper - Microsoft Research}},
 url = {https://www.microsoft.com/en-us/research/academic-program/write-great-research-paper/}
}

@inproceedings{Tay2020HYPERGRIDTASKS,
 author = {Yi Tay and
Zhe Zhao and
Dara Bahri and
Donald Metzler and
Da{-}Cheng Juan},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/TayZBMJ21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {HyperGrid Transformers: Towards {A} Single Model for Multiple Tasks},
 url = {https://openreview.net/forum?id=hiq1rHO8pNT},
 year = {2021}
}

@inproceedings{HaHYPERNETWORKS,
 author = {David Ha and
Andrew M. Dai and
Quoc V. Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HaDL17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {HyperNetworks},
 url = {https://openreview.net/forum?id=rkpACe1lx},
 year = {2017}
}

@article{Zhou2020Informer:Forecasting,
 author = {Zhou, Haoyi and Zhang, Shanghang and Peng, Jieqi and Zhang, Shuai and Li, Jianxin and Xiong, Hui and Zhang, Wancai},
 journal = {ArXiv preprint},
 title = {{Informer: Beyond Efficient Transformer for Long Sequence Time-Series Forecasting}},
 url = {https://arxiv.org/abs/2012.07436},
 volume = {abs/2012.07436},
 year = {2020}
}

@inproceedings{GevaInjectingModels,
 address = {Online},
 author = {Geva, Mor  and
Gupta, Ankit  and
Berant, Jonathan},
 booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/2020.acl-main.89},
 pages = {946--958},
 publisher = {Association for Computational Linguistics},
 title = {Injecting Numerical Reasoning Skills into Language Models},
 url = {https://aclanthology.org/2020.acl-main.89},
 year = {2020}
}

@techreport{LentonIVY:PORTABILITY,
 arxivid = {2102.02886v3},
 author = {Lenton, Daniel and Pardo, Fabio and Falck, Fabian and James, Stephen and Clark, Ronald},
 title = {{IVY: TEMPLATED DEEP LEARNING FOR INTER-FRAMEWORK PORTABILITY}},
 url = {https://ivy-dl.org.}
}

@techreport{NvidiaLargeHours,
 arxivid = {1808.01371v2},
 author = {Nvidia, Raul Puri and Nvidia, Robert Kirby and Nvidia, Nikolai Yakovenko and Catanzaro, Bryan},
 title = {{Large Scale Language Modeling: Converging on 40GB of Text in Four Hours}},
 url = {https://github.com/NVIDIA/sentiment-}
}

@inproceedings{BunelLEARNINGPROGRAMS,
 author = {Rudy Bunel and
Alban Desmaison and
M. Pawan Kumar and
Philip H. S. Torr and
Pushmeet Kohli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/BunelDKTK17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Learning to superoptimize programs},
 url = {https://openreview.net/forum?id=r1rz6U5lg},
 year = {2017}
}

@article{MoweiWang2017MachineOpportunities,
 author = {{Mowei Wang} and {Yong Cui} and {Xin Wang} and {Shihan Xiao} and {Junchen Jiang}},
 doi = {10.1109/MNET.2017.1700200},
 title = {{Machine Learning for Networking: Workflow, Advances and Opportunities}},
 year = {2017}
}

@article{Maziarka2020MoleculeTransformer,
 author = {Maziarka, Łukasz and Danel, Tomasz and Mucha, Sławomir and Rataj, Krzysztof and Tabor, Jacek and Jastrz{\c{e}}bski, Stanisław},
 journal = {ArXiv preprint},
 title = {{Molecule Attention Transformer}},
 url = {https://arxiv.org/abs/2002.08264},
 volume = {abs/2002.08264},
 year = {2020}
}

@inproceedings{GuptaNEURALTEXT,
 author = {Nitish Gupta and
Kevin Lin and
Dan Roth and
Sameer Singh and
Matt Gardner},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/GuptaLR0020.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Neural Module Networks for Reasoning over Text},
 url = {https://openreview.net/forum?id=SygWvAVFPr},
 year = {2020}
}

@misc{Laskin2020ParallelUpdates,
 arxivid = {2012.03837},
 author = {Laskin, Michael and Abbeel, Pieter and Metz, Luke and Sohl-Dickstein, Jascha and Nabarro, Seth and Noune, Badreddine and Luschi, Carlo and Saroufim, Mark},
 booktitle = {arXiv},
 issn = {23318422},
 title = {{Parallel training of deep networks with local updates}},
 url = {https://openreview.net/forum?id=ufS1zWbRCEa},
 year = {2020}
}

@inproceedings{HoulsbyParameter-EfficientNLP,
 author = {Neil Houlsby and
Andrei Giurgiu and
Stanislaw Jastrzebski and
Bruna Morrone and
Quentin de Laroussilhe and
Andrea Gesmundo and
Mona Attariyan and
Sylvain Gelly},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/HoulsbyGJMLGAG19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {2790--2799},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Parameter-Efficient Transfer Learning for {NLP}},
 url = {http://proceedings.mlr.press/v97/houlsby19a.html},
 volume = {97},
 year = {2019}
}

@inproceedings{Jaegle2021Perceiver:Attention,
 author = {Andrew Jaegle and
Felix Gimeno and
Andy Brock and
Oriol Vinyals and
Andrew Zisserman and
Jo{\~{a}}o Carreira},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/JaegleGBVZC21.bib},
 booktitle = {Proceedings of the 38th International Conference on Machine Learning,
{ICML} 2021, 18-24 July 2021, Virtual Event},
 editor = {Marina Meila and
Tong Zhang},
 pages = {4651--4664},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 25 Aug 2021 01:00:00 +0200},
 title = {Perceiver: General Perception with Iterative Attention},
 url = {http://proceedings.mlr.press/v139/jaegle21a.html},
 volume = {139},
 year = {2021}
}

@article{Yang2019PipeMare:Training,
 author = {Yang, Bowen and Zhang, Jian and Li, Jonathan and R{\'{e}}, Christopher and Aberger, Christopher R. and De Sa, Christopher},
 journal = {ArXiv preprint},
 title = {{PipeMare: Asynchronous Pipeline Parallel DNN Training}},
 url = {https://arxiv.org/abs/1910.05124},
 volume = {abs/1910.05124},
 year = {2019}
}

@inproceedings{KlicperaPREDICTPAGERANK,
 author = {Johannes Klicpera and
Aleksandar Bojchevski and
Stephan G{\"{u}}nnemann},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KlicperaBG19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Predict then Propagate: Graph Neural Networks meet Personalized PageRank},
 url = {https://openreview.net/forum?id=H1gL-2A9Ym},
 year = {2019}
}

@inproceedings{LisaLiPrefix-Tuning:Generation,
 address = {Online},
 author = {Li, Xiang Lisa  and
Liang, Percy},
 booktitle = {Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
 doi = {10.18653/v1/2021.acl-long.353},
 pages = {4582--4597},
 publisher = {Association for Computational Linguistics},
 title = {Prefix-Tuning: Optimizing Continuous Prompts for Generation},
 url = {https://aclanthology.org/2021.acl-long.353},
 year = {2021}
}

@inproceedings{Lowe2019PuttingRepresentations,
 author = {Sindy L{\"{o}}we and
Peter O'Connor and
Bastiaan S. Veeling},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LoweOV19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {3033--3045},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Putting An End to End-to-End: Gradient-Isolated Learning of Representations},
 url = {https://proceedings.neurips.cc/paper/2019/hash/851300ee84c2b80ed40f51ed26d866fc-Abstract.html},
 year = {2019}
}

@inproceedings{Peng2021RandomAttention,
 author = {Hao Peng and
Nikolaos Pappas and
Dani Yogatama and
Roy Schwartz and
Noah A. Smith and
Lingpeng Kong},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/Peng0Y0SK21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Random Feature Attention},
 url = {https://openreview.net/forum?id=QtTKTdVrFBB},
 year = {2021}
}

@inproceedings{WangREVISITINGTRAINING,
 author = {Yulin Wang and
Zanlin Ni and
Shiji Song and
Le Yang and
Gao Huang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/WangNSYH21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Revisiting Locally Supervised Learning: an Alternative to End-to-end
Training},
 url = {https://openreview.net/forum?id=fAbkE6ant2},
 year = {2021}
}

@inproceedings{Lee2019Self-AttentionPooling,
 author = {Junhyun Lee and
Inyeop Lee and
Jaewoo Kang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/LeeLK19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {3734--3743},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Self-Attention Graph Pooling},
 url = {http://proceedings.mlr.press/v97/lee19c.html},
 volume = {97},
 year = {2019}
}

@inproceedings{Press2020Shortformer:Inputs,
 address = {Online},
 author = {Press, Ofir  and
Smith, Noah A.  and
Lewis, Mike},
 booktitle = {Proceedings of the 59th Annual Meeting of the Association for Computational Linguistics and the 11th International Joint Conference on Natural Language Processing (Volume 1: Long Papers)},
 doi = {10.18653/v1/2021.acl-long.427},
 pages = {5493--5505},
 publisher = {Association for Computational Linguistics},
 title = {Shortformer: Better Language Modeling using Shorter Inputs},
 url = {https://aclanthology.org/2021.acl-long.427},
 year = {2021}
}

@techreport{LiuTheSurvey,
 arxivid = {2002.03794v4},
 author = {Liu, Yi and Liu, Xiaoyan and Sun, Qingxiao and You, Xin and Yang, Hailong and Luan, Zhongzhi and Gan, Lin and Yang, Guangwen and Qian, Depei},
 keywords = {Additional Key Words and Phrases: Neural Networks, Compiler, Deep Learning, Intermediate Representation, Optimization},
 title = {{The Deep Learning Compiler: A Comprehensive Survey}},
 url = {https://github.com/buaa-hipo/dlcompiler-comparison}
}

@techreport{GaoTheModeling,
 arxivid = {2101.00027v1},
 author = {Gao, Leo and Biderman, Stella and Black, Sid and Golding, Laurence and Hoppe, Travis and Foster, Charles and Phang, Jason and He, Horace and Thite, Anish and Nabeshima, Noa and Presser, Shawn and Leahy Eleutherai, Connor},
 title = {{The Pile: An 800GB Dataset of Diverse Text for Language Modeling}},
 url = {https://pile.eleuther.ai/}
}

@techreport{Soro2020TinyMLAI,
 author = {Soro, Stanislava},
 title = {{TinyML for Ubiquitous Edge AI}},
 year = {2020}
}

@techreport{BaghdadiTIRAMISU:Code,
 arxivid = {1804.10694v5},
 author = {Baghdadi, Riyadh and Ray, Jessica and Romdhane, Malek Ben and Sozzo, Emanuele Del and Akkas, Abdurrahman and Zhang, Yunming and Google, Patricia Suriana and Adobe, Shoaib Kamil and Amarasinghe, Saman},
 keywords = {Code Generation, Deep Learning, Distributed Systems, GPUs, Index Terms-Code Optimization, Polyhe-dral Model, Tensors},
 title = {{TIRAMISU: A Polyhedral Compiler for Expressing Fast and Portable Code}},
 url = {http://tiramisu-compiler.org/}
}

@inproceedings{NklandTrainingSignals,
 author = {Arild N{\o}kland and
Lars Hiller Eidnes},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/NoklandE19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {4839--4850},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Training Neural Networks with Local Error Signals},
 url = {http://proceedings.mlr.press/v97/nokland19a.html},
 volume = {97},
 year = {2019}
}

@inproceedings{CzarneckiUnderstandingInterfaces,
 author = {Wojciech Marian Czarnecki and
Grzegorz Swirszcz and
Max Jaderberg and
Simon Osindero and
Oriol Vinyals and
Koray Kavukcuoglu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/CzarneckiSJOVK17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {904--912},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Understanding Synthetic Gradients and Decoupled Neural Interfaces},
 url = {http://proceedings.mlr.press/v70/czarnecki17a.html},
 volume = {70},
 year = {2017}
}

@inproceedings{LuoUnderstandingNetworks,
 author = {Wenjie Luo and
Yujia Li and
Raquel Urtasun and
Richard S. Zemel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LuoLUZ16.bib},
 booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
on Neural Information Processing Systems 2016, December 5-10, 2016,
Barcelona, Spain},
 editor = {Daniel D. Lee and
Masashi Sugiyama and
Ulrike von Luxburg and
Isabelle Guyon and
Roman Garnett},
 pages = {4898--4906},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Understanding the Effective Receptive Field in Deep Convolutional
Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2016/hash/c8067ad1937f728f51288b3eb986afaa-Abstract.html},
 year = {2016}
}

@article{Wu2020VisualVision,
 author = {Wu, Bichen and Xu, Chenfeng and Dai, Xiaoliang and Wan, Alvin and Zhang, Peizhao and Yan, Zhicheng and Tomizuka, Masayoshi and Gonzalez, Joseph and Keutzer, Kurt and Vajda, Peter},
 journal = {ArXiv preprint},
 title = {{Visual Transformers: Token-based Image Representation and Processing for Computer Vision}},
 url = {https://arxiv.org/abs/2006.03677},
 volume = {abs/2006.03677},
 year = {2020}
}

@article{a._de_palma_traffic_2011,
 author = {{A. de Palma} and Lindsey, R.},
 journal = {Transportation Research Part C},
 pages = {1377--1399},
 title = {Traffic Congestion Pricing Methodologies and Technologies},
 volume = {19},
 year = {2011}
}

@book{aashto_highway_2012,
 author = {{AASHTO}},
 title = {Highway {{Safety Manual}}},
 year = {2012}
}

@misc{abadi_tensorflow_2015,
 abstract = {TensorFlow is a machine learning system that operates at large scale and in heterogeneous environments. TensorFlow uses dataflow graphs to represent computation, shared state, and the operations that mutate that state. It maps the nodes of a dataflow graph across many machines in a cluster, and within a machine across multiple computational devices, including multicore CPUs, generalpurpose GPUs, and custom-designed ASICs known as Tensor Processing Units (TPUs). This architecture gives flexibility to the application developer: whereas in previous ``parameter server'' designs the management of shared state is built into the system, TensorFlow enables developers to experiment with novel optimizations and training algorithms. TensorFlow supports a variety of applications, with a focus on training and inference on deep neural networks. Several Google services use TensorFlow in production, we have released it as an open-source project, and it has become widely used for machine learning research. In this paper, we describe the TensorFlow dataflow model and demonstrate the compelling performance that TensorFlow achieves for several real-world applications.},
 author = {Abadi, Mart{\i}n and Barham, Paul and Chen, Jianmin and Chen, Zhifeng and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Irving, Geoffrey and Isard, Michael and Kudlur, Manjunath and Levenberg, Josh and Monga, Rajat and Moore, Sherry and Murray, Derek G and Steiner, Benoit and Tucker, Paul and Vasudevan, Vijay and Warden, Pete and Wicke, Martin and Yu, Yuan and Zheng, Xiaoqiang},
 file = {/home/matt/Zotero/storage/WI2G5GSP/Abadi et al. - TensorFlow A system for large-scale machine learn.pdf},
 howpublished = {https://tensorflow.org},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {{{TensorFlow}}: {{Large}}-{{Scale Machine Learning}} on {{Heterogeneous Systems}}},
 year = {2015}
}

@article{abbas_real-time_2001,
 author = {Abbas, M. and Bullock, D. and Head, L.},
 journal = {Transportation Research Record},
 pages = {26--39},
 title = {Real-Time Offset Transitioning Algorithm for Coordinatinng Traffic Signals},
 volume = {1748},
 year = {2001}
}

@article{abdulhai_reinforcement_2003,
 abstract = {The ability to exert real-time, adaptive control of transportation processes is the core of many intelligent transportation systems decision support tools. Reinforcement learning, an artificial intelligence approach undergoing development in the machinelearning community, offers key advantages in this regard. The ability of a control agent to learn relationships between control actions and their effect on the environment while pursuing a goal is a distinct improvement over prespecified models of the environment. Prespecified models are a prerequisite of conventional control methods and their accuracy limits the performance of control agents. This paper contains an introduction to Q-learning, a simple yet powerful reinforcement learning algorithm, and presents a case study involving application to traffic signal control. Encouraging results of the application to an isolated traffic signal, particularly under variable traffic conditions, are presented. A broader research effort is outlined, including extension to linear and networked signal systems and integration with dynamic route guidance. The research objective involves optimal control of heavily congested traffic across a two-dimensional road network\textemdash a challenging task for conventional traffic signal control methodologies.},
 author = {Abdulhai, Baher and Pringle, Rob and Karakoulas, Grigoris J.},
 doi = {10.1061/(ASCE)0733-947X(2003)129:3(278)},
 file = {/home/matt/Zotero/storage/NRIKVGQF/Abdulhai et al. - 2003 - Reinforcement Learning for iTruei Adaptive Tr.pdf},
 issn = {0733-947X, 1943-5436},
 journal = {Journal of Transportation Engineering},
 language = {en},
 number = {3},
 pages = {278--285},
 title = {Reinforcement {{Learning}} for {{{\emph{True}}}} {{Adaptive Traffic Signal Control}}},
 volume = {129},
 year = {2003}
}

@article{abernethy_new_2009,
 abstract = {We present a general approach for collaborative filtering (CF) using spectral regularization to learn linear operators mapping a set of ``users'' to a set of possibly desired ``objects''. In particular, several recent low-rank type matrix-completion methods for CF are shown to be special cases of our proposed framework. Unlike existing regularization-based CF, our approach can be used to incorporate additional information such as attributes of the users/objects\textemdash a feature currently lacking in existing regularization-based CF approaches\textemdash using popular and well-known kernel methods. We provide novel representer theorems that we use to develop new estimation methods. We then provide learning algorithms based on low-rank decompositions and test them on a standard CF data set. The experiments indicate the advantages of generalizing the existing regularization-based CF methods to incorporate related information about users and objects. Finally, we show that certain multi-task learning methods can be also seen as special cases of our proposed approach.},
 author = {Abernethy, Jacob and Bach, Francis and Evgeniou, Theodoros and Vert, Jean-Philippe},
 file = {/home/matt/Zotero/storage/6JQ7SC5Y/Abernethy et al. - A New Approach to Collaborative Filtering Operato.pdf},
 journal = {Journal of Machine Learning Research},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {803--826},
 title = {A {{New Approach}} to {{Collaborative Filtering}}: {{Operator Estimation}} with {{Spectral Regularization}}},
 volume = {10},
 year = {2009}
}

@article{abou-zeid_mass_2013,
 abstract = {This paper presents a review of the literature on mass effects and their importance in choice behavior, i.e. how individual behavior is influenced by the behavior of others, with the goal of extracting lessons for transportation policy. An overview of psychological theories explaining the process underlying mass effects and conformity behavior is given. This is followed by a presentation of evidence of mass effects on choice behavior both outside and within transportation planning, covering contexts ranging from long term choices such as residential location to short term decisions such as driving behavior. Based on this review, modeling approaches for studying mass effects and their data requirements are then synthesized, highlighting the advantages and limitations of each. The paper concludes with a discussion of the importance of leveraging the power of mass effects for designing transportation policies aimed at promoting sustainable and safe mobility, and of challenges for future work in this area.},
 author = {{Abou-Zeid}, M. and Schm{\"o}cker, J.-D. and Belgiawan, P. F. and Fujii, S.},
 doi = {10.1179/1942786713Z.00000000011},
 file = {/home/matt/Zotero/storage/BZKJUPQN/Abou-Zeid et al. - 2013 - Mass effects and mobility decisions.pdf;/home/matt/Zotero/storage/XG7AY7VH/1942786713Z.html},
 issn = {1942-7867},
 journal = {Transportation Letters},
 number = {3},
 pages = {115--130},
 title = {Mass Effects and Mobility Decisions},
 volume = {5},
 year = {2013}
}

@article{aboudolas_perimeter_2013,
 author = {Aboudolas, K. and Geroliminis, N.},
 journal = {Transportation Research, Part B},
 pages = {265--281},
 title = {Perimeter and Boundary Flow Control in Multi-Reservoir Heterogeneous Networks},
 volume = {55},
 year = {2013}
}

@article{aboudolas_rolling-horizon_2009,
 author = {Aboudolas, K. and Papageorgiou, M. and Kouvelas, A. and Kosmatopoulos, E.},
 journal = {Transportation Research, Part C},
 pages = {680--694},
 title = {A Rolling-Horizon Quadratic-Programming Approach to the Signal Control Problem in Large-Scale Congested Urban Road Networks},
 volume = {17},
 year = {2009}
}

@article{aboudolas_store-and-forward_2009,
 author = {Aboudolas, K. and Papageorgiou, M. and Kosmatopoulos, E.},
 journal = {Transportation Research, Part C},
 pages = {163--174},
 title = {Store-and-Forward Based Methods for the Signal Control Problem in Large-Scale Congested Urban Road Networks},
 volume = {17},
 year = {2009}
}

@article{abramovich_positive_1992,
 abstract = {A Krein operator is a positive operator, acting on a partially ordered Banach space, that carries positive elements to strong units. The purpose of this paper is to present a survey of the remarkable spectral properties (most of which were established by M.G. Krein) of these operators. The proofs presented here seem to be simpler than the ones existing in the literature. Some new results are also obtained. For instance, it is shown that every positive operator on a Krein space which is not a multiple of the identity operator has a nontrivial hyperinvariant subspace.},
 author = {Abramovich, Y. A. and Aliprantis, C. D. and Burkinshaw, O.},
 doi = {10.1007/BF00046631},
 file = {/home/matt/Zotero/storage/HZDSH9L4/Abramovich et al. - 1992 - Positive operators on Krein spaces.pdf},
 issn = {1572-9036},
 journal = {Acta Applicandae Mathematica},
 language = {en},
 number = {1},
 pages = {1--22},
 title = {Positive Operators on {{Krein}} Spaces},
 volume = {27},
 year = {1992}
}

@article{achiam_towards_2019,
 author = {Achiam, Joshua and Knight, Ethan and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {Towards {{Characterizing Divergence}} in {{Deep Q}}-{{Learning}}},
 url = {https://arxiv.org/abs/1903.08894},
 volume = {abs/1903.08894},
 year = {2019}
}

@book{adamatzky_cellular_2018,
 address = {{New York, NY}},
 doi = {10.1007/978-1-4939-8700-9},
 editor = {Adamatzky, Andrew},
 isbn = {978-1-4939-8699-6 978-1-4939-8700-9},
 language = {en},
 publisher = {{Springer US}},
 shorttitle = {Cellular {{Automata}}},
 title = {Cellular {{Automata}}: {{A Volume}} in the {{Encyclopedia}} of {{Complexity}} and {{Systems Science}}, {{Second Edition}}},
 year = {2018}
}

@article{adams_learning_2019,
 author = {Adams, Andrew and Durand, Fr{\'e}do and {Ragan-Kelley}, Jonathan and Ma, Karima and Anderson, Luke and Baghdadi, Riyadh and Li, Tzu-Mao and Gharbi, Micha{\"e}l and Steiner, Benoit and Johnson, Steven and Fatahalian, Kayvon},
 doi = {10.1145/3306346.3322967},
 file = {/home/matt/Zotero/storage/WYZURKYP/Adams et al. - 2019 - Learning to optimize halide with tree search and r.pdf},
 issn = {07300301},
 journal = {ACM Transactions on Graphics},
 language = {en},
 number = {4},
 pages = {121:1-121:12},
 title = {Learning to Optimize Halide with Tree Search and Random Programs},
 volume = {38},
 year = {2019}
}

@book{adeli_intelligent_2008,
 abstract = {Recent estimates hypothesize that the US will need \$1.6 trillion dollars for the rehabilitation, replacement, and maintenance of existing infrastructure systems},
 author = {Adeli, Hojjat and Jiang, Xiaomo},
 doi = {10.1201/9781482281767},
 file = {/home/matt/Zotero/storage/V3M2VFR4/9780429182778.html},
 isbn = {978-0-429-18277-8},
 language = {en},
 publisher = {{CRC Press}},
 shorttitle = {Intelligent {{Infrastructure}}},
 title = {Intelligent {{Infrastructure}}: {{Neural Networks}}, {{Wavelets}}, and {{Chaos Theory}} for {{Intelligent Transportation Systems}} and {{Smart Structures}}},
 year = {2008}
}

@techreport{administration_wim_1998,
 author = {Administration, Federal Highway},
 number = {FHWA-RD-98-104},
 title = {{{WIM Scale Calibration}}: {{A Vital Activity}} for {{LTPP Sites}}},
 year = {1998}
}

@book{aguigjui_detector_2010,
 author = {Aguigjui, K. and Sowers, B.},
 title = {Detector {{Technology}}},
 year = {2010}
}

@article{ahmad_automatically_2019,
 author = {Ahmad, Maaz Bin Safeer and {Ragan-Kelley}, Jonathan and Cheung, Alvin and Kamil, Shoaib},
 doi = {10.1145/3355089.3356549},
 file = {/home/matt/Zotero/storage/9LRITWFH/Ahmad et al. - 2019 - Automatically translating image processing librari.pdf},
 issn = {0730-0301, 1557-7368},
 journal = {ACM Transactions on Graphics (TOG)},
 language = {en},
 number = {6},
 pages = {1--13},
 title = {Automatically Translating Image Processing Libraries to Halide},
 volume = {38},
 year = {2019}
}

@phdthesis{akametalu_learning-based_2018,
 abstract = {Robotic systems are becoming more pervasive, and have the potential to significantly improve human lives. However, for these benefits to be realized it is critical that the safe operation of these systems be guaranteed. Reachability analysis has proven to be an effective tool for providing safety certificates for dynamical systems, given a model of the system. A major challenge in assuring safety, is that systems often have uncertainty due to the hard-to-model complex physical interactions, or lack of knowledge of the behavior of external agents, on which safety may depend.This thesis uses Hamilton-Jacobi (HJ) reachability analysis to robustly guarantee safety for systems with uncertainty. In the presence of uncertainty there must be a balance between conservativeness as it pertains to safety and performance as it pertains to other system objectives, and we also account for this through reachability analysis. In addition, this thesis also explores methods for modifying the analysis as more data is collected from the robotics system, which ultimately allows for improved performance. This is referred to here as learning-based reachability analysis. The thesis concludes with a new HJ reachability formulation that enhances the learning-based analysis. The myriad of ideas presented throughout the thesis are demonstrated on various examples.},
 author = {Akametalu, Anayo Kenechukwu},
 file = {/home/matt/Zotero/storage/RDRMAXSP/Akametalu - 2018 - A Learning-Based Approach to Safety for Uncertain .pdf;/home/matt/Zotero/storage/R43X2HGW/7319h9gd.html},
 language = {en},
 school = {UC Berkeley},
 title = {A {{Learning}}-{{Based Approach}} to {{Safety}} for {{Uncertain Robotic Systems}}},
 year = {2018}
}

@inproceedings{alabdulmohsin_support_2015,
 abstract = {Training support vector machines (SVM) with indefinite kernels has recently attracted attention in the machine learning community. This is partly due to the fact that many similarity functions that arise in practice are not symmetric positive semidefinite, i.e. the Mercer condition is not satisfied, or the Mercer condition is difficult to verify. Previous work on training SVM with indefinite kernels has generally fallen into three categories: (1) positive semidefinite kernel approximation, (2) non-convex optimization, and (3) learning in Krein spaces. All approaches are not fully satisfactory. They have either introduced sources of inconsistency in handling training and test examples using kernel approximation, settled for approximate local minimum solutions using non-convex optimization, or produced nonsparse solutions. In this paper, we establish both theoretically and experimentally that the 1-norm SVM, proposed more than 10 years ago for embedded feature selection, is a better solution for extending SVM to indefinite kernels. More specifically, 1-norm SVM can be interpreted as a structural risk minimization method that seeks a decision boundary with large similarity margin in the original space. It uses a linear programming formulation that remains convex even if the kernel matrix is indefinite, and hence can always be solved quite efficiently. Also, it uses the indefinite similarity function (or distance) directly without any transformation, and, hence, it always treats both training and test examples consistently. Finally, it achieves the highest accuracy among all methods that train SVM with indefinite kernels with a statistically significant evidence while also retaining sparsity of the support vector set.},
 author = {Alabdulmohsin, Ibrahim and Gao, Xin and Zhang, Xiangliang},
 booktitle = {Proceedings of the {{Sixth Asian Conference}} on {{Machine Learning}}},
 file = {/home/matt/Zotero/storage/X2L38RHE/Alabdulmohsin et al. - Support vector machines with indeﬁnite kernels.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {32--47},
 publisher = {{PMLR}},
 title = {Support Vector Machines with Indefinite Kernels},
 volume = {39},
 year = {2015}
}

@inproceedings{alemi_fixing_2018,
 author = {Alexander A. Alemi and
Ben Poole and
Ian Fischer and
Joshua V. Dillon and
Rif A. Saurous and
Kevin Murphy},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/AlemiPFDS018.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {159--168},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Fixing a Broken {ELBO}},
 url = {http://proceedings.mlr.press/v80/alemi18a.html},
 volume = {80},
 year = {2018}
}

@article{alemi_uncertainty_2018,
 author = {Alemi, Alexander A. and Fischer, Ian and Dillon, Joshua V.},
 journal = {ArXiv preprint},
 title = {Uncertainty in the {{Variational Information Bottleneck}}},
 url = {https://arxiv.org/abs/1807.00906},
 volume = {abs/1807.00906},
 year = {2018}
}

@inproceedings{alhasoun_streetify_2019,
 author = {Fahad Alhasoun and
Marta C. Gonz{\'{a}}lez},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/bigdataconf/AlhasounG19.bib},
 booktitle = {2019 {IEEE} International Conference on Big Data (Big Data), Los Angeles,
CA, USA, December 9-12, 2019},
 doi = {10.1109/BigData47090.2019.9006384},
 pages = {2001--2006},
 publisher = {{IEEE}},
 timestamp = {Fri, 06 Mar 2020 00:00:00 +0100},
 title = {Streetify: Using Street View Imagery And Deep Learning For Urban Streets
Development},
 url = {https://doi.org/10.1109/BigData47090.2019.9006384},
 year = {2019}
}

@inproceedings{alhasoun_urban_2019,
 abstract = {The classification of streets on road networks has been focused on the vehicular transportational features of streets. Examples of street labels include arterials, major roads, minor roads and so forth based on their transportational use. City authorities on the other hand have been shifting to more wholistic planning of streets. The modern approach towards designing and planning streets is more inclusive of the street context, meaning the side use of a street combined with the transportational features of a street. Several city authorities are developing new classification schemes for street context that extends traditional classification methods to include the use of land on the sides of a street. In those classification schemes, streets are labeled for example as commercial throughway, residential neighborhood, park etc. This modern approach to urban planning have been adopted by major cities such as the city of San Francisco, the states of Florida and Pennsylvania among many others. Currently, the process of labeling streets according to their contexts is manual and hence is tedious and time consuming. It will require manual labor to regularly relabel streets as the city develops. In this paper, we propose an approach to collect and label imagery data then deploy advancements in computer vision towards modern urban planning. We propose a framework for automatic classification of street contexts. After collecting and labeling street imagery, we train deep convolutional neural networks (CNN) to perform the classification of street context. We show that CNN models can perform well achieving accuracies in the 81\% to 87\% range. We test various CNN architectures and report on their performances. We then visualize samples from the embedding space of streets using the t-SNE method. We also apply class activation mapping methods to interpret the features in street imagery contributing to output classification from a model.},
 address = {{Boca Raton, FL, USA}},
 author = {Alhasoun, Fahad and Gonzalez, Marta},
 booktitle = {2019 18th {{IEEE International Conference On Machine Learning And Applications}} ({{ICMLA}})},
 doi = {10.1109/ICMLA.2019.00198},
 file = {/home/matt/Zotero/storage/N9BIBN63/Alhasoun and Gonzalez - 2019 - Urban Street Contexts Classification Using Convolu.pdf},
 isbn = {978-1-72814-550-1},
 language = {en},
 pages = {1198--1204},
 publisher = {{IEEE}},
 title = {Urban {{Street Contexts Classification Using Convolutional Neural Networks}} and {{Streets Imagery}}},
 year = {2019}
}

@article{ali_discrimination_2019,
 author = {Ali, Muhammad and Sapiezynski, Piotr and Bogen, Miranda and Korolova, Aleksandra and Mislove, Alan and Rieke, Aaron},
 journal = {ArXiv preprint},
 title = {Discrimination through Optimization: {{How Facebook}}'s Ad Delivery Can Lead to Skewed Outcomes},
 url = {https://arxiv.org/abs/1904.02095},
 volume = {abs/1904.02095},
 year = {2019}
}

@inproceedings{alistarh_qsgd_2017,
 author = {Dan Alistarh and
Demjan Grubic and
Jerry Li and
Ryota Tomioka and
Milan Vojnovic},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/AlistarhG0TV17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {1709--1720},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {{QSGD:} Communication-Efficient {SGD} via Gradient Quantization and
Encoding},
 url = {https://proceedings.neurips.cc/paper/2017/hash/6c340f25839e6acdc73414517203f5f0-Abstract.html},
 year = {2017}
}

@inproceedings{allen_analogies_2019,
 author = {Carl Allen and
Timothy M. Hospedales},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/AllenH19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {223--231},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Analogies Explained: Towards Understanding Word Embeddings},
 url = {http://proceedings.mlr.press/v97/allen19a.html},
 volume = {97},
 year = {2019}
}

@article{allsop_estimating_1972,
 abstract = {reserve capacity},
 author = {Allsop, R. E.},
 journal = {Transportation Research},
 pages = {245--255},
 title = {Estimating the Traffic Capacity of a Signalized Road Junction},
 volume = {6},
 year = {1972}
}

@inproceedings{allstrom_evaluation_2012,
 abstract = {Real-time estimations of current and future traffic states are an essential part of traffic management and traffic information systems. Within the Mobile Millennium project considerable effort has been invested in the research and development of a real-time estimation system that can fuse several sources of data collected in California. During the past year this system has been adapted to also handle traffic data collected in Stockholm. This paper provides an overview of the model used for highways and presents results from an initial evaluation of the system. As part of the evaluation process, GPS data collected in an earlier field-test and estimations generated by the existing system used by the TMC in Stockholm, are compared with the estimations generated by the Mobile Millennium system. Given that the Mobile Millennium Stockholm system has not undergone any calibration, the results from the evaluation are considered promising. The estimated travel times correspond well to those measured in the field test. Furthermore, the estimations generated by the Mobile Millennium system can be regarded as superior to those of existing traffic management system in Stockholm. The highway model was found to perform well even with a reduction in the number of sensors providing data. The findings of this study indicate the robustness of the Mobile Millennium system and demonstrate how the system can be migrated to other geographical areas with similar sources of available data.},
 author = {Allstr{\"o}m, A. and Gundleg{\aa}rd, D. and Rydergren, C.},
 booktitle = {2012 15th {{International IEEE Conference}} on {{Intelligent Transportation Systems}}},
 doi = {10.1109/ITSC.2012.6338823},
 file = {/home/matt/Zotero/storage/HS988HEA/Allström et al. - 2012 - Evaluation of travel time estimation based on LWR-.pdf;/home/matt/Zotero/storage/Z8FAFJAM/6338823.html},
 pages = {1644--1649},
 shorttitle = {Evaluation of Travel Time Estimation Based on {{LWR}}-v and {{CTM}}-v},
 title = {Evaluation of Travel Time Estimation Based on {{LWR}}-v and {{CTM}}-v: {{A}} Case Study in {{Stockholm}}},
 year = {2012}
}

@article{almasri_online_2005,
 author = {Almasri, E. and Friedrich, B.},
 journal = {ITS Hanover},
 title = {Online Offset Optimization in Urban Networks Based on Cell Transmission Model.},
 year = {2005}
}

@inproceedings{alon_bottleneck_2021,
 author = {Uri Alon and
Eran Yahav},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/0002Y21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {On the Bottleneck of Graph Neural Networks and its Practical Implications},
 url = {https://openreview.net/forum?id=i80OPhOCVH2},
 year = {2021}
}

@article{alpay_remarks_1991,
 abstract = {The one-to-one correspondence between positive functions and reproducing kernel Hilbert spaces was extended by L. Schwartz to a (onto, but not one-to-one) correspondence between difference of positive functions and reproducing kernel Krein spaces. After discussing this result, we prove that a matrix valued function K(z,lj) symmetric and jointly analytic in z and \=u) in a neighborhood of the origin is the reproducing kernel of a reproducing kernel Krein space. We conclude with an example showing that such a function can be the reproducing kernel of two different Krein spaces.},
 author = {Alpay, Daniel},
 doi = {10.1216/rmjm/1181072903},
 file = {/home/matt/Zotero/storage/GWHFJY3R/Alpay - 1991 - Some Remarks on Reproducing Kernel Krein Spaces.pdf},
 issn = {0035-7596},
 journal = {Rocky Mountain Journal of Mathematics},
 language = {en},
 number = {4},
 pages = {1189--1205},
 title = {Some {{Remarks}} on {{Reproducing Kernel Krein Spaces}}},
 volume = {21},
 year = {1991}
}

@article{alvarez_kernels_2012,
 author = {{\'A}lvarez, Mauricio A. and Rosasco, Lorenzo and Lawrence, Neil D.},
 doi = {10.1561/2200000036},
 file = {/home/matt/Zotero/storage/GEUR5TR2/Álvarez et al. - 2012 - Kernels for Vector-Valued Functions A Review.pdf},
 issn = {1935-8237, 1935-8245},
 journal = {Foundations and Trends\textregistered{} in Machine Learning},
 language = {en},
 number = {3},
 pages = {195--266},
 shorttitle = {Kernels for {{Vector}}-{{Valued Functions}}},
 title = {Kernels for {{Vector}}-{{Valued Functions}}: {{A Review}}},
 volume = {4},
 year = {2012}
}

@article{alvarez_safe_199,
 author = {Alvarez, L. and Horowitz, R.},
 journal = {Vehicle System Dynamics Special Issue: IVHS},
 number = {1},
 pages = {23--56},
 title = {Safe {{Platooning}} in {{Automated Highway Systems}}. {{Part I}}: {{Safety Regions Design}}},
 volume = {32},
 year = {199}
}

@article{alvarez_safe_199-1,
 author = {Alvarez, L. and Horowitz, R.},
 journal = {Vehicle System Dynamics Special Issue: IVHS},
 number = {1},
 pages = {57--84},
 title = {Safe {{Platooning}} in {{Automated Highway Systems}}. {{Part II}}: {{Velocity Tracking Controller}}},
 volume = {32},
 year = {199}
}

@article{alvarez_safe_1999,
 author = {Alvarez, Luis and Horowitz, Roberto},
 file = {/home/matt/Zotero/storage/57ZIBQ4R/Alvarex_VSD_1999_safe_platooning_Part_I.pdf},
 journal = {Vehicle System Dynamics},
 number = {1},
 pages = {23--55},
 shorttitle = {Safe Platooning in Automated Highway Systems Part {{I}}},
 title = {Safe Platooning in Automated Highway Systems Part {{I}}: {{Safety}} Regions Design},
 volume = {32},
 year = {1999}
}

@incollection{amato_pragmatic-pedagogic_2020,
 address = {{Cham}},
 author = {Fisac, Jaime F. and Gates, Monica A. and Hamrick, Jessica B. and Liu, Chang and {Hadfield-Menell}, Dylan and Palaniappan, Malayandi and Malik, Dhruv and Sastry, S. Shankar and Griffiths, Thomas L. and Dragan, Anca D.},
 booktitle = {Robotics {{Research}}},
 doi = {10.1007/978-3-030-28619-4_7},
 editor = {Amato, Nancy M. and Hager, Greg and Thomas, Shawna and {Torres-Torriti}, Miguel},
 file = {/home/matt/Zotero/storage/HK7TVK7R/Fisac et al. - 2020 - Pragmatic-Pedagogic Value Alignment.pdf},
 isbn = {978-3-030-28618-7 978-3-030-28619-4},
 language = {en},
 pages = {49--57},
 publisher = {{Springer International Publishing}},
 title = {Pragmatic-{{Pedagogic Value Alignment}}},
 volume = {10},
 year = {2020}
}

@phdthesis{amin_cyber_2011,
 abstract = {The instrumentation of infrastructure systems by embedded sensors, computation, and communication networks has enabled significant advances in their management. Examples include monitoring of structural health, traffic congestion, environmental hazards, and energy usage. The use of homogeneous (especially, commercially available off-the-shelf) information technology (IT) solutions makes infrastructure systems subject to correlated hardware malfunctions and software bugs. Over the past decade, many concerns have been raised about the vulnerabilities of infrastructure systems to both random failures and security attacks. Cyber-security of Supervisory Control and Data Acquisition (SCADA) systems is especially important, because these systems are employed for sensing and control of large physical infrastructures. So far, the existing research in robust and fault-tolerant control does not account for cyber attacks on networked control system (NCS) components. Also, the existing research in computer security neither considers the attacks targeting NCS components nor accounts for their interactions with the physical system. The goal of this thesis is to bridge this gap by focusing on (1) security threat assessment, (2) model-based attack diagnosis, and (3) resilient control design. First, cyber-security assessment for SCADA systems is performed based on well-defined attacker and defender objectives. The mathematical model of SCADA systems considered in this work has two control levels: regulatory control using distributed proportional-integral (PI) controllers, and supervisory fault diagnosis based on approximate dynamical system models. The performance of a PI control based regulatory scheme and a model-based supervisory diagnostic scheme is studied under a class of deception attacks. In order to test the system resilience, a class of stealthy attacks which can evade detection by SCADA systems is presented. Second, design of attack diagnosis schemes that incorporate the knowledge of physical dynamics of the system is presented. For SCADA systems used to manage water canal networks, an observer-based attack diagnostic scheme, in which each observer estimates the state of a reduced-order flow model, is presented. The observer parameters are computed using a convex optimization method, and the performance of this scheme is tested on a number of attack scenarios. An application of the theoretical results is illustrated by a field operational test performed on the SCADA system of the Gignac water canal system, located in Montpellier, France. A successful experimental cyber-attack on the sensors and actuators of this canal network revealed new vulnerabilities of the current SCADA system implementation. Another illustration includes security analysis of two benchmark scenarios: the Tennessee Eastman process control system (TE-PCS) and a power system state estimator (PSSE). In both these cases, model-based statistical detection schemes are used to study stealthy deception attacks. For the case of TE-PCS, design of practically implementable attack-detection and response mechanisms to maintain operational safety is presented. For the case of PSSE, it is assumed that the attacker only has a partial knowledge of the actual system model. For a set of attacker objectives, the trade-off between the attacker knowledge and possible impact of a successful attack on the performance of false data detection schemes is studied. Third, the stability of linear hyperbolic systems of PDEs when the boundary control actions and the system parameters switch discontinuously between a finite set of modes is studied. Switched PDE models can describe a class of fault and attack scenarios resulting from intermittent withdrawals through offtake nodes and compromise of sensor-control data. Motivated by such scenarios, a new condition for stability of linear hyperbolic systems of PDEs under arbitrary switching of boundary control actions and system parameters is derived. A class of switching attack strategies is presented, which violate the stability condition and result in unstable flow dynamics.Fourth, the problem of controlling stochastic linear systems for networked control settings is considered when the sensor-control data is prone to packet loss and jamming. For a class of packet drop models, feedback control policies which minimize a given objective function subject to safety constraints are synthesized. For marginally stable systems, under mild hypotheses on the noise introduced by the control channel and large enough control authority, the synthesis of a control policy that render the state of the closed-loop system mean-square bounded is presented.Finally, a class of games involving discrete interdependent risks is considered when each player is a NCS, and their security is interdependent due to the exposure to network induced risks. The problem of security decisions of individual players is formulated as a two-stage non-cooperative game defined as follows: in the first stage, the players decide whether to invest in security or not; and in the second stage, they apply control inputs to minimize the average operational costs. The characterization of the equilibria of the game is presented, which includes the determination of the individually optimal security levels. The presence of interdependent security causes a negative externality, and the individual players tend to under invest in security relative to the social optimum. From these results, for a wide parameter range, public policy incentivising higher security investments is desirable.},
 author = {Amin, Saurabh},
 file = {/home/matt/Zotero/storage/4RFK4ZCP/Amin - 2011 - On Cyber Security for Networked Control Systems.pdf;/home/matt/Zotero/storage/ZZDDHXJ5/0x42r322.html},
 language = {en},
 school = {UC Berkeley},
 title = {On {{Cyber Security}} for {{Networked Control Systems}}},
 year = {2011}
}

@article{ancha_active_2020,
 author = {Ancha, Siddharth and Raaj, Yaadhav and Hu, Peiyun and Narasimhan, Srinivasa G. and Held, David},
 journal = {ArXiv preprint},
 title = {Active {{Perception}} Using {{Light Curtains}} for {{Autonomous Driving}}},
 url = {https://arxiv.org/abs/2008.02191},
 volume = {abs/2008.02191},
 year = {2020}
}

@article{andrieu_particle_2010,
 author = {Andrieu, Christophe and Doucet, Arnaud and Holenstein, Roman},
 file = {/home/matt/Zotero/storage/K5ZAJJIH/j.1467-9868.2009.00736.x.pdf},
 journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
 number = {3},
 pages = {269--342},
 title = {Particle {{Markov Chain Monte Carlo}} Methods},
 volume = {72},
 year = {2010}
}

@inproceedings{anonymous_flag_2020,
 abstract = {Data augmentation helps neural networks generalize better, but it remains an open question how to effectively augment graph data to enhance the performance of GNNs (Graph Neural Networks). While...},
 author = {Anonymous},
 booktitle = {Submitted to {{International Conference}} on {{Learning Representations}}},
 file = {/home/matt/Zotero/storage/5IRZCID8/Anonymous - 2020 - FLAG Adversarial Data Augmentation for Graph Neur.pdf;/home/matt/Zotero/storage/LKYYRMB7/forum.html},
 language = {en},
 shorttitle = {{{FLAG}}},
 title = {{{FLAG}}: {{Adversarial Data Augmentation}} for {{Graph Neural Networks}}},
 year = {2020}
}

@inproceedings{anonymous_how_2020,
 author = {Dongkwan Kim and
Alice H. Oh},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KimO21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {How to Find Your Friendly Neighborhood: Graph Attention Design with
Self-Supervision},
 url = {https://openreview.net/forum?id=Wi5KUNlqWty},
 year = {2021}
}

@inproceedings{anonymous_structured_2019,
 author = {Jannik Kossen and
Karl Stelzner and
Marcel Hussing and
Claas Voelcker and
Kristian Kersting},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KossenSHVK20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Structured Object-Aware Physics Prediction for Video Modeling and
Planning},
 url = {https://openreview.net/forum?id=B1e-kxSKDH},
 year = {2020}
}

@inproceedings{anonymous_trans-caps_2020,
 abstract = {Capsule Networks (CapsNets) have shown to be a promising alternative to Convolutional Neural Networks (CNNs) in many computer vision tasks, due to their ability to encode object viewpoint...},
 author = {Anonymous},
 booktitle = {Submitted to {{International Conference}} on {{Learning Representations}}},
 file = {/home/matt/Zotero/storage/WSMY856X/Anonymous - 2020 - Trans-Caps Transformer Capsule Networks with Self.pdf;/home/matt/Zotero/storage/UX4QQL23/forum.html},
 language = {en},
 shorttitle = {Trans-{{Caps}}},
 title = {Trans-{{Caps}}: {{Transformer Capsule Networks}} with {{Self}}-Attention {{Routing}}},
 year = {2020}
}

@article{ardekani_macroscopic_2011,
 author = {Ardekani, Siamak A. and Ghandehari, Mostafa and Nepal, Shiva M.},
 file = {/home/matt/Zotero/storage/U4PF837W/MacroscopicSpeedFlowManagedLanes.pdf},
 journal = {Buletinul Institutului Politehnic din lasi. Sectia Constructii, Arhitectura},
 number = {1},
 pages = {149},
 title = {Macroscopic Speed-Flow Models for Characterization of Freeway and Managed Lanes},
 volume = {57},
 year = {2011}
}

@article{argyriou_when_2009,
 abstract = {We consider a general class of regularization methods which learn a vector of parameters on the basis of linear measurements. It is well known that if the regularizer is a nondecreasing function of the L2 norm, then the learned vector is a linear combination of the input data. This result, known as the representer theorem, lies at the basis of kernel-based methods in machine learning. In this paper, we prove the necessity of the above condition, in the case of differentiable regularizers. We further extend our analysis to regularization methods which learn a matrix, a problem which is motivated by the application to multi-task learning. In this context, we study a more general representer theorem, which holds for a larger class of regularizers. We provide a necessary and sufficient condition characterizing this class of matrix regularizers and we highlight some concrete examples of practical importance. Our analysis uses basic principles from matrix theory, especially the useful notion of matrix nondecreasing functions.},
 author = {Argyriou, Andreas and Micchelli, Charles A and Pontil, Massimiliano},
 file = {/home/matt/Zotero/storage/JM9IB5ZP/Argyriou et al. - When Is There a Representer Theorem Vector Versus.pdf},
 journal = {Journal of Machine Learning Research},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {2507--2529},
 title = {When {{Is There}} a {{Representer Theorem}}? {{Vector Versus Matrix Regularizers}}},
 volume = {10},
 year = {2009}
}

@article{arnott_integrated_2006,
 author = {Arnott, R. and Inci, E.},
 journal = {Journal of Urban Economics},
 pages = {418--442},
 title = {An Integrated Model of Downtown Parking and Traffic Congestion},
 volume = {60},
 year = {2006}
}

@article{arnott_properties_1993,
 author = {Arnott, R. and {\noopsort{palma}}de Palma, A. and Lindsey, R.},
 journal = {Transportation Science},
 number = {2},
 pages = {148--160},
 title = {Properties of {{Dynamic Traffic Equilibrium Involving Bottlenecks}}},
 volume = {27},
 year = {1993}
}

@article{arnott_structural_1993,
 author = {Arnott, R. and {\noopsort{palma}}de Palma, A. and Lindsey, R.},
 journal = {American Economic Review},
 number = {1},
 pages = {161--179},
 title = {A {{Structural Model}} of {{Peak}}-{{Period Congestion}}: {{A Traffic Bottleneck}} with {{Elastic Demand}}},
 volume = {83},
 year = {1993}
}

@article{aronszajn_theory_1950,
 author = {Aronszajn, N.},
 doi = {10.2307/1990404},
 file = {/home/matt/Zotero/storage/YY8BUYUU/Aronszajn - 1950 - Theory of Reproducing Kernels.pdf},
 issn = {0002-9947},
 journal = {Transactions of the American Mathematical Society},
 number = {3},
 pages = {337--404},
 publisher = {{American Mathematical Society}},
 title = {Theory of {{Reproducing Kernels}}},
 volume = {68},
 year = {1950}
}

@inproceedings{arora_dropout_2020,
 author = {Raman Arora and
Peter Bartlett and
Poorya Mianjy and
Nathan Srebro},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/AroraBMS21.bib},
 booktitle = {Proceedings of the 38th International Conference on Machine Learning,
{ICML} 2021, 18-24 July 2021, Virtual Event},
 editor = {Marina Meila and
Tong Zhang},
 pages = {351--361},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 25 Aug 2021 01:00:00 +0200},
 title = {Dropout: Explicit Forms and Capacity Control},
 url = {http://proceedings.mlr.press/v139/arora21a.html},
 volume = {139},
 year = {2021}
}

@article{arulampalam_tutorial_2002,
 author = {Arulampalam, M. S. and Maskell, S. and Gordon, N. and Clapp, T.},
 doi = {10.1109/78.978374},
 issn = {1053-587X},
 journal = {IEEE Transactions on Signal Processing},
 number = {2},
 pages = {174--188},
 title = {A Tutorial on Particle Filters for Online Nonlinear/Non-{{Gaussian Bayesian}} Tracking},
 volume = {50},
 year = {2002}
}

@article{ashok_estimation_2002,
 author = {Ashok, K. and {Ben-Akiva}, M. E.},
 journal = {Transportation Science},
 number = {2},
 pages = {184--198},
 title = {Estimation and Prediction of Time-Dependent Origin-Destination Flows with a Stochastic Mapping to Path Flows and Link Flows},
 volume = {36},
 year = {2002}
}

@inproceedings{askari_effect_2017,
 abstract = {The paper evaluates the influence of the maximum vehicle acceleration and variable proportions of ACC/CACC vehicles on the throughput of an intersection. Two cases are studied: (1) free road downstream of the intersection; and (2) red light at some distance downstream of the intersection. Simulation of a 4-mile stretch of an arterial with 13 signalized intersections is used to evaluate the impact of (C)ACC vehicles on the mean and standard deviation of travel time as the proportion of (C)ACC vehicles is increased. The results suggest a very high urban mobility benefit of (C)ACC vehicles at little or no cost in infrastructure.},
 author = {Askari, Armin and Farias, Daniel Albarnaz and Kurzhanskiy, Alex A. and Varaiya, Pravin},
 booktitle = {2017 {{IEEE Intelligent Vehicles Symposium}} ({{IV}})},
 doi = {10.1109/IVS.2017.7995889},
 file = {/home/matt/Zotero/storage/G69MZ6RK/Askari et al. - 2017 - Effect of adaptive and cooperative adaptive cruise.pdf;/home/matt/Zotero/storage/FYNBKZRZ/7995889.html},
 issn = {null},
 pages = {1287--1292},
 title = {Effect of Adaptive and Cooperative Adaptive Cruise Control on Throughput of Signalized Arterials},
 year = {2017}
}

@book{association_of_bay_area_governments_and_metropolitan_transportation_commission_draft_2013,
 author = {{Association of Bay Area Governments and Metropolitan Transportation Commission}},
 title = {Draft {{Plan Bay Area}}, {{Strategy}} for a {{Sustainable Region}}},
 year = {2013}
}

@inproceedings{athalye_obfuscated_2018,
 author = {Anish Athalye and
Nicholas Carlini and
David A. Wagner},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/AthalyeC018.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {274--283},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Obfuscated Gradients Give a False Sense of Security: Circumventing
Defenses to Adversarial Examples},
 url = {http://proceedings.mlr.press/v80/athalye18a.html},
 volume = {80},
 year = {2018}
}

@article{athey_beyond_2017,
 author = {Athey, Susan},
 doi = {10.1126/science.aal4321},
 file = {/home/matt/Zotero/storage/JXWTTUI3/Athey - 2017 - Beyond prediction Using big data for policy probl.pdf},
 issn = {0036-8075, 1095-9203},
 journal = {Science},
 language = {en},
 number = {6324},
 pages = {483--485},
 shorttitle = {Beyond Prediction},
 title = {Beyond Prediction: {{Using}} Big Data for Policy Problems},
 volume = {355},
 year = {2017}
}

@article{attali_approximations_1997,
 author = {Attali, Jean-Gabriel and Pag{\`e}s, Gilles},
 doi = {10.1016/S0893-6080(97)00010-5},
 file = {/home/matt/Zotero/storage/VEGEBIYH/PAGi - Approximations of Functions by a Multilayer Percep.pdf},
 issn = {08936080},
 journal = {Neural Networks},
 language = {en},
 number = {6},
 pages = {1069--1081},
 shorttitle = {Approximations of {{Functions}} by a {{Multilayer Perceptron}}},
 title = {Approximations of {{Functions}} by a {{Multilayer Perceptron}}: A {{New Approach}}},
 volume = {10},
 year = {1997}
}

@article{aw_derivation_2002,
 author = {Aw, A. and Klar, A. and Rascle, M. and Materne, T.},
 doi = {10.1137/S0036139900380955},
 file = {/home/matt/Zotero/storage/MK8AMGUZ/aw_et_al_derivation_of_continuum_traffic_flow_from_microscopic.pdf},
 issn = {0036-1399},
 journal = {SIAM Journal on Applied Mathematics},
 language = {en},
 number = {1},
 pages = {259--278},
 title = {Derivation of {{Continuum Traffic Flow Models}} from {{Microscopic Follow}}-the-{{Leader Models}}},
 volume = {63},
 year = {2002}
}

@article{aw_resurrection_2000,
 author = {Aw, A. and Rascle, Michel},
 doi = {10.1137/S0036139997332099},
 file = {/home/matt/Documents/Papers/aw_raschle_resurrection.pdf},
 issn = {0036-1399},
 journal = {SIAM Journal on Applied Mathematics},
 number = {3},
 pages = {916--938},
 title = {Resurrection of "{{Second Order}}" {{Models}} of {{Traffic Flow}}},
 volume = {60},
 year = {2000}
}

@article{azadi_semantic_2019,
 author = {Azadi, Samaneh and Tschannen, Michael and Tzeng, Eric and Gelly, Sylvain and Darrell, Trevor and Lucic, Mario},
 journal = {ArXiv preprint},
 title = {Semantic {{Bottleneck Scene Generation}}},
 url = {https://arxiv.org/abs/1911.11357},
 volume = {abs/1911.11357},
 year = {2019}
}

@inproceedings{azencot_forecasting_2020,
 author = {Omri Azencot and
N. Benjamin Erichson and
Vanessa Lin and
Michael W. Mahoney},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/AzencotELM20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {475--485},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Forecasting Sequential Data Using Consistent Koopman Autoencoders},
 url = {http://proceedings.mlr.press/v119/azencot20a.html},
 volume = {119},
 year = {2020}
}

@article{azizov_linear_1981,
 abstract = {The paper contains a survey of papers reviewed in Ref. Zh. Matematika from 1953\textendash 1978 on the theory of linear operators in (mainly Hibert) spaces with indefinite metric and their applications to various domains of mathematics and mechanics. As a preliminary, the needed results on the geometry of spaces with indefinite metric are described.},
 author = {Azizov, T. Ya. and Iokhvidov, I. S.},
 doi = {10.1007/BF01375563},
 file = {/home/matt/Zotero/storage/YKGYIYUI/Azizov and Iokhvidov - 1981 - Linear operators in spaces with indefinite metric .pdf},
 issn = {1573-8795},
 journal = {Journal of Soviet Mathematics},
 language = {en},
 number = {4},
 pages = {438--490},
 title = {Linear Operators in Spaces with Indefinite Metric and Their Applications},
 volume = {15},
 year = {1981}
}

@article{ba_layer_2016,
 author = {Ba, Jimmy Lei and Kiros, Jamie Ryan and Hinton, Geoffrey E.},
 journal = {ArXiv preprint},
 title = {Layer {{Normalization}}},
 url = {https://arxiv.org/abs/1607.06450},
 volume = {abs/1607.06450},
 year = {2016}
}

@inproceedings{bae_design_2019,
 abstract = {This paper presents the design and implementation results of an ecological adaptive cruise controller (ECO-ACC) which exploits driving automation and connectivity. The controller avoids front collisions and traffic light violations, and is designed to reduce the energy consumption of connected automated vehicles by utilizing historical and real-time signal phase and timing data of traffic lights that adapt to the current traffic conditions. We propose an optimization-based generation of a reference velocity, and a velocity-tracking model predictive controller that avoids front collisions and violations. We present an experimental setup encompassing the real vehicle and controller in the loop, and an environment simulator in which the traffic flow and the traffic light patterns are calibrated on real-world data. We present simulation and experimental results, finding a significant potential for energy consumption reduction, even in the presence of traffic.},
 author = {Bae, S. and Kim, Y. and Guanetti, J. and Borrelli, F. and Moura, S.},
 booktitle = {2019 {{American Control Conference}} ({{ACC}})},
 file = {/home/matt/Zotero/storage/CTBTD2PP/Bae et al_2019_Design and Implementation of Ecological Adaptive Cruise Control for Autonomous.pdf;/home/matt/Zotero/storage/IIPN28BA/8814905.html},
 pages = {4628--4634},
 title = {Design and {{Implementation}} of {{Ecological Adaptive Cruise Control}} for {{Autonomous Driving}} with {{Communication}} to {{Traffic Lights}}},
 year = {2019}
}

@article{bagnato_unconstrained_2019,
 author = {Bagnato, Luca and Punzo, Antonio},
 journal = {ArXiv preprint},
 title = {Unconstrained Representation of Orthogonal Matrices with Application to Common Principle Components},
 url = {https://arxiv.org/abs/1906.00587},
 volume = {abs/1906.00587},
 year = {2019}
}

@inproceedings{bahdanau_neural_2015,
 author = {Dzmitry Bahdanau and
Kyunghyun Cho and
Yoshua Bengio},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/BahdanauCB14.bib},
 booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Fri, 29 Mar 2019 00:00:00 +0100},
 title = {Neural Machine Translation by Jointly Learning to Align and Translate},
 url = {http://arxiv.org/abs/1409.0473},
 year = {2015}
}

@inproceedings{bahdanau_systematic_2019,
 author = {Dzmitry Bahdanau and
Shikhar Murty and
Michael Noukhovitch and
Thien Huu Nguyen and
Harm de Vries and
Aaron C. Courville},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/BahdanauMNNVC19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Systematic Generalization: What Is Required and Can It Be Learned?},
 url = {https://openreview.net/forum?id=HkezXnA9YX},
 year = {2019}
}

@article{bai_empirical_2018,
 author = {Bai, Shaojie and Kolter, J. Zico and Koltun, Vladlen},
 journal = {ArXiv preprint},
 title = {An {{Empirical Evaluation}} of {{Generic Convolutional}} and {{Recurrent Networks}} for {{Sequence Modeling}}},
 url = {https://arxiv.org/abs/1803.01271},
 volume = {abs/1803.01271},
 year = {2018}
}

@article{bai_length_2012,
 author = {Bai, H. and Liu, H. and Zhao, Y. and Wang, N.},
 journal = {International Journal of Advancements in Computing Technology},
 number = {4},
 pages = {156--164},
 title = {Length Otimization of Traffic Signal Cycle},
 volume = {4},
 year = {2012}
}

@inproceedings{bajcsy_efficient_2019,
 abstract = {Real-world autonomous vehicles often operate in a priori unknown environments. Since most of these systems are safety-critical, it is important to ensure they operate safely even when faced with environmental uncertainty. Current safety analysis tools enable autonomous systems to reason about safety given full information about the state of the environment a priori. However, these tools do not scale well to scenarios where the environment is being sensed in real time, such as during navigation tasks. In this work, we propose a novel, real-time safety analysis method based on Hamilton-Jacobi reachability that provides strong safety guarantees despite the unknown parts of the environment. Our safety method is planner-agnostic and provides guarantees for a variety of mapping sensors. We demonstrate our approach in simulation and in hardware to provide safety guarantees around a state-of-the-art vision-based, learning-based planner. Videos of our approach and experiments are available on the project website1.},
 author = {Bajcsy, Andrea and Bansal, Somil and Bronstein, Eli and Tolani, Varun and Tomlin, Claire J.},
 booktitle = {2019 {{IEEE}} 58th {{Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
 doi = {10.1109/CDC40024.2019.9030133},
 file = {/home/matt/Zotero/storage/GBF4993D/Bajcsy et al. - 2019 - An Efficient Reachability-Based Framework for Prov.pdf;/home/matt/Zotero/storage/7DWJM7UQ/9030133.html},
 issn = {2576-2370},
 pages = {1758--1765},
 title = {An {{Efficient Reachability}}-{{Based Framework}} for {{Provably Safe Autonomous Navigation}} in {{Unknown Environments}}},
 year = {2019}
}

@article{balakrishna_-policy_2019,
 author = {Balakrishna, Ashwin and Thananjeyan, Brijen and Lee, Jonathan and Li, Felix and Zahed, Arsh and Gonzalez, Joseph E. and Goldberg, Ken},
 journal = {ArXiv preprint},
 title = {On-{{Policy Robot Imitation Learning}} from a {{Converging Supervisor}}},
 url = {https://arxiv.org/abs/1907.03423},
 volume = {abs/1907.03423},
 year = {2019}
}

@article{balcan_theory_2008,
 abstract = {Kernel functions have become an extremely popular tool in machine learning, with an attractive theory as well. This theory views a kernel as implicitly mapping data points into a possibly very high dimensional space, and describes a kernel function as being good for a given learning problem if data is separable by a large margin in that implicit space. However, while quite elegant, this theory does not necessarily correspond to the intuition of a good kernel as a good measure of similarity, and the underlying margin in the implicit space usually is not apparent in ``natural'' representations of the data. Therefore, it may be difficult for a domain expert to use the theory to help design an appropriate kernel for the learning task at hand. Moreover, the requirement of positive semi-definiteness may rule out the most natural pairwise similarity functions for the given problem domain.},
 author = {Balcan, Maria-Florina and Blum, Avrim and Srebro, Nathan},
 doi = {10.1007/s10994-008-5059-5},
 file = {/home/matt/Zotero/storage/8DSJK2JR/Balcan et al. - 2008 - A theory of learning with similarity functions.pdf},
 issn = {0885-6125, 1573-0565},
 journal = {Machine Learning},
 language = {en},
 number = {1-2},
 pages = {89--112},
 title = {A Theory of Learning with Similarity Functions},
 volume = {72},
 year = {2008}
}

@inproceedings{baldi_understanding_2013,
 author = {Pierre Baldi and
Peter J. Sadowski},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/BaldiS13.bib},
 booktitle = {Advances in Neural Information Processing Systems 26: 27th Annual
Conference on Neural Information Processing Systems 2013. Proceedings
of a meeting held December 5-8, 2013, Lake Tahoe, Nevada, United States},
 editor = {Christopher J. C. Burges and
L{\'{e}}on Bottou and
Zoubin Ghahramani and
Kilian Q. Weinberger},
 pages = {2814--2822},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Understanding Dropout},
 url = {https://proceedings.neurips.cc/paper/2013/hash/71f6278d140af599e06ad9bf1ba03cb0-Abstract.html},
 year = {2013}
}

@techreport{balke_development_2005,
 author = {Balke, K. and Charara, H. and Parker, R.},
 institution = {{Texas Transportation Institute}},
 number = {FHWA/TX-05/0-4422-2},
 title = {Development of a Traffic Signal Performance System ({{TSPMS}})},
 year = {2005}
}

@book{bandeira_tightness_2014,
 author = {Bandeira, Afonso S. and Boumal, Nicolas and Singer, Amit},
 title = {Tightness of the Maximum Likelihood Semidefinite Relaxation for Angular Synchronization},
 year = {2014}
}

@inproceedings{bangura_nonlinear_2012,
 author = {Bangura, Moses and Mahony, Robert and others},
 booktitle = {Australasian Conference on Robotics and Automation},
 file = {/home/matt/Zotero/storage/FIWJXXCS/pap121.pdf},
 pages = {1--10},
 title = {Nonlinear Dynamic Modeling for High Performance Control of a Quadrotor},
 year = {2012}
}

@article{bansal_hamilton-jacobi_2019,
 author = {Bansal, Somil and Bajcsy, Andrea and Ratner, Ellis and Dragan, Anca D. and Tomlin, Claire J.},
 journal = {ArXiv preprint},
 title = {A {{Hamilton}}-{{Jacobi Reachability}}-{{Based Framework}} for {{Predicting}} and {{Analyzing Human Motion}} for {{Safe Planning}}},
 url = {https://arxiv.org/abs/1910.13369},
 volume = {abs/1910.13369},
 year = {2019}
}

@article{bargmann_hilbert_1961,
 author = {Bargmann, V.},
 doi = {10.1002/cpa.3160140303},
 file = {/home/matt/Zotero/storage/R9ZCBWRA/Bargmann - 1961 - On a Hilbert space of analytic functions and an as.pdf},
 issn = {00103640, 10970312},
 journal = {Communications on Pure and Applied Mathematics},
 language = {en},
 number = {3},
 pages = {187--214},
 title = {On a {{Hilbert}} Space of Analytic Functions and an Associated Integral Transform Part {{I}}},
 volume = {14},
 year = {1961}
}

@article{baric_decentralized_2012,
 author = {Baric, M. and Borrelli, F.},
 doi = {10.1109/TAC.2011.2169629},
 issn = {0018-9286},
 journal = {IEEE Transactions On Automatic Control},
 number = {57},
 pages = {1018--1024},
 title = {Decentralized {{Robust Control Invariance}} for a {{Network}} of {{Storage Devices}}},
 volume = {4},
 year = {2012}
}

@inproceedings{barla_histogram_2003,
 abstract = {In this paper we address the problem of classifying images, by exploiting global features that describe color and illu, mination properties, and by using the statistical learning paradigm. The contribution of this paper is twofold. First, we show that histogram intersection has the requited mathematical properties to be used as a kernel function for Support Vector Machines (SVMs). Second, we give two examples of how a SVM, equipped with such a kernel, can achievevery promising results on image classifcationbased on color information.},
 address = {{Barcelona, Spain}},
 author = {Barla, A. and Odone, F. and Verri, A.},
 booktitle = {Proceedings 2003 {{International Conference}} on {{Image Processing}} ({{Cat}}. {{No}}.{{03CH37429}})},
 doi = {10.1109/ICIP.2003.1247294},
 file = {/home/matt/Zotero/storage/EV89AN8E/Barla et al. - 2003 - Histogram intersection kernel for image classifica.pdf},
 isbn = {978-0-7803-7750-9},
 language = {en},
 pages = {III-513-16},
 publisher = {{IEEE}},
 title = {Histogram Intersection Kernel for Image Classification},
 volume = {2},
 year = {2003}
}

@article{baron-cohen_does_1985,
 abstract = {We use a new model of metarepresentational development to predict a cognitive deficit which could explain a crucial component of the social impairment in childhood autism. One of the manifestations of a basic metarepresentational capacity is a `theory of mind'. We have reason to believe that autistic children lack such a `theory'. If this were so, then they would be unable to impute beliefs to others and to predict their behaviour. This hypothesis was tested using Wimmer and Perner's puppet play paradigm. Normal children and those with Down's syndrome were used as controls for a group of autistic children. Even though the mental age of the autistic children was higher than that of the controls, they alone failed to impute beliefs to others. Thus the dysfunction we have postulated and demonstrated is independent of mental retardation and specific to autism.},
 author = {{Baron-Cohen}, Simon and Leslie, Alan M. and Frith, Uta},
 doi = {10.1016/0010-0277(85)90022-8},
 file = {/home/matt/Zotero/storage/FDXANIEU/Baron-Cohen et al. - 1985 - Does the autistic child have a “theory of mind” .pdf},
 issn = {00100277},
 journal = {Cognition},
 language = {en},
 number = {1},
 pages = {37--46},
 title = {Does the Autistic Child Have a ``Theory of Mind'' ?},
 volume = {21},
 year = {1985}
}

@article{bartlett_local_2005,
 author = {Bartlett, Peter L. and Bousquet, Olivier and Mendelson, Shahar},
 doi = {10.1214/009053605000000282},
 file = {/home/matt/Zotero/storage/EEJUP8T4/bartlett_local_rademacher_complexities.pdf},
 issn = {0090-5364},
 journal = {The Annals of Statistics},
 language = {en},
 number = {4},
 pages = {1497--1537},
 title = {Local {{Rademacher}} Complexities},
 volume = {33},
 year = {2005}
}

@article{baselines,
 author = {Dhariwal, Prafulla and Hesse, Christopher and Klimov, Oleg and Nichol, Alex and Plappert, Matthias and Radford, Alec and Schulman, John and Sidor, Szymon and Wu, Yuhuai and Zhokhov, Peter},
 journal = {GitHub repository},
 keywords = {⛔ No DOI found},
 publisher = {{GitHub}},
 title = {{{OpenAI Baselines}}},
 year = {2017}
}

@article{battaglia_relational_2018,
 author = {Battaglia, Peter W. and Hamrick, Jessica B. and Bapst, Victor and {Sanchez-Gonzalez}, Alvaro and Zambaldi, Vinicius and Malinowski, Mateusz and Tacchetti, Andrea and Raposo, David and Santoro, Adam and Faulkner, Ryan and Gulcehre, Caglar and Song, Francis and Ballard, Andrew and Gilmer, Justin and Dahl, George and Vaswani, Ashish and Allen, Kelsey and Nash, Charles and Langston, Victoria and Dyer, Chris and Heess, Nicolas and Wierstra, Daan and Kohli, Pushmeet and Botvinick, Matt and Vinyals, Oriol and Li, Yujia and Pascanu, Razvan},
 journal = {ArXiv preprint},
 title = {Relational Inductive Biases, Deep Learning, and Graph Networks},
 url = {https://arxiv.org/abs/1806.01261},
 volume = {abs/1806.01261},
 year = {2018}
}

@inproceedings{beaini_directional_2021,
 author = {Dominique Beaini and
Saro Passaro and
Vincent L{\'{e}}tourneau and
William L. Hamilton and
Gabriele Corso and
Pietro Li{\'{o}}},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/BeainiPLHCL21.bib},
 booktitle = {Proceedings of the 38th International Conference on Machine Learning,
{ICML} 2021, 18-24 July 2021, Virtual Event},
 editor = {Marina Meila and
Tong Zhang},
 pages = {748--758},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 25 Aug 2021 01:00:00 +0200},
 title = {Directional Graph Networks},
 url = {http://proceedings.mlr.press/v139/beani21a.html},
 volume = {139},
 year = {2021}
}

@incollection{behrisch_sumos_2014,
 address = {{Berlin, Heidelberg}},
 author = {Erdmann, Jakob and Krajzewicz, Daniel},
 booktitle = {Simulation of {{Urban Mobility}}},
 doi = {10.1007/978-3-662-45079-6_1},
 editor = {Behrisch, Michael and Krajzewicz, Daniel and Weber, Melanie},
 file = {/home/matt/Zotero/storage/DM58TBMY/sumo_road_network_model.pdf},
 isbn = {978-3-662-45078-9 978-3-662-45079-6},
 pages = {3--17},
 publisher = {{Springer Berlin Heidelberg}},
 title = {{{SUMO}}'s {{Road Intersection Model}}},
 volume = {8594},
 year = {2014}
}

@inproceedings{behrmann_invertible_2019,
 author = {Jens Behrmann and
Will Grathwohl and
Ricky T. Q. Chen and
David Duvenaud and
J{\"{o}}rn{-}Henrik Jacobsen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/BehrmannGCDJ19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {573--582},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Invertible Residual Networks},
 url = {http://proceedings.mlr.press/v97/behrmann19a.html},
 volume = {97},
 year = {2019}
}

@inproceedings{bell_time-dependent_1996,
 author = {Bell, M. G. H. and Lam, W. H. K. and Iida, Y.},
 booktitle = {Proceedings of the 13th {{International Symposium}} on {{Transportation}} and {{Traffic Theory}}},
 editor = {Lesort, J. B.},
 pages = {385--403},
 title = {A {{Time}}-Dependent Multi-Class Path Flow Estimator},
 year = {1996}
}

@article{belletti_expert_2017,
 author = {Belletti, Francois and Haziza, Daniel and Gomes, Gabriel and Bayen, Alexandre M},
 doi = {10.1109/TITS.2017.2725912},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 title = {Expert {{Level}} Control of {{Ramp Metering}} Based on {{Multi}}-Task {{Deep Reinforcement Learning}}},
 year = {2017}
}

@book{bemporad_model_2004,
 annotation = {Published: The Mathworks, Inc.},
 author = {Bemporad, A. and Morari, M. and Ricker, N. L.},
 title = {Model {{Predictive Control Toolbox}} for {{Matlab}}},
 year = {2004}
}

@article{ben-akiva_dynamic_1986,
 author = {{Ben-Akiva}, M. and {\noopsort{palma}}de Palma, A. and Kanaroglou, K.},
 journal = {Transportation Science},
 pages = {164--181},
 title = {Dynamic Model of {{Peak}} Period Traffic Congestion with Elastic Arrival Rates},
 volume = {20},
 year = {1986}
}

@article{ben-akiva_network_2001,
 author = {{Ben-Akiva}, M. and Bierlaire, M. and Burton, D. and Koutsopolous, H. N. and Mishalani, R.},
 journal = {Networks and Spatial Economics},
 pages = {293--318},
 title = {Network State Estimation and Prediction for Real-Time Traffic Management},
 year = {2001}
}

@inproceedings{benavidez_landing_2014,
 author = {Benavidez, Patrick and Lambert, Josue and Jaimes, Aldo and Jamshidi, Mo},
 booktitle = {World {{Automation Congress}} ({{WAC}}), 2014},
 file = {/home/matt/Zotero/storage/4J5QVQZB/landing_cuadracopter_mobile_base_IEEE.pdf;/home/matt/Zotero/storage/Q9GAJUM8/Landing_control_of_quadcopter.pdf},
 pages = {803--812},
 publisher = {{IEEE}},
 title = {Landing of an Ardrone 2.0 Quadcopter on a Mobile Base Using Fuzzy Logic},
 year = {2014}
}

@incollection{bergendorff_congestion_1997,
 author = {Bergendorff, P. and Hearn, D. W. and Ramana, M. V.},
 booktitle = {Network {{Optimization}}},
 editor = {Pardalos, P. M. and Hearn, D. W. and Hager, W. W.},
 pages = {51--71},
 publisher = {{Springer-Verlag}},
 series = {Lecture {{Notes}} in {{Economics}} and {{Mathematical Systems}},},
 title = {Congestion {{Toll Pricing}} of {{Traffic Networks}},},
 volume = {450},
 year = {1997}
}

@article{berseth_smirl_2020,
 author = {Berseth, Glen and Geng, Daniel and Devin, Coline and Rhinehart, Nicholas and Finn, Chelsea and Jayaraman, Dinesh and Levine, Sergey},
 journal = {ArXiv preprint},
 title = {{{SMiRL}}: {{Surprise Minimizing RL}} in {{Dynamic Environments}}},
 url = {https://arxiv.org/abs/1912.05510},
 volume = {abs/1912.05510},
 year = {2019}
}

@inproceedings{bertelli_kernelized_2011,
 author = {Luca Bertelli and
Tianli Yu and
Diem Vu and
Burak Gokturk},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/BertelliYVG11.bib},
 booktitle = {The 24th {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2011, Colorado Springs, CO, USA, 20-25 June 2011},
 doi = {10.1109/CVPR.2011.5995597},
 pages = {2153--2160},
 publisher = {{IEEE} Computer Society},
 timestamp = {Fri, 02 Jun 2017 01:00:00 +0200},
 title = {Kernelized structural {SVM} learning for supervised object segmentation},
 url = {https://doi.org/10.1109/CVPR.2011.5995597},
 year = {2011}
}

@unpublished{bertini_r._evaluation_2001,
 author = {{Bertini, R.} and Tantiyanugulchai, S. and Anderson, E. and Lindgren, R. and Leal, M.},
 title = {Evaluation of {{Region}} 2 {{Incident Response Program}} Using Archived Data},
 year = {2001}
}

@inproceedings{bertini_r._toward_2003,
 author = {{Bertini, R.}},
 booktitle = {{{IEEE}} 6th {{International Conference}} on {{Intelligent Transportation Systems}}},
 title = {Toward the Systematic Diagnosis of Freeway Bottleneck Activation},
 year = {2003}
}

@article{bhatti_hostile_2017,
 abstract = {An attacker's ability to control a maritime surface vessel by broadcasting counterfeit civil Global Positioning System (GPS) signals is analyzed and demonstrated. The aim of this work is to explore civil maritime transportation's vulnerability to deceptive GPS signals and to develop a detection technique that is compatible with sensors commonly available on modern ships. It is shown that despite access to a variety of high-quality navigation and surveillance sensors, modern maritime navigation depends crucially on satellite navigation and that a deception attack can be disguised as the effects of slowly-changing ocean currents. An innovations-based detection framework that optimally chooses the measurement sampling interval to minimize the probability of a ship exceeding its alert limits without detection is developed and analyzed. A field experiment confirms the vulnerability analysis by demonstrating hostile control of a 65-m yacht in the Mediterranean Sea. Copyright \textcopyright{} 2017 Institute of Navigation.},
 author = {Bhatti, Jahshan and Humphreys, Todd E.},
 doi = {10.1002/navi.183},
 file = {/home/matt/Zotero/storage/CHAAA53Z/Bhatti and Humphreys - 2017 - Hostile Control of Ships via False GPS Signals De.pdf},
 issn = {00281522},
 journal = {Navigation},
 language = {en},
 number = {1},
 pages = {51--66},
 shorttitle = {Hostile {{Control}} of {{Ships}} via {{False GPS Signals}}},
 title = {Hostile {{Control}} of {{Ships}} via {{False GPS Signals}}: {{Demonstration}} and {{Detection}}},
 volume = {64},
 year = {2017}
}

@article{bianco_benchmark_2018,
 abstract = {This work presents an in-depth analysis of the majority of the deep neural networks (DNNs) proposed in the state of the art for image recognition. For each DNN multiple performance indices are observed, such as recognition accuracy, model complexity, computational complexity, memory usage, and inference time. The behavior of such performance indices and some combinations of them are analyzed and discussed. To measure the indices we experiment the use of DNNs on two different computer architectures, a workstation equipped with a NVIDIA Titan X Pascal and an embedded system based on a NVIDIA Jetson TX1 board. This experimentation allows a direct comparison between DNNs running on machines with very different computational capacity. This study is useful for researchers to have a complete view of what solutions have been explored so far and in which research directions are worth exploring in the future; and for practitioners to select the DNN architecture(s) that better fit the resource constraints of practical deployments and applications. To complete this work, all the DNNs, as well as the software used for the analysis, are available online.},
 archiveprefix = {arXiv},
 author = {Bianco, Simone and Cadene, Remi and Celona, Luigi and Napoletano, Paolo},
 doi = {10.1109/ACCESS.2018.2877890},
 eprint = {1810.00736},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/YLL65FYK/Bianco et al. - 2018 - Benchmark Analysis of Representative Deep Neural N.pdf},
 issn = {2169-3536},
 journal = {IEEE Access},
 language = {en},
 pages = {64270--64277},
 title = {Benchmark {{Analysis}} of {{Representative Deep Neural Network Architectures}}},
 volume = {6},
 year = {2018}
}

@article{bierlaire_efficient_2004,
 author = {Bierlaire, M. and Crittin, F.},
 journal = {Operations Research},
 number = {1},
 pages = {116--127},
 title = {An Efficient Algorithm for Real-Time Estimation and Prediction of Dynamic {{OD}} Table},
 volume = {52},
 year = {2004}
}

@book{bilger_auto_2013,
 annotation = {Published: The New Yorker},
 author = {Bilger, B.},
 title = {{{AUTO CORRECT}}: {{Has}} the Self-Driving Car at Last Arrived?},
 year = {2013}
}

@article{birkhoff_orthogonality_1935,
 abstract = {Project Euclid - mathematics and statistics online},
 author = {Birkhoff, Garrett},
 doi = {10.1215/S0012-7094-35-00115-6},
 file = {/home/matt/Zotero/storage/8RY8IR7L/Birkhoff - 1935 - Orthogonality in linear metric spaces.pdf;/home/matt/Zotero/storage/XIHK95HH/1077488974.html},
 issn = {0012-7094, 1547-7398},
 journal = {Duke Mathematical Journal},
 language = {en},
 mrnumber = {MR1545873},
 number = {2},
 pages = {169--172},
 title = {Orthogonality in Linear Metric Spaces},
 volume = {1},
 year = {1935},
 zmnumber = {0012.30604}
}

@article{blake_its_2002,
 author = {Blake, Laurie},
 journal = {Minneapolis - St. Paul Star Tribune},
 title = {It's {{September}} \textendash{} When Traffic Again Turns Ugly},
 year = {2002}
}

@article{blanchini_any_2000,
 author = {Blanchini, Franco and Miani, Stefano},
 journal = {SJCO},
 keywords = {constrained control,convex analysis,domain of attraction,Lyapunov functions,tracking},
 number = {3},
 pages = {971--994},
 title = {Any {{Domain}} of {{Attraction}} for a {{Linear Constrained System}} Is a {{Tracking Domain}} of {{Attraction}}},
 volume = {38},
 year = {2000}
}

@article{blanchini_control_1990,
 author = {Blanchini, F.},
 journal = {JOTA},
 number = {1},
 pages = {29--40},
 title = {Control Synthesis for Discrete Time Systems with Control and State Bounds in the Presence of Disturbances},
 volume = {65},
 year = {1990}
}

@article{blanchini_feedback_1990,
 author = {Blanchini, F.},
 journal = {TAC},
 number = {11},
 pages = {1231--1234},
 title = {Feedback Control for Linear Time-Invariant Systems with State and Control Bounds in the Presence of Disturbances},
 volume = {AC-35},
 year = {1990}
}

@article{blanchini_feedback_2000,
 author = {Blanchini, F. and Pesenti, R. and Rinaldi, F. and Ukovich, W.},
 journal = {TRA},
 number = {3},
 pages = {313--317},
 title = {Feedback {{Control}} of {{Production}}\textendash{{Distribution Systems}} with {{Unknown Demand}} and {{Delays}}},
 volume = {16},
 year = {2000}
}

@article{blanchini_least_1997,
 author = {Blanchini, F. and Rinaldi, F. and Ukovich, W.},
 journal = {TRA},
 number = {5},
 pages = {633--645},
 title = {Least {{Inventory Control}} of {{Multistorage Systems}} with {{Non}}\textendash{{Stochastic Unknown Inputs}}},
 volume = {13},
 year = {1997}
}

@article{blanchini_network_1997,
 author = {Blanchini, F. and Rinaldi, F. and Ukovich, W.},
 journal = {SIOPT},
 number = {2},
 pages = {560--578},
 title = {A {{Network Design Problem}} for a {{Distribution System}} with {{Uncertain Demands}}},
 volume = {7},
 year = {1997}
}

@article{blanchini_nonquadratic_1995,
 author = {Blanchini, F.},
 journal = {AUTO},
 number = {3},
 pages = {451--461},
 title = {Nonquadratic {{Lyapunov}} Functions for Robust Control},
 volume = {31},
 year = {1995}
}

@inproceedings{blanchini_robust_1993,
 author = {Blanchini, F.},
 booktitle = {{{CDC93}}},
 pages = {2592--2593},
 title = {Robust Control for Uncertain Linear Systems via Polyhedral {{Lyapunov}} Functions},
 volume = {3},
 year = {1993}
}

@article{blanchini_set_1999,
 author = {Blanchini, F.},
 journal = {AUTO},
 number = {11},
 pages = {1747--1767},
 title = {Set Invariance in Control - {{A}} Survey},
 volume = {35},
 year = {1999}
}

@article{blanchini_ultimate_1994,
 author = {Blanchini, F.},
 journal = {TAC},
 number = {2},
 pages = {428--433},
 title = {Ultimate Boundedness Control for Uncertain Discrete-Time Systems via Set-Induced {{Lyapunov}} Functions},
 volume = {39},
 year = {1994}
}

@article{blandin_sequential_2012,
 author = {Blandin, S{\'e}bastien and Couque, Adrien and Bayen, Alexandre and Work, Daniel},
 doi = {10.1016/j.physd.2012.05.005},
 file = {/home/matt/Documents/Papers/blandin_sequential_data_assim.pdf.pdf},
 issn = {01672789},
 journal = {Physica D: Nonlinear Phenomena},
 language = {en},
 number = {17},
 pages = {1421--1440},
 title = {On Sequential Data Assimilation for Scalar Macroscopic Traffic Flow Models},
 volume = {241},
 year = {2012}
}

@article{blei_nested_2010,
 abstract = {We present the nested Chinese restaurant process (nCRP), a stochastic process that assigns probability distributions to ensembles of in\TH nitely deep, in\TH nitely branching trees. We show how this stochastic process can be used as a prior distribution in a Bayesian nonparametric model of document collections. Speci\TH cally, we present an application to information retrieval in which documents are modeled as paths down a random tree, and the preferential attachment dynamics of the nCRP leads to clustering of documents according to sharing of topics at multiple levels of abstraction. Given a corpus of documents, a posterior inference algorithm \TH nds an approximation to a posterior distribution over trees, topics and allocations of words to levels of the tree. We demonstrate this algorithm on collections of scienti\TH c abstracts from several journals. This model exempli\TH es a recent trend in statistical machine learning\textemdash the use of Bayesian nonparametric methods to infer distributions on \ss exible data structures.},
 author = {Blei, David M. and Griffiths, Thomas L. and Jordan, Michael I.},
 doi = {10.1145/1667053.1667056},
 file = {/home/matt/Zotero/storage/MTMPKM9Z/Blei et al. - 2010 - The nested chinese restaurant process and bayesian.pdf},
 issn = {00045411},
 journal = {Journal of the ACM},
 language = {en},
 number = {2},
 pages = {1--30},
 title = {The Nested Chinese Restaurant Process and Bayesian Nonparametric Inference of Topic Hierarchies},
 volume = {57},
 year = {2010}
}

@article{blei_variational_2017,
 abstract = {One of the core problems of modern statistics is to approximate difficult-to-compute probability densities. This problem is especially important in Bayesian statistics, which frames all inference about unknown quantities as a calculation involving the posterior density. In this article, we review variational inference (VI), a method from machine learning that approximates probability densities through optimization. VI has been used in many applications and tends to be faster than classical methods, such as Markov chain Monte Carlo sampling. The idea behind VI is to first posit a family of densities and then to find a member of that family which is close to the target density. Closeness is measured by Kullback\textendash Leibler divergence. We review the ideas behind mean-field variational inference, discuss the special case of VI applied to exponential family models, present a full example with a Bayesian mixture of Gaussians, and derive a variant that uses stochastic optimization to scale up to massive data. We discuss modern research in VI and highlight important open problems. VI is powerful, but it is not yet well understood. Our hope in writing this article is to catalyze statistical research on this class of algorithms. Supplementary materials for this article are available online.},
 author = {Blei, David M. and Kucukelbir, Alp and McAuliffe, Jon D.},
 doi = {10.1080/01621459.2017.1285773},
 file = {/home/matt/Zotero/storage/5YUY84D2/Blei et al. - 2017 - Variational Inference A Review for Statisticians.pdf;/home/matt/Zotero/storage/WVFMVW7C/01621459.2017.html},
 issn = {0162-1459},
 journal = {Journal of the American Statistical Association},
 number = {518},
 pages = {859--877},
 shorttitle = {Variational {{Inference}}},
 title = {Variational {{Inference}}: {{A Review}} for {{Statisticians}}},
 volume = {112},
 year = {2017}
}

@article{bliemer_dynamic_2007,
 author = {Bliemer, Michiel},
 doi = {10.3141/2029-02},
 file = {/home/matt/Zotero/storage/CS9I2BB8/bliemer_dynamic_queueing.pdf;/home/matt/Zotero/storage/ZA233PTH/flotterod_2011_TRB_operational_macroscopic.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {14--21},
 title = {Dynamic {{Queuing}} and {{Spillback}} in {{Analytical Multiclass Dynamic Network Loading Model}}},
 volume = {2029},
 year = {2007}
}

@article{bliemer_impact_2008,
 author = {Bliemer, Michiel and Bovy, Piet},
 doi = {10.3141/2076-02},
 file = {/home/matt/Zotero/storage/JADKBZEZ/bliemer_bovy_routechoice.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {10--19},
 title = {Impact of {{Route Choice Set}} on {{Route Choice Probabilities}}},
 volume = {2076},
 year = {2008}
}

@book{board_highway_2000,
 author = {Board, Transportation Research},
 title = {Highway {{Capacity Manual}} 2000},
 year = {2000}
}

@inproceedings{bobu_less_2020,
 abstract = {Robots need models of human behavior for both inferring human goals and preferences, and predicting what people will do. A common model is the Boltzmann noisily-rational decision model, which assumes people approximately optimize a reward function and choose trajectories in proportion to their exponentiated reward. While this model has been successful in a variety of robotics domains, its roots lie in econometrics, and in modeling decisions among different discrete options, each with its own utility or reward. In contrast, human trajectories lie in a continuous space, with continuous-valued features that influence the reward function. We propose that it is time to rethink the Boltzmann model, and design it from the ground up to operate over such trajectory spaces. We introduce a model that explicitly accounts for distances between trajectories, rather than only their rewards. Rather than each trajectory affecting the decision independently, similar trajectories now affect the decision together. We start by showing that our model better explains human behavior in a user study. We then analyze the implications this has for robot inference, first in toy environments where we have ground truth and find more accurate inference, and finally for a 7DOF robot arm learning from user demonstrations.},
 archiveprefix = {arXiv},
 author = {Bobu, Andreea and Scobee, Dexter R. R. and Fisac, Jaime F. and Sastry, S. Shankar and Dragan, Anca D.},
 booktitle = {Proceedings of the 2020 {{ACM}}/{{IEEE International Conference}} on {{Human}}-{{Robot Interaction}}},
 doi = {10.1145/3319502.3374811},
 eprint = {2001.04465},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/EWC5443C/Bobu et al. - 2020 - LESS is More Rethinking Probabilistic Models of H.pdf},
 language = {en},
 pages = {429--437},
 shorttitle = {{{LESS}} Is {{More}}},
 title = {{{LESS}} Is {{More}}: {{Rethinking Probabilistic Models}} of {{Human Behavior}}},
 year = {2020}
}

@article{bobu_quantifying_2020,
 abstract = {The human input has enabled autonomous systems to improve their capabilities and achieve complex behaviors that are otherwise challenging to generate automatically. Recent work focuses on how robots can use such inputs\textemdash such as, demonstrations or corrections\textemdash to learn intended objectives. These techniques assume that the human`s desired objective already exists within the robot's hypothesis space. In reality, this assumption is often inaccurate: there will always be situations where the person might care about aspects of the task that the robot does not know about. Without this knowledge, the robot cannot infer the correct objective. Hence, when the robot's hypothesis space is misspecified, even methods that keep track of uncertainty over the objective fail because they reason about which hypothesis might be correct, and not whether any of the hypotheses are correct. In this article, we posit that the robot should reason explicitly about how well it can explain human inputs given its hypothesis space and use that situational confidence to inform how it should incorporate the human input. We demonstrate our method on a 7 degrees-of-freedom robot manipulator in learning from two important types of human inputs: demonstrations of motion planning tasks and physical corrections during the robot's task execution.},
 author = {Bobu, Andreea and Bajcsy, Andrea and Fisac, Jaime F. and Deglurkar, Sampada and Dragan, Anca D.},
 doi = {10.1109/TRO.2020.2971415},
 file = {/home/matt/Zotero/storage/XP7ED34J/Bobu et al. - 2020 - Quantifying Hypothesis Space Misspecification in L.pdf},
 issn = {1552-3098, 1941-0468},
 journal = {IEEE Transactions on Robotics},
 language = {en},
 pages = {1--20},
 title = {Quantifying {{Hypothesis Space Misspecification}} in {{Learning From Human}}\textendash{{Robot Demonstrations}} and {{Physical Corrections}}},
 year = {2020}
}

@article{boel_compositional_2006,
 author = {Boel, Ren{\'e} and Mihaylova, Lyudmila},
 doi = {10.1016/j.trb.2005.05.001},
 file = {/home/matt/Zotero/storage/SRKJ3G6A/boel_compositional.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {4},
 pages = {319--334},
 title = {A Compositional Stochastic Model for Real Time Freeway Traffic Simulation},
 volume = {40},
 year = {2006}
}

@book{bognar_indefinite_1974,
 address = {{Berlin, Heidelberg}},
 author = {Bogn{\'a}r, J{\'a}nos},
 doi = {10.1007/978-3-642-65567-8},
 isbn = {978-3-642-65569-2 978-3-642-65567-8},
 publisher = {{Springer Berlin Heidelberg}},
 title = {Indefinite {{Inner Product Spaces}}},
 year = {1974}
}

@article{boik_local_1998,
 author = {Boik, Robert J.},
 doi = {10.1006/jmva.1998.1766},
 file = {/home/matt/Zotero/storage/ZYZ2527Z/Boik - 1998 - A Local Parameterization of Orthogonal and Semi-Or.pdf},
 issn = {0047259X},
 journal = {Journal of Multivariate Analysis},
 language = {en},
 number = {2},
 pages = {244--276},
 title = {A {{Local Parameterization}} of {{Orthogonal}} and {{Semi}}-{{Orthogonal Matrices}} with {{Applications}}},
 volume = {67},
 year = {1998}
}

@inproceedings{bolukbasi_man_2016,
 author = {Tolga Bolukbasi and
Kai{-}Wei Chang and
James Y. Zou and
Venkatesh Saligrama and
Adam Tauman Kalai},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/BolukbasiCZSK16.bib},
 booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
on Neural Information Processing Systems 2016, December 5-10, 2016,
Barcelona, Spain},
 editor = {Daniel D. Lee and
Masashi Sugiyama and
Ulrike von Luxburg and
Isabelle Guyon and
Roman Garnett},
 pages = {4349--4357},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Man is to Computer Programmer as Woman is to Homemaker? Debiasing
Word Embeddings},
 url = {https://proceedings.neurips.cc/paper/2016/hash/a486cd07e4ac3d270571622f4f316ec5-Abstract.html},
 year = {2016}
}

@book{booz_allen__hamilton_california_1999,
 author = {{Booz Allen \& Hamilton}},
 title = {California {{Life}}-{{Cycle Benefit}}/{{Cost Analysis Model}}},
 year = {1999}
}

@article{borkar_dynamic_2003,
 author = {Borkar, V. S. and Kumar, P. R.},
 journal = {IEEE Transactions On Automatic Control},
 number = {3},
 title = {Dynamic {{Cesaro}}\textendash{{Wardrop Equilibration}} in {{Networks}}},
 volume = {48},
 year = {2003}
}

@inproceedings{bouabdallah_backstepping_2005,
 author = {Bouabdallah, Samir and Siegwart, Roland},
 booktitle = {Robotics and {{Automation}}, 2005. {{ICRA}} 2005. {{Proceedings}} of the 2005 {{IEEE International Conference}} On},
 file = {/home/matt/Zotero/storage/ZBHSV49R/backstepping_quadrarotor_control.pdf},
 pages = {2247--2252},
 publisher = {{IEEE}},
 title = {Backstepping and Sliding-Mode Techniques Applied to an Indoor Micro Quadrotor},
 year = {2005}
}

@article{boyce_retrospective_2005,
 author = {Boyce, D. E. and Mahmassani, H. and Nagurney, A.},
 journal = {Papers in Regional Science},
 number = {4},
 pages = {85--103},
 title = {A Retrospective on {{Beckmann}}, {{McGuire}} and {{Winsten}}, \textbackslash{{emphStudies}} in the {{Economics}} of {{Transportation}}},
 volume = {84},
 year = {2005}
}

@book{boyd_convex_2004,
 address = {{Cambridge, UK ; New York}},
 author = {Boyd, Stephen P. and Vandenberghe, Lieven},
 file = {/home/matt/Zotero/storage/IWCZD2Z7/Boyd and Vandenberghe - 2004 - Convex optimization.pdf},
 isbn = {978-0-521-83378-3},
 lccn = {QA402.5 .B69 2004},
 publisher = {{Cambridge University Press}},
 title = {Convex Optimization},
 year = {2004}
}

@article{braess_uber_1969,
 author = {Braess, D.},
 journal = {Unternehmensforschung},
 pages = {258--268},
 title = {\"Uber Ein {{Paradoxen}} Aus Der {{Verkehrsplannung}}},
 volume = {12},
 year = {1969}
}

@inproceedings{britz_massive_2017,
 address = {Copenhagen, Denmark},
 author = {Britz, Denny  and
Goldie, Anna  and
Luong, Minh-Thang  and
Le, Quoc},
 booktitle = {Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing},
 doi = {10.18653/v1/D17-1151},
 pages = {1442--1451},
 publisher = {Association for Computational Linguistics},
 title = {Massive Exploration of Neural Machine Translation Architectures},
 url = {https://aclanthology.org/D17-1151},
 year = {2017}
}

@article{brockman_openai_2016,
 author = {Brockman, Greg and Cheung, Vicki and Pettersson, Ludwig and Schneider, Jonas and Schulman, John and Tang, Jie and Zaremba, Wojciech},
 journal = {ArXiv preprint},
 title = {{{OpenAI Gym}}},
 url = {https://arxiv.org/abs/1606.01540},
 volume = {abs/1606.01540},
 year = {2016}
}

@article{bronstein_geometric_2017,
 author = {Bronstein, Michael M. and Bruna, Joan and LeCun, Yann and Szlam, Arthur and Vandergheynst, Pierre},
 doi = {10.1109/MSP.2017.2693418},
 file = {/home/matt/Zotero/storage/CXMTD6VH/bronstein_vanderghesit_2017_geometric_deep_learning.pdf},
 issn = {1053-5888},
 journal = {IEEE Signal Processing Magazine},
 number = {4},
 pages = {18--42},
 shorttitle = {Geometric {{Deep Learning}}},
 title = {Geometric {{Deep Learning}}: {{Going}} beyond {{Euclidean}} Data},
 volume = {34},
 year = {2017}
}

@article{brossard_graph_2020,
 author = {Brossard, R{\'e}my and Frigo, Oriel and Dehaene, David},
 journal = {ArXiv preprint},
 title = {Graph Convolutions That Can Finally Model Local Structure},
 url = {https://arxiv.org/abs/2011.15069},
 volume = {abs/2011.15069},
 year = {2020}
}

@inproceedings{brown_language_2020,
 author = {Tom B. Brown and
Benjamin Mann and
Nick Ryder and
Melanie Subbiah and
Jared Kaplan and
Prafulla Dhariwal and
Arvind Neelakantan and
Pranav Shyam and
Girish Sastry and
Amanda Askell and
Sandhini Agarwal and
Ariel Herbert{-}Voss and
Gretchen Krueger and
Tom Henighan and
Rewon Child and
Aditya Ramesh and
Daniel M. Ziegler and
Jeffrey Wu and
Clemens Winter and
Christopher Hesse and
Mark Chen and
Eric Sigler and
Mateusz Litwin and
Scott Gray and
Benjamin Chess and
Jack Clark and
Christopher Berner and
Sam McCandlish and
Alec Radford and
Ilya Sutskever and
Dario Amodei},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/BrownMRSKDNSSAA20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Language Models are Few-Shot Learners},
 url = {https://proceedings.neurips.cc/paper/2020/hash/1457c0d6bfcb4967418bfb8ac142f64a-Abstract.html},
 year = {2020}
}

@inproceedings{brown_trouble_2017,
 author = {Barry A. T. Brown and
Eric Laurier},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/chi/BrownL17.bib},
 booktitle = {Proceedings of the 2017 {CHI} Conference on Human Factors in Computing
Systems, Denver, CO, USA, May 06-11, 2017},
 doi = {10.1145/3025453.3025462},
 editor = {Gloria Mark and
Susan R. Fussell and
Cliff Lampe and
m. c. schraefel and
Juan Pablo Hourcade and
Caroline Appert and
Daniel Wigdor},
 pages = {416--429},
 publisher = {{ACM}},
 timestamp = {Tue, 06 Nov 2018 00:00:00 +0100},
 title = {The Trouble with Autopilots: Assisted and Autonomous Driving on the
Social Road},
 url = {https://doi.org/10.1145/3025453.3025462},
 year = {2017}
}

@inproceedings{bruna_spectral_2014,
 author = {Joan Bruna and
Wojciech Zaremba and
Arthur Szlam and
Yann LeCun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/BrunaZSL13.bib},
 booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Fri, 29 Mar 2019 00:00:00 +0100},
 title = {Spectral Networks and Locally Connected Networks on Graphs},
 url = {http://arxiv.org/abs/1312.6203},
 year = {2014}
}

@inproceedings{bucki_rectangular_2020,
 abstract = {We present a novel multicopter trajectory planning algorithm (RAPPIDS) that is capable of quickly finding local collision-free trajectories given a single depth image from an onboard camera. The algorithm leverages a new pyramidbased spatial partitioning method that enables rapid collision detection between candidate trajectories and the environment. Due to its efficiency, the algorithm can be run at high rates on computationally constrained hardware, evaluating thousands of candidate trajectories in milliseconds. The performance of the algorithm is compared to existing collision checking methods in simulation, showing our method to be capable of evaluating orders of magnitude more trajectories per second. Experimental results are presented showing a quadcopter quickly navigating a previously unseen cluttered environment by running the algorithm on an ODROID-XU4 at 30 Hz.},
 archiveprefix = {arXiv},
 author = {Bucki, Nathan and Lee, Junseok and Mueller, Mark W.},
 booktitle = {Submitted to {{IEEE Robotics}} and {{Automation Letters}}},
 eprint = {2003.01245},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/WLJDNPBK/Bucki et al. - 2020 - Rectangular Pyramid Partitioning using Integrated .pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 shorttitle = {Rectangular {{Pyramid Partitioning}} Using {{Integrated Depth Sensors}} ({{RAPPIDS}})},
 title = {Rectangular {{Pyramid Partitioning}} Using {{Integrated Depth Sensors}} ({{RAPPIDS}}): {{A Fast Planner}} for {{Multicopter Navigation}}},
 year = {2020}
}

@article{bucknell_trade-off_2014,
 abstract = {The rapid-growth of smartphones with embedded navigation systems such as GPS modules provides new ways of monitoring traffic. These devices can register and send a great amount of traffic related data, which can be used for traffic state estimation. In such a case, the amount of data collected depends on two variables: the penetration rate of devices in traffic flow (P) and their data sampling frequency (z). Referring to data composition as the way certain number of observations is collected, in terms of P and z, we need to understand the relation between the amount and composition of data collected, and the accuracy achieved in traffic state estimation. This was accomplished through an in-depth analysis of two datasets of vehicle trajectories on freeways. The first dataset consists of trajectories over a real freeway, while the second dataset is obtained through microsimulation. Hypothetical scenarios of data sent by equipped vehicles were created, based on the composition of data collected. Different values of P and z were used, and each unique combination defined a specific scenario. Traffic states were estimated through two simple methods, and a more advanced one that incorporates traffic flow theory. A measure to quantify data to be collected was proposed, based on travel time, number of vehicles, penetration rate and sampling frequency. The error was below 6\% for every scenario in each dataset. Also, increasing data reduced variability in data count estimation. The performance of the different estimation methods varied through each dataset and scenario. Since the same number of observations can be gathered with different combinations of P and z, the effect of data composition was analyzed (a trade-off between penetration rate and sampling frequency). Different situations were found. In some, an increase in penetration rate is more effective to reduce estimation error than an increase in sampling frequency, considering an equal increase in observations. In other areas, the opposite relationship was found. Between these areas, an indifference curve was found. In fact, this curve is the solution to the optimization problem of minimizing the error given any fixed number of observations. As a general result, increasing sampling frequency (penetration rate) is more beneficial when the current sampling frequency (penetration rate) is low, independent of the penetration rate (sampling frequency).},
 author = {Bucknell, Christopher and Herrera, Juan C.},
 doi = {10.1016/j.trc.2014.05.007},
 file = {/home/matt/Zotero/storage/6Z3Y6PBH/Bucknell and Herrera - 2014 - A trade-off analysis between penetration rate and .pdf;/home/matt/Zotero/storage/XLRJFK9J/S0968090X1400120X.html},
 issn = {0968-090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 pages = {132--150},
 title = {A Trade-off Analysis between Penetration Rate and Sampling Frequency of Mobile Sensors in Traffic State Estimation},
 volume = {46},
 year = {2014}
}

@inproceedings{buisson_strada_1996,
 author = {Buisson, C. and {J-P. Lebacque} and Lesort, J. B.},
 booktitle = {{{CESA}}'96 {{IMACS Multiconference}}},
 title = {{{STRADA}}, a Discretized Macroscopic Model of Vehicular Traffic Flow in Complex Networks Based on the {{Godunov}} Scheme},
 year = {1996}
}

@article{bujarbaruah_learning_2019,
 author = {Bujarbaruah, Monimoy and Shetty, Akhil and Poolla, Kameshwar and Borrelli, Francesco},
 journal = {ArXiv preprint},
 title = {Learning {{Robustness}} with {{Bounded Failure}}: {{An Iterative MPC Approach}}},
 url = {https://arxiv.org/abs/1911.09910},
 volume = {abs/1911.09910},
 year = {2019}
}

@article{bullock_evaluation_2008,
 author = {Bullock, D. M. and Day, C. M. and Haseman, R. and Jr, T. M. Brennan and Wasson, J. S. and Sturdevant, J. R.},
 journal = {Transportation Research Record},
 pages = {37--49},
 title = {Evaluation of {{Arterial Signal Coordination}}: {{Methodologies}} for {{Visualizing High}}-{{Resolution Event Data}} and {{Measuring Travel Time}}},
 volume = {2192},
 year = {2008}
}

@article{bulusu_anomalous_2020,
 author = {Bulusu, Saikiran and Kailkhura, Bhavya and Li, Bo and Varshney, Pramod K. and Song, Dawn},
 journal = {ArXiv preprint},
 title = {Anomalous {{Instance Detection}} in {{Deep Learning}}: {{A Survey}}},
 url = {https://arxiv.org/abs/2003.06979},
 volume = {abs/2003.06979},
 year = {2020}
}

@inproceedings{burda_large-scale_2019,
 author = {Yuri Burda and
Harrison Edwards and
Deepak Pathak and
Amos J. Storkey and
Trevor Darrell and
Alexei A. Efros},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/BurdaEPSDE19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Large-Scale Study of Curiosity-Driven Learning},
 url = {https://openreview.net/forum?id=rJNwDjAqYX},
 year = {2019}
}

@article{byrnes_is_2011,
 author = {Byrnes, M.},
 journal = {The Atlantic Cities},
 title = {Is Bicycle Commuting Really Catching on? {{And}} If so, Where?},
 year = {2011}
}

@article{byun_flow_2020,
 author = {Byun, Jaeseung and M{\"a}kiharju, Simo A. and Mueller, Mark W.},
 journal = {ArXiv preprint},
 title = {A Flow Disturbance Estimation and Rejection Strategy of Multirotors with Round Trip Trajectories},
 url = {https://arxiv.org/abs/2003.02974},
 volume = {abs/2003.02974},
 year = {2020}
}

@article{c.d.cottrill_future_2013,
 author = {{C.D.Cottrill} and Pereira, F. C. and Zhao, F. and Dias, I. F. and Lim, H. B. and {Ben-Akiva}, M. and Zegras, P. C.},
 journal = {92nd Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 number = {Paper 13-4849-2},
 title = {The {{Future Mobility Survey}}: {{Experiences}} in Developing a Smartphone-Based Travel Survey in {{Singapore}}},
 year = {2013}
}

@article{c.oh_recognizing_2007,
 author = {{C.Oh} and Ritchie, S. G.},
 journal = {Pattern Recognition Letters},
 number = {9},
 pages = {1041--1049},
 title = {Recognizing Vehicle Classification Information from Blade Sensor Signature},
 volume = {28},
 year = {2007}
}

@article{cabannes_regrets_2019,
 author = {Cabannes, Th{\'e}ophile and Sangiovanni, Marco and Keimer, Alexander and Bayen, Alexandre M.},
 doi = {10/gf9cxw},
 file = {/home/matt/Zotero/storage/IW9HT3NV/Cabannes et al_2019_Regrets in Routing Networks.pdf},
 issn = {2374-0353},
 journal = {ACM Transactions on Spatial Algorithms and Systems (TSAS)},
 number = {2},
 pages = {9},
 shorttitle = {Regrets in {{Routing Networks}}},
 title = {Regrets in {{Routing Networks}}: {{Measuring}} the {{Impact}} of {{Routing Apps}} in {{Traffic}}},
 volume = {5},
 year = {2019}
}

@article{cabannes_regrets_2019-1,
 author = {Cabannes, Th{\'e}ophile and Sangiovanni, Marco and Keimer, Alexander and Bayen, Alexandre M.},
 doi = {10.1145/3325916},
 issn = {23740353},
 journal = {ACM Transactions on Spatial Algorithms and Systems},
 language = {en},
 number = {2},
 pages = {1--19},
 shorttitle = {Regrets in {{Routing Networks}}},
 title = {Regrets in {{Routing Networks}}: {{Measuring}} the {{Impact}} of {{Routing Apps}} in {{Traffic}}},
 volume = {5},
 year = {2019}
}

@article{cabannes_regrets_2019-2,
 abstract = {The impact of the recent increase in routing apps usage on road traffic remains uncertain to this day. The article introduces, for the first time, a criterion to evaluate a distance between an observed state of traffic and the user equilibrium of the traffic assignment: the average marginal regret. The average marginal regret provides a quantitative measure of the impact of routing apps on traffic using only link flows, link travel times, and travel demand. In non-atomic routing games (or static traffic assignment models), the average marginal regret is a measure of selfish drivers' behaviors. Unlike the price of anarchy, the average marginal regret in the routing game can be computed in polynomial time without any knowledge of user equilibria and socially optimal states of traffic. First, this article demonstrates on a small example that the average marginal regret is more appropriate to define proximity between an observed state of traffic and an user equilibrium state of traffic than comparing flows, travel times, or total cost. Then, experiments on two different models of app usage and three networks (including the whole L.A. network with more than 50,000 nodes) demonstrate that the average marginal regret decreases with an increase of app usage. Sensitivity analysis of the equilibrium state with respect to the app usage ratio proves that the average marginal regret monotonically decreases to 0 with an increase of app usage. Finally, using a toy example, the article concludes that app usage could become the new Braess paradox.},
 author = {Cabannes, Th{\'e}ophile and Sangiovanni, Marco and Keimer, Alexander and Bayen, Alexandre M.},
 doi = {10.1145/3325916},
 file = {/home/matt/Zotero/storage/R92RB6F5/Cabannes et al_2019_Regrets in Routing Networks.pdf},
 issn = {2374-0353},
 journal = {ACM Trans. Spatial Algorithms Syst.},
 number = {2},
 pages = {9:1--9:19},
 shorttitle = {Regrets in {{Routing Networks}}},
 title = {Regrets in {{Routing Networks}}: {{Measuring}} the {{Impact}} of {{Routing Apps}} in {{Traffic}}},
 volume = {5},
 year = {2019}
}

@inproceedings{caesar_nuscenes_2020,
 author = {Holger Caesar and
Varun Bankiti and
Alex H. Lang and
Sourabh Vora and
Venice Erin Liong and
Qiang Xu and
Anush Krishnan and
Yu Pan and
Giancarlo Baldan and
Oscar Beijbom},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/CaesarBLVLXKPBB20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.01164},
 pages = {11618--11628},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {nuScenes: {A} Multimodal Dataset for Autonomous Driving},
 url = {https://doi.org/10.1109/CVPR42600.2020.01164},
 year = {2020}
}

@article{cai_adaptive_2009,
 author = {Cai, C. and Wong, C. K. and Heydecker, B. G.},
 journal = {Transportation Research, Part C},
 number = {5},
 pages = {456--474},
 title = {Adaptive Traffic Signal Control Using Approximate Dynamic Programming},
 volume = {17},
 year = {2009}
}

@inproceedings{cai_zeroq_2020,
 author = {Yaohui Cai and
Zhewei Yao and
Zhen Dong and
Amir Gholami and
Michael W. Mahoney and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/CaiYDGMK20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.01318},
 pages = {13166--13175},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {ZeroQ: {A} Novel Zero Shot Quantization Framework},
 url = {https://doi.org/10.1109/CVPR42600.2020.01318},
 year = {2020}
}

@book{california_department_of_transportation_2000-2002_2002,
 author = {{California Department of Transportation}},
 title = {2000-2002 {{California Statewide Household Travel Survey}}},
 year = {2002}
}

@unpublished{california_department_of_transportation_2002_2003,
 author = {{California Department of Transportation}},
 title = {2002 {{HICOMP Report}}},
 year = {2003}
}

@techreport{california_department_of_transportation_2009_2009,
 author = {{California Department of Transportation}},
 title = {2009 {{Ten}}-{{Year State Highway Operation}} and {{Protection Plan}}},
 year = {2009}
}

@book{california_department_of_transportation_california_2013,
 author = {{California Department of Transportation}},
 title = {{{CALIFORNIA HIGH}}-{{OCCUPANCY VEHICLE LANE DEGRADATION ACTION PLAN}}},
 year = {2013}
}

@book{california_department_of_transportation_district_4_office_of_highway_operations_hov_2002,
 author = {{California Department of Transportation, District 4, Office of Highway Operations}},
 title = {{{HOV}} Lanes in the {{Bay Area}}},
 year = {2002}
}

@book{california_department_of_transportation_division_of_transportation_system_information_highway_2002,
 author = {{California Department of Transportation, Division of Transportation System Information}},
 title = {Highway {{Performance Monitoring System}}},
 year = {2002}
}

@book{california_department_of_transportation_strategic_2006,
 author = {{California Department of Transportation}},
 title = {Strategic {{Growth Plan}}},
 year = {2006}
}

@book{california_performance_reviewthe_government_for_the_people_for_a_change_inf04_2004,
 author = {{California Performance Review\textemdash The Government for the People for a Change}},
 title = {{{INF04 Performance Measures Are Needed}} in {{Traffic Operations}}},
 year = {2004}
}

@techreport{cambridge_systematics_inc_short-term_1994,
 author = {{Cambridge Systematics, Inc}},
 institution = {{U.S. Department of Transportation}},
 number = {DOT-T-95-05},
 title = {Short-{{Term Travel Model Improvements}}},
 year = {1994}
}

@book{cambridge_systematics_inc._twin_2001,
 author = {{Cambridge Systematics, Inc.}},
 title = {Twin {{Cities Ramp Meter Evaluation}}: {{Executive Summary}}},
 year = {2001}
}

@article{candes_introduction_2008,
 author = {Candes, E.J. and Wakin, M.B.},
 doi = {10.1109/MSP.2007.914731},
 file = {/home/matt/Zotero/storage/89KJ7EEV/CandesWatkinCS.pdf},
 issn = {1053-5888},
 journal = {IEEE Signal Processing Magazine},
 number = {2},
 pages = {21--30},
 title = {An {{Introduction To Compressive Sampling}}},
 volume = {25},
 year = {2008}
}

@article{cao_instance-aware_2021,
 author = {Cao, Jinkun and Wang, Xin and Darrell, Trevor and Yu, Fisher},
 journal = {ArXiv preprint},
 title = {Instance-{{Aware Predictive Navigation}} in {{Multi}}-{{Agent Environments}}},
 url = {https://arxiv.org/abs/2101.05893},
 volume = {abs/2101.05893},
 year = {2021}
}

@article{carion_end--end_2020,
 author = {Carion, Nicolas and Massa, Francisco and Synnaeve, Gabriel and Usunier, Nicolas and Kirillov, Alexander and Zagoruyko, Sergey},
 journal = {ArXiv preprint},
 title = {End-to-{{End Object Detection}} with {{Transformers}}},
 url = {https://arxiv.org/abs/2005.12872},
 volume = {abs/2005.12872},
 year = {2020}
}

@article{carlini_towards_2016,
 author = {Carlini, Nicholas and Wagner, David},
 journal = {ArXiv preprint},
 title = {Towards {{Evaluating}} the {{Robustness}} of {{Neural Networks}}},
 url = {https://arxiv.org/abs/1608.04644},
 volume = {abs/1608.04644},
 year = {2016}
}

@article{caron_particle_2007,
 author = {Caron, Franois and Davy, Manuel and Duflos, Emmanuel and Vanheeghe, Philippe},
 doi = {10.1109/TSP.2007.893914},
 file = {/home/matt/Zotero/storage/SF3F96U5/04203044.pdf},
 issn = {1053-587X},
 journal = {IEEE Transactions on Signal Processing},
 number = {6},
 pages = {2703--2719},
 shorttitle = {Particle {{Filtering}} for {{Multisensor Data Fusion With Switching Observation Models}}},
 title = {Particle {{Filtering}} for {{Multisensor Data Fusion With Switching Observation Models}}: {{Application}} to {{Land Vehicle Positioning}}},
 volume = {55},
 year = {2007}
}

@article{carrion_value_2012,
 abstract = {Travel time reliability is a fundamental factor in travel behavior. It represents the temporal uncertainty experienced by travelers in their movement between any two nodes in a network. The importance of the time reliability depends on the penalties incurred by the travelers. In road networks, travelers consider the existence of a trip travel time uncertainty in different choice situations (departure time, route, mode, and others). In this paper, a systematic review of the current state of research in travel time reliability, and more explicitly in the value of travel time reliability is presented. Moreover, a meta-analysis is performed in order to determine the reasons behind the discrepancy among the reliability estimates.},
 author = {Carrion, Carlos and Levinson, David},
 doi = {10.1016/j.tra.2012.01.003},
 file = {/home/matt/Zotero/storage/MGX5R8CF/Carrion and Levinson - 2012 - Value of travel time reliability A review of curr.pdf;/home/matt/Zotero/storage/AB6MQU6N/S0965856412000043.html},
 issn = {0965-8564},
 journal = {Transportation Research Part A: Policy and Practice},
 number = {4},
 pages = {720--741},
 shorttitle = {Value of Travel Time Reliability},
 title = {Value of Travel Time Reliability: {{A}} Review of Current Evidence},
 volume = {46},
 year = {2012}
}

@article{casas_spatially-aware_2019,
 author = {Casas, Sergio and Gulino, Cole and Liao, Renjie and Urtasun, Raquel},
 journal = {ArXiv preprint},
 title = {Spatially-{{Aware Graph Neural Networks}} for {{Relational Behavior Forecasting}} from {{Sensor Data}}},
 url = {https://arxiv.org/abs/1910.08233},
 volume = {abs/1910.08233},
 year = {2019}
}

@article{cascetta_fixed_2001,
 abstract = {},
 author = {Cascetta, E. and Postorino, M.},
 journal = {Transportation Science},
 keywords = {},
 number = {2},
 pages = {134--147},
 title = {Fixed Point Approaches to the Estimation of o/d Matrices Using Traffic Counts on Congested Networks},
 volume = {35},
 year = {2001}
}

@article{casella_rao-blackwellisation_1996,
 author = {Casella, George and Robert, Christian P.},
 doi = {10.1093/biomet/83.1.81},
 journal = {Biometrika},
 number = {1},
 pages = {81--94},
 title = {Rao-{{Blackwellisation}} of Sampling Schemes},
 volume = {83},
 year = {1996}
}

@article{cassandras_smart_2016,
 abstract = {The emerging prototype for a Smart City is one of an urban environment with a new generation of innovative services for transportation, energy distribution, healthcare, environmental monitoring, business, commerce, emergency response, and social activities. Enabling the technology for such a setting requires a viewpoint of Smart Cities as cyber-physical systems (CPSs) that include new software platforms and strict requirements for mobility, security, safety, privacy, and the processing of massive amounts of information. This paper identifies some key defining characteristics of a Smart City, discusses some lessons learned from viewing them as CPSs, and outlines some fundamental research issues that remain largely open.},
 author = {Cassandras, Christos G.},
 doi = {10.1016/J.ENG.2016.02.012},
 file = {/home/matt/Zotero/storage/9ISE2TJZ/Cassandras - 2016 - Smart Cities as Cyber-Physical Social Systems.pdf;/home/matt/Zotero/storage/V58XV36A/S2095809916309420.html},
 issn = {2095-8099},
 journal = {Engineering},
 number = {2},
 pages = {156--158},
 title = {Smart {{Cities}} as {{Cyber}}-{{Physical Social Systems}}},
 volume = {2},
 year = {2016}
}

@techreport{cassidy_empirical_2006,
 author = {Cassidy, M. J. and Daganzo, C. F. and Jang, K. and Chung, K.},
 institution = {{Institute of Transportation Studies, University of California, Berkeley}},
 number = {UCB-ITS-RR-2006-6},
 title = {Empirical {{Reassessment}} of {{Traffic Operations}}: {{Freeway Bottlenecks}} and the {{Case}} for {{HOV Lanes}}},
 year = {2006}
}

@article{cassidy_freeway_2003,
 author = {Cassidy, M. J.},
 journal = {Transportation Research Record},
 pages = {1--5},
 title = {Freeway On-Ramp Metering, Delay Savings and the Diverge Bottleneck},
 volume = {1856},
 year = {2003}
}

@article{cassidy_m._traffic_1999,
 author = {{Cassidy, M.} and Bertini, R.},
 journal = {Transportation Research B},
 pages = {25--42},
 title = {Some Traffic Features at Freeway Bottlenecks},
 volume = {33B},
 year = {1999}
}

@unpublished{cassidy_m.j._increasing_2004,
 author = {{Cassidy, M.J.} and Rudjanakanoknad, J.},
 title = {Increasing Capacity of an Isolated Merge by Metering Its On-Ramp},
 year = {2004}
}

@article{cassidy_problem_2015,
 author = {Cassidy, Michael J. and Kim, Kwangho and Ni, Wei and Gu, Weihua},
 doi = {http://dx.doi.org/10.1016/j.tra.2015.07.001},
 issn = {0965-8564},
 journal = {Transportation Research Part A: Policy and Practice},
 pages = {307--319},
 title = {A Problem of Limited-Access Special Lanes. {{Part I}}: {{Spatiotemporal}} Studies of Real Freeway Traffic},
 volume = {80},
 year = {2015}
}

@article{cassidy_smoothing_2010,
 author = {Cassidy, Michael J. and Jang, Kitae and Daganzo, Carlos F.},
 doi = {10.1016/j.tra.2009.11.002},
 file = {/home/matt/Zotero/storage/YTWY78MJ/cassidy_jang_daganzo_smoothing_effect_2010.pdf},
 issn = {09658564},
 journal = {Transportation Research Part A: Policy and Practice},
 language = {en},
 number = {2},
 pages = {65--75},
 title = {The Smoothing Effect of Carpool Lanes on Freeway Bottlenecks},
 volume = {44},
 year = {2010}
}

@incollection{cassidy_spatiotemporal_2009,
 abstract = {The paper explores some of the impacts of setting aside road lanes for the exclusive use of select vehicle classes. We examine first the case of lanes that are reserved for carpools, and then extend the analysis to bus-only lanes. In doing so, the paper makes three contributions. The first is methodological: it illustrates the importance of analyzing freeway data in full spatiotemporal detail. The second is physical: data reveal that carpool lanes are not as damaging as previously reported. In fact, these lanes are found to smooth traffic in adjacent lanes so much (by diminishing disruptive vehicle interactions near bottlenecks) that even substantially underutilized carpool lanes can increase bottleneck discharge flows. The third contribution is theoretical: it uses the smoothing phenomenon to show how the judicious deployment of bus-only lanes on freeways and city streets can favorably affect not just buses, but also cars.},
 address = {{Boston, MA}},
 author = {Cassidy, Michael J. and Daganzo, Carlos F. and Jang, Kitae and Chung, Koohong},
 booktitle = {Transportation and {{Traffic Theory}} 2009: {{Golden Jubilee}}: {{Papers}} Selected for Presentation at {{ISTTT18}}},
 editor = {Lam, William H. K. and Wong, S. C. and Lo, Hong K.},
 isbn = {978-1-4419-0820-9},
 pages = {57--74},
 publisher = {{Springer US}},
 title = {Spatiotemporal {{Effects}} of {{Segregating Different Vehicle Classes}} on {{Separate Lanes}}},
 year = {2009}
}

@article{caveney_before_2003,
 author = {Caveney, Derek and Dickmanns, Dirk and Hedrick, J Karl},
 journal = {Automatisierungstechnik},
 number = {5},
 pages = {230--238},
 title = {Before the Controller: {{A}} Multiple Target Tracking Routine for Driver Assistance Systems},
 volume = {51},
 year = {2003}
}

@techreport{cayford_netcell_1997,
 author = {Cayford, R. and Lin, W.-H. and Daganzo, C. F.},
 institution = {{California PATH, University of California, Berkeley, CA 94720}},
 number = {UCB-ITS-PRR-97-23},
 title = {The {{NETCELL}} Simulation Package: Technical Description.},
 year = {1997}
}

@article{ceder_algorithm_2001,
 abstract = {a self-tuning system for controlling signalized intersections in undersaturated and oversaturated conditions is depicted. the green allocation problem becomes a linear programming problem},
 author = {Ceder, A. and Reshetnik, I.},
 journal = {Journal of the Operational Research Society},
 keywords = {},
 number = {6},
 pages = {615--622},
 title = {An {{Algorithm}} to {{Minimize Queues}} at {{Signalized Intersections}}},
 volume = {52},
 year = {2001}
}

@inproceedings{cettolo_report_2014,
 abstract = {The paper overviews the 11th evaluation campaign organized by the IWSLT workshop. The 2014 evaluation offered multiple tracks on lecture transcription and translation based on the TED Talks corpus. In particular, this year IWSLT included three automatic speech recognition tracks, on English, German and Italian, five speech translation tracks, from English to French, English to German, German to English, English to Italian, and Italian to English, and five text translation track, also from English to French, English to German, German to English, English to Italian, and Italian to English. In addition to the official tracks, speech and text translation optional tracks were offered, globally involving 12 other languages: Arabic, Spanish, Portuguese (B), Hebrew, Chinese, Polish, Persian, Slovenian, Turkish, Dutch, Romanian, Russian. Overall, 21 teams participated in the evaluation, for a total of 76 primary runs submitted. Participants were also asked to submit runs on the 2013 test set (progress test set), in order to measure the progress of systems with respect to the previous year. All runs were evaluated with objective metrics, and submissions for two of the official text translation tracks were also evaluated with human post-editing.},
 author = {Cettolo, Mauro and Niehues, Jan and Stuker, Sebastian and Bentivogli, Luisa and Federico, Marcello},
 booktitle = {Proceedings of the {{International Workshop}} in {{Spoken Language Translation}}},
 file = {/home/matt/Zotero/storage/SJWTDHI2/Cettolo et al. - 2014 - Report on the 11th IWSLT Evaluation Campaign, IWSL.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Report on the 11th {{IWSLT Evaluation Campaign}}, {{IWSLT}} 2014},
 year = {2014}
}

@article{ceylan_reserve_2004,
 abstract = {reserve or spare capacity available to accommodate the inevitable day-to-day fluctuations in demand},
 author = {Ceylan, H. and Bell, M. G. H.},
 journal = {Journal of Intelligent Transportation Systems},
 pages = {87--99},
 title = {Reserve {{Capacity}} for a {{Road Network Under Optimized Fixed Time Traffic Signal Control}}},
 volume = {8},
 year = {2004}
}

@techreport{chada_effectiveness_2002,
 address = {{University of South Florida}},
 author = {Chada, S. and Newland, R.},
 institution = {{National Center For Transit Research (NCTR)}},
 number = {NCTR-416-04},
 title = {Effectiveness of {{Bus Signal Priority}}: {{Final Report}}},
 year = {2002}
}

@article{chai_multipath_2019,
 author = {Chai, Yuning and Sapp, Benjamin and Bansal, Mayank and Anguelov, Dragomir},
 journal = {ArXiv preprint},
 title = {{{MultiPath}}: {{Multiple Probabilistic Anchor Trajectory Hypotheses}} for {{Behavior Prediction}}},
 url = {https://arxiv.org/abs/1910.05449},
 volume = {abs/1910.05449},
 year = {2019}
}

@inproceedings{Chakraborty_2019_CVPR_Workshops,
 author = {Chakraborty, Rudrasis and Wang, Jiayun and Yu, Stella X.},
 booktitle = {The {{IEEE}} Conference on Computer Vision and Pattern Recognition ({{CVPR}}) Workshops},
 file = {/home/matt/Zotero/storage/YBVQCTWV/Chakraborty et al. - 2019 - Sur-real frechet mean and distance transform for .pdf},
 title = {Sur-Real: Frechet Mean and Distance Transform for Complex-Valued Deep Learning},
 year = {2019}
}

@article{chalaki_zero-shot_2019,
 author = {Chalaki, Behdad and Beaver, Logan E. and Remer, Ben and Jang, Kathy and Vinitsky, Eugene and Bayen, Alexandre M. and Malikopoulos, Andreas A.},
 journal = {ArXiv preprint},
 title = {Zero-{{Shot Autonomous Vehicle Policy Transfer}}: {{From Simulation}} to {{Real}}-{{World}} via {{Adversarial Learning}}},
 url = {https://arxiv.org/abs/1903.05252},
 volume = {abs/1903.05252},
 year = {2019}
}

@article{chamberland_decentralized_2003,
 author = {Chamberland, J. F. and Veeravalli, V. V.},
 doi = {10.1109/TSP.2002.806982},
 issn = {1053-587X},
 journal = {IEEE Transactions on Signal Processing},
 number = {2},
 pages = {407--416},
 title = {Decentralized Detection in Sensor Networks},
 volume = {51},
 year = {2003}
}

@inproceedings{chan_everybody_2019,
 author = {Caroline Chan and
Shiry Ginosar and
Tinghui Zhou and
Alexei A. Efros},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/ChanGZE19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00603},
 pages = {5932--5941},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Everybody Dance Now},
 url = {https://doi.org/10.1109/ICCV.2019.00603},
 year = {2019}
}

@inproceedings{chan_everybody_nodate,
 author = {Caroline Chan and
Shiry Ginosar and
Tinghui Zhou and
Alexei A. Efros},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/ChanGZE19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00603},
 pages = {5932--5941},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Everybody Dance Now},
 url = {https://doi.org/10.1109/ICCV.2019.00603},
 year = {2019}
}

@inproceedings{chan_measuring_2020,
 author = {Stephanie C. Y. Chan and
Samuel Fishman and
Anoop Korattikara and
John Canny and
Sergio Guadarrama},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ChanFKCG20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Measuring the Reliability of Reinforcement Learning Algorithms},
 url = {https://openreview.net/forum?id=SJlpYJBKvH},
 year = {2020}
}

@techreport{chang_review_2008,
 author = {Chang, Mark and Wiegmann, John and Smith, Andrew and Bilotto, Claudia},
 institution = {{Federal Highway Administration}},
 number = {FHWA-HOP-09-029},
 title = {A {{Review}} of {{HOV Lane Performance}} and {{Policy Options}} in the {{United States}}},
 type = {Report},
 year = {2008}
}

@article{chardon_plate_2011,
 author = {Chardon, G. and Leblanc, A. and Daudet, L.},
 doi = {10.1016/j.jsv.2011.07.003},
 file = {/home/matt/Zotero/storage/D6IB535G/CS_plate_wave.pdf},
 issn = {0022460X},
 journal = {Journal of Sound and Vibration},
 language = {en},
 number = {23},
 pages = {5678--5689},
 title = {Plate Impulse Response Spatial Interpolation with Sub-{{Nyquist}} Sampling},
 volume = {330},
 year = {2011}
}

@article{chatterji_oracle_2020,
 author = {Chatterji, Niladri S. and Bartlett, Peter L. and Long, Philip M.},
 journal = {ArXiv preprint},
 title = {Oracle Lower Bounds for Stochastic Gradient Sampling Algorithms},
 url = {https://arxiv.org/abs/2002.00291},
 volume = {abs/2002.00291},
 year = {2020}
}

@inproceedings{chebotar_combining_2017,
 author = {Yevgen Chebotar and
Karol Hausman and
Marvin Zhang and
Gaurav S. Sukhatme and
Stefan Schaal and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ChebotarHZSSL17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {703--711},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Combining Model-Based and Model-Free Updates for Trajectory-Centric
Reinforcement Learning},
 url = {http://proceedings.mlr.press/v70/chebotar17a.html},
 volume = {70},
 year = {2017}
}

@article{chen_alchemy_2019,
 author = {Chen, Guangyong and Chen, Pengfei and Hsieh, Chang-Yu and Lee, Chee-Kong and Liao, Benben and Liao, Renjie and Liu, Weiwen and Qiu, Jiezhong and Sun, Qiming and Tang, Jie and Zemel, Richard and Zhang, Shengyu},
 journal = {ArXiv preprint},
 title = {Alchemy: {{A Quantum Chemistry Dataset}} for {{Benchmarking AI Models}}},
 url = {https://arxiv.org/abs/1906.09427},
 volume = {abs/1906.09427},
 year = {2019}
}

@inproceedings{chen_best_2018,
 address = {Melbourne, Australia},
 author = {Chen, Mia Xu  and
Firat, Orhan  and
Bapna, Ankur  and
Johnson, Melvin  and
Macherey, Wolfgang  and
Foster, George  and
Jones, Llion  and
Schuster, Mike  and
Shazeer, Noam  and
Parmar, Niki  and
Vaswani, Ashish  and
Uszkoreit, Jakob  and
Kaiser, Lukasz  and
Chen, Zhifeng  and
Wu, Yonghui  and
Hughes, Macduff},
 booktitle = {Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
 doi = {10.18653/v1/P18-1008},
 pages = {76--86},
 publisher = {Association for Computational Linguistics},
 title = {The Best of Both Worlds: Combining Recent Advances in Neural Machine Translation},
 url = {https://aclanthology.org/P18-1008},
 year = {2018}
}

@article{chen_c._causes_2001,
 author = {{Chen, C.} and Jia, Z. and Varaiya, P.},
 journal = {IEEE Control Systems Magazine},
 number = {4},
 pages = {26--33},
 title = {Causes and Cures of Highway Congestion},
 volume = {21},
 year = {2001}
}

@inproceedings{chen_deep_2019,
 abstract = {The development of a powertrain controller for automated driving systems (ADS) using a learning-based approach is presented in this paper. The goal is to create an intelligent agent to learn from driving experience and integrate the operation of each powertrain unit to benefit vehicle driving performance and efficiency. The feature of reinforcement learning (RL) that the agent interacts with environment to improve its policy mimics the learning process of a human driver. Therefore, we have adopted the RL methodology to train the agent for the intelligent powertrain control problem in this study. In this paper, a vehicle powertrain control strategist named Intelligent Powertrain Agent (IPA) based on deep Q-learning network (DQN) is proposed. In the application for an ADS, the IPA receives trajectory maneuver demands from a decision-making module of an ADS, observes the vehicle states and driving environment as the inputs, and outputs the control commands to the powertrain system. As a case study, the IPA is applied to a parallel hybrid vehicle to demonstrate its capability. Through the training process, the IPA is able to learn how to operate powertrain units in an integrated way to deal with varied driving conditions, and vehicle's speed chasing ability and power management are improved along with its driving experience.},
 address = {{Auckland, New Zealand}},
 author = {Chen, I-Ming and Zhao, Cong and Chan, Ching-Yao},
 booktitle = {2019 {{IEEE Intelligent Transportation Systems Conference}} ({{ITSC}})},
 doi = {10.1109/ITSC.2019.8917076},
 file = {/home/matt/Zotero/storage/PG5IQPPR/Chen et al. - 2019 - A Deep Reinforcement Learning-Based Approach to In.pdf},
 isbn = {978-1-5386-7024-8},
 language = {en},
 pages = {2620--2625},
 publisher = {{IEEE}},
 title = {A {{Deep Reinforcement Learning}}-{{Based Approach}} to {{Intelligent Powertrain Control}} for {{Automated Vehicles}}},
 year = {2019}
}

@article{chen_detecting_2003,
 abstract = {Single-loop detectors provide the most abundant source of traffic data in California, but loop data samples are often missing or invalid. A method is described that detects bad data samples and imputes missing or bad samples to form a complete grid of clean data, in real time. The diagnostics algorithm and the imputation algorithm that implement this method are operational on 14,871 loops in six districts of the California Department of Transportation. The diagnostics algorithm detects bad (malfunctioning) single-loop detectors from their volume and occupancy measurements. Its novelty is its use of time series of many samples, instead of basing decisions on single samples, as in previous approaches. The imputation algorithm models the relationship between neighboring loops as linear and uses linear regression to estimate the value of missing or bad samples. This gives a better estimate than previous methods because it uses historical data to learn how pairs of neighboring loops behave. Detection of bad loops and imputation of loop data are important because they allow algorithms that use loop data to perform analysis without requiring them to compensate for missing or incorrect data samples.},
 author = {Chen, Chao and Kwon, Jaimyoung and Rice, John and Skabardonis, Alexander and Varaiya, Pravin},
 doi = {10.3141/1855-20},
 file = {/home/matt/Zotero/storage/2NU6SRME/Chen et al. - 2003 - Detecting Errors and Imputing Missing Data for Sin.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 language = {en},
 number = {1},
 pages = {160--167},
 title = {Detecting {{Errors}} and {{Imputing Missing Data}} for {{Single}}-{{Loop Surveillance Systems}}},
 volume = {1855},
 year = {2003}
}

@techreport{chen_development_2004,
 address = {{Irvine, California}},
 author = {Chen, A. and Chootinan, P. and Recker, W. and Zhang, H. M.},
 institution = {{Institute of Transportation Studies, University of California}},
 number = {PATH Research Report UCI-ITS-TS-WP-04-13},
 title = {Development of a Path Flow Estimator for Deriving Steady-State and Time-Dependent Origin-Destination Trip Tables},
 year = {2004}
}

@article{chen_evidence_2013,
 author = {Chen, Y. and Ebenstein, A. and Greenstone, M. and Li, H.},
 journal = {Proc. National Academy of Sciences},
 number = {32},
 pages = {12936--12941},
 title = {Evidence on the Impact of Sustained Exposure to Air Pollution on Life Expectancy from {{China}}'s {{Huai River}} Policy},
 volume = {112},
 year = {2013}
}

@inproceedings{chen_execution-guided_2019,
 author = {Xinyun Chen and
Chang Liu and
Dawn Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ChenLS19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Execution-Guided Neural Program Synthesis},
 url = {https://openreview.net/forum?id=H1gfOiAqYm},
 year = {2019}
}

@inproceedings{chen_infogan_2016,
 author = {Xi Chen and
Yan Duan and
Rein Houthooft and
John Schulman and
Ilya Sutskever and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/ChenCDHSSA16.bib},
 booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
on Neural Information Processing Systems 2016, December 5-10, 2016,
Barcelona, Spain},
 editor = {Daniel D. Lee and
Masashi Sugiyama and
Ulrike von Luxburg and
Isabelle Guyon and
Roman Garnett},
 pages = {2172--2180},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {InfoGAN: Interpretable Representation Learning by Information Maximizing
Generative Adversarial Nets},
 url = {https://proceedings.neurips.cc/paper/2016/hash/7c9d0b1f96aebd7b5eca8c3edaa19ebb-Abstract.html},
 year = {2016}
}

@article{chen_interpretable_2020,
 author = {Chen, Jianyu and Li, Shengbo Eben and Tomizuka, Masayoshi},
 journal = {ArXiv preprint},
 title = {Interpretable {{End}}-to-End {{Urban Autonomous Driving}} with {{Latent Deep Reinforcement Learning}}},
 url = {https://arxiv.org/abs/2001.08726},
 volume = {abs/2001.08726},
 year = {2020}
}

@unpublished{chen_max_2001,
 author = {Chen, C. and Varaiya, P.},
 title = {Max Flow in {{D12}} Occurs at 60 Mph},
 year = {2001}
}

@inproceedings{chen_measuring_2020,
 author = {Deli Chen and
Yankai Lin and
Wei Li and
Peng Li and
Jie Zhou and
Xu Sun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/ChenLLLZS20.bib},
 booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
2020, The Thirty-Second Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
February 7-12, 2020},
 pages = {3438--3445},
 publisher = {{AAAI} Press},
 timestamp = {Wed, 02 Dec 2020 00:00:00 +0100},
 title = {Measuring and Relieving the Over-Smoothing Problem for Graph Neural
Networks from the Topological View},
 url = {https://aaai.org/ojs/index.php/AAAI/article/view/5747},
 year = {2020}
}

@inproceedings{chen_multi-label_2019,
 author = {Zhao{-}Min Chen and
Xiu{-}Shen Wei and
Peng Wang and
Yanwen Guo},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/ChenWWG19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00532},
 pages = {5177--5186},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 16 Nov 2020 00:00:00 +0100},
 title = {Multi-Label Image Recognition With Graph Convolutional Networks},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Chen\_Multi-Label\_Image\_Recognition\_With\_Graph\_Convolutional\_Networks\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{chen_neural_2018,
 author = {Tian Qi Chen and
Yulia Rubanova and
Jesse Bettencourt and
David Duvenaud},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/ChenRBD18.bib},
 booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
on Neural Information Processing Systems 2018, NeurIPS 2018, December
3-8, 2018, Montr{\'{e}}al, Canada},
 editor = {Samy Bengio and
Hanna M. Wallach and
Hugo Larochelle and
Kristen Grauman and
Nicol{\`{o}} Cesa{-}Bianchi and
Roman Garnett},
 pages = {6572--6583},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Neural Ordinary Differential Equations},
 url = {https://proceedings.neurips.cc/paper/2018/hash/69386f6bb1dfed68692a24c8686939b9-Abstract.html},
 year = {2018}
}

@article{chen_new_2020,
 author = {Chen, Yinbo and Wang, Xiaolong and Liu, Zhuang and Xu, Huijuan and Darrell, Trevor},
 journal = {ArXiv preprint},
 title = {A {{New Meta}}-{{Baseline}} for {{Few}}-{{Shot Learning}}},
 url = {https://arxiv.org/abs/2003.04390},
 volume = {abs/2003.04390},
 year = {2020}
}

@article{chen_real-time_2004,
 author = {Chen, Yunqiang and Rui, Yong},
 doi = {10.1109/JPROC.2003.823146},
 issn = {0018-9219},
 journal = {Proc. of IEEE},
 number = {3},
 pages = {485--494},
 title = {Real-Time Speaker Tracking Using Particle Filter Sensor Fusion},
 volume = {92},
 year = {2004}
}

@article{chen_refit_2020,
 abstract = {Deep neural networks (DNNs) have achieved tremendous success in various fields; however, training these models from scratch could be computationally expensive and requires a lot of training data. Recent work has explored different watermarking techniques to protect the pre-trained deep neural networks from potential copyright infringements. Although several existing techniques could effectively embed such watermarks into the DNNs, they could be vulnerable to adversaries who aim at removing the watermarks.},
 archiveprefix = {arXiv},
 author = {Chen, Xinyun and Wang, Wenxiao and Bender, Chris and Ding, Yiming and Jia, Ruoxi and Li, Bo and Song, Dawn},
 eprint = {1911.07205},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/PR2DQLQL/Chen et al. - 2020 - REFIT a Unified Watermark Removal Framework for D.pdf},
 journal = {ICML 2019 Workshop on Security and Privacy of Machine Learning},
 keywords = {⛔ No DOI found},
 language = {en},
 shorttitle = {{{REFIT}}},
 title = {{{REFIT}}: A {{Unified Watermark Removal Framework}} for {{Deep Learning Systems}} with {{Limited Data}}},
 year = {2020}
}

@article{chen_similarity-based_2009,
 abstract = {This paper reviews and extends the field of similarity-based classification, presenting new analyses, algorithms, data sets, and a comprehensive set of experimental results for a rich collection of classification problems. Specifically, the generalizability of using similarities as features is analyzed, design goals and methods for weighting nearest-neighbors for similarity-based learning are proposed, and different methods for consistently converting similarities into kernels are compared. Experiments on eight real data sets compare eight approaches and their variants to similarity-based learning.},
 author = {Chen, Yihua and Garcia, Eric K and Gupta, Maya R and Rahimi, Ali and Cazzanti, Luca},
 file = {/home/matt/Zotero/storage/ZVKFHAGL/Chen et al. - Similarity-based Classiﬁcation Concepts and Algor.pdf},
 journal = {Journal of Machine Learning Research},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {747--776},
 title = {Similarity-Based {{Classification}}: {{Concepts}} and {{Algorithms}}},
 volume = {10},
 year = {2009}
}

@article{chen_systematic_2004,
 author = {Chen, C. and Skabardonis, A. and Varaiya, P.},
 journal = {Transportation Research Record},
 pages = {46--52},
 title = {Systematic Identification of Freeway Bottlenecks},
 volume = {1867},
 year = {2004}
}

@article{chen_tracking_2019,
 abstract = {Emotion recognition is an essential human ability critical for social functioning. It is widely assumed that identifying facial expression is the key to this, and models of emotion recognition have mainly focused on facial and bodily features in static, unnatural conditions. We developed a method called affective tracking to reveal and quantify the enormous contribution of visual context to affect (valence and arousal) perception. When characters' faces and bodies were masked in silent videos, viewers inferred the affect of the invisible characters successfully and in high agreement based solely on visual context. We further show that the context is not only sufficient but also necessary to accurately perceive human affect over time, as it provides a substantial and unique contribution beyond the information available from face and body. Our method (which we have made publicly available) reveals that emotion recognition is, at its heart, an issue of context as much as it is about faces.},
 author = {Chen, Zhimin and Whitney, David},
 doi = {10.1073/pnas.1812250116},
 file = {/home/matt/Zotero/storage/EYIWEP96/Chen and Whitney - 2019 - Tracking the affective state of unseen persons.pdf},
 issn = {0027-8424, 1091-6490},
 journal = {Proceedings of the National Academy of Sciences},
 language = {en},
 number = {15},
 pages = {7559--7564},
 title = {Tracking the Affective State of Unseen Persons},
 volume = {116},
 year = {2019}
}

@inproceedings{chen_training_2008,
 author = {Jianhui Chen and
Jieping Ye},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ChenY08.bib},
 booktitle = {Machine Learning, Proceedings of the Twenty-Fifth International Conference
{(ICML} 2008), Helsinki, Finland, June 5-9, 2008},
 doi = {10.1145/1390156.1390174},
 editor = {William W. Cohen and
Andrew McCallum and
Sam T. Roweis},
 pages = {136--143},
 publisher = {{ACM}},
 series = {{ACM} International Conference Proceeding Series},
 timestamp = {Tue, 06 Nov 2018 00:00:00 +0100},
 title = {Training {SVM} with indefinite kernels},
 url = {https://doi.org/10.1145/1390156.1390174},
 volume = {307},
 year = {2008}
}

@inproceedings{cheng_human_2019,
 abstract = {Human motion prediction is an important component to facilitate human robot interaction. Robots need to accurately predict human's future movement in order to safely plan its own motion trajectories and efficiently collaborate with humans. Many recent approaches predict human's movement using deep learning methods, such as recurrent neural networks. However, existing methods lack the ability to adapt to time-varying human behaviors, and many of them do not quantify uncertainties in the prediction. This paper proposes an approach that uses a semi-adaptable neural network for human motion prediction, and provides uncertainty bounds of the predictions in real time. In particular, a neural network is trained offline to represent the human motion transition model, and then recursive least square parameter adaptation algorithm (RLS-PAA) is adopted for online parameter adaptation of the neural network and for uncertainty estimation. Experiments on several human motion datasets verify that the proposed method significantly outperforms the state-of-the-art approach in terms of prediction accuracy and computation efficiency.},
 author = {Cheng, Yujiao and Zhao, Weiye and Liu, Changliu and Tomizuka, Masayoshi},
 booktitle = {2019 {{American Control Conference}} ({{ACC}})},
 file = {/home/matt/Zotero/storage/IM9CVXJS/Cheng et al. - 2019 - Human Motion Prediction using Semi-adaptable Neura.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {4884--4890},
 title = {Human {{Motion Prediction}} Using {{Semi}}-Adaptable {{Neural Networks}}},
 year = {2019}
}

@article{cheng_three_2016,
 abstract = {Three broad questions about China's ``Belt and Road Initiative'' are raised. First, what are likely to be the real objectives behind the Initiative? Second, are investment and trade, considered the ``major task'' of the Initiative by China, to be driven by market-based transactions, or will they be a form of foreign aid that is not based on economic calculation of gains and losses? Third, which of the 60 or so countries in Asia, Europe and Africa along the Belt and Road will likely be the Initiative's priority targets of economic cooperation?},
 author = {Cheng, Leonard K.},
 doi = {10.1016/j.chieco.2016.07.008},
 file = {/home/matt/Zotero/storage/7VNHX4XR/Cheng - 2016 - Three questions on China's “Belt and Road Initiati.pdf;/home/matt/Zotero/storage/WNJ8XVD3/S1043951X16300797.html},
 issn = {1043-951X},
 journal = {China Economic Review},
 pages = {309--313},
 title = {Three Questions on {{China}}'s ``{{Belt}} and {{Road Initiative}}''},
 volume = {40},
 year = {2016}
}

@inproceedings{cheung_superposition_2019,
 author = {Brian Cheung and
Alexander Terekhov and
Yubei Chen and
Pulkit Agrawal and
Bruno A. Olshausen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/CheungTCAO19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {10867--10876},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Superposition of many models into one},
 url = {https://proceedings.neurips.cc/paper/2019/hash/4c7a167bb329bd92580a99ce422d6fa6-Abstract.html},
 year = {2019}
}

@article{cheung_traffic_2005,
 author = {Cheung, S. Y. and Coleri, S. and Dundar, B. and Ganesh, S. and {C-W. Tan} and Varaiya, P.},
 journal = {Transportation Research Record},
 number = {1917},
 pages = {173--181},
 title = {Traffic {{Measurement}} and {{Vehicle Classification}} with a {{Single Magnetic Sensor}}},
 year = {2005}
}

@article{chiang_learning_2018,
 author = {Chiang, Hao-Tien Lewis and Faust, Aleksandra and Fiser, Marek and Francis, Anthony},
 journal = {ArXiv preprint},
 title = {Learning {{Navigation Behaviors End}}-to-{{End}} with {{AutoRL}}},
 url = {https://arxiv.org/abs/1809.10124},
 volume = {abs/1809.10124},
 year = {2018}
}

@book{chicago_department_of_transportation_chicago_2012,
 author = {{Chicago Department of Transportation}},
 title = {Chicago {{Streets}} for {{Cycling Plan}} 2020},
 year = {2012}
}

@article{chin_one_2020,
 author = {Chin, Ting-Wu and Chuang, Pierce I.-Jen and Chandra, Vikas and Marculescu, Diana},
 journal = {ArXiv preprint},
 title = {One {{Weight Bitwidth}} to {{Rule Them All}}},
 url = {https://arxiv.org/abs/2008.09916},
 volume = {abs/2008.09916},
 year = {2020}
}

@techreport{chin_temporary_2002,
 address = {{National Transportation Research Center, Knowville, TN 37932}},
 author = {Chin, S. M. and Franzese, O. and Greene, D. L. and {H.L.Hwang} and Gibson, R. C.},
 institution = {{Oak Ridge National Laboragtory}},
 number = {ORNL/TM-2002/3},
 title = {Temporary Losses of Highway Capacity and Impacts on Performance},
 year = {2002}
}

@misc{chollet2015keras,
 author = {Chollet, Fran{\c c}ois and others},
 howpublished = {https://keras.io},
 keywords = {⛔ No DOI found},
 title = {Keras},
 year = {2015}
}

@inproceedings{choromanski_rethinking_2021,
 author = {Krzysztof Marcin Choromanski and
Valerii Likhosherstov and
David Dohan and
Xingyou Song and
Andreea Gane and
Tam{\'{a}}s Sarl{\'{o}}s and
Peter Hawkins and
Jared Quincy Davis and
Afroz Mohiuddin and
Lukasz Kaiser and
David Benjamin Belanger and
Lucy J. Colwell and
Adrian Weller},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ChoromanskiLDSG21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Rethinking Attention with Performers},
 url = {https://openreview.net/forum?id=Ua6zuk0WRH},
 year = {2021}
}

@inproceedings{chou_backstepping-based_2019,
 abstract = {The time-gap regulation problem for a cascaded system consisting of platooned automated vehicles following a leading non-automated vehicle is investigated in this article. Under the assumption of uniform boundedness of the acceleration of the leading vehicle, a control design scheme is proposed via an extension of integral backstepping control method, where additional terms that counter the impact due to the speed change of the non-automated vehicle are used. Each automated vehicle is actuated by one backstepping controller, demonstrated by a recursive control design procedure based on induction. As a result, both the time-gap error and the speed error between each pair of consecutive vehicles are proven to be ultimately bounded by some constants that can be tuned to be arbitrarily close to zero. In particular, the regulated time-gap guarantees enough time for the following vehicle in each pair to react to the velocity change of its preceding vehicle. Simulation is carried out to validate the proposed controllers.},
 author = {Chou, F. and Tang, S. and Lu, X. and Bayen, A.},
 booktitle = {2019 {{American Control Conference}} ({{ACC}})},
 file = {/home/matt/Zotero/storage/2X68Y6I5/Chou et al_2019_Backstepping-Based Time-Gap Regulation for Platoons.pdf;/home/matt/Zotero/storage/BQT7ZNWF/8814914.html},
 pages = {730--735},
 title = {Backstepping-{{Based Time}}-{{Gap Regulation}} for {{Platoons}}},
 year = {2019}
}

@inproceedings{chowdhuri_multinet_2019,
 abstract = {Autonomous driving requires operation in different behavioral modes ranging from lane following and intersection crossing to turning and stopping. However, most existing deep learning approaches to autonomous driving do not consider the behavioral mode in the training strategy. This paper describes a technique for learning multiple distinct behavioral modes in a single deep neural network through the use of multi-modal multi-task learning. We study the effectiveness of this approach, denoted MultiNet, using self-driving model cars for driving in unstructured environments such as sidewalks and unpaved roads. Using labeled data from over one hundred hours of driving our fleet of 1/10th scale model cars, we trained different neural networks to predict the steering angle and driving speed of the vehicle in different behavioral modes. We show that in each case, MultiNet networks outperform networks trained on individual modes while using a fraction of the total number of parameters.},
 author = {Chowdhuri, S. and Pankaj, T. and Zipser, K.},
 booktitle = {2019 {{IEEE Winter Conference}} on {{Applications}} of {{Computer Vision}} ({{WACV}})},
 doi = {10.1109/WACV.2019.00164},
 file = {/home/matt/Zotero/storage/RSH6NK73/Chowdhuri et al. - 2019 - MultiNet Multi-Modal Multi-Task Learning for Auto.pdf;/home/matt/Zotero/storage/QPDXBZPK/8658798.html},
 pages = {1496--1504},
 shorttitle = {{{MultiNet}}},
 title = {{{MultiNet}}: {{Multi}}-{{Modal Multi}}-{{Task Learning}} for {{Autonomous Driving}}},
 year = {2019}
}

@article{chu_new_2013,
 author = {Chu, J.},
 journal = {MIT News Office},
 title = {New Algorithm Finds Best Routes for One-Way Car Sharing},
 year = {2013}
}

@article{ciuffo_thirty_2012,
 abstract = {Researchers and practitioners commonly use car-following models for road traffic studies. Although dozens of models have been presented so far, the one proposed by Peter G. Gipps in 1981 is still one of the most extensively used. However, many features of the model are still not well known or neglected in common applications. In this context, the current study summarizes and analyzes the main findings available in the scientific literature for the Gipps' car-following model and introduces some of its novel features that may improve its capability to reproduce real trajectory data. In particular, the structure of the acceleration component of the model is analytically investigated for what concerns the meaning of some parameters that in common practice are usually kept to some empirically derived fixed values. Possible versions of Gipps' model are presented, and their performance to reproduce real vehicle trajectories is evaluated and compared. The results achieved show the necessity for these parameters to be calibrated to improve the model's predictive capabilities.},
 author = {Ciuffo, Biagio and Punzo, Vincenzo and Montanino, Marcello},
 doi = {10.3141/2315-10},
 file = {/home/matt/Zotero/storage/6P5V6VIY/Ciuffo et al. - 2012 - Thirty Years of Gipps’ Car-Following Model Applic.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 language = {en},
 number = {1},
 pages = {89--99},
 shorttitle = {Thirty {{Years}} of {{Gipps}}' {{Car}}-{{Following Model}}},
 title = {Thirty {{Years}} of {{Gipps}}' {{Car}}-{{Following Model}}: {{Applications}}, {{Developments}}, and {{New Features}}},
 volume = {2315},
 year = {2012}
}

@article{clarkson_uniformly_1936,
 author = {Clarkson, James A.},
 doi = {10.1090/S0002-9947-1936-1501880-4},
 file = {/home/matt/Zotero/storage/M4X2Y52G/Clarkson - 1936 - Uniformly convex spaces.pdf},
 issn = {0002-9947},
 journal = {Transactions of the American Mathematical Society},
 language = {en},
 number = {3},
 pages = {396--396},
 title = {Uniformly Convex Spaces},
 volume = {40},
 year = {1936}
}

@article{claudel_convex_2011,
 author = {Claudel, Christian G. and Bayen, Alexandre M.},
 doi = {10.1137/090778754},
 file = {/home/matt/Zotero/storage/5RS9WAMQ/ClaudelBayenConvexAssimilation.pdf},
 issn = {0363-0129, 1095-7138},
 journal = {SIAM Journal on Control and Optimization},
 language = {en},
 number = {2},
 pages = {383--402},
 title = {Convex {{Formulations}} of {{Data Assimilation Problems}} for a {{Class}} of {{Hamilton}}\textendash{{Jacobi Equations}}},
 volume = {49},
 year = {2011}
}

@article{claudel_lax-hopf_2010,
 author = {Claudel, Christian G and Bayen, Alexandre M},
 doi = {10.1109/TAC.2010.2041976},
 file = {/home/matt/Zotero/storage/3WGJWUPE/ClaudelBayen_LaxHopf.pdf},
 issn = {0018-9286, 1558-2523},
 journal = {IEEE Transactions on Automatic Control},
 number = {5},
 pages = {1142--1157},
 shorttitle = {Lax\&\#x2013;{{Hopf Based Incorporation}} of {{Internal Boundary Conditions Into Hamilton}}\&\#x2013;{{Jacobi Equation}}. {{Part I}}},
 title = {Lax-{{Hopf Based Incorporation}} of {{Internal Boundary Conditions Into Hamilton}}-{{Jacobi Equation}}. {{Part I}}: {{Theory}}},
 volume = {55},
 year = {2010}
}

@article{claudel_solutions_2014,
 author = {Claudel, Christian G. and Chamoin, Timothee and Bayen, Alexandre M.},
 doi = {10.1109/TCST.2013.2238940},
 file = {/home/matt/Zotero/storage/KVHBKKAD/ClaudelBayenSolutionsEstimationLP.pdf},
 issn = {1063-6536, 1558-0865},
 journal = {IEEE Transactions on Control Systems Technology},
 number = {1},
 pages = {273--280},
 title = {Solutions to {{Estimation Problems}} for {{Scalar Hamilton}}\&\#x2013;{{Jacobi Equations Using Linear Programming}}},
 volume = {22},
 year = {2014}
}

@article{clements_economic_2017,
 abstract = {Connected and fully automated or autonomous vehicles (CAVs) may soon dominate the automotive industry. Once CAVs are sufficiently reliable and affordable, they will penetrate markets and thereby generate economic ripple effects throughout industries. This paper synthesizes and expands on existing analyses of the economic effects of CAVs in the United States across 13 industries and the overall economy. CAVs will soon be central to the automotive industry, with software composing a greater share of vehicle value than previously. The number of vehicles purchased each year may fall because of vehicle sharing, but rising travel distances may increase vehicle sales. The opportunity for heavy-truck drivers to do other work or rest during long drives may lower freight costs and increase capacity. Personal transport may shift toward shared autonomous vehicle fleet use, reducing that of taxis, buses, and other forms of group travel. Fewer collisions and more law-abiding vehicles will lower demand for auto repair, traffic police, medical, insurance, and legal services. CAVs will also lead to new methods for managing travel demand and the repurposing of curbside and off-street parking and will generate major savings from productivity gains during hands-free travel and reduction of pain and suffering costs from crashes. If CAVs eventually capture a large share of the automotive market, they are estimated to have economic impacts of \$1.2 trillion or \$3,800 per American per year. This paper presents important considerations for CAVs' overall effects and quantifies those impacts.},
 author = {Clements, Lewis M. and Kockelman, Kara M.},
 doi = {10.3141/2606-14},
 file = {/home/matt/Zotero/storage/URT57HAY/Clements and Kockelman - 2017 - Economic Effects of Automated Vehicles.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 language = {en},
 number = {1},
 pages = {106--114},
 title = {Economic {{Effects}} of {{Automated Vehicles}}},
 volume = {2606},
 year = {2017}
}

@article{cleveland_robust_1979,
 author = {Cleveland, W.S.},
 journal = {Journal of the American Statistical Association},
 number = {368},
 pages = {829--836},
 title = {Robust Locally Weighted Regression and Smoothing Scatterplots},
 volume = {74},
 year = {1979}
}

@article{codina_dynamic_1995,
 author = {Codina, E. and Barcelo, J.},
 journal = {Annals of Operations Research},
 pages = {1--58},
 title = {Dynamic Traffic Assignment: {{Considerations}} on Some Deterministic Modelling Approaches},
 volume = {60},
 year = {1995}
}

@article{coifman_empirical_2015,
 author = {Coifman, Benjamin},
 doi = {10.1016/j.trb.2015.04.006},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {54--65},
 shorttitle = {Empirical Flow-Density and Speed-Spacing Relationships},
 title = {Empirical Flow-Density and Speed-Spacing Relationships: {{Evidence}} of Vehicle Length Dependency},
 volume = {78},
 year = {2015}
}

@article{coifman_extended_2010,
 author = {Coifman, Benjamin and Kim, Seoungbum},
 journal = {19th International Symposium of Transportation and Traffic Theory},
 title = {Extended {{Bottlenecks}}, the {{Fundamental Relationship}}, and {{Capacity Drop}} on {{Freeways}}},
 year = {2010}
}

@article{colombo_2x2_2002,
 author = {Colombo, R. M.},
 journal = {Math. Comput. Modelling},
 pages = {683--688},
 title = {On a 2x2 Hyperbolic Traffic Model.},
 volume = {35},
 year = {2002}
}

@article{colombo_hyperbolic_2002,
 author = {Colombo, R. M.},
 journal = {SIAM Journal of Applied Mathematics},
 number = {2},
 pages = {708--721},
 title = {Hyperbolic Phase Transitions in Traffic Flow.},
 volume = {63},
 year = {2002}
}

@book{commission_i-680_nodate,
 author = {Commission, Alameda County Transportation},
 title = {I-680 {{Southbound Express Lane}}, {{Annual Report FY2012}}-2013},
 year = {n.d.}
}

@book{commission_i-680_nodate-1,
 author = {Commission, Alameda County Transportation},
 title = {I-680 {{Southbound Express Lane}}, {{Annual Report FY2011}}-2012},
 year = {n.d.}
}

@book{commission_i-680_nodate-2,
 author = {Commission, Alameda County Transportation},
 title = {I-680 {{Southbound Express Lane}}, {{Annual Report FY2010}}-2011},
 year = {n.d.}
}

@book{committee_future_2004,
 annotation = {Published: A discussion Paper prepared for the TRB Regional Transportation System Management and Operations Committee and the AASHTO Subcommittee on System Operations and Management Task Force on Traveler Information},
 author = {Committee, TRB Freeway Operations},
 title = {The {{Future}} of {{Travel Time Data}}-{{A Paradigm Shift}}.},
 year = {2004}
}

@article{congress_smart_1996,
 author = {Congress, N.},
 journal = {Public Roads, Magazine of the Federal Highway Administration},
 number = {2},
 title = {Smart {{Road}}, {{Smart Car}}: {{The Automated Highway System}}},
 volume = {60},
 year = {1996}
}

@phdthesis{coogan_synthesis_2015,
 abstract = {Engineering advances have enabled systems that are increasingly complex while, simultaneously, expectations for the closed-loop behavior of these systems have become more demanding. The resulting combination of complexity and desired behavior requires correct-by-design approaches to system analysis and control. In this dissertation, we develop a class of scalable and automated verification and control synthesis techniques for networked systems. To motivate our study and to demonstrate the applicability of our results, we focus on transportation networks. The formal analysis and synthesis approaches which are the emphasis of much of this dissertation require a discrete representation of the system in the form of a finite abstraction for the system's behavior. A finite abstraction models the states and dynamics of the system with a finite set of properties and transitions which capture all the phenomena of interest. We first present a broad class of systems which are mixed monotone, that is, systems for which the state evolution can be decomposed into an increasing and decreasing component. For such systems, we develop an efficient abstraction algorithm to enable correct-by-design control synthesis. We then use this approach to synthesize control strategies for transportation flow networks.We next turn our attention to qualitative analysis of the dynamics present in traffic flow networks. We propose a macroscopic network flow model in continuous time suitable for analysis as a dynamical system, and we analyze equilibrium flows as well as convergence. We show that the same mixed monotone property that enables efficient abstraction allows us to prove global asymptotic stability by embedding the flow network in a larger system.These contributions provide the theoretical foundation for correct-by-design control of a large class of networked physical systems. By focusing on transportation networks, we show concretely how these results apply to a domain that is of considerable practical importance.},
 author = {Coogan, Samuel Donald},
 file = {/home/matt/Zotero/storage/I7FGTAG3/Coogan - 2015 - Synthesis and Verification of Networked Systems wi.pdf;/home/matt/Zotero/storage/HZ2FC379/7vm2r8sb.html},
 language = {en},
 school = {UC Berkeley},
 title = {Synthesis and {{Verification}} of {{Networked Systems}} with {{Applications}} to {{Transportation Networks}}},
 year = {2015}
}

@inproceedings{cordonnier_relationship_2020,
 author = {Jean{-}Baptiste Cordonnier and
Andreas Loukas and
Martin Jaggi},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/CordonnierLJ20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {On the Relationship between Self-Attention and Convolutional Layers},
 url = {https://openreview.net/forum?id=HJlnC1rKPB},
 year = {2020}
}

@article{cortes_support-vector_1995,
 abstract = {The support-vector network is a new leaming machine for two-group classification problems. The machine conceptually implements the following idea: input vectors are non-linearly mapped to a very highdimension feature space. In this feature space a linear decision surface is constructed. Special properties of the decision surface ensures high generalization ability of the learning machine. The idea behind the support-vector network was previously implemented for the restricted case where the training data can be separated without errors. We here extend this result to non-separable training data.},
 author = {Cortes, Corinna and Vapnik, Vladimir},
 doi = {10.1007/BF00994018},
 file = {/home/matt/Zotero/storage/WBYVHHF4/Cortes and Vapnik - 1995 - Support-vector networks.pdf},
 issn = {0885-6125, 1573-0565},
 journal = {Machine Learning},
 language = {en},
 number = {3},
 pages = {273--297},
 title = {Support-Vector Networks},
 volume = {20},
 year = {1995}
}

@article{corthout_non-unique_2012,
 author = {Corthout, Ruben and Fl{\"o}tter{\"o}d, Gunnar and Viti, Francesco and Tamp{\`e}re, Chris M.J.},
 doi = {10.1016/j.trb.2011.10.011},
 file = {/home/matt/Zotero/storage/PS53NDJT/corthout_nonunique_flows.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {3},
 pages = {343--359},
 title = {Non-Unique Flows in Macroscopic First-Order Intersection Models},
 volume = {46},
 year = {2012}
}

@article{courant_uber_1928,
 author = {Courant, R. and Friedrichs, K. and Lewy, H.},
 journal = {Mathematische Annalen},
 number = {1},
 pages = {32--74},
 title = {\"Uber Die Partiellen {{Differenzengleichungen}} Der Mathematischen {{Physik}}.},
 volume = {100},
 year = {1928}
}

@book{crabtree_remote_2003,
 address = {{Kentucky Transportation Center}},
 annotation = {Published: Powerpoint Presentation},
 author = {Crabtree, J.},
 title = {The {{Remote Monitoring System}} and {{Virtual Weigh Station}}},
 year = {2003}
}

@article{cremer_new_1987,
 author = {Cremer, M. and Keller, H.},
 journal = {Transportation Research B},
 number = {2},
 pages = {117--132},
 title = {A New Class of Dynamic Methods for the Identification of Origin-Destination Flows},
 volume = {21},
 year = {1987}
}

@article{cruz_calculus_1991,
 author = {Cruz, R. L.},
 journal = {IEEE Trans. Information Theory},
 number = {1},
 pages = {114--141},
 title = {A Calculus for Network Delay. {{Part I}}: {{Network}} Elements in Isolation. {{Part II}}: {{Network}} Analysis},
 volume = {37},
 year = {1991}
}

@inproceedings{cui_stabilizing_2017,
 author = {Cui, Shumo and Seibold, Benjamin and Stern, Raphael and Work, Daniel B.},
 booktitle = {Intelligent {{Vehicles Symposium}} ({{IV}}), 2017 {{IEEE}}},
 doi = {10.1109/IVS.2017.7995897},
 file = {/home/matt/Zotero/storage/538HZUT3/cui_work_stabilizing_traffic_flow_2017.pdf},
 pages = {1336--1341},
 publisher = {{IEEE}},
 shorttitle = {Stabilizing Traffic Flow via a Single Autonomous Vehicle},
 title = {Stabilizing Traffic Flow via a Single Autonomous Vehicle: {{Possibilities}} and Limitations},
 year = {2017}
}

@article{cui_traffic_2018,
 author = {Cui, Zhiyong and Henrickson, Kristian and Ke, Ruimin and Wang, Yinhai},
 journal = {ArXiv preprint},
 title = {Traffic {{Graph Convolutional Recurrent Neural Network}}: {{A Deep Learning Framework}} for {{Network}}-{{Scale Traffic Learning}} and {{Forecasting}}},
 url = {https://arxiv.org/abs/1802.07007},
 volume = {abs/1802.07007},
 year = {2018}
}

@article{cui_traffic_2019,
 author = {Cui, Zhiyong and Henrickson, Kristian and Ke, Ruimin and Wang, Yinhai},
 doi = {10.1109/TITS.2019.2950416},
 file = {/home/matt/Zotero/storage/GBSJD8BP/Cui et al. - 2019 - Traffic Graph Convolutional Recurrent Neural Netwo.pdf},
 issn = {1524-9050, 1558-0016},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 pages = {1--12},
 shorttitle = {Traffic {{Graph Convolutional Recurrent Neural Network}}},
 title = {Traffic {{Graph Convolutional Recurrent Neural Network}}: {{A Deep Learning Framework}} for {{Network}}-{{Scale Traffic Learning}} and {{Forecasting}}},
 year = {2019}
}

@article{cybenko_approximation_1989,
 abstract = {In this paper we demonstrate that finite linear combinations of compositions of a fixed, univariate function and a set of affine functionals can uniformly approximate any continuous function ofn real variables with support in the unit hypercube; only mild conditions are imposed on the univariate function. Our results settle an open question about representability in the class of single hidden layer neural networks. In particular, we show that arbitrary decision regions can be arbitrarily well approximated by continuous feedforward neural networks with only a single internal, hidden layer and any continuous sigmoidal nonlinearity. The paper discusses approximation properties of other possible types of nonlinearities that might be implemented by artificial neural networks.},
 author = {Cybenko, G.},
 doi = {10.1007/BF02551274},
 file = {/home/matt/Zotero/storage/SC3RN9S2/Cybenko - 1989 - Approximation by superpositions of a sigmoidal fun.pdf},
 issn = {1435-568X},
 journal = {Mathematics of Control, Signals and Systems},
 language = {en},
 number = {4},
 pages = {303--314},
 title = {Approximation by Superpositions of a Sigmoidal Function},
 volume = {2},
 year = {1989}
}

@article{daganzo_behavioral_2002,
 author = {Daganzo, Carlos F},
 doi = {10.1016/S0191-2615(00)00042-4},
 file = {/home/matt/Zotero/storage/8ZBD5NC5/1992_TRB_daganzo_multilane.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {2},
 pages = {131--158},
 shorttitle = {A Behavioral Theory of Multi-Lane Traffic Flow. {{Part I}}},
 title = {A Behavioral Theory of Multi-Lane Traffic Flow. {{Part I}}: {{Long}} Homogeneous Freeway Sections},
 volume = {36},
 year = {2002}
}

@article{daganzo_cell_1994,
 author = {Daganzo, Carlos F.},
 doi = {10.1016/0191-2615(94)90002-7},
 journal = {Transportation Research Part B: Methodological},
 number = {4},
 pages = {269--287},
 title = {The Cell Transmission Model: {{A}} Dynamic Representation of Highway Traffic Consistent with the Hydrodynamic Theory},
 volume = {28},
 year = {1994}
}

@article{daganzo_cell_1995,
 author = {Daganzo, Carlos F.},
 doi = {10.1016/0191-2615(94)00022-R},
 file = {/home/matt/Documents/Papers/daganzo_ctm2.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {2},
 pages = {79--93},
 shorttitle = {The Cell Transmission Model, Part {{II}}},
 title = {The Cell Transmission Model, {{Part II}}: {{Network}} Traffic},
 volume = {29},
 year = {1995}
}

@article{daganzo_continuum_1997,
 author = {Daganzo, Carlos F.},
 doi = {10.1016/S0191-2615(96)00017-3},
 file = {/home/matt/Zotero/storage/K46RGD3Q/1997_TRB_dynamics_of_freeways_with_special_lanes.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {2},
 pages = {83--102},
 title = {A Continuum Theory of Traffic Dynamics for Freeways with Special Lanes},
 volume = {31},
 year = {1997}
}

@article{daganzo_effects_2008,
 author = {Daganzo, Carlos F. and Cassidy, Michael J.},
 doi = {10.1016/j.trb.2008.03.002},
 file = {/home/matt/Zotero/storage/NUI6QJ4M/2008_TRC_daganzo_cassidy_hovoncongestion.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {10},
 pages = {861--872},
 title = {Effects of High Occupancy Vehicle Lanes on Freeway Congestion},
 volume = {42},
 year = {2008}
}

@article{daganzo_requiem_1995,
 author = {Daganzo, C.},
 journal = {Transportation Research, Part B},
 pages = {277--286},
 title = {Requiem for Second-Order Fluid Approximations of Traffic Flow},
 volume = {29},
 year = {1995}
}

@article{daganzo_simple_1997,
 author = {Daganzo, Carlos F. and Lin, Wei-Hua and Del Castillo, Jose M.},
 file = {/home/matt/Zotero/storage/9I2C6FAV/1997_TRB_daganzo_physical_principle_sim_special_lanes.pdf},
 journal = {Transportation Research Part B: Methodological},
 number = {2},
 pages = {103--125},
 title = {A Simple Physical Principle for the Simulation of Freeways with Special Lanes and Priority Vehicles},
 volume = {31},
 year = {1997}
}

@article{daganzo_urban_2007,
 author = {Daganzo, C. F.},
 journal = {Transportation Research, Part B},
 pages = {49--62},
 title = {Urban Gridlock: Macroscopic Modeling and Mitigation Approaches},
 volume = {41},
 year = {2007}
}

@inproceedings{dai_diagnosing_2019,
 author = {Bin Dai and
David P. Wipf},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/DaiW19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Diagnosing and Enhancing {VAE} Models},
 url = {https://openreview.net/forum?id=B1e0X3C9tQ},
 year = {2019}
}

@inproceedings{dai_funnel-transformer_2020,
 author = {Zihang Dai and
Guokun Lai and
Yiming Yang and
Quoc Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/DaiLY020.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Funnel-Transformer: Filtering out Sequential Redundancy for Efficient
Language Processing},
 url = {https://proceedings.neurips.cc/paper/2020/hash/2cd2915e69546904e4e5d4a2ac9e1652-Abstract.html},
 year = {2020}
}

@article{dai_maximum_2005,
 author = {Dai, J. G. and Lin, W.},
 journal = {Operations Research},
 number = {2},
 pages = {197--218},
 title = {Maximum Pressure Policies in Stochastic Processing Networks},
 volume = {53},
 year = {2005}
}

@article{dai_positive_1995,
 abstract = {we prove that a queueing networkis positive Harris recurrent if the corresponding fluid limit model eventually reaches zero and stays there regardless of the initial system configuration. As an application of the result, we prove that single class networks, multiclass feedforward networks and first-buffer-first-served preemptive},
 author = {Dai, J. G.},
 journal = {Annals of Applied Probability},
 keywords = {},
 number = {1},
 pages = {49--77},
 title = {On {{Positive Harris Recurrence}} of {{Multiclass Queueing Networks}}: {{A Unified Approach Via Fluid Limit Models}}},
 volume = {5},
 year = {1995}
}

@inproceedings{dai_transformer-xl_2019,
 address = {Florence, Italy},
 author = {Dai, Zihang  and
Yang, Zhilin  and
Yang, Yiming  and
Carbonell, Jaime  and
Le, Quoc  and
Salakhutdinov, Ruslan},
 booktitle = {Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/P19-1285},
 pages = {2978--2988},
 publisher = {Association for Computational Linguistics},
 title = {Transformer-{XL}: Attentive Language Models beyond a Fixed-Length Context},
 url = {https://aclanthology.org/P19-1285},
 year = {2019}
}

@techreport{dailey_improved_1993,
 author = {Dailey, D.},
 institution = {{Washington State DOT}},
 number = {WA-RD 3001},
 title = {Improved Error Detection for Inductive Loop Sensors},
 year = {1993}
}

@article{dailey_statistical_1999,
 author = {Dailey, D.},
 journal = {Transportation Research B},
 number = {5},
 pages = {313--322},
 title = {A Statistical Algorithm for Estimating Speed from Single Loop Volume and Occupancy Measurements},
 volume = {33B},
 year = {1999}
}

@article{darbha_benefits_2019,
 abstract = {In this paper, we investigate the benefits of vehicle-to-vehicle (V2V) communication for autonomous vehicles and provide results on how V2V information helps reduce employable time headway in the presence of parasitic lags. For a string of vehicles adopting a constant time headway policy and availing the on-board information of predecessor's vehicle position and velocity, the minimum employable time headway (hmin) must be lower bounded by 2{$\tau$}0 for string stability, where {$\tau$}0 is the maximum parasitic actuation lag. In this paper, we quantify the benefits of using V2V communication in terms of a reduction in the employable time headway: 1) If the position and velocity information of r immediately preceding vehicles is used, then hmin can be reduced to 4{$\tau$}0/(1 + r); 2) furthermore, if the acceleration of `r' immediately preceding vehicles is used, then hmin can be reduced to 2{$\tau$}0/(1 + r); and 3) if the position, velocity, and acceleration of the immediate and the r-th predecessors are used, then hmin {$\geq$} 2{$\tau$}0/(1 + r). Note that cases (2) and (3) provide the same lower bound on the minimum employable time headway; however, case (3) requires much less communicated information.},
 author = {Darbha, Swaroop and Konduri, Shyamprasad and Pagilla, Prabhakar R.},
 doi = {10.1109/TITS.2018.2859765},
 file = {/home/matt/Zotero/storage/TPH2UML9/Darbha et al. - 2019 - Benefits of V2V Communication for Autonomous and C.pdf;/home/matt/Zotero/storage/4I6PXVEC/8463512.html},
 issn = {1558-0016},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {5},
 pages = {1954--1963},
 title = {Benefits of {{V2V Communication}} for {{Autonomous}} and {{Connected Vehicles}}},
 volume = {20},
 year = {2019}
}

@article{dargay_vehicle_2007,
 author = {Dargay, J. and Gately, D. and Sommer, M.},
 journal = {Energy Journal},
 number = {4},
 pages = {143--170},
 title = {Vehicle {{Ownership}} and {{Income Growth}}, {{Worldwide}}: 1960-2030},
 volume = {28},
 year = {2007}
}

@article{das_likelihood_2019,
 author = {Das, Hari Prasanna and Abbeel, Pieter and Spanos, Costas J.},
 journal = {ArXiv preprint},
 title = {Likelihood {{Contribution}} Based {{Multi}}-Scale {{Architecture}} for {{Generative Flows}}},
 url = {https://arxiv.org/abs/1908.01686},
 volume = {abs/1908.01686},
 year = {2019}
}

@inproceedings{dasari_robonet_2019,
 abstract = {Robot learning has emerged as a promising tool for taming the complexity and diversity of the real world. Methods based on high-capacity models, such as deep networks, hold the promise of providing effective generalization to a wide range of open-world environments. However, these same methods typically require large amounts of diverse training data to generalize effectively. In contrast, most robotic learning experiments are small-scale, single-domain, and single-robot. This leads to a frequent tension in robotic learning: how can we learn generalizable robotic controllers without having to collect impractically large amounts of data for each separate experiment? In this paper, we propose RoboNet, an open database for sharing robotic experience, which provides an initial pool of 15 million video frames, from 7 different robot platforms, and study how it can be used to learn generalizable models for vision-based robotic manipulation. We combine the dataset with two different learning algorithms: visual foresight, which uses forward video prediction models, and supervised inverse models. Our experiments test the learned algorithms' ability to work across new objects, new tasks, new scenes, new camera viewpoints, new grippers, or even entirely new robots. In our final experiment, we find that by pre-training on RoboNet and fine-tuning on data from a held-out Franka or Kuka robot, we can exceed the performance of a robot-specific training approach that uses 4x-20x more data. For videos and data, see the project webpage: https://www.robonet.wiki/},
 archiveprefix = {arXiv},
 author = {Dasari, Sudeep and Ebert, Frederik and Tian, Stephen and Nair, Suraj and Bucher, Bernadette and Schmeckpeper, Karl and Singh, Siddharth and Levine, Sergey and Finn, Chelsea},
 booktitle = {3rd {{Conference}} on {{Robot Learning}} ({{CoRL}} 2019)},
 eprint = {1910.11215},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/7B7SHJWN/Dasari et al. - 2020 - RoboNet Large-Scale Multi-Robot Learning.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 shorttitle = {{{RoboNet}}},
 title = {{{RoboNet}}: {{Large}}-{{Scale Multi}}-{{Robot Learning}}},
 year = {2019}
}

@inproceedings{dauphin_language_2017,
 author = {Yann N. Dauphin and
Angela Fan and
Michael Auli and
David Grangier},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/DauphinFAG17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {933--941},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Language Modeling with Gated Convolutional Networks},
 url = {http://proceedings.mlr.press/v70/dauphin17a.html},
 volume = {70},
 year = {2017}
}

@article{davies_mobileye_2013,
 author = {Davies, C.},
 journal = {SlashGear.com},
 title = {Mobileye Wants Self-Driving Cars by 2016 at a Fraction of {{Google}}'s Costs},
 year = {2013}
}

@article{davis_using_1984,
 author = {Davis, G. and Nihan, N.},
 journal = {Transportation Research, Part A},
 number = {5/6},
 pages = {431--438},
 title = {Using {{Time}}-{{Series Designs}} to {{Estimate Changes}} in {{Freeway Level}} of {{Service}}, {{Despite Missing Data}}},
 volume = {18A},
 year = {1984}
}

@article{day_reflexive_1941,
 author = {Day, Mahlon M.},
 doi = {10.1090/S0002-9904-1941-07451-3},
 file = {/home/matt/Zotero/storage/M3FDL5ES/Day - 1941 - Reflexive Banach spaces not isomorphic to uniforml.pdf},
 issn = {0002-9904},
 journal = {Bulletin of the American Mathematical Society},
 language = {en},
 number = {4},
 pages = {313--318},
 title = {Reflexive {{Banach}} Spaces Not Isomorphic to Uniformly Convex Spaces},
 volume = {47},
 year = {1941}
}

@inproceedings{de_cao_molgan_2018,
 abstract = {Deep generative models for graph-structured data offer a new angle on the problem of chemical synthesis: by optimizing differentiable models that directly generate molecular graphs, it is possible to side-step expensive search procedures in the discrete and vast space of chemical structures. We introduce MolGAN, an implicit, likelihood-free generative model for small molecular graphs that circumvents the need for expensive graph matching procedures or node ordering heuristics of previous likelihood-based methods. Our method adapts generative adversarial networks (GANs) to operate directly on graph-structured data. We combine our approach with a reinforcement learning objective to encourage the generation of molecules with specific desired chemical properties. In experiments on the QM9 chemical database, we demonstrate that our model is capable of generating close to 100\% valid compounds. MolGAN compares favorably both to recent proposals that use string-based (SMILES) representations of molecules and to a likelihood-based method that directly generates graphs, albeit being susceptible to mode collapse.},
 archiveprefix = {arXiv},
 author = {De Cao, Nicola and Kipf, Thomas},
 booktitle = {{{ICML Workshop}} on {{Theoretical Foundations}} and {{Applications}} of {{Deep Generative Models}}},
 eprint = {1805.11973},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/M7SY3F9I/De Cao and Kipf - 2018 - MolGAN An implicit generative model for small mol.pdf;/home/matt/Zotero/storage/FCB8GAEU/1805.html},
 shorttitle = {{{MolGAN}}},
 title = {{{MolGAN}}: {{An}} Implicit Generative Model for Small Molecular Graphs},
 year = {2018}
}

@inproceedings{de_freitas_rao-blackwellised_2002,
 author = {De Freitas, Nando},
 booktitle = {Aerospace {{Conference Proceedings}}, 2002. {{IEEE}}},
 file = {/home/matt/Zotero/storage/VSZ6BCZZ/defrietas_pf_faultdetect.pdf},
 pages = {4--4},
 publisher = {{IEEE}},
 title = {Rao-{{Blackwellised}} Particle Filtering for Fault Diagnosis},
 volume = {4},
 year = {2002}
}

@inproceedings{de_haan_causal_2019,
 author = {Pim de Haan and
Dinesh Jayaraman and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/HaanJL19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {11693--11704},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Causal Confusion in Imitation Learning},
 url = {https://proceedings.neurips.cc/paper/2019/hash/947018640bf36a2bb609d3557a285329-Abstract.html},
 year = {2019}
}

@inproceedings{de_haan_causal_2019-1,
 author = {Pim de Haan and
Dinesh Jayaraman and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/HaanJL19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {11693--11704},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Causal Confusion in Imitation Learning},
 url = {https://proceedings.neurips.cc/paper/2019/hash/947018640bf36a2bb609d3557a285329-Abstract.html},
 year = {2019}
}

@article{de_vries_bitcoins_2018,
 abstract = {The electricity that is expended in the process of mining Bitcoin has become a topic of heavy debate over the past few years. It is a process that makes Bitcoin extremely energy-hungry by design, as the currency requires a huge amount of hash calculations for its ultimate goal of processing financial transactions without intermediaries (peer-to-peer). The primary fuel for each of these calculations is electricity. The Bitcoin network can be estimated to consume at least 2.55 gigawatts of electricity currently, and potentially 7.67 gigawatts in the future, making it~comparable with countries such as Ireland (3.1 gigawatts) and Austria (8.2~gigawatts). Economic models tell us that Bitcoin's electricity consumption will gravitate toward the latter number. A look at Bitcoin miner production estimates suggests that this number could already be reached in 2018.},
 author = {{\noopsort{vries}}{de Vries}, Alex},
 doi = {10.1016/j.joule.2018.04.016},
 file = {/home/matt/Zotero/storage/RG5C2CMR/de Vries - 2018 - Bitcoin's Growing Energy Problem.pdf;/home/matt/Zotero/storage/2D938JIS/S2542435118301776.html},
 issn = {2542-4351},
 journal = {Joule},
 language = {en},
 number = {5},
 pages = {801--805},
 title = {Bitcoin's {{Growing Energy Problem}}},
 volume = {2},
 year = {2018}
}

@inproceedings{de-gang_chen_generalized_2008,
 abstract = {The support vector machine (SVM) is well understood when kernel functions are positive definite. However, in practice, indefinite kernels arise and demand application in SVM. These indefinite kernels often yield good empirical classification results. However, they are hard to understand for missing geometrical and theoretical understanding. In this paper we focus our topic on the structure of feature space related to indefinite kernels. We develop a new method by improving Mercer theorem to construct the mapping that maps input data set into the high-dimensional feature space for indefinite kernels. Via this mapping, structure of the feature space is easily observed. By this, we obtain a sound framework and motivation for SVM with indefinite kernels.},
 author = {{De-Gang Chen} and {Heng-You Wang} and Tsang, Eric C.C.},
 booktitle = {2008 {{International Conference}} on {{Machine Learning}} and {{Cybernetics}}},
 doi = {10.1109/ICMLC.2008.4620508},
 file = {/home/matt/Zotero/storage/TBBVI3B5/De-Gang Chen et al. - 2008 - Generalized Mercer theorem and its application to .pdf;/home/matt/Zotero/storage/JRPP3Y2W/4620508.html},
 issn = {2160-1348},
 pages = {774--777},
 title = {Generalized {{Mercer}} Theorem and Its Application to Feature Space Related to Indefinite Kernels},
 volume = {2},
 year = {2008}
}

@article{dean_recommendations_2020,
 abstract = {Recommender systems often rely on models which are trained to maximize accuracy in predicting user preferences. When the systems are deployed, these models determine the availability of content and information to different users. The gap between these objectives gives rise to a potential for unintended consequences, contributing to phenomena such as filter bubbles and polarization. In this work, we consider directly the information availability problem through the lens of user recourse. Using ideas of reachability, we propose a computationally efficient audit for top-N linear recommender models. Furthermore, we describe the relationship between model complexity and the effort necessary for users to exert control over their recommendations. We use this insight to provide a novel perspective on the user cold-start problem. Finally, we demonstrate these concepts with an empirical investigation of a state-of-the-art model trained on a widely used movie ratings dataset.},
 author = {Dean, Sarah and Rich, Sarah and Recht, Benjamin},
 doi = {10.1145/3351095.3372866},
 file = {/home/matt/Zotero/storage/ETPWHAYX/Dean et al. - 2020 - Recommendations and User Agency The Reachability .pdf},
 journal = {FAT* '20: Proceedings of the 2020 Conference on Fairness, Accountability, and Transparency},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {436--445},
 title = {Recommendations and {{User Agency}}: {{The Reachability}} of {{Collaboratively}}-{{Filtered Information}}},
 year = {2020}
}

@article{dean_robust_2019,
 author = {Dean, Sarah and Matni, Nikolai and Recht, Benjamin and Ye, Vickie},
 journal = {ArXiv preprint},
 title = {Robust {{Guarantees}} for {{Perception}}-{{Based Control}}},
 url = {https://arxiv.org/abs/1907.03680},
 volume = {abs/1907.03680},
 year = {2019}
}

@inproceedings{defferrard_convolutional_2016,
 author = {Micha{\"{e}}l Defferrard and
Xavier Bresson and
Pierre Vandergheynst},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/DefferrardBV16.bib},
 booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
on Neural Information Processing Systems 2016, December 5-10, 2016,
Barcelona, Spain},
 editor = {Daniel D. Lee and
Masashi Sugiyama and
Ulrike von Luxburg and
Isabelle Guyon and
Roman Garnett},
 pages = {3837--3845},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Convolutional Neural Networks on Graphs with Fast Localized Spectral
Filtering},
 url = {https://proceedings.neurips.cc/paper/2016/hash/04df4d434d481c5bb723be1b6df1ee65-Abstract.html},
 year = {2016}
}

@inproceedings{dehghani_universal_2019,
 author = {Mostafa Dehghani and
Stephan Gouws and
Oriol Vinyals and
Jakob Uszkoreit and
Lukasz Kaiser},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/DehghaniGVUK19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Universal Transformers},
 url = {https://openreview.net/forum?id=HyzdRiR9Y7},
 year = {2019}
}

@inproceedings{deisenroth_pilco_2011,
 author = {Marc Peter Deisenroth and
Carl Edward Rasmussen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/DeisenrothR11.bib},
 booktitle = {Proceedings of the 28th International Conference on Machine Learning,
{ICML} 2011, Bellevue, Washington, USA, June 28 - July 2, 2011},
 editor = {Lise Getoor and
Tobias Scheffer},
 pages = {465--472},
 publisher = {Omnipress},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {{PILCO:} {A} Model-Based and Data-Efficient Approach to Policy Search},
 url = {https://icml.cc/2011/papers/323\_icmlpaper.pdf},
 year = {2011}
}

@article{dempster_maximum_1977,
 author = {Dempster, A. P. and Laird, N. M. and Rubin, D. B.},
 journal = {J. Royal Statstical Society, B},
 number = {1},
 pages = {1--38},
 title = {Maximum {{Likelihood}} from Incomplete Data via the {{EM}} Algorithm},
 volume = {39},
 year = {1977}
}

@article{dendrinos_traffic-flow_1994,
 abstract = {Taking off from findings involving Fast Fourier Transforms of urban traffic-flow time series, the observed nonperiodic component of transportation flow rates becomes the focus of this paper. A theory of the microscopic as well as macroscopic traffic behavior involved is put forward, and specific tests searching for chaotic dynamic are discussed. This topic is representative of a class of subjects in socio-spatial analysis that involve nonperiodic dynamics. It identifies possible chaotic patterns on residuals of such dynamics from approximate temporal (mainly daily) cycles.},
 author = {Dendrinos, Dimitrios S.},
 doi = {10.1016/0960-0779(94)90069-8},
 file = {/home/matt/Zotero/storage/WC5N46GP/Dendrinos - 1994 - Traffic-flow dynamics A search for chaos.pdf;/home/matt/Zotero/storage/DUW83MQX/0960077994900698.html},
 issn = {0960-0779},
 journal = {Chaos, Solitons \& Fractals},
 number = {4},
 pages = {605--617},
 shorttitle = {Traffic-Flow Dynamics},
 title = {Traffic-Flow Dynamics: {{A}} Search for Chaos},
 volume = {4},
 year = {1994}
}

@book{department_for_transport_road_2007,
 author = {{Department for Transport}},
 title = {Road {{Pricing}}},
 year = {2007}
}

@article{dervisoglu_automatic_2009,
 author = {Dervisoglu, G. and Gomes, G. and Kwon, J. and Muralidharan, A. and Varaiya, P. and Horowitz, R.},
 journal = {88th Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {Automatic Calibration of the Fundamental Diagram and Empirical Obsevations on Capacity},
 year = {2009}
}

@inproceedings{desai_calibration_2020,
 address = {Online},
 author = {Desai, Shrey  and
Durrett, Greg},
 booktitle = {Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)},
 doi = {10.18653/v1/2020.emnlp-main.21},
 pages = {295--302},
 publisher = {Association for Computational Linguistics},
 title = {Calibration of Pre-trained Transformers},
 url = {https://aclanthology.org/2020.emnlp-main.21},
 year = {2020}
}

@inproceedings{desai_negotiable_2018,
 author = {Nishant Desai and
Andrew Critch and
Stuart J. Russell},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/DesaiCR18.bib},
 booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
on Neural Information Processing Systems 2018, NeurIPS 2018, December
3-8, 2018, Montr{\'{e}}al, Canada},
 editor = {Samy Bengio and
Hanna M. Wallach and
Hugo Larochelle and
Kristen Grauman and
Nicol{\`{o}} Cesa{-}Bianchi and
Roman Garnett},
 pages = {4717--4725},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Negotiable Reinforcement Learning for Pareto Optimal Sequential Decision-Making},
 url = {https://proceedings.neurips.cc/paper/2018/hash/5b8e4fd39d9786228649a8a8bec4e008-Abstract.html},
 year = {2018}
}

@article{devin_plan_2019,
 author = {Devin, Coline and Geng, Daniel and Abbeel, Pieter and Darrell, Trevor and Levine, Sergey},
 journal = {ArXiv preprint},
 title = {Plan {{Arithmetic}}: {{Compositional Plan Vectors}} for {{Multi}}-{{Task Control}}},
 url = {https://arxiv.org/abs/1910.14033},
 volume = {abs/1910.14033},
 year = {2019}
}

@article{devine_widening_2002,
 author = {Devine, Denis},
 journal = {North County Times},
 title = {Widening of {{I}}-5/805 Interchange No Panacea},
 year = {2002}
}

@inproceedings{devlin_bert_2018,
 address = {Minneapolis, Minnesota},
 author = {Devlin, Jacob  and
Chang, Ming-Wei  and
Lee, Kenton  and
Toutanova, Kristina},
 booktitle = {Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)},
 doi = {10.18653/v1/N19-1423},
 pages = {4171--4186},
 publisher = {Association for Computational Linguistics},
 title = {{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding},
 url = {https://aclanthology.org/N19-1423},
 year = {2019}
}

@inproceedings{devlin_bert_2019,
 address = {Minneapolis, Minnesota},
 author = {Devlin, Jacob  and
Chang, Ming-Wei  and
Lee, Kenton  and
Toutanova, Kristina},
 booktitle = {Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)},
 doi = {10.18653/v1/N19-1423},
 pages = {4171--4186},
 publisher = {Association for Computational Linguistics},
 title = {{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding},
 url = {https://aclanthology.org/N19-1423},
 year = {2019}
}

@article{dey_review_2016,
 abstract = {Cooperative adaptive cruise control (CACC) systems have the potential to increase traffic throughput by allowing smaller headway between vehicles and moving vehicles safely in a platoon at a harmonized speed. CACC systems have been attracting significant attention from both academia and industry since connectivity between vehicles will become mandatory for new vehicles in the USA in the near future. In this paper, we review three basic and important aspects of CACC systems: communications, driver characteristics, and controls to identify the most challenging issues for their real-world deployment. Different routing protocols that support the data communication requirements between vehicles in the CACC platoon are reviewed. Promising and suitable protocols are identified. Driver characteristics related issues, such as how to keep drivers engaged in driving tasks during CACC operations, are discussed. To achieve mass acceptance, the control design needs to depict real-world traffic variability such as communication effects, driver behavior, and traffic composition. Thus, this paper also discusses the issues that existing CACC control modules face when considering close to ideal driving conditions.},
 author = {Dey, K. C. and Yan, L. and Wang, X. and Wang, Y. and Shen, H. and Chowdhury, M. and Yu, L. and Qiu, C. and Soundararaj, V.},
 doi = {10.1109/TITS.2015.2483063},
 file = {/home/matt/Zotero/storage/JJ2H8VLY/Dey et al. - 2016 - A Review of Communication, Driver Characteristics,.pdf;/home/matt/Zotero/storage/UQWVXLSD/7314936.html},
 issn = {1524-9050},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {2},
 pages = {491--509},
 title = {A {{Review}} of {{Communication}}, {{Driver Characteristics}}, and {{Controls Aspects}} of {{Cooperative Adaptive Cruise Control}} ({{CACC}})},
 volume = {17},
 year = {2016}
}

@article{dhillon_weighted_2007,
 author = {Dhillon, Inderjit S. and Guan, Yuqiang and Kulis, Brian},
 doi = {10.1109/TPAMI.2007.1115},
 issn = {0162-8828},
 journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
 number = {11},
 pages = {1944--1957},
 title = {Weighted {{Graph Cuts}} without {{Eigenvectors A Multilevel Approach}}},
 volume = {29},
 year = {2007}
}

@inproceedings{dhingra_differentiable_2020,
 author = {Bhuwan Dhingra and
Manzil Zaheer and
Vidhisha Balachandran and
Graham Neubig and
Ruslan Salakhutdinov and
William W. Cohen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/DhingraZBNSC20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Differentiable Reasoning over a Virtual Knowledge Base},
 url = {https://openreview.net/forum?id=SJxstlHFPH},
 year = {2020}
}

@article{diakaki_extensions_2003,
 abstract = {The objectives, approach, advantages, and some application results of recent extensions of the traffic-responsive urban control (TUC) strategy are presented.},
 author = {Diakaki, C. and Dinopoulou, V. and Aboudolas, K. and Papageorgiou, M. and {Ben-Shabat}, E. and Seider, E. and Leibov, A.},
 journal = {Transportation Research Record},
 pages = {202--211},
 title = {Extensions and {{New Applications}} of the {{Traffic}}-{{Responsive Urban Control Strategy}}},
 volume = {1856},
 year = {2003}
}

@article{diakaki_integrated_2000,
 author = {Diakaki, C. and Papageorgiou, M. and McLean, T.},
 journal = {Transportation Research Record},
 number = {1727},
 pages = {101--111},
 title = {Integrated {{Traffic}}-{{Responsive Urban Corridor Control Strategy}} in {{Glasgow}}, {{Scotland}}.},
 year = {2000}
}

@article{dial_minimal-revenue_1999,
 author = {Dial, R. B.},
 journal = {Transportation Research, Part B},
 number = {},
 pages = {189--202},
 title = {Minimal-Revenue Congestion Pricing Part {{I}}: {{A}} Fast Algorithm for the Single-Origin Case},
 volume = {33},
 year = {1999}
}

@article{diamond_impact_2009,
 author = {Diamond, David},
 doi = {http://dx.doi.org/10.1016/j.enpol.2008.09.094},
 issn = {0301-4215},
 journal = {Energy Policy},
 number = {3},
 pages = {972--983},
 title = {The Impact of Government Incentives for Hybrid-Electric Vehicles: {{Evidence}} from {{US}} States},
 volume = {37},
 year = {2009}
}

@article{dib_optimal_2014,
 author = {Dib, W. and Chasse, A. and Moulin, P. and Sciarretta, A. and Corde, G.},
 journal = {Control Engineering Practice},
 pages = {299--307},
 title = {Optimal Energy Management for an Electric Vehicle in Eco-Driving Applications},
 volume = {29},
 year = {2014}
}

@article{diehl_edge_2019,
 author = {Diehl, Frederik},
 journal = {ArXiv preprint},
 title = {Edge {{Contraction Pooling}} for {{Graph Neural Networks}}},
 url = {https://arxiv.org/abs/1905.10990},
 volume = {abs/1905.10990},
 year = {2019}
}

@article{dixon_real-time_2002,
 author = {Dixon, M. P. and Rilett, L. R.},
 journal = {Computer-Aided Civil and Infrastructure Engineering},
 pages = {7--21},
 title = {Real-Time {{OD}} Estimation Using Automatic Vehicle Identification and Traffic Count Data},
 volume = {17},
 year = {2002}
}

@book{dks_associates_2002_2003,
 author = {{DKS Associates}},
 title = {2002 {{High Occupancy Vehicle}} ({{HOV}}) {{Lane Master Plan Update}}. {{Prepared}} for {{Metropolitan Transportation Commission}}, {{Caltrans District}} 4 and the {{California Highway Patrol Golden Gate Division}}},
 year = {2003}
}

@book{dks_associates_interstate_2010,
 author = {{DKS Associates}},
 title = {Interstate 80 {{Integrated Corridor Mobility Project}}: {{Final Corridor System Management Plan}}},
 year = {2010}
}

@article{doersch_tutorial_2016,
 author = {Doersch, Carl},
 journal = {ArXiv preprint},
 title = {Tutorial on {{Variational Autoencoders}}},
 url = {https://arxiv.org/abs/1606.05908},
 volume = {abs/1606.05908},
 year = {2016}
}

@article{dogan_unified_2016,
 author = {Do{\u g}an, {\"U}r{\"u}n and Glasmachers, Tobias and Igel, Christian},
 file = {/home/matt/Zotero/storage/5Y69ETUP/11-229.pdf},
 journal = {Journal of Machine Learning Research},
 number = {45},
 pages = {1--32},
 title = {A {{Unified View}} on {{Multi}}-Class {{Support Vector Classification}}},
 volume = {17},
 year = {2016}
}

@inproceedings{dolgov_practical_2008,
 abstract = {We describe a practical path-planning algorithm that generates smooth paths for an autonomous vehicle operating in an unknown environment, where obstacles are detected online by the robot's sensors. This work was motivated by and experimentally validated in the 2007 DARPA Urban Challenge, where robotic vehicles had to autonomously navigate parking lots. Our approach has two main steps. The first step uses a variant of the well-known A* search algorithm, applied to the 3D kinematic state space of the vehicle, but with a modified state-update rule that captures the continuous state of the vehicle in the discrete nodes of A* (thus guaranteeing kinematic feasibility of the path). The second step then improves the quality of the solution via numeric non-linear optimization, leading to a local (and frequently global) optimum. The path-planning algorithm described in this paper was used by the Stanford Racing Teams robot, Junior, in the Urban Challenge. Junior demonstrated flawless performance in complex general path-planning tasks such as navigating parking lots and executing U-turns on blocked roads, with typical fullcycle replaning times of 50\textendash 300ms.},
 author = {Dolgov, Dmitri and Thrun, Sebastian and Montemerlo, Michael and Diebel, James},
 booktitle = {Proceedings of the 1st {{International Symposium}} on {{Search Techniques}} in {{Artificial Intelligence}} and {{Robotics}} ({{STAIR}})},
 file = {/home/matt/Zotero/storage/Z2FNT87R/Dolgov et al. - Practical Search Techniques in Path Planning for A.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {18--80},
 publisher = {{AAAI}},
 title = {Practical {{Search Techniques}} in {{Path Planning}} for {{Autonomous Driving}}},
 volume = {1001},
 year = {2008}
}

@inproceedings{dong_hawq_2019,
 author = {Zhen Dong and
Zhewei Yao and
Amir Gholami and
Michael W. Mahoney and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/DongYGMK19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00038},
 pages = {293--302},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {{HAWQ:} Hessian AWare Quantization of Neural Networks With Mixed-Precision},
 url = {https://doi.org/10.1109/ICCV.2019.00038},
 year = {2019}
}

@inproceedings{dong_hawq-v2_2019,
 author = {Zhen Dong and
Zhewei Yao and
Daiyaan Arfeen and
Amir Gholami and
Michael W. Mahoney and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/DongYAGMK20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {{HAWQ-V2:} Hessian Aware trace-Weighted Quantization of Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2020/hash/d77c703536718b95308130ff2e5cf9ee-Abstract.html},
 year = {2020}
}

@inproceedings{dosovitskiy_carla_2017,
 abstract = {We introduce CARLA, an open-source simulator for autonomous driving research. CARLA has been developed from the ground up to support development, training, and validation of autonomous urban driving systems. In addition to open-source code and protocols, CARLA provides open digital assets (urban layouts, buildings, vehicles) that were created for this purpose and can be used freely. The simulation platform supports flexible specification of sensor suites and environmental conditions. We use CARLA to study the performance of three approaches to autonomous driving: a classic modular pipeline, an endto-end model trained via imitation learning, and an end-to-end model trained via reinforcement learning. The approaches are evaluated in controlled scenarios of increasing difficulty, and their performance is examined via metrics provided by CARLA, illustrating the platform's utility for autonomous driving research.},
 address = {{Mountain View, USA}},
 archiveprefix = {arXiv},
 author = {Dosovitskiy, Alexey and Ros, German and Codevilla, Felipe and Lopez, Antonio and Koltun, Vladlen},
 booktitle = {Proceedings of the 1st {{Conference}} on {{Robot Learning}} ({{CoRL}})},
 eprint = {1711.03938},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/SWC5MTR4/Dosovitskiy et al. - 2017 - CARLA An Open Urban Driving Simulator.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 shorttitle = {{{CARLA}}},
 title = {{{CARLA}}: {{An Open Urban Driving Simulator}}},
 year = {2017}
}

@inproceedings{dosovitskiy_image_2020,
 author = {Alexey Dosovitskiy and
Lucas Beyer and
Alexander Kolesnikov and
Dirk Weissenborn and
Xiaohua Zhai and
Thomas Unterthiner and
Mostafa Dehghani and
Matthias Minderer and
Georg Heigold and
Sylvain Gelly and
Jakob Uszkoreit and
Neil Houlsby},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/DosovitskiyB0WZ21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {An Image is Worth 16x16 Words: Transformers for Image Recognition
at Scale},
 url = {https://openreview.net/forum?id=YicbFdNTTy},
 year = {2021}
}

@inproceedings{douc_comparison_2005,
 author = {Douc, Randal and Capp{\'e}, Olivier},
 booktitle = {Image and {{Signal Processing}} and {{Analysis}}, 2005. {{ISPA}} 2005. {{Proceedings}} of the 4th {{International Symposium}} On},
 file = {/home/matt/Zotero/storage/IMKHFUYE/douc_comparison_of_pf_resampling_schemes.pdf},
 pages = {64--69},
 publisher = {{IEEE}},
 title = {Comparison of Resampling Schemes for Particle Filtering},
 year = {2005}
}

@inproceedings{doucet_rao-blackwellised_2000,
 address = {{Stanford, California}},
 author = {Doucet, Arnaud and {\noopsort{freitas}}{de Freitas}, Nando and Murphy, Kevin and Russell, Stuart},
 booktitle = {Proceedings of the 16th {{Conference}} on {{Uncertainty}} in {{Artificial Intelligence}}},
 isbn = {1-55860-709-9},
 pages = {176--183},
 publisher = {{Morgan Kaufmann Publishers Inc.}},
 title = {Rao-Blackwellised {{Particle Filtering}} for {{Dynamic Bayesian Networks}}},
 year = {2000}
}

@incollection{doucet_tutorial_2011,
 author = {Doucet, Arnaud and Johansen, Adam M.},
 booktitle = {The {{Oxford Handbook}} of {{Nonlinear Filtering}}},
 file = {/home/matt/Zotero/storage/IWKTTHNH/doucet_johansen_tutorialPF2011.pdf},
 isbn = {978-0-19-953290-2},
 pages = {656--704},
 publisher = {{Oxford University Press}},
 title = {A Tutorial on Particle Filtering and Smoothing: {{Fifteen}} Years Later},
 year = {2011}
}

@book{dowling_associates_berkeley_transportation_systems_and_system_metrics_group_measuring_2002,
 author = {{Dowling Associates, Berkeley Transportation Systems and System Metrics Group}},
 title = {Measuring {{Non}}-{{Recurrent Traffic Congestion}}: {{Final Report}}},
 year = {2002}
}

@techreport{dowling_traffic_2012,
 author = {Dowling, R. and Ashiabor, S.},
 institution = {{Transportation Research Board}},
 number = {NCHRP 03-97},
 title = {Traffic {{Signal Analysis}} with {{Varying Demands}} and {{Capacities}}, {{Draft Final Report}}},
 year = {2012}
}

@article{downs_law_1962,
 author = {Downs, A.},
 journal = {Traffic Quarterly},
 pages = {393--409},
 title = {The Law of Peak Hour Expressway Congestion},
 volume = {16},
 year = {1962}
}

@article{doyle_architecture_2011,
 abstract = {This paper aims to bridge progress in neuroscience involving sophisticated quantitative analysis of behavior, including the use of robust control, with other relevant conceptual and theoretical frameworks from systems engineering, systems biology, and mathematics. Familiar and accessible case studies are used to illustrate concepts of robustness, organization, and architecture (modularity and protocols) that are central to understanding complex networks. These essential organizational features are hidden during normal function of a system but are fundamental for understanding the nature, design, and function of complex biologic and technologic systems.},
 author = {Doyle, John C. and Csete, Marie},
 doi = {10.1073/pnas.1103557108},
 file = {/home/matt/Zotero/storage/99LB2XBW/Doyle and Csete - 2011 - Architecture, constraints, and behavior.pdf;/home/matt/Zotero/storage/Y6ZRYD2D/15624.html},
 issn = {0027-8424, 1091-6490},
 journal = {Proceedings of the National Academy of Sciences},
 language = {en},
 number = {Supplement 3},
 pages = {15624--15630},
 pmid = {21788505},
 title = {Architecture, Constraints, and Behavior},
 volume = {108},
 year = {2011}
}

@inproceedings{drews_aggressive_2017,
 abstract = {We present a framework for vision-based model predictive control (MPC) for the task of aggressive, high-speed autonomous driving. Our approach uses deep convolutional neural networks to predict cos...},
 author = {Drews, Paul and Williams, Grady and Goldfain, Brian and Theodorou, Evangelos A. and Rehg, James M.},
 booktitle = {Conference on {{Robot Learning}}},
 file = {/home/matt/Zotero/storage/5H4GZGM8/Drews et al. - 2017 - Aggressive Deep Driving Combining Convolutional N.pdf;/home/matt/Zotero/storage/CIRQ6345/drews17a.html;/home/matt/Zotero/storage/YKC9QKLR/drews17a.html},
 issn = {2640-3498},
 language = {en},
 pages = {133--142},
 publisher = {{PMLR}},
 shorttitle = {Aggressive {{Deep Driving}}},
 title = {Aggressive {{Deep Driving}}: {{Combining Convolutional Neural Networks}} and {{Model Predictive Control}}},
 year = {2017}
}

@article{du_isolation_2014,
 author = {Du, Miao and Mhaskar, Prashant},
 doi = {10.1016/j.automatica.2014.02.017},
 file = {/home/matt/Zotero/storage/DW48DPX8/1-s2.0-S0005109814000557-main.pdf},
 issn = {00051098},
 journal = {Automatica},
 language = {en},
 number = {4},
 pages = {1066--1074},
 title = {Isolation and Handling of Sensor Faults in Nonlinear Systems},
 volume = {50},
 year = {2014}
}

@inproceedings{du_lifelong_2019,
 abstract = {Anomaly detection is essential towards ensuring system security and reliability. Powered by constantly generated system data, deep learning has been found both effective and flexible to use, with its ability to extract patterns without much domain knowledge. Existing anomaly detection research focuses on a scenario referred to as zero-positive, which means that the detection model is only trained for normal (i.e., negative) data. In a real application scenario, there may be additional manually inspected positive data provided after the system is deployed. We refer to this scenario as lifelong anomaly detection. However, we find that existing approaches are not easy to adopt such new knowledge to improve system performance.},
 address = {{London United Kingdom}},
 author = {Du, Min and Chen, Zhi and Liu, Chang and Oak, Rajvardhan and Song, Dawn},
 booktitle = {Proceedings of the 2019 {{ACM SIGSAC Conference}} on {{Computer}} and {{Communications Security}}},
 doi = {10.1145/3319535.3363226},
 file = {/home/matt/Zotero/storage/KMQ399GT/Du et al. - 2019 - Lifelong Anomaly Detection Through Unlearning.pdf},
 isbn = {978-1-4503-6747-9},
 language = {en},
 pages = {1283--1297},
 publisher = {{ACM}},
 title = {Lifelong {{Anomaly Detection Through Unlearning}}},
 year = {2019}
}

@article{du_model_2019,
 author = {Du, Yilun and Lin, Toru and Mordatch, Igor},
 journal = {ArXiv preprint},
 title = {Model {{Based Planning}} with {{Energy Based Models}}},
 url = {https://arxiv.org/abs/1909.06878},
 volume = {abs/1909.06878},
 year = {2019}
}

@inproceedings{du_robust_2020,
 author = {Min Du and
Ruoxi Jia and
Dawn Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/DuJS20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Robust anomaly detection and backdoor attack detection via differential
privacy},
 url = {https://openreview.net/forum?id=SJx0q1rtvS},
 year = {2020}
}

@inproceedings{duan_benchmarking_2016,
 author = {Yan Duan and
Xi Chen and
Rein Houthooft and
John Schulman and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/DuanCHSA16.bib},
 booktitle = {Proceedings of the 33nd International Conference on Machine Learning,
{ICML} 2016, New York City, NY, USA, June 19-24, 2016},
 editor = {Maria{-}Florina Balcan and
Kilian Q. Weinberger},
 pages = {1329--1338},
 publisher = {JMLR.org},
 series = {{JMLR} Workshop and Conference Proceedings},
 timestamp = {Wed, 29 May 2019 01:00:00 +0200},
 title = {Benchmarking Deep Reinforcement Learning for Continuous Control},
 url = {http://proceedings.mlr.press/v48/duan16.html},
 volume = {48},
 year = {2016}
}

@inproceedings{duan_fault_2005,
 author = {Duan, Zhuo-hua and Cai, Zi-xing and {Jin-xia}, Yu},
 booktitle = {Robotics and {{Automation}}, 2005. {{ICRA}} 2005. {{Proceedings}} of the 2005 {{IEEE International Conference}} On},
 file = {/home/matt/Zotero/storage/2U2WGVN9/01570640.pdf},
 pages = {3428--3433},
 publisher = {{IEEE}},
 shorttitle = {Fault Diagnosis and Fault Tolerant Control for Wheeled Mobile Robots under Unknown Environments},
 title = {Fault Diagnosis and Fault Tolerant Control for Wheeled Mobile Robots under Unknown Environments: {{A}} Survey},
 year = {2005}
}

@article{dumoulin_guide_2016,
 author = {Dumoulin, Vincent and Visin, Francesco},
 journal = {ArXiv preprint},
 title = {A Guide to Convolution Arithmetic for Deep Learning},
 url = {https://arxiv.org/abs/1603.07285},
 volume = {abs/1603.07285},
 year = {2016}
}

@unpublished{dumville_initial_2018,
 author = {Dumville, Mark},
 title = {Initial {{Findings}} from the {{STRIKE3 GNSS Interference Monitoring Network}}},
 year = {2018}
}

@inproceedings{duvenaud_convolutional_2015,
 author = {David Duvenaud and
Dougal Maclaurin and
Jorge Aguilera{-}Iparraguirre and
Rafael G{\'{o}}mez{-}Bombarelli and
Timothy Hirzel and
Al{\'{a}}n Aspuru{-}Guzik and
Ryan P. Adams},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/DuvenaudMABHAA15.bib},
 booktitle = {Advances in Neural Information Processing Systems 28: Annual Conference
on Neural Information Processing Systems 2015, December 7-12, 2015,
Montreal, Quebec, Canada},
 editor = {Corinna Cortes and
Neil D. Lawrence and
Daniel D. Lee and
Masashi Sugiyama and
Roman Garnett},
 pages = {2224--2232},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Convolutional Networks on Graphs for Learning Molecular Fingerprints},
 url = {https://proceedings.neurips.cc/paper/2015/hash/f9be311e65d81a9ad8150a60844bb94c-Abstract.html},
 year = {2015}
}

@article{dwivedi_generalization_2021,
 author = {Dwivedi, Vijay Prakash and Bresson, Xavier},
 journal = {ArXiv preprint},
 title = {A {{Generalization}} of {{Transformer Networks}} to {{Graphs}}},
 url = {https://arxiv.org/abs/2012.09699},
 volume = {abs/2012.09699},
 year = {2020}
}

@inproceedings{ebrahimi_uncertainty-guided_2019,
 author = {Sayna Ebrahimi and
Mohamed Elhoseiny and
Trevor Darrell and
Marcus Rohrbach},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/EbrahimiEDR20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Uncertainty-guided Continual Learning with Bayesian Neural Networks},
 url = {https://openreview.net/forum?id=HklUCCVKDB},
 year = {2020}
}

@inproceedings{edie_discussion_1965,
 author = {Edie, L. C.},
 booktitle = {Proceedings of the 2nd {{International Symposium}} on the {{Theory}} of {{Traffic Flow}}, {{Paris}}, {{France}}},
 title = {Discussion of Traffic Stream Measurements and Definitions},
 year = {1965}
}

@article{ekbatani_congestion_2012,
 author = {Ekbatani, M. K. and Kouvelas, A. and Papamichail, I. and Papageorgiou, M.},
 journal = {Transportation Research, Part B},
 pages = {1393--1403},
 title = {Congestion {{Control}} in {{Urban Networks}} via {{Feedback Gating}}},
 volume = {46},
 year = {2012}
}

@book{ekeland_infinite-dimensional_1983,
 address = {{Chicago}},
 author = {Ekeland, Ivar and Turnbull, Thomas},
 isbn = {978-0-226-19987-0 978-0-226-19988-7},
 lccn = {QA402.5 .E39 1983},
 publisher = {{University of Chicago Press}},
 series = {Chicago Lectures in Mathematics},
 title = {Infinite-Dimensional Optimization and Convexity},
 year = {1983}
}

@inproceedings{eliasof_diffgcn_2020,
 author = {Moshe Eliasof and
Eran Treister},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/EliasofT20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {DiffGCN: Graph Convolutional Networks via Differential Operators and
Algebraic Multigrid Pooling},
 url = {https://proceedings.neurips.cc/paper/2020/hash/d16a974d4d6d0d71b29bfbfe045f1da7-Abstract.html},
 year = {2020}
}

@article{elloumi_metacor_1994,
 author = {Elloumi, N. and Haj Salem, H. and Papageorgiou, M.},
 journal = {TRIennal Symposium on Transport Analysis, Capri},
 title = {{{METACOR}}: {{A}} Dynamic Macroscopic Modeling Tool for Urban Corridor.},
 volume = {1},
 year = {1994}
}

@article{elmer_bmw_2013,
 author = {Elmer, S},
 journal = {AutoGuide},
 title = {{{BMW Targets}} 2020 for {{Self}}-{{Driving Cars}}},
 year = {2013}
}

@article{elvira_adapting_2017,
 author = {Elvira, V{\'i}ctor and M{\'i}guez, Joaqu{\'i}n and Djuri{\'c}, Petar M.},
 doi = {10.1109/TSP.2016.2637324},
 file = {/home/matt/Zotero/storage/5NY7Q98R/elvira_djuric_adapting_number_particles_2017_arxiv.pdf},
 issn = {1053-587X, 1941-0476},
 journal = {IEEE Transactions on Signal Processing},
 number = {7},
 pages = {1781--1794},
 title = {Adapting the {{Number}} of {{Particles}} in {{Sequential Monte Carlo Methods}} through an {{Online Scheme}} for {{Convergence Assessment}}},
 volume = {65},
 year = {2017}
}

@misc{erdos_team_erdos_2020,
 abstract = {Elastic Robot Dataflow Operating System. Contribute to erdos-project/erdos development by creating an account on GitHub.},
 author = {{ERDOS Team}},
 copyright = {Apache-2.0 License         ,                 Apache-2.0 License},
 howpublished = {ERDOS},
 title = {{{ERDOS}}: {{Elastic Robot Dataflow Operating System}}},
 year = {2020}
}

@inproceedings{eysenbach_rewriting_2020,
 author = {Ben Eysenbach and
Xinyang Geng and
Sergey Levine and
Russ R. Salakhutdinov},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/EysenbachGLS20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Rewriting History with Inverse {RL:} Hindsight Inference for Policy
Improvement},
 url = {https://proceedings.neurips.cc/paper/2020/hash/a97da629b098b75c294dffdc3e463904-Abstract.html},
 year = {2020}
}

@article{fagnant_preparing_2015,
 abstract = {Autonomous vehicles (AVs) represent a potentially disruptive yet beneficial change to our transportation system. This new technology has the potential to impact vehicle safety, congestion, and travel behavior. All told, major social AV impacts in the form of crash savings, travel time reduction, fuel efficiency and parking benefits are estimated to approach \$2000 to per year per AV, and may eventually approach nearly \$4000 when comprehensive crash costs are accounted for. Yet barriers to implementation and mass-market penetration remain. Initial costs will likely be unaffordable. Licensing and testing standards in the U.S. are being developed at the state level, rather than nationally, which may lead to inconsistencies across states. Liability details remain undefined, security concerns linger, and without new privacy standards, a default lack of privacy for personal travel may become the norm. The impacts and interactions with other components of the transportation system, as well as implementation details, remain uncertain. To address these concerns, the federal government should expand research in these areas and create a nationally recognized licensing framework for AVs, determining appropriate standards for liability, security, and data privacy.},
 author = {Fagnant, Daniel J. and Kockelman, Kara},
 doi = {10.1016/j.tra.2015.04.003},
 file = {/home/matt/Zotero/storage/FAHZHY5F/Fagnant and Kockelman - 2015 - Preparing a nation for autonomous vehicles opport.pdf;/home/matt/Zotero/storage/HW6EXUV3/S0965856415000804.html},
 issn = {0965-8564},
 journal = {Transportation Research Part A: Policy and Practice},
 pages = {167--181},
 shorttitle = {Preparing a Nation for Autonomous Vehicles},
 title = {Preparing a Nation for Autonomous Vehicles: Opportunities, Barriers and Policy Recommendations},
 volume = {77},
 year = {2015}
}

@article{fan_collapsed_2017,
 author = {Fan, Shimao and Sun, Ye and Piccoli, Benedetto and Seibold, Benjamin and Work, Daniel B.},
 journal = {ArXiv preprint},
 title = {A {{Collapsed Generalized Aw}}-{{Rascle}}-{{Zhang Model}} and {{Its Model Accuracy}}},
 url = {https://arxiv.org/abs/1702.03624},
 volume = {abs/1702.03624},
 year = {2017}
}

@article{fang_smart_2012,
 author = {Fang, Xi and Misra, Satyajayant and Xue, Guoliang and Yang, Dejun},
 doi = {10.1109/SURV.2011.101911.00087},
 file = {/home/matt/Zotero/storage/4I3FNIG5/fang_smartgrid.pdf},
 issn = {1553-877X},
 journal = {IEEE Communications Surveys \& Tutorials},
 number = {4},
 pages = {944--980},
 shorttitle = {Smart {{Grid}} \&\#x2014; {{The New}} and {{Improved Power Grid}}},
 title = {Smart {{Grid}} \&\#x2014; {{The New}} and {{Improved Power Grid}}: {{A Survey}}},
 volume = {14},
 year = {24}
}

@inproceedings{farhi_logit_2013,
 author = {Farhi, Nadir and {Haj-Salem}, Habib and Khoshyaran, Megan and Lebacque, Jean-Patrick and Salvarani, Francesco and Schnetzler, Bernard and De Vuyst, Florian},
 booktitle = {Transportation {{Research Board}} 92nd {{Annual Meeting Compendium}} of {{Papers}}},
 title = {The {{Logit}} Lane Assignment Model: First Results},
 year = {2013}
}

@article{fasshauer_solving_2015,
 abstract = {In this paper we solve support vector machines in reproducing kernel Banach spaces (RKBSs) instead of the traditional methods in reproducing kernel Hilbert spaces (RKHSs). Using the orthogonality of semi-inner-products of RKBSs, we can obtain the finite-dimensional representations of the dual (normalized-duality-mapping) elements of support vector machine solutions. In addition, we can use Fourier transform techniques to introduce the concept of reproduction in a generalized native space such that it becomes a reproducing kernel Banach space, which can even be embedded into Sobolev spaces. Moreover, its reproducing kernel is associated with a positive definite function. The representations of the optimal solutions of support vector machines (regularized empirical risks) in these reproducing kernel Banach spaces are formulated explicitly and finite-dimensionally in terms of the positive definite functions, and their finite numbers of suitable parameters can be computed by the fixed point iteration. We also give some typical examples of reproducing kernel Banach spaces induced by Mat\'ern functions (Sobolev splines) such that their support vector machine solutions even are computable efficiently. Moreover, each of their reproducing bases includes information from multiple training data points. These kernel-based algorithms give a fresh numerical tool for support vector classifiers.},
 author = {Fasshauer, Gregory E. and Hickernell, Fred J. and Ye, Qi},
 doi = {10.1016/j.acha.2014.03.007},
 file = {/home/matt/Zotero/storage/AHRJT932/Fasshauer et al. - 2015 - Solving support vector machines in reproducing ker.pdf;/home/matt/Zotero/storage/2JDS5R85/S1063520314000475.html},
 issn = {1063-5203},
 journal = {Applied and Computational Harmonic Analysis},
 language = {en},
 number = {1},
 pages = {115--139},
 title = {Solving Support Vector Machines in Reproducing Kernel {{Banach}} Spaces with Positive Definite Functions},
 volume = {38},
 year = {2015}
}

@article{faust_evolving_2019,
 author = {Faust, Aleksandra and Francis, Anthony and Mehta, Dar},
 journal = {ArXiv preprint},
 title = {Evolving {{Rewards}} to {{Automate Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1905.07628},
 volume = {abs/1905.07628},
 year = {2019}
}

@article{fax_information_2004,
 author = {Fax, J. A. and Murray, R. M.},
 journal = {IEEE Trans. Auto. Contr.},
 number = {9},
 pages = {1465--1476},
 title = {Information Flow and Cooperative Control of Vehicle Formations},
 volume = {49},
 year = {2004}
}

@techreport{federal_highway_administration_11th_2003,
 address = {{Washington DC}},
 author = {{Federal Highway Administration}},
 number = {FHWA-OP-03-100},
 title = {11th {{International Conference}} on {{High}}-{{Occupancy Vehicle Systems Conference Proceedings}}, {{October}} 2002, {{Seattle}}, {{WA}}},
 year = {2003}
}

@article{federal_highway_administration_demo_1997,
 author = {{Federal Highway Administration}},
 journal = {Public Roads},
 number = {1},
 title = {Demo '97: {{Proving AHS Works}}},
 volume = {61},
 year = {1997}
}

@techreport{federal_highway_administration_traffic_2008,
 author = {{Federal Highway Administration}},
 institution = {{U.S. Department of Transportation}},
 number = {FHWA-HOP-08-024},
 title = {Traffic {{Signal Timing Manual}}},
 year = {2008}
}

@article{feldman_optmization_2002,
 author = {Feldman, O. and Maher, M.},
 journal = {34th Annual Universities' Transport Study Group Conference, Napier University, Edinburgh},
 title = {Optmization of Traffic Signals Using a Cell Transmission Model.},
 year = {2002}
}

@inproceedings{feng_codebert_2020,
 address = {Online},
 author = {Feng, Zhangyin  and
Guo, Daya  and
Tang, Duyu  and
Duan, Nan  and
Feng, Xiaocheng  and
Gong, Ming  and
Shou, Linjun  and
Qin, Bing  and
Liu, Ting  and
Jiang, Daxin  and
Zhou, Ming},
 booktitle = {Findings of the Association for Computational Linguistics: EMNLP 2020},
 doi = {10.18653/v1/2020.findings-emnlp.139},
 pages = {1536--1547},
 publisher = {Association for Computational Linguistics},
 title = {{C}ode{BERT}: A Pre-Trained Model for Programming and Natural Languages},
 url = {https://aclanthology.org/2020.findings-emnlp.139},
 year = {2020}
}

@inproceedings{fernandes_structured_2020,
 author = {Patrick Fernandes and
Miltiadis Allamanis and
Marc Brockschmidt},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/FernandesAB19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Structured Neural Summarization},
 url = {https://openreview.net/forum?id=H1ersoRqtm},
 year = {2019}
}

@book{ferrara_freeway_2018,
 address = {{Cham}},
 author = {Ferrara, Antonella and Sacone, Simona and Siri, Silvia},
 doi = {10.1007/978-3-319-75961-6},
 file = {/home/matt/Zotero/storage/XIQ85XGI/2018 - Freeway traffic modelling and control.pdf},
 isbn = {978-3-319-75959-3 978-3-319-75961-6},
 publisher = {{Springer International Publishing}},
 title = {Freeway {{Traffic Modelling}} and {{Control}}},
 year = {2018}
}

@incollection{ferrara_state_2018,
 address = {{Cham}},
 author = {Ferrara, Antonella and Sacone, Simona and Siri, Silvia},
 booktitle = {Freeway {{Traffic Modelling}} and {{Control}}},
 isbn = {978-3-319-75961-6},
 pages = {169--190},
 publisher = {{Springer International Publishing}},
 title = {State {{Estimation}} in {{Freeway Traffic Systems}}},
 year = {2018}
}

@article{feygin_bistro_2019,
 author = {Feygin, Sidney A. and Lazarus, Jessica R. and Forscher, Edward H. and {Golfier-Vetterli}, Valentine and Lee, Jonathan W. and Gupta, Abhishek and Waraich, Rashid A. and Sheppard, Colin J. R. and Bayen, Alexandre M.},
 journal = {ArXiv preprint},
 title = {{{BISTRO}}: {{Berkeley Integrated System}} for {{Transportation Optimization}}},
 url = {https://arxiv.org/abs/1908.03821},
 volume = {abs/1908.03821},
 year = {2019}
}

@book{fhwa_moving_2012,
 author = {{FHWA}},
 title = {Moving {{Ahead}} for {{Progress}} in the 21st {{Century Act}} ({{MAP}}-21)},
 year = {2012}
}

@inproceedings{filos_can_2020,
 author = {Angelos Filos and
Panagiotis Tigkas and
Rowan McAllister and
Nicholas Rhinehart and
Sergey Levine and
Yarin Gal},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/FilosTMRLG20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {3145--3153},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Can Autonomous Vehicles Identify, Recover From, and Adapt to Distribution
Shifts?},
 url = {http://proceedings.mlr.press/v119/filos20a.html},
 volume = {119},
 year = {2020}
}

@inproceedings{firoozi_safe_2019,
 abstract = {We present the design of a safe Adaptive Cruise Control (ACC) which uses road grade and lead vehicle motion preview. The ACC controller is designed by using a Model Predictive Control (MPC) framework to optimize comfort, safety, energy-efficiency and speed tracking accuracy. Safety is achieved by online computation of a robust invariant terminal set. The paper presents a novel approach to compute such set which is less conservative than existing methods. The proposed controller ensures safe inter-vehicle spacing at all times despite changes in the road grade and uncertainty in the predicted motion of the lead vehicle. Simulation results compare the proposed controller with a controller that does not incorporate prior grade knowledge on two scenarios including car-following and autonomous intersection crossing. The results demonstrate the effectiveness of the proposed control algorithm.},
 author = {Firoozi, R. and Nazari, S. and Guanetti, J. and O'Gorman, R. and Borrelli, F.},
 booktitle = {2019 {{American Control Conference}} ({{ACC}})},
 file = {/home/matt/Zotero/storage/V9DGG78H/Firoozi et al_2019_Safe Adaptive Cruise Control with Road Grade Preview and $-mathbfV2-mathbfV$.pdf;/home/matt/Zotero/storage/GRRSWY53/8814928.html},
 pages = {4448--4453},
 title = {Safe {{Adaptive Cruise Control}} with {{Road Grade Preview}} and \$\textbackslash{{mathbfV2}}\textbackslash{{mathbfV}}\$ {{Communication}}},
 year = {2019}
}

@inproceedings{fisac_hierarchical_2019,
 abstract = {The actions of an autonomous vehicle on the road affect and are affected by those of other drivers, whether overtaking, negotiating a merge, or avoiding an accident. This mutual dependence, best captured by dynamic game theory, creates a strong coupling between the vehicle's planning and its predictions of other drivers' behavior, and constitutes an open problem with direct implications on the safety and viability of autonomous driving technology. Unfortunately, dynamic games are too computationally demanding to meet the real-time constraints of autonomous driving in its continuous state and action space. In this paper, we introduce a novel game-theoretic trajectory planning algorithm for autonomous driving, that enables real-time performance by hierarchically decomposing the underlying dynamic game into a long-horizon ``strategic'' game with simplified dynamics and full information structure, and a short-horizon ``tactical'' game with full dynamics and a simplified information structure. The value of the strategic game is used to guide the tactical planning, implicitly extending the planning horizon, pushing the local trajectory optimization closer to global solutions, and, most importantly, quantitatively accounting for the autonomous vehicle and the human driver's ability and incentives to influence each other. In addition, our approach admits non-deterministic models of human decision-making, rather than relying on perfectly rational predictions. Our results showcase richer, safer, and more effective autonomous behavior in comparison to existing techniques.},
 author = {Fisac, Jaime F. and Bronstein, Eli and Stefansson, Elis and Sadigh, Dorsa and Sastry, S. Shankar and Dragan, Anca D.},
 booktitle = {2019 {{International Conference}} on {{Robotics}} and {{Automation}} ({{ICRA}})},
 doi = {10.1109/ICRA.2019.8794007},
 file = {/home/matt/Zotero/storage/5ITCZ94I/Fisac et al. - 2019 - Hierarchical Game-Theoretic Planning for Autonomou.pdf;/home/matt/Zotero/storage/9F6VJYNE/8794007.html},
 issn = {1050-4729},
 pages = {9590--9596},
 title = {Hierarchical {{Game}}-{{Theoretic Planning}} for {{Autonomous Vehicles}}},
 year = {2019}
}

@article{fisher_logic_1935,
 author = {Fisher, R. A.},
 doi = {10.2307/2342435},
 file = {/home/matt/Zotero/storage/S2WSCFU9/Fisher - 1935 - The Logic of Inductive Inference.pdf},
 issn = {0952-8385},
 journal = {Journal of the Royal Statistical Society},
 number = {1},
 pages = {39--82},
 title = {The {{Logic}} of {{Inductive Inference}}},
 volume = {98},
 year = {1935}
}

@article{fisher_statistical_1935,
 author = {Fisher, Ronald Aylmer},
 journal = {Nature},
 pages = {474},
 title = {Statistical Tests},
 volume = {136},
 year = {1935}
}

@article{fitzpatrick_operating_2017,
 author = {Fitzpatrick, Kay and Avelar, Raul and Lindheimer, Tom{\'a}s E.},
 doi = {10.3141/2616-01},
 file = {/home/matt/Zotero/storage/ZQW2N99N/Fitzpatrick et al. - 2017 - Operating Speed on a Buffer-Separated Managed Lane.pdf},
 issn = {0361-1981, 2169-4052},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 number = {1},
 pages = {1--9},
 title = {Operating {{Speed}} on a {{Buffer}}-{{Separated Managed Lane}}},
 volume = {2616},
 year = {2017}
}

@article{fletcher_mitcornell_2008,
 author = {Fletcher, Luke and Teller, Seth and Olson, Edwin and Moore, David and Kuwata, Yoshiaki and How, Jonathan and Leonard, John and Miller, Isaac and Campbell, Mark and Huttenlocher, Dan and Nathan, Aaron and Kline, Frank-Robert},
 journal = {ArXiv preprint},
 title = {The {{MIT}}\textendash{{Cornell}} Collision and Why It Happened},
 url = {https://arxiv.org/abs/10.1002},
 volume = {abs/10.1002},
 year = {2010}
}

@book{florida_department_of_transportation_lpr_2006,
 author = {{Florida Department of Transportation}},
 title = {{{LPR Field Test Results Report}}},
 year = {2006}
}

@article{flotterod_operational_2011,
 author = {Fl{\"o}tter{\"o}d, Gunnar and Rohde, Jannis},
 doi = {10.1016/j.trb.2011.04.001},
 file = {/home/matt/Documents/Papers/flotterod_2011_TRB_operational_macroscopic.pdf;/home/matt/Zotero/storage/5INN78Q6/flotterod_2011_TRB_operational_macroscopic.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {6},
 pages = {903--922},
 title = {Operational Macroscopic Modeling of Complex Urban Road Intersections},
 volume = {45},
 year = {2011}
}

@article{flury_bayesian_2011,
 author = {Flury, Thomas and Shephard, Neil},
 doi = {10.1017/S0266466610000599},
 file = {/home/matt/Zotero/storage/KCU5E2WF/S0266466610000599a.pdf},
 issn = {0266-4666, 1469-4360},
 journal = {Econometric Theory},
 language = {en},
 number = {05},
 pages = {933--956},
 shorttitle = {{{BAYESIAN INFERENCE BASED ONLY ON SIMULATED LIKELIHOOD}}},
 title = {Bayesian {{Inference Based}} Only on {{Simulated Likelihood}}: {{Particle Filter Analysis}} of {{Dynamic Economic Models}}},
 volume = {27},
 year = {2011}
}

@inproceedings{foerster_counterfactual_2018,
 author = {Jakob N. Foerster and
Gregory Farquhar and
Triantafyllos Afouras and
Nantas Nardelli and
Shimon Whiteson},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/FoersterFANW18.bib},
 booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
(AAAI-18), the 30th innovative Applications of Artificial Intelligence
(IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
Artificial Intelligence (EAAI-18), New Orleans, Louisiana, USA, February
2-7, 2018},
 editor = {Sheila A. McIlraith and
Kilian Q. Weinberger},
 pages = {2974--2982},
 publisher = {{AAAI} Press},
 timestamp = {Mon, 22 Oct 2018 01:00:00 +0200},
 title = {Counterfactual Multi-Agent Policy Gradients},
 url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/17193},
 year = {2018}
}

@inproceedings{foerster_learning_2016,
 author = {Jakob N. Foerster and
Yannis M. Assael and
Nando de Freitas and
Shimon Whiteson},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/FoersterAFW16.bib},
 booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
on Neural Information Processing Systems 2016, December 5-10, 2016,
Barcelona, Spain},
 editor = {Daniel D. Lee and
Masashi Sugiyama and
Ulrike von Luxburg and
Isabelle Guyon and
Roman Garnett},
 pages = {2137--2145},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Learning to Communicate with Deep Multi-Agent Reinforcement Learning},
 url = {https://proceedings.neurips.cc/paper/2016/hash/c7635bfd99248a2cdef8249ef7bfbef4-Abstract.html},
 year = {2016}
}

@inproceedings{ford_adversarial_2019,
 author = {Justin Gilmer and
Nicolas Ford and
Nicholas Carlini and
Ekin D. Cubuk},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/GilmerFCC19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {2280--2289},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Adversarial Examples Are a Natural Consequence of Test Error in Noise},
 url = {http://proceedings.mlr.press/v97/gilmer19a.html},
 volume = {97},
 year = {2019}
}

@article{fox_hierarchical_2019,
 author = {Fox, Roy and Shin, Richard and Paul, William and Zou, Yitian and Song, Dawn and Goldberg, Ken and Abbeel, Pieter and Stoica, Ion},
 journal = {ArXiv preprint},
 title = {Hierarchical {{Variational Imitation Learning}} of {{Control Programs}}},
 url = {https://arxiv.org/abs/1912.12612},
 volume = {abs/1912.12612},
 year = {2019}
}

@article{frazier_chaos_2004,
 abstract = {Chaos theory is used to analyze highly complex systems and thus may be useful for transportation applications. A series of analyses with which to find and exploit chaos is outlined, including time delays and embedding dimensions, Fourier power series, the correlation dimension, the largest Lyapunov exponent, and predictions. As an example, traffic flow data are analyzed and found to be chaotic, although it is shown that this could be the result of high-frequency noise. When used with a low-pass filter, predictions based on chaos theory are shown to have greater predictive power than a nonlinear least-squares method.},
 author = {Frazier, Christopher and Kockelman, Kara M.},
 doi = {10.3141/1897-02},
 file = {/home/matt/Zotero/storage/58I263R2/Frazier and Kockelman - 2004 - Chaos Theory and Transportation Systems Instructi.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 language = {en},
 number = {1},
 pages = {9--17},
 shorttitle = {Chaos {{Theory}} and {{Transportation Systems}}},
 title = {Chaos {{Theory}} and {{Transportation Systems}}: {{Instructive Example}}},
 volume = {1897},
 year = {2004}
}

@article{fremont_formal_2020,
 author = {Fremont, Daniel J. and Kim, Edward and Pant, Yash Vardhan and Seshia, Sanjit A. and Acharya, Atul and Bruso, Xantha and Wells, Paul and Lemke, Steve and Lu, Qiang and Mehta, Shalin},
 journal = {ArXiv preprint},
 title = {Formal {{Scenario}}-{{Based Testing}} of {{Autonomous Vehicles}}: {{From Simulation}} to the {{Real World}}},
 url = {https://arxiv.org/abs/2003.07739},
 volume = {abs/2003.07739},
 year = {2020}
}

@inproceedings{fremont_scenic_2019,
 address = {{Phoenix, AZ, USA}},
 author = {Fremont, Daniel J. and Dreossi, Tommaso and Ghosh, Shromona and Yue, Xiangyu and {Sangiovanni-Vincentelli}, Alberto L. and Seshia, Sanjit A.},
 booktitle = {Proceedings of the 40th {{ACM SIGPLAN Conference}} on {{Programming Language Design}} and {{Implementation}}  - {{PLDI}} 2019},
 doi = {10.1145/3314221.3314633},
 file = {/home/matt/Zotero/storage/W53PCNL9/Fremont et al. - 2019 - Scenic a language for scenario specification and .pdf},
 isbn = {978-1-4503-6712-7},
 language = {en},
 pages = {63--78},
 publisher = {{ACM Press}},
 shorttitle = {Scenic},
 title = {Scenic: A Language for Scenario Specification and Scene Generation},
 year = {2019}
}

@article{fu_analysis_2002,
 author = {Fu, T. T. and Cebon, D.},
 journal = {Int. J. Heavy Vehicle Systems},
 pages = {281--297},
 title = {Analysis of a Truck Suspension Database},
 volume = {19},
 year = {2002}
}

@inproceedings{fu_diagnosing_2019,
 author = {Justin Fu and
Aviral Kumar and
Matthew Soh and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/FuKSL19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {2021--2030},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Diagnosing Bottlenecks in Deep Q-learning Algorithms},
 url = {http://proceedings.mlr.press/v97/fu19a.html},
 volume = {97},
 year = {2019}
}

@article{funahashi_approximate_1989,
 abstract = {In this paper, we prove that any continuous mapping can be approximately realized by RumelhartHinton-Williams' multilayer neural networks with at least one hidden layer whose output functions are sigmoid functions. The starting point of the proof for the one hidden layer case is an integral formula recently proposed by Irie-Miyake and from this, the general case (for any number of hidden layers) can be proved by induction.},
 author = {Funahashi, Ken-Ichi},
 doi = {10.1016/0893-6080(89)90003-8},
 file = {/home/matt/Zotero/storage/YVSZ4GRK/Funahashi - 1989 - On the approximate realization of continuous mappi.pdf},
 issn = {08936080},
 journal = {Neural Networks},
 language = {en},
 number = {3},
 pages = {183--192},
 title = {On the Approximate Realization of Continuous Mappings by Neural Networks},
 volume = {2},
 year = {1989}
}

@article{g._gomes_optimal_2006,
 author = {{G. Gomes} and Horowitz, R.},
 journal = {Transportation Research, Part C},
 number = {4},
 pages = {244--262},
 title = {Optimal Freeway Ramp Metering Using the Asymmetric Cell Transmission Model},
 volume = {14},
 year = {2006}
}

@article{galceran_multipolicy_2017,
 author = {Galceran, Enric and Cunningham, Alexander G. and Eustice, Ryan M. and Olson, Edwin},
 doi = {10.1007/s10514-017-9619-z},
 file = {/home/matt/Zotero/storage/RIUSMTD6/Galceran et al. - 2017 - Multipolicy decision-making for autonomous driving.pdf},
 issn = {0929-5593, 1573-7527},
 journal = {Autonomous Robots},
 language = {en},
 number = {6},
 pages = {1367--1382},
 shorttitle = {Multipolicy Decision-Making for Autonomous Driving via Changepoint-Based Behavior Prediction},
 title = {Multipolicy Decision-Making for Autonomous Driving via Changepoint-Based Behavior Prediction: {{Theory}} and Experiment},
 volume = {41},
 year = {2017}
}

@article{gale_theorem_1957,
 author = {Gale, David},
 journal = {Pacific J. Math.},
 number = {2},
 pages = {1073--1082},
 title = {A Theorem on Flows in Networks},
 volume = {7},
 year = {1957}
}

@article{gannes_san_2013,
 author = {Gannes, L.},
 journal = {AllThingsD},
 title = {San {{Francisco May Crack Down}} on {{Corporate Shuttle Buses}}},
 year = {2013}
}

@inproceedings{gao_graph_2019,
 author = {Hongyang Gao and
Shuiwang Ji},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/GaoJ19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {2083--2092},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Graph U-Nets},
 url = {http://proceedings.mlr.press/v97/gao19a.html},
 volume = {97},
 year = {2019}
}

@article{gao_survey_2015,
 author = {Gao, Zhiwei and Cecati, Carlo and Ding, Steven X.},
 doi = {10.1109/TIE.2015.2417501},
 file = {/home/matt/Zotero/storage/R5RJC2NE/gao_surveyoffault_part1.pdf},
 issn = {0278-0046, 1557-9948},
 journal = {IEEE Transactions on Industrial Electronics},
 number = {6},
 pages = {3757--3767},
 shorttitle = {A {{Survey}} of {{Fault Diagnosis}} and {{Fault}}-{{Tolerant Techniques}}\&amp;\#x2014;{{Part I}}},
 title = {A {{Survey}} of {{Fault Diagnosis}} and {{Fault}}-{{Tolerant Techniques}} -- {{Part I}}: {{Fault Diagnosis With Model}}-{{Based}} and {{Signal}}-{{Based Approaches}}},
 volume = {62},
 year = {2015}
}

@article{garavello_traffic_2006,
 author = {Garavello, Mauro and Piccoli, Benedetto},
 doi = {10.1080/03605300500358053},
 file = {/home/matt/Zotero/storage/4XSTUQK3/garavello_piccolli_network_awrascle.pdf},
 issn = {0360-5302, 1532-4133},
 journal = {Communications in Partial Differential Equations},
 language = {en},
 number = {2},
 pages = {243--275},
 title = {Traffic {{Flow}} on a {{Road Network Using}} the {{Aw}}\textendash{{Rascle Model}}},
 volume = {31},
 year = {2006}
}

@article{gartner_arterial-based_2002,
 author = {Gartner, N. and Stamadiadis, C.},
 journal = {Mathematical and Computer Modelling},
 pages = {657--671},
 title = {Arterial-Based Control of Traffic Flow in Urban Grid Networks},
 volume = {35},
 year = {2002}
}

@article{gartner_multi-band_1991,
 author = {Gartner, N. and Assman, S. and Lasaga, F. and Hou, D.},
 journal = {Transportation Research, Part B},
 number = {1},
 pages = {55--74},
 title = {A Multi-Band Approach to Arterial Traffic Signal Optimization},
 volume = {25},
 year = {1991}
}

@inproceedings{gaskell_hardshoulder_2004,
 author = {Gaskell, A. and Gasson, J. and Beale, S.},
 booktitle = {12th {{IEE International Conference}} on {{Road Transport Information}} and {{Control}}},
 pages = {154--159},
 title = {Hardshoulder Monitoring System for Active Traffic Management},
 year = {2004}
}

@article{gazis_car-following_1959,
 author = {Gazis, Denos C. and Herman, Robert and Potts, Renfrey B.},
 doi = {10.1287/opre.7.4.499},
 journal = {Operations Research},
 number = {4},
 pages = {499--505},
 title = {Car-{{Following Theory}} of {{Steady}}-{{State Traffic Flow}}},
 volume = {7},
 year = {1959}
}

@article{gazis_density_1962,
 author = {Gazis, Denos C. and Herman, Robert and Weiss, George H.},
 doi = {10.1287/opre.10.5.658},
 journal = {Operations Research},
 number = {5},
 pages = {658--667},
 title = {Density {{Oscillations Between Lanes}} of a {{Multilane Highway}}},
 volume = {10},
 year = {1962}
}

@article{ge_dynamics_2014,
 author = {Ge, Jin I. and Orosz, G{\'a}bor},
 doi = {10.1016/j.trc.2014.04.014},
 issn = {0968-090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 pages = {46--64},
 title = {Dynamics of Connected Vehicle Systems with Delayed Acceleration Feedback},
 volume = {46},
 year = {2014}
}

@article{gealy_quasi-direct_2019,
 author = {Gealy, David V. and McKinley, Stephen and Yi, Brent and Wu, Philipp and Downey, Phillip R. and Balke, Greg and Zhao, Allan and Guo, Menglong and Thomasson, Rachel and Sinclair, Anthony and Cuellar, Peter and McCarthy, Zoe and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {Quasi-{{Direct Drive}} for {{Low}}-{{Cost Compliant Robotic Manipulation}}},
 url = {https://arxiv.org/abs/1904.03815},
 volume = {abs/1904.03815},
 year = {2019}
}

@inproceedings{gehring_convolutional_2017,
 author = {Jonas Gehring and
Michael Auli and
David Grangier and
Denis Yarats and
Yann N. Dauphin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/GehringAGYD17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {1243--1252},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Convolutional Sequence to Sequence Learning},
 url = {http://proceedings.mlr.press/v70/gehring17a.html},
 volume = {70},
 year = {2017}
}

@article{geiger_vision_2013,
 abstract = {We present a novel dataset captured from a VW station wagon for use in mobile robotics and autonomous driving research. In total, we recorded 6 hours of traffic scenarios at 10\textendash 100 Hz using a variety of sensor modalities such as high-resolution color and grayscale stereo cameras, a Velodyne 3D laser scanner and a high-precision GPS/IMU inertial navigation system. The scenarios are diverse, capturing real-world traffic situations, and range from freeways over rural areas to inner-city scenes with many static and dynamic objects. Our data is calibrated, synchronized and timestamped, and we provide the rectified and raw image sequences. Our dataset also contains object labels in the form of 3D tracklets, and we provide online benchmarks for stereo, optical flow, object detection and other tasks. This paper describes our recording platform, the data format and the utilities that we provide.},
 author = {Geiger, A and Lenz, P and Stiller, C and Urtasun, R},
 doi = {10.1177/0278364913491297},
 file = {/home/matt/Zotero/storage/BF3CKPX2/Geiger et al. - 2013 - Vision meets robotics The KITTI dataset.pdf},
 issn = {0278-3649},
 journal = {The International Journal of Robotics Research},
 language = {en},
 number = {11},
 pages = {1231--1237},
 publisher = {{SAGE Publications Ltd STM}},
 shorttitle = {Vision Meets Robotics},
 title = {Vision Meets Robotics: {{The KITTI}} Dataset},
 volume = {32},
 year = {2013}
}

@article{genders_using_2016,
 author = {Genders, Wade and Razavi, Saiedeh},
 journal = {ArXiv preprint},
 title = {Using a {{Deep Reinforcement Learning Agent}} for {{Traffic Signal Control}}},
 url = {https://arxiv.org/abs/1611.01142},
 volume = {abs/1611.01142},
 year = {2016}
}

@techreport{general_growth_2007,
 author = {General, Office of Inspector},
 institution = {{Department of Transportation}},
 number = {Project ID: CR-2007-079},
 title = {Growth in {{Highway Construction}} and {{Maintenance Costs}}},
 year = {2007}
}

@article{gentile_spillback_2007,
 author = {Gentile, G. and Meschini, L. and Papola, N.},
 doi = {10.1016/j.trb.2007.04.011},
 journal = {Transportation Research Part B: Methodological},
 number = {10},
 pages = {1114--1138},
 title = {Spillback Congestion in Dynamic Traffic Assignment: A Macroscopic Flow Model with Time-Varying Bottlenecks.},
 volume = {41},
 year = {2007}
}

@incollection{georgiev_construction_2014,
 abstract = {We extend the idea of reproducing kernel Hilbert spaces (RKHS) to Banach spaces, developing a theory of pairs of reproducing kernel Banach spaces (RKBS) without the requirement of existence of semi-inner product (which requirement is already explored in another construction of RKBS). We present several natural examples, which involve RKBS of functions with supremum norm and with {$\mathscr{l}$}p-norm (1 {$\leq$} p {$\leq$} {$\infty$}). Special attention is devoted to the case of a pair of RKBS \$\$(B,\{B\}\^\{\textbackslash sharp \})\$\$in which B has sup-norm and \$\$\{B\}\^\{\textbackslash sharp \}\$\$has {$\mathscr{l}$}1-norm. Namely, we show that if \$\$(B,\{B\}\^\{\textbackslash sharp \})\$\$is generated by a universal kernel and B is furnished with the sup-norm, then \$\$\{B\}\^\{\textbackslash sharp \}\$\$, furnished with the {$\mathscr{l}$}1-norm, is linearly isomorphically embedded in the dual of B. We reformulate the classical classification problem (support vector machine classifier) to RKBS and suggest that it will have sparse solutions when the RKBS is furnished with the {$\mathscr{l}$}1-norm.},
 address = {{New York, NY}},
 author = {Georgiev, Pando G. and {S{\'a}nchez-Gonz{\'a}lez}, Luis and Pardalos, Panos M.},
 booktitle = {Constructive {{Nonsmooth Analysis}} and {{Related Topics}}},
 doi = {10.1007/978-1-4614-8615-2_4},
 editor = {Demyanov, Vladimir F. and Pardalos, Panos M. and Batsyn, Mikhail},
 file = {/home/matt/Zotero/storage/SQMCFNXI/Georgiev et al. - 2014 - Construction of Pairs of Reproducing Kernel Banach.pdf},
 isbn = {978-1-4614-8615-2},
 pages = {39--57},
 publisher = {{Springer New York}},
 title = {Construction of {{Pairs}} of {{Reproducing Kernel Banach Spaces}}},
 year = {2014}
}

@article{gerdes_vehicle_1997,
 author = {Gerdes, JC and Hedrick, JK},
 journal = {Control Engineering Practice},
 number = {11},
 pages = {1607--1614},
 title = {Vehicle Speed and Spacing Control via Coordinated Throttle and Brake Actuation},
 volume = {5},
 year = {1997}
}

@article{geroliminis_existence_2008,
 author = {Geroliminis, N. and Daganzo, C. F.},
 journal = {Transportation Research Part B},
 number = {9},
 pages = {759--770},
 title = {Existence of Urban-Scale Macroscopic Fundamental Diagrams: {{Some}} Experimental Findings},
 volume = {42},
 year = {2008}
}

@article{geroliminis_optimal_2013,
 author = {Geroliminis, N. and Haddad, J. and Ramezani, M},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {1},
 pages = {348--359},
 title = {Optimal Perimeter Control for Two Urban Regions with Macroscopic Fundamental Diagrams: {{A}} Model Predictive Approach},
 volume = {14},
 year = {2013}
}

@techreport{gettman_operation_2012,
 author = {Gettman, D. and Abbas, M. and Liu, H. and Skabardonis, A. and Adam, Z. and Wu, X. and Hu, H. and Boyer, T. and Walker, S. and Phillips, S. and Allen, S. and Madrigal, G. and Tong, J.},
 institution = {{Transportation Research Board}},
 number = {NCHRP 03-90},
 title = {{{OPERATION OF TRAFFIC SIGNAL SYSTEMS IN OVERSATURATED CONDITIONS}}, {{Draft Final Report}}},
 year = {2012}
}

@techreport{gettman_overview_2012,
 author = {Gettman, D.},
 institution = {{Kimley-Horn and Associates}},
 number = {FHWA SBIR DTRT57-10-C-10044},
 title = {Overview of the {{Kadence}} Real-Time Adaptive Control System},
 year = {2012}
}

@techreport{gettman_surrogate_2008,
 author = {Gettman, D. and Pu, L. and Sayed, T. and Shelby, S.},
 institution = {{Siemens Energy \& Automation, Inc.}},
 number = {FHWA-HRT-08-051},
 title = {Surrogate {{Safety Assessment Model}} and {{Validation}}: {{Final Report}}},
 year = {2008}
}

@book{geyer_complexity_2010,
 address = {{London ; New York}},
 annotation = {OCLC: ocn326678318},
 author = {Geyer, Robert and Rihani, Samir},
 isbn = {978-0-415-55662-0 978-0-415-55663-7 978-0-203-85692-5},
 lccn = {H97 .G49 2010},
 publisher = {{Routledge}},
 shorttitle = {Complexity and Public Policy},
 title = {Complexity and Public Policy: A New Approach to Twenty-First Century Politics, Policy and Society},
 year = {2010}
}

@article{ghosh_communication-efficient_2019,
 author = {Ghosh, Avishek and Maity, Raj Kumar and Kadhe, Swanand and Mazumdar, Arya and Ramchandran, Kannan},
 journal = {ArXiv preprint},
 title = {Communication-{{Efficient}} and {{Byzantine}}-{{Robust Distributed Learning}}},
 url = {https://arxiv.org/abs/1911.09721},
 volume = {abs/1911.09721},
 year = {2019}
}

@article{ghosh_counterexample-guided_2019,
 author = {Ghosh, Shromona and Ravanbakhsh, Hadi and Seshia, Sanjit A.},
 journal = {ArXiv preprint},
 title = {Counterexample-{{Guided Synthesis}} of {{Perception Models}} and {{Control}}},
 url = {https://arxiv.org/abs/1911.01523},
 volume = {abs/1911.01523},
 year = {2019}
}

@inproceedings{ghosh_interactive_2019,
 author = {Arnab Ghosh and
Richard Zhang and
Puneet K. Dokania and
Oliver Wang and
Alexei A. Efros and
Philip H. S. Torr and
Eli Shechtman},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/Ghosh0DWETS19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00126},
 pages = {1171--1180},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Interactive Sketch {\&} Fill: Multiclass Sketch-to-Image Translation},
 url = {https://doi.org/10.1109/ICCV.2019.00126},
 year = {2019}
}

@article{ghosh_learning_2019,
 author = {Ghosh, Dibya and Gupta, Abhishek and Fu, Justin and Reddy, Ashwin and Devin, Coline and Eysenbach, Benjamin and Levine, Sergey},
 journal = {ArXiv preprint},
 title = {Learning {{To Reach Goals Without Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1912.06088},
 volume = {abs/1912.06088},
 year = {2019}
}

@article{ghosh_robust_2019,
 author = {Ghosh, Avishek and Hong, Justin and Yin, Dong and Ramchandran, Kannan},
 journal = {ArXiv preprint},
 title = {Robust {{Federated Learning}} in a {{Heterogeneous Environment}}},
 url = {https://arxiv.org/abs/1906.06629},
 volume = {abs/1906.06629},
 year = {2019}
}

@inproceedings{giaccone_maximal_2005,
 author = {Giaccone, P. and Leonardi, E. and Shah, D.},
 booktitle = {Proceedings {{IEEE INFOCOM}}},
 pages = {971--980},
 title = {On the Maximal Throughput of Networks with Finite Buffers and Its Application to Buffered Crossbars},
 volume = {2},
 year = {2005}
}

@article{gibb_model_2011,
 author = {Gibb, John},
 doi = {10.3141/2263-13},
 file = {/home/matt/Documents/Papers/gibb_nodemodel.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {113--122},
 title = {Model of {{Traffic Flow Capacity Constraint Through Nodes}} for {{Dynamic Network Loading}} with {{Queue Spillback}}},
 volume = {2263},
 year = {2011}
}

@article{giles_classes_1967,
 author = {Giles, J. R.},
 doi = {10.2307/1994599},
 file = {/home/matt/Zotero/storage/FL572FFE/Giles - 1967 - Classes of Semi-Inner-Product Spaces.pdf},
 issn = {0002-9947},
 journal = {Transactions of the American Mathematical Society},
 number = {3},
 pages = {436--446},
 title = {Classes of {{Semi}}-{{Inner}}-{{Product Spaces}}},
 volume = {129},
 year = {1967}
}

@inproceedings{gilmer_neural_2017,
 author = {Justin Gilmer and
Samuel S. Schoenholz and
Patrick F. Riley and
Oriol Vinyals and
George E. Dahl},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/GilmerSRVD17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {1263--1272},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Neural Message Passing for Quantum Chemistry},
 url = {http://proceedings.mlr.press/v70/gilmer17a.html},
 volume = {70},
 year = {2017}
}

@article{gipps_behavioural_1981,
 author = {Gipps, P.G.},
 doi = {10.1016/0191-2615(81)90037-0},
 file = {/home/matt/Zotero/storage/8KXFXHNG/gipps_1982_carfollowing.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {2},
 pages = {105--111},
 title = {A Behavioural Car-Following Model for Computer Simulation},
 volume = {15},
 year = {1981}
}

@article{girard_selection_2005,
 author = {Girard, Anouck R and De Sousa, J Borges and Hedrick, J Karl},
 journal = {Proceedings of the Institution of Mechanical Engineers, Part I: Journal of Systems and Control Engineering},
 number = {1},
 pages = {1--14},
 title = {A Selection of Recent Advances in Networked Multivehicle Systems},
 volume = {219},
 year = {2005}
}

@article{gisbrecht_metric_2015,
 abstract = {Domain specific (dis-)similarity or proximity measures used e.g. in alignment algorithms of sequence data are popular to analyze complicated data objects and to cover domain specific data properties. Without an underlying vector space these data are given as pairwise (dis-)similarities only. The few available methods for such data focus widely on similarities and do not scale to large datasets. Kernel methods are very effective for metric similarity matrices, also at large scale, but costly transformations are necessary starting with non-metric (dis-) similarities. We propose an integrative combination of Nystr\"om approximation, potential double centering and eigenvalue correction to obtain valid kernel matrices at linear costs in the number of samples. By the proposed approach effective kernel approaches become accessible. Experiments with several larger (dis-)similarity datasets show that the proposed method achieves much better runtime performance than the standard strategy while keeping competitive model accuracy. The main contribution is an efficient and accurate technique, to convert (potentially non-metric) large scale dissimilarity matrices into approximated positive semi-definite kernel matrices at linear costs.},
 author = {Gisbrecht, Andrej and Schleif, Frank-Michael},
 doi = {10.1016/j.neucom.2015.04.017},
 file = {/home/matt/Zotero/storage/2FLCBBS2/Gisbrecht and Schleif - 2015 - Metric and non-metric proximity transformations at.pdf},
 issn = {09252312},
 journal = {Neurocomputing},
 language = {en},
 pages = {643--657},
 title = {Metric and Non-Metric Proximity Transformations at Linear Costs},
 volume = {167},
 year = {2015}
}

@inproceedings{gleave_adversarial_2019,
 author = {Adam Gleave and
Michael Dennis and
Cody Wild and
Neel Kant and
Sergey Levine and
Stuart Russell},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/GleaveDWKLR20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Mon, 06 Jul 2020 01:00:00 +0200},
 title = {Adversarial Policies: Attacking Deep Reinforcement Learning},
 url = {https://openreview.net/forum?id=HJgEMpVFwB},
 year = {2020}
}

@article{godunov_difference_1959,
 author = {Godunov, S.},
 journal = {Matematicheskii Sbornik},
 language = {Russian},
 pages = {271--306},
 title = {{A difference method for numerical calculation of discontinuous solutions of hydrodynamic equations}},
 volume = {47},
 year = {1959}
}

@misc{gog_erdos_2019,
 author = {Gog, Ionel and others},
 title = {{{ERDOS}}: {{A Platform}} for {{Self}}-{{Driving Cars}}},
 year = {2019}
}

@article{golabi_statewide_1982,
 author = {Golabi, K. and Kulkarni, R. B. and Way, G. B.},
 journal = {Interfaces},
 title = {A {{Statewide Pavement Management System}}},
 volume = {12},
 year = {1982}
}

@article{gomes_bandwidth_2015,
 author = {Gomes, G.},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {99},
 pages = {1--12},
 title = {Bandwidth Maximization Using Vehicle Arrival Functions},
 volume = {16},
 year = {2015}
}

@article{gomes_behavior_2008,
 author = {Gomes, G. and R. Horowitz, R. and Kurzhanskiy, A. A. and Kwon, J. and {P.Varaiya}},
 journal = {Transportation Research, Part C},
 number = {4},
 pages = {485--513},
 title = {Behavior of the {{Cell Transmission Model}} and {{Effectiveness}} of {{Ramp Metering}}},
 volume = {16},
 year = {2008}
}

@book{gomes_congestion_nodate,
 author = {Gomes, G. and Horowitz, R. and Kurzhanskiy, A. A. and Varaiya, P. and Kwon, J.},
 title = {Congestion in the {{ACTM}} Model}
}

@article{gomes_framework_2020,
 abstract = {This paper introduces a new approach to hybrid traffic modelling, along with its implementation in software. The software allows modellers to assign traffic models to individual links in a network. Each model is a plugin that implements a series of methods, referred to as the modelling interface. These methods are used by the program to exchange information between adjacent models. Traffic controllers are implemented in a similar manner. The paper outlines the important components of the method: the network description, the description of demands, and the modelling and control interfaces. We include tests demonstrating the propagation of congestion between pairs of macroscopic, mesoscopic, and microscopic models. Open Traffic Models is an open-source implementation of these concepts, and is available at https://github.com/ggomes/otm-sim.},
 author = {Gomes, Gabriel},
 doi = {10.1080/17477778.2020.1766387},
 file = {/home/matt/Zotero/storage/NKSHG3UF/Gomes - 2020 - A framework for hybrid simulation of transportatio.pdf},
 issn = {1747-7778, 1747-7786},
 journal = {Journal of Simulation},
 language = {en},
 pages = {1--16},
 title = {A Framework for Hybrid Simulation of Transportation Networks},
 year = {2020}
}

@article{gomes_qualitative_2008,
 author = {Gomes, G. and Horowitz, R. and Kurzhanskiy, A. A. and Varaiya, P. and Kwon, J.},
 journal = {Transportation Research, Part C},
 number = {4},
 pages = {485--513},
 title = {Qualitative {{Theory}} of the {{Cell Transmission Model}}},
 volume = {16},
 year = {2008}
}

@inproceedings{gomez_reversible_2017,
 author = {Aidan N. Gomez and
Mengye Ren and
Raquel Urtasun and
Roger B. Grosse},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/GomezRUG17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {2214--2224},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {The Reversible Residual Network: Backpropagation Without Storing Activations},
 url = {https://proceedings.neurips.cc/paper/2017/hash/f9be311e65d81a9ad8150a60844bb94c-Abstract.html},
 year = {2017}
}

@inproceedings{goodfellow_deep_2016,
 author = {Ruslan Salakhutdinov},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/kdd/Salakhutdinov14.bib},
 booktitle = {The 20th {ACM} {SIGKDD} International Conference on Knowledge Discovery
and Data Mining, {KDD} '14, New York, NY, {USA} - August 24 - 27,
2014},
 doi = {10.1145/2623330.2630809},
 editor = {Sofus A. Macskassy and
Claudia Perlich and
Jure Leskovec and
Wei Wang and
Rayid Ghani},
 pages = {1973},
 publisher = {{ACM}},
 timestamp = {Tue, 06 Nov 2018 00:00:00 +0100},
 title = {Deep learning},
 url = {https://doi.org/10.1145/2623330.2630809},
 year = {2014}
}

@article{gordon_novel_1993,
 abstract = {An algorithm, the bootstrap filter, is proposed for implementing recursive Bayesian filters. The required density of the state vector is represented as a set of random samples, which are updated and propagated by the algorithm. The method is not restricted by assumptions of linearity or Gaussian noise: it may be applied to any state transition or measurement model. A simulation example of the bearings only tracking problem is presented. This simulation includes schemes for improving the efficiency of the basic algorithm. For this example, the performance of the bootstrap filter is greatly superior to the standard extended Kalman filter.},
 author = {Gordon, N.J. and Salmond, D.J. and Smith, A.F.M.},
 doi = {10.1049/ip-f-2.1993.0015},
 file = {/home/matt/Zotero/storage/FC97Z85F/Gordon et al. - 1993 - Novel approach to nonlinearnon-Gaussian Bayesian .pdf},
 issn = {0956375X},
 journal = {IEE Proceedings F Radar and Signal Processing},
 language = {en},
 number = {2},
 pages = {107},
 title = {Novel Approach to Nonlinear/Non-{{Gaussian Bayesian}} State Estimation},
 volume = {140},
 year = {1993}
}

@article{gouk_regularisation_2018,
 author = {Gouk, Henry and Frank, Eibe and Pfahringer, Bernhard and Cree, Michael},
 journal = {ArXiv preprint},
 title = {Regularisation of {{Neural Networks}} by {{Enforcing Lipschitz Continuity}}},
 url = {https://arxiv.org/abs/1804.04368},
 volume = {abs/1804.04368},
 year = {2018}
}

@inproceedings{graepel_classification_1998,
 abstract = {We investigate the problem of learning a classification task on data represented in terms of their pairwise proximities. This representation does not refer to an explicit feature representation of the data items and is thus more general than the standard approach of using Euclidean feature vectors, from which pairwise proximities can always be calculated. Our first approach is based on a combined linear embedding and classification procedure resulting in an extension of the Optimal Hyperplane algorithm to pseudo-Euclidean data. As an alternative we present another approach based on a linear threshold model in the proximity values themselves, which is optimized using Structural Risk Minimization. We show that prior knowledge about the problem can be incorporated by the choice of distance measures and examine different metrics W.r.t. their generalization. Finally, the algorithms are successfully applied to protein structure data and to data from the cat's cerebral cortex. They show better performance than K-nearest-neighbor classification.},
 author = {Graepel, Thore and Herbrich, Ralf and {Bollmann-Sdorra}, Peter and Obermayer, Klaus},
 booktitle = {Advances in {{Neural Information Processing Systems}}},
 file = {/home/matt/Zotero/storage/XUWYVA3X/Graepel et al. - Classification on Pairwise Proximity Data.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {438--444},
 title = {Classification on {{Pairwise Proximity Data}}},
 volume = {11},
 year = {1998}
}

@article{grant_m42_2008,
 author = {Grant, D.},
 journal = {87th Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {M42 {{Active Traffic Management Pilot Project}}},
 year = {2008}
}

@inproceedings{grauman_pyramid_2005,
 abstract = {Discriminative learning is challenging when examples are sets of features, and the sets vary in cardinality and lack any sort of meaningful ordering. Kernel-based classification methods can learn complex decision boundaries, but a kernel over unordered set inputs must somehow solve for correspondences \textendash{} generally a computationally expensive task that becomes impractical for large set sizes. We present a new fast kernel function which maps unordered feature sets to multi-resolution histograms and computes a weighted histogram intersection in this space. This ``pyramid match'' computation is linear in the number of features, and it implicitly finds correspondences based on the finest resolution histogram cell where a matched pair first appears. Since the kernel does not penalize the presence of extra features, it is robust to clutter. We show the kernel function is positive-definite, making it valid for use in learning algorithms whose optimal solutions are guaranteed only for Mercer kernels. We demonstrate our algorithm on object recognition tasks and show it to be accurate and dramatically faster than current approaches.},
 address = {{Beijing, China}},
 author = {Grauman, K. and Darrell, T.},
 booktitle = {Tenth {{IEEE International Conference}} on {{Computer Vision}} ({{ICCV}}'05) {{Volume}} 1},
 doi = {10.1109/ICCV.2005.239},
 file = {/home/matt/Zotero/storage/8KW5SJAY/Grauman and Darrell - 2005 - The pyramid match kernel discriminative classific.pdf},
 isbn = {978-0-7695-2334-7},
 language = {en},
 pages = {1458-1465 Vol. 2},
 publisher = {{IEEE}},
 shorttitle = {The Pyramid Match Kernel},
 title = {The Pyramid Match Kernel: Discriminative Classification with Sets of Image Features},
 year = {2005}
}

@article{graves_generating_2014,
 author = {Graves, Alex},
 journal = {ArXiv preprint},
 title = {Generating {{Sequences With Recurrent Neural Networks}}},
 url = {https://arxiv.org/abs/1308.0850},
 volume = {abs/1308.0850},
 year = {2013}
}

@article{gray_unified_2013,
 author = {Gray, Andrew and Ali, Mohammad and Gao, Yiqi and Hedrick, J Karl and Borrelli, Francesco},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {3},
 pages = {1490--1499},
 title = {A {{Unified Approach}} to {{Threat Assessment}} and {{Control}} for {{Automotive Active Safety}}},
 volume = {14},
 year = {2013}
}

@article{greene_latent_2003,
 abstract = {The multinomial logit model (MNL) has for many years provided the fundamental platform for the analysis of discrete choice. The basic model\~Os several shortcomings, most notably its inherent assumption of independence from irrelevant alternatives have motivated researchers to develop a variety of alternative formulations. The mixed logit model stands as one of the most significant of these extensions. This paper proposes a semi-parametric extension of the MNL, based on the latent class formulation, which resembles the mixed logit model but which relaxes its requirement that the analyst makes specific assumptions about the distributions of parameters across individuals. An application of the model to the choice of long distance travel by three road types (2-lane, 4-lane without a median and 4-lane with a median) by car in New Zealand is used to compare the MNL latent class model with mixed logit.},
 author = {Greene, William H. and Hensher, David A.},
 doi = {10.1016/S0191-2615(02)00046-2},
 file = {/home/matt/Zotero/storage/A98R3IQ8/Greene and Hensher - 2003 - A latent class model for discrete choice analysis.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {8},
 pages = {681--698},
 shorttitle = {A Latent Class Model for Discrete Choice Analysis},
 title = {A Latent Class Model for Discrete Choice Analysis: Contrasts with Mixed Logit},
 volume = {37},
 year = {2003}
}

@article{greenshields_study_1935,
 author = {Greenshields, B. D. and Channing, W. and Miller, H.},
 journal = {Proceedings of the 14th Annual Meeting of the Highway Research Board},
 pages = {448--477},
 title = {A Study of Highway Capacity.},
 year = {1935}
}

@article{grembek_making_2019,
 author = {Grembek, Offer and Kurzhanskiy, Alex and Medury, Aditya and Varaiya, Pravin and Yu, Mengqiao},
 doi = {10.1016/j.trc.2019.02.017},
 file = {/home/matt/Zotero/storage/NMK2UEBJ/Grembek et al. - 2019 - Making intersections safer with I2V communication.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {396--410},
 title = {Making Intersections Safer with {{I2V}} Communication},
 volume = {102},
 year = {2019}
}

@unpublished{group_freeway_2003,
 author = {Group, System Metrics},
 title = {Freeway {{Performance Report}}},
 year = {2003}
}

@article{guanetti_control_2018,
 abstract = {Autonomous driving technology pledges safety, convenience, and energy efficiency. Its challenges include the unknown intentions of other road users: communication between vehicles and with the road infrastructure is a possible approach to enhance awareness and enable cooperation. Connected and automated vehicles (CAVs) have the potential to disrupt mobility, extending what is possible with driving automation and connectivity alone. Applications include real-time control and planning with increased awareness, routing with micro-scale traffic information, coordinated platooning using traffic signals information, and eco-mobility on demand with guaranteed parking. This paper introduces a control and planning architecture for CAVs, and surveys the state of the art on each functional block therein; the main focus is on techniques to improve energy efficiency. We provide an overview of existing algorithms and their mutual interactions, we present promising optimization-based approaches to CAVs control and identify future challenges.},
 author = {Guanetti, Jacopo and Kim, Yeojun and Borrelli, Francesco},
 doi = {10.1016/j.arcontrol.2018.04.011},
 file = {/home/matt/Zotero/storage/V8U2T4ZY/Guanetti et al. - 2018 - Control of connected and automated vehicles State.pdf;/home/matt/Zotero/storage/KBZQQ9BJ/S1367578818300336.html},
 issn = {1367-5788},
 journal = {Annual Reviews in Control},
 language = {en},
 pages = {18--40},
 shorttitle = {Control of Connected and Automated Vehicles},
 title = {Control of Connected and Automated Vehicles: {{State}} of the Art and Future Challenges},
 volume = {45},
 year = {2018}
}

@article{gubbi_internet_2013,
 author = {Gubbi, Jayavardhana and Buyya, Rajkumar and Marusic, Slaven and Palaniswami, Marimuthu},
 doi = {10.1016/j.future.2013.01.010},
 issn = {0167739X},
 journal = {Future Generation Computer Systems},
 language = {en},
 number = {7},
 pages = {1645--1660},
 shorttitle = {Internet of {{Things}} ({{IoT}})},
 title = {Internet of {{Things}} ({{IoT}}): {{A}} Vision, Architectural Elements, and Future Directions},
 volume = {29},
 year = {2013}
}

@inproceedings{guo_calibration_2017,
 author = {Chuan Guo and
Geoff Pleiss and
Yu Sun and
Kilian Q. Weinberger},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/GuoPSW17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {1321--1330},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {On Calibration of Modern Neural Networks},
 url = {http://proceedings.mlr.press/v70/guo17a.html},
 volume = {70},
 year = {2017}
}

@techreport{guo_evaluating_2010,
 author = {Guo, F. and Klauer, S. G. and McGill, M. T. and Dingus, T. A.},
 institution = {{Virginia Tech Transportation Institute}},
 number = {DOT HS 811 382},
 title = {Evaluating the {{Relationship Between}} near {{Crashes}} and Crashes: {{Can}} near Crashes {{Serve}} as a {{Surrogate Safety Metric}} for Crashes?},
 year = {2010}
}

@article{guo_humanlike_2018,
 abstract = {It is crucial to understand the surrounding cars with respect to the road context and interact with them harmoniously for the success of autonomous cars used in the mixed urban traffic. In this paper, a vision-based approach is proposed to implement the humanlike autonomous driving function along a predefined lane-level route in the complex urban environment with daily traffic. At first, the surrounding cars are located in the lane level by a deep neural network based detector with a low-cost lane graph. Subsequently, a Bayesian network is employed to classify the detected cars into six categories based on their states of operation, i.e., leader car, parked car, tail-end car, exiting car, merging car, and other car. Finally, a hybrid potential map, consisting of a trajectory-induction potential and a risk-prevention potential, is constructed for each of the cars according to their categories, which will be combined to be used for generating an appropriate behavior. Particularly, both of the trajectory-induction potentials and the risk-prevention potentials are learned from naturalistic driving data of the same situations in the daily urban traffic to encode the human driving skills and experiences. Therefore, the behavior generated based on the proposed learning-based potentials is close to a humanlike performance, which is important to achieve harmony in the mixed traffic. Experimental results in various typical but challenging urban traffic scenes have substantiated the effectiveness of the proposed system.},
 author = {Guo, C. and Kidono, K. and Terashima, R. and Kojima, Y.},
 doi = {10.1109/TIV.2017.2788194},
 file = {/home/matt/Zotero/storage/G4XUPIQC/Guo et al. - 2018 - Humanlike Behavior Generation in Urban Environment.pdf;/home/matt/Zotero/storage/3BCXM7QQ/8241707.html},
 issn = {2379-8904},
 journal = {IEEE Transactions on Intelligent Vehicles},
 number = {1},
 pages = {46--60},
 title = {Humanlike {{Behavior Generation}} in {{Urban Environment Based}} on {{Learning}}-{{Based Potentials With}} a {{Low}}-{{Cost Lane Graph}}},
 volume = {3},
 year = {2018}
}

@article{guo_reinforcement_2019,
 author = {Guo, Mengyu and Wang, Pin and Chan, Ching-Yao and Askary, Sid},
 journal = {ArXiv preprint},
 title = {A {{Reinforcement Learning Approach}} for {{Intelligent Traffic Signal Control}} at {{Urban Intersections}}},
 url = {https://arxiv.org/abs/1905.07698},
 volume = {abs/1905.07698},
 year = {2019}
}

@article{guohui_simulation-based_2009,
 author = {Guohui, Zhang and Shuming, Yan and Yinhai, Wang},
 doi = {10.1061/(ASCE)0733-947X(2009)135:10(677)},
 file = {/home/matt/Zotero/storage/EMRK2WKI/Zhang Guohui et al. - 2009 - Simulation-Based Investigation on High-Occupancy T.pdf;/home/matt/Zotero/storage/ZUQKP797/(ASCE)0733-947X(2009)13510(677).html},
 journal = {Journal of Transportation Engineering},
 number = {10},
 pages = {677--686},
 title = {Simulation-{{Based Investigation}} on {{High}}-{{Occupancy Toll Lane Operations}} for {{Washington State Route}} 167},
 volume = {135},
 year = {2009}
}

@article{gupta_relay_2019,
 author = {Gupta, Abhishek and Kumar, Vikash and Lynch, Corey and Levine, Sergey and Hausman, Karol},
 journal = {ArXiv preprint},
 title = {Relay {{Policy Learning}}: {{Solving Long}}-{{Horizon Tasks}} via {{Imitation}} and {{Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1910.11956},
 volume = {abs/1910.11956},
 year = {2019}
}

@article{h._payne_freeflo_1979,
 author = {{H. Payne}},
 journal = {Transportation Research Record},
 pages = {68--77},
 title = {{{FREEFLO}}: {{A}} Macroscopic Simulation Model of Freeway Traffic},
 volume = {722},
 year = {1979}
}

@article{h._payne_models_1971,
 author = {{H. Payne}},
 journal = {Mathematical Models of Public Systems},
 number = {1},
 pages = {51--61},
 title = {Models of Freeway Traffic and Control},
 volume = {28},
 year = {1971}
}

@inproceedings{ha_hypernetworks_2016,
 author = {David Ha and
Andrew M. Dai and
Quoc V. Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HaDL17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {HyperNetworks},
 url = {https://openreview.net/forum?id=rkpACe1lx},
 year = {2017}
}

@article{ha_learning_2020,
 author = {Ha, Sehoon and Xu, Peng and Tan, Zhenyu and Levine, Sergey and Tan, Jie},
 journal = {ArXiv preprint},
 title = {Learning to {{Walk}} in the {{Real World}} with {{Minimal Human Effort}}},
 url = {https://arxiv.org/abs/2002.08550},
 volume = {abs/2002.08550},
 year = {2020}
}

@inproceedings{ha_neural_2017,
 author = {David Ha and
Douglas Eck},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HaE18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {A Neural Representation of Sketch Drawings},
 url = {https://openreview.net/forum?id=Hy6GHpkCW},
 year = {2018}
}

@inproceedings{haan_gauge_2021,
 author = {Pim de Haan and
Maurice Weiler and
Taco Cohen and
Max Welling},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HaanWCW21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Gauge Equivariant Mesh CNNs: Anisotropic convolutions on geometric
graphs},
 url = {https://openreview.net/forum?id=Jnspzp-oIZE},
 year = {2021}
}

@phdthesis{haarnoja_acquiring_2018,
 abstract = {In this thesis, we study how maximum entropy framework can provide efficient deep reinforcement learning (deep RL) algorithms that solve tasks consistently and sample efficiently. This framework has several intriguing properties. First, the optimal policies are stochastic, improving exploration and preventing convergence to local optima, particularly when the objective is multimodal. Second, the entropy term provides regularization, resulting in more consistent and robust learning when compared to deterministic methods. Third, maximum entropy policies are composable, that is, two or more policies can be combined, and the resulting policy can be shown to be approximately optimal for the sum of the constituent task rewards. And fourth, the view of maximum entropy RL as probabilistic inference provides a foundation for building hierarchical policies that can solve complex and sparse reward tasks. In the first part, we will devise new algorithms based on this framework, starting from soft Q-learning that learns expressive energy-based policies, to soft actor-critic that provides simplicity and convenience of actor-critic methods, and ending with automatic temperature adjustment scheme that practically eliminates the need for hyperparameter tuning, which is a crucial feature for real-world applications where tuning of hyperparameters can be prohibitively expensive. In the second part, we will discuss extensions enabled by the inherent stochasticity of maximum entropy polices, including compositionality and hierarchical learning. We will demonstrate the effectiveness of the proposed algorithms on both simulated and real-world robotic manipulation and locomotion tasks.},
 author = {Haarnoja, Tuomas},
 file = {/home/matt/Zotero/storage/JE5FFJNS/Haarnoja - 2018 - Acquiring Diverse Robot Skills via Maximum Entropy.pdf;/home/matt/Zotero/storage/Z7Q39XFT/25g6573w.html},
 language = {en},
 school = {UC Berkeley},
 title = {Acquiring {{Diverse Robot Skills}} via {{Maximum Entropy Deep Reinforcement Learning}}},
 year = {2018}
}

@inproceedings{haarnoja_soft_2018,
 author = {Tuomas Haarnoja and
Aurick Zhou and
Pieter Abbeel and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/HaarnojaZAL18.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {1856--1865},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Soft Actor-Critic: Off-Policy Maximum Entropy Deep Reinforcement Learning
with a Stochastic Actor},
 url = {http://proceedings.mlr.press/v80/haarnoja18b.html},
 volume = {80},
 year = {2018}
}

@inproceedings{hafner_learning_2019,
 author = {Danijar Hafner and
Timothy P. Lillicrap and
Ian Fischer and
Ruben Villegas and
David Ha and
Honglak Lee and
James Davidson},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/HafnerLFVHLD19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {2555--2565},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Learning Latent Dynamics for Planning from Pixels},
 url = {http://proceedings.mlr.press/v97/hafner19a.html},
 volume = {97},
 year = {2019}
}

@article{hakhamaneshi_bagnet_2019,
 author = {Hakhamaneshi, Kourosh and Werblun, Nick and Abbeel, Pieter and Stojanovic, Vladimir},
 journal = {ArXiv preprint},
 title = {{{BagNet}}: {{Berkeley Analog Generator}} with {{Layout Optimizer Boosted}} with {{Deep Neural Networks}}},
 url = {https://arxiv.org/abs/1907.10515},
 volume = {abs/1907.10515},
 year = {2019}
}

@article{hakhamaneshi_gacem_2020,
 author = {Hakhamaneshi, Kourosh and Settaluri, Keertana and Abbeel, Pieter and Stojanovic, Vladimir},
 journal = {ArXiv preprint},
 title = {{{GACEM}}: {{Generalized Autoregressive Cross Entropy Method}} for {{Multi}}-{{Modal Black Box Constraint Satisfaction}}},
 url = {https://arxiv.org/abs/2002.07236},
 volume = {abs/2002.07236},
 year = {2020}
}

@inproceedings{hakhamaneshi_late_2019,
 abstract = {A deep neural network (DNN) based stochastic combinatorial optimization framework is presented that can find the optimal sizing of circuits in a sample-efficient manner. This sample efficiency allows us to unify this framework with generator-based tools like Berkeley Analog Generator (BAG) [1] to directly optimize layout, given the high level circuit specifications. We use this tool to design an optical link receiver layout, satisfying high-level design specifications, using post-layout simulations of only 348 design instances. Compared to an evolutionary algorithm without our DNN-based discriminator, our framework improves the sample efficiency and run time by more than 200x.},
 author = {Hakhamaneshi, K. and Werblun, N. and Abbeel, P. and Stojanovi{\'c}, V.},
 booktitle = {2019 56th {{ACM}}/{{IEEE Design Automation Conference}} ({{DAC}})},
 file = {/home/matt/Zotero/storage/7TM4RDYL/Hakhamaneshi et al_2019_Late Breaking Results.pdf;/home/matt/Zotero/storage/92YYAN6J/8807032.html},
 pages = {1--2},
 shorttitle = {Late {{Breaking Results}}},
 title = {Late {{Breaking Results}}: {{Analog Circuit Generator}} Based on {{Deep Neural Network}} Enhanced {{Combinatorial}} Optimization},
 year = {2019}
}

@article{hall_capacity_1990,
 author = {Hall, Fred L. and Hall, Lisa M.},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 keywords = {⛔ No DOI found},
 pages = {108--118},
 title = {Capacity and Speed-Flow Analysis of the {{Queen Elizabeth Way}} in {{Ontario}}},
 volume = {1287},
 year = {1990}
}

@article{hall_empirical_1986,
 author = {Hall, Fred L. and Allen, Brian L. and Gunter, Margot A.},
 file = {/home/matt/Zotero/storage/CM3FDFPW/1986_Hall_empericalAnalysisofFlowDensity.pdf},
 journal = {Transportation Research Part A: General},
 number = {3},
 pages = {197--210},
 title = {Empirical Analysis of Freeway Flow-Density Relationships},
 volume = {20},
 year = {1986}
}

@unpublished{hallenbach_m.e._measurement_2003,
 author = {{Hallenbach, M.E.} and Ishimaru, J. M. and Nee, J.},
 title = {Measurement of Recurring versus Non-Recurring Congestion},
 year = {2003}
}

@inproceedings{hamilton_inductive_2017,
 author = {William L. Hamilton and
Zhitao Ying and
Jure Leskovec},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/HamiltonYL17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {1024--1034},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Inductive Representation Learning on Large Graphs},
 url = {https://proceedings.neurips.cc/paper/2017/hash/5dd9db5e033da9c6fb5ba83c7a7ebea9-Abstract.html},
 year = {2017}
}

@article{hamilton_representation_2018,
 author = {Hamilton, William L. and Ying, Rex and Leskovec, Jure},
 journal = {ArXiv preprint},
 title = {Representation {{Learning}} on {{Graphs}}: {{Methods}} and {{Applications}}},
 url = {https://arxiv.org/abs/1709.05584},
 volume = {abs/1709.05584},
 year = {2017}
}

@article{hanin_approximating_2018,
 author = {Hanin, Boris and Sellke, Mark},
 journal = {ArXiv preprint},
 title = {Approximating {{Continuous Functions}} by {{ReLU Nets}} of {{Minimal Width}}},
 url = {https://arxiv.org/abs/1710.11278},
 volume = {abs/1710.11278},
 year = {2017}
}

@article{haoui_wireless_2008,
 author = {Haoui, A. and Kavaler, R. and Varaiya, P.},
 journal = {Transportation Research, Part C},
 number = {3},
 pages = {294--306},
 title = {Wireless Magnetic Sensors for Traffic Surveillance},
 volume = {16},
 year = {2008}
}

@article{hardy_contingency_2013,
 abstract = {This paper presents a novel optimization-based path planner that is capable of planning multiple contingency paths to directly account for uncertainties in the future trajectories of dynamic obstacles. This planner addresses the particular problem of probabilistic collision avoidance for autonomous road vehicles that are required to safely interact, in close proximity, with other vehicles with unknown intentions. The presented path planner utilizes an efficient spline-based trajectory representation and fast but accurate collision probability bounds to simultaneously optimize multiple continuous contingency paths in real time. These collision probability bounds are efficient enough for real-time evaluation, yet accurate enough to allow for practical close-proximity driving behaviors such as passing an obstacle vehicle in an adjacent lane. An obstacle trajectory clustering algorithm is also presented to enable the path planner to scale to multiple-obstacle scenarios. Simulation results show that the contingency planner allows for a more aggressive driving style than planning a single path without compromising the overall safety of the robot.},
 author = {Hardy, Jason and Campbell, Mark},
 doi = {10.1109/TRO.2013.2254033},
 file = {/home/matt/Zotero/storage/6HTRRCWX/Hardy and Campbell - 2013 - Contingency Planning Over Probabilistic Obstacle P.pdf},
 issn = {1552-3098, 1941-0468},
 journal = {IEEE Transactions on Robotics},
 language = {en},
 number = {4},
 pages = {913--929},
 title = {Contingency {{Planning Over Probabilistic Obstacle Predictions}} for {{Autonomous Road Vehicles}}},
 volume = {29},
 year = {2013}
}

@article{harrison_brownian_1993,
 author = {Harrison, J. M. and Nguyen, V.},
 journal = {Queueing Systems},
 pages = {5--40},
 title = {Brownian Models Ofmulticlass Queueing Networks: {{Current}} Status and Open Problems},
 volume = {13},
 year = {1993}
}

@inproceedings{hartikainen_dynamical_2019,
 author = {Kristian Hartikainen and
Xinyang Geng and
Tuomas Haarnoja and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HartikainenGHL20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Dynamical Distance Learning for Semi-Supervised and Unsupervised Skill
Discovery},
 url = {https://openreview.net/forum?id=H1lmhaVtvr},
 year = {2020}
}

@article{hau_congestion_2005,
 author = {Hau, T. D.},
 journal = {Transportmetrica},
 number = {2},
 pages = {87--116},
 title = {Congestion Pricing Mechanisms for Roads, Part {{I}}-{{Conceptual}} Framework},
 volume = {2},
 year = {2005}
}

@article{hau_economic_2005,
 author = {Hau, T. D.},
 journal = {Transportmetrica},
 number = {2},
 pages = {81--117, 119--149},
 title = {Economic Fundamentals of Road Pricing: A Diagrammatic Analysis, Part {{I}}-{{Fundamentals}}; Part {{II}}-{{Relaxation}} of Assumptions},
 volume = {1},
 year = {2005}
}

@inproceedings{haut_second_2005,
 author = {Haut, B. and Bastin, G.},
 booktitle = {Proceedings of the {{IEEE Intelligent Transportation Systems Conference}}},
 pages = {178--184},
 title = {A Second Order Model for Road Traffic Networks},
 year = {2005}
}

@article{haut_second_2007,
 author = {Haut, Bertrand and Bastin, Georges},
 doi = {10.3934/nhm.2007.2.227},
 file = {/home/matt/Zotero/storage/XXHGSUZE/2007_haut_bastin_secondorderjunction.pdf},
 journal = {Networks and Heterogeneous Media},
 number = {2},
 pages = {227--253},
 title = {A Second Order Model of Road Junctions in Fluid Models of Traffic Networks},
 volume = {2},
 year = {2007}
}

@inproceedings{he_decision_2018,
 author = {Warren He and
Bo Li and
Dawn Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/He0S18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Decision Boundary Analysis of Adversarial Examples},
 url = {https://openreview.net/forum?id=BkpiPMbA-},
 year = {2018}
}

@inproceedings{he_deep_2016,
 author = {Kaiming He and
Xiangyu Zhang and
Shaoqing Ren and
Jian Sun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/HeZRS16.bib},
 booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
 doi = {10.1109/CVPR.2016.90},
 pages = {770--778},
 publisher = {{IEEE} Computer Society},
 timestamp = {Wed, 17 Apr 2019 01:00:00 +0200},
 title = {Deep Residual Learning for Image Recognition},
 url = {https://doi.org/10.1109/CVPR.2016.90},
 year = {2016}
}

@inproceedings{he_identity_2016,
 abstract = {Deep residual networks [1] have emerged as a family of extremely deep architectures showing compelling accuracy and nice convergence behaviors. In this paper, we analyze the propagation formulations behind the residual building blocks, which suggest that the forward and backward signals can be directly propagated from one block to any other block, when using identity mappings as the skip connections and after-addition activation. A series of ablation experiments support the importance of these identity mappings. This motivates us to propose a new residual unit, which makes training easier and improves generalization. We report improved results using a 1001-layer ResNet on CIFAR-10 (4.62\% error) and CIFAR-100, and a 200-layer ResNet on ImageNet. Code is available at: https://github.com/KaimingHe/ resnet-1k-layers.},
 archiveprefix = {arXiv},
 author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
 booktitle = {European {{Conference}} on {{Computer Vision}}},
 eprint = {1603.05027},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/4M5QQNXD/He et al. - 2016 - Identity Mappings in Deep Residual Networks.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {630--645},
 title = {Identity {{Mappings}} in {{Deep Residual Networks}}},
 year = {2016}
}

@inproceedings{he_kernelized_2017,
 author = {Lifang He and
Chun{-}Ta Lu and
Guixiang Ma and
Shen Wang and
LinLin Shen and
Philip S. Yu and
Ann B. Ragin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/HeLMWSYR17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {1442--1451},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 06 May 2020 01:00:00 +0200},
 title = {Kernelized Support Tensor Machines},
 url = {http://proceedings.mlr.press/v70/he17a.html},
 volume = {70},
 year = {2017}
}

@inproceedings{he_momentum_2020,
 author = {Kaiming He and
Haoqi Fan and
Yuxin Wu and
Saining Xie and
Ross B. Girshick},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/He0WXG20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.00975},
 pages = {9726--9735},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {Momentum Contrast for Unsupervised Visual Representation Learning},
 url = {https://doi.org/10.1109/CVPR42600.2020.00975},
 year = {2020}
}

@phdthesis{heba_dynamic_2014,
 author = {Heba, ElKholy},
 file = {/home/matt/Zotero/storage/2KDH83UE/Heba_ElKholy_Thesis_S2014.pdf},
 school = {American University in Cairo},
 title = {Dynamic Modeling and Control of a {{Quadrotor}} Using Linear and Nonlinear Approaches},
 year = {2014}
}

@article{hedrick_control_1994,
 author = {Hedrick, JK and Tomizuka, Masayoshi and Varaiya, P},
 journal = {Control Systems, IEEE},
 number = {6},
 pages = {21--32},
 title = {Control Issues in Automated Highway Systems},
 volume = {14},
 year = {1994}
}

@article{hedrick_tools_2011,
 author = {Hedrick, J Karl and Basso, Brandon and Love, Joshua and Lavis, Benjamin M},
 journal = {Journal of Dynamic Systems, Measurement, and Control},
 number = {2},
 pages = {024001},
 title = {Tools and {{Techniques}} for {{Mobile Sensor Network Control}}},
 volume = {133},
 year = {2011}
}

@inproceedings{hejna_iii_hierarchically_2020,
 author = {Donald J. Hejna III and
Lerrel Pinto and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/HejnaPA20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {4159--4171},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Hierarchically Decoupled Imitation For Morphological Transfer},
 url = {http://proceedings.mlr.press/v119/hejna20a.html},
 volume = {119},
 year = {2020}
}

@article{helbing_d._traffic_2001,
 author = {{Helbing, D.}},
 journal = {Reviews of Modern Physics},
 pages = {1067--1141},
 title = {Traffic and Related Self-Driven Many-Particle Systems},
 volume = {73},
 year = {2001}
}

@article{helbing_gas-kinetic_1996,
 author = {Helbing, Dirk},
 doi = {10.1103/PhysRevE.53.2366},
 journal = {Phys. Rev. E},
 number = {3},
 pages = {2366--2381},
 title = {Gas-Kinetic Derivation of {{Navier}}-{{Stokes}}-like Traffic Equations},
 volume = {53},
 year = {1996}
}

@article{helbing_improved_1995,
 author = {Helbing, D.},
 journal = {Physical Review E},
 pages = {3164--3169},
 title = {Improved Fluid Dynamic Model for Vehicular Traffic},
 year = {1995}
}

@inproceedings{helmbold_surprising_2017,
 author = {David P. Helmbold and
Philip M. Long},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/colt/HelmboldL17.bib},
 booktitle = {Proceedings of the 30th Conference on Learning Theory, {COLT} 2017,
Amsterdam, The Netherlands, 7-10 July 2017},
 editor = {Satyen Kale and
Ohad Shamir},
 pages = {1123--1146},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Surprising properties of dropout in deep networks},
 url = {http://proceedings.mlr.press/v65/helmbold17a.html},
 volume = {65},
 year = {2017}
}

@inproceedings{henderson_deep_2017,
 author = {Peter Henderson and
Riashat Islam and
Philip Bachman and
Joelle Pineau and
Doina Precup and
David Meger},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/0002IBPPM18.bib},
 booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
(AAAI-18), the 30th innovative Applications of Artificial Intelligence
(IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
Artificial Intelligence (EAAI-18), New Orleans, Louisiana, USA, February
2-7, 2018},
 editor = {Sheila A. McIlraith and
Kilian Q. Weinberger},
 pages = {3207--3214},
 publisher = {{AAAI} Press},
 timestamp = {Mon, 22 Oct 2018 01:00:00 +0200},
 title = {Deep Reinforcement Learning That Matters},
 url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/16669},
 year = {2018}
}

@article{hendrycks_benchmark_2019,
 author = {Hendrycks, Dan and Basart, Steven and Mazeika, Mantas and Mostajabi, Mohammadreza and Steinhardt, Jacob and Song, Dawn},
 journal = {ArXiv preprint},
 title = {A {{Benchmark}} for {{Anomaly Segmentation}}},
 url = {https://arxiv.org/abs/1911.11132},
 volume = {abs/1911.11132},
 year = {2019}
}

@inproceedings{hendrycks_benchmarking_2018,
 author = {Dan Hendrycks and
Thomas G. Dietterich},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HendrycksD19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Benchmarking Neural Network Robustness to Common Corruptions and Perturbations},
 url = {https://openreview.net/forum?id=HJz6tiCqYm},
 year = {2019}
}

@inproceedings{hendrycks_using_2019,
 author = {Dan Hendrycks and
Mantas Mazeika and
Saurav Kadavath and
Dawn Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/HendrycksMKS19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {15637--15648},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Using Self-Supervised Learning Can Improve Model Robustness and Uncertainty},
 url = {https://proceedings.neurips.cc/paper/2019/hash/a2b15837edac15df90721968986f7f8e-Abstract.html},
 year = {2019}
}

@article{hernandez-leal_is_2018,
 author = {{Hernandez-Leal}, Pablo and Kartal, Bilal and Taylor, Matthew E.},
 journal = {ArXiv preprint},
 title = {Is Multiagent Deep Reinforcement Learning the Answer or the Question? {{A}} Brief Survey},
 url = {https://arxiv.org/abs/1810.05587},
 volume = {abs/1810.05587},
 year = {2018}
}

@article{herty_coupling_2006,
 author = {Herty, M. and Rascle, M.},
 doi = {10.1137/05062617X},
 file = {/home/matt/Documents/Papers/herty_rascle_awrascle_network.pdf},
 issn = {0036-1410, 1095-7154},
 journal = {SIAM Journal on Mathematical Analysis},
 language = {en},
 number = {2},
 pages = {595--616},
 title = {Coupling {{Conditions}} for a {{Class}} of {{Second}}-{{Order Models}} for {{Traffic Flow}}},
 volume = {38},
 year = {2006}
}

@article{herzig_learning_2020,
 author = {Herzig, Roei and Bar, Amir and Xu, Huijuan and Chechik, Gal and Darrell, Trevor and Globerson, Amir},
 journal = {ArXiv preprint},
 title = {Learning {{Canonical Representations}} for {{Scene Graph}} to {{Image Generation}}},
 url = {https://arxiv.org/abs/1912.07414},
 volume = {abs/1912.07414},
 year = {2019}
}

@inproceedings{hessel_rainbow_2017,
 author = {Matteo Hessel and
Joseph Modayil and
Hado van Hasselt and
Tom Schaul and
Georg Ostrovski and
Will Dabney and
Dan Horgan and
Bilal Piot and
Mohammad Gheshlaghi Azar and
David Silver},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/HesselMHSODHPAS18.bib},
 booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
(AAAI-18), the 30th innovative Applications of Artificial Intelligence
(IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
Artificial Intelligence (EAAI-18), New Orleans, Louisiana, USA, February
2-7, 2018},
 editor = {Sheila A. McIlraith and
Kilian Q. Weinberger},
 pages = {3215--3222},
 publisher = {{AAAI} Press},
 timestamp = {Mon, 22 Oct 2018 01:00:00 +0200},
 title = {Rainbow: Combining Improvements in Deep Reinforcement Learning},
 url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/17204},
 year = {2018}
}

@article{heydecker_objectives_2004,
 abstract = {present a control theoretic formulation for it that distinguishes the various roles of detector data, objectives of optimisation, and control feedback},
 author = {Heydecker, B. G.},
 journal = {Journal of Intelligent Transportation Systems},
 pages = {63--76},
 title = {Objectives, Stimulus and Feedback in Signal Control of Road Traffic},
 volume = {8},
 year = {2004}
}

@inproceedings{higgins_-vae_2017,
 author = {Irina Higgins and
Lo{\"{\i}}c Matthey and
Arka Pal and
Christopher Burgess and
Xavier Glorot and
Matthew Botvinick and
Shakir Mohamed and
Alexander Lerchner},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HigginsMPBGBML17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {beta-VAE: Learning Basic Visual Concepts with a Constrained Variational
Framework},
 url = {https://openreview.net/forum?id=Sy2fzU9gl},
 year = {2017}
}

@book{hilkevitch_dearborn_nodate,
 annotation = {Published: Chicago Tribune, 12/21/12},
 author = {Hilkevitch, J.},
 title = {Dearborn, a Test for {{Loop}}'s First Protected Bike Lanes}
}

@inproceedings{hinton_matrix_2018,
 author = {Geoffrey E. Hinton and
Sara Sabour and
Nicholas Frosst},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HintonSF18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Matrix capsules with {EM} routing},
 url = {https://openreview.net/forum?id=HJWLfGWRb},
 year = {2018}
}

@inproceedings{hinton_transforming_2011,
 abstract = {The artificial neural networks that are used to recognize shapes typically use one or more layers of learned feature detectors that produce scalar outputs. By contrast, the computer vision community uses complicated, hand-engineered features, like SIFT [6], that produce a whole vector of outputs including an explicit representation of the pose of the feature. We show how neural networks can be used to learn features that output a whole vector of instantiation parameters and we argue that this is a much more promising way of dealing with variations in position, orientation, scale and lighting than the methods currently employed in the neural networks community. It is also more promising than the handengineered features currently used in computer vision because it provides an efficient way of adapting the features to the domain.},
 address = {{Berlin, Heidelberg}},
 author = {Hinton, Geoffrey E. and Krizhevsky, Alex and Wang, Sida D.},
 booktitle = {Artificial {{Neural Networks}} and {{Machine Learning}} \textendash{} {{ICANN}} 2011},
 doi = {10.1007/978-3-642-21735-7_6},
 file = {/home/matt/Zotero/storage/YYEKQ7VG/Hinton et al. - 2011 - Transforming Auto-Encoders.pdf},
 isbn = {978-3-642-21734-0 978-3-642-21735-7},
 language = {en},
 pages = {44--51},
 publisher = {{Springer Berlin Heidelberg}},
 title = {Transforming {{Auto}}-{{Encoders}}},
 volume = {6791},
 year = {2011}
}

@article{hirsch_monotone_2005,
 author = {Hirsch, M. W. and Smith, H.},
 journal = {Journal of Difference Equations and Applications},
 number = {4-5},
 pages = {379--398},
 title = {Monotone Maps: A Review},
 volume = {11},
 year = {2005}
}

@inproceedings{ho_compression_2019,
 author = {Jonathan Ho and
Evan Lohn and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/HoLA19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {3874--3883},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Compression with Flows via Local Bits-Back Coding},
 url = {https://proceedings.neurips.cc/paper/2019/hash/f6e794a75c5d51de081dbefa224304f9-Abstract.html},
 year = {2019}
}

@inproceedings{ho_population_2019,
 author = {Daniel Ho and
Eric Liang and
Xi Chen and
Ion Stoica and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/HoLCSA19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {2731--2741},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 24 Sep 2019 01:00:00 +0200},
 title = {Population Based Augmentation: Efficient Learning of Augmentation
Policy Schedules},
 url = {http://proceedings.mlr.press/v97/ho19b.html},
 volume = {97},
 year = {2019}
}

@article{hochreiter_long_1997,
 author = {Hochreiter, Sepp and Schmidhuber, J{\"u}rgen},
 doi = {10.1162/neco.1997.9.8.1735},
 file = {/home/matt/Zotero/storage/JITSTRD7/Hochreiter and Schmidhuber - 1997 - Long Short-Term Memory.pdf},
 issn = {0899-7667, 1530-888X},
 journal = {Neural Computation},
 language = {en},
 number = {8},
 pages = {1735--1780},
 title = {Long {{Short}}-{{Term Memory}}},
 volume = {9},
 year = {1997}
}

@phdthesis{hofleitner_hybrid_2013,
 abstract = {Mathematical models are a mathematical abstraction of the physical reality which is of great importance to understand the behavior of a system, make estimations and predictions and so on. They range from models based on physical laws to models learned empirically, as measurements are collected, and referred to as data-driven models. A model is based on a series of choices which influence its complexity and realism. These choices represent trade-offs between different competing objectives including interpretability, scalability, accuracy, adequation to the available data, robustness or computational complexity. The thesis investigates the advantages and disadvantages of models based on physical laws versus data-driven models through the example of signalized queuing networks such as urban transportation networks.The dynamics of conservation flow networks are accurately represented by a first order partial differential equation. Using Hamilton-Jacobi theory, the thesis underlines the importance to leverage physical laws to reconstruct missing information (\textbackslash emph\{e.g.\} signal or bottleneck characteristics) and estimate the state of the network at any time and location. Noise and uncertainty in the measurements can be integrated in the model. When measurements are sparse, the state of the network cannot be estimated at every time and location on the network. Instead, the thesis shows how to leverage other characteristics, such as periodicity. From deterministic dynamics, the thesis derives the probability distribution functions of physical entities (\textbackslash emph\{e.g.\} waiting time, density) by marginalizing the periodic variable. Using a Dynamic Bayesian Network formulation and exploiting the convexity structure of the system, the thesis shows how this modeling leads to realistic estimations and predictions, even when little measurements are available. Finally, the thesis investigates how sparse modeling and dimensionality reduction can provide insights on the large scale behavior of the network. Large scale dynamics and patterns are hard to model accurately based on physical laws. They can be discovered through data mining algorithms and integrated into physical models.},
 author = {Hofleitner, Aude},
 file = {/home/matt/Zotero/storage/7LH34CEB/Hofleitner - 2013 - A hybrid approach of physical laws and data-driven.pdf;/home/matt/Zotero/storage/KQT5Y97S/3p53c6zj.html},
 language = {en},
 school = {UC Berkeley},
 shorttitle = {A Hybrid Approach of Physical Laws and Data-Driven Modeling for Estimation},
 title = {A Hybrid Approach of Physical Laws and Data-Driven Modeling for Estimation: The Example of Queuing Networks},
 year = {2013}
}

@article{hofmann_kernel_2008,
 author = {Hofmann, Thomas and Sch{\"o}lkopf, Bernhard and Smola, Alexander J.},
 doi = {10.1214/009053607000000677},
 file = {/home/matt/Zotero/storage/QEA345N6/Hofmann et al. - 2008 - Kernel methods in machine learning.pdf},
 issn = {0090-5364},
 journal = {The Annals of Statistics},
 language = {en},
 number = {3},
 pages = {1171--1220},
 title = {Kernel Methods in Machine Learning},
 volume = {36},
 year = {2008}
}

@book{hoh_virtual_2008,
 annotation = {Published: Proc. 6th Int'l Conf. on Mobile Systems, Applications, and Services (Mobisys '08)},
 author = {Hoh, B. and Gruteser, M. and Herring, R. and Bann, J. and Work, D. and {J-C. Herrera} and Bayen, A. M. and Annavaram, M. and Jacobson, Q.},
 title = {Virtual Trip Lines for Distributed Privacy-Preserving Traffic Monitoring},
 year = {2008}
}

@article{holden_mathematical_1995,
 author = {Holden, Helge and Risebro, Nils Henrik},
 doi = {10.1137/S0036141093243289},
 file = {/home/matt/Zotero/storage/FDWMSFF3/1995_holden_risebro_riemann_solver.pdf},
 journal = {SIAM Journal on Mathematical Analysis},
 number = {4},
 pages = {999--1017},
 title = {A Mathematical Model of Traffic Flow on a Network of Unidirectional Roads},
 volume = {26},
 year = {1995}
}

@book{holland_complexity_2014,
 abstract = {From the movement of flocks of birds to the Internet, environmental sustainability, and market regulation, the study and understanding of complex non-linear systems has become highly influential over the last thirty years. Complexity: A Very Short Introduction introduces the key elements and conceptual framework of complexity. From complex physical systems such as fluid flow and the difficulties of predicting weather, to complex adaptive systems such as the highly diverse and interdependent ecosystems of rainforests, it combines simple, well-known examples\textemdash Adam Smith's pin factory, Charles Darwin's comet orchid, and Herbert Simon's ``watchmaker''\textemdash with an account of the approaches, involving agents and urn models, taken by complexity theory.},
 address = {{New York, NY}},
 author = {Holland, John H.},
 edition = {1st},
 file = {/home/matt/Zotero/storage/8L99HY7Y/actrade-9780199662548.html},
 isbn = {978-0-19-966254-8},
 language = {en\_US},
 publisher = {{Oxford University Press}},
 shorttitle = {Complexity},
 title = {Complexity: {{A Very Short Introduction}}},
 year = {2014}
}

@book{holland_signals_2012,
 abstract = {An overarching framework for comparing and steering complex adaptive systems is developed through understanding the mechanisms that generate their intricate signal/boundary hierarchies. Complex adaptive systems (cas), including ecosystems, governments, biological cells, and markets, are characterized by intricate hierarchical arrangements of boundaries and signals. In ecosystems, for example, niches act as semi-permeable boundaries, and smells and visual patterns serve as signals; governments have departmental hierarchies with memoranda acting as signals; and so it is with other cas. Despite a wealth of data and descriptions concerning different cas, there remain many unanswered questions about "steering" these systems. In Signals and Boundaries, John Holland argues that understanding the origin of the intricate signal/border hierarchies of these systems is the key to answering such questions. He develops an overarching framework for comparing and steering cas through the mechanisms that generate their signal/boundary hierarchies. Holland lays out a path for developing the framework that emphasizes agents, niches, theory, and mathematical models. He discusses, among other topics, theory construction; signal-processing agents; networks as representations of signal/boundary interaction; adaptation; recombination and reproduction; the use of tagged urn models (adapted from elementary probability theory) to represent boundary hierarchies; finitely generated systems as a way to tie the models examined into a single framework; the framework itself, illustrated by a simple finitely generated version of the development of a multi-celled organism; and Markov processes.},
 address = {{Cambridge, Massachusetts}},
 author = {Holland, John H.},
 file = {/home/matt/Zotero/storage/8EXKYER8/detail.html},
 isbn = {978-0-262-30589-1},
 publisher = {{MIT Press}},
 shorttitle = {Signals and {{Boundaries}}},
 title = {Signals and {{Boundaries}}: {{Building Blocks}} for {{Complex Adaptive Systems}}},
 year = {2012}
}

@article{holland_statistics_1986,
 author = {Holland, Paul W.},
 doi = {10.2307/2289064},
 file = {/home/matt/Zotero/storage/8K9V7SMK/Statistics and Causal Inference.pdf},
 issn = {01621459},
 journal = {Journal of the American Statistical Association},
 number = {396},
 pages = {945},
 title = {Statistics and {{Causal Inference}}},
 volume = {81},
 year = {1986}
}

@article{holmes_volvo_2011,
 author = {Holmes, J.},
 journal = {MotorTrend},
 title = {Volvo {{Says Autonomous Car Convoys Could Be Reality By}} 2020},
 year = {2011}
}

@article{hoogendoorn_continuum_2000,
 author = {Hoogendoorn, Serge P. and Bovy, Piet H. L.},
 doi = {http://dx.doi.org/10.1016/S0191-2615(99)00017-X},
 file = {/home/matt/Zotero/storage/W8AZAP2X/2000_TRB_multiclass_continuum.pdf},
 issn = {0191-2615},
 journal = {Transportation Research Part B: Methodological},
 number = {2},
 pages = {123--146},
 title = {Continuum Modeling of Multiclass Traffic Flow},
 volume = {34},
 year = {2000}
}

@article{hoogendoorn_gas-kinetic_1999,
 abstract = {A gas\textendash kinetic traffic flow model is presented that describes the traffic flow operations of heterogeneous traffic on specific lanes of a motorway. To realistically portray the multilane dynamics of traffic flow, traffic is described as a collection of vehicle platoons that consist of an unconstrained vehicle followed by a nonnegative number of constrained followers. It is shown that the gas\textendash kinetic dynamics of this unconstrained and constrained traffic are governed by continuum and noncontinuum processes. The continuum processes describe smooth changes in the mesoscopic traffic flow variables caused by motions in the phase space. The noncontinuum processes reflect, among other things, deceleration of vehicles due to interactions between vehicles from the same and from different user classes, immediate lane changing, postponed lane changing by constrained drivers, and spontaneous lane changing by free-flowing drivers. Finally, it is shown how the multilane-multiclass model relates to traditional aggregate-lane and mixed-class gas\textendash kinetic equations. This is accomplished by aggregation across the motorway lanes and the user classes. It is shown that the expression reflecting vehicle interactions in traditional models is only valid for dilute traffic. A remedial expression is proposed.},
 author = {Hoogendoorn, Serge P. and Bovy, Piet H. L.},
 doi = {10.3141/1678-19},
 file = {/home/matt/Zotero/storage/3TGZNT8Z/Hoogendoorn and Bovy - 1999 - Gas–Kinetic Model for Multilane Heterogeneous Traf.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 language = {en},
 number = {1},
 pages = {150--159},
 title = {Gas-{{Kinetic Model}} for {{Multilane Heterogeneous Traffic Flow}}},
 volume = {1678},
 year = {1999}
}

@article{hoogendoorn_state---art_2001,
 abstract = {Abstract, Nowadays traffic flow and congestion is one of the main societal and economical problems related to transportation in industrialized countries. In this respect, managing traffic in congested networks requires a clear understanding of traffic flow operations; i.e. insights into what causes congestion, what determines the time and location of traffic breakdown, how does the congestion propagate through the network, etc., are essential. For this purpose, during the past fifty years, a wide range of traffic flow theories and models have been developed to answer these research questions. This paper presents a overview of some fifty years of modelling vehicular traffic flow. A rich variety of modelling approaches developed so far and in use today will be discussed and compared. The considered models are classified based on the level-of-detail with which the vehicular flow is described. For each of the categories, issues like modelling accuracy, applicability, generalizability, and model calibration and validation are discussed.},
 author = {Hoogendoorn, S P and Bovy, P H L},
 doi = {10.1177/095965180121500402},
 file = {/home/matt/Zotero/storage/JV8ERHD7/Hoogendoorn and Bovy - 2001 - State-of-the-art of vehicular traffic flow modelli.pdf},
 issn = {0959-6518},
 journal = {Proceedings of the Institution of Mechanical Engineers, Part I: Journal of Systems and Control Engineering},
 language = {en},
 number = {4},
 pages = {283--303},
 title = {State-of-the-Art of Vehicular Traffic Flow Modelling},
 volume = {215},
 year = {2001}
}

@inproceedings{horgan_distributed_2018,
 author = {Dan Horgan and
John Quan and
David Budden and
Gabriel Barth{-}Maron and
Matteo Hessel and
Hado van Hasselt and
David Silver},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HorganQBBHHS18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Distributed Prioritized Experience Replay},
 url = {https://openreview.net/forum?id=H1Dy---0Z},
 year = {2018}
}

@inproceedings{Hornauer_2019_CVPR_Workshops,
 author = {Hornauer, Sascha and Yellapragada, Baladitya and Ranjbar, Arian and Yu, Stella},
 booktitle = {The {{IEEE}} Conference on Computer Vision and Pattern Recognition ({{CVPR}}) Workshops},
 file = {/home/matt/Zotero/storage/QW2MI824/Hornauer et al. - 2019 - Driving scene retrieval by example from large-scal.pdf},
 title = {Driving Scene Retrieval by Example from Large-Scale Data},
 year = {2019}
}

@article{hornik_approximation_1991,
 abstract = {We show that standard multilayer feedforward networks with as few as a single hidden layer and arbitrary bounded and nonconstant activation function are universal approximators with respect to Lp({$\mu$}) performance criteria, for arbitrary finite input environment measures {$\mu$}, provided only that sufficiently many hidden units are available. If the activation function is continuous, bounded and nonconstant, then continuous mappings can be learned uniformly over compact input sets. We also give very general conditions ensuring that networks with sufficiently smooth activation functions are capable of arbitrarily accurate approximation to a function and its derivatives.},
 author = {Hornik, Kurt},
 doi = {10.1016/0893-6080(91)90009-T},
 file = {/home/matt/Zotero/storage/AMNJBXUG/Hornik - 1991 - Approximation capabilities of multilayer feedforwa.pdf;/home/matt/Zotero/storage/D39UREKW/089360809190009T.html},
 issn = {0893-6080},
 journal = {Neural Networks},
 number = {2},
 pages = {251--257},
 title = {Approximation Capabilities of Multilayer Feedforward Networks},
 volume = {4},
 year = {1991}
}

@article{hornik_multilayer_1989,
 abstract = {This paper rigorously establishes that standard multilayer feedforward networks with as few as one hidden layer using arbitrary squashing functions are capable of approximating any Borel measurable function from one finite dimensional space to another to any desired degree of accuracy, provided sufficiently many hidden units are available. In this sense, multilayer feedforward networks are a class of universal approximators.},
 author = {Hornik, Kurt and Stinchcombe, Maxwell and White, Halbert},
 doi = {10.1016/0893-6080(89)90020-8},
 file = {/home/matt/Zotero/storage/IPKQQFC2/Hornik et al. - 1989 - Multilayer feedforward networks are universal appr.pdf;/home/matt/Zotero/storage/WN26IBRT/0893608089900208.html},
 issn = {0893-6080},
 journal = {Neural Networks},
 number = {5},
 pages = {359--366},
 title = {Multilayer Feedforward Networks Are Universal Approximators},
 volume = {2},
 year = {1989}
}

@article{horowitz_control_2000,
 author = {Horowitz, R. and Variya, P.},
 journal = {Proceedings of the IEEE: Special Issue on Hybrid Systems},
 number = {7},
 pages = {913--25},
 title = {Control {{Design}} of an {{Automated Highway System}}},
 volume = {88},
 year = {2000}
}

@article{horvath_generalized_2014,
 abstract = {In earlier papers we changed the concept of the inner product to a more general one, to the so-called Minkowski product. This product changes on the tangent space hence we could investigate a more general structure than a Riemannian manifold. Particularly interesting such a model is when the negative direct component has dimension one and the model shows a certain space-time character. We will discuss this case here. We give a deterministic and a non-deterministic (random) variant of such a model. As we showed, the deterministic model can be defined also with a ``shape function''.},
 author = {Horv{\'a}th, {\'A}. G.},
 doi = {10.1007/s00010-013-0250-6},
 file = {/home/matt/Zotero/storage/9Y278VYC/Horváth - 2014 - Generalized Minkowski space with changing shape.pdf},
 issn = {0001-9054, 1420-8903},
 journal = {Aequationes mathematicae},
 language = {en},
 number = {3},
 pages = {337--377},
 title = {Generalized {{Minkowski}} Space with Changing Shape},
 volume = {87},
 year = {2014}
}

@article{horvath_isometries_2017,
 abstract = {In this paper we review the known facts on isometries of Minkowski geometries and prove some new results on them. We give the normal forms of two special classes of operators and also characterize the isometry group of Minkowski 3-spaces in which the unit sphere does not contain an ellipse.},
 author = {Horv{\'a}th, {\'A}kos G.},
 doi = {10.1016/j.laa.2016.09.038},
 file = {/home/matt/Zotero/storage/TD89KY8I/Horváth - 2017 - Isometries of Minkowski geometries.pdf;/home/matt/Zotero/storage/PYNVGGR8/S0024379516304554.html},
 issn = {0024-3795},
 journal = {Linear Algebra and its Applications},
 language = {en},
 pages = {172--190},
 title = {Isometries of {{Minkowski}} Geometries},
 volume = {512},
 year = {2017}
}

@article{horvath_semi-indefinite_2010,
 abstract = {In this paper we develop the theories of normed linear spaces and of linear spaces with indefinite metric, for finite dimensions both of which are also called Minkowski spaces in the literature. In the first part of this paper we collect the common properties of the semi- and indefinite inner products and define the semi-indefinite inner product as well as the corresponding semi-indefinite inner product space. We give a generalized concept of the Minkowski space embedded in a semi-indefinite inner product space using the concept of a new product, which contains the classical cases as special ones. In the second part we investigate the real, finite-dimensional generalized Minkowski space and its sphere of radius i. We prove that it can be regarded as a so-called Minkowski\textendash Finsler space, and if it is homogeneous with respect to linear isometries, then the Minkowski\textendash Finsler distance of its points can be determined by the Minkowski product.},
 author = {Horv{\'a}th, {\'A}. G.},
 doi = {10.1016/j.geomphys.2010.04.006},
 file = {/home/matt/Zotero/storage/W8NRL53I/Horváth - 2010 - Semi-indefinite inner product and generalized Mink.pdf;/home/matt/Zotero/storage/YEVDXXXE/S039304401000077X.html},
 issn = {0393-0440},
 journal = {Journal of Geometry and Physics},
 language = {en},
 number = {9},
 pages = {1190--1208},
 title = {Semi-Indefinite Inner Product and Generalized {{Minkowski}} Spaces},
 volume = {60},
 year = {2010}
}

@misc{how_caltrans_builds_projects,
 author = {{Caltrans Office of Project Development Procedures}},
 file = {/home/matt/Zotero/storage/YBVF2REV/How_Caltrans_Builds_Projects_HCBP_2011a-9-13-11.pdf},
 publisher = {{California Department of Transportation}},
 title = {How {{Caltrans Builds Projects}}},
 year = {2011}
}

@article{hu_generic_2019,
 abstract = {Accurately predicting future behaviors of surrounding vehicles is an essential capability for autonomous vehicles in order to plan safe and feasible trajectories. The behaviors of others, however, are full of uncertainties. Both rational and irrational behaviors exist, and the autonomous vehicles need to be aware of this in their prediction module. The prediction module is also expected to generate reasonable results in the presence of unseen and corner scenarios. Two types of prediction models are typically used to solve the prediction problem: learning-based model and planning-based model. Learning-based model utilizes real driving data to model the human behaviors. Depending on the structure of the data, learning-based models can predict both rational and irrational behaviors. But the balance between them cannot be customized, which creates challenges in generalizing the prediction results. Planning-based model, on the other hand, usually assumes human as a rational agent, i.e., it anticipates only rational behavior of human drivers. In this paper, a generic prediction architecture is proposed to address various rationalities in human behavior. We leverage the advantages from both learning-based and planning-based prediction models. The proposed approach is able to predict continuous trajectories that well-reflect possible future situations of other drivers. Moreover, the prediction performance remains stable under various unseen driving scenarios. A case study under a real-world roundabout scenario is provided to demonstrate the performance and capability of the proposed prediction architecture.},
 archiveprefix = {arXiv},
 author = {Hu, Yeping and Sun, Liting and Tomizuka, Masayoshi},
 doi = {10.1109/ITSC.2019.8917105},
 eprint = {1907.10170},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/BUTAJULQ/Hu et al_2019_Generic Prediction Architecture Considering both Rational and Irrational.pdf;/home/matt/Zotero/storage/JXD3939C/1907.html},
 journal = {IEEE Intelligent Transportation Systems Conference (ITSC)},
 pages = {3539--3546},
 title = {Generic {{Prediction Architecture Considering}} Both {{Rational}} and {{Irrational Driving Behaviors}}},
 year = {2019}
}

@inproceedings{hu_iterative_2019,
 author = {Ronghang Hu and
Amanpreet Singh and
Trevor Darrell and
Marcus Rohrbach},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/HuSDR20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.01001},
 pages = {9989--9999},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {Iterative Answer Prediction With Pointer-Augmented Multimodal Transformers
for TextVQA},
 url = {https://doi.org/10.1109/CVPR42600.2020.01001},
 year = {2020}
}

@inproceedings{hu_language-conditioned_2019,
 author = {Ronghang Hu and
Anna Rohrbach and
Trevor Darrell and
Kate Saenko},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/HuRDS19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.01039},
 pages = {10293--10302},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Language-Conditioned Graph Networks for Relational Reasoning},
 url = {https://doi.org/10.1109/ICCV.2019.01039},
 year = {2019}
}

@inproceedings{hu_open_2020,
 author = {Weihua Hu and
Matthias Fey and
Marinka Zitnik and
Yuxiao Dong and
Hongyu Ren and
Bowen Liu and
Michele Catasta and
Jure Leskovec},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/HuFZDRLCL20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Open Graph Benchmark: Datasets for Machine Learning on Graphs},
 url = {https://proceedings.neurips.cc/paper/2020/hash/fb60d411a5c5b72b2e7d3527cfc84fd0-Abstract.html},
 year = {2020}
}

@inproceedings{huang_algorithm-hardware_2019,
 abstract = {FPGAs provide a flexible and efficient platform to accelerate rapidly-changing algorithms for computer vision. The majority of existing work focuses on accelerating image classification, while other fundamental vision problems, including object detection and instance segmentation, have not been adequately addressed. Compared with image classification, detection problems are more sensitive to the spatial variance of objects, and therefore, require specialized convolutions to aggregate spatial information. To address this, recent work proposes dynamic deformable convolution to augment regular convolutions. Regular convolutions process a fixed grid of pixels across all the spatial locations in an image, while dynamic deformable convolutions may access arbitrary pixels in the image and the access pattern is input-dependent and varies per spatial location. These properties lead to inefficient memory accesses of inputs with existing hardware. In this work, we first investigate the overhead of the deformable convolution on embedded FPGA SoCs, and then show the accuracy-latency tradeoffs for a set of algorithm modifications including full versus depthwise, fixed-shape, and limited-range. These modifications benefit the energy efficiency for embedded devices in general as they reduce the compute complexity. We then build an efficient object detection network with modified deformable convolutions and quantize the network using state-of-the-art quantization methods. We implement a unified hardware engine on FPGA to support all the operations in the network. Preliminary experiments show that little accuracy is compromised and speedup can be achieved with our co-design optimization for the deformable convolution.},
 archiveprefix = {arXiv},
 author = {Huang, Qijing and Wang, Dequan and Gao, Yizhao and Cai, Yaohui and Dong, Zhen and Wu, Bichen and Keutzer, Kurt and Wawrzynek, John},
 booktitle = {The 5th {{Workshop}} on {{Energy Efficient Machine Learning}} and {{Cognitive Computing}}},
 eprint = {2002.08357},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/QNAG62NY/Huang et al. - 2020 - Algorithm-hardware Co-design for Deformable Convol.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Algorithm-Hardware {{Co}}-Design for {{Deformable Convolution}}},
 year = {2019}
}

@inproceedings{huang_attpool_2019,
 author = {Jingjia Huang and
Zhangheng Li and
Nannan Li and
Shan Liu and
Ge Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/HuangLLLL19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00658},
 pages = {6479--6488},
 publisher = {{IEEE}},
 timestamp = {Sat, 21 Nov 2020 00:00:00 +0100},
 title = {AttPool: Towards Hierarchical Feature Representation in Graph Convolutional
Networks via Attention Mechanism},
 url = {https://doi.org/10.1109/ICCV.2019.00658},
 year = {2019}
}

@inproceedings{huang_combining_2021,
 author = {Qian Huang and
Horace He and
Abhay Singh and
Ser{-}Nam Lim and
Austin R. Benson},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/HuangHSLB21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Combining Label Propagation and Simple Models out-performs Graph Neural
Networks},
 url = {https://openreview.net/forum?id=8E1-f3VhX1o},
 year = {2021}
}

@inproceedings{huang_densely_2018,
 author = {Gao Huang and
Zhuang Liu and
Laurens van der Maaten and
Kilian Q. Weinberger},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/HuangLMW17.bib},
 booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
 doi = {10.1109/CVPR.2017.243},
 pages = {2261--2269},
 publisher = {{IEEE} Computer Society},
 timestamp = {Mon, 10 Sep 2018 01:00:00 +0200},
 title = {Densely Connected Convolutional Networks},
 url = {https://doi.org/10.1109/CVPR.2017.243},
 year = {2017}
}

@article{huang_indefinite_2017,
 abstract = {Because of several successful applications, indefinite kernels have attracted many research interests in recent years. This paper addresses indefinite learning in the framework of least squares support vector machines (LS-SVM). Unlike existing indefinite kernel learning methods, which usually involve non-convex problems, the indefinite LS-SVM is still easy to solve, but the kernel trick and primal-dual relationship for LS-SVM with a Mercer kernel is no longer valid. In this paper, we give a feature space interpretation for indefinite LS-SVM. In the same framework, kernel principal component analysis with an infinite kernel is discussed as well. In numerical experiments, LS-SVM with indefinite kernels for classification and kernel principal component analysis is evaluated. Its good performance together with the feature space interpretation given in this paper imply the potential use of indefinite LS-SVM in real applications.},
 author = {Huang, Xiaolin and Maier, Andreas and Hornegger, Joachim and Suykens, Johan A. K.},
 doi = {10.1016/j.acha.2016.09.001},
 file = {/home/matt/Zotero/storage/SZEHDHHM/Huang et al. - 2017 - Indefinite kernels in least squares support vector.pdf;/home/matt/Zotero/storage/FUTEM85C/S1063520316300495.html},
 issn = {1063-5203},
 journal = {Applied and Computational Harmonic Analysis},
 language = {en},
 number = {1},
 pages = {162--172},
 title = {Indefinite Kernels in Least Squares Support Vector Machines and Principal Component Analysis},
 volume = {43},
 year = {2017}
}

@article{huang_modeling_2002,
 author = {Huang, H. J. and Lam, W. H. K.},
 journal = {Transportation Research, Part B},
 pages = {253--273},
 title = {Modeling and Solving Dynamic User Equilibrium Route and Departure Time Choice Problem in Network with Queues},
 volume = {36},
 year = {2002}
}

@article{huang_nonverbal_2019,
 author = {Huang, Sandy H. and Huang, Isabella and Pandya, Ravi and Dragan, Anca D.},
 journal = {ArXiv preprint},
 title = {Nonverbal {{Robot Feedback}} for {{Human Teachers}}},
 url = {https://arxiv.org/abs/1911.02320},
 volume = {abs/1911.02320},
 year = {2019}
}

@article{huang_understanding_2016,
 abstract = {The Belt \& Road Initiative is China's greatest international economic ambition, aiming at stimulating economic development in a vast region covering sub regions in Asia, Europe and Africa, which accounts for 64\% of world population and 30\% of world GDP. The Initiative is devised to reconfigure China's external sector in order to continue its strong growth. While infrastructure development plays a central role, the Belt \& Road Initiative is a comprehensive one, including also policy dialogue, unimpeded trade, financial support and people-to-people exchange. It is too early to assess the impact of this ambitious Initiative. It certainly has the potential of turning the underdeveloped ``Belt \& Road'' region into a new vibrant economic pillar and contributing to economic policy thinking by incorporating successful experiences of emerging market economies. However, the Initiative also faces very high barriers, including lack of central coordination mechanism, potential clash of different political regimes and beliefs and financial viability of cross-border projects.},
 author = {Huang, Yiping},
 doi = {10.1016/j.chieco.2016.07.007},
 file = {/home/matt/Zotero/storage/ETWWJ3VU/Huang - 2016 - Understanding China's Belt & Road Initiative Moti.pdf;/home/matt/Zotero/storage/YPZC62JY/S1043951X16300785.html},
 issn = {1043-951X},
 journal = {China Economic Review},
 pages = {314--321},
 shorttitle = {Understanding {{China}}'s {{Belt}} \& {{Road Initiative}}},
 title = {Understanding {{China}}'s {{Belt}} \& {{Road Initiative}}: {{Motivation}}, Framework and Assessment},
 volume = {40},
 year = {2016}
}

@inproceedings{Hwang_2019_CVPR,
 author = {Jyh{-}Jing Hwang and
Tsung{-}Wei Ke and
Jianbo Shi and
Stella X. Yu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/HwangKSY19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00418},
 pages = {4056--4065},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Adversarial Structure Matching for Structured Prediction Tasks},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Hwang\_Adversarial\_Structure\_Matching\_for\_Structured\_Prediction\_Tasks\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{hwang_applying_2020,
 abstract = {Recent advances in depth-sensing have significantly increased accuracy, resolution, and frame rate, as shown in the 1920x1200 resolution and 13 frames per second Zivid RGBD camera. In this study, we explore the potential of depth sensing for efficient and reliable automation of surgical subtasks. We consider a monochrome (all red) version of the peg transfer task from the Fundamentals of Laparoscopic Surgery training suite implemented with the da Vinci Research Kit (dVRK). We use calibration techniques that allow the imprecise, cable-driven da Vinci to reduce error from 4\textendash 5 mm to 1\textendash 2 mm in the task space. We report experimental results for a handover-free version of the peg transfer task, performing 20 and 5 physical episodes with single- and bilateral-arm setups, respectively. Results over 236 and 49 total block transfer attempts for the single- and bilateral-arm peg transfer cases suggest that reliability can be attained with 86.9 \% and 78.0 \% for each individual block, with respective block transfer speeds of 10.02 and 5.72 seconds. Supplementary material is available at https://sites.google.com/view/peg-transfer.},
 archiveprefix = {arXiv},
 author = {Hwang, Minho and Seita, Daniel and Thananjeyan, Brijen and Ichnowski, Jeffrey and Paradis, Samuel and Fer, Danyal and Low, Thomas and Goldberg, Ken},
 booktitle = {International {{Symposium}} on {{Medical Robotics}}},
 eprint = {2002.06302},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/YXEKFUK6/Hwang et al. - 2020 - Applying Depth-Sensing to Automated Surgical Manip.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Applying {{Depth}}-{{Sensing}} to {{Automated Surgical Manipulation}} with a Da {{Vinci Robot}}},
 year = {2020}
}

@article{hwang_survey_2010,
 author = {Hwang, Inseok and Kim, Sungwan and Kim, Youdan and Seah, Chze Eng},
 doi = {10.1109/TCST.2009.2026285},
 file = {/home/matt/Zotero/storage/D5QBMXDX/05282515.pdf},
 issn = {1063-6536, 1558-0865},
 journal = {IEEE Transactions on Control Systems Technology},
 number = {3},
 pages = {636--653},
 title = {A {{Survey}} of {{Fault Detection}}, {{Isolation}}, and {{Reconfiguration Methods}}},
 volume = {18},
 year = {2010}
}

@book{ibm_ibm_2014,
 annotation = {Published: ITS 3C Summit},
 author = {{IBM}},
 title = {{{IBM Transportation Management Center}}},
 year = {2014}
}

@article{ichnowski_gomp_2020,
 author = {Ichnowski, Jeffrey and Danielczuk, Michael and Xu, Jingyi and Satish, Vishal and Goldberg, Ken},
 journal = {ArXiv preprint},
 title = {{{GOMP}}: {{Grasp}}-{{Optimized Motion Planning}} for {{Bin Picking}}},
 url = {https://arxiv.org/abs/2003.02401},
 volume = {abs/2003.02401},
 year = {2020}
}

@inproceedings{inala_neurosymbolic_2020,
 author = {Jeevana Priya Inala and
Yichen Yang and
James Paulos and
Yewen Pu and
Osbert Bastani and
Vijay Kumar and
Martin Rinard and
Armando Solar{-}Lezama},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/Inala0PPB0RS20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Neurosymbolic Transformers for Multi-Agent Communication},
 url = {https://proceedings.neurips.cc/paper/2020/hash/9d740bd0f36aaa312c8d504e28c42163-Abstract.html},
 year = {2020}
}

@inproceedings{inala_neurosymbolic_2021,
 author = {Jeevana Priya Inala and
Yichen Yang and
James Paulos and
Yewen Pu and
Osbert Bastani and
Vijay Kumar and
Martin Rinard and
Armando Solar{-}Lezama},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/Inala0PPB0RS20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Neurosymbolic Transformers for Multi-Agent Communication},
 url = {https://proceedings.neurips.cc/paper/2020/hash/9d740bd0f36aaa312c8d504e28c42163-Abstract.html},
 year = {2020}
}

@techreport{inc_twin_2001,
 author = {Inc, Cambridge Systematics},
 institution = {{Minnesota Department of Transportation}},
 number = {HF2891},
 title = {Twin {{Cities Ramp Meter Evaluation}}},
 year = {2001}
}

@inproceedings{iqbal_actor-attention-critic_2019,
 author = {Shariq Iqbal and
Fei Sha},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/IqbalS19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {2961--2970},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Actor-Attention-Critic for Multi-Agent Reinforcement Learning},
 url = {http://proceedings.mlr.press/v97/iqbal19a.html},
 volume = {97},
 year = {2019}
}

@inproceedings{isard_dryad_2007,
 abstract = {Dryad is a general-purpose distributed execution engine for coarse-grain data-parallel applications. A Dryad application combines computational "vertices" with communication "channels" to form a dataflow graph. Dryad runs the application by executing the vertices of this graph on a set of available computers, communicating as appropriate through flies, TCP pipes, and shared-memory FIFOs. The vertices provided by the application developer are quite simple and are usually written as sequential programs with no thread creation or locking. Concurrency arises from Dryad scheduling vertices to run simultaneously on multiple computers, or on multiple CPU cores within a computer. The application can discover the size and placement of data at run time, and modify the graph as the computation progresses to make efficient use of the available resources. Dryad is designed to scale from powerful multi-core single computers, through small clusters of computers, to data centers with thousands of computers. The Dryad execution engine handles all the difficult problems of creating a large distributed, concurrent application: scheduling the use of computers and their CPUs, recovering from communication or computer failures, and transporting data between vertices.},
 address = {{Lisbon, Portugal}},
 author = {Isard, Michael and Budiu, Mihai and Yu, Yuan and Birrell, Andrew and Fetterly, Dennis},
 booktitle = {Proceedings of the 2nd {{ACM SIGOPS}}/{{EuroSys European Conference}} on {{Computer Systems}} 2007},
 doi = {10.1145/1272996.1273005},
 file = {/home/matt/Zotero/storage/6GDLQJEJ/Isard et al. - 2007 - Dryad distributed data-parallel programs from seq.pdf},
 isbn = {978-1-59593-636-3},
 pages = {59--72},
 publisher = {{Association for Computing Machinery}},
 series = {{{EuroSys}} '07},
 shorttitle = {Dryad},
 title = {Dryad: Distributed Data-Parallel Programs from Sequential Building Blocks},
 year = {2007}
}

@inproceedings{ishak_topological_2006,
 author = {Ishak, S. and Alecsandru, C. and Seedah, D.},
 booktitle = {Applications of {{Advanced Technology}} in {{Transportation}} ({{AAAT}})},
 editor = {{K.C.P. Wang, B.L. Smith, D.R. Uzarski, S.C. Wong}},
 title = {Topological and {{Operational Improvements}} to a {{Cell}}-{{Transmission}}-{{Based Simulation Model}}},
 year = {2006}
}

@book{its_international_benefits_2013,
 author = {{ITS International}},
 title = {Benefits of {{Florida}}'s Traffic Signal Retiming},
 year = {2013}
}

@book{its_international_bluetooth_2013,
 author = {{ITS International}},
 title = {Bluetooth and {{Wi}}-{{Fi}} Offer New Options for Travel Time Measurements},
 year = {2013}
}

@article{ivanov_data_2020,
 author = {Ivanov, Andrei and Dryden, Nikoli and {Ben-Nun}, Tal and Li, Shigang and Hoefler, Torsten},
 journal = {ArXiv preprint},
 title = {Data {{Movement Is All You Need}}: {{A Case Study}} on {{Optimizing Transformers}}},
 url = {https://arxiv.org/abs/2007.00072},
 volume = {abs/2007.00072},
 year = {2020}
}

@inproceedings{ivanovic_generative_2018,
 address = {{Madrid}},
 author = {Ivanovic, Boris and Schmerling, Edward and Leung, Karen and Pavone, Marco},
 booktitle = {2018 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}} ({{IROS}})},
 doi = {10.1109/IROS.2018.8594393},
 file = {/home/matt/Zotero/storage/XBGKM2KD/Ivanovic et al. - 2018 - Generative Modeling of Multimodal Multi-Human Beha.pdf},
 isbn = {978-1-5386-8094-0},
 pages = {3088--3095},
 publisher = {{IEEE}},
 title = {Generative {{Modeling}} of {{Multimodal Multi}}-{{Human Behavior}}},
 year = {2018}
}

@article{ivanovic_mats_2021,
 author = {Ivanovic, Boris and Elhafsi, Amine and Rosman, Guy and Gaidon, Adrien and Pavone, Marco},
 journal = {ArXiv preprint},
 title = {{{MATS}}: {{An Interpretable Trajectory Forecasting Representation}} for {{Planning}} and {{Control}}},
 url = {https://arxiv.org/abs/2009.07517},
 volume = {abs/2009.07517},
 year = {2020}
}

@inproceedings{ivanovic_trajectron_2019,
 author = {Boris Ivanovic and
Marco Pavone},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/IvanovicP19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00246},
 pages = {2375--2384},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {The Trajectron: Probabilistic Multi-Agent Trajectory Modeling With
Dynamic Spatiotemporal Graphs},
 url = {https://doi.org/10.1109/ICCV.2019.00246},
 year = {2019}
}

@article{jabari_node_2016,
 author = {Jabari, Saif Eddin},
 doi = {10.1016/j.trb.2016.06.001},
 file = {/home/matt/Documents/Papers/jabari_congested_node_2016.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {229--249},
 title = {Node Modeling for Congested Urban Road Networks},
 volume = {91},
 year = {2016}
}

@article{jabari_stochastic_2012,
 abstract = {In a variety of applications of traffic flow, including traffic simulation, real-time estimation and prediction, one requires a probabilistic model of traffic flow. The usual approach to constructing such models involves the addition of random noise terms to deterministic equations, which could lead to negative traffic densities and mean dynamics that are inconsistent with the original deterministic dynamics. This paper offers a new stochastic model of traffic flow that addresses these issues. The source of randomness in the proposed model is the uncertainty inherent in driver gap choice, which is represented by random state dependent vehicle time headways. A wide range of time headway distributions is allowed. From the random time headways, counting processes are defined, which represent cumulative flows across cell boundaries in a discrete space and continuous time conservation framework. We show that our construction implicitly ensures non-negativity of traffic densities and that the fluid limit of the stochastic model is consistent with cell transmission model (CTM) based deterministic dynamics.},
 author = {Jabari, Saif Eddin and Liu, Henry X.},
 doi = {10.1016/j.trb.2011.09.006},
 file = {/home/matt/Zotero/storage/GYASFDMS/Jabari and Liu - 2012 - A stochastic model of traffic flow Theoretical fo.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {1},
 pages = {156--174},
 shorttitle = {A Stochastic Model of Traffic Flow},
 title = {A Stochastic Model of Traffic Flow: {{Theoretical}} Foundations},
 volume = {46},
 year = {2012}
}

@article{jabari_stochastic_2013,
 abstract = {A Gaussian approximation of the stochastic traffic flow model of Jabari and Liu (2012) is proposed. The Gaussian approximation is characterized by deterministic mean and covariance dynamics; the mean dynamics are those of the Godunov scheme. By deriving the Gaussian model, as opposed to assuming Gaussian noise arbitrarily, covariance matrices of traffic variables follow from the physics of traffic flow and can be computed using only few parameters, regardless of system size or how finely the system is discretized. Stationary behavior of the covariance dynamics is analyzed and it is shown that the covariance matrices are bounded. Consequently, Kalman filters that use the proposed model are stochastically observable, which is a critical issue in real time estimation of traffic dynamics. Model validation was carried out in a real-world signalized arterial setting, where cycleby-cycle maximum queue sizes were estimated using the Gaussian model as a description of state dynamics. The estimated queue sizes were compared to observed maximum queue sizes and the results indicate very good agreement between estimated and observed queue sizes.},
 author = {Jabari, Saif Eddin and Liu, Henry X.},
 doi = {10.1016/j.trb.2012.09.004},
 file = {/home/matt/Zotero/storage/4FXKGCUS/Jabari and Liu - 2013 - A stochastic model of traffic flow Gaussian appro.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {15--41},
 shorttitle = {A Stochastic Model of Traffic Flow},
 title = {A Stochastic Model of Traffic Flow: {{Gaussian}} Approximation and Estimation},
 volume = {47},
 year = {2013}
}

@article{jacob_assessment_2000,
 author = {Jacob, B.},
 journal = {Intl J Heavy Vehicle Systems},
 number = {2/3},
 pages = {136--152},
 title = {Assessment of the Accuracy and Classification of Weigh-in-Motion Systems {{Part}} 1: {{Statistical}} Background},
 volume = {7},
 year = {2000}
}

@book{jacobs_death_1961,
 address = {{New York, NY}},
 author = {Jacobs, Jane},
 isbn = {978-0-679-74195-X},
 lccn = {HT167 .J33 1992},
 publisher = {{Random House}},
 title = {The Death and Life of Great {{American}} Cities},
 year = {1961}
}

@inproceedings{jacobsen_i-revnet_2018,
 author = {J{\"{o}}rn{-}Henrik Jacobsen and
Arnold W. M. Smeulders and
Edouard Oyallon},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/JacobsenSO18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {i-RevNet: Deep Invertible Networks},
 url = {https://openreview.net/forum?id=HJsjkMb0Z},
 year = {2018}
}

@article{jain_contrastive_2020,
 author = {Jain, Paras and Jain, Ajay and Zhang, Tianjun and Abbeel, Pieter and Gonzalez, Joseph E. and Stoica, Ion},
 journal = {ArXiv preprint},
 title = {Contrastive {{Code Representation Learning}}},
 url = {https://arxiv.org/abs/2007.04973},
 volume = {abs/2007.04973},
 year = {2020}
}

@article{jain_staging_2020,
 author = {Jain, Karan P. and Tang, Jerry and Sreenath, Koushil and Mueller, Mark W.},
 journal = {ArXiv preprint},
 title = {Staging Energy Sources to Extend Flight Time of a Multirotor {{UAV}}},
 url = {https://arxiv.org/abs/2003.04290},
 volume = {abs/2003.04290},
 year = {2020}
}

@inproceedings{jain_structural-rnn_2016,
 author = {Ashesh Jain and
Amir Roshan Zamir and
Silvio Savarese and
Ashutosh Saxena},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/JainZSS16.bib},
 booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2016, Las Vegas, NV, USA, June 27-30, 2016},
 doi = {10.1109/CVPR.2016.573},
 pages = {5308--5317},
 publisher = {{IEEE} Computer Society},
 timestamp = {Thu, 25 May 2017 01:00:00 +0200},
 title = {Structural-RNN: Deep Learning on Spatio-Temporal Graphs},
 url = {https://doi.org/10.1109/CVPR.2016.573},
 year = {2016}
}

@article{james_orthogonality_1947,
 author = {James, Robert C.},
 doi = {10.2307/1990220},
 file = {/home/matt/Zotero/storage/HG2KCWF5/James - Orthogonality and Linear Functionals in Normed Lin.pdf;/home/matt/Zotero/storage/WYI4EJKI/1-s2.0-S0893608097000105-main.pdf},
 issn = {0002-9947},
 journal = {Transactions of the American Mathematical Society},
 number = {2},
 pages = {265--292},
 title = {Orthogonality and {{Linear Functionals}} in {{Normed Linear Spaces}}},
 volume = {61},
 year = {1947}
}

@incollection{jamshidi_landing_2014,
 address = {{Cham}},
 author = {Benavidez, Patrick J. and Lambert, Josue and Jaimes, Aldo and Jamshidi, Mo},
 booktitle = {Advance {{Trends}} in {{Soft Computing}}},
 editor = {Jamshidi, Mo and Kreinovich, Vladik and Kacprzyk, Janusz},
 file = {/home/matt/Zotero/storage/7M9PCK2H/landing_cuadracopter_mobile_base_Fuzzy_springer.pdf},
 isbn = {978-3-319-03673-1 978-3-319-03674-8},
 pages = {429--437},
 publisher = {{Springer International Publishing}},
 title = {Landing of a {{Quadcopter}} on a {{Mobile Base Using Fuzzy Logic}}},
 volume = {312},
 year = {2014}
}

@article{jamshidnejad_integrated_2019,
 author = {Jamshidnejad, Anahita and Gomes, Gabriel and Bayen, Alexandre M. and De Schutter, Bart},
 journal = {ArXiv preprint},
 title = {Integrated {{Offline}} and {{Online Optimization}}-{{Based Control}} in a {{Base}}-{{Parallel Architecture}}},
 url = {https://arxiv.org/abs/1907.05464},
 volume = {abs/1907.05464},
 year = {2019}
}

@article{janai_computer_2020,
 abstract = {Computer Vision for Autonomous Vehicles: Problems, Datasets and State of the Art},
 author = {Janai, Joel and G{\"u}ney, Fatma and Behl, Aseem and Geiger, Andreas},
 doi = {10.1561/0600000079},
 file = {/home/matt/Zotero/storage/67U8UQNU/Janai et al. - 2020 - Computer Vision for Autonomous Vehicles Problems,.pdf;/home/matt/Zotero/storage/8DA6349J/CGV-079.html;/home/matt/Zotero/storage/QX9DFT6P/CGV-079.html},
 issn = {1572-2740, 1572-2759},
 journal = {Foundations and Trends\textregistered{} in Computer Graphics and Vision},
 language = {English},
 number = {1\textendash 3},
 pages = {1--308},
 publisher = {{Now Publishers, Inc.}},
 shorttitle = {Computer {{Vision}} for {{Autonomous Vehicles}}},
 title = {Computer {{Vision}} for {{Autonomous Vehicles}}: {{Problems}}, {{Datasets}} and {{State}} of the {{Art}}},
 volume = {12},
 year = {2020}
}

@article{jang_dual_2012,
 author = {Jang, Kitae and Cassidy, Michael J.},
 doi = {10.1016/j.tra.2012.01.008},
 file = {/home/matt/Zotero/storage/KDI4NTVC/2012_TRA_jangcassidy_dualinfluences.pdf},
 issn = {09658564},
 journal = {Transportation Research Part A: Policy and Practice},
 language = {en},
 number = {7},
 pages = {1108--1123},
 title = {Dual Influences on Vehicle Speed in Special-Use Lanes and Critique of {{US}} Regulation},
 volume = {46},
 year = {2012}
}

@inproceedings{jang_simulation_2019,
 author = {Jang, Kathy and Vinitsky, Eugene and Chalaki, Behdad and Remer, Ben and Beaver, Logan and Malikopoulos, Andreas A. and Bayen, Alexandre},
 booktitle = {Proceedings of the 10th {{ACM}}/{{IEEE International Conference}} on {{Cyber}}-{{Physical Systems}}},
 doi = {10.1145/3302509.3313784},
 file = {/home/matt/Zotero/storage/8PKLDYFW/Jang et al. - 2019 - Simulation to scaled city zero-shot policy transf.pdf},
 isbn = {978-1-4503-6285-6},
 pages = {291--300},
 publisher = {{ACM}},
 shorttitle = {Simulation to Scaled City},
 title = {Simulation to Scaled City: Zero-Shot Policy Transfer for Traffic Control via Autonomous Vehicles},
 year = {2019}
}

@article{jang_traffic_2012,
 author = {Jang, Kitae and Oum, Sanghyouk and Chan, Ching-Yao},
 doi = {10.3141/2278-20},
 file = {/home/matt/Zotero/storage/FM9NTCTX/2012_TRR_jang_friction.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {180--193},
 shorttitle = {Traffic {{Characteristics}} of {{High}}-{{Occupancy Vehicle Facilities}}},
 title = {Traffic {{Characteristics}} of {{High}}-{{Occupancy Vehicle Facilities}}: {{Comparison}} of {{Contiguous}} and {{Buffer}}-{{Separated Lanes}}},
 volume = {2278},
 year = {2012}
}

@article{janocha_loss_2017,
 author = {Janocha, Katarzyna and Czarnecki, Wojciech Marian},
 journal = {ArXiv preprint},
 title = {On {{Loss Functions}} for {{Deep Neural Networks}} in {{Classification}}},
 url = {https://arxiv.org/abs/1702.05659},
 volume = {abs/1702.05659},
 year = {2017}
}

@article{jayakrishnan_evaluation_1994,
 author = {Jayakrishnan, R. and Mahmassani, H. S. and Lin, T.-Y.},
 journal = {Transportation Research C},
 number = {3},
 pages = {129--147},
 title = {An Evaluation Tool for Advanced Traffic Information and Management Systems in Urban Networks},
 volume = {2},
 year = {1994}
}

@inproceedings{jayaraman_time-agnostic_2019,
 author = {Dinesh Jayaraman and
Frederik Ebert and
Alexei A. Efros and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/JayaramanEEL19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Time-Agnostic Prediction: Predicting Predictable Video Frames},
 url = {https://openreview.net/forum?id=SyzVb3CcFX},
 year = {2019}
}

@inproceedings{jeon_reward-rational_2020,
 author = {Hong Jun Jeon and
Smitha Milli and
Anca D. Dragan},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/JeonMD20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Reward-rational (implicit) choice: {A} unifying formalism for reward
learning},
 url = {https://proceedings.neurips.cc/paper/2020/hash/2f10c1578a0706e06b6d7db6f0b4a6af-Abstract.html},
 year = {2020}
}

@inproceedings{ji_invariant_2019,
 author = {Xu Ji and
Andrea Vedaldi and
Jo{\~{a}}o F. Henriques},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/JiVH19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00996},
 pages = {9864--9873},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Invariant Information Clustering for Unsupervised Image Classification
and Segmentation},
 url = {https://doi.org/10.1109/ICCV.2019.00996},
 year = {2019}
}

@unpublished{jia_congestion_2000,
 author = {Jia, Z. and Varaiya, P. and Chen, C. and Petty, K. and Skabardonis, A.},
 title = {Congestion, Excess Demand and Effective Capacity in {{California}} Freeways},
 year = {2000}
}

@article{jia_empirical_2019,
 author = {Jia, Ruoxi and Sun, Xuehui and Xu, Jiacen and Zhang, Ce and Li, Bo and Song, Dawn},
 journal = {ArXiv preprint},
 title = {An {{Empirical}} and {{Comparative Analysis}} of {{Data Valuation}} with {{Scalable Algorithms}}},
 url = {https://arxiv.org/abs/1911.07128},
 volume = {abs/1911.07128},
 year = {2019}
}

@unpublished{jia_maximum_2001,
 author = {Jia, Z. and Varaiya, P. and Chen, C. and Petty, K. and Skabardonis, A.},
 title = {Maximum Throughput in {{LA}} Occurs at 60 Mph},
 year = {2001}
}

@inproceedings{jia_pems_2001,
 author = {Jia, Zhanfeng and Chen, Chao and Coifman, Ben and Varaiya, Pravin},
 booktitle = {2001 {{IEEE Intelligent Transportation Systems Proceedings}}},
 doi = {10.1109/ITSC.2001.948715},
 file = {/home/matt/Zotero/storage/83EV7328/jia_pems.pdf},
 isbn = {0-7803-7194-1},
 pages = {536--541},
 publisher = {{IEEE}},
 title = {The {{PeMS}} Algorithms for Accurate, Real-Time Estimates of g-Factors and Speeds from Single-Loop Detectors},
 year = {2001}
}

@inproceedings{jia_towards_2019,
 author = {Ruoxi Jia and
David Dao and
Boxin Wang and
Frances Ann Hubis and
Nick Hynes and
Nezihe Merve G{\"{u}}rel and
Bo Li and
Ce Zhang and
Dawn Song and
Costas J. Spanos},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aistats/JiaDWHHGLZSS19.bib},
 booktitle = {The 22nd International Conference on Artificial Intelligence and Statistics,
{AISTATS} 2019, 16-18 April 2019, Naha, Okinawa, Japan},
 editor = {Kamalika Chaudhuri and
Masashi Sugiyama},
 pages = {1167--1176},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 12 Jan 2021 00:00:00 +0100},
 title = {Towards Efficient Data Valuation Based on the Shapley Value},
 url = {http://proceedings.mlr.press/v89/jia19a.html},
 volume = {89},
 year = {2019}
}

@unpublished{jia_z._maximum_2001,
 author = {{Jia, Z.} and Varaiya, P. and Chen, C. and Petty, K. and Skabardonis, A.},
 title = {Maximum Throughput in {{LA}} Freeways Occurs at 60 Mph v. 4},
 year = {2001}
}

@inproceedings{jiang_learning_2018,
 author = {Jiechuan Jiang and
Zongqing Lu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/JiangL18.bib},
 booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
on Neural Information Processing Systems 2018, NeurIPS 2018, December
3-8, 2018, Montr{\'{e}}al, Canada},
 editor = {Samy Bengio and
Hanna M. Wallach and
Hugo Larochelle and
Kristen Grauman and
Nicol{\`{o}} Cesa{-}Bianchi and
Roman Garnett},
 pages = {7265--7275},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Learning Attentional Communication for Multi-Agent Cooperation},
 url = {https://proceedings.neurips.cc/paper/2018/hash/6a8018b3a00b69c008601b8becae392b-Abstract.html},
 year = {2018}
}

@article{jin_distribution_2003,
 author = {Jin, W.L. and Zhang, H. M.},
 journal = {Transportation Research, Part B},
 number = {6},
 pages = {521--540},
 title = {On the Distribution Schemes for Determining Flows through a Merge.},
 volume = {37},
 year = {2003}
}

@book{jin_gnss_2014,
 address = {{Dordrecht}},
 author = {Jin, Shuanggen and Cardellach, Estel and Xie, Feiqin},
 file = {/home/matt/Zotero/storage/YFRKKT8A/Jin - 2013 - GNSS remote sensing theory, methods and applicati.pdf},
 isbn = {978-94-007-7481-0},
 language = {en},
 publisher = {{Springer}},
 shorttitle = {{{GNSS Remote Sensing}}},
 title = {{{GNSS Remote Sensing}}: {{Theory}}, {{Methods}} and {{Applications}}},
 year = {2014}
}

@inproceedings{jin_hierarchical_2020,
 author = {Wengong Jin and
Regina Barzilay and
Tommi S. Jaakkola},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/JinBJ20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {4839--4848},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Hierarchical Generation of Molecular Graphs using Structural Motifs},
 url = {http://proceedings.mlr.press/v119/jin20a.html},
 volume = {119},
 year = {2020}
}

@article{jin_kinematic_2010,
 abstract = {Frequent lane-changes in highway merging, diverging, and weaving areas could disrupt traffic flow and, even worse, lead to accidents. In this paper, we propose a simple model for studying bottleneck effects of lane-changing traffic and aggregate traffic dynamics of a roadway with lane-changing areas. Based on the observation that, when changing its lane, a vehicle affects traffic on both its current and target lanes, we propose to capture such lateral interactions by introducing a new lane-changing intensity variable. With a modified fundamental diagram, we are able to study the impacts of lane-changing traffic on overall traffic flow. In addition, the corresponding traffic dynamics can be described with a simple kinematic wave model. For a location-dependent lane-changing intensity variable, we discuss kinematic wave solutions of the Riemann problem of the new model and introduce a supply\textendash demand method for its numerical solutions. With both theoretical and empirical analysis, we demonstrate that lane-changes could have significant bottleneck effects on overall traffic flow. In the future, we will be interested in studying lane-changing intensities for different road geometries, locations, on-ramp/off-ramp flows, as well as traffic conditions. The new modeling framework could be helpful for developing ramp-metering and other lane management strategies to mitigate the bottleneck effects of lane-changes.},
 author = {Jin, Wen-Long},
 doi = {10.1016/j.trb.2009.12.014},
 file = {/home/matt/Zotero/storage/DD6GPTZS/Jin - 2010 - A kinematic wave theory of lane-changing traffic f.pdf;/home/matt/Zotero/storage/VKDMNXVL/Jin - 2010 - A kinematic wave theory of lane-changing traffic f.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {8-9},
 pages = {1001--1021},
 title = {A Kinematic Wave Theory of Lane-Changing Traffic Flow},
 volume = {44},
 year = {2010}
}

@article{jin_multi-commodity_2013,
 abstract = {Systematic lane changes can seriously deteriorate traffic safety and efficiency inside lanedrop, merge, and other bottleneck areas. In our previous studies (Jin, 2010a,b), a phenomenological model of lane-changing traffic flow was proposed, calibrated, and analyzed based on a new concept of lane-changing intensity. In this study, we further consider weaving and non-weaving vehicles as two commodities and develop a multi-commodity, behavioral Lighthill\textendash Whitham\textendash Richards (LWR) model of lane-changing traffic flow. Based on a macroscopic model of lane-changing behaviors, we derive a fundamental diagram with parameters determined by car-following and lane-changing characteristics as well as road geometry and traffic composition. We further calibrate and validate fundamental diagrams corresponding to a triangular car-following fundamental diagram with NGSIM data. We introduce an entropy condition for the multi-commodity LWR model and solve the Riemann problem inside a homogeneous lane-changing area. From the Riemann solutions, we derive a flux function in terms of traffic demand and supply. Then we apply the model to study lane-changing traffic dynamics inside a lane-drop area and show that the smoothing effect of HOV lanes is consistent with observations in existing studies. The new theory of lane-changing traffic flow can be readily incorporated into Cell Transmission Model, and this study could lead to better strategies for mitigating bottleneck effects of lane-changing traffic flow.},
 author = {Jin, Wen-Long},
 doi = {10.1016/j.trb.2013.06.002},
 file = {/home/matt/Zotero/storage/4XU5QTXU/Jin - 2013 - A multi-commodity Lighthill–Whitham–Richards model.pdf;/home/matt/Zotero/storage/F87TX5P7/Jin - 2013 - A multi-commodity Lighthill–Whitham–Richards model.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {361--377},
 title = {A Multi-Commodity {{Lighthill}}\textendash{{Whitham}}\textendash{{Richards}} Model of Lane-Changing Traffic Flow},
 volume = {57},
 year = {2013}
}

@article{jin_riemann_2017,
 author = {Jin, Wen-Long},
 doi = {10.1016/j.trb.2016.12.007},
 file = {/home/matt/Zotero/storage/QXQVSFH3/jin_riemannsolver_junction.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {21--41},
 title = {A {{Riemann}} Solver for a System of Hyperbolic Conservation Laws at a General Road Junction},
 volume = {98},
 year = {2017}
}

@inproceedings{jin_robust_2019,
 abstract = {Cable manipulation is a challenging task for robots. The major challenge is that cables have high degrees of freedom and are easy to deform during manipulation. In this paper, we propose a novel framework SPR-RWLS to manipulate cables, which includes real-time cable tracking and robust local deformation model approximation. For cable tracking, structure preserved registration (SPR) is utilized to robustly estimate the movement of selected points on a cable even in the presence of sensor noise, outliers, and occlusions. Robust weighted least squares (RWLS) is then applied to calculate the local deformation model of the cable under uncertainties. We show that SPR-RWLS enables the dual-arm robots to manipulate cables with different thicknesses and lengths to different desired curvatures in multiple scenarios. We also show that real-time implementation of the proposed method can be simplified by parallel computation.},
 address = {{Macau, China}},
 author = {Jin, Shiyu and Wang, Changhao and Tomizuka, Masayoshi},
 booktitle = {2019 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}} ({{IROS}})},
 doi = {10.1109/IROS40897.2019.8968157},
 file = {/home/matt/Zotero/storage/N3NCRQDB/Jin et al. - 2019 - Robust Deformation Model Approximation for Robotic.pdf},
 isbn = {978-1-72814-004-9},
 language = {en},
 pages = {6586--6593},
 publisher = {{IEEE}},
 title = {Robust {{Deformation Model Approximation}} for {{Robotic Cable Manipulation}}},
 year = {2019}
}

@article{johnson_audi_2013,
 author = {Johnson, D.},
 journal = {Left Lane News},
 title = {Audi Predicts Self-Driving Cars by 2020},
 year = {2013}
}

@inproceedings{johnson_clevr_2017,
 author = {Justin Johnson and
Bharath Hariharan and
Laurens van der Maaten and
Li Fei{-}Fei and
C. Lawrence Zitnick and
Ross B. Girshick},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/JohnsonHMFZG17.bib},
 booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
 doi = {10.1109/CVPR.2017.215},
 pages = {1988--1997},
 publisher = {{IEEE} Computer Society},
 timestamp = {Sat, 30 May 2020 01:00:00 +0200},
 title = {{CLEVR:} {A} Diagnostic Dataset for Compositional Language and Elementary
Visual Reasoning},
 url = {https://doi.org/10.1109/CVPR.2017.215},
 year = {2017}
}

@article{joshi_spanbert_2020,
 author = {Joshi, Mandar  and
Chen, Danqi  and
Liu, Yinhan  and
Weld, Daniel S.  and
Zettlemoyer, Luke  and
Levy, Omer},
 doi = {10.1162/tacl_a_00300},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {64--77},
 title = {{S}pan{BERT}: Improving Pre-training by Representing and Predicting Spans},
 url = {https://aclanthology.org/2020.tacl-1.5},
 volume = {8},
 year = {2020}
}

@article{jovanovic_passivity-based_2008,
 author = {Jovanovic, M. and Arcak, M. and Sontag, E.},
 journal = {IEEE Trans. Auto. Contr.},
 number = {1},
 pages = {75--86},
 title = {A Passivity-Based Approach to Stability of Spatially Distributed Systems with Interconnection Structure},
 volume = {53},
 year = {2008}
}

@techreport{jr_freeway_1997,
 author = {Jr, James D. Carvel and Balke, Kevin and Ullman, Jerry and Fitzpatrick, Katerine and Nowlin, Lewis and Brehmer, Christopher},
 institution = {{Department of Transportation, Federal Highway Administration}},
 number = {FHWA-SA-97-064},
 title = {Freeway {{Management Handbook}}},
 year = {1997}
}

@article{jr_i-394_2007,
 author = {Jr, L. W. Munnich and Buckeye, {and} K. R.},
 journal = {Transportation Research Record},
 number = {1996},
 pages = {49--57},
 title = {I-394 {{MnPASS High}}-{{Occupancy Toll Lanes Planning}} and {{Operational Issues}} and {{Outcomes}} ({{Lessons Learned}} in {{Year}} 1)},
 year = {2007}
}

@inproceedings{ju_e-abs_2020,
 abstract = {Schott et al. introduced Analysis-by-Synthesis (ABS), a generative-model-based classifier that achieves state-of-the-art robustness on MNIST but does not scale to complex datasets, such as SVHN. In this paper, we present E-ABS, an improvement to ABS that achieves better accuracy and robustness than ABS on complex datasets. Inspired by recent findings on the shortcomings of generative models in handling out-of-distribution samples, E-ABS improves on ABS using adversarial autoencoders with a discriminative loss. Our experiments show that E-ABS outperforms both ABS and adversarial training on SVHN and a European traffic sign dataset, achieving state-ofthe-art robustness on these datasets.},
 author = {Ju, An and Wagner, David},
 booktitle = {Submitted to 37th {{International Conference}} on {{Machine Learning}} ({{ICML}} 2020)},
 file = {/home/matt/Zotero/storage/5WTSY226/Ju and Wagner - E-ABS Extending the Analysis-By-Synthesis Robust .pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {E-{{ABS}}: {{Extending}} the {{Analysis}}-{{By}}-{{Synthesis Robust Classification Model}} to {{Complex Image Domains}}},
 year = {2020}
}

@article{kahn_badgr_2020,
 author = {Kahn, Gregory and Abbeel, Pieter and Levine, Sergey},
 journal = {ArXiv preprint},
 title = {{{BADGR}}: {{An Autonomous Self}}-{{Supervised Learning}}-{{Based Navigation System}}},
 url = {https://arxiv.org/abs/2002.05700},
 volume = {abs/2002.05700},
 year = {2020}
}

@article{kalman_new_1960,
 author = {Kalman, Rudolf Emil},
 doi = {10.1115/1.3662552},
 file = {/home/matt/Zotero/storage/7KVDMHBH/Kalman - 1960 - A New Approach to Linear Filtering and Prediction .pdf;/home/matt/Zotero/storage/I9CVTZVU/article.html},
 issn = {0021-9223},
 journal = {Journal of Basic Engineering},
 number = {1},
 pages = {35--45},
 title = {A {{New Approach}} to {{Linear Filtering}} and {{Prediction Problems}}},
 volume = {82},
 year = {1960}
}

@article{kang_emergency_2004,
 author = {Kang, Y and Hedrick, JK},
 journal = {International journal of automotive technology},
 number = {2},
 pages = {89--94},
 title = {Emergency Braking Control of a Platoon Using String Stable Controller},
 volume = {5},
 year = {2004}
}

@inproceedings{kang_few-shot_2018,
 author = {Bingyi Kang and
Zhuang Liu and
Xin Wang and
Fisher Yu and
Jiashi Feng and
Trevor Darrell},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/KangLWYFD19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00851},
 pages = {8419--8428},
 publisher = {{IEEE}},
 timestamp = {Tue, 17 Mar 2020 00:00:00 +0100},
 title = {Few-Shot Object Detection via Feature Reweighting},
 url = {https://doi.org/10.1109/ICCV.2019.00851},
 year = {2019}
}

@article{kannan_adversarial_2018,
 author = {Kannan, Harini and Kurakin, Alexey and Goodfellow, Ian},
 journal = {ArXiv preprint},
 title = {Adversarial {{Logit Pairing}}},
 url = {https://arxiv.org/abs/1803.06373},
 volume = {abs/1803.06373},
 year = {2018}
}

@inproceedings{kapania_hybrid_2019,
 abstract = {As autonomous vehicles (AVs) inch closer to reality, a central requirement for acceptance will be earning the trust of humans in everyday driving situations. In particular, the interaction between AVs and pedestrians is of high importance, as every human is a pedestrian at some point of the day. This paper considers the interaction of a pedestrian and an autonomous vehicle at a mid-block, unsignalized intersection where there is ambiguity over when the pedestrian should cross and when and how the vehicle should yield. By modeling pedestrian behavior through the concept of gap acceptance, the authors show that a hybrid controller with just four distinct modes allows an autonomous vehicle to successfully interact with a pedestrian across a continuous spectrum of possible crosswalk entry behaviors. The controller is validated through extensive simulation and compared to an alternate POMDP solution and experimental results are provided on a research vehicle for a virtual pedestrian.},
 author = {Kapania, N. R. and Govindarajan, V. and Borrelli, F. and Gerdes, J. C.},
 booktitle = {2019 {{IEEE Intelligent Vehicles Symposium}} ({{IV}})},
 doi = {10.1109/IVS.2019.8814116},
 file = {/home/matt/Zotero/storage/E44LK8H2/Kapania et al_2019_A Hybrid Control Design for Autonomous Vehicles at Uncontrolled Crosswalks.pdf;/home/matt/Zotero/storage/WCUGWBBH/8814116.html},
 pages = {1604--1611},
 title = {A {{Hybrid Control Design}} for {{Autonomous Vehicles}} at {{Uncontrolled Crosswalks}}},
 year = {2019}
}

@article{kaplan_chinas_2017,
 abstract = {This study analyses the feasibility of China's One Belt, One Road (OBOR) initiative from an institutionalist perspective. The initiative is undertaken as a `geo-functional institutionalist' project, and this strengthens its feasibility. Firstly, the initiative aims to institutionalize a new international structure paralleling the existing Westerndominated one through which China could re-organize its position as an `agenda entrepreneur' in the world without any clash with the West. Secondly, the initiative follows a functionalist strategy. It offers a `win-win'functionalist framework without any hegemonic ambition; thus, the initiative attracts the attention of the rest of the world. China also follows a pure functionalist and bilateral/regional way to deal with the heterogeneity problem among the target countries. However, China's institutionalization attempt might be isomorphic with the existing Western-dominated system in terms of its hegemonic structure due to the cognitive limitations in finding alternatives, and this might ruin the feasibility of the initiative.},
 author = {Kaplan, Yilmaz},
 doi = {10.1515/bjes-2017-0002},
 file = {/home/matt/Zotero/storage/BDJFLUD4/Kaplan - 2017 - China’s OBOR as a Geo-Functional Institutionalist .pdf},
 issn = {2228-0596},
 journal = {Baltic Journal of European Studies},
 language = {en},
 number = {1},
 pages = {7--23},
 title = {China's {{OBOR}} as a {{Geo}}-{{Functional Institutionalist Project}}},
 volume = {7},
 year = {2017}
}

@article{kaplan_scaling_2020,
 author = {Kaplan, Jared and McCandlish, Sam and Henighan, Tom and Brown, Tom B. and Chess, Benjamin and Child, Rewon and Gray, Scott and Radford, Alec and Wu, Jeffrey and Amodei, Dario},
 journal = {ArXiv preprint},
 title = {Scaling {{Laws}} for {{Neural Language Models}}},
 url = {https://arxiv.org/abs/2001.08361},
 volume = {abs/2001.08361},
 year = {2020}
}

@article{kar_random_2012,
 author = {Kar, Purushottam and Karnick, Harish},
 journal = {ArXiv preprint},
 title = {Random {{Feature Maps}} for {{Dot Product Kernels}}},
 url = {https://arxiv.org/abs/1201.6530},
 volume = {abs/1201.6530},
 year = {2012}
}

@article{karaman_sampling-based_2011,
 author = {Karaman, Sertac and Frazzoli, Emilio},
 doi = {10.1177/0278364911406761},
 file = {/home/matt/Zotero/storage/LXXSH44V/Karaman and Frazzoli - 2011 - Sampling-based algorithms for optimal motion plann.pdf},
 issn = {0278-3649, 1741-3176},
 journal = {The International Journal of Robotics Research},
 language = {en},
 number = {7},
 pages = {846--894},
 title = {Sampling-Based Algorithms for Optimal Motion Planning},
 volume = {30},
 year = {2011}
}

@article{karamihas_pavement_2004,
 author = {Karamihas, S. M. and Rada, G. R. and Ostrom, B. K. and Simpson, A. L. and Wiser, L. J.},
 journal = {Transportation Research Record},
 pages = {116--123},
 title = {Pavement {{Smoothness}} at {{Weigh}}-in-{{Motion Sites}}: {{Developing Specifications}} for the {{Long}}-{{Term Pavement Performance Program}}},
 volume = {1870},
 year = {2004}
}

@inproceedings{karimireddy_scaffold_2020,
 author = {Sai Praneeth Karimireddy and
Satyen Kale and
Mehryar Mohri and
Sashank J. Reddi and
Sebastian U. Stich and
Ananda Theertha Suresh},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/KarimireddyKMRS20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {5132--5143},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {{SCAFFOLD:} Stochastic Controlled Averaging for Federated Learning},
 url = {http://proceedings.mlr.press/v119/karimireddy20a.html},
 volume = {119},
 year = {2020}
}

@inproceedings{karl_deep_2017,
 author = {Maximilian Karl and
Maximilian Soelch and
Justin Bayer and
Patrick van der Smagt},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KarlSBS17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Mon, 31 Aug 2020 01:00:00 +0200},
 title = {Deep Variational Bayes Filters: Unsupervised Learning of State Space
Models from Raw Data},
 url = {https://openreview.net/forum?id=HyTqHL5xg},
 year = {2017}
}

@article{katrakazas_real-time_2015,
 abstract = {Currently autonomous or self-driving vehicles are at the heart of academia and industry research because of its multi-faceted advantages that includes improved safety, reduced congestion, lower emissions and greater mobility. Software is the key driving factor underpinning autonomy within which planning algorithms that are responsible for mission-critical decision making hold a significant position. While transporting passengers or goods from a given origin to a given destination, motion planning methods incorporate searching for a path to follow, avoiding obstacles and generating the best trajectory that ensures safety, comfort and efficiency. A range of different planning approaches have been proposed in the literature. The purpose of this paper is to review existing approaches and then compare and contrast different methods employed for the motion planning of autonomous on-road driving that consists of (1) finding a path, (2) searching for the safest manoeuvre and (3) determining the most feasible trajectory. Methods developed by researchers in each of these three levels exhibit varying levels of complexity and performance accuracy. This paper presents a critical evaluation of each of these methods, in terms of their advantages/disadvantages, inherent limitations, feasibility, optimality, handling of obstacles and testing operational environments.},
 author = {Katrakazas, Christos and Quddus, Mohammed and Chen, Wen-Hua and Deka, Lipika},
 doi = {10.1016/j.trc.2015.09.011},
 file = {/home/matt/Zotero/storage/XGYQW7KL/Katrakazas et al. - 2015 - Real-time motion planning methods for autonomous o.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {416--442},
 shorttitle = {Real-Time Motion Planning Methods for Autonomous on-Road Driving},
 title = {Real-Time Motion Planning Methods for Autonomous on-Road Driving: {{State}}-of-the-Art and Future Research Directions},
 volume = {60},
 year = {2015}
}

@article{keeler_optimal_1977,
 author = {Keeler, T. E. and Small, K. A.},
 journal = {Journal of Political Economy},
 number = {},
 pages = {1--25},
 title = {Optimal Peak Load Pricing, Investment, and Service Levels on Urban Expressways},
 volume = {85},
 year = {1977}
}

@article{kehoe_survey_2015,
 abstract = {The Cloud infrastructure and its extensive set of Internet-accessible resources has potential to provide significant benefits to robots and automation systems. We consider robots and automation systems that rely on data or code from a network to support their operation, i.e., where not all sensing, computation, and memory is integrated into a standalone system. This survey is organized around four potential benefits of the Cloud: 1) Big Data: access to libraries of images, maps, trajectories, and descriptive data; 2) Cloud Computing: access to parallel grid computing on demand for statistical analysis, learning, and motion planning; 3) Collective Robot Learning: robots sharing trajectories, control policies, and outcomes; and 4) Human Computation: use of crowdsourcing to tap human skills for analyzing images and video, classification, learning, and error recovery. The Cloud can also improve robots and automation systems by providing access to: a) datasets, publications, models, benchmarks, and simulation tools; b) open competitions for designs and systems; and c) open-source software. This survey includes over 150 references on results and open challenges. A website with new developments and updates is available at: http://goldberg.berkeley.edu/cloud-robotics/.},
 author = {Kehoe, B. and Patil, S. and Abbeel, P. and Goldberg, K.},
 doi = {10.1109/TASE.2014.2376492},
 file = {/home/matt/Zotero/storage/WDPMEPX8/Kehoe et al. - 2015 - A Survey of Research on Cloud Robotics and Automat.pdf;/home/matt/Zotero/storage/ZALRIU6D/7006734.html},
 issn = {1545-5955},
 journal = {IEEE Transactions on Automation Science and Engineering},
 keywords = {Automation,automation system,Big data,Big Data,cloud automation,cloud computing,Cloud computing,cloud robotics,collective robot learning,Computational modeling,control engineering computing,crowdsourcing,grid computing,groupware,human computation,learning (artificial intelligence),open source,outsourcing,parallel grid computing,parallel processing,Robot kinematics,Robot sensing systems,robots,robots sharing trajectory},
 number = {2},
 pages = {398--409},
 title = {A {{Survey}} of {{Research}} on {{Cloud Robotics}} and {{Automation}}},
 volume = {12},
 year = {2015}
}

@techreport{kell_traffic_1990,
 author = {Kell, James H. and Fullerton, Iris J. and Mills, Milton K.},
 institution = {{U.S. Department of Transportation, Federal Highway Administration, Office of Research and Development}},
 number = {FHWA-IP-90-002},
 title = {Traffic {{Detector Handbook}}},
 year = {1990}
}

@article{kelly_charging_1997,
 author = {Kelly, F. P.},
 journal = {European Transactions on Telcommunications},
 pages = {33--37},
 title = {Charging and Rate Control for Elastic Traffic},
 volume = {8},
 year = {1997}
}

@article{kelly_road_2006,
 author = {Kelly, F. P.},
 journal = {Ingenia},
 pages = {36--40},
 title = {Road {{Pricing}}},
 volume = {29},
 year = {2006}
}

@inproceedings{kendall_what_2017,
 author = {Alex Kendall and
Yarin Gal},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KendallG17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {5574--5584},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {What Uncertainties Do We Need in Bayesian Deep Learning for Computer
Vision?},
 url = {https://proceedings.neurips.cc/paper/2017/hash/2650d6089a6d640c5e85b2b88265dc2b-Abstract.html},
 year = {2017}
}

@article{kerns_unmanned_2014,
 author = {Kerns, Andrew J. and Shepard, Daniel P. and Bhatti, Jahshan A. and Humphreys, Todd E.},
 doi = {10.1002/rob.21513},
 file = {/home/matt/Zotero/storage/9ZWYE36R/Kerns et al. - 2014 - Unmanned Aircraft Capture and Control Via GPS Spoo.pdf},
 issn = {15564959},
 journal = {Journal of Field Robotics},
 language = {en},
 number = {4},
 pages = {617--636},
 shorttitle = {Unmanned {{Aircraft Capture}} and {{Control Via GPS Spoofing}}},
 title = {Unmanned {{Aircraft Capture}} and {{Control Via GPS Spoofing}}: {{Unmanned Aircraft Capture}} and {{Control}}},
 volume = {31},
 year = {2014}
}

@article{kesur_optimization_2012,
 author = {Kesur, K.B.},
 journal = {Journal of Advanced Transportation},
 number = {5},
 pages = {431--442},
 title = {Optimization of Mixed Cycle Length Traffic Signals},
 volume = {48},
 year = {2012}
}

@inproceedings{keysers_measuring_2020,
 author = {Daniel Keysers and
Nathanael Sch{\"{a}}rli and
Nathan Scales and
Hylke Buisman and
Daniel Furrer and
Sergii Kashubin and
Nikola Momchev and
Danila Sinopalnikov and
Lukasz Stafiniak and
Tibor Tihon and
Dmitry Tsarkov and
Xiao Wang and
Marc van Zee and
Olivier Bousquet},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KeysersSSBFKMSS20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Measuring Compositional Generalization: {A} Comprehensive Method on
Realistic Data},
 url = {https://openreview.net/forum?id=SygcCnNKwr},
 year = {2020}
}

@inproceedings{khandelwal_generalization_2020,
 author = {Urvashi Khandelwal and
Omer Levy and
Dan Jurafsky and
Luke Zettlemoyer and
Mike Lewis},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KhandelwalLJZL20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Generalization through Memorization: Nearest Neighbor Language Models},
 url = {https://openreview.net/forum?id=HklBjCEKvH},
 year = {2020}
}

@inproceedings{khasahmadi_memory-based_2020,
 author = {Amir Hosein Khas Ahmadi and
Kaveh Hassani and
Parsa Moradi and
Leo Lee and
Quaid Morris},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/AhmadiHMLM20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Memory-Based Graph Networks},
 url = {https://openreview.net/forum?id=r1laNeBYPB},
 year = {2020}
}

@inproceedings{khout_integrating_2009,
 author = {Khout, N. and Borrelli, F. and Hedrick, K.},
 booktitle = {12th {{IFAC Symposium}} on {{Control}} in {{Transportation Systems}}. {{Redondo Beach}}, {{California}}},
 title = {Integrating {{Traffic Data}} and {{Model Predictive Control}} to {{Improve Fuel Economy}}},
 year = {Semptember 2009}
}

@inproceedings{khout_utilization_2008,
 author = {Khout, N. and Borrelli, F. and Hedrick, K.},
 booktitle = {15th {{World Congress}} on {{ITS}}},
 title = {Utilization {{Of Intelligent Transport Systems Information To Increase Fuel Economy Through Engine Control}}},
 year = {2008}
}

@inproceedings{Kim_2019_CVPR,
 author = {Jinkyu Kim and
Teruhisa Misu and
Yi{-}Ting Chen and
Ashish Tawari and
John F. Canny},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/KimMCTC19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.01084},
 pages = {10591--10599},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Grounding Human-To-Vehicle Advice for Self-Driving Vehicles},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Kim\_Grounding\_Human-To-Vehicle\_Advice\_for\_Self-Driving\_Vehicles\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{kim_code_2020,
 author = {Kim, Seohyun and Zhao, Jinman and Tian, Yuchi and Chandra, Satish},
 journal = {ArXiv preprint},
 title = {Code {{Prediction}} by {{Feeding Trees}} to {{Transformers}}},
 url = {https://arxiv.org/abs/2003.13848},
 volume = {abs/2003.13848},
 year = {2020}
}

@inproceedings{kim_grounding_nodate,
 author = {Jinkyu Kim and
Teruhisa Misu and
Yi{-}Ting Chen and
Ashish Tawari and
John F. Canny},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/KimMCTC19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.01084},
 pages = {10591--10599},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Grounding Human-To-Vehicle Advice for Self-Driving Vehicles},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Kim\_Grounding\_Human-To-Vehicle\_Advice\_for\_Self-Driving\_Vehicles\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{kim_hardware---loop_2019,
 author = {Kim, Yeojun and Tay, Samuel and Guanetti, Jacopo and Borrelli, Francesco and Miller, Ryan},
 journal = {ArXiv preprint},
 title = {Hardware-{{In}}-the-{{Loop}} for {{Connected Automated Vehicles Testing}} in {{Real Traffic}}},
 url = {https://arxiv.org/abs/1907.09052},
 volume = {abs/1907.09052},
 year = {2019}
}

@inproceedings{kim_representation_2019,
 author = {Geewook Kim and
Akifumi Okuno and
Kazuki Fukui and
Hidetoshi Shimodaira},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/ijcai/KimOFS19.bib},
 booktitle = {Proceedings of the Twenty-Eighth International Joint Conference on
Artificial Intelligence, {IJCAI} 2019, Macao, China, August 10-16,
2019},
 doi = {10.24963/ijcai.2019/699},
 editor = {Sarit Kraus},
 pages = {5031--5038},
 publisher = {ijcai.org},
 timestamp = {Tue, 20 Aug 2019 01:00:00 +0200},
 title = {Representation Learning with Weighted Inner Product for Universal
Approximation of General Similarities},
 url = {https://doi.org/10.24963/ijcai.2019/699},
 year = {2019}
}

@inproceedings{kim_robust_2019,
 abstract = {We propose a cooperative adaptive cruise control which exploits a front vehicle acceleration forecast, available via vehicle-to-vehicle communication, to reduce vehicle energy consumption. The proposed control design can be applied to groups or platoons of cooperative vehicles, which locally optimize performance while maintaining their relative distance bounded at all times. The proposed approach adopts a learning-based model predictive control scheme, and maximizes performance while guaranteeing robust safety against the uncertainty on the front vehicle acceleration forecast. Simulations show the validity of the proposed control design.},
 author = {Kim, Y. and Guanetti, J. and Borrelli, F.},
 booktitle = {2019 18th {{European Control Conference}} ({{ECC}})},
 doi = {10.23919/ECC.2019.8796252},
 file = {/home/matt/Zotero/storage/KZECBLBH/Kim et al_2019_Robust Eco Adaptive Cruise Control for Cooperative Vehicles.pdf;/home/matt/Zotero/storage/IZZT3IKK/8796252.html},
 pages = {1214--1219},
 title = {Robust {{Eco Adaptive Cruise Control}} for {{Cooperative Vehicles}}},
 year = {2019}
}

@article{kim_safety_2018,
 abstract = {This paper investigates the crash-rate distribution of the freeway weaving segments with a bufferseparated high-occupancy-vehicle lane. For this purpose, crash, traffic and geometry data were extracted from various sources. These extracted data were either spatially or spatiotemporally matched with one another, and used for both descriptive and model-based analyses. The descriptive analysis revealed that crash-rate distributions of the weaving segments depend not only on the class of the subject highway but also on the presence of an access point. This finding was statistically confirmed by crash frequency models. Notably, both descriptive and model-based analyses showed that weaving segments with an access point tend to show lower crash-rates than the counterparts without one. One might attribute this counterintuitive phenomenon to a certain underlying tendency by which traffic engineers or planners generally follow in selecting locations of an access point along the freeway. Further research is required to resolve such a conjecture.},
 author = {Kim, Kwangho and Park, Byung-Jung},
 doi = {10.1080/17457300.2018.1431943},
 file = {/home/matt/Zotero/storage/TMPM5ZM2/Kim and Park - 2018 - Safety features of freeway weaving segments with a.pdf},
 issn = {1745-7300, 1745-7319},
 journal = {International Journal of Injury Control and Safety Promotion},
 language = {en},
 number = {3},
 pages = {284--292},
 title = {Safety Features of Freeway Weaving Segments with a Buffer-Separated High-Occupancy-Vehicle ({{HOV}}) Lane},
 volume = {25},
 year = {2018}
}

@article{kimeldorf_results_1971,
 abstract = {This report derives explicit solutions to problems involving Tchebycheffian spline functions. We use a reproducing kernel Hilbert space which depends on the smoothness criterion, but not on the form of the data, to solve explicitly Hermite-Birkhoff interpolation and smoothing problems. Sard's best approximation to linear functionals and smoothing with respect to linear inequality constraints are also discussed. Some of the results are used to show that spline interpolation and smoothing is equivalent to prediction and filtering on realizations of certain stochastic processes.},
 author = {Kimeldorf, George and Wahba, Grace},
 doi = {10.1016/0022-247X(71)90184-3},
 file = {/home/matt/Zotero/storage/YAFZKU4C/Kimeldorf and Wahba - 1971 - Some results on Tchebycheffian spline functions.pdf;/home/matt/Zotero/storage/NMSRFALT/0022247X71901843.html},
 issn = {0022-247X},
 journal = {Journal of Mathematical Analysis and Applications},
 language = {en},
 number = {1},
 pages = {82--95},
 title = {Some Results on {{Tchebycheffian}} Spline Functions},
 volume = {33},
 year = {1971}
}

@inproceedings{kingma_adam_2015,
 author = {Diederik P. Kingma and
Jimmy Ba},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/KingmaB14.bib},
 booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Adam: {A} Method for Stochastic Optimization},
 url = {http://arxiv.org/abs/1412.6980},
 year = {2015}
}

@inproceedings{kingma_bit-swap_2019,
 author = {Friso H. Kingma and
Pieter Abbeel and
Jonathan Ho},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/KingmaAH19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {3408--3417},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Bit-Swap: Recursive Bits-Back Coding for Lossless Compression with
Hierarchical Latent Variables},
 url = {http://proceedings.mlr.press/v97/kingma19a.html},
 volume = {97},
 year = {2019}
}

@inproceedings{kingma_glow_2018,
 author = {Diederik P. Kingma and
Prafulla Dhariwal},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KingmaD18.bib},
 booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
on Neural Information Processing Systems 2018, NeurIPS 2018, December
3-8, 2018, Montr{\'{e}}al, Canada},
 editor = {Samy Bengio and
Hanna M. Wallach and
Hugo Larochelle and
Kristen Grauman and
Nicol{\`{o}} Cesa{-}Bianchi and
Roman Garnett},
 pages = {10236--10245},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Glow: Generative Flow with Invertible 1x1 Convolutions},
 url = {https://proceedings.neurips.cc/paper/2018/hash/d139db6a236200b21cc7f752979132d0-Abstract.html},
 year = {2018}
}

@misc{kipf_keras-gcn_2017,
 author = {Kipf, Thomas N. and others},
 howpublished = {https://github.com/tkipf/keras-gcn},
 keywords = {⛔ No DOI found},
 title = {Keras-{{GCN}}},
 year = {2017}
}

@inproceedings{kipf_semi-supervised_2017,
 author = {Thomas N. Kipf and
Max Welling},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KipfW17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Semi-Supervised Classification with Graph Convolutional Networks},
 url = {https://openreview.net/forum?id=SJU4ayYgl},
 year = {2017}
}

@inproceedings{kitaev_reformer_2020,
 author = {Nikita Kitaev and
Lukasz Kaiser and
Anselm Levskaya},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KitaevKL20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Reformer: The Efficient Transformer},
 url = {https://openreview.net/forum?id=rkgNKkHtvB},
 year = {2020}
}

@article{kitchin_big_2014,
 abstract = {This article examines how the availability of Big Data, coupled with new data analytics, challenges established epistemologies across the sciences, social sciences and humanities, and assesses the extent to which they are engendering paradigm shifts across multiple disciplines. In particular, it critically explores new forms of empiricism that declare `the end of theory', the creation of data-driven rather than knowledge-driven science, and the development of digital humanities and computational social sciences that propose radically different ways to make sense of culture, history, economy and society. It is argued that: (1) Big Data and new data analytics are disruptive innovations which are reconfiguring in many instances how research is conducted; and (2) there is an urgent need for wider critical reflection within the academy on the epistemological implications of the unfolding data revolution, a task that has barely begun to be tackled despite the rapid changes in research practices presently taking place. After critically reviewing emerging epistemological positions, it is contended that a potentially fruitful approach would be the development of a situated, reflexive and contextually nuanced epistemology.},
 author = {Kitchin, Rob},
 doi = {10.1177/2053951714528481},
 file = {/home/matt/Zotero/storage/479QYQ5C/Kitchin - 2014 - Big Data, new epistemologies and paradigm shifts.pdf},
 issn = {2053-9517, 2053-9517},
 journal = {Big Data \& Society},
 language = {en},
 number = {1},
 pages = {205395171452848},
 title = {Big {{Data}}, New Epistemologies and Paradigm Shifts},
 volume = {1},
 year = {2014}
}

@book{kittelson_and_associates_southbound_2013,
 author = {{Kittelson and Associates}},
 title = {Southbound {{I}}-680 {{Express Lane Performance Evaluation An After Study}}: {{Executive Summary}}},
 year = {2013}
}

@techreport{klein_detection_1996,
 address = {{McLean, VA}},
 author = {Klein, Lawrence A.},
 institution = {{Federal Highway Administration}},
 number = {FHWA-RD-95-100},
 title = {Detection Technology for {{IVHS}}},
 year = {1996}
}

@inproceedings{klicpera_directional_2020,
 author = {Johannes Klicpera and
Janek Gro{\ss} and
Stephan G{\"{u}}nnemann},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/KlicperaGG20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Directional Message Passing for Molecular Graphs},
 url = {https://openreview.net/forum?id=B1eWbxStPH},
 year = {2020}
}

@phdthesis{koehler_applied_2016,
 abstract = {Industrial large-scale control problems present an interesting algorithmic design challenge. A number of controllers must cooperate in real-time on a network of embedded hardware with limited computing power in order to maximize system efficiency while respecting constraints and despite communication delays. Model predictive control (MPC) can automatically synthesize a centralized controller which optimizes an objective function subject to a system model, constraints, and predictions of disturbance. Unfortunately, the computations required by model predictive controllers for large-scale systems often limit its industrial implementation only to medium-scale slow processes.Distributed model predictive control (DMPC) enters the picture as a way to decentralize a large-scale model predictive control problem. The main idea of DMPC is to split the computations required by the MPC problem amongst distributed processors that can compute in parallel and communicate iteratively to find a solution. Some popularly proposed solutions are distributed optimization algorithms such as dual decomposition and the alternating direction method of multipliers (ADMM). However, these algorithms ignore two practical challenges: substantial communication delays present in control systems and also problem non-convexity.This thesis presents two novel and practically effective DMPC algorithms. The first DMPC algorithm is based on a primal-dual active-set method which achieves fast convergence, making it suitable for large-scale control applications which have a large communication delay across its communication network. In particular, this algorithm is suited for MPC problems with a quadratic cost, linear dynamics, forecasted demand, and box constraints. We measure the performance of this algorithm and show that it significantly outperforms both dual decomposition and ADMM in the presence of communication delay. The second DMPC algorithm is based on an inexact interior point method which is suited for nonlinear optimization problems. The parallel computation of the algorithm exploits iterative linear algebra methods for the main linear algebra computations in the algorithm. We show that the splitting of the algorithm is flexible and can thus be applied to various distributed platform configurations.The two proposed algorithms are applied to two main energy and transportation control problems. The first application is energy efficient building control. Buildings represent 40\% of energy consumption in the United States. Thus, it is significant to improve the energy efficiency of buildings. The goal is to minimize energy consumption subject to the physics of the building (e.g. heat transfer laws), the constraints of the actuators as well as the desired operating constraints (thermal comfort of the occupants), and heat load on the system. In this thesis, we describe the control systems of forced air building systems in practice. We discuss the ``Trim and Respond'' algorithm which is a distributed control algorithm that is used in practice, and show that it performs similarly to a one-step explicit DMPC algorithm. Then, we apply the novel distributed primal-dual active-set method and provide extensive numerical results for the building MPC problem.The second main application is the control of ramp metering signals to optimize traffic flow through a freeway system. This application is particularly important since urban congestion has more than doubled in the past few decades. The ramp metering problem is to maximize freeway throughput subject to freeway dynamics (derived from mass conservation), actuation constraints, freeway capacity constraints, and predicted traffic demand. In this thesis, we develop a hybrid model predictive controller for ramp metering that is guaranteed to be persistently feasible and stable. This contrasts to previous work on MPC for ramp metering where such guarantees are absent. We apply a smoothing method to the hybrid model predictive controller and apply the inexact interior point method to this nonlinear non-convex ramp metering problem.},
 author = {Koehler, Sarah Muraoka},
 file = {/home/matt/Zotero/storage/WWHWLGFN/Koehler - 2016 - Applied Distributed Model Predictive Control for E.pdf;/home/matt/Zotero/storage/FR4T7JSP/4h91r4sg.html},
 language = {en},
 school = {UC Berkeley},
 title = {Applied {{Distributed Model Predictive Control}} for {{Energy Efficient Buildings}} and {{Ramp Metering}}},
 year = {2016}
}

@article{kohler_cellular_2015,
 abstract = {We define cellular non-deterministic automata (CNDA) in the spirit of non-deterministic automata theory. They are different from the well-known stochastic automata. We propose the concept of deterministic superautomata to analyze the dynamical behavior of a CNDA and show especially that a CNDA can be embedded in a deterministic cellular automaton. As an application we discuss a connection between certain partial differential equations and CNDA.},
 author = {Kohler, D. and M{\"u}ller, J. and Wever, U.},
 doi = {10.1016/j.physd.2015.08.001},
 file = {/home/matt/Zotero/storage/N9ZKBIDK/Kohler et al. - 2015 - Cellular non-deterministic automata and partial di.pdf;/home/matt/Zotero/storage/PCELAGZA/S0167278915001487.html},
 issn = {0167-2789},
 journal = {Physica D: Nonlinear Phenomena},
 pages = {1--16},
 title = {Cellular Non-Deterministic Automata and Partial Differential Equations},
 volume = {311-312},
 year = {2015}
}

@inproceedings{koshi_findings_1983,
 author = {Koshi, M. and Iwasaki, M. and Ohkura, I.},
 booktitle = {Proceedings of the 8th {{International Symposium}} on {{Transportation}} and {{Traffic Flow Theory}}},
 pages = {403--426},
 title = {Some Findings and an Overview on Vehicular Flow Characteristics},
 volume = {198},
 year = {1983}
}

@inproceedings{kosiorek_stacked_2019,
 author = {Adam R. Kosiorek and
Sara Sabour and
Yee Whye Teh and
Geoffrey E. Hinton},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KosiorekSTH19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {15486--15496},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Stacked Capsule Autoencoders},
 url = {https://proceedings.neurips.cc/paper/2019/hash/2e0d41e02c5be4668ec1b0730b3346a8-Abstract.html},
 year = {2019}
}

@article{kotaru_geometric_2020,
 abstract = {Abstract             In this paper, we study the quadrotor unmanned aerial vehicle (UAV) attitude control on special orthogonal group (SO(3)) in the presence of unknown disturbances and model uncertainties. L1 adaptive control for UAVs using Euler angles/quaternions is shown to exhibit robustness and precise attitude tracking in the presence of disturbances and uncertainties. However, it is well known that dynamical models and controllers that use Euler angle representations are prone to singularities and typically have smaller regions of attraction while quaternion representations are subject to the unwinding phenomenon. To avoid such complexities, we present a geometric L1 adaptation control law to estimate the uncertainties. A model reference adaptive control approach is implemented, with the attitude errors between the quadrotor model and the reference model defined on the manifold. Control laws for the quadrotor and reference models are developed directly on SO(3) to track the desired trajectory while rejecting the uncertainties. Control Lyapunov function-based analysis is used to show the exponential input-to-state stability of the attitude errors. The proposed L1 adaptive controller is validated using numerical simulations. Preliminary experimental results are shown comparing a geometric proportional-derivative controller to the geometric L1 adaptive controller. Experimental validation of the proposed controller is carried out on an Autel X-star quadrotor.},
 author = {Kotaru, Prasanth and Edmonson, Ryan and Sreenath, Koushil},
 doi = {10.1115/1.4045558},
 file = {/home/matt/Zotero/storage/37JIJP5Z/Kotaru et al. - 2020 - Geometric L1 Adaptive Attitude Control for a Quadr.pdf},
 issn = {0022-0434, 1528-9028},
 journal = {Journal of Dynamic Systems, Measurement, and Control},
 language = {en},
 number = {3},
 pages = {031003},
 title = {Geometric {{L1 Adaptive Attitude Control}} for a {{Quadrotor Unmanned Aerial Vehicle}}},
 volume = {142},
 year = {2020}
}

@article{kotaru_geometric_2020-1,
 author = {Kotaru, Prasanth and Edmonson, Ryan and Sreenath, Koushil},
 journal = {ArXiv preprint},
 title = {Geometric {{L1 Adaptive Attitude Control}} for a {{Quadrotor Unmanned Aerial Vehicle}}},
 url = {https://arxiv.org/abs/1910.07730},
 volume = {abs/1910.07730},
 year = {2019}
}

@article{kotaru_multiple_2019,
 author = {Kotaru, Prasanth and Sreenath, Koushil},
 journal = {ArXiv preprint},
 title = {Multiple Quadrotors Carrying a Flexible Hose: Dynamics, Differential Flatness and Control},
 url = {https://arxiv.org/abs/1911.12650},
 volume = {abs/1911.12650},
 year = {2019}
}

@inproceedings{kotsia_support_2011,
 author = {Irene Kotsia and
Ioannis Patras},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/KotsiaP11.bib},
 booktitle = {The 24th {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2011, Colorado Springs, CO, USA, 20-25 June 2011},
 doi = {10.1109/CVPR.2011.5995663},
 pages = {633--640},
 publisher = {{IEEE} Computer Society},
 timestamp = {Sat, 19 Oct 2019 01:00:00 +0200},
 title = {Support tucker machines},
 url = {https://doi.org/10.1109/CVPR.2011.5995663},
 year = {2011}
}

@article{kotsialos_optimal_1999,
 author = {Kotsialos, A. and Papageorgiou, M. and Messmer, A.},
 journal = {Proceedings of the 14th International Symposium of Transportation and Traffic Theory, Jerusalem},
 pages = {621--644},
 title = {Optimal {{Co}}-Ordinated and {{Integrated Motorway Network Traffic Control}}.},
 year = {1999}
}

@book{koukoumidis_signalguru_2012,
 author = {Koukoumidis, E. and Peh, L.-S. and Martonosi, M.},
 title = {{{SignalGuru}}: {{Leveraging Mobile Phones}} for {{Collaborative Traffic Signal Schedule Advisory}}},
 year = {2012}
}

@article{krajzewicz_recent_2012,
 author = {Krajzewicz, Daniel and Erdmann, Jakob and Behrisch, Michael and Bieker, Laura},
 journal = {International Journal On Advances in Systems and Measurements},
 number = {3\&4},
 pages = {128--138},
 title = {Recent {{Development}} and {{Applications}} of {{SUMO}} - {{Simulation}} of {{Urban MObility}}},
 volume = {5},
 year = {2012}
}

@inproceedings{krauth_finite-time_2019,
 author = {Karl Krauth and
Stephen Tu and
Benjamin Recht},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KrauthTR19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {8512--8522},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Finite-time Analysis of Approximate Policy Iteration for the Linear
Quadratic Regulator},
 url = {https://proceedings.neurips.cc/paper/2019/hash/aaebdb8bb6b0e73f6c3c54a0ab0c6415-Abstract.html},
 year = {2019}
}

@inproceedings{kreidieh_dissipating_2018,
 abstract = {This article demonstrates the ability for model-free reinforcement learning (RL) techniques to generate traffic control strategies for connected and automated vehicles (CAVs) in various network geometries. This method is demonstrated to achieve near complete wave dissipation in a straight open road network with only 10\% CAV penetration, while penetration rates as low as 2.5\% are revealed to contribute greatly to reductions in the frequency and magnitude of formed waves. Moreover, a study of controllers generated in closed network scenarios exhibiting otherwise similar densities and perturbing behaviors confirms that closed network policies generalize to open network tasks, and presents the potential role of transfer learning in fine-tuning the parameters of these policies. Videos of the results are available at: https://sites.google.com/view/itsc-dissipating-waves.},
 author = {Kreidieh, A. R. and Wu, C. and Bayen, A. M.},
 booktitle = {2018 21st {{International Conference}} on {{Intelligent Transportation Systems}} ({{ITSC}})},
 doi = {10.1109/ITSC.2018.8569485},
 file = {/home/matt/Zotero/storage/CU9RXX7G/Kreidieh et al. - 2018 - Dissipating stop-and-go waves in closed and open n.pdf;/home/matt/Zotero/storage/TJ8MHF2I/8569485.html},
 pages = {1475--1480},
 title = {Dissipating Stop-and-Go Waves in Closed and Open Networks via Deep Reinforcement Learning},
 year = {2018}
}

@inproceedings{kreidieh_inter-level_2019,
 abstract = {This article presents a novel algorithm for promoting cooperation between internal actors in a goal-conditioned hierarchical reinforcement learning (HRL) policy. Current techniques for HRL policy optimization treat the higher and lower level policies as separate entities which are trained to maximize different objective functions, rendering the HRL problem formulation more similar to a general sum game than a single-agent task. Within this setting, we hypothesize that improved cooperation between the internal agents of a hierarchy can simplify the credit assignment problem from the perspective of the high-level policies, thereby leading to significant improvements to training in situations where intricate sets of action primitives must be performed to yield improvements in performance. In order to promote cooperation within this setting, we propose the inclusion of a connected gradient term to the gradient computations of the higher level policies1. Our method is demonstrated to achieve superior results to existing techniques in a set of difficult long time horizon tasks.},
 archiveprefix = {arXiv},
 author = {Kreidieh, Abdul Rahman and Parajuli, Samyak and Lichtle, Nathan and You, Yiling and Nasr, Rayyan and Bayen, Alexandre M.},
 booktitle = {Submitted to {{International Conference}} on {{Autonomous Agents}} and {{Multiagent Systems}} ({{AAMAS}} 2020)},
 eprint = {1912.02368},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/M4FD55BS/Kreidieh et al. - 2019 - Inter-Level Cooperation in Hierarchical Reinforcem.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Inter-{{Level Cooperation}} in {{Hierarchical Reinforcement Learning}}},
 year = {2019}
}

@inproceedings{krizhevsky_imagenet_2012,
 author = {Alex Krizhevsky and
Ilya Sutskever and
Geoffrey E. Hinton},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KrizhevskySH12.bib},
 booktitle = {Advances in Neural Information Processing Systems 25: 26th Annual
Conference on Neural Information Processing Systems 2012. Proceedings
of a meeting held December 3-6, 2012, Lake Tahoe, Nevada, United States},
 editor = {Peter L. Bartlett and
Fernando C. N. Pereira and
Christopher J. C. Burges and
L{\'{e}}on Bottou and
Kilian Q. Weinberger},
 pages = {1106--1114},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {ImageNet Classification with Deep Convolutional Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2012/hash/c399862d3b9d6b76c8436e924a68c45b-Abstract.html},
 year = {2012}
}

@inproceedings{kudo_subword_2018,
 address = {Melbourne, Australia},
 author = {Kudo, Taku},
 booktitle = {Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
 doi = {10.18653/v1/P18-1007},
 pages = {66--75},
 publisher = {Association for Computational Linguistics},
 title = {Subword Regularization: Improving Neural Network Translation Models with Multiple Subword Candidates},
 url = {https://aclanthology.org/P18-1007},
 year = {2018}
}

@inproceedings{kumar_discor_2020,
 author = {Aviral Kumar and
Abhishek Gupta and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/Kumar0L20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {DisCor: Corrective Feedback in Reinforcement Learning via Distribution
Correction},
 url = {https://proceedings.neurips.cc/paper/2020/hash/d7f426ccbc6db7e235c57958c21c5dfa-Abstract.html},
 year = {2020}
}

@inproceedings{kumar_model_2019,
 author = {Aviral Kumar and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KumarL20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Model Inversion Networks for Model-Based Optimization},
 url = {https://proceedings.neurips.cc/paper/2020/hash/373e4c5d8edfa8b74fd4b6791d0cf6dc-Abstract.html},
 year = {2020}
}

@article{kumar_reward-conditioned_2019,
 author = {Kumar, Aviral and Peng, Xue Bin and Levine, Sergey},
 journal = {ArXiv preprint},
 title = {Reward-{{Conditioned Policies}}},
 url = {https://arxiv.org/abs/1912.13465},
 volume = {abs/1912.13465},
 year = {2019}
}

@inproceedings{kumar_stabilizing_2019,
 author = {Aviral Kumar and
Justin Fu and
Matthew Soh and
George Tucker and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/KumarFSTL19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {11761--11771},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Stabilizing Off-Policy Q-Learning via Bootstrapping Error Reduction},
 url = {https://proceedings.neurips.cc/paper/2019/hash/c2073ffa77b5357a498057413bb09d3a-Abstract.html},
 year = {2019}
}

@article{kuo_expert-level_2019,
 abstract = {Computed tomography (CT) of the head is used worldwide to diagnose neurologic emergencies. However, expertise is required to interpret these scans, and even highly trained experts may miss subtle life-threatening findings. For head CT, a unique challenge is to identify, with perfect or near-perfect sensitivity and very high specificity, often small subtle abnormalities on a multislice cross-sectional (three-dimensional [3D]) imaging modality that is characterized by poor soft tissue contrast, low signal-to-noise using current low radiation-dose protocols, and a high incidence of artifacts. We trained a fully convolutional neural network with 4,396 head CT scans performed at the University of California at San Francisco and affiliated hospitals and compared the algorithm's performance to that of 4 American Board of Radiology (ABR) certified radiologists on an independent test set of 200 randomly selected head CT scans. Our algorithm demonstrated the highest accuracy to date for this clinical application, with a receiver operating characteristic (ROC) area under the curve (AUC) of 0.991 {$\pm$} 0.006 for identification of examinations positive for acute intracranial hemorrhage, and also exceeded the performance of 2 of 4 radiologists. We demonstrate an end-to-end network that performs joint classification and segmentation with examination-level classification comparable to experts, in addition to robust localization of abnormalities, including some that are missed by radiologists, both of which are critically important elements for this application.},
 author = {Kuo, Weicheng and H{\"{\cyrchar\cyra}}ne, Christian and Mukherjee, Pratik and Malik, Jitendra and Yuh, Esther L.},
 doi = {10.1073/pnas.1908021116},
 file = {/home/matt/Zotero/storage/RKHHBD3M/Kuo et al. - 2019 - Expert-level detection of acute intracranial hemor.pdf},
 issn = {0027-8424, 1091-6490},
 journal = {Proceedings of the National Academy of Sciences},
 language = {en},
 number = {45},
 pages = {22737--22745},
 title = {Expert-Level Detection of Acute Intracranial Hemorrhage on Head Computed Tomography Using Deep Learning},
 volume = {116},
 year = {2019}
}

@article{kurant_layered_2006,
 abstract = {Many complex networks are only a part of larger systems, where a number of coexisting topologies interact and depend on each other. We introduce a layered model to facilitate the description and analysis of such systems. As an example of its application, we study the load distribution in three transportation systems, where the lower layer is the physical infrastructure and the upper layer represents the traffic flows. This layered view allows us to capture the fundamental differences between the real load and commonly used load estimators, which explains why these estimators fail to approximate the real load.},
 author = {Kurant, Maciej and Thiran, Patrick},
 doi = {10.1103/PhysRevLett.96.138701},
 file = {/home/matt/Zotero/storage/N4CHCB5U/Kurant and Thiran - 2006 - Layered Complex Networks.pdf;/home/matt/Zotero/storage/BFQXST4B/PhysRevLett.96.html},
 journal = {Physical Review Letters},
 number = {13},
 pages = {138701},
 title = {Layered {{Complex Networks}}},
 volume = {96},
 year = {2006}
}

@article{kurzhanskiy_active_2010,
 author = {Kurzhanskiy, A. A. and Varaiya, P.},
 journal = {Phil. Trans. R. Soc. A},
 pages = {4607--4626},
 title = {Active Traffic Management on Road Networks: A Macroscopic Approach},
 volume = {368},
 year = {2010}
}

@article{kurzhanskiy_guaranteed_2012,
 author = {Kurzhanskiy, A. A. and Varaiya, P.},
 journal = {Transportation Research, Part C},
 pages = {163--180},
 title = {Guaranteed Prediction and Estimation of the State of a Road Network},
 volume = {21},
 year = {2012}
}

@article{kurzhanskiy_traffic_2015,
 author = {Kurzhanskiy, Alex A. and Varaiya, Pravin},
 doi = {10.1016/j.ecotra.2015.03.002},
 file = {/home/matt/Documents/Papers/HOV-HOT/kurvaraiyaeconomics.pdf},
 issn = {22120122},
 journal = {Economics of Transportation},
 language = {en},
 number = {3},
 pages = {135--146},
 shorttitle = {Traffic Management},
 title = {Traffic Management: {{An}} Outlook},
 volume = {4},
 year = {2015}
}

@article{kwon_components_2006,
 author = {Kwon, J. and Mauch, M. and Varaiya, P.},
 journal = {Transportation Research Record},
 pages = {84--91},
 title = {Components of Congestion: {{Delay}} from Incidents, Special Events, Lane Closures, Weather, Potential Ramp Metering Gain, and Excess Demand},
 volume = {1959},
 year = {2006}
}

@article{kwon_effectiveness_2008,
 author = {Kwon, Jaimyoung and Varaiya, Pravin},
 doi = {10.1016/j.trc.2007.06.008},
 file = {/home/matt/Zotero/storage/XKAE3ZXS/2007_TRC_effectiveness_HOV_lane.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 number = {1},
 pages = {98--115},
 title = {Effectiveness of {{California}}'s {{High Occupancy Vehicle}} ({{HOV}}) System},
 volume = {16},
 year = {2008}
}

@book{kwon_j._bottleneck_2004,
 author = {{Kwon, J.}},
 title = {Bottleneck {{Analysis}} and {{Delay Causality Study}}: {{Draft Final Report}}},
 year = {2004}
}

@article{kwon_j._estimation_2003,
 author = {{Kwon, J.} and Varaiya, P. and Skabardonis, A.},
 journal = {Transportation Research Record},
 pages = {106--117},
 title = {Estimation of Truck Traffic Volume from Single Loop Detectors with Lane-to-Lane Speed Correlation},
 volume = {1856},
 year = {2003}
}

@article{kwon_j._statistical_2005,
 author = {{Kwon, J.} and Chen, C. and Varaiya, P.},
 journal = {Transportation Research Record},
 pages = {124--132},
 title = {Statistical Methods for Detecting Spatial Configuration Errors in Traffic Surveillance},
 volume = {1870},
 year = {2005}
}

@article{kwon_joint_2003,
 author = {Kwon, J.},
 journal = {82nd Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {Joint Estimation of the Traffic Speed and Mean Vehicle Length from Single-Loop Detector Data.},
 year = {2003}
}

@article{kwon_probe_2007,
 author = {Kwon, J. and Petty, K. and Varaiya, P.},
 journal = {Transportation Research Record},
 pages = {57--63},
 title = {Probe {{Vehicle Runs}} or {{Loop Detectors}}?},
 volume = {2012},
 year = {2007}
}

@unpublished{kwon_quality_2002,
 author = {Kwon, J.},
 title = {{{QUALITY OF DOUBLE LOOP DATA FROM SAN FRANCISCO BAY AREA}}},
 year = {2002}
}

@article{kwon_real-time_2005,
 author = {Kwon, J. and Varaiya, P.},
 journal = {84th Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {Real-Time Estimation of Origin-Destination Matrices with Partial Trajectories from Electronic Toll Connection Tag Data},
 year = {2005}
}

@article{kwong_arterial_2009,
 author = {Kwong, K. and Kavaler, R. and Rajagopal, R. and Varaiya, P.},
 journal = {Transportation Research, Part C},
 number = {6},
 pages = {586--606},
 title = {Arterial Travel Time Estimation Based on Vehicle Re-Identification Using Wireless Sensors},
 volume = {17},
 year = {2009}
}

@article{kwong_practical_2009,
 author = {Kwong, K. and Kavaler, R. and Rajagopal, R. and Varaiya, P.},
 journal = {88th Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {A Practical Scheme for Arterial Travel Time Estimation Based on Vehicle Re-Identification Using Wireless Sensors},
 year = {2009}
}

@article{kwong_real-time_2009,
 author = {Kwong, K. and Kavaler, R. and Rajagopal, R. and Varaiya, P.},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 title = {Real-Time Measurement of Link Vehicle Count and Travel Time in a Road Network},
 year = {2009}
}

@article{lago_spillovers_2007,
 author = {Lago, A. and Daganzo, C. F.},
 journal = {Transportation Research, Part B},
 pages = {670--683},
 title = {Spillovers, Merging Traffic and the Morning Commute},
 volume = {41},
 year = {2007}
}

@article{lakshmanan_broader_2011,
 abstract = {A major question in Economic Geography relates to the scale and nature of transport infrastructure's contribution to the broader economy. While Cost-Benefit Analysis (CBA) is the most widely used of the three potential approaches, the recent interest in the wider economic benefits of transport infrastructure has spawned a variety of macroeconomic models. However, the estimates of magnitudes and direction of economic impacts of infrastructure by various macroeconomic models are sharply different, and these models shed little light on causal mechanisms linking transport and the economy. This paper has two aims: first, to highlight the wider economic benefits of transport infrastructure from the observed role of railroads and waterways in economic development, and two by reviewing recent theoretical developments to identify the multiple causal mechanisms which link transport and economic growth such as : market expansion, gains from trade, technological shifts, processes of spatial agglomeration and processes of innovation and commercialization of new knowledge in urban clusters (made possible by transport improvements). Hence the need for developing general equilibrium analyses of transport-economy linkages.},
 author = {Lakshmanan, T. R.},
 doi = {10.1016/j.jtrangeo.2010.01.001},
 file = {/home/matt/Zotero/storage/P6KZUFET/Lakshmanan - 2011 - The broader economic consequences of transport inf.pdf;/home/matt/Zotero/storage/GDJWPGI2/S0966692310000037.html},
 issn = {0966-6923},
 journal = {Journal of Transport Geography},
 number = {1},
 pages = {1--12},
 title = {The Broader Economic Consequences of Transport Infrastructure Investments},
 volume = {19},
 year = {2011}
}

@article{lambert_low-level_2019,
 author = {Lambert, Nathan O. and Drew, Daniel S. and Yaconelli, Joseph and Levine, Sergey and Calandra, Roberto and Pister, Kristofer S. J.},
 doi = {10.1109/LRA.2019.2930489},
 file = {/home/matt/Zotero/storage/ESWCP7GI/Lambert et al. - 2019 - Low-Level Control of a Quadrotor With Deep Model-B.pdf},
 issn = {2377-3766, 2377-3774},
 journal = {IEEE Robotics and Automation Letters},
 number = {4},
 pages = {4224--4230},
 title = {Low-{{Level Control}} of a {{Quadrotor With Deep Model}}-{{Based Reinforcement Learning}}},
 volume = {4},
 year = {2019}
}

@inproceedings{lambert_objective_2020,
 abstract = {Model-based reinforcement learning (MBRL) has been shown to be a powerful framework for data-efficiently learning control of continuous tasks. Recent work in MBRL has mostly focused on using more advanced function approximators and planning schemes, with little development of the general framework. In this paper, we identify a fundamental issue of the standard MBRL framework -- what we call the objective mismatch issue. Objective mismatch arises when one objective is optimized in the hope that a second, often uncorrelated, metric will also be optimized. In the context of MBRL, we characterize the objective mismatch between training the forward dynamics model w.r.t.\textasciitilde the likelihood of the one-step ahead prediction, and the overall goal of improving performance on a downstream control task. For example, this issue can emerge with the realization that dynamics models effective for a specific task do not necessarily need to be globally accurate, and vice versa globally accurate models might not be sufficiently accurate locally to obtain good control performance on a specific task. In our experiments, we study this objective mismatch issue and demonstrate that the likelihood of one-step ahead predictions is not always correlated with control performance. This observation highlights a critical limitation in the MBRL framework which will require further research to be fully understood and addressed. We propose an initial method to mitigate the mismatch issue by re-weighting dynamics model training. Building on it, we conclude with a discussion about other potential directions of research for addressing this issue.},
 archiveprefix = {arXiv},
 author = {Lambert, Nathan and Amos, Brandon and Yadan, Omry and Calandra, Roberto},
 booktitle = {Proceedings of the 2nd {{Conference}} on {{Learning}} for {{Dynamics}} and {{Control}}},
 eprint = {2002.04523},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/HVJ7V9CK/Lambert et al. - 2021 - Objective Mismatch in Model-based Reinforcement Le.pdf;/home/matt/Zotero/storage/SQB8VTTZ/2002.html},
 pages = {761--770},
 publisher = {{PMLR}},
 title = {Objective {{Mismatch}} in {{Model}}-Based {{Reinforcement Learning}}},
 volume = {120},
 year = {2020}
}

@inproceedings{lan_albert_2020,
 author = {Zhenzhong Lan and
Mingda Chen and
Sebastian Goodman and
Kevin Gimpel and
Piyush Sharma and
Radu Soricut},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LanCGGSS20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {{ALBERT:} {A} Lite {BERT} for Self-supervised Learning of Language
Representations},
 url = {https://openreview.net/forum?id=H1eA7AEtvS},
 year = {2020}
}

@inproceedings{landi_prediction_2019,
 abstract = {The raise of collaborative robotics has allowed to create new spaces where robots and humans work in proximity. Consequently, to predict human movements and his/her final intention becomes crucial to anticipate robot next move, preserving safety and increasing efficiency. In this paper we propose a human-arm prediction algorithm that allows to infer if the human operator is moving towards the robot to intentionally interact with it. The human hand position is tracked by an RGB-D camera online. By combining the Minimum Jerk model with Semi-Adaptable Neural Networks we obtain a reliable prediction of the human hand trajectory and final target in a short amount of time. The proposed algorithm was tested in a multi-movements scenario with FANUC LR Mate 200iD/7L industrial robot.},
 address = {{Macau, China}},
 author = {Landi, Chiara Talignani and Cheng, Yujiao and Ferraguti, Federica and Bonfe, Marcello and Secchi, Cristian and Tomizuka, Masayoshi},
 booktitle = {2019 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}} ({{IROS}})},
 doi = {10.1109/IROS40897.2019.8968559},
 file = {/home/matt/Zotero/storage/3G6JX7IS/Landi et al. - 2019 - Prediction of Human Arm Target for Robot Reaching .pdf},
 isbn = {978-1-72814-004-9},
 language = {en},
 pages = {5950--5957},
 publisher = {{IEEE}},
 title = {Prediction of {{Human Arm Target}} for {{Robot Reaching Movements}}},
 year = {2019}
}

@inproceedings{laptev_time-series_2017,
 abstract = {Accurate time-series forecasting during high variance segments (e.g., holidays), is critical for anomaly detection, optimal resource allocation, budget planning and other related tasks. At Uber accurate prediction for completed trips during special events can lead to a more efficient driver allocation resulting in a decreased wait time for the riders.},
 author = {Laptev, Nikolay and Yosinski, Jason and Li, Li Erran and Smyl, Slawek},
 booktitle = {International {{Conference}} on {{Machine Learning}}},
 file = {/home/matt/Zotero/storage/GUME8Y5F/Laptev et al. - Time-series Extreme Event Forecasting with Neural .pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {5},
 title = {Time-Series {{Extreme Event Forecasting}} with {{Neural Networks}} at {{Uber}}},
 volume = {37},
 year = {2017}
}

@phdthesis{laskey_and_2018,
 abstract = {As an alternative to explicit programming for robots, Deep Imitation learning has two drawbacks: sample complexity and covariate shift. One approach to Imitation Learning is Behavior Cloning, in which arobot observes a supervisor and then infers a control policy. A known problem with this approach is that even slight departures from the supervisor's demonstrations can compound over the policy's roll-out resulting in errors; this concept of drift and resulting error is commonly referred to as covariate shift On-policy techniques reduce covariate shift by iteratively collecting corrective actions for the current robot policy. To reduce sample complexity of these approaches, we propose a novel active learning algorithm, SHIV (Svm-based reduction in Human InterVention). While evaluating SHIV, we reconsider the trade-off between Off- and On-Policy methods and find that: 1) On-Policy methods are challenging for humans supervisors and 2) performance varies with the expressiveness of the policy class. To make Off-Policy methods more robust for expressive policies we propose a second algorithm, DART (Disturbances Augmenting Robot Trajectories), which injects optimized noise into the supervisor's control stream to simulate error during data collection. This dissertation contributes two aforementioned algorithms, experimental evaluation with three robots evaluating their performance on tasks ranging from grasping in clutter to singulation to bed-making, and the design of a novel first-order urban driving simulator (FLUIDS) that can fill gaps in existing benchmarks for Imitation Learning to rapidly test algorithm performance in terms of generalization.},
 author = {Laskey, Michael David},
 file = {/home/matt/Zotero/storage/4BGMYZZZ/Laskey - 2018 - On and Off-Policy Deep Imitation Learning for Robo.pdf;/home/matt/Zotero/storage/7255LNLK/5rn6n8nb.html},
 language = {en},
 school = {UC Berkeley},
 title = {On and {{Off}}-{{Policy Deep Imitation Learning}} for {{Robotics}}},
 year = {2018}
}

@inproceedings{laskin_reinforcement_2020,
 author = {Michael Laskin and
Kimin Lee and
Adam Stooke and
Lerrel Pinto and
Pieter Abbeel and
Aravind Srinivas},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LaskinLSPAS20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Reinforcement Learning with Augmented Data},
 url = {https://proceedings.neurips.cc/paper/2020/hash/e615c82aba461681ade82da2da38004a-Abstract.html},
 year = {2020}
}

@inproceedings{laskin_sparse_2020,
 author = {Scott Emmons and
Ajay Jain and
Michael Laskin and
Thanard Kurutach and
Pieter Abbeel and
Deepak Pathak},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/EmmonsJLKAP20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Sparse Graphical Memory for Robust Planning},
 url = {https://proceedings.neurips.cc/paper/2020/hash/385822e359afa26d52b5b286226f2cea-Abstract.html},
 year = {2020}
}

@inproceedings{laskin_sparse_2020-1,
 author = {Scott Emmons and
Ajay Jain and
Michael Laskin and
Thanard Kurutach and
Pieter Abbeel and
Deepak Pathak},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/EmmonsJLKAP20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Sparse Graphical Memory for Robust Planning},
 url = {https://proceedings.neurips.cc/paper/2020/hash/385822e359afa26d52b5b286226f2cea-Abstract.html},
 year = {2020}
}

@article{lawler_procedure_1972,
 author = {Lawler, E.},
 journal = {Management Science},
 number = {7},
 pages = {401--405},
 title = {A {{Procedure}} for {{Computing}} the \textbackslash em {{K Best}} Solutions to {{Discrete Optimization Problems}} and {{Its Application}} to the {{Shortest Path Problem}}},
 volume = {18},
 year = {1972}
}

@inproceedings{lazaridou_multi-agent_2017,
 author = {Angeliki Lazaridou and
Alexander Peysakhovich and
Marco Baroni},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LazaridouPB17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 04 Apr 2019 01:00:00 +0200},
 title = {Multi-Agent Cooperation and the Emergence of (Natural) Language},
 url = {https://openreview.net/forum?id=Hk8N3Sclg},
 year = {2017}
}

@inproceedings{lazebnik_beyond_2006,
 abstract = {This paper presents a method for recognizing scene categories based on approximate global geometric correspondence. This technique works by partitioning the image into increasingly fine sub-regions and computing histograms of local features found inside each sub-region. The resulting ``spatial pyramid'' is a simple and computationally efficient extension of an orderless bag-of-features image representation, and it shows significantly improved performance on challenging scene categorization tasks. Specifically, our proposed method exceeds the state of the art on the Caltech-101 database and achieves high accuracy on a large database of fifteen natural scene categories. The spatial pyramid framework also offers insights into the success of several recently proposed image descriptions, including Torralba's ``gist'' and Lowe's SIFT descriptors.},
 address = {{New York, NY, USA}},
 author = {Lazebnik, S. and Schmid, C. and Ponce, J.},
 booktitle = {2006 {{IEEE Computer Society Conference}} on {{Computer Vision}} and {{Pattern Recognition}} - {{Volume}} 2 ({{CVPR}}'06)},
 doi = {10.1109/CVPR.2006.68},
 file = {/home/matt/Zotero/storage/PZAQSR3E/Lazebnik et al. - 2006 - Beyond Bags of Features Spatial Pyramid Matching .pdf},
 isbn = {978-0-7695-2597-6},
 language = {en},
 pages = {2169--2178},
 publisher = {{IEEE}},
 shorttitle = {Beyond {{Bags}} of {{Features}}},
 title = {Beyond {{Bags}} of {{Features}}: {{Spatial Pyramid Matching}} for {{Recognizing Natural Scene Categories}}},
 volume = {2},
 year = {2006}
}

@article{lebacque_awrascle_2007,
 author = {Lebacque, Jean-Patrick and Mammar, Salim and {Haj-Salem}, Habib},
 doi = {10.1016/j.trb.2006.11.005},
 file = {/home/matt/Documents/Papers/lebacque_2o_riemann_2007.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {7},
 pages = {710--721},
 shorttitle = {The {{Aw}}\textendash{{Rascle}} and {{Zhang}}'s Model},
 title = {The {{Aw}}\textendash{{Rascle}} and {{Zhang}}'s Model: {{Vacuum}} Problems, Existence and Regularity of the Solutions of the {{Riemann}} Problem},
 volume = {41},
 year = {2007}
}

@inproceedings{lebacque_first-order_2005,
 author = {Lebacque, Jean-Patrick. and Khoshyaran, M.M.},
 booktitle = {The 16th {{International Symposium}} on {{Transportation}} and {{Traffic Theory}} ({{ISTTT}})},
 pages = {365--386},
 title = {First-Order Macroscopic Traffic Flow Models: Intersection Modeling, Network Modeling},
 year = {2005}
}

@inproceedings{lebacque_generic_2007,
 author = {Lebacque, Jean-Patrick and Mammar, Salim and {Haj-Salem}, Habib},
 booktitle = {Proceedings of the 2007 {{Symposium}} on {{Transportation}} and {{Traffic Theory}}},
 file = {/home/matt/Zotero/storage/VRHWI6I2/lebacque_genericsecondorder.pdf},
 keywords = {⛔ No DOI found},
 pages = {755--776},
 title = {Generic Second Order Traffic Flow Modelling},
 year = {2007}
}

@article{leclercq_calibration_2005,
 author = {Leclercq, L.},
 journal = {Transportation Research Record},
 pages = {226--234},
 title = {Calibration of {{Flow}}{{Density Relationships}} on {{Urban Streets}}},
 volume = {1934},
 year = {2005}
}

@inproceedings{leclercq_lagrangian_2007,
 author = {Leclercq, Ludovic and Laval, Jorge and Chevallier, Estelle},
 booktitle = {Proceedings of the 17th {{International Symposium}} on {{Transportation}} and {{Traffic Theory}}},
 file = {/home/matt/Zotero/storage/QHPUR763/LeclerqLaval_Lagrangian.pdf},
 pages = {735--753},
 publisher = {{Elsevier}},
 title = {The {{Lagrangian}} Coordinates and What It Means for First Order Traffic Flow Models},
 year = {2007}
}

@inproceedings{lecun_deep_2015,
 author = {Ruslan Salakhutdinov},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/kdd/Salakhutdinov14.bib},
 booktitle = {The 20th {ACM} {SIGKDD} International Conference on Knowledge Discovery
and Data Mining, {KDD} '14, New York, NY, {USA} - August 24 - 27,
2014},
 doi = {10.1145/2623330.2630809},
 editor = {Sofus A. Macskassy and
Claudia Perlich and
Jure Leskovec and
Wei Wang and
Rayid Ghani},
 pages = {1973},
 publisher = {{ACM}},
 timestamp = {Tue, 06 Nov 2018 00:00:00 +0100},
 title = {Deep learning},
 url = {https://doi.org/10.1145/2623330.2630809},
 year = {2014}
}

@article{lecun_gradient-based_1998,
 abstract = {Multilayer neural networks trained with the back-propagation algorithm constitute the best example of a successful gradient based learning technique. Given an appropriate network architecture, gradient-based learning algorithms can be used to synthesize a complex decision surface that can classify high-dimensional patterns, such as handwritten characters, with minimal preprocessing. This paper reviews various methods applied to handwritten character recognition and compares them on a standard handwritten digit recognition task. Convolutional neural networks, which are specifically designed to deal with the variability of 2D shapes, are shown to outperform all other techniques. Real-life document recognition systems are composed of multiple modules including field extraction, segmentation recognition, and language modeling. A new learning paradigm, called graph transformer networks (GTN), allows such multimodule systems to be trained globally using gradient-based methods so as to minimize an overall performance measure. Two systems for online handwriting recognition are described. Experiments demonstrate the advantage of global training, and the flexibility of graph transformer networks. A graph transformer network for reading a bank cheque is also described. It uses convolutional neural network character recognizers combined with global training techniques to provide record accuracy on business and personal cheques. It is deployed commercially and reads several million cheques per day.},
 author = {LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
 doi = {10.1109/5.726791},
 file = {/home/matt/Zotero/storage/QPCSJ96N/Lecun et al. - 1998 - Gradient-based learning applied to document recogn.pdf;/home/matt/Zotero/storage/XFRAZFEI/726791.html},
 issn = {0018-9219, 1558-2256},
 journal = {Proceedings of the IEEE},
 number = {11},
 pages = {2278--2324},
 title = {Gradient-Based Learning Applied to Document Recognition},
 volume = {86},
 year = {1998}
}

@inproceedings{lecun_handwritten_1990,
 abstract = {We present an application of back-propagation networks to handwritten digit recognition. Minimal preprocessing of the data was required, but architecture of the network was highly constrained and specifically designed for the task. The input of the network consists of normalized images of isolated digits. The method has 1\% error rate and about a 9\% reject rate on zipcode digits provided by the U.S. Postal Service.},
 author = {LeCun, Yann and Boser, Bernhard E and Denker, John S and Henderson, Donnie and Howard, R E and Hubbard, Wayne E and Jackel, Lawrence D},
 booktitle = {Advances in {{Neural Information Processing Systems}}},
 file = {/home/matt/Zotero/storage/NASKF6KZ/LeCun et al. - Handwritten Digit Recognition with a Back-Propagat.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {396--404},
 title = {Handwritten {{Digit Recognition}} with a {{Back}}-{{Propagation Network}}},
 year = {1990}
}

@inproceedings{lee_continuous_2019,
 abstract = {Online learning is a powerful tool for analyzing iterative algorithms. However, the classic adversarial setup sometimes fails to capture certain regularity in online problems in practice. Motivated by this, we establish a new setup, called Continuous Online Learning (COL), where the gradient of online loss function changes continuously across rounds with respect to the learner's decisions. We show that COL covers and more appropriately describes many interesting applications, from general equilibrium problems (EPs) to optimization in episodic MDPs. Using this new setup, we revisit the difficulty of achieving sublinear dynamic regret. We prove that there is a fundamental equivalence between achieving sublinear dynamic regret in COL and solving certain EPs, and we present a reduction from dynamic regret to both static regret and convergence rate of the associated EP. At the end, we specialize these new insights into online imitation learning and show improved understanding of its learning stability.},
 archiveprefix = {arXiv},
 author = {Lee, Jonathan and Cheng, Ching-An and Goldberg, Ken and Boots, Byron},
 booktitle = {Optimization {{Foundations}} for {{Reinforcement Learning Workshop}} at {{NeurIPS}} 2019},
 eprint = {1912.01261},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/9G8VD8G8/Lee et al. - 2019 - Continuous Online Learning and New Insights to Onl.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Continuous {{Online Learning}} and {{New Insights}} to {{Online Imitation Learning}}},
 year = {2019}
}

@phdthesis{lee_increased_2018,
 abstract = {In this thesis leg spines have been used in a variety of systems including traction for horizontal running, and a gripping mechanism for jumping on inclines. These spines were inspired by collapsible leg spines found on insects and spiders that provide a passive mechanism for increased traction while running over complex terrain. I used this architectural advantage as biological inspiration to increase the traction with a VelociRoACH, a high speed terrestrial robot. These spines exhibited anisotropic properties in the fore-aft and lateral directions, with a 2:1 holding-to-release force ratio on corkboard (0.2 N to 0.1 N). This increase in effective friction coefficient at the foot-to-surface contact points increased the running speed on flat ground and 20 degrees inclines and the maximum incline the robot can traverse by 10 degrees. The VelociRoACH with spines is able to engage the surface and pull up to 0.36 N whereas without spines it slips while pulling 0.2 N, increasing the useful work in pulling a load. The spines also allow the robot to remain dynamically stable and resist torque disturbances.After preliminary experiments using bio-inspired spines on the VelociRoACH, the various structures insects use to enhance interaction with the substrate during jumping were examined. The effectiveness of spines at the base of cricket tibia and attachment pads on tarsi were tested in providing traction on various surfaces by measuring jump kinetic energy using high-speed video. Both substrate and attachment structure significantly affected jump kinetic energy, but most significantly spines increased jumping performance by 82\% on Styrofoam. Inspired by crickets, similar experiments were performed on a 2.5g jumping robot for more controlled tests. The addition of spines increased jump kinetic energy on Styrofoam by 65\%, and doubled its jump distance to 40cm. Adding rubber attachment pads allowed the robot to jump on Teflon, increasing the kinetic energy from 0 to 7.8mJ. Leg spines appear critical for maximum jumping performance on surfaces that allow penetration and attachment pads can increase performance on smooth surfaces. Lastly, spines were used in a gripper mechanism for the monopedal jumping robot, Salto, to reduce slip and provide adhesion capabilities. The mechanism pushes in angled spines along their length and is kinematically constrained to engage/disengage with leg crouch/extension. The resulting gripper introduces no new actuators, enables jumping on penetrable inclines up to 60 degrees, as opposed to a rubber ball foot that works up to 20 degrees, and enables static adhesion to hold 7.5 times the robot's weight from a ceiling.Overall leg and foot spines have been shown to be an effective means of increasing performance in traction and jumping without requiring additional actuators, degrees of freedom, batteries or control. This is especially useful for small robots that have limited real estate and weight constraints. However, using spines as a passive mechanical solution for traction can be used in larger robots and other applications as well.},
 author = {Lee, Jessica Stephanie},
 file = {/home/matt/Zotero/storage/62RPB77Z/Lee - 2018 - Increased Millirobot Traction in Running and Jumpi.pdf;/home/matt/Zotero/storage/2SGYAQ8K/5n60q91v.html},
 language = {en},
 school = {UC Berkeley},
 title = {Increased {{Millirobot Traction}} in {{Running}} and {{Jumping}} through {{Leg Spines}}},
 year = {2018}
}

@book{lee_introduction_2017,
 address = {{Cambridge, Massachusetts}},
 author = {Lee, Edward A. and Seshia, Sanjit A.},
 edition = {Second edition},
 file = {/home/matt/Zotero/storage/DAFCDNIW/Lee and Seshia - 2017 - Introduction to embedded systems a cyber-physical.pdf},
 isbn = {978-0-262-53381-2},
 language = {en},
 lccn = {TK7895.E42 L445 2017},
 publisher = {{MIT Press}},
 shorttitle = {Introduction to Embedded Systems},
 title = {Introduction to Embedded Systems: A Cyber-Physical Systems Approach},
 year = {2017}
}

@article{lee_macroscopic_2001,
 author = {Lee, H. K. and Lee, H.-W. and Kim, D.},
 file = {/home/matt/Zotero/storage/SVNKRJ87/lee_macro_from_micro.pdf},
 journal = {Physical Review E},
 number = {5},
 pages = {056126},
 title = {Macroscopic Traffic Models from Microscopic Car-Following Models},
 volume = {64},
 year = {2001}
}

@article{lee_real-time_2015,
 abstract = {In this study, we develop a real-time estimation approach for lane-based queue lengths. Our aim is to determine the numbers of queued vehicles in each lane, based on detector information at isolated signalized junctions. The challenges involved in this task are to identify whether there is a residual queue at the start time of each cycle and to determine the proportions of lane-to-lane traffic volumes in each lane. Discriminant models are developed based on time occupancy rates and impulse memories, as calculated by the detector and signal information from a set of upstream and downstream detectors. To determine the proportions of total traffic volume in each lane, the downstream arrivals for each cycle are estimated by using the Kalman filter, which is based on upstream arrivals and downstream discharges collected during the previous cycle. Both the computer simulations and the case study of real-world traffic show that the proposed method is robust and accurate for the estimation of lane-based queue lengths in real time under a wide range of traffic conditions. Calibrated discriminant models play a significant role in determining whether there are residual queued vehicles in each lane at the start time of each cycle. In addition, downstream arrivals estimated by the Kalman filter enhance the accuracy of the estimates by minimizing any error terms caused by lane-changing behavior.},
 author = {Lee, Seunghyeon and Wong, S.C. and Li, Y.C.},
 doi = {10.1016/j.trc.2015.03.019},
 file = {/home/matt/Zotero/storage/RD8PQER9/Lee et al. - 2015 - Real-time estimation of lane-based queue lengths a.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {1--17},
 title = {Real-Time Estimation of Lane-Based Queue Lengths at Isolated Signalized Junctions},
 volume = {56},
 year = {2015}
}

@inproceedings{lee_self-attention_2019,
 author = {Junhyun Lee and
Inyeop Lee and
Jaewoo Kang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/LeeLK19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {3734--3743},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Self-Attention Graph Pooling},
 url = {http://proceedings.mlr.press/v97/lee19c.html},
 volume = {97},
 year = {2019}
}

@inproceedings{lee_stochastic_2019,
 author = {Alex X. Lee and
Anusha Nagabandi and
Pieter Abbeel and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LeeNAL20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Stochastic Latent Actor-Critic: Deep Reinforcement Learning with a
Latent Variable Model},
 url = {https://proceedings.neurips.cc/paper/2020/hash/08058bf500242562c0d031ff830ad094-Abstract.html},
 year = {2020}
}

@inproceedings{lee_stochastic_2020,
 author = {Alex X. Lee and
Anusha Nagabandi and
Pieter Abbeel and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LeeNAL20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Stochastic Latent Actor-Critic: Deep Reinforcement Learning with a
Latent Variable Model},
 url = {https://proceedings.neurips.cc/paper/2020/hash/08058bf500242562c0d031ff830ad094-Abstract.html},
 year = {2020}
}

@book{legislative_analysts_office_hov_2000,
 author = {{Legislative Analyst's Office}},
 title = {{{HOV}} Lanes in {{California}}: {{Are}} They Acheiving Their Goals?},
 year = {2000}
}

@article{legrain_am_2015,
 abstract = {The stress of commuting has serious public health and social implications. By comparing stress across different modes it is possible to determine which modes are more heavily contributing to this potential health and social issue. This study uses a large-scale university travel survey to compare commuter stress across three modes of transportation (walking, driving, and using public transit). It also investigates the specific factors that contribute to stress using these modes. Using ordered logistic regressions, the study develops a general model of stress and three mode-specific models. Results show that driving is the most stressful mode of transportation when compared to others. We also find that stressors for some modes are not stressors for others. Knowing which specific factors make certain modes stressful will help transportation and public health professionals make commuting a safer, more enjoyable, and less stressful activity; in turn this could mitigate the potentially serious health outcomes of a stressful commute.},
 author = {Legrain, Alexander and Eluru, Naveen and {El-Geneidy}, Ahmed M.},
 doi = {10.1016/j.trf.2015.08.001},
 file = {/home/matt/Zotero/storage/7QYKNE9G/Legrain et al. - 2015 - Am stressed, must travel The relationship between.pdf;/home/matt/Zotero/storage/48CG6369/S1369847815001370.html},
 issn = {1369-8478},
 journal = {Transportation Research Part F: Traffic Psychology and Behaviour},
 pages = {141--151},
 shorttitle = {Am Stressed, Must Travel},
 title = {Am Stressed, Must Travel: {{The}} Relationship between Mode Choice and Commuting Stress},
 volume = {34},
 year = {2015}
}

@article{lehmann_fisher_1993,
 author = {Lehmann, E. L.},
 doi = {10.2307/2291263},
 file = {/home/matt/Zotero/storage/DRIYSVFZ/Lehmann - 1993 - The Fisher, Neyman-Pearson Theories of Testing Hyp.pdf},
 issn = {01621459},
 journal = {Journal of the American Statistical Association},
 number = {424},
 pages = {1242--1249},
 shorttitle = {The {{Fisher}}, {{Neyman}}-{{Pearson Theories}} of {{Testing Hypotheses}}},
 title = {The {{Fisher}}, {{Neyman}}-{{Pearson Theories}} of {{Testing Hypotheses}}: {{One Theory}} or {{Two}}?},
 volume = {88},
 year = {1993}
}

@article{levie_cayleynets_2017,
 author = {Levie, Ron and Monti, Federico and Bresson, Xavier and Bronstein, Michael M.},
 journal = {ArXiv preprint},
 title = {{{CayleyNets}}: {{Graph Convolutional Neural Networks}} with {{Complex Rational Spectral Filters}}},
 url = {https://arxiv.org/abs/1705.07664},
 volume = {abs/1705.07664},
 year = {2017}
}

@book{levine_n._methodology_1994,
 annotation = {Published: Report submitted to the California Air Resources Board and the California Department of Transportation (Office of Traffic Improvement).},
 author = {{Levine, N.} and Wachs, M.},
 title = {Methodology for {{Vehicle Occupancy Measurement}}},
 year = {1994}
}

@article{levine_reinforcement_2018,
 author = {Levine, Sergey},
 journal = {ArXiv preprint},
 title = {Reinforcement {{Learning}} and {{Control}} as {{Probabilistic Inference}}: {{Tutorial}} and {{Review}}},
 url = {https://arxiv.org/abs/1805.00909},
 volume = {abs/1805.00909},
 year = {2018}
}

@inproceedings{levy_linguistic_2014,
 address = {Ann Arbor, Michigan},
 author = {Levy, Omer  and
Goldberg, Yoav},
 booktitle = {Proceedings of the Eighteenth Conference on Computational Natural Language Learning},
 doi = {10.3115/v1/W14-1618},
 pages = {171--180},
 publisher = {Association for Computational Linguistics},
 title = {Linguistic Regularities in Sparse and Explicit Word Representations},
 url = {https://aclanthology.org/W14-1618},
 year = {2014}
}

@article{li_ahs_1997,
 author = {Li, Perry and Alvarez, Luis and Horowitz, Roberto},
 file = {/home/matt/Zotero/storage/3ZHAFSN4/27j_Li_AVHS_safe_control_IEEE_TCST97.pdf},
 journal = {Control Systems Technology, IEEE Transactions on},
 number = {6},
 pages = {614--628},
 title = {{{AHS}} Safe Control Laws for Platoon Leaders},
 volume = {5},
 year = {1997}
}

@inproceedings{li_deeper_2018,
 author = {Qimai Li and
Zhichao Han and
Xiao{-}Ming Wu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/LiHW18.bib},
 booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
(AAAI-18), the 30th innovative Applications of Artificial Intelligence
(IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
Artificial Intelligence (EAAI-18), New Orleans, Louisiana, USA, February
2-7, 2018},
 editor = {Sheila A. McIlraith and
Kilian Q. Weinberger},
 pages = {3538--3545},
 publisher = {{AAAI} Press},
 timestamp = {Mon, 22 Oct 2018 01:00:00 +0200},
 title = {Deeper Insights Into Graph Convolutional Networks for Semi-Supervised
Learning},
 url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/16098},
 year = {2018}
}

@inproceedings{li_diffusion_2018,
 author = {Yaguang Li and
Rose Yu and
Cyrus Shahabi and
Yan Liu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LiYS018.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Diffusion Convolutional Recurrent Neural Network: Data-Driven Traffic
Forecasting},
 url = {https://openreview.net/forum?id=SJiHXGWAZ},
 year = {2018}
}

@article{li_explaining_2001,
 author = {Li, Jianling},
 file = {/home/matt/Zotero/storage/XQIFGH5M/LiExplainingHOTuse.pdf},
 journal = {Transportation Research Part D: Transport and Environment},
 number = {1},
 pages = {61--74},
 title = {Explaining High-Occupancy-Toll Lane Use},
 volume = {6},
 year = {2001}
}

@inproceedings{li_generalized_2020,
 author = {Alexander C. Li and
Lerrel Pinto and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LiPA20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Generalized Hindsight for Reinforcement Learning},
 url = {https://proceedings.neurips.cc/paper/2020/hash/57e5cb96e22546001f1d6520ff11d9ba-Abstract.html},
 year = {2020}
}

@article{li_generic_2019,
 abstract = {Accurately tracking and predicting behaviors of surrounding objects are key prerequisites for intelligent systems such as autonomous vehicles to achieve safe and high-quality decision making and motion planning. However, there still remain challenges for multi-target tracking due to object number fluctuation and occlusion. To overcome these challenges, we propose a constrained mixture sequential Monte Carlo (CMSMC) method in which a mixture representation is incorporated in the estimated posterior distribution to maintain multi-modality. Multiple targets can be tracked simultaneously within a unified framework without explicit data association between observations and tracking targets. The framework can incorporate an arbitrary prediction model as the implicit proposal distribution of the CMSMC method. An example in this paper is a learning-based model for hierarchical time-series prediction, which consists of a behavior recognition module and a state evolution module. Both modules in the proposed model are generic and flexible so as to be applied to a class of time-series prediction problems where behaviors can be separated into different levels. Finally, the proposed framework is applied to a numerical case study as well as a task of on-road vehicle tracking, behavior recognition, and prediction in highway scenarios. Instead of only focusing on forecasting trajectory of a single entity, we jointly predict continuous motions for interactive entities simultaneously. The proposed approaches are evaluated from multiple aspects, which demonstrate great potential for intelligent vehicular systems and traffic surveillance systems.},
 author = {Li, J. and Zhan, W. and Hu, Y. and Tomizuka, M.},
 doi = {10.1109/TITS.2019.2930310},
 file = {/home/matt/Zotero/storage/LY2UJTJT/Li et al_2019_Generic Tracking and Probabilistic Prediction Framework and Its Application in.pdf;/home/matt/Zotero/storage/F4XHLD5J/8789525.html},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 pages = {1--16},
 title = {Generic {{Tracking}} and {{Probabilistic Prediction Framework}} and {{Its Application}} in {{Autonomous Driving}}},
 year = {2019}
}

@inproceedings{li_learning_2018,
 abstract = {Graphs are fundamental data structures which concisely capture the relational structure in many important real-world domains, such as knowledge graphs, physical and social interactions, language, and chemistry. Here we introduce a powerful new approach for learning generative models over graphs, which can capture both their structure and attributes. Our approach uses graph neural networks to express probabilistic dependencies among a graph's nodes and edges, and can, in principle, learn distributions over any arbitrary graph. In a series of experiments our results show that once trained, our models can generate good quality samples of both synthetic graphs as well as real molecular graphs, both unconditionally and conditioned on data. Compared to baselines that do not use graph-structured representations, our models often perform far better. We also explore key challenges of learning generative models of graphs, such as how to handle symmetries and ordering of elements during the graph generation process, and offer possible solutions. Our work is the first and most general approach for learning generative models over arbitrary graphs, and opens new directions for moving away from restrictions of vector- and sequence-like knowledge representations, toward more expressive and flexible relational data structures.},
 archiveprefix = {arXiv},
 author = {Li, Yujia and Vinyals, Oriol and Dyer, Chris and Pascanu, Razvan and Battaglia, Peter},
 booktitle = {Proceedings of the 35th {{International Conference}} on {{Machine Learning}}},
 eprint = {1803.03324},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/Y4QMKYET/Li et al. - 2018 - Learning Deep Generative Models of Graphs.pdf;/home/matt/Zotero/storage/ZPR4RZJV/1803.html},
 publisher = {{PMLR}},
 title = {Learning {{Deep Generative Models}} of {{Graphs}}},
 volume = {80},
 year = {2018}
}

@article{li_learning_2019,
 author = {Li, Zengyi and Chen, Yubei and Sommer, Friedrich T.},
 journal = {ArXiv preprint},
 title = {Learning {{Energy}}-{{Based Models}} in {{High}}-{{Dimensional Spaces}} with {{Multi}}-Scale {{Denoising Score Matching}}},
 url = {https://arxiv.org/abs/1910.07762},
 volume = {abs/1910.07762},
 year = {2019}
}

@article{li_linear_1999,
 author = {Li, Y. and Ziliaskopoulos, A. K. and Waller, S. T.},
 journal = {Transportation Research Record},
 pages = {52--59},
 title = {Linear {{Programming}} Formulations for System Optimium {{Dynamic Traffic Assignment}} with Arrival Time-Based and Departure-Time Based Demands},
 volume = {1667},
 year = {1999}
}

@inproceedings{li_neural_2018,
 abstract = {A capsule is a collection of neurons which represents different variants of a pattern in the network. The routing scheme ensures only certain capsules which resemble lower counterparts in the higher layer should be activated. However, the computational complexity becomes a bottleneck for scaling up to larger networks, as lower capsules need to correspond to each and every higher capsule. To resolve this limitation, we approximate the routing process with two branches: a master branch which collects primary information from its direct contact in the lower layer and an aide branch that replenishes master based on pattern variants encoded in other lower capsules. Compared with previous iterative and unsupervised routing scheme, these two branches are communicated in a fast, supervised and one-time pass fashion. The complexity and runtime of the model are therefore decreased by a large margin. Motivated by the routing to make higher capsule have agreement with lower capsule, we extend the mechanism as a compensation for the rapid loss of information in nearby layers. We devise a feedback agreement unit to send back higher capsules as feedback. It could be regarded as an additional regularization to the network. The feedback agreement is achieved by comparing the optimal transport divergence between two distributions (lower and higher capsules). Such an add-on witnesses a unanimous gain in both capsule and vanilla networks. Our proposed EncapNet performs favorably better against previous state-of-the-arts on CIFAR10/100, SVHN and a subset of ImageNet.},
 archiveprefix = {arXiv},
 author = {Li, Hongyang and Guo, Xiaoyang and Dai, Bo and Ouyang, Wanli and Wang, Xiaogang},
 booktitle = {The {{European Conference}} on {{Computer Vision}} ({{ECCV}})},
 doi = {10.1007/978-3-030-01252-6_16},
 eprint = {1808.03749},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/XNQXW6LR/Li et al. - 2018 - Neural Network Encapsulation.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Neural {{Network Encapsulation}}},
 year = {2018}
}

@article{li_social-wagdat_2020,
 author = {Li, Jiachen and Ma, Hengbo and Zhang, Zhihao and Tomizuka, Masayoshi},
 journal = {ArXiv preprint},
 title = {Social-{{WaGDAT}}: {{Interaction}}-Aware {{Trajectory Prediction}} via {{Wasserstein Graph Double}}-{{Attention Network}}},
 url = {https://arxiv.org/abs/2002.06241},
 volume = {abs/2002.06241},
 year = {2020}
}

@article{li_train_2020,
 author = {Li, Zhuohan and Wallace, Eric and Shen, Sheng and Lin, Kevin and Keutzer, Kurt and Klein, Dan and Gonzalez, Joseph E.},
 journal = {ArXiv preprint},
 title = {Train {{Large}}, {{Then Compress}}: {{Rethinking Model Size}} for {{Efficient Training}} and {{Inference}} of {{Transformers}}},
 url = {https://arxiv.org/abs/2002.11794},
 volume = {abs/2002.11794},
 year = {2020}
}

@inproceedings{liang_rllib_2018,
 author = {Eric Liang and
Richard Liaw and
Robert Nishihara and
Philipp Moritz and
Roy Fox and
Ken Goldberg and
Joseph Gonzalez and
Michael I. Jordan and
Ion Stoica},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/LiangLNMFGGJS18.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {3059--3068},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Thu, 30 Apr 2020 01:00:00 +0200},
 title = {RLlib: Abstractions for Distributed Reinforcement Learning},
 url = {http://proceedings.mlr.press/v80/liang18b.html},
 volume = {80},
 year = {2018}
}

@inproceedings{liaw_hypersched_2019,
 abstract = {Prior research in resource scheduling for machine learning training workloads has largely focused on minimizing job completion times. Commonly, these model training workloads collectively search over a large number of parameter values that control the learning process in a hyperparameter search. It is preferable to identify and maximally provision the best-performing hyperparameter configuration (trial) to achieve the highest accuracy result as soon as possible. To optimally trade-off evaluating multiple configurations and training the most promising ones by a fixed deadline, we design and build HyperSched\textemdash a dynamic application-level resource scheduler to track, identify, and preferentially allocate resources to the best performing trials to maximize accuracy by the deadline. HyperSched leverages three properties of a hyperparameter search workload overlooked in prior work \textendash{} trial disposability, progressively identifiable rankings among different configurations, and space-time constraints \textendash{} to outperform standard hyperparameter search algorithms across a variety of benchmarks.},
 address = {{Santa Cruz, CA, USA}},
 author = {Liaw, Richard and Bhardwaj, Romil and Dunlap, Lisa and Zou, Yitian and Gonzalez, Joseph E. and Stoica, Ion and Tumanov, Alexey},
 booktitle = {Proceedings of the {{ACM Symposium}} on {{Cloud Computing}}  - {{SoCC}} '19},
 doi = {10.1145/3357223.3362719},
 file = {/home/matt/Zotero/storage/35DMI8HV/Liaw et al. - 2019 - HyperSched Dynamic Resource Reallocation for Mode.pdf},
 isbn = {978-1-4503-6973-2},
 language = {en},
 pages = {61--73},
 publisher = {{ACM Press}},
 shorttitle = {{{HyperSched}}},
 title = {{{HyperSched}}: {{Dynamic Resource Reallocation}} for {{Model Development}} on a {{Deadline}}},
 year = {2019}
}

@article{liebenstein_allocative_1966,
 author = {Liebenstein, H.},
 journal = {American Economic Review},
 number = {3},
 pages = {392--415},
 title = {Allocative {{Efficiency}} vs.\textbackslash{} {{X}}-{{Efficiency}}},
 volume = {56},
 year = {1966}
}

@article{lieu_corflo_1991,
 author = {Lieu, H. and Santiago, A. J.},
 journal = {Traffic Management, Proceedings of the Engineering Foundation Conference, Palm Coast, Florida},
 title = {{{CORFLO}}: {{An}} Integrated Traffic Simulation System for Corridors.},
 year = {1991}
}

@article{lighthill_kinematic_1955,
 author = {Lighthill, M. and Whitham, G.},
 journal = {Proceedings of the Royal Society of London, Part A},
 number = {1178},
 pages = {281--345},
 title = {On Kinematic Waves {{I}}: {{Flow}} Movement in Long Rivers. {{II}}: {{A}} Theory of Traffic Flow on Long Crowded Roads},
 volume = {229},
 year = {1955}
}

@article{lighthill_kinematic_1955_pt1,
 abstract = {In this paper and in part II, we give the theory of a distinctive type of wave motion, which arises in any one-dimensional flow problem when there is an approximate functional relation at each point between the flow q (quantity passing a given point in unit time) and concentration k (quantity per unit distance). The wave property then follows directly from the equation of continuity satisfied by q and k. In view of this, these waves are described as `kinematic', as distinct from the classical wave motions, which depend also on Newton's second law of motion and are therefore called `dynamic'. Kinematic waves travel with the velocity dq/dk, and the flow q remains constant on each kinematic wave. Since the velocity of propagation of each wave depends upon the value of q carried by it, successive waves may coalesce to form `kinematic shock waves '. From the point of view of kinematic wave theory, there is a discontinuous increase in q at a shock, but in reality a shock wave is a relatively narrow region in which (owing to the rapid increase of q) terms neglected by the flow concentration relation become important. The general properties of kinematic waves and shock waves are discussed in detail in \textsection 1. One example included in \textsection 1 is the interpretation of the group-velocity phenomenon in a dispersive medium as a particular case of the kinematic wave phenomenon. The remainder of part I is devoted to a detailed treatment of flood movement in long rivers, a problem in which kinematic waves play the leading role although dynamic waves (in this case, the long gravity waves) also appear. First (\textsection 2), we consider the variety of factors which can influence the approximate flow-concentration relation, and survey the various formulae which have been used in attempts to describe it. Then follows a more mathematical section (\textsection 3) in which the role of the dynamic waves is clarified. From the full equations of motion for an idealized problem it is shown that at the `Froude numbers' appropriate to flood waves, the dynamic waves are rapidly attenuated and the main disturbance is carried downstream by the kinematic waves; some account is then given of the behaviour of the flow at higher Froude numbers. Also in \textsection 3, the full equations of motion are used to investigate the structure of the kinematic shock; for this problem, the shock is the `monoclinal flood wave' which is well known in the literature of this subject. The final sections (\textsection\textsection 4 and 5) contain the application of the theory of kinematic waves to the determination of flood movement. In \textsection 4 it is shown how the waves (including shock waves) travelling downstream from an observation point may be deduced from a knowledge of the variation with time of the flow at the observation point; this section then concludes with a brief account of the effect on the waves of tributaries and run-off. In \textsection 5, the modifications (similar to diffusion effects) which arise due to the slight dependence of the flow-concentration curve on the rate of change of flow or concentration, are described and methods for their inclusion in the theory are given.},
 author = {Lighthill, Michael James and Whitham, G. B.},
 doi = {10.1098/rspa.1955.0088},
 file = {/home/matt/Zotero/storage/23WA7GFE/Lighthill Michael James and Whitham G. B. - 1955 - On kinematic waves I. Flood movement in long river.pdf;/home/matt/Zotero/storage/2UAW53NL/rspa.1955.html},
 journal = {Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
 number = {1178},
 pages = {281--316},
 title = {On Kinematic Waves {{I}}. {{Flood}} Movement in Long Rivers},
 volume = {229},
 year = {1955}
}

@article{lighthill_kinematic_1955_pt2,
 author = {Lighthill, M. J. and Whitham, G. B.},
 doi = {10.1098/rspa.1955.0089},
 file = {/home/matt/Zotero/storage/6VX98ZPW/1955 - On kinematic waves II. A theory of traffic flow on.pdf},
 issn = {2053-9169},
 journal = {Proceedings of the Royal Society of London. Series A. Mathematical and Physical Sciences},
 language = {en},
 number = {1178},
 pages = {317--345},
 title = {On Kinematic Waves {{II}}. {{A}} Theory of Traffic Flow on Long Crowded Roads},
 volume = {229},
 year = {1955}
}

@inproceedings{lillicrap_continuous_2016,
 author = {Timothy P. Lillicrap and
Jonathan J. Hunt and
Alexander Pritzel and
Nicolas Heess and
Tom Erez and
Yuval Tassa and
David Silver and
Daan Wierstra},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/LillicrapHPHETS15.bib},
 booktitle = {4th International Conference on Learning Representations, {ICLR} 2016,
San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Continuous control with deep reinforcement learning},
 url = {http://arxiv.org/abs/1509.02971},
 year = {2016}
}

@article{lin_analysis_1993,
 author = {Lin, Feng-Bor},
 journal = {Transportation Planning Journal},
 number = {4},
 pages = {445--478},
 title = {Analysis {{Of Traffic Flow Characteristics On Sun Yat}}-{{Sen National Freeway For Capacity And Level}}-{{Of}}-{{Service Analysis}}},
 volume = {22},
 year = {1993}
}

@inproceedings{lin_feature_2017,
 author = {Tsung{-}Yi Lin and
Piotr Doll{\'{a}}r and
Ross B. Girshick and
Kaiming He and
Bharath Hariharan and
Serge J. Belongie},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/LinDGHHB17.bib},
 booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
 doi = {10.1109/CVPR.2017.106},
 pages = {936--944},
 publisher = {{IEEE} Computer Society},
 timestamp = {Tue, 14 Nov 2017 00:00:00 +0100},
 title = {Feature Pyramid Networks for Object Detection},
 url = {https://doi.org/10.1109/CVPR.2017.106},
 year = {2017}
}

@article{lin_grammar-based_2019,
 author = {Lin, Kevin and Bogin, Ben and Neumann, Mark and Berant, Jonathan and Gardner, Matt},
 journal = {ArXiv preprint},
 title = {Grammar-Based {{Neural Text}}-to-{{SQL Generation}}},
 url = {https://arxiv.org/abs/1905.13326},
 volume = {abs/1905.13326},
 year = {2019}
}

@article{lin_headway_2005,
 author = {Lin, F. B. and Thomas, D. R.},
 journal = {Transportation Research Record},
 number = {1920},
 pages = {81--85},
 title = {Headway {{Compression During Queue Discharge}} at {{Signalized Intersections}}},
 year = {2005}
}

@article{lin_methodology_1998,
 author = {Lin, Feng-Bor and Su, Cheng-Wei},
 journal = {Transportation Planning Journal},
 number = {1},
 pages = {1--34},
 title = {A {{Methodology For Capacity And Level}}-{{Of}}-{{Service Analysis Of Freeway Basic Selections}}},
 volume = {27},
 year = {1998}
}

@article{lin_reproducing_2019,
 author = {Lin, Rongrong and Zhang, Haizhang and Zhang, Jun},
 journal = {ArXiv preprint},
 title = {On {{Reproducing Kernel Banach Spaces}}: {{Generic Definitions}} and {{Unified Framework}} of {{Constructions}}},
 url = {https://arxiv.org/abs/1901.01002},
 volume = {abs/1901.01002},
 year = {2019}
}

@article{lin_short-term_2004,
 author = {Lin, W.-H. and Kulkarni, A. and Mirchandani, P.},
 journal = {Intelligent Transportation Systems},
 pages = {143-154},
 title = {Short-{{Term Arterial Travel Time Prediction}} for {{Advanced Traveler Information Systems}}},
 volume = {8},
 year = {2004}
}

@techreport{lin_study_2003,
 abstract = {The sigmoid kernel was quite popular for support vector machines due to its origin from neural networks. Although it is known that the kernel matrix may not be positive semi-definite (PSD), other properties are not fully studied. In this paper, we discuss such non-PSD kernels through the viewpoint of separability. Results help to validate the possible use of non-PSD kernels. One example shows that the sigmoid kernel matrix is conditionally positive definite (CPD) in certain parameters and thus are valid kernels there. However, we also explain that the sigmoid kernel is not better than the RBF kernel in general. Experiments are given to illustrate our analysis. Finally, we discuss how to solve the non-convex dual problems by SMO-type decomposition methods. Suitable modifications for any symmetric non-PSD kernel matrices are proposed with convergence proofs.},
 address = {{Taipei, Taiwan}},
 author = {Lin, Hsuan-Tien and Lin, Chih-Jen},
 file = {/home/matt/Zotero/storage/S88FJCR4/Lin and Lin - A Study on Sigmoid Kernels for SVM and the Trainin.pdf},
 institution = {{National Taiwan University}},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {A {{Study}} on {{Sigmoid Kernels}} for {{SVM}} and the {{Training}} of Non-{{PSD Kernels}} by {{SMO}}-Type {{Methods}}},
 year = {2003}
}

@book{lindley_applying_2012,
 annotation = {Published: ITS World Congress},
 author = {Lindley, J. A.},
 title = {Applying {{Systems Engineering}} to {{Implementation}} of {{Adaptive Signal Control Technology}}},
 year = {2012}
}

@techreport{lindley_j._qualification_1986,
 author = {{Lindley, J.}},
 institution = {{Federal Highway Report}},
 number = {RD/87-052},
 title = {Qualification of Urban Freeway Congestion and Analysis of Remedial Measures},
 year = {1986}
}

@article{lioris_control_2014-1,
 author = {Lioris, J. and Kurzhanskiy, A. and Triantafyllos, D. and Varaiya, P},
 journal = {12th IFAC-IEEE Workshop on Discrete Event Systems, Ecole Normale Superieure de Cachan, France},
 title = {Control Experiments for a Network of Signalized Intersections Using the '.{{Q}}'},
 year = {2014}
}

@article{lipton_troubling_2018,
 author = {Lipton, Zachary C. and Steinhardt, Jacob},
 journal = {ArXiv preprint},
 title = {Troubling {{Trends}} in {{Machine Learning Scholarship}}},
 url = {https://arxiv.org/abs/1807.03341},
 volume = {abs/1807.03341},
 year = {2018}
}

@article{little_synchronizing_1966,
 author = {Little, J.},
 journal = {Operations Research},
 number = {4},
 pages = {568--594},
 title = {The Synchronizing Traffic Signals by Mixed-Integer Linear Programming},
 volume = {14},
 year = {1966}
}

@inproceedings{Liu_2019_CVPR,
 author = {Ziwei Liu and
Zhongqi Miao and
Xiaohang Zhan and
Jiayun Wang and
Boqing Gong and
Stella X. Yu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/0002MZWGY19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00264},
 pages = {2537--2546},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Large-Scale Long-Tailed Recognition in an Open World},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Liu\_Large-Scale\_Long-Tailed\_Recognition\_in\_an\_Open\_World\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{liu_analysis_2011,
 author = {Liu, Xiaoyue and Schroeder, Bastian and Thomson, Timothy and Wang, Yinhai and Rouphail, Nagui and Yin, Yafeng},
 doi = {10.3141/2262-07},
 file = {/home/matt/Zotero/storage/V5U6XZKX/2011_TRR_friction_effect.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {62--73},
 title = {Analysis of {{Operational Interactions Between Freeway Managed Lanes}} and {{Parallel}}, {{General Purpose Lanes}}},
 volume = {2262},
 year = {2011}
}

@inproceedings{liu_delayed_2018,
 author = {Lydia T. Liu and
Sarah Dean and
Esther Rolf and
Max Simchowitz and
Moritz Hardt},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/ijcai/LiuDRSH19.bib},
 booktitle = {Proceedings of the Twenty-Eighth International Joint Conference on
Artificial Intelligence, {IJCAI} 2019, Macao, China, August 10-16,
2019},
 doi = {10.24963/ijcai.2019/862},
 editor = {Sarit Kraus},
 pages = {6196--6200},
 publisher = {ijcai.org},
 timestamp = {Tue, 20 Aug 2019 01:00:00 +0200},
 title = {Delayed Impact of Fair Machine Learning},
 url = {https://doi.org/10.24963/ijcai.2019/862},
 year = {2019}
}

@inproceedings{liu_delving_2016,
 author = {Yanpei Liu and
Xinyun Chen and
Chang Liu and
Dawn Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LiuCLS17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Delving into Transferable Adversarial Examples and Black-box Attacks},
 url = {https://openreview.net/forum?id=Sys6GJqxl},
 year = {2017}
}

@inproceedings{liu_energy-based_2021,
 author = {Weitang Liu and
Xiaoyun Wang and
John D. Owens and
Yixuan Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LiuWOL20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Energy-based Out-of-distribution Detection},
 url = {https://proceedings.neurips.cc/paper/2020/hash/f5496252609c43eb8a3d147ab9b9c006-Abstract.html},
 year = {2020}
}

@article{liu_estimation_1996,
 author = {Liu, S. and Fricker, J. D.},
 journal = {Transportation Research A},
 number = {4},
 pages = {287--305},
 title = {Estimation of a Trip Table and the {{$\Theta$}} Parameter in a Stochastic Network},
 volume = {30},
 year = {1996}
}

@inproceedings{liu_hallucinative_2020,
 author = {Kara Liu and
Thanard Kurutach and
Christine Tung and
Pieter Abbeel and
Aviv Tamar},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/LiuKTAT20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {6259--6270},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Hallucinative Topological Memory for Zero-Shot Visual Planning},
 url = {http://proceedings.mlr.press/v119/liu20h.html},
 volume = {119},
 year = {2020}
}

@article{liu_improved_1998,
 author = {Liu, G. and Lyrintzis, A. S. and Michalopoulos, P. G.},
 journal = {Transportation Research Record},
 number = {1644},
 pages = {37--46},
 title = {Improved {{High}}-{{Order Model}} for {{Freeway Traffic Flow}}.},
 year = {1998}
}

@inproceedings{liu_large-scale_nodate,
 author = {Ziwei Liu and
Zhongqi Miao and
Xiaohang Zhan and
Jiayun Wang and
Boqing Gong and
Stella X. Yu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/0002MZWGY19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00264},
 pages = {2537--2546},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Large-Scale Long-Tailed Recognition in an Open World},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Liu\_Large-Scale\_Long-Tailed\_Recognition\_in\_an\_Open\_World\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{liu_meltdown_2016,
 author = {Liu, Dehong and Gu, Hongmei and Xing, Tiancai},
 doi = {10.1016/j.iref.2016.07.011},
 file = {/home/matt/Zotero/storage/5QKS6WGR/liu_chinese_meltdown_2015.pdf},
 issn = {10590560},
 journal = {International Review of Economics \& Finance},
 language = {en},
 pages = {504--517},
 title = {The Meltdown of the {{Chinese}} Equity Market in the Summer of 2015},
 volume = {45},
 year = {2016}
}

@article{liu_modeling_2012,
 author = {Liu, Xiaoyue and Zhang, Guohui and Lao, Yunteng and Wang, Yinhai},
 doi = {10.3141/2278-18},
 file = {/home/matt/Zotero/storage/NJIQHMEI/2012_TRR_managed_lane_friction_modeling.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {163--170},
 shorttitle = {Modeling {{Traffic Flow Dynamics}} on {{Managed Lane Facility}}},
 title = {Modeling {{Traffic Flow Dynamics}} on {{Managed Lane Facility}}: {{Approach Based}} on {{Cell Transmission Model}}},
 volume = {2278},
 year = {2012}
}

@article{liu_real-time_2009,
 author = {Liu, Henry X. and Wu, Xinkai and Ma, Wenteng and Hu, Heng},
 doi = {10.1016/j.trc.2009.02.003},
 file = {/home/matt/Zotero/storage/D7H88QFI/Real-time_queue_length_estimation_for_congested_si.pdf},
 issn = {0968090X},
 journal = {Transportation Research C: Emerging Technologies},
 language = {en},
 number = {4},
 pages = {412--427},
 title = {Real-Time Queue Length Estimation for Congested Signalized Intersections},
 volume = {17},
 year = {2009}
}

@article{liu_reverse_2008,
 author = {Liu, H. and Balke, K. N. and Lin, W.-H.},
 journal = {Transportation Research, Part C},
 pages = {742--754},
 title = {A Reverse Causal-Effect Modeling Approach for Signal Control of an Oversaturated Intersection},
 volume = {16},
 year = {2008}
}

@article{liu_roberta_2019,
 author = {Liu, Yinhan and Ott, Myle and Goyal, Naman and Du, Jingfei and Joshi, Mandar and Chen, Danqi and Levy, Omer and Lewis, Mike and Zettlemoyer, Luke and Stoyanov, Veselin},
 journal = {ArXiv preprint},
 title = {{{RoBERTa}}: {{A Robustly Optimized BERT Pretraining Approach}}},
 url = {https://arxiv.org/abs/1907.11692},
 volume = {abs/1907.11692},
 year = {2019}
}

@article{liu_sensor_2013,
 author = {Liu, Ming and Shi, Peng},
 doi = {10.1016/j.automatica.2013.01.030},
 file = {/home/matt/Zotero/storage/4P59AND7/1-s2.0-S0005109813000319-main.pdf},
 issn = {00051098},
 journal = {Automatica},
 language = {en},
 number = {5},
 pages = {1242--1250},
 title = {Sensor Fault Estimation and Tolerant Control for {{It\^o}} Stochastic Systems with a Descriptor Sliding Mode Approach},
 volume = {49},
 year = {2013}
}

@article{liu_sequence_2019,
 author = {Liu, Yang and Luo, Yunan and Zhong, Yuanyi and Chen, Xi and Liu, Qiang and Peng, Jian},
 journal = {ArXiv preprint},
 title = {Sequence {{Modeling}} of {{Temporal Credit Assignment}} for {{Episodic Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1905.13420},
 volume = {abs/1905.13420},
 year = {2019}
}

@inproceedings{liu_shared-private_2019,
 address = {Florence, Italy},
 author = {Liu, Xuebo  and
Wong, Derek F.  and
Liu, Yang  and
Chao, Lidia S.  and
Xiao, Tong  and
Zhu, Jingbo},
 booktitle = {Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/P19-1352},
 pages = {3613--3622},
 publisher = {Association for Computational Linguistics},
 title = {Shared-Private Bilingual Word Embeddings for Neural Machine Translation},
 url = {https://aclanthology.org/P19-1352},
 year = {2019}
}

@inproceedings{liu_ssd_2016,
 abstract = {We present a method for detecting objects in images using a single deep neural network. Our approach, named SSD, discretizes the output space of bounding boxes into a set of default boxes over different aspect ratios and scales per feature map location. At prediction time, the network generates scores for the presence of each object category in each default box and produces adjustments to the box to better match the object shape. Additionally, the network combines predictions from multiple feature maps with different resolutions to naturally handle objects of various sizes. SSD is simple relative to methods that require object proposals because it completely eliminates proposal generation and subsequent pixel or feature resampling stages and encapsulates all computation in a single network. This makes SSD easy to train and straightforward to integrate into systems that require a detection component. Experimental results on the PASCAL VOC, COCO, and ILSVRC datasets confirm that SSD has competitive accuracy to methods that utilize an additional object proposal step and is much faster, while providing a unified framework for both training and inference. For \$\$300 \textbackslash times 300\$\$300\texttimes 300input, SSD achieves 74.3~\% mAP on VOC2007 test at 59~FPS on a Nvidia Titan X and for \$\$512 \textbackslash times 512\$\$512\texttimes 512input, SSD achieves 76.9~\% mAP, outperforming a comparable state of the art Faster R-CNN model. Compared to other single stage methods, SSD has much better accuracy even with a smaller input image size. Code is available at https://github.com/weiliu89/caffe/tree/ssd.},
 address = {{Cham}},
 author = {Liu, Wei and Anguelov, Dragomir and Erhan, Dumitru and Szegedy, Christian and Reed, Scott and Fu, Cheng-Yang and Berg, Alexander C.},
 booktitle = {European {{Conference}} on {{Computer Vision}} ({{ECCV}})},
 editor = {Leibe, Bastian and Matas, Jiri and Sebe, Nicu and Welling, Max},
 isbn = {978-3-319-46448-0},
 pages = {21--37},
 publisher = {{Springer International Publishing}},
 title = {{{SSD}}: {{Single Shot MultiBox Detector}}},
 year = {2016}
}

@article{liu_transferable_2019,
 author = {Liu, Zhuang and Zhou, Tinghui and Shen, Zhiqiang and Kang, Bingyi and Darrell, Trevor},
 journal = {ArXiv preprint},
 title = {Transferable {{Recognition}}-{{Aware Image Processing}}},
 url = {https://arxiv.org/abs/1910.09185},
 volume = {abs/1910.09185},
 year = {2019}
}

@article{liu_unpaired_2019,
 author = {Liu, Runtao and Yu, Qian and Yu, Stella},
 journal = {ArXiv preprint},
 title = {An {{Unpaired Sketch}}-to-{{Photo Translation Model}}},
 url = {https://arxiv.org/abs/1909.08313},
 volume = {abs/1909.08313},
 year = {2019}
}

@inproceedings{liu_variance_2020,
 author = {Liyuan Liu and
Haoming Jiang and
Pengcheng He and
Weizhu Chen and
Xiaodong Liu and
Jianfeng Gao and
Jiawei Han},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LiuJHCLG020.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {On the Variance of the Adaptive Learning Rate and Beyond},
 url = {https://openreview.net/forum?id=rkgz2aEKDr},
 year = {2020}
}

@article{liu_virtual_2009,
 author = {Liu, H. X. and Ma, W.},
 journal = {Transportation Resaerch, Part C},
 number = {1},
 pages = {11--26},
 title = {A Virtual Vehicle Probe Model for Time-Dependent Arterial Travel Time Estimation},
 volume = {17},
 year = {2009}
}

@article{lo_cell-based_2001,
 author = {Lo, H. K.},
 journal = {Transportation Science},
 number = {2},
 pages = {148--164},
 title = {A {{Cell}}-{{Based Traffic Control Formulation}}: {{Strategies}} and {{Benefits}} of {{Dynamic Timing Plans}}},
 volume = {35},
 year = {2001}
}

@article{lo_cell-based_2002,
 author = {Lo, H. K. and Szeto, W. Y.},
 journal = {Transportation Research, Part B},
 pages = {421--443},
 title = {A Cell-Based Variational Inequality Formulation of the Dynamic User Optimal Assignment Problem},
 volume = {36},
 year = {2002}
}

@article{lo_control_2004,
 author = {Lo, H. K. and Chow, A. H. F.},
 journal = {Journal of Transportation Engineering},
 number = {4},
 pages = {721--744},
 title = {Control Strategies for Oversaturated Traffic.},
 volume = {130},
 year = {2004}
}

@article{lo_dynamic_2001,
 author = {Lo, H. K. and Chang, E. and Chan, Y. C.},
 journal = {Transportation Research, A},
 pages = {721--744},
 title = {Dynamic Network Traffic Control.},
 volume = {35},
 year = {2001}
}

@inproceedings{long_evolutionary_2020,
 author = {Qian Long and
Zihan Zhou and
Abhinav Gupta and
Fei Fang and
Yi Wu and
Xiaolong Wang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LongZ0FWW20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Mon, 17 Aug 2020 01:00:00 +0200},
 title = {Evolutionary Population Curriculum for Scaling Multi-Agent Reinforcement
Learning},
 url = {https://openreview.net/forum?id=SJxbHkrKDH},
 year = {2020}
}

@inproceedings{long_evolutionary_2020-1,
 author = {Qian Long and
Zihan Zhou and
Abhinav Gupta and
Fei Fang and
Yi Wu and
Xiaolong Wang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LongZ0FWW20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Mon, 17 Aug 2020 01:00:00 +0200},
 title = {Evolutionary Population Curriculum for Scaling Multi-Agent Reinforcement
Learning},
 url = {https://openreview.net/forum?id=SJxbHkrKDH},
 year = {2020}
}

@inproceedings{long_fully_2015,
 author = {Jonathan Long and
Evan Shelhamer and
Trevor Darrell},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/LongSD15.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2015, Boston, MA, USA, June 7-12, 2015},
 doi = {10.1109/CVPR.2015.7298965},
 pages = {3431--3440},
 publisher = {{IEEE} Computer Society},
 timestamp = {Wed, 06 Feb 2019 00:00:00 +0100},
 title = {Fully convolutional networks for semantic segmentation},
 url = {https://doi.org/10.1109/CVPR.2015.7298965},
 year = {2015}
}

@article{loosli_learning_2016,
 abstract = {This paper presents a theoretical foundation for an SVM solver in Kre{\u \i}n spaces. Up to now, all methods are based either on the matrix correction, or on non-convex minimization, or on feature-space embedding. Here we justify and evaluate a solution that uses the original (indefinite) similarity measure, in the original Kre{\u \i}n space. This solution is the result of a stabilization procedure. We establish the correspondence between the stabilization problem (which has to be solved) and a classical SVM based on minimization (which is easy to solve). We provide simple equations to go from one to the other (in both directions). This link between stabilization and minimization problems is the key to obtain a solution in the original Kre{\u \i}n space. Using KSVM, one can solve SVM with usually troublesome kernels (large negative eigenvalues or large numbers of negative eigenvalues). We show experiments showing that our algorithm KSVM outperforms all previously proposed approaches to deal with indefinite matrices in SVM-like kernel methods.},
 author = {Loosli, Ga{\"e}lle and Canu, St{\'e}phane and Ong, Cheng Soon},
 doi = {10.1109/TPAMI.2015.2477830},
 file = {/home/matt/Zotero/storage/BTY78CR3/Loosli et al. - 2016 - Learning SVM in Kreĭn Spaces.pdf;/home/matt/Zotero/storage/VBIUGIMY/7254195.html},
 issn = {1939-3539},
 journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
 number = {6},
 pages = {1204--1216},
 title = {Learning {{SVM}} in {{Kre{\u \i}n Spaces}}},
 volume = {38},
 year = {2016}
}

@inproceedings{loshchilov_sgdr_2017,
 author = {Ilya Loshchilov and
Frank Hutter},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LoshchilovH17.bib},
 booktitle = {5th International Conference on Learning Representations, {ICLR} 2017,
Toulon, France, April 24-26, 2017, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {{SGDR:} Stochastic Gradient Descent with Warm Restarts},
 url = {https://openreview.net/forum?id=Skq89Scxx},
 year = {2017}
}

@article{lou_optimal_2011,
 author = {Lou, Yingyan and Yin, Yafeng and Laval, Jorge A.},
 doi = {10.1016/j.trc.2010.03.008},
 file = {/home/matt/Zotero/storage/F79TF3EJ/LoutOptimalPricingHOT.pdf;/home/matt/Zotero/storage/RINGWI5T/1-s2.0-S0965856497000487-main.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 number = {1},
 pages = {64--74},
 title = {Optimal Dynamic Pricing Strategies for High-Occupancy/Toll Lanes},
 volume = {19},
 year = {2011}
}

@inproceedings{lovisari_data_2015,
 author = {Lovisari, Enrico and {Canudas de Wit}, Carlos and Kibangou, Alain Y.},
 booktitle = {2015 54th {{IEEE Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
 doi = {10.1109/CDC.2015.7402641},
 file = {/home/matt/Zotero/storage/AJC9FXQF/LoCaKiDensityReconstruction_CDC15.pdf;/home/matt/Zotero/storage/AVW5IVF4/DensityReconstructionPaper.pdf},
 pages = {2804--2809},
 publisher = {{IEEE}},
 title = {Data Fusion Algorithms for Density Reconstruction in Road Transportation Networks},
 year = {2015}
}

@article{lovisari_density/flow_2016,
 author = {Lovisari, E. and {Canudas de Wit}, C. and Kibangou, A. Y.},
 doi = {10.1016/j.trc.2016.06.019},
 file = {/home/matt/Zotero/storage/JNKXMDC5/1-s2.0-S0968090X16300936-main.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {451--476},
 title = {Density/{{Flow}} Reconstruction via Heterogeneous Sources and {{Optimal Sensor Placement}} in Road Networks},
 volume = {69},
 year = {2016}
}

@article{lowe_chemical_2011,
 author = {Lowe, Daniel M. and Corbett, Peter T. and {Murray-Rust}, Peter and Glen, Robert C.},
 doi = {10.1021/ci100384d},
 file = {/home/matt/Zotero/storage/4RLM3QSA/Lowe et al. - 2011 - Chemical Name to Structure OPSIN, an Open Source .pdf},
 issn = {1549-9596, 1549-960X},
 journal = {Journal of Chemical Information and Modeling},
 language = {en},
 number = {3},
 pages = {739--753},
 shorttitle = {Chemical {{Name}} to {{Structure}}},
 title = {Chemical {{Name}} to {{Structure}}: {{OPSIN}}, an {{Open Source Solution}}},
 volume = {51},
 year = {2011}
}

@inproceedings{lowe_multi-agent_2017,
 author = {Ryan Lowe and
Yi Wu and
Aviv Tamar and
Jean Harb and
Pieter Abbeel and
Igor Mordatch},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LoweWTHAM17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {6379--6390},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Multi-Agent Actor-Critic for Mixed Cooperative-Competitive Environments},
 url = {https://proceedings.neurips.cc/paper/2017/hash/68a9750337a418a86fe06c1991a1d64c-Abstract.html},
 year = {2017}
}

@inproceedings{lu_adaptive_2019,
 abstract = {We study learning control in an online lifelong learning scenario, where mistakes can compound catastrophically into the future, and the underlying dynamics of the environment change. Traditional model-free reinforcement learning methods struggle in this setting, as they activate failure modes early in their lifetimes, have difficulty recovering from them later on, and struggle to adapt to changing worlds. On the other hand, model-based planning methods are more robust, but require significant computational resources to deploy. Under constrained computation limits, it becomes important to allocate the agent's resources wisely, which requires the agent to understand both its own performance and the current state of the environment \textendash{} knowing that its mastery over control in the current dynamics is poor, the agent should dedicate more time to planning. We present a new algorithm, Adaptive Online Planning (AOP), that is capable of achieving strong performance in this setting by combining model-based planning with model-free learning. By measuring the performance of the planner and the uncertainty of the model-free components, AOP is able to call upon more extensive planning only when necessary, leading to reduced computation times. We show empirically that AOP capably handles novel states and adapts effectively in the face of unpredictable changes in the world, even when traditional reinforcement learning methods struggle.},
 archiveprefix = {arXiv},
 author = {Lu, Kevin and Mordatch, Igor and Abbeel, Pieter},
 booktitle = {Deep {{Reinforcement Learning Workshop}} at {{NeurIPS}} 2019},
 eprint = {1912.01188},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/8AU6696X/Lu et al. - 2019 - Adaptive Online Planning for Continual Lifelong Le.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Adaptive {{Online Planning}} for {{Continual Lifelong Learning}}},
 year = {2019}
}

@article{lu_automated_2004,
 author = {Lu, Xiao-Yun and Tan, Han-Shue and Shladover, Steven E and Hedrick, J Karl},
 journal = {Vehicle System Dynamics},
 number = {2},
 pages = {85--107},
 title = {Automated Vehicle Merging Maneuver Implementation for {{AHS}}},
 volume = {41},
 year = {2004}
}

@article{lu_connected_2014,
 abstract = {Providing various wireless connectivities for vehicles enables the communication between vehicles and their internal and external environments. Such a connected vehicle solution is expected to be the next frontier for automotive revolution and the key to the evolution to next generation intelligent transportation systems (ITSs). Moreover, connected vehicles are also the building blocks of emerging Internet of Vehicles (IoV). Extensive research activities and numerous industrial initiatives have paved the way for the coming era of connected vehicles. In this paper, we focus on wireless technologies and potential challenges to provide vehicle-to-x connectivity. In particular, we discuss the challenges and review the state-of-the-art wireless solutions for vehicle-to-sensor, vehicle-to-vehicle, vehicle-to-Internet, and vehicle-to-road infrastructure connectivities. We also identify future research issues for building connected vehicles.},
 author = {Lu, N. and Cheng, N. and Zhang, N. and Shen, X. and Mark, J. W.},
 doi = {10.1109/JIOT.2014.2327587},
 file = {/home/matt/Zotero/storage/GU43RQ8S/Lu et al. - 2014 - Connected Vehicles Solutions and Challenges.pdf;/home/matt/Zotero/storage/U37BZ9I4/6823640.html},
 issn = {2327-4662},
 journal = {IEEE Internet of Things Journal},
 number = {4},
 pages = {289--299},
 shorttitle = {Connected {{Vehicles}}},
 title = {Connected {{Vehicles}}: {{Solutions}} and {{Challenges}}},
 volume = {1},
 year = {2014}
}

@article{lu_distributed_1991,
 author = {Lu, S. H. and P.R. Kumar},
 journal = {IEEE Trans. Automatic Control},
 number = {12},
 pages = {1406--1416},
 title = {Distributed Scheduling Based on Due Dates and Buffer Priorities},
 volume = {36},
 year = {1991}
}

@article{lu_impact_2004,
 author = {Lu, Xiao-Yun and Hedrick, J Karl},
 journal = {International journal of vehicle autonomous systems},
 number = {1},
 pages = {40--70},
 title = {Impact of Combined Longitudinal, Lateral and Vertical Control on Autonomous Road Vehicle Design},
 volume = {2},
 year = {2004}
}

@inproceedings{lu_implicit_2021,
 author = {Cheng Lu and
Jianfei Chen and
Chongxuan Li and
Qiuhao Wang and
Jun Zhu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/Lu0LWZ21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Tue, 10 Aug 2021 01:00:00 +0200},
 title = {Implicit Normalizing Flows},
 url = {https://openreview.net/forum?id=8PS8m9oYtNy},
 year = {2021}
}

@article{lu_longitudinal_2003,
 author = {Lu, Xiao-Yun and Hedrick, J Karl},
 journal = {International Journal of Control},
 number = {2},
 pages = {193--202},
 title = {Longitudinal Control Algorithm for Automated Vehicle Merging},
 volume = {76},
 year = {2003}
}

@article{lu_predictive_2019,
 author = {Lu, Xingyu and Tiomkin, Stas and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {Predictive {{Coding}} for {{Boosting Deep Reinforcement Learning}} with {{Sparse Rewards}}},
 url = {https://arxiv.org/abs/1912.13414},
 volume = {abs/1912.13414},
 year = {2019}
}

@article{lu_understanding_2019,
 author = {Lu, Yiping and Li, Zhuohan and He, Di and Sun, Zhiqing and Dong, Bin and Qin, Tao and Wang, Liwei and Liu, Tie-Yan},
 journal = {ArXiv preprint},
 title = {Understanding and {{Improving Transformer From}} a {{Multi}}-{{Particle Dynamic System Point}} of {{View}}},
 url = {https://arxiv.org/abs/1906.02762},
 volume = {abs/1906.02762},
 year = {2019}
}

@article{lumer_semi-inner-product_1961,
 abstract = {Advancing research. Creating connections.},
 author = {Lumer, G.},
 doi = {10.1090/S0002-9947-1961-0133024-2},
 file = {/home/matt/Zotero/storage/5UB3C8JY/Lumer - 1961 - Semi-inner-product spaces.pdf;/home/matt/Zotero/storage/PE8GKPGQ/home.html},
 issn = {0002-9947, 1088-6850},
 journal = {Transactions of the American Mathematical Society},
 language = {en},
 number = {1},
 pages = {29--43},
 title = {Semi-Inner-Product Spaces},
 volume = {100},
 year = {1961}
}

@inproceedings{luo_adaptive_2019,
 author = {Liangchen Luo and
Yuanhao Xiong and
Yan Liu and
Xu Sun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LuoXLS19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Adaptive Gradient Methods with Dynamic Bound of Learning Rate},
 url = {https://openreview.net/forum?id=Bkg3g2R9FX},
 year = {2019}
}

@inproceedings{luo_algorithmic_2021,
 author = {Yuping Luo and
Huazhe Xu and
Yuanzhi Li and
Yuandong Tian and
Trevor Darrell and
Tengyu Ma},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/LuoXLTDM19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Algorithmic Framework for Model-based Deep Reinforcement Learning
with Theoretical Guarantees},
 url = {https://openreview.net/forum?id=BJe1E2R5KX},
 year = {2019}
}

@inproceedings{luong_effective_2015,
 address = {Lisbon, Portugal},
 author = {Luong, Thang  and
Pham, Hieu  and
Manning, Christopher D.},
 booktitle = {Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing},
 doi = {10.18653/v1/D15-1166},
 pages = {1412--1421},
 publisher = {Association for Computational Linguistics},
 title = {Effective Approaches to Attention-based Neural Machine Translation},
 url = {https://aclanthology.org/D15-1166},
 year = {2015}
}

@inproceedings{luss_support_2008,
 author = {Ronny Luss and
Alexandre d'Aspremont},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/LussD07.bib},
 booktitle = {Advances in Neural Information Processing Systems 20, Proceedings
of the Twenty-First Annual Conference on Neural Information Processing
Systems, Vancouver, British Columbia, Canada, December 3-6, 2007},
 editor = {John C. Platt and
Daphne Koller and
Yoram Singer and
Sam T. Roweis},
 pages = {953--960},
 publisher = {Curran Associates, Inc.},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Support Vector Machine Classification with Indefinite Kernels},
 url = {https://proceedings.neurips.cc/paper/2007/hash/c0c7c76d30bd3dcaefc96f40275bdc0a-Abstract.html},
 year = {2007}
}

@article{lv_traffic_2015,
 abstract = {Accurate and timely traffic flow information is important for the successful deployment of intelligent transportation systems. Over the last few years, traffic data have been exploding, and we have truly entered the era of big data for transportation. Existing traffic flow prediction methods mainly use shallow traffic prediction models and are still unsatisfying for many real-world applications. This situation inspires us to rethink the traffic flow prediction problem based on deep architecture models with big traffic data. In this paper, a novel deep-learning-based traffic flow prediction method is proposed, which considers the spatial and temporal correlations inherently. A stacked autoencoder model is used to learn generic traffic flow features, and it is trained in a greedy layerwise fashion. To the best of our knowledge, this is the first time that a deep architecture model is applied using autoencoders as building blocks to represent traffic flow features for prediction. Moreover, experiments demonstrate that the proposed method for traffic flow prediction has superior performance.},
 author = {Lv, Y. and Duan, Y. and Kang, W. and Li, Z. and Wang, F.},
 doi = {10.1109/TITS.2014.2345663},
 file = {/home/matt/Zotero/storage/K2ZGW7NE/Lv et al. - 2015 - Traffic Flow Prediction With Big Data A Deep Lear.pdf;/home/matt/Zotero/storage/MR7SQEBS/6894591.html},
 issn = {1524-9050},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {2},
 pages = {865--873},
 shorttitle = {Traffic {{Flow Prediction With Big Data}}},
 title = {Traffic {{Flow Prediction With Big Data}}: {{A Deep Learning Approach}}},
 volume = {16},
 year = {2015}
}

@inproceedings{lyle_comparative_nodate,
 author = {Clare Lyle and
Marc G. Bellemare and
Pablo Samuel Castro},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/LyleBC19.bib},
 booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
2019, The Thirty-First Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
USA, January 27 - February 1, 2019},
 doi = {10.1609/aaai.v33i01.33014504},
 pages = {4504--4511},
 publisher = {{AAAI} Press},
 timestamp = {Wed, 25 Sep 2019 01:00:00 +0200},
 title = {A Comparative Analysis of Expected and Distributional Reinforcement
Learning},
 url = {https://doi.org/10.1609/aaai.v33i01.33014504},
 year = {2019}
}

@article{lyrintzis_development_1994,
 author = {Lyrintzis, A. S. and Liu, G. and Michalopoulos, P. G.},
 journal = {Transportation Research Record},
 number = {1547},
 pages = {174--183},
 title = {Development and {{Comparative Evaluation}} of {{High}}-{{Order Traffic Flow Models}}},
 year = {1994}
}

@article{ma_dynamic_2019,
 abstract = {In this work, we utilize a dynamic Bayesian network for an inferential analysis of driving-related risks based on our assessment of real-world driving data. On-road driving tests are carried out to gather and analyze data to identify different evaluation indicators of driving-related risks. These indicators include the distance between vehicles, acceleration, steering entropy, visual distraction duration, visual glance speed, and blink frequency. Moreover, these indicators are processed to build a driving-related risk evaluation model based on the dynamic Bayesian network. The validity of this model is further tested by experimental data. The results show that this model can achieve a reasonable quantitative evaluation of driving-related risks. Vehicle operation-related risks can be further divided into four levels of safety, namely, levels I to IV. The lowest risk is observed at level I, whereas level IV has the highest risk. Among the indicators for risk evaluation, the distance between vehicles is the most sensitive control indicator of vehicle operation-related risks. The research findings provide various methodologies that could be utilized for evaluation and early warning of driving-related risks. Thus, a theoretical foundation to seek solutions for the safety of advanced driving assistance system is formed.},
 author = {Ma, Y. and Qi, S. and Fan, L. and Lu, W. and Chan, C. and Zhang, Y.},
 doi = {10.1109/ACCESS.2019.2941959},
 file = {/home/matt/Zotero/storage/QUFYAP6G/Ma et al_2019_Dynamic Bayesian Network Approach to Evaluate Vehicle Driving Risk Based on.pdf;/home/matt/Zotero/storage/J7FL76KX/8840844.html},
 journal = {IEEE Access},
 pages = {135050--135062},
 title = {Dynamic {{Bayesian Network Approach}} to {{Evaluate Vehicle Driving Risk Based}} on {{On}}-{{Road Experiment Driving Data}}},
 volume = {7},
 year = {2019}
}

@inproceedings{ma_wasserstein_2019,
 abstract = {Since prediction plays a significant role in enhancing the performance of decision making and planning procedures, the requirement of advanced methods of prediction becomes urgent. Although many literatures propose methods to make prediction on a single agent, there is still a challenging and open problem on how to make prediction for multi-agent systems. In this work, by leveraging the power of statistics and information theory, we propose a novel deep latent variable model based on Wasserstein auto-encoder, which is able to learn a complex probabilistic distribution. Models such as neural networks cannot guarantee the satisfaction of dynamic system constraints directly. Therefore, we also propose a novel generative model structure to enable our approach to satisfy the kinematic constraints automatically. We test our model on both numerical examples and a real-world application to demonstrate its accuracy and efficiency. The results show that the proposed model achieves a better prediction accuracy than the other state-of-the-art methods under common evaluation metrics. Moreover, we introduce statistics to evaluate if the generative model literally learns the interaction patterns between different agents in the environments.},
 author = {Ma, H. and Li, J. and Zhan, W. and Tomizuka, M.},
 booktitle = {2019 {{IEEE Intelligent Vehicles Symposium}} ({{IV}})},
 doi = {10.1109/IVS.2019.8813783},
 file = {/home/matt/Zotero/storage/UTQV3MY2/Ma et al_2019_Wasserstein Generative Learning with Kinematic Constraints for Probabilistic.pdf;/home/matt/Zotero/storage/76HCSPSE/8813783.html},
 pages = {2477--2483},
 title = {Wasserstein {{Generative Learning}} with {{Kinematic Constraints}} for {{Probabilistic Interactive Driving Behavior Prediction}}},
 year = {2019}
}

@inproceedings{madry_towards_2018,
 author = {Aleksander Madry and
Aleksandar Makelov and
Ludwig Schmidt and
Dimitris Tsipras and
Adrian Vladu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/MadryMSTV18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Towards Deep Learning Models Resistant to Adversarial Attacks},
 url = {https://openreview.net/forum?id=rJzIBfZAb},
 year = {2018}
}

@phdthesis{mahler_efficient_2018,
 abstract = {While humans can grasp and manipulate novel objects with ease, rapid and reliable robot grasping of a wide variety of objects is highly challenging due to sensor noise, partial observability, imprecise control, and hardware limitations.Analytic approaches to robot grasping use models from physics to predict grasp success but require precise knowledge of the robot and objects in the environment, making them well-suited for controlled industrial applications but difficult to scale to many objects.On the other hand, deep neural networks trained on large datasets of grasps labeled with empirical successes and failures can rapidly plan grasps across a diverse set of objects, but data collection is tedious, robot-specific, and prone to mislabeling.To improve the efficiency of learning deep grasping policies, we propose a hybrid method to automate dataset collection by generating millions of synthetic 3D point clouds, robot grasps, and success metrics using analytic models of contact, collision geometry, and image formation.We present the Dexterity-Network (Dex-Net), a framework for generating training datasets by analyzing mechanical models of contact forces and torques under stochastic perturbations across thousands of 3D object CAD models.We describe dataset generation models for training policies to lift and transport novel objects from a tabletop or cluttered bin using a 3D depth sensor and a parallel-jaw (two-finger) or suction cup gripper.To study the effects of learning from massive amounts of training data, we generate datasets containing millions of training examples using distributed Cloud computing, simulations, and parallel GPU processing.We use these datasets to train robust grasping policies based on Grasp Quality Convolutional Neural Networks (GQ-CNNs) that take as input a depth image and a candidate grasp with up to five degrees of freedom and predict the probability of grasp success on an object in the image.To transfer from simulation to reality, we develop novel analytic grasp success metrics based on resisting disturbing forces and torques under stochastic perturbations and bounding an object's mobility under an energy field such as gravity. In addition, we study techniques in algorithmic supervision to guide dataset collection using full knowledge of the object geometry and pose in simulation.We explore extensions to learning policies that sequentially pick novel objects from dense clutter in a bin and that can rapidly decide which gripper hardware is best in a particular scenario.To substantiate the method, we describe thousands of experimental trials on a physical robot which suggest that deep learning on synthetic Dex-Net datasets can be used to rapidly and reliably plan grasps across a diverse set of novel objects for a variety of depth sensors, robot grippers, and robot arms.Results suggest that policies trained on Dex-Net datasets can achieve up to 95\% success in picking novel objects from densely cluttered bins at a rate of over 310 mean picks per hour with no additional training or tuning on the physical system.},
 author = {Mahler, Jeffrey Brian},
 file = {/home/matt/Zotero/storage/MGRRKMZN/Mahler - 2018 - Efficient Policy Learning for Robust Robot Graspin.pdf;/home/matt/Zotero/storage/8I5CWRNG/21f0t7pd.html},
 language = {en},
 school = {UC Berkeley},
 title = {Efficient {{Policy Learning}} for {{Robust Robot Grasping}}},
 year = {2018}
}

@article{mahmassani_dyanmic_2001,
 author = {Mahmassani, H. S.},
 journal = {Networks and Spatial Economics},
 pages = {267--292},
 title = {Dyanmic Network Traffic Assignment and Simulation Methodology for Advanced System Management Applications},
 year = {2001}
}

@inproceedings{maji_classification_2008,
 author = {Subhransu Maji and
Alexander C. Berg and
Jitendra Malik},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/MajiBM08.bib},
 booktitle = {2008 {IEEE} Computer Society Conference on Computer Vision and Pattern
Recognition {(CVPR} 2008), 24-26 June 2008, Anchorage, Alaska, {USA}},
 doi = {10.1109/CVPR.2008.4587630},
 publisher = {{IEEE} Computer Society},
 timestamp = {Thu, 25 May 2017 01:00:00 +0200},
 title = {Classification using intersection kernel support vector machines is
efficient},
 url = {https://doi.org/10.1109/CVPR.2008.4587630},
 year = {2008}
}

@inproceedings{malik_derivative-free_2020,
 author = {Dhruv Malik and
Ashwin Pananjady and
Kush Bhatia and
Koulik Khamaru and
Peter L. Bartlett and
Martin J. Wainwright},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aistats/MalikPBKBW19.bib},
 booktitle = {The 22nd International Conference on Artificial Intelligence and Statistics,
{AISTATS} 2019, 16-18 April 2019, Naha, Okinawa, Japan},
 editor = {Kamalika Chaudhuri and
Masashi Sugiyama},
 pages = {2916--2925},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 08 Oct 2019 01:00:00 +0200},
 title = {Derivative-Free Methods for Policy Optimization: Guarantees for Linear
Quadratic Systems},
 url = {http://proceedings.mlr.press/v89/malik19a.html},
 volume = {89},
 year = {2019}
}

@article{malik_simple_2019,
 abstract = {Simultaneously estimating the 3D shape and pose of a hand in real time is a new and challenging computer graphics problem, which is important for animation and interactions with 3D objects in virtual environments with personalized hand shapes. CNN-based direct hand pose estimation methods are the state-of-the-art approaches, but they can only regress a 3D hand pose from a single depth image. In this study, we developed a simple and effective real-time CNN-based direct regression approach for simultaneously estimating the 3D hand shape and pose, as well as structure constraints for both egocentric and third person viewpoints by learning from the synthetic depth. In addition, we produced the first million-scale egocentric synthetic dataset called SynHandEgo, which contains egocentric depth images with accurate shape and pose annotations, as well as color segmentation of the hand parts. Our network is trained based on combined real and synthetic datasets with full supervision of the hand pose and structure constraints, and semi-supervision of the hand mesh. Our approach performed better than the state-of-the-art methods based on the SynHand5M synthetic dataset in terms of both the 3D shape and pose recovery. By learning simultaneously using real and synthetic data, we demonstrated the feasibility of hand mesh recovery from two real hand pose datasets, i.e., BigHand2.2M and NYU. Moreover, our method obtained more accurate estimates of the 3D hand poses based on the NYU dataset compared with the existing methods that output more than joint positions. The SynHandEgo dataset has been made publicly available to promote further research in the emerging domain of hand shape and pose recovery from egocentric viewpoints (https://bit.ly/2WMWM5u).},
 author = {Malik, Jameel and Elhayek, Ahmed and Nunnari, Fabrizio and Stricker, Didier},
 doi = {10.1016/j.cag.2019.10.002},
 file = {/home/matt/Zotero/storage/4AQLQPLI/Malik et al. - 2019 - Simple and effective deep hand shape and pose regr.pdf},
 issn = {00978493},
 journal = {Computers \& Graphics},
 language = {en},
 pages = {85--91},
 title = {Simple and Effective Deep Hand Shape and Pose Regression from a Single Depth Image},
 volume = {85},
 year = {2019}
}

@phdthesis{malito_deformation_2018,
 abstract = {Each year close to one millions patients within the United States, receive a total joint replacement (TJR) to alleviate pain from severe debilitating osteoarthritis. TJRs can comprise hip, knee, shoulder, and even elbow and ankle replacements. Though these implants differ in anatomical function they have a consistent theme, a hard-on-soft bearing couple consisting of hard cobalt chrome (CoCr) and soft ultra-high molecular weight polyethylene (UHMWPE). UHMWPE is a semi-crystalline polymer with 2-6 million g/mol where long molecular chains create high entanglements and help give the material high energetic toughness. These molecular characteristics also provide a low coefficient of friction desirable for TJRs. This coupling pair has been the standard of care for nearly sixty years however not without some complications. TJRs primarily fail from wear debris that is liberated from the UHMWPE bearing surface. This wear debris is caused by successive plastic deformation from implant loading leading to crack initiation below the implant surface. Crack initiation leads to fatigue crack growth with the eventual liberation of debris. As a result of this detriment, there have been several changes to the formulations that make up UHMWPE. These changes primarily include radiation cross-linking to improve wear resistance. Increased wear resistance comes with concomitant trade-offs to the mechanical properties of the material.Radiation cross-linking through gamma irradiation, introduces free radicals to the material. Free- radical need to be eliminated otherwise they will react with the body and cause the polymer to oxidize in an in vivo environment. To alleviate these free-radicals post processing is performed. This post processing usually consists of thermal annealing treatments either above or below the melt temperature of UHMWPE. More recently, UHMWPE materials have moved away from post irradiation annealing in favor of antioxidant additions to the material. These antioxidants, such as vitamin E, are added to stabilize the material after irradiation and to prevent any possibility of oxidative embrittlement during in vivo operation. All of these unique additions to UHMWPE pose the important question of how the material's fundamental mechanical properties are affected. There is a plethora of research data on the mechanical properties of UHMWPE and some of its material formulations, however when one dives into the procedural methods of these studies there are significant inconsistencies.These inconsistencies are rooted in the procedures used to analyze and create material mechanical properties. Unlike metallic materials where methods for analyzing mechanical properties are very well understood, polymeric materials offer a more complex challenge when interpreting their constitutive behavior. This is extremely important when polymeric materials, such as UHMWPE are used in safety critical applications such as TJRs. These challenges increase when UHMWPE is tailored through combinations of resin type, radiation cross-linking, and antioxidant additions. As a result there is a need to answer from a methodological perspective how the mechanical properties of UHMWPE change with different material formulations under different loading scenarios.This dissertation provides a comprehensive and thorough assessment of the mechanical properties of UHMWPE across 12 different material formulations focusing on how the methods used to analyze mechanical behavior can be extremely important. First, a comprehensive microstructural analysis is performed through differential scanning calorimetry (DSC) and small angle x-ray scattering (SAXS) to gather microstructure data for its potential effect on mechanical properties. Then tensile deformation in UHMWPE and its various material formulations are investigated. Engineering versus true tensile stress-strain data is looked at to elucidate the differences between analysis methods for determining elastic properties, yield, post yield, and ultimate behavior. Tensile constitutive properties are then compared to properties determined from compression and nanoindentation in an effort to understand material deformation trends across measurement methods. Then microstructure and tensile analysis are applied in the determination of the elastic-plastic fracture, or J-integral, toughness behavior of UHMWPE. Finally, this study concludes with a mechanistic analysis of the crack growth mechanisms to validate fracture toughness methods.},
 author = {Malito, Louis Gregory},
 file = {/home/matt/Zotero/storage/DNPLVT2Z/Malito - 2018 - The Deformation, Yielding, and Fracture of Ultra-H.pdf;/home/matt/Zotero/storage/C5UHZMLV/1wd9m59h.html},
 language = {en},
 school = {UC Berkeley},
 title = {The {{Deformation}}, {{Yielding}}, and {{Fracture}} of {{Ultra}}-{{High Molecular Weight Polyethylene}} for {{Use}} in {{Total Joint Replacements}}},
 year = {2018}
}

@inproceedings{mao_modelling_2019,
 abstract = {Modelling and exploiting teammates' policies in cooperative multi-agent systems have long been an interest and also a big challenge for the reinforcement learning (RL) community. The interest lies in the fact that if the agent knows the teammates' policies, it can adjust its own policy accordingly to arrive at proper cooperations; while the challenge is that the agents' policies are changing continuously due to they are learning concurrently, which imposes difficulty to model the dynamic policies of teammates accurately. In this paper, we present ATTention Multi-Agent Deep Deterministic Policy Gradient (ATT-MADDPG) to address this challenge. ATT-MADDPG extends DDPG, a single-agent actor-critic RL method, with two special designs. First, in order to model the teammates' policies, the agent should get access to the observations and actions of teammates. ATT-MADDPG adopts a centralized critic to collect such information. Second, to model the teammates' policies using the collected information in an effective way, ATT-MADDPG enhances the centralized critic with an attention mechanism. This attention mechanism introduces a special structure to explicitly model the dynamic joint policy of teammates, making sure that the collected information can be processed efficiently. We evaluate ATT-MADDPG on both benchmark tasks and the real-world packet routing tasks. Experimental results show that it not only outperforms the state-of-the-art RL-based methods and rule-based methods by a large margin, but also achieves better performance in terms of scalability and robustness.},
 archiveprefix = {arXiv},
 author = {Mao, Hangyu and Zhang, Zhengchao and Xiao, Zhen and Gong, Zhibo},
 booktitle = {Proceedings of the 18th {{International Conference}} on {{Autonomous Agents}} and {{Multiagent Systems}}},
 eprint = {1811.07029},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/ULMA97UR/Mao et al. - 2018 - Modelling the Dynamic Joint Policy of Teammates wi.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Modelling the {{Dynamic Joint Policy}} of {{Teammates}} with {{Attention Multi}}-Agent {{DDPG}}},
 year = {2019}
}

@article{margellos_hamiltonjacobi_2011,
 abstract = {A new framework for formulating reachability problems with competing inputs, nonlinear dynamics, and state constraints as optimal control problems is developed. Such reach-avoid problems arise in, among others, the study of safety problems in hybrid systems. Earlier approaches to reach-avoid computations are either restricted to linear systems, or face numerical difficulties due to possible discontinuities in the Hamiltonian of the optimal control problem. The main advantage of the approach proposed in this paper is that it can be applied to a general class of target-hitting continuous dynamic games with nonlinear dynamics, and has very good properties in terms of its numerical solution, since the value function and the Hamiltonian of the system are both continuous. The performance of the proposed method is demonstrated by applying it to a case study, which involves the target-hitting problem of an underactuated underwater vehicle in the presence of obstacles.},
 author = {Margellos, Kostas and Lygeros, John},
 doi = {10.1109/TAC.2011.2105730},
 file = {/home/matt/Zotero/storage/LPFMY2GE/5685555.html},
 issn = {1558-2523},
 journal = {IEEE Transactions on Automatic Control},
 number = {8},
 pages = {1849--1861},
 title = {Hamilton\textendash{{Jacobi Formulation}} for {{Reach}}\textendash{{Avoid Differential Games}}},
 volume = {56},
 year = {2011}
}

@article{martin_predicting_2020,
 author = {Martin, Charles H. and Tongsu and Peng and Mahoney, Michael W.},
 journal = {ArXiv preprint},
 title = {Predicting Trends in the Quality of State-of-the-Art Neural Networks without Access to Training or Testing Data},
 url = {https://arxiv.org/abs/2002.06716},
 volume = {abs/2002.06716},
 year = {2020}
}

@article{martini_geometry_2001,
 abstract = {We survey elementary results in Minkowski spaces (i.e. finite dimensional Banach spaces) that deserve to be collected together, and give simple proofs for some of them. We place special emphasis on planar results. Many of these results have often been rediscovered as lemmas to other results. In Part I we cover the following topics: The triangle inequality and consequences such as the monotonicity lemma, geometric characterizations of strict convexity, normality (Birkhoff orthogonality), conjugate diameters and Radon curves, equilateral triangles and the affine regular hexagon construction, equilateral sets, circles: intersection, circumscribed, characterizations, circumference and area, inscribed equilateral polygons.},
 author = {Martini, Horst and Swanepoel, Konrad J. and Wei{\ss}, Gunter},
 doi = {10.1016/S0723-0869(01)80025-6},
 file = {/home/matt/Zotero/storage/XQANE3F2/Martini et al. - 2001 - The geometry of Minkowski spaces — A survey. Part .pdf;/home/matt/Zotero/storage/WQ7YJCCV/S0723086901800256.html},
 issn = {0723-0869},
 journal = {Expositiones Mathematicae},
 language = {en},
 number = {2},
 pages = {97--142},
 title = {The Geometry of {{Minkowski}} Spaces \textemdash{} {{A}} Survey. {{Part I}}},
 volume = {19},
 year = {2001}
}

@article{martini_geometry_2004,
 abstract = {In this second part of a series of surveys on the geometry of finite dimensional Banach spaces (Minkowski spaces) we discuss results that refer to the following three topics: bodies of constant Minkowski width, generalized convexity notions that are important for Minkowski spaces, and bisectors as well as Voronoi diagrams in Minkowski spaces.},
 author = {Martini, H. and Swanepoel, K. J.},
 doi = {10.1016/S0723-0869(04)80009-4},
 file = {/home/matt/Zotero/storage/LUQILCK5/Martini and Swanepoel - 2004 - The geometry of minkowski spaces — A survey. Part .pdf;/home/matt/Zotero/storage/PCSSQKEY/S0723086904800094.html},
 issn = {0723-0869},
 journal = {Expositiones Mathematicae},
 language = {en},
 number = {2},
 pages = {93--144},
 title = {The Geometry of Minkowski Spaces \textemdash{} {{A}} Survey. {{Part II}}},
 volume = {22},
 year = {2004}
}

@book{maryland_department_of_transportation_evaluation_2006,
 author = {{Maryland Department of Transportation}},
 title = {Evaluation of the {{License Plate Recognition System}}},
 year = {2006}
}

@inproceedings{materzynska_something-else_2019,
 author = {Joanna Materzynska and
Tete Xiao and
Roei Herzig and
Huijuan Xu and
Xiaolong Wang and
Trevor Darrell},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/MaterzynskaXHXW20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.00113},
 pages = {1046--1056},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {Something-Else: Compositional Action Recognition With Spatial-Temporal
Interaction Networks},
 url = {https://doi.org/10.1109/CVPR42600.2020.00113},
 year = {2020}
}

@phdthesis{mather_market_2018,
 abstract = {Contemporary power systems are characterized by increasing penetrations of renewable and distributed energy resources (DERs), which present both opportunities and challenges for reliable system operation. Uncertainty in renewable generation must be managed over both shorter and longer timescales, necessitating greater flexibility in the supply and demand of electricity. Fortunately, this rise in renewables has been accompanied by the growth of flexible energy resources such as energy storage and aggregated demand flexibility. However, these assets are generally not adequately integrated into existing electricity market structures leading to many benefits of their flexibility going unrealized. Additionally, distributed energy resources, such as rooftop solar and electric vehicles, present a challenge to the traditional top-down management of power systems, requiring new decentralized control and market architectures to ensure their safe operation and to maximize their value. This dissertation tackles a range of questions relating to the integration of flexible and distributed resources into electricity markets in the presence of uncertainty, using techniques from control theory, game theory, multiparametric programming, and distributed optimization.The main contributions of this dissertation encompass novel analysis and design of markets, both centralized and decentralized, that explicitly integrate distributed and flexible resources, numerical methods providing exact solutions to multi-leader follower equilibrium problems among strategic bidders, and insights into the role of virtual bidders in managing demand uncertainty in two-stage markets. Chapter 1 introduces the context for the dissertation, describing trends driving the energy industry and the challenges and opportunities they pose. Current practice and existing literature are described with regard to uncertainty, flexibility, and decentralized markets and control. Chapter 2 lays out the mathematical background for the dissertation, describing models for power flow, electricity markets, and market participants, in addition to the theory of multiparametric programming. Chapter 3 demonstrates the equivalence of virtual bidding and stochastic optimization in two-stage markets under certain conditions. It also characterizes the equilibrium of a crowd of virtual bidders with heterogeneous beliefs and explores simple learning strategies for virtual bidders to reach equilibrium. Chapter 4 studies robust Cournot-Bertrand equilibria among generation firms. Firms anticipate demand and renewable uncertainty and optimize their actions to ensure their profits are robust to this uncertainty. The chapter concludes by discussing the effects on market outcomes of this behavior. Chapter 5 addresses the more general topic of strategic bidding by generation firms in electricity markets. This question involves solving non-convex bilevel optimization problems, which form part of the wider class of multi-leader follower problems. Both the single firm problem, constituting an MPEC, and the multi-firm equilibrium problem, constituting an EPEC, are solved exactly using techniques from multiparametric programming. This latter contribution, in particular, represents a significant advance over current methods, generalizing the solution of supply function equilibrium problems to cases with asymmetric players and transmission constraints. Chapter 6 analyzes a number of regulatory models for the integration of energy storage into wholesale electricity markets, including Open Access Storage, and investigates the implications and incentives of a variety of storage ownership structures under each model. Chapter 7 demonstrates the potential of load flexibility for congestion relief, defining the notion of a congestion-free dispatch. Chapter 8 describes the design of a decentralized coordination mechanism for DERs in a microgrid using blockchain technology. The implementation uses ADMM with a smart contract on the blockchain serving as the ADMM coordinator. Chapter 9 illustrates the design of an open-gate forward market with specific flexibility products for DERs, allowing users to hedge better against uncertainty and correctly express and maximize the value of their flexibility. A number of algorithms are presented to address the combinatorial scheduling and pricing problem involved with flexible loads.},
 author = {Mather, Jonathan William},
 file = {/home/matt/Zotero/storage/LJP6JCCV/Mather - 2018 - Market Design and Analysis for Uncertain, Flexible.pdf;/home/matt/Zotero/storage/EFSPJHI8/6dq291zg.html},
 language = {en},
 school = {UC Berkeley},
 title = {Market {{Design}} and {{Analysis}} for {{Uncertain}}, {{Flexible}}, and {{Decentralized Power Systems}}},
 year = {2018}
}

@article{mazumdar_gradient-based_2020,
 abstract = {We introduce a general framework for competitive gradient-based learning that encompasses a wide breadth of multiagent learning algorithms, and analyze the limiting behavior of competitive gradientbased learning algorithms using dynamical systems theory. For both general-sum and potential games, we characterize a nonnegligible subset of the local Nash equilibria that will be avoided if each agent employs a gradient-based learning algorithm. We also shed light on the issue of convergence to non-Nash strategies in general- and zero-sum games, which may have no relevance to the underlying game, and arise solely due to the choice of algorithm. The existence and frequency of such strategies may explain some of the difficulties encountered when using gradient descent in zero-sum games as, e.g., in the training of generative adversarial networks. To reinforce the theoretical contributions, we provide empirical results that highlight the frequency of linear quadratic dynamic games (a benchmark for multiagent reinforcement learning) that admit global Nash equilibria that are almost surely avoided by policy gradient.},
 author = {Mazumdar, Eric and Ratliff, Lillian J. and Sastry, S. Shankar},
 doi = {10.1137/18M1231298},
 file = {/home/matt/Zotero/storage/QLWIKY5V/Mazumdar et al. - 2020 - On Gradient-Based Learning in Continuous Games.pdf},
 issn = {2577-0187},
 journal = {SIAM Journal on Mathematics of Data Science},
 language = {en},
 number = {1},
 pages = {103--131},
 title = {On {{Gradient}}-{{Based Learning}} in {{Continuous Games}}},
 volume = {2},
 year = {2020}
}

@incollection{mcfadden_conditional_1973,
 address = {{New York}},
 author = {McFadden, Daniel},
 booktitle = {Frontiers in {{Econometrics}}},
 editor = {Zarembka, P.},
 file = {/home/matt/Documents/Papers/mcfadden_conditional_logit.pdf},
 pages = {105--142},
 publisher = {{Academic Press}},
 title = {Conditional {{Logit Analysis}} of {{Qualitative Choice Behavior}}},
 year = {1973}
}

@article{mckeown_achieving_1999,
 author = {McKeown, N. and Mekkittikul, A. and Anantharam, V. and Walrand, J.},
 journal = {IEEE Trans. Communications},
 number = {8},
 pages = {1260--1267},
 title = {Achieving 100 Percent Throughput in an Input-Queued Switch},
 volume = {47},
 year = {1999}
}

@article{mckeown_scheduling_1993,
 author = {McKeown, N. and Varaiya, P. and Walrand, J.},
 journal = {Electronic Letters},
 number = {25},
 pages = {2174--2175},
 title = {Scheduling Cells in an Input-Buffered Switch},
 volume = {29},
 year = {1993}
}

@book{mcmillan_regional_2006,
 author = {McMillan, T.},
 title = {Regional {{High}}-{{Occupancy}}/{{Toll}} ({{HOT}}) {{Lane Network Study Preliminary Results}}},
 year = {2006}
}

@article{mehr_game_2018,
 author = {Mehr, Negar and Li, Ruolin and Horowitz, Roberto},
 journal = {ArXiv preprint},
 title = {A {{Game Theoretic Macroscopic Model}} of {{Bypassing}} at {{Traffic Diverges}} with {{Applications}} to {{Mixed Autonomy Networks}}},
 url = {https://arxiv.org/abs/1809.02762},
 volume = {abs/1809.02762},
 year = {2018}
}

@article{mehr_how_2019,
 abstract = {It is known that connected and autonomous vehicles are capable of maintaining shorter headway and distances when they form platoons of vehicles. Thus, such technologies can potentially increase the road capacities of traffic networks. Consequently, it is envisioned that their deployment will also increase the overall network mobility. In this paper, we examine the validity of this expected impact, assuming that drivers select their routes selfishly, in traffic networks with mixed vehicle autonomy, i.e. traffic networks with both regular and autonomous vehicles. We consider a nonatomic routing game on a network with inelastic (fixed) demands for a set of network O/D pairs, and study how replacing a fraction of regular vehicles by autonomous vehicles will affect the mobility of the network. Using well known US bureau of public roads (BPR) traffic delay models, we show that the resulting Wardrop equilibrium is not necessarily unique for networks with mixed autonomy. Then, we state the conditions under which the total network delay at equilibrium is guaranteed to decrease as the fraction of autonomous vehicles increases. However, we show that when these conditions do not hold, counter},
 author = {Mehr, N. and Horowitz, R.},
 doi = {10.1109/TCNS.2019.2918682},
 file = {/home/matt/Zotero/storage/PJ5WTJZE/Mehr and Horowitz - 2019 - How Will the Presence of Autonomous Vehicles Affec.pdf;/home/matt/Zotero/storage/P3RIUNY7/8721089.html},
 issn = {2325-5870},
 journal = {IEEE Transactions on Control of Network Systems},
 pages = {1--1},
 title = {How {{Will}} the {{Presence}} of {{Autonomous Vehicles Affect}} the {{Equilibrium State}} of {{Traffic Networks}}?},
 year = {2019}
}

@inproceedings{mehr_probabilistic_2016,
 author = {Mehr, Negar and Sadigh, Dorsa and Horowitz, Roberto},
 doi = {10.1109/ACC.2016.7525023},
 file = {/home/matt/Zotero/storage/VEJ8J5GK/07525023.pdf},
 isbn = {978-1-4673-8682-1},
 pages = {880--880},
 publisher = {{IEEE}},
 title = {Probabilistic Controller Synthesis for Freeway Traffic Networks},
 year = {2016}
}

@inproceedings{mei_neural_2017,
 author = {Hongyuan Mei and
Jason Eisner},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/MeiE17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {6754--6764},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {The Neural Hawkes Process: {A} Neurally Self-Modulating Multivariate
Point Process},
 url = {https://proceedings.neurips.cc/paper/2017/hash/6463c88460bd63bbe256e495c63aa40b-Abstract.html},
 year = {2017}
}

@article{mendis_goslp_2018,
 abstract = {Modern microprocessors are equipped with single instruction multiple data (SIMD) or vector instruction sets which allow compilers to exploit superword level parallelism (SLP), a type of fine-grained parallelism. Current SLP auto-vectorization techniques use heuristics to discover vectorization opportunities in high-level language code. These heuristics are fragile, local and typically only present one vectorization strategy that is either accepted or rejected by a cost model. We present goSLP, a novel SLP auto-vectorization framework which solves the statement packing problem in a pairwise optimal manner. Using an integer linear programming (ILP) solver, goSLP searches the entire space of statement packing opportunities for a whole function at a time, while limiting total compilation time to a few minutes. Furthermore, goSLP optimally solves the vector permutation selection problem using dynamic programming. We implemented goSLP in the LLVM compiler infrastructure, achieving a geometric mean speedup of 7.58\% on SPEC2017fp, 2.42\% on SPEC2006fp and 4.07\% on NAS benchmarks compared to LLVM's existing SLP auto-vectorizer.},
 author = {Mendis, Charith and Amarasinghe, Saman},
 doi = {10.1145/3276480},
 file = {/home/matt/Zotero/storage/PDZDPCVJ/Mendis and Amarasinghe - 2018 - goSLP globally optimized superword level parallel.pdf},
 issn = {2475-1421},
 journal = {Proceedings of the ACM on Programming Languages},
 language = {en},
 number = {OOPSLA},
 pages = {1--28},
 shorttitle = {{{goSLP}}},
 title = {{{goSLP}}: Globally Optimized Superword Level Parallelism Framework},
 volume = {2},
 year = {2018}
}

@inproceedings{mendonca_guided_2019,
 author = {Russell Mendonca and
Abhishek Gupta and
Rosen Kralev and
Pieter Abbeel and
Sergey Levine and
Chelsea Finn},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/Mendonca0KALF19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {9653--9664},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Guided Meta-Policy Search},
 url = {https://proceedings.neurips.cc/paper/2019/hash/d324a0cc02881779dcda44a675fdcaaa-Abstract.html},
 year = {2019}
}

@article{menendez_effects_2007,
 author = {Menendez, Monica and Daganzo, Carlos F.},
 doi = {10.1016/j.trb.2007.03.001},
 file = {/home/matt/Zotero/storage/RN9N84F5/2008_TRB_effects_of_hov_on_bottlenecks.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {8},
 pages = {809--822},
 title = {Effects of {{HOV}} Lanes on Freeway Bottlenecks},
 volume = {41},
 year = {2007}
}

@article{menendez_m._and_c._daganzo_assessment_2004,
 author = {{Menendez, M. and C. Daganzo}},
 journal = {Transportation Research Record},
 title = {Assessment of the Impact of Incidents near Bottlenecks: {{Strategies}} to Reduce Delay},
 year = {2004}
}

@article{mennucci_asymmetric_2013,
 abstract = {In this paper we discuss asymmetric length structures and asymmetric metric spaces. A length structure induces a (semi)distance function; by using the total variation formula, a (semi)distance function induces a length. In the first part we identify a topology in the set of paths that best describes when the above operations are idempotent. As a typical application, we consider the length of paths defined by a Finslerian functional in Calculus of Variations.},
 author = {Mennucci, Andrea C.G.},
 doi = {10.2478/agms-2013-0004},
 file = {/home/matt/Zotero/storage/CDZGMHTX/Mennucci - 2013 - On Asymmetric Distances.pdf},
 issn = {2299-3274},
 journal = {Analysis and Geometry in Metric Spaces},
 language = {en},
 pages = {200--231},
 title = {On {{Asymmetric Distances}}},
 volume = {1},
 year = {2013}
}

@inproceedings{mesquita_rethinking_2020,
 author = {Diego P. P. Mesquita and
Amauri H. Souza Jr. and
Samuel Kaski},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/MesquitaSK20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Rethinking pooling in graph neural networks},
 url = {https://proceedings.neurips.cc/paper/2020/hash/1764183ef03fc7324eb58c3842bd9a57-Abstract.html},
 year = {2020}
}

@article{messmer_metanet_1990,
 author = {Messmer, A. and Papageorgiou, M.},
 journal = {Traffic Engineering and Control},
 number = {8/9},
 pages = {466--470},
 title = {{{METANET}}: {{A}} Macroscopic Simulation Program for Motorway Networks.},
 volume = {31},
 year = {1990}
}

@misc{metropolitan_transportation_commission_bay_2019,
 author = {{Metropolitan Transportation Commission}},
 howpublished = {http://bayareaexpresslanes.org},
 title = {Bay {{Area Express Lanes}}},
 year = {2019}
}

@article{mezzadri_how_2007,
 author = {Mezzadri, Francesco},
 journal = {ArXiv preprint},
 title = {How to Generate Random Matrices from the Classical Compact Groups},
 url = {https://arxiv.org/abs/m},
 volume = {abs/m},
 year = {20m}
}

@inproceedings{micchelli_function_2004,
 author = {Charles A. Micchelli and
Massimiliano Pontil},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/colt/MicchelliP04.bib},
 booktitle = {Learning Theory, 17th Annual Conference on Learning Theory, {COLT}
2004, Banff, Canada, July 1-4, 2004, Proceedings},
 doi = {10.1007/978-3-540-27819-1\_18},
 editor = {John Shawe{-}Taylor and
Yoram Singer},
 pages = {255--269},
 publisher = {Springer},
 series = {Lecture Notes in Computer Science},
 timestamp = {Sun, 21 May 2017 01:00:00 +0200},
 title = {A Function Representation for Learning in Banach Spaces},
 url = {https://doi.org/10.1007/978-3-540-27819-1\_18},
 volume = {3120},
 year = {2004}
}

@article{michalaka_simulating_2013,
 abstract = {Microscopic simulation is critical for evaluating the operation strategies of managed lanes. However, most existing tools are limited in their ability to simulate dynamic tolling strategies of managed lanes, particularly those with multiple segments. Three sets of modeling components are developed in this paper to demonstrate simulation of high-occupancy toll (HOT) lane operations. The first component implements three pricing strategies: responsive pricing; a closed-loop, control-based algorithm; and time-of-day pricing. The second component mimics drivers' lane choice behaviors in the presence of tolls, and the third represents different toll structures for multisegment HOT lane facilities. An enhanced version of CORSIM, which contains these new modeling components, is validated by simulation experiments involving the 95 Express network in South Florida.},
 author = {Michalaka, Dimitra and Yin, Yafeng and Hale, David},
 doi = {10.3141/2396-14},
 file = {/home/matt/Zotero/storage/SUN3URVB/Michalaka et al. - 2013 - Simulating High-Occupancy Toll Lane Operations.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 language = {en},
 number = {1},
 pages = {124--132},
 title = {Simulating {{High}}-{{Occupancy Toll Lane Operations}}},
 volume = {2396},
 year = {2013}
}

@article{mihaylova_freeway_2007,
 author = {Mihaylova, Lyudmila and Boel, Ren{\'e} and Hegyi, Andreas},
 doi = {10.1016/j.automatica.2006.08.023},
 file = {/home/matt/Zotero/storage/ITX4EJ6U/Mihaylova_PF.pdf},
 issn = {00051098},
 journal = {Automatica},
 language = {en},
 number = {2},
 pages = {290--300},
 title = {Freeway Traffic Estimation within Particle Filtering Framework},
 volume = {43},
 year = {2007}
}

@inproceedings{mikolov_linguistic_2013,
 address = {Atlanta, Georgia},
 author = {Mikolov, Tomas  and
Yih, Wen-tau  and
Zweig, Geoffrey},
 booktitle = {Proceedings of the 2013 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies},
 pages = {746--751},
 publisher = {Association for Computational Linguistics},
 title = {Linguistic Regularities in Continuous Space Word Representations},
 url = {https://aclanthology.org/N13-1090},
 year = {2013}
}

@article{milanes_cooperative_2014,
 author = {Milanes, Vicente and Shladover, S. E. and Spring, John and Nowakowski, Christopher and Kawazoe, Hiroshi and Nakamura, Masahide},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 pages = {296--305},
 title = {Cooperative {{Adaptive Cruise Control}} in {{Real Traffic Situations}}},
 volume = {15},
 year = {2014}
}

@book{miller_complex_2007,
 address = {{Princeton, N.J}},
 author = {Miller, John H. and Page, Scott E.},
 isbn = {978-0-691-12702-6 978-0-691-13096-5},
 lccn = {H61.25 .M55 2007},
 publisher = {{Princeton University Press}},
 series = {Princeton Studies in Complexity},
 shorttitle = {Complex Adaptive Systems},
 title = {Complex Adaptive Systems: An Introduction to Computational Models of Social Life},
 year = {2007}
}

@article{miller_settings_1963,
 abstract = {A formula is derived for the average delay to vehicles at junctions controlled by fixed-cycle traffic signals. The predicted delays are close to those observed in practice. Optimum signal settings are then derived using the delay formula.},
 author = {Miller, A. J.},
 journal = {Operations Research},
 keywords = {},
 number = {4},
 pages = {373--386},
 title = {Settings for Fixed-Cycle Traffic Signals},
 volume = {14},
 year = {1963}
}

@book{minsky_perceptrons_1969,
 address = {{Cambridge, Massachusetts}},
 annotation = {OCLC: 833070641},
 author = {Minsky, Marvin and Papert, Seymour A.},
 file = {/home/matt/Zotero/storage/8BNIEYID/Minsky and Papert - 1972 - Perceptrons an introduction to computational geom.pdf},
 isbn = {978-0-262-13043-1 978-0-262-63022-1},
 language = {eng},
 publisher = {{The MIT Press}},
 shorttitle = {Perceptrons},
 title = {Perceptrons: An Introduction to Computational Geometry},
 year = {1969}
}

@article{mirchandani_queuing_2007,
 author = {Mirchandani, P. B. and Zou, N.},
 journal = {IEEE Trans. Intelligent Transportation Systems},
 number = {1},
 pages = {50--59},
 title = {Queuing {{Models}} for {{Analysis}} of {{Traffic Adaptive Signal Control}}},
 volume = {8},
 year = {2007}
}

@article{mirchandani_real-time_2001,
 author = {Mirchandani, P. and Head, L.},
 journal = {Transportation Research, Part C},
 pages = {415--432},
 title = {A Real-Time Traffic Signal Control System: Architecture, Algorithms, and Analysis},
 volume = {9},
 year = {2001}
}

@article{mirhoseini_chip_2020,
 author = {Mirhoseini, Azalia and Goldie, Anna and Yazgan, Mustafa and Jiang, Joe and Songhori, Ebrahim and Wang, Shen and Lee, Young-Joon and Johnson, Eric and Pathak, Omkar and Bae, Sungmin and Nazi, Azade and Pak, Jiwoo and Tong, Andy and Srinivasa, Kavya and Hang, William and Tuncer, Emre and Babu, Anand and Le, Quoc V. and Laudon, James and Ho, Richard and Carpenter, Roger and Dean, Jeff},
 journal = {ArXiv preprint},
 title = {Chip {{Placement}} with {{Deep Reinforcement Learning}}},
 url = {https://arxiv.org/abs/2004.10746},
 volume = {abs/2004.10746},
 year = {2020}
}

@inproceedings{mirhoseini_hierarchical_2018,
 author = {Azalia Mirhoseini and
Anna Goldie and
Hieu Pham and
Benoit Steiner and
Quoc V. Le and
Jeff Dean},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/MirhoseiniGPSLD18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {A Hierarchical Model for Device Placement},
 url = {https://openreview.net/forum?id=Hkc-TeZ0W},
 year = {2018}
}

@article{mishalani_uniform_1995,
 author = {Mishalani, R. G. and Koutsopoulos, H. N.},
 journal = {Journal of Infrastructure Systems},
 number = {1},
 pages = {44--55},
 title = {Uniform {{Infrastructure Fields}}: {{Definition}} and {{Identification}}},
 volume = {1},
 year = {1995}
}

@book{mitchell_complexity_2009,
 address = {{New York, NY}},
 author = {Mitchell, Melanie},
 isbn = {978-0-19-512441-5},
 publisher = {{Oxford University Press}},
 title = {Complexity: {{A Guided Tour}}},
 year = {2009}
}

@techreport{mitchell_need_1980,
 address = {{New Jersey, USA}},
 author = {Mitchell, Tom M},
 file = {/home/matt/Zotero/storage/9VV3VMZ4/Mitchell - The Need for Biases in Learning Generalizations.pdf},
 institution = {{Rutgers University, Department of Computer Science}},
 keywords = {⛔ No DOI found},
 language = {en},
 number = {CBM-TR-117},
 title = {The {{Need}} for {{Biases}} in {{Learning Generalizations}}},
 year = {1980}
}

@inproceedings{mobahi_self-distillation_2020,
 author = {Hossein Mobahi and
Mehrdad Farajtabar and
Peter L. Bartlett},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/MobahiFB20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Self-Distillation Amplifies Regularization in Hilbert Space},
 url = {https://proceedings.neurips.cc/paper/2020/hash/2288f691b58edecadcc9a8691762b4fd-Abstract.html},
 year = {2020}
}

@inproceedings{monti_geometric_2017,
 author = {Federico Monti and
Davide Boscaini and
Jonathan Masci and
Emanuele Rodol{\`{a}} and
Jan Svoboda and
Michael M. Bronstein},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/MontiBMRSB17.bib},
 booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
 doi = {10.1109/CVPR.2017.576},
 pages = {5425--5434},
 publisher = {{IEEE} Computer Society},
 timestamp = {Tue, 14 Nov 2017 00:00:00 +0100},
 title = {Geometric Deep Learning on Graphs and Manifolds Using Mixture Model
CNNs},
 url = {https://doi.org/10.1109/CVPR.2017.576},
 year = {2017}
}

@inproceedings{monti_geometric_2017-1,
 author = {Federico Monti and
Michael M. Bronstein and
Xavier Bresson},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/MontiBB17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {3697--3707},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Geometric Matrix Completion with Recurrent Multi-Graph Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2017/hash/2eace51d8f796d04991c831a07059758-Abstract.html},
 year = {2017}
}

@article{moon_multi-target_2005,
 author = {Moon, Il-ki and Yi, Kyongsu and Caveney, Derek and Hedrick, J Karl},
 journal = {Journal of mechanical science and technology},
 number = {9},
 pages = {1742--1752},
 title = {A Multi-Target Tracking Algorithm for Application to Adaptive Cruise Control},
 volume = {19},
 year = {2005}
}

@inproceedings{mordatch_emergence_2018,
 author = {Igor Mordatch and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/MordatchA18.bib},
 booktitle = {Proceedings of the Thirty-Second {AAAI} Conference on Artificial Intelligence,
(AAAI-18), the 30th innovative Applications of Artificial Intelligence
(IAAI-18), and the 8th {AAAI} Symposium on Educational Advances in
Artificial Intelligence (EAAI-18), New Orleans, Louisiana, USA, February
2-7, 2018},
 editor = {Sheila A. McIlraith and
Kilian Q. Weinberger},
 pages = {1495--1502},
 publisher = {{AAAI} Press},
 timestamp = {Mon, 22 Oct 2018 01:00:00 +0200},
 title = {Emergence of Grounded Compositional Language in Multi-Agent Populations},
 url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI18/paper/view/17007},
 year = {2018}
}

@article{morgan_synchronizing_1964,
 author = {Morgan, J. and Little, J.},
 journal = {Operations Research},
 number = {6},
 pages = {896--912},
 title = {Synchronizing Traffic Signals for Maximum Bandwidth},
 volume = {12},
 year = {1964}
}

@inproceedings{moritz_ray_2018,
 abstract = {The next generation of AI applications will continuously interact with the environment and learn from these interactions. These applications impose new and demanding systems requirements, both in terms of performance and flexibility. In this paper, we consider these requirements and present Ray\textemdash a distributed system to address them. Ray implements a unified interface that can express both task-parallel and actor-based computations, supported by a single dynamic execution engine. To meet the performance requirements, Ray employs a distributed scheduler and a distributed and fault-tolerant store to manage the system's control state. In our experiments, we demonstrate scaling beyond 1.8 million tasks per second and better performance than existing specialized systems for several challenging reinforcement learning applications.},
 archiveprefix = {arXiv},
 author = {Moritz, Philipp and Nishihara, Robert and Wang, Stephanie and Tumanov, Alexey and Liaw, Richard and Liang, Eric and Elibol, Melih and Yang, Zongheng and Paul, William and Jordan, Michael I. and Stoica, Ion},
 booktitle = {13th {{USENIX Symposium}} on {{Operating Systems Design}} and {{Implementation}}},
 eprint = {1712.05889},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/IA8TUHZM/Moritz et al. - 2017 - Ray A Distributed Framework for Emerging AI Appli.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {561--577},
 shorttitle = {Ray},
 title = {Ray: {{A Distributed Framework}} for {{Emerging AI Applications}}},
 year = {2018}
}

@techreport{mortazavi_travel_2009,
 author = {Mortazavi, A. and Pan, X. and Jun, E. and Odioso, M},
 institution = {{California Center for Innovative Transportation, University of California, Berkeley}},
 number = {UCB-ITS-CWP-2009-2},
 title = {Travel {{Times}} on {{Changeable Message Signs Volume II}} \textemdash{} {{Evaluation}} of {{Transit Message Signs}}},
 year = {2009}
}

@article{motamedi_acceptance_2019,
 abstract = {Objective: This study aims to develop user acceptance models for two concepts of full driving automation: personally owned and shared use. Background: Many manufacturers have been investing considerably in and actively developing full driving automation. However, factors influencing user acceptance of full driving automation are not yet fully understood. Method: This study consisted of two parts: focus group discussions and online surveys. A total of 30 potential users participated in focus groups to discuss their perception of full driving automation acceptance. Based on the findings from focus group discussions, theoretical foundations, and empirical evidence, we hypothesized the acceptance models for both personally owned and shared-use concepts. We tested the models with 310 and 250 participants, respectively, online. Results: The results of focus groups indicated that users' concerns are centered around safety, usefulness, compatibility, trust, and ease of use. The survey results revealed the important roles of perceived usefulness and perceived safety in both models, whereas the direct impact of perceived ease of use was found to be insignificant. The indirect impact of perceived ease of use was less significant in the personally owned than in the shared-use model, whereas usefulness, trust, and compatibility played more important roles in the personally owned when compared with the shared-use model. Conclusion: The findings uncovered a chain of constructs that affect behavioral intention to use for both full driving automation concepts.},
 author = {Motamedi, Sanaz and Wang, Pei and Zhang, Tingting and Chan, Ching-Yao},
 doi = {10.1177/0018720819870658},
 file = {/home/matt/Zotero/storage/6T7SNJIT/Motamedi et al. - 2019 - Acceptance of Full Driving Automation Personally .pdf},
 issn = {0018-7208, 1547-8181},
 journal = {Human Factors: The Journal of the Human Factors and Ergonomics Society},
 language = {en},
 pages = {001872081987065},
 shorttitle = {Acceptance of {{Full Driving Automation}}},
 title = {Acceptance of {{Full Driving Automation}}: {{Personally Owned}} and {{Shared}}-{{Use Concepts}}},
 year = {2019}
}

@article{mounce_convergence_2006,
 author = {Mounce, R.},
 journal = {Transportation Research, Part B},
 pages = {779--791},
 title = {Convergence in a Continuous Dynamic Queueing Model for Traffic Networks},
 volume = {40},
 year = {2006}
}

@article{mozaffari_deep_2019,
 author = {Mozaffari, Sajjad and {Al-Jarrah}, Omar Y. and Dianati, Mehrdad and Jennings, Paul and Mouzakitis, Alexandros},
 journal = {ArXiv preprint},
 title = {Deep {{Learning}}-Based {{Vehicle Behaviour Prediction For Autonomous Driving Applications}}: {{A Review}}},
 url = {https://arxiv.org/abs/1912.11676},
 volume = {abs/1912.11676},
 year = {2019}
}

@article{mozaffari_deep_2020,
 author = {Mozaffari, Sajjad and {Al-Jarrah}, Omar Y. and Dianati, Mehrdad and Jennings, Paul and Mouzakitis, Alexandros},
 doi = {10.1109/TITS.2020.3012034},
 file = {/home/matt/Zotero/storage/UF7BERXH/Mozaffari et al. - 2020 - Deep Learning-Based Vehicle Behavior Prediction fo.pdf},
 issn = {1524-9050, 1558-0016},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 pages = {1--15},
 shorttitle = {Deep {{Learning}}-{{Based Vehicle Behavior Prediction}} for {{Autonomous Driving Applications}}},
 title = {Deep {{Learning}}-{{Based Vehicle Behavior Prediction}} for {{Autonomous Driving Applications}}: {{A Review}}},
 year = {2020}
}

@inproceedings{muller_when_2019,
 author = {Rafael M{\"{u}}ller and
Simon Kornblith and
Geoffrey E. Hinton},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/MullerKH19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {4696--4705},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {When does label smoothing help?},
 url = {https://proceedings.neurips.cc/paper/2019/hash/f1748d6b0fd9d439f71450117eba2725-Abstract.html},
 year = {2019}
}

@article{munjal_propagation_1971,
 author = {Munjal, P. K. and Pipes, L. A.},
 doi = {http://dx.doi.org/10.1016/0041-1647(71)90036-0},
 issn = {0041-1647},
 journal = {Transportation Research},
 number = {4},
 pages = {241--255},
 title = {Propagation of On-Ramp Density Perturbations on Unidirectional Two- and Three-Lane Freeways},
 volume = {5},
 year = {1971}
}

@article{munnell_policy_1992,
 abstract = {In the late 1980s, David Aschauer (1989) triggered a long overdue dialogue among economists and political leaders when he published a study arguing that much of the decline in U.S. productivity that occurred in the 1970s was precipitated by declining rates of public capital investment. My own work confirmed these results (Munnell, 1990a). Spending advocates seized on these findings as support for increased public investment. The enthusiasm among policymakers for the early Aschauer results was matched, if not surpassed, by skepticism on the part of many economists. Critics of these studies charged that the methodology was flawed, that the direction of causation between public investment and output growth is unclear and that, even if the historical empirical relationships were estimated correctly, they provide no clear indications for current policy. Who's right? What do we know and not know about the link between public infrastructure and productivity? And what are the implications of these results for policy?},
 author = {Munnell, Alicia H.},
 doi = {10.1257/jep.6.4.189},
 file = {/home/matt/Zotero/storage/TYMPV2NQ/Munnell - 1992 - Policy Watch Infrastructure Investment and Econom.pdf;/home/matt/Zotero/storage/P4256QLD/articles.html},
 issn = {0895-3309},
 journal = {Journal of Economic Perspectives},
 language = {en},
 number = {4},
 pages = {189--198},
 shorttitle = {Policy {{Watch}}},
 title = {Policy {{Watch}}: {{Infrastructure Investment}} and {{Economic Growth}}},
 volume = {6},
 year = {1992}
}

@article{munoz_bottleneck_2002,
 author = {Munoz, Juan Carlos and Daganzo, Carlos F.},
 journal = {Transportation research part A, Policy and practice},
 number = {6},
 pages = {483--505},
 title = {The Bottleneck Mechanism of a Freeway Diverge},
 volume = {36A},
 year = {2002}
}

@inproceedings{munoz_traffic_2003,
 author = {Munoz, L. and Sun, X. and Horowitz, R. and Alvarez, A.},
 booktitle = {Proceedings of {{American Control Conference}}},
 title = {Traffic Density Estimation with the Cell Transmission Model},
 volume = {5},
 year = {2003}
}

@phdthesis{munsing_optimization_2018,
 abstract = {This dissertation develops an interdisciplinary approach to integrating renewable energy resources into energy markets, using tools from optimization theory, power systems, and economics. It advances prior work with the development of a set of tools for securing distributed and fully-decentralized optimization problems, including both algorithmic guards against attacks by malicious nodes, and system architectures which can enable decentralized security checks. Leveraging the emerging technologies of blockchains and smart contracts, it develops a new paradigm of blockchain-secured distributed optimization, demonstrated with simulation of a microgrid which is able to securely operate without oversight from a utility or central operator.As the goal of interdisciplinary research is to show mastery of each field and extend current knowledge by exploring their intersection, the chapters of this dissertation are designed to support that goal:\textbullet{} Chapter 1 provides background on the technical challenges of integrating high amounts of renewable energy into the electricity system, and discusses technologies and policies which can address those challenges.\textbullet{} Chapter 2 introduces the idea of applying optimization tools to energy systems by studying a small-scale energy harvesting system in which batteries and capacitors are used to meet a defined load, and constraints force the use of nonlinear optimization techniques.\textbullet{} Chapter 3 explores how large-scale energy storage systems can be designed and sited to maximize profits from participating in wholesale energy markets, using a linear program which demonstrates how convex optimization tools can be united with energy market data to create scalable tools for modeling large networks.\textbullet{} Chapter 4 expands the study of market-based models by examining the strategic operation of generation resources on a congested network. We use game theory to model participants' behavior, power flow models to reflect the underlying constraints of the physical network, and robust convex optimization to explore how uncertainty is integrated into decision-making.\textbullet{} Chapter 5 discusses how decentralized optimization models can facilitate scalable optimization tools, and explores the security risks which these optimization models introduce. Tools for detection and mitigation of attacks are explored and tested on a simple problem. Potential architectures for securing decentralized optimization are explored, including blockchains and smart contracts.\textbullet{} Chapter 6 extends this approach by developing a blockchain-secured fully-decentralized optimization for a microgrid dispatch problem, coordinating distributed energy resources. By demonstrating the usefulness of this blockchain-secured optimization model, this culminating chapter shows how difficult optimization models can be scalably solved in a manner which respects privacy while guaranteeing security.\textbullet{} The Appendices present tutorial material on the tools used throughout the paper, and are supplemented by the code in the author's github repository: https://github.com/emunsing/tutorials},
 author = {Munsing, Eric},
 file = {/home/matt/Zotero/storage/B6F2G3ND/Munsing - 2018 - Optimization Tools for Constrained Energy Markets.pdf;/home/matt/Zotero/storage/TPK7VW4S/5wr8t03d.html},
 language = {en},
 school = {UC Berkeley},
 title = {Optimization {{Tools}} for {{Constrained Energy Markets}}},
 year = {2018}
}

@inproceedings{muralidharan_freeway_2009,
 author = {Muralidharan, A. and Dervisoglu, G. and Horowitz, R.},
 booktitle = {Proc. of the 2009 {{American Control Conference}}},
 doi = {10.1109/ACC.2009.5160597},
 pages = {2916--2921},
 title = {Freeway Traffic Flow Simulation Using the {{Link Node Cell}} Transmission Model},
 year = {2009}
}

@article{muralidharan_imputation_2009,
 abstract = {The Tools for Operational Planning is a suite of tools that uses the link\textendash node cell transmission model for macroscopic freeway traffic simulations for specifying operational strategies such as ramp metering and demand and incident management. Traffic flow and occupancy data from loop detectors are used for calibrating these models and specifying the inputs to the simulation. Flow data from ramps, however, are often found to be missing or incorrect. This paper elaborates an imputation procedure used to determine these ramp flows. This automated imputation procedure is based on an adaptive identification technique that attempts to minimize the error between the simulated and the measured densities. Simulation results using the imputed flow data indicate good conformation with loop detector measurements.},
 author = {Muralidharan, Ajith and Horowitz, Roberto},
 doi = {10.3141/2099-07},
 file = {/home/matt/Zotero/storage/56PLX8NP/Muralidharan and Horowitz - 2009 - Imputation of Ramp Flow Data for Freeway Traffic S.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record},
 language = {en},
 number = {1},
 pages = {58--64},
 title = {Imputation of {{Ramp Flow Data}} for {{Freeway Traffic Simulation}}},
 volume = {2099},
 year = {2009}
}

@phdthesis{muralidharan_tools_2012,
 abstract = {This dissertation presents algorithmic tools that are useful to transportation engineers for freeway traffic modeling and control. A modeling framework that utilizes the link-node cell transmission model (LN-CTM) to simulate traffic dynamics on a chosen freeway network is presented here. A data driven approach, which utilizes available detector measurements on the freeway network to calibrate and specify the model is also illustrated. Flow measurements in ramps, which are needed to specify demands and routing characteristics for the freeway, are usually not available. Two novel imputation algorithms which estimate the missing ramp flows in the freeway network are presented. These algorithms employ a model based estimation procedure, that calculates the unknown on-ramp flows and off-ramp split ratios which can be fed into the model to match the observed mainline density and flow measurements. A detailed analysis of the convergence of these algorithms is presented, along with the advantages of these individual approaches. The final model, specified with the imputed ramp flows is able to replicate the traffic dynamics with good accuracy, as seen by error rates around 5-8\% for density/flows contours, and the accurate replication of the bottleneck locations. These imputation algorithms, used within our modeling framework, enables a user to build a freeway model simulating multiple days of freeway behavior, within a week.A model based optimal predictive controller for freeway congestion control, which utilizes the LN-CTM as its underlying model is also presented. The approach searches for solutions represented by a combination of ramp metering and variable speed limits. The optimization problem corresponding to the optimal control problem based on the LN-CTM is non-convex and non-linear. A relaxation method is presented to solve this problem efficiently using an equivalent linear program, before generating the solution to the original problem using a new mapping algorithm. The predictive controller is also extended to cover situations when ramp weaving and/or capacity drop exists in the freeway network. In this case, a set of heuristics are presented and the optimal control problem is solved using a sequence of linear programs, before mapping the solutions back to the original problem.},
 author = {Muralidharan, Ajith},
 file = {/home/matt/Zotero/storage/ZGLMPJ9C/Muralidharan - 2012 - Tools for modeling and control of freeway networks.pdf;/home/matt/Zotero/storage/ZSUWUA24/7995d36h.html},
 language = {en},
 school = {UC Berkeley},
 title = {Tools for Modeling and Control of Freeway Networks},
 year = {2012}
}

@article{murphy_dempster-shafer_1998,
 author = {Murphy, Robin R.},
 file = {/home/matt/Zotero/storage/QVWXJ3GZ/00681240.pdf},
 journal = {Robotics and Automation, IEEE Transactions on},
 number = {2},
 pages = {197--206},
 title = {Dempster-{{Shafer}} Theory for Sensor Fusion in Autonomous Mobile Robots},
 volume = {14},
 year = {1998}
}

@inproceedings{murray_naiad_2013,
 abstract = {Naiad is a distributed system for executing data parallel, cyclic dataflow programs. It offers the high throughput of batch processors, the low latency of stream processors, and the ability to perform iterative and incremental computations. Although existing systems offer some of these features, applications that require all three have relied on multiple platforms, at the expense of efficiency, maintainability, and simplicity. Naiad resolves the complexities of combining these features in one framework. A new computational model, timely dataflow, underlies Naiad and captures opportunities for parallelism across a wide class of algorithms. This model enriches dataflow computation with timestamps that represent logical points in the computation and provide the basis for an efficient, lightweight coordination mechanism.},
 address = {{Farminton, Pennsylvania}},
 author = {Murray, Derek G. and McSherry, Frank and Isaacs, Rebecca and Isard, Michael and Barham, Paul and Abadi, Mart{\'i}n},
 booktitle = {Proceedings of the {{Twenty}}-{{Fourth ACM Symposium}} on {{Operating Systems Principles}} - {{SOSP}} '13},
 doi = {10.1145/2517349.2522738},
 file = {/home/matt/Zotero/storage/8CUW75GS/Murray et al. - 2013 - Naiad a timely dataflow system.pdf},
 isbn = {978-1-4503-2388-8},
 language = {en},
 pages = {439--455},
 publisher = {{ACM Press}},
 shorttitle = {Naiad},
 title = {Naiad: A Timely Dataflow System},
 year = {2013}
}

@article{myers_ond_1986,
 author = {Myers, E. W.},
 journal = {Algorithmica},
 pages = {251--266},
 title = {An {{O}}({{ND}}) Difference Algorithm and Its Variations},
 volume = {1},
 year = {1986}
}

@inproceedings{nagel_traffic_1994,
 author = {Nagel, Kai and Rasmussen, Steen},
 booktitle = {Artificial {{Life IV}}: {{Proceedings}} of the {{Fourth International Workshop}} on the {{Synthesis}} and {{Simulation}} of {{Living Systems}}},
 file = {/home/matt/Zotero/storage/7KQL6E8B/download.pdf},
 pages = {222--235},
 publisher = {{MIT Press}},
 title = {Traffic at the Edge of Chaos},
 volume = {4},
 year = {1994}
}

@article{nar_persistency_2019,
 author = {Nar, Kamil and Sastry, S. Shankar},
 journal = {ArXiv preprint},
 title = {Persistency of {{Excitation}} for {{Robustness}} of {{Neural Networks}}},
 url = {https://arxiv.org/abs/1911.01043},
 volume = {abs/1911.01043},
 year = {2019}
}

@book{national_traffic_operations_coalition_2007_2007,
 author = {{National Traffic Operations Coalition}},
 title = {2007 {{National Traffic Report Card}}},
 year = {2007}
}

@book{national_traffic_operations_coalition_2012_2012,
 author = {{National Traffic Operations Coalition}},
 title = {2012 {{National Traffic Report Card}}},
 year = {2012}
}

@article{neely_dynamic_2005,
 author = {Neely, M. J. and Modiano, E. and Rohrs, C. E.},
 journal = {IEEE Journal on Selected Areas in Communications},
 number = {1},
 pages = {89--103},
 title = {Dynamic Power Allocation and Routing for Time-Varying Wireless Networks},
 volume = {23},
 year = {2005}
}

@inproceedings{nemati_non-linear_2014,
 author = {Nemati, Alireza and Kumar, Manish},
 booktitle = {{{ASME}} 2014 {{Dynamic Systems}} and {{Control Conference}}},
 file = {/home/matt/Zotero/storage/WJK5HATR/V003T48A005-DSCC2014-6293.pdf},
 pages = {V003T48A005--V003T48A005},
 publisher = {{American Society of Mechanical Engineers}},
 title = {Non-{{Linear Control}} of {{Tilting}}-{{Quadcopter Using Feedback Linearization Based Motion Control}}},
 year = {2014}
}

@article{neubig_neural_2017,
 author = {Neubig, Graham},
 journal = {ArXiv preprint},
 title = {Neural {{Machine Translation}} and {{Sequence}}-to-Sequence {{Models}}: {{A Tutorial}}},
 url = {https://arxiv.org/abs/1703.01619},
 volume = {abs/1703.01619},
 year = {2017}
}

@inproceedings{NEURIPS2020_b6af2c97,
 author = {Tianlong Chen and
Jonathan Frankle and
Shiyu Chang and
Sijia Liu and
Yang Zhang and
Zhangyang Wang and
Michael Carbin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/ChenFC0ZWC20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {The Lottery Ticket Hypothesis for Pre-trained {BERT} Networks},
 url = {https://proceedings.neurips.cc/paper/2020/hash/b6af2c9703f203a2794be03d443af2e3-Abstract.html},
 year = {2020}
}

@article{newell_approximation_1965,
 author = {Newell, G. F.},
 journal = {SIAM Review},
 number = {2},
 pages = {223--240},
 title = {Approximation Methods for Queues with Application to the Fixed-Cycle Traffic Light},
 volume = {7},
 year = {1965}
}

@article{newell_morning_nodate,
 author = {Newell, G. F.},
 journal = {Transportation Science},
 number = {},
 pages = {74--88},
 title = {The Morning Commute for Nonidentical Travelers},
 volume = {1987},
 year = {21}
}

@article{newell_simplified_1993,
 abstract = {For a freeway having various entrance and exit ramps, the methods described in Part I are used to relate the cumulative flow curve at any junction to the net cumulative entrance flow at this junction, and the cumulative flow curves for the freeway at the next upstream junction and/ or the next downstream junction. If the type of flow-density relations typical of freeway traffic are idealized by a triangular shaped curve with only two wave speeds, one for free-flowing traffic (positive) and the other for congested traffic (negative), then the relationship is easy to evaluate. The cumulative flow curve at the junction is simply the lower envelope of a translation of the cumulative curve from upstream and a different translation of the cumulative curve from downstream. This relationship is the basic building block for a freeway flow prediction model described in Part III.},
 author = {Newell, G. F.},
 doi = {10.1016/0191-2615(93)90039-D},
 file = {/home/matt/Zotero/storage/WC6GGZQ5/Newell - 1993 - A simplified theory of kinematic waves in highway .pdf;/home/matt/Zotero/storage/Q5QM29GL/019126159390039D.html},
 issn = {0191-2615},
 journal = {Transportation Research Part B: Methodological},
 number = {4},
 pages = {289--303},
 shorttitle = {A Simplified Theory of Kinematic Waves in Highway Traffic, Part {{II}}},
 title = {A Simplified Theory of Kinematic Waves in Highway Traffic, Part {{II}}: {{Queueing}} at Freeway Bottlenecks},
 volume = {27},
 year = {1993}
}

@article{neyman_problem_1933,
 author = {Neyman, Jerzy and Pearson, Egon S},
 journal = {Philosophical Transactions of the Royal Society of London A},
 pages = {289--337},
 title = {On the Problem of the Most Efficient Test of Statistical Hypotheses},
 volume = {231},
 year = {1933}
}

@article{neyman_testing_1933,
 author = {Neyman, Jerzy and Pearson, Egon S},
 journal = {Proceedings of the Cambridge Philosophical Society},
 pages = {492--510},
 title = {The Testing of Statistical Hypotheses in Relation to Probabilites a Priori},
 volume = {29},
 year = {1933}
}

@article{neyman_use_1928,
 author = {Neyman, Jerzy and Pearson, Egon S},
 journal = {Biometrika},
 pages = {175--240},
 title = {On the Use and Interpretation of Certain Test Criteria for Purposes of Statistical Inference: {{Part I}}},
 volume = {20A},
 year = {1928}
}

@inproceedings{ng_bev-seg_2020,
 abstract = {Bird's-eye-view (BEV) is a powerful and widely adopted representation for road scenes that captures surrounding objects and their spatial locations, along with overall context in the scene. In this work, we focus on bird's eye semantic segmentation, a task that predicts pixel-wise semantic segmentation in BEV from side RGB images. This task is made possible by simulators such as Carla, which allow for cheap data collection, arbitrary camera placements, and supervision in ways otherwise not possible in the real world. There are two main challenges to this task: the view transformation from side view to bird's eye view, as well as transfer learning to unseen domains. Existing work transforms between views through fully connected layers and transfer learns via GANs. This suffers from a lack of depth reasoning and performance degradation across domains. Our novel 2-staged perception pipeline explicitly predicts pixel depths and combines them with pixel semantics in an efficient manner, allowing the model to leverage depth information to infer objects' spatial locations in the BEV. In addition, we transfer learning by abstracting high-level geometric features and predicting an intermediate representation that is common across different domains. We publish a new dataset called BEVSEG-Carla and show that our approach improves state-of-the-art by 24\% mIoU and performs well when transferred to a new domain.},
 archiveprefix = {arXiv},
 author = {Ng, Mong H. and Radia, Kaahan and Chen, Jianfei and Wang, Dequan and Gog, Ionel and Gonzalez, Joseph E.},
 booktitle = {{{CVPR}} 2020 {{Workshop}} on {{Scalability}} in {{Autonomous Driving}}},
 eprint = {2006.11436},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/32NR4UVE/Ng et al. - 2020 - BEV-Seg Bird's Eye View Semantic Segmentation Usi.pdf;/home/matt/Zotero/storage/H8QLKNZM/2006.html},
 shorttitle = {{{BEV}}-{{Seg}}},
 title = {{{BEV}}-{{Seg}}: {{Bird}}'s {{Eye View Semantic Segmentation Using Geometry}} and {{Semantic Point Cloud}}},
 year = {2020}
}

@inproceedings{ng_facebook_nodate,
 address = {Florence, Italy},
 author = {Ng, Nathan  and
Yee, Kyra  and
Baevski, Alexei  and
Ott, Myle  and
Auli, Michael  and
Edunov, Sergey},
 booktitle = {Proceedings of the Fourth Conference on Machine Translation (Volume 2: Shared Task Papers, Day 1)},
 doi = {10.18653/v1/W19-5333},
 pages = {314--319},
 publisher = {Association for Computational Linguistics},
 title = {{F}acebook {FAIR}{'}s {WMT}19 News Translation Task Submission},
 url = {https://aclanthology.org/W19-5333},
 year = {2019}
}

@article{ngoduy_calibration_2012,
 author = {Ngoduy, D. and Maher, M.J.},
 doi = {10.1016/j.trc.2012.02.007},
 file = {/home/matt/Zotero/storage/VA2DDTAX/ngodyu_crossentropy_2ndorder_calib.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {102--121},
 title = {Calibration of Second Order Traffic Models Using Continuous Cross Entropy Method},
 volume = {24},
 year = {2012}
}

@inproceedings{nguyen_tree-structured_2020,
 author = {Xuan{-}Phi Nguyen and
Shafiq R. Joty and
Steven C. H. Hoi and
Richard Socher},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/NguyenJHS20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Fri, 17 Jul 2020 01:00:00 +0200},
 title = {Tree-Structured Attention with Hierarchical Accumulation},
 url = {https://openreview.net/forum?id=HJxK5pEYvr},
 year = {2020}
}

@techreport{nhtsa_crash_2010,
 author = {{NHTSA}},
 institution = {{National Highway Traffic Safety Administration}},
 number = {DOT HS 811 366},
 title = {Crash {{Factors}} in {{Intersection}}-{{Related Crashes}}: {{An On}}-{{Scene Perspective}}},
 year = {2010}
}

@article{ni_simplified_2005,
 author = {Ni, Daiheng and Leonard, John D.},
 doi = {10.1016/j.apm.2005.02.008},
 file = {/home/matt/Zotero/storage/77ZACHRI/ni_leonard_merge_2005.pdf},
 issn = {0307904X},
 journal = {Applied Mathematical Modelling},
 language = {en},
 number = {11},
 pages = {1054--1072},
 title = {A Simplified Kinematic Wave Model at a Merge Bottleneck},
 volume = {29},
 year = {2005}
}

@article{nichols_google_2013,
 author = {Nichols, S.},
 journal = {TechRadar},
 title = {Google Wants Some Form of Self-Driving Cars on Roads by 2018},
 year = {2013}
}

@techreport{nichols_quality_2004,
 abstract = {virtual weigh stations in Indiana were found to be approximately 55 times more effective than the static weigh stations for overweight truck identification. require a high level of WIM data accuracy and reliability},
 author = {Nichols, A. and Bullock, D.},
 institution = {{Purdue University}},
 number = {FHWA/IN/JTRP-2004/12},
 title = {Quality {{Control Procedures}} for {{Weigh}}-in-{{Motion Data}}},
 year = {2004}
}

@article{nie_comparative_2005,
 author = {Nie, Xiaojian and Zhang, H Michael},
 journal = {Networks and Spatial Economics},
 number = {1},
 pages = {89--115},
 title = {A Comparative Study of Some Macroscopic Link Models Used in Dynamic Traffic Assignment},
 volume = {5},
 year = {2005}
}

@article{nie_quasi-oracle_2017,
 author = {Nie, Xinkun and Wager, Stefan},
 journal = {ArXiv preprint},
 title = {Quasi-{{Oracle Estimation}} of {{Heterogeneous Treatment Effects}}},
 url = {https://arxiv.org/abs/1712.04912},
 volume = {abs/1712.04912},
 year = {2017}
}

@article{nihan_aid_1997,
 author = {Nihan, N.},
 journal = {Journal Of Transportation Engineering},
 number = {6},
 pages = {454--458},
 title = {Aid {{To Determining Freeway Metering Rates And Detecting Loop Errors}}},
 volume = {123},
 year = {1997}
}

@misc{noauthor_blandin_sequential_data_assim.pdf_nodate,
 file = {/home/matt/Documents/Papers/blandin_sequential_data_assim.pdf.pdf},
 title = {Blandin\_sequential\_data\_assim.Pdf}
}

@book{noauthor_california_nodate,
 title = {California {{Highway Patrol Incident}} Website}
}

@book{noauthor_caltrans_nodate,
 title = {Caltrans Today}
}

@book{noauthor_i-15sr-163_2003,
 annotation = {Published: Caltrans website},
 title = {I-15({{SR}}-163 to {{SR}}-78): {{Operational}} Improvements and Managed Lanes},
 year = {2003}
}

@book{noauthor_i-5/i-805_2003,
 annotation = {Published: Caltrans website},
 title = {I-5/{{I}}-805 Widening Project},
 year = {2003}
}

@book{noauthor_mapping_2018,
 address = {{New York, NY}},
 edition = {1st edition},
 file = {/home/matt/Zotero/storage/M9SQBFR5/2018 - Mapping China's 'one belt one road' initiative.pdf},
 isbn = {978-3-319-92200-3},
 language = {en},
 number = {13996},
 publisher = {{Springer Science+Business Media}},
 series = {International Political Economy Series},
 title = {Mapping {{China}}'s 'one Belt One Road' Initiative},
 year = {2018}
}

@article{noauthor_sir_2006,
 file = {/home/matt/Zotero/storage/G5S42UB9/2006 - The SIR model and the Foundations of Public Health.pdf},
 language = {en},
 number = {1},
 pages = {17},
 title = {The {{SIR}} Model and the {{Foundations}} of {{Public Health}}},
 year = {2006}
}

@misc{noauthor_torch.nn_nodate,
 file = {/home/matt/Zotero/storage/L5BGFHDA/nn.html},
 howpublished = {https://pytorch.org/docs/stable/nn.html\#bceloss},
 title = {Torch.Nn \textemdash{} {{PyTorch}} Master Documentation}
}

@book{northrop_introduction_2011,
 address = {{Boca Raton}},
 author = {Northrop, Robert B.},
 isbn = {978-1-4398-3901-0},
 lccn = {Q175.32.C65 N67 2011},
 publisher = {{CRC Press}},
 title = {Introduction to Complexity and Complex Systems},
 year = {2011}
}

@inproceedings{nunzio_arterial_2015,
 author = {Nunzio, Giovanni De and Gomes, Gabriel and {\noopsort{wit}}de Wit, Carlos Canudas and Horowitz, Roberto and Moulin, Philippe},
 booktitle = {{{IEEE Conference}} on {{Decision}} and {{Control}}},
 title = {Arterial {{Bandwidth}} and {{Energy Consumption Optimization}} via {{Signal Offsets Control}} and {{Variable Speed Limits}}},
 year = {2015}
}

@article{obenberger_managed_2004,
 annotation = {Publication Number FHWA-HRT-05-002},
 author = {Obenberger, Jon},
 journal = {Public Roads},
 number = {3},
 pages = {48--55},
 title = {Managed {{Lanes}}: {{Combining Access Control}}, {{Vehicle Eligibility}}, and {{Pricing Strategies Can Help Mitigate Congestion}} and {{Improve Mobility}} on the {{Nation}}'s {{Busiest Roadways}}},
 volume = {68},
 year = {2004}
}

@inproceedings{oglic_learning_2018,
 abstract = {We formulate a novel regularized risk minimization problem for learning in reproducing kernel Kre\textasciibreve\i n spaces and show that the strong representer theorem applies to it. As a result of the latter, the learning problem can be expressed as the minimization of a quadratic form over a hypersphere of constant radius. We present an algorithm that can find a globally optimal solution to this nonconvex optimization problem in time cubic in the number of instances. Moreover, we derive the gradient of the solution with respect to its hyperparameters and, in this way, provide means for efficient hyperparameter tuning. The approach comes with a generalization bound expressed in terms of the Rademacher complexity of the corresponding hypothesis space. The major advantage over standard kernel methods is the ability to learn with various domain specific similarity measures for which positive definiteness does not hold or is difficult to establish. The approach is evaluated empirically using indefinite kernels defined on structured as well as vectorial data. The empirical results demonstrate a superior performance of our approach over the state-of-the-art baselines.},
 author = {Oglic, Dino and G{\"a}rtner, Thomas},
 booktitle = {Proceedings of the 35th {{International Conference}} on {{Machine Learning}}},
 file = {/home/matt/Zotero/storage/MBARHD9T/Oglic and Gärtner - 2018 - Learning in Reproducing Kernel Kreı̆n Spaces.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {3859--3867},
 publisher = {{PMLR}},
 title = {Learning in {{Reproducing Kernel Kre{\u \i}n Spaces}}},
 volume = {80},
 year = {2018}
}

@inproceedings{oglic_scalable_2019,
 abstract = {We provide the first mathematically complete derivation of the Nystr\"om method for low-rank approximation of indefinite kernels and propose an efficient method for finding an approximate eigendecomposition of such kernel matrices. Building on this result, we devise highly scalable methods for learning in reproducing kernel Kre\textasciibreve\i n spaces. The devised approaches provide a principled and theoretically well-founded means to tackle large scale learning problems with indefinite kernels. The main motivation for our work comes from problems with structured representations (e.g., graphs, strings, time-series), where it is relatively easy to devise a pairwise (dis)similarity function based on intuition and/or knowledge of domain experts. Such functions are typically not positive definite and it is often well beyond the expertise of practitioners to verify this condition. The effectiveness of the devised approaches is evaluated empirically using indefinite kernels defined on structured and vectorial data representations.},
 author = {Oglic, Dino and G{\"a}rtner, Thomas},
 booktitle = {Proceedings of the 36th {{International Conference}} on {{Machine Learning}}},
 file = {/home/matt/Zotero/storage/6SICWHQK/Oglic and Gärtner - Scalable Learning in Reproducing Kernel Kreın Spac.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {4912--4921},
 publisher = {{PMLR}},
 title = {Scalable {{Learning}} in {{Reproducing Kernel Kre{\u \i}n Spaces}}},
 volume = {97},
 year = {2019}
}

@article{oh_real-time_2002,
 author = {Oh, C. and Ritchie, S. G.},
 journal = {Transportation Research Record},
 number = {1802},
 pages = {97--104},
 title = {Real-{{Time Inductive}}-{{Signature}}-{{Based Level}} of {{Service}} for {{Signalized Intersections}}},
 year = {2002}
}

@inproceedings{okuno_probabilistic_2018,
 author = {Akifumi Okuno and
Tetsuya Hada and
Hidetoshi Shimodaira},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/OkunoHS18.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {3885--3894},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {A probabilistic framework for multi-view feature learning with many-to-many
associations via neural networks},
 url = {http://proceedings.mlr.press/v80/okuno18a.html},
 volume = {80},
 year = {2018}
}

@article{olazaran_sociological_1996,
 author = {Olazaran, Mikel},
 doi = {10.1177/030631296026003005},
 file = {/home/matt/Zotero/storage/RE369M4Y/Olazaran - 1996 - A Sociological Study of the Official History of th.pdf},
 journal = {Social Studies of Science},
 language = {en},
 number = {3},
 pages = {611--659},
 title = {A {{Sociological Study}} of the {{Official History}} of the {{Perceptrons Controversy}}},
 volume = {26},
 year = {1996}
}

@article{oliver_traffic_1961,
 author = {Oliver, Robert M.},
 doi = {10.1287/opre.9.6.802},
 file = {/home/matt/Zotero/storage/HZ66Z2R3/oliver_traffic_counting_distribution.pdf},
 issn = {0030-364X, 1526-5463},
 journal = {Operations Research},
 language = {en},
 number = {6},
 pages = {802--810},
 title = {A {{Traffic Counting Distribution}}},
 volume = {9},
 year = {1961}
}

@techreport{on-road_automated_driving_orad_committee_taxonomy_2018,
 author = {{On-Road Automated Driving (ORAD) committee}},
 doi = {10.4271/J3016_201806},
 file = {/home/matt/Zotero/storage/YY5YZGQ8/J3016_201806.pdf},
 institution = {{SAE International}},
 language = {en},
 number = {J3016\_201806},
 title = {Taxonomy and {{Definitions}} for {{Terms Related}} to {{Driving Automation Systems}} for {{On}}-{{Road Motor Vehicles}}},
 year = {2018}
}

@inproceedings{ong_learning_2004,
 author = {Cheng Soon Ong and
Xavier Mary and
St{\'{e}}phane Canu and
Alexander J. Smola},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/OngMCS04.bib},
 booktitle = {Machine Learning, Proceedings of the Twenty-first International Conference
{(ICML} 2004), Banff, Alberta, Canada, July 4-8, 2004},
 doi = {10.1145/1015330.1015443},
 editor = {Carla E. Brodley},
 publisher = {{ACM}},
 series = {{ACM} International Conference Proceeding Series},
 timestamp = {Tue, 06 Nov 2018 00:00:00 +0100},
 title = {Learning with non-positive kernels},
 url = {https://doi.org/10.1145/1015330.1015443},
 volume = {69},
 year = {2004}
}

@article{oord_wavenet_2016,
 author = {{\noopsort{oord}}van den Oord, Aaron and Dieleman, Sander and Zen, Heiga and Simonyan, Karen and Vinyals, Oriol and Graves, Alex and Kalchbrenner, Nal and Senior, Andrew and Kavukcuoglu, Koray},
 journal = {ArXiv preprint},
 title = {{{WaveNet}}: {{A Generative Model}} for {{Raw Audio}}},
 url = {https://arxiv.org/abs/1609.03499},
 volume = {abs/1609.03499},
 year = {2016}
}

@article{orosz_exciting_2009-2,
 author = {Orosz, G{\'a}bor and Wilson, R. Eddie and Szalai, R{\'o}bert and St{\'e}p{\'a}n, G{\'a}bor},
 doi = {10.1103/PhysRevE.80.046205},
 file = {/home/matt/Zotero/storage/FS2Q9C5H/Orosz et al. - 2009 - Exciting traffic jams Nonlinear phenomena behind .pdf},
 issn = {1539-3755, 1550-2376},
 journal = {Physical Review E},
 language = {en},
 number = {4},
 pages = {046205},
 shorttitle = {Exciting Traffic Jams},
 title = {Exciting Traffic Jams: {{Nonlinear}} Phenomena behind Traffic Jam Formation on Highways},
 volume = {80},
 year = {2009}
}

@article{orosz_traffic_2010,
 author = {Orosz, G{\'a}bor and Wilson, R. Eddie and St{\'e}p{\'a}n, G{\'a}bor},
 doi = {10.1098/rsta.2010.0205},
 file = {/home/matt/Zotero/storage/2QLCDEG5/Orosz et al. - 2010 - Traffic jams dynamics and control.pdf},
 issn = {1364-503X, 1471-2962},
 journal = {Philosophical Transactions of the Royal Society A: Mathematical, Physical and Engineering Sciences},
 language = {en},
 number = {1928},
 pages = {4455--4479},
 shorttitle = {Traffic Jams},
 title = {Traffic Jams: Dynamics and Control},
 volume = {368},
 year = {2010}
}

@article{osorio_analytic_2009,
 author = {Osorio, C. and Bierlaire, M.},
 journal = {European Journal of Operational Research},
 pages = {996--1007},
 title = {An Analytic Finite Capacity Queueing Network Model Capturing the Propagation of Congestion and Blocking},
 volume = {196},
 year = {2009}
}

@inproceedings{osorio_multiple_2008,
 abstract = {excellent literature review},
 author = {Osorio, C. and Bierlaire, M.},
 booktitle = {Swiss {{Transport Research Conference}}},
 title = {A Multiple Model Approach for Traffic Signal Optimization in the City of {{Lausanne}}},
 year = {2008}
}

@inproceedings{ott_fairseq_2019,
 address = {Minneapolis, Minnesota},
 author = {Ott, Myle  and
Edunov, Sergey  and
Baevski, Alexei  and
Fan, Angela  and
Gross, Sam  and
Ng, Nathan  and
Grangier, David  and
Auli, Michael},
 booktitle = {Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics (Demonstrations)},
 doi = {10.18653/v1/N19-4009},
 pages = {48--53},
 publisher = {Association for Computational Linguistics},
 title = {fairseq: A Fast, Extensible Toolkit for Sequence Modeling},
 url = {https://aclanthology.org/N19-4009},
 year = {2019}
}

@incollection{owen_importance_2013,
 author = {Owen, Art B.},
 booktitle = {Monte {{Carlo}} Theory, Methods and Examples},
 title = {Importance Sampling},
 year = {2013}
}

@article{paden_survey_2016,
 abstract = {Self-driving vehicles are a maturing technology with the potential to reshape mobility by enhancing the safety, accessibility, efficiency, and convenience of automotive transportation. Safety-critical tasks that must be executed by a self-driving vehicle include planning of motions through a dynamic environment shared with other vehicles and pedestrians, and their robust executions via feedback control. The objective of this paper is to survey the current state of the art on planning and control algorithms with particular regard to the urban setting. A selection of proposed techniques is reviewed along with a discussion of their effectiveness. The surveyed approaches differ in the vehicle mobility model used, in assumptions on the structure of the environment, and in computational requirements. The side by side comparison presented in this survey helps to gain insight into the strengths and limitations of the reviewed approaches and assists with system level design choices.},
 author = {Paden, Brian and Cap, Michal and Yong, Sze Zheng and Yershov, Dmitry and Frazzoli, Emilio},
 doi = {10.1109/TIV.2016.2578706},
 file = {/home/matt/Zotero/storage/QYL3TNMG/Paden et al. - 2016 - A Survey of Motion Planning and Control Techniques.pdf},
 issn = {2379-8904, 2379-8858},
 journal = {IEEE Transactions on Intelligent Vehicles},
 language = {en},
 number = {1},
 pages = {33--55},
 title = {A {{Survey}} of {{Motion Planning}} and {{Control Techniques}} for {{Self}}-{{Driving Urban Vehicles}}},
 volume = {1},
 year = {2016}
}

@article{pagani_power_2013,
 abstract = {The statistical tools of Complex Network Analysis are of useful to understand salient properties of complex systems, may these be natural or pertaining human engineered infrastructures. One of these that is receiving growing attention for its societal relevance is that of electricity distribution. In this paper, we present a survey of the most relevant scientific studies investigating the properties of different Power Grids~infrastructures using Complex Network Analysis~techniques and methodologies. We categorize and explore the most relevant literature works considering general topological properties, physical properties, and differences between the various graph-related indicators and reliability aspects. We also trace the evolution in such field of the approach of study during the years to see the improvement achieved in the analysis.},
 author = {Pagani, Giuliano Andrea and Aiello, Marco},
 doi = {10.1016/j.physa.2013.01.023},
 file = {/home/matt/Zotero/storage/CKCHLBLV/Pagani and Aiello - 2013 - The Power Grid as a complex network A survey.pdf;/home/matt/Zotero/storage/TRRZAFI4/S0378437113000575.html},
 issn = {0378-4371},
 journal = {Physica A: Statistical Mechanics and its Applications},
 number = {11},
 pages = {2688--2700},
 shorttitle = {The {{Power Grid}}~as a Complex Network},
 title = {The {{Power Grid}}~as a Complex Network: {{A}} Survey},
 volume = {392},
 year = {2013}
}

@article{paganini_congestion_2005,
 author = {Paganini, F. and Wang, Z. and Doyle, J. C. and Low, S. H.},
 journal = {IEEE/ACM Transactions On Networking},
 number = {1},
 pages = {43--56},
 title = {Congestion {{Control}} for {{High Performance}}, {{Stability}}, and {{Fairness}} in {{General Networks}}},
 volume = {13},
 year = {2005}
}

@inproceedings{Pan_2019_CVPR_Workshops,
 author = {Pan, Xinlei and Chakraborty, Rudrasis and Yu, Stella},
 booktitle = {The {{IEEE}} Conference on Computer Vision and Pattern Recognition ({{CVPR}}) Workshops},
 title = {Visual Similarity from Optimizing Feature and Memory on a Hypersphere},
 year = {2019}
}

@inproceedings{pan_2d_2021,
 author = {Xingang Pan and
Bo Dai and
Ziwei Liu and
Chen Change Loy and
Ping Luo},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/PanDLLL21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Fri, 05 Nov 2021 00:00:00 +0100},
 title = {Do 2D GANs Know 3D Shape? Unsupervised 3D Shape Reconstruction from
2D Image GANs},
 url = {https://openreview.net/forum?id=FGqiDsBUKL0},
 year = {2021}
}

@article{pan_risk_2019,
 author = {Pan, Xinlei and Seita, Daniel and Gao, Yang and Canny, John},
 journal = {ArXiv preprint},
 title = {Risk {{Averse Robust Adversarial Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1904.00511},
 volume = {abs/1904.00511},
 year = {2019}
}

@inproceedings{pan_semantic_2019-2,
 abstract = {Visual anticipation of ego and object motion over a short time horizons is a key feature of human-level performance in complex environments. We propose a driving policy learning framework that predicts feature representations of future visual inputs; our predictive model infers not only future events but also semantics, which provide a visual explanation of policy decisions. Our Semantic Predictive Control (SPC) framework predicts future semantic segmentation and events by aggregating multi-scale feature maps. A guidance model assists action selection and enables efficient sampling-based optimization. Experiments on multiple simulation environments show that networks which implement SPC can outperform existing modelbased reinforcement learning algorithms in terms of data efficiency and total rewards while providing clear explanations for the policy's behavior.},
 address = {{Montreal, QC, Canada}},
 author = {Pan, Xinlei and Chen, Xiangyu and Cai, Qizhi and Canny, John and Yu, Fisher},
 booktitle = {2019 {{International Conference}} on {{Robotics}} and {{Automation}} ({{ICRA}})},
 doi = {10.1109/ICRA.2019.8794437},
 file = {/home/matt/Zotero/storage/NJAYFGQF/Pan et al. - 2019 - Semantic Predictive Control for Explainable and Ef.pdf},
 isbn = {978-1-5386-6027-0},
 language = {en},
 pages = {3203--3209},
 publisher = {{IEEE}},
 title = {Semantic {{Predictive Control}} for {{Explainable}} and {{Efficient Policy Learning}}},
 year = {2019}
}

@inproceedings{pan_visual_2019,
 abstract = {Supervised learning of classification from annotated images develops a latent feature representation that captures semantic visual similarity. We propose an unsupervised metric learning method that develops apparent visual similarity from images alone. Our method maps highdimensional visual data onto a low-dimensional hypersphere and consolidate such feature representations into a visual memory representation. Optimizing the feature mapping and visual memory on a hypersphere achieves maximal discrimination among instances. Our formulation and solution is not only more principled in theory than closely related unsupervised instance discrimination algorithms, but also better in practice in terms of classification accuracy, convergence rate, and feature transferability. We also show that our learned feature can be very useful for vision-based reinforcement learning tasks to improve sample efficiency.},
 author = {Pan, Xinlei and Chakraborty, Rudrasis and Yu, Stella},
 booktitle = {The {{IEEE}} Conference on Computer Vision and Pattern Recognition ({{CVPR}}) Workshops},
 file = {/home/matt/Zotero/storage/8W9S5Z4W/Pan et al. - Visual Similarity from Optimizing Feature and Memo.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Visual {{Similarity}} from {{Optimizing Feature}} and {{Memory On A Hypersphere}}},
 year = {2019}
}

@article{panda_multiple_2019,
 author = {Panda, Manoj and Ngoduy, Dong and Vu, Hai L.},
 doi = {10.1016/j.trb.2019.06.009},
 file = {/home/matt/Zotero/storage/VP2E4N87/10.1016@j.trb.2019.06.009-1.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {280--306},
 title = {Multiple Model Stochastic Filtering for Traffic Density Estimation on Urban Arterials},
 volume = {126},
 year = {2019}
}

@article{pant_mesh_2002,
 author = {Pant, Aniruddha and Seiler, Peter and Hedrick, Karl},
 journal = {IEEE Transactions on Automatic Control},
 number = {2},
 pages = {403--407},
 title = {Mesh Stability of Look-Ahead Interconnected Systems},
 volume = {47},
 year = {2002}
}

@techreport{papadimitriou_brain_2019,
 abstract = {Abstract                        Assemblies are large populations of neurons believed to imprint memories, concepts, words and other cognitive information. We identify             a repertoire of operations             on assemblies. These operations correspond to properties of assemblies observed in experiments, and can be shown, analytically and through simulations, to be realizable by generic, randomly connected populations of neurons with Hebbian plasticity and inhibition. Operations on assemblies include: projection (duplicating an assembly by creating a new assembly in a downstream brain area); reciprocal projection (a variant of projection also entailing synaptic connectivity from the newly created assembly to the original one); association (increasing the overlap of two assemblies in the same brain area to reflect cooccurrence or similarity of the corresponding concepts); merge (creating a new assembly with ample synaptic connectivity to and from two existing ones); and pattern-completion (firing of an assembly, with some probability, in response to the firing of some but not all of its neurons). Our analytical results establishing the plausibility of these operations are proved in a simplified mathematical model of cortex: a finite set of brain areas each containing             n             excitatory neurons, with             random             connectivity that is both recurrent (within an area) and afferent (between areas). Within one area and at any time, only             k             of the             n             neurons fire \textemdash{} an assumption that models inhibition and serves to define both assemblies and areas \textemdash{} while synaptic weights are modified by Hebbian plasticity, as well as homeostasis. Importantly, all neural apparatus needed for the functionality of the assembly operations is created on the fly through the randomness of the synaptic network, the selection of the             k             neurons with the highest synaptic input, and Hebbian plasticity, without any special neural circuits assumed to be in place. Assemblies and their operations constitute a computational model of the brain which we call the             Assembly Calculus             , occupying a level of detail intermediate between the level of spiking neurons and synapses, and that of the whole brain. As with high-level programming languages, a computation in the Assembly Calculus (that is, a coherent sequence of assembly operations accomplishing a task) can ultimately be reduced \textemdash{} ``compiled down'' \textemdash{} to computation by neurons and synapses; however, it would be far more cumbersome and opaque to represent the same computation that way. The resulting computational system can be shown, under assumptions, to be in principle capable of carrying out arbitrary computations. We hypothesize that something like it may underlie higher human cognitive functions such as reasoning, planning, and language. In particular, we propose a plausible brain architecture based on assemblies for implementing the syntactic processing of language in cortex, which is consistent with recent experimental results.},
 author = {Papadimitriou, Christos H. and Vempala, Santosh S. and Mitropolsky, Daniel and Collins, Michael and Maass, Wolfgang},
 doi = {10.1101/869156},
 file = {/home/matt/Zotero/storage/ASWU6MPX/Papadimitriou et al. - 2019 - Brain computation by assemblies of neurons.pdf},
 institution = {{Neuroscience}},
 language = {en},
 title = {Brain Computation by Assemblies of Neurons},
 type = {Preprint},
 year = {2019}
}

@article{papageorgiou_alinea_1991,
 author = {Papageorgiou, M. and {Hadj-Salem}, H. and Blosseville, J.},
 journal = {Transportation Research Record},
 pages = {58--64},
 title = {{{ALINEA}}: A Local Feedback Control Law for on-Ramp Metering},
 volume = {1320},
 year = {1991}
}

@article{papageorgiou_alinea_1997,
 author = {Papageorgiou, M. and {Hadj-Salem}, H. and Middleham, F.},
 journal = {Transportation Research Record},
 pages = {90--98},
 title = {{{ALINEA}} Local Ramp Metering: {{Summary}} of Field Results},
 volume = {1603},
 year = {1997}
}

@book{papageorgiou_applications_1983,
 author = {Papageorgiou, M.},
 publisher = {{Springer}},
 series = {Lecture {{Notes}} in {{Control}} and {{Information Sciences}}, 50},
 title = {Applications of {{Automatic Control Concepts}} to {{Traffic Flow Modeling}} and {{Control}}},
 year = {1983}
}

@article{papageorgiou_dynamic_1989,
 author = {Papageorgiou, M.},
 journal = {Transportation Research, B},
 pages = {29--48},
 title = {Dynamic Modelling, Assignment and Route Guidance in Traffic Networks.},
 volume = {23},
 year = {1989}
}

@article{papageorgiou_freeway_2002,
 abstract = {Recurrent and nonrecurrent congestion on freeways may be alleviated if today's "spontaneous" infrastructure utilization is replaced by an orderly, controllable operation via comprehensive application of ramp metering and freeway-to-freeway control, combined with powerful optimal control techniques. This paper first explains why ramp metering can lead to a dramatic amelioration of traffic conditions on freeways. An overview of ramp metering algorithms is provided next, ranging from early fixed-time approaches to traffic-responsive regulators and to modern sophisticated nonlinear optimal control schemes. Finally, a large-scale example demonstrates the high potential of advanced ramp metering approaches.},
 author = {Papageorgiou, M. and Kotsialos, A.},
 doi = {10.1109/TITS.2002.806803},
 file = {/home/matt/Zotero/storage/9L2HAM25/Papageorgiou and Kotsialos - 2002 - Freeway ramp metering an overview.pdf;/home/matt/Zotero/storage/9BP399TS/1166514.html},
 issn = {1524-9050},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {4},
 pages = {271--281},
 shorttitle = {Freeway Ramp Metering},
 title = {Freeway Ramp Metering: An Overview},
 volume = {3},
 year = {2002}
}

@article{papageorgiou_modelling_1990,
 author = {Papageorgiou, M. and Blosseville, J.-M. and {H. Hadj-Salem}},
 journal = {Transportation Research A},
 number = {5},
 pages = {345--370},
 title = {Modelling and Real-Time Control of Traffic Flow on the Southern Part of {{Boulevard Peripherique}} in {{Paris}}. {{I}}: {{Modelling}}. {{II}}: {{Coordinated}} on-Ramp Metering},
 volume = {24A},
 year = {1990}
}

@article{papageorgiou_real-time_2008,
 author = {Papageorgiou, M. and Papamichail, I. and Spiliopoulou, I. and Lentzakis, A. F.},
 journal = {Transportation Research, Part C},
 number = {5},
 pages = {535--553},
 title = {Real-Time Merging Traffic Control with Applications to Toll Plaza and Work Zone Management},
 volume = {16},
 year = {2008}
}

@article{papageorgiou_relating_2008,
 author = {Papageorgiou, M. and Vigos, G.},
 journal = {Transportation Research, Part C},
 pages = {1--17},
 title = {Relating Time-Occupancy Measurements to Space-Occupancy and Link Vehicle-Count},
 volume = {16},
 year = {2008}
}

@article{papageorgiou_remarks_1998,
 author = {Papageorgiou, Markos},
 file = {/home/matt/Zotero/storage/EB3SUP3W/1-s2.0-S0965856497000487-main.pdf},
 journal = {Transportation Research Part A: Policy and Practice},
 number = {5},
 pages = {323--329},
 title = {Some Remarks on Macroscopic Traffic Flow Modelling},
 volume = {32},
 year = {1998}
}

@article{papageorgiou_review_2003,
 author = {Papageorgiou, M. and Kiakaki, C. and Dinopoulou, V. and Kotsialos, A. and {Yibing Wang}},
 doi = {10.1109/JPROC.2003.819610},
 file = {/home/matt/Zotero/storage/M8NAS9QS/Papageorgiou et al. - 2003 - Review of road traffic control strategies.pdf},
 issn = {0018-9219},
 journal = {Proceedings of the IEEE},
 language = {en},
 number = {12},
 pages = {2043--2067},
 title = {Review of Road Traffic Control Strategies},
 volume = {91},
 year = {2003}
}

@article{papageoriou_effects_2008,
 author = {Papageoriou, M. and Kosmatopoulos, E. and Papamichail, I. and McCabe, K.},
 journal = {87th Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {Effects of {{Variable Speed Limits}} on {{Motorway Traffic Flow}}},
 year = {2008}
}

@article{papamichail_hero_2010,
 author = {Papamichail, I. and Papageorgiou, M. and Vong, V. and Gaffney, J.},
 journal = {89th Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {{{HERO Coordinated Ramp Metering Im}}- Plemented at {{Monash Freeway}}, {{Australia}}},
 year = {2010}
}

@article{papamichail_heuristic_2010,
 author = {Papamichail, Ioannis and Papageorgiou, Markos and Vong, Vincent and Gaffney, John},
 doi = {10.3141/2178-02},
 file = {/home/matt/Zotero/storage/LD2GTZZC/Papamichail et al. - 2010 - Heuristic Ramp-Metering Coordination Strategy Impl.pdf},
 issn = {0361-1981, 2169-4052},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 number = {1},
 pages = {10--20},
 title = {Heuristic {{Ramp}}-{{Metering Coordination Strategy Implemented}} at {{Monash Freeway}}, {{Australia}}},
 volume = {2178},
 year = {2010}
}

@book{papamichail_integrated_2008,
 annotation = {Published: Technical Report, Dynamic Systems and Simulation Laboratory, Technical University of Crete},
 author = {Papamichail, I. and Kampitaki, K. and Papageorgiou, M. and Messmer, A.},
 title = {Integrated {{Ramp Metering}} and {{Variable Speed Limit Control}} of {{Motorway Traffic Flow}}},
 year = {2008}
}

@article{papamichail_traffic-responsive_2008,
 author = {Papamichail, I. and Papageorgiou, M.},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {1},
 pages = {111--121},
 title = {Traffic-Responsive Linked Ramp-Metering Control},
 volume = {9},
 year = {2008}
}

@article{papola_maximal_1998,
 author = {Papola, N. and Fusco, G.},
 journal = {Transportation Research, Part B},
 number = {4},
 pages = {277--288},
 title = {Maximal Bandwidth Problem: {{A}} New Algorithm Based on the Property of Periodicity of the System},
 volume = {32},
 year = {1998}
}

@article{park_diverse_2020,
 author = {Park, Seong Hyeon and Lee, Gyubok and Bhat, Manoj and Seo, Jimin and Kang, Minseok and Francis, Jonathan and Jadhav, Ashwin R. and Liang, Paul Pu and Morency, Louis-Philippe},
 journal = {ArXiv preprint},
 title = {Diverse and {{Admissible Trajectory Forecasting}} through {{Multimodal Context Understanding}}},
 url = {https://arxiv.org/abs/2003.03212},
 volume = {abs/2003.03212},
 year = {2020}
}

@inproceedings{pascale_adaptive_2011,
 author = {Pascale, A. and Nicoli, M.},
 booktitle = {{{IEEE Statistical Signal Processing Workshop}} ({{SSP}})},
 pages = {177--180},
 title = {Adaptive {{Bayesian}} Network for Traffic Flow Prediction},
 year = {2011}
}

@inproceedings{paszke_automatic_2017,
 abstract = {In this article, we describe an automatic differentiation module of PyTorch \textemdash{} a library designed to enable rapid research on machine learning models. It builds upon a few projects, most notably Lua...},
 author = {Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
 booktitle = {{{NeurIPS Autodiff Workshop}}},
 file = {/home/matt/Zotero/storage/BVIXFGN6/Paszke et al. - 2017 - Automatic differentiation in PyTorch.pdf;/home/matt/Zotero/storage/HZ88SHBF/forum.html},
 title = {Automatic {{Differentiation}} in {{PyTorch}}},
 year = {2017}
}

@inproceedings{paszke_pytorch_2019,
 author = {Adam Paszke and
Sam Gross and
Francisco Massa and
Adam Lerer and
James Bradbury and
Gregory Chanan and
Trevor Killeen and
Zeming Lin and
Natalia Gimelshein and
Luca Antiga and
Alban Desmaison and
Andreas K{\"{o}}pf and
Edward Yang and
Zachary DeVito and
Martin Raison and
Alykhan Tejani and
Sasank Chilamkurthy and
Benoit Steiner and
Lu Fang and
Junjie Bai and
Soumith Chintala},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/PaszkeGMLBCKLGA19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {8024--8035},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {PyTorch: An Imperative Style, High-Performance Deep Learning Library},
 url = {https://proceedings.neurips.cc/paper/2019/hash/bdbca288fee7f92f2bfa9f7012727740-Abstract.html},
 year = {2019}
}

@book{path_berkeley_nodate,
 author = {PATH, California},
 title = {Berkeley {{Advanced Transportation Simulator}} ({{BeATS}})}
}

@inproceedings{pathak_learning_2019,
 author = {Deepak Pathak and
Christopher Lu and
Trevor Darrell and
Phillip Isola and
Alexei A. Efros},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/PathakLDIE19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {2292--2302},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Learning to Control Self-Assembling Morphologies: {A} Study of Generalization
via Modularity},
 url = {https://proceedings.neurips.cc/paper/2019/hash/c26820b8a4c1b3c2aa868d6d57e14a79-Abstract.html},
 year = {2019}
}

@inproceedings{pathak_learning_nodate,
 author = {Deepak Pathak and
Christopher Lu and
Trevor Darrell and
Phillip Isola and
Alexei A. Efros},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/PathakLDIE19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {2292--2302},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Learning to Control Self-Assembling Morphologies: {A} Study of Generalization
via Modularity},
 url = {https://proceedings.neurips.cc/paper/2019/hash/c26820b8a4c1b3c2aa868d6d57e14a79-Abstract.html},
 year = {2019}
}

@article{patire_how_2015,
 author = {Patire, Anthony D. and Wright, Matthew and Prodhomme, Boris and Bayen, Alexandre M.},
 doi = {10.1016/j.trc.2015.02.011},
 issn = {0968-090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 keywords = {Data fusion,Estimation,GPS,Probe data,Travel time},
 pages = {325--342},
 title = {How Much {{GPS}} Data Do We Need?},
 volume = {58},
 year = {2015}
}

@techreport{payne_development_1976,
 address = {{Washington DC}},
 author = {Payne, H. J. and Helfenbein, E. D. and Knobel, H. C.},
 institution = {{Federal Highway Administration}},
 number = {FHWA-RD-76-20},
 title = {Development {{And Testing Of Incident Detection Algorithms}}},
 year = {1976}
}

@book{pb_americas_inc._regional_2006,
 author = {{PB Americas, Inc.}},
 title = {Regional {{HOT}} Lanes Network Feasibility Study: {{Task}} 4\textendash{{Policy}} and Operation Considerations for a Regionwide {{Bay Area HOT}} Lane Network. {{Prepared}} for {{Metropolitan Transportation Commission}} and {{California Department}} of {{Transportation}}.},
 year = {2006}
}

@book{pb_americas_inc._regional_2007,
 author = {{PB Americas, Inc.}},
 title = {Regional {{HOT}} Lanes Network Feasibility Study: {{Task}} 3\textendash{{Initial}} Assessment Report. {{Prepared}} for {{Metropolitan Transportation Commission}} and {{California Department}} of {{Transportation}}.},
 year = {2007}
}

@article{pearl_causal_nodate,
 abstract = {The primary aim of this paper is to show how graphical models can be used as a mathematical language for integrating statistical and subject-matter information. In particular, the paper develops a principled, nonparametric framework for causal inference, in which diagrams are queried to determine if the assumptions available are sufficient for identifying causal effects from nonexperimental data. If so the diagrams can be queried to produce mathematical expressions for causal effects in terms of observed distributions; otherwise, the diagrams can be queried to suggest additional observations or auxiliary experiments from which the desired inferences can be obtained.},
 author = {Pearl, Judea},
 file = {/home/matt/Zotero/storage/KDRKJHCV/Pearl - Causal diagrams for empirical research (CW^-ijt-h .pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {42},
 title = {Causal Diagrams for Empirical Research ({{CW}}\^-Ijt-h {{Ddisic}}\^us\^sioin\^s))}
}

@misc{pems_california_2019,
 author = {{PeMS}},
 howpublished = {http://pems.dot.ca.gov},
 title = {California {{Performance Measurement System}}},
 year = {2019}
}

@inproceedings{peng_bayesian_2019,
 abstract = {In the autonomous driving area, interaction between vehicles is still a piece of puzzle which has not been fully resolved. The ability to intelligently and safely interact with other vehicles can not only improve self driving quality but also be beneficial to the global driving environment. In this paper, a Bayesian persuasive driving algorithm based on optimization is proposed, where the ego vehicle is the persuader (information sender) and the surrounding vehicle is the persuadee (information receiver). In the persuasion process, the ego vehicle aims at changing the surrounding vehicle's posterior belief of the world state by providing certain information via signaling in order to achieve a lower cost for both players. The information received by the surrounding vehicle and its belief of the world state are described by Gaussian distributions. Simulation results in several common traffic scenarios are provided to demonstrate the proposed algorithm's capability of handling interaction situations involving surrounding vehicles with different driving characteristics.},
 author = {Peng, C. and Tomizuka, M.},
 booktitle = {2019 {{American Control Conference}} ({{ACC}})},
 file = {/home/matt/Zotero/storage/YPIDR3AB/Peng_Tomizuka_2019_Bayesian Persuasive Driving.pdf;/home/matt/Zotero/storage/8M2YPRCQ/8814319.html},
 pages = {723--729},
 title = {Bayesian {{Persuasive Driving}}},
 year = {2019}
}

@inproceedings{peng_federated_2020,
 author = {Xingchao Peng and
Zijun Huang and
Yizhe Zhu and
Kate Saenko},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/PengHZS20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Federated Adversarial Domain Adaptation},
 url = {https://openreview.net/forum?id=HJezF3VYPB},
 year = {2020}
}

@inproceedings{peng_mcp_2019,
 author = {Xue Bin Peng and
Michael Chang and
Grace Zhang and
Pieter Abbeel and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/Peng0ZAL19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {3681--3692},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {{MCP:} Learning Composable Hierarchical Control with Multiplicative
Compositional Policies},
 url = {https://proceedings.neurips.cc/paper/2019/hash/95192c98732387165bf8e396c0f2dad2-Abstract.html},
 year = {2019}
}

@article{peng_multiagent_2017,
 author = {Peng, Peng and Wen, Ying and Yang, Yaodong and Yuan, Quan and Tang, Zhenkun and Long, Haitao and Wang, Jun},
 journal = {ArXiv preprint},
 title = {Multiagent {{Bidirectionally}}-{{Coordinated Nets}}: {{Emergence}} of {{Human}}-Level {{Coordination}} in {{Learning}} to {{Play StarCraft Combat Games}}},
 url = {https://arxiv.org/abs/1703.10069},
 volume = {abs/1703.10069},
 year = {2017}
}

@article{peter_j._bickel_measuring_2007,
 author = {Peter J. Bickel, Chao Chen, Jaimyoung Kwon, John Rice, Erik van Zwet, Pravin Varaiya},
 doi = {10.1214/07-STS238},
 issn = {0883-4237},
 journal = {Statistical Science},
 number = {4},
 pages = {581--597},
 title = {Measuring {{Traffic}}},
 volume = {22},
 year = {2007}
}

@article{petersen_matrix_2012,
 author = {Petersen, Kaare Brandt and Pedersen, Michael Syskind},
 file = {/home/matt/Zotero/storage/L4QS9G4P/Petersen and Pedersen - [ httpmatrixcookbook.com ].pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {The {{Matrix Cookbook}}},
 year = {2012}
}

@article{petty_freeway_1996,
 author = {Petty, K. and Noeimi, H. and Sanwal, K. and Rydzewski, D. and Skabardonis, A. and Varaiya, P. and {Al-Deek}, H.},
 journal = {Transportation Research, Part C},
 number = {2},
 pages = {71--85},
 title = {The Freeway Service Patrol Evaluation Project: {{Database}} Support Programs, and Accessibility},
 volume = {4},
 year = {1996}
}

@article{petty_new_2002,
 author = {Petty, K. and Ostland, M. and Kwon, J. and Rice, J. and Bickel, P.},
 journal = {Transportation Research, Part C},
 number = {3},
 pages = {189--204},
 title = {A New Methodology for Evaluating Incident Detection Algorithms},
 volume = {10},
 year = {2002}
}

@inproceedings{pfaff_learning_2021,
 author = {Tobias Pfaff and
Meire Fortunato and
Alvaro Sanchez{-}Gonzalez and
Peter W. Battaglia},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/PfaffFSB21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Learning Mesh-Based Simulation with Graph Networks},
 url = {https://openreview.net/forum?id=roNqYL0\_XP},
 year = {2021}
}

@inproceedings{piacentini_vacs_2019,
 abstract = {The advent of connected, automated and autonomous vehicles introduces the possibility for new traffic control approaches. Vehicles equipped with automation and communication systems can be exploited both as sensor and actuators for traffic control actions, thus avoiding the need for new infrastructure. In this paper a multi-class extension of the macroscopic Cell Transmission Model is adopted to describe the interaction between different classes of vehicles, for example human-driven and connected/automated. The vehicle classes are distinguished on the basis of their time headways and their speed. By means of a Model Predictive Control approach, the optimal free-flow speed for the class of connected/automated vehicles is computed and applied to them with the aim of reducing congestion on the highway. The effectiveness of the proposed control law is analyzed depending on the penetration rate of controlled vehicles and the approach is assessed in simulations.},
 author = {Piacentini, G. and {\v C}i{\v c}i{\'c}, M. and Ferrara, A. and Johansson, K. H.},
 booktitle = {2019 18th {{European Control Conference}} ({{ECC}})},
 doi = {10.23919/ECC.2019.8796094},
 file = {/home/matt/Zotero/storage/64A7NUGU/Piacentini et al. - 2019 - VACS equipped vehicles for congestion dissipation .pdf;/home/matt/Zotero/storage/BQALM2EJ/8796094.html},
 pages = {2203--2208},
 title = {{{VACS}} Equipped Vehicles for Congestion Dissipation in Multi-Class {{CTM}} Framework},
 year = {2019}
}

@article{pillai_restricted_1998,
 author = {Pillai, R. and Rathi, A. and Cohen, S.},
 journal = {Transportation Research, Part B},
 number = {8},
 pages = {517--529},
 title = {A Restricted Branch-and-Bound Approach for Generating Maximum Bandwidth Signal Timing Plans for Traffic Networks},
 volume = {32},
 year = {1998}
}

@phdthesis{pineda_advanced_2017,
 abstract = {Spark plugs have been igniting combustible mixtures like those found in automotive engines for over a century, and the principles of the associated ignition techniques using thermal plasma (inductive or capacitive sparks) have remained relatively unchanged during that time. However, internal combustion engines are increasingly operating with boosted intake pressures (i.e. turbo- or super-charged) in order to maintain power output while simultaneously reducing engine size and weight, and they are also operating with increased recirculated exhaust gas dilution to reduce the production of harmful nitrogen oxides. This ``downsizing'' to increase fuel economy compounded with diluting to decrease emissions leads to challenges in both obtaining traditional ignition and promoting sufficiently fast combustion under this operating paradigm. In conjunction with appropriate electrode design, transient non-thermal plasma can exploit certain non-equilibrium chemistry and physics to bypass these challenges and ultimately promote more reliable ignition and faster combustion. Applied and fundamental experimental investigations of two different advanced ignition techniques are presented: 1) corona discharges igniting gasoline/air/exhaust mixtures in a boosted direct- injection single cylinder research engine and 2) repetitively pulsed nanosecond discharges igniting methane/air mixtures in a constant volume chamber. The engine experimental results show significant decreases in fuel consumption and nitrogen oxide emissions under boosted operation, and both experiments demonstrate more robust ignition and faster flame development. The constant volume chamber results in particular raise important questions about the relative contributions of chemistry and transport to the experimentally observed combustion enhancement. These results highlight the critical importance of electrode design in advanced ignition techniques\textemdash the shape and position of electrodes greatly influences the hydrodynamics of developing flame kernels into fuel-air charges. While this work demonstrates that non-thermal plasma ignition is a promising solution to both increase fuel economy and decrease emissions of future automotive engines, much work remains to be done to understand the beneficial coupling between the detailed non-thermal plasma chemistry and the hydrodynamics associated with these real ignition devices.},
 author = {Pineda, Daniel Ivan},
 file = {/home/matt/Zotero/storage/L6XTRU5A/Pineda - 2017 - Advanced ignition for automotive engines.pdf;/home/matt/Zotero/storage/GWD6LQS6/2f2362sg.html},
 language = {en},
 school = {UC Berkeley},
 title = {Advanced Ignition for Automotive Engines},
 year = {2017}
}

@article{pineda_mbrl-lib_2021,
 author = {Pineda, Luis and Amos, Brandon and Zhang, Amy and Lambert, Nathan O. and Calandra, Roberto},
 journal = {ArXiv preprint},
 title = {{{MBRL}}-{{Lib}}: {{A Modular Library}} for {{Model}}-Based {{Reinforcement Learning}}},
 url = {https://arxiv.org/abs/2104.10159},
 volume = {abs/2104.10159},
 year = {2021}
}

@inproceedings{pmlr-v70-arjovsky17a,
 author = {Mart{\'{\i}}n Arjovsky and
Soumith Chintala and
L{\'{e}}on Bottou},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ArjovskyCB17.bib},
 booktitle = {Proceedings of the 34th International Conference on Machine Learning,
{ICML} 2017, Sydney, NSW, Australia, 6-11 August 2017},
 editor = {Doina Precup and
Yee Whye Teh},
 pages = {214--223},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Wasserstein Generative Adversarial Networks},
 url = {http://proceedings.mlr.press/v70/arjovsky17a.html},
 volume = {70},
 year = {2017}
}

@article{ponnu_speed-spacing_2015,
 abstract = {This paper examines the traffic dynamics underlying a recently observed phenomenon, the so called ``sympathy of speeds'' whereby a high occupancy vehicle (HOV) lane seemingly exhibits lower vehicular capacity and lower flow at speeds throughout the congested regime compared to the adjacent general purpose (GP) lanes. Unlike previous studies this paper examines a time-of-day HOV lane. During the non-HOV periods the study lane reverts to a GP lane, thereby providing a control condition for the specific lane and location. This work uses the single vehicle passage (svp) method to group vehicle passages before measuring the traffic state and extends the svp to bin vehicles in the study lane based on the relative speed to the adjacent lane. The extended svp method allows the work to also study the impacts during the non-HOV periods when the study lane serves GP vehicles. This work finds that: (1) during the non-HOV periods the study lane exhibited behavior indistinguishable from the adjacent GP lane. (2) The sympathy of speeds persists throughout the day, even when the study lane serves GP vehicles. (3) The relative speed to the adjacent lane provided a better predictor of behavior than whether or not the HOV restriction is active. In short, the car following behavior that gives rise to the sympathy of speeds is unrelated to the HOV restriction per se, persisting under GP operations as well.},
 author = {Ponnu, Balaji and Coifman, Benjamin},
 doi = {10.1016/j.trb.2015.09.012},
 file = {/home/matt/Zotero/storage/NPXSIRVQ/Ponnu and Coifman - 2015 - Speed-spacing dependency on relative speed from th.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {74--90},
 shorttitle = {Speed-Spacing Dependency on Relative Speed from the Adjacent Lane},
 title = {Speed-Spacing Dependency on Relative Speed from the Adjacent Lane: {{New}} Insights for Car Following Models},
 volume = {82},
 year = {2015}
}

@article{ponnu_when_2017,
 abstract = {This paper presents an empirical study of the fundamental relationship between speed, v, and flow, q, (denoted vqFR) under low flow in the uncongested regime. Using new analytical techniques to extract more information from loop detector data, the vqFR from a time of day HOV lane exhibits high v that slowly drops as q increases. This curve arises after binning several million vehicles by q and only considering those bins with q {$<$} 1200 vph. A surprising thing happens when further binning the data by the adjacent lane speed (v2): the vqFR expands in to a fan of curves that decrease in magnitude and slope with decreasing v2. Yet each curve in the fan continues to exhibit uncongested trends, ranging from a flat curve consistent with recent editions of the Highway Capacity Manual to downward sloping curves. It is shown that this behavior was not due to the HOV operations per se, the same behavior also arises in the non-HOV period when the lane serves all vehicles and it is also observed at another facility without any HOV restrictions. This dependency on the adjacent lane is absent from most traffic flow theories.},
 author = {Ponnu, Balaji and Coifman, Benjamin},
 doi = {10.1016/j.trb.2017.05.006},
 file = {/home/matt/Zotero/storage/Q2F9QUZM/Ponnu and Coifman - 2017 - When adjacent lane dependencies dominate the uncon.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {602--615},
 title = {When Adjacent Lane Dependencies Dominate the Uncongested Regime of the Fundamental Relationship},
 volume = {104},
 year = {2017}
}

@article{poole_metanet_2012,
 author = {Poole, A. and Kotsialos, A.},
 doi = {10.3182/20120912-3-BG-2031.00002},
 file = {/home/matt/Zotero/storage/U32Q6JVT/poole_2012_traffic_calibration_ga.pdf},
 issn = {14746670},
 journal = {IFAC Proceedings Volumes},
 language = {en},
 number = {24},
 pages = {7--12},
 title = {{{METANET Model Validation}} Using a {{Genetic Algorithm}}},
 volume = {45},
 year = {2012}
}

@article{poole_second_2016,
 author = {Poole, Adam and Kotsialos, Apostolos},
 doi = {10.1016/j.trc.2016.07.008},
 file = {/home/matt/Zotero/storage/KP4FUX5K/poole_2016_calibration_particleswarm.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {356--381},
 title = {Second Order Macroscopic Traffic Flow Model Validation Using Automatic Differentiation with Resilient Backpropagation and Particle Swarm Optimisation Algorithms},
 volume = {71},
 year = {2016}
}

@inproceedings{post_call_2018,
 address = {Brussels, Belgium},
 author = {Post, Matt},
 booktitle = {Proceedings of the Third Conference on Machine Translation: Research Papers},
 doi = {10.18653/v1/W18-6319},
 pages = {186--191},
 publisher = {Association for Computational Linguistics},
 title = {A Call for Clarity in Reporting {BLEU} Scores},
 url = {https://aclanthology.org/W18-6319},
 year = {2018}
}

@article{preisinger_daimler_2013,
 author = {Preisinger, I.},
 journal = {Reuters},
 title = {Daimler Aims to Launch Self-Driving Car by 2020},
 year = {2013}
}

@article{premack_does_1978,
 abstract = {An individual has a theory of mind if he imputes mental states to himself and others. A system of inferences of this kind is properly viewed as a theory because such states are not directly observable, and the system can be used to make predictions about the behavior of others. As to the mental states the chimpanzee may infer, consider those inferred by our own species, for example, purpose or intention, as well as knowledge, belief, thinking, doubt, guessing, pretending, liking, and so forth. To determine whether or not the chimpanzee infers states of this kind, we showed an adult chimpanzee a series of videotaped scenes of a human actor struggling with a variety of problems. Some problems were simple, involving inaccessible food \textendash{} bananas vertically or horizontally out of reach, behind a box, and so forth \textendash{} as in the original Kohler problems; others were more complex, involving an actor unable to extricate himself from a locked cage, shivering because of a malfunctioning heater, or unable to play a phonograph because it was unplugged. With each videotape the chimpanzee was given several photographs, one a solution to the problem, such as a stick for the inaccessible bananas, a key for the locked up actor, a lit wick for the malfunctioning heater. The chimpanzee's consistent choice of the correct photographs can be understood by assuming that the animal recognized the videotape as representing a problem, understood the actor's purpose, and chose alternatives compatible with that purpose.},
 author = {Premack, David and Woodruff, Guy},
 doi = {10.1017/S0140525X00076512},
 file = {/home/matt/Zotero/storage/NK42SVMN/Premack and Woodruff - 1978 - Does the chimpanzee have a theory of mind.pdf;/home/matt/Zotero/storage/LQT9YSWI/1E96B02CD9850016B7C93BC6D2FEF1D0.html},
 issn = {1469-1825, 0140-525X},
 journal = {Behavioral and Brain Sciences},
 language = {en},
 number = {4},
 pages = {515--526},
 publisher = {{Cambridge University Press}},
 title = {Does the Chimpanzee Have a Theory of Mind?},
 volume = {1},
 year = {1978}
}

@inproceedings{press_improving_2020,
 address = {Online},
 author = {Press, Ofir  and
Smith, Noah A.  and
Levy, Omer},
 booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/2020.acl-main.270},
 pages = {2996--3005},
 publisher = {Association for Computational Linguistics},
 title = {Improving Transformer Models by Reordering their Sublayers},
 url = {https://aclanthology.org/2020.acl-main.270},
 year = {2020}
}

@article{puy_unifying_2017,
 author = {Puy, Gilles and Kitic, Srdan and P{\'e}rez, Patrick},
 journal = {ArXiv preprint},
 title = {Unifying Local and Non-Local Signal Processing with Graph {{CNNs}}},
 url = {https://arxiv.org/abs/1702.07759},
 volume = {abs/1702.07759},
 year = {2017}
}

@article{qing-jie_kong_approach_2009,
 author = {{Qing-Jie Kong} and {Zhipeng Li} and {Yikai Chen} and {Yuncai Liu}},
 doi = {10.1109/TITS.2009.2026308},
 file = {/home/matt/Documents/Papers/kong_2009_urban_by_fusing_multisource.pdf},
 issn = {1524-9050, 1558-0016},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {3},
 pages = {499--511},
 title = {An {{Approach}} to {{Urban Traffic State Estimation}} by {{Fusing Multisource Information}}},
 volume = {10},
 year = {2009}
}

@article{r.w._denney_jr._traffic_2013,
 author = {{R.W. Denney, Jr.} and Olson, P. R.},
 journal = {IMSA},
 pages = {28--32},
 title = {Traffic {{Signal Operations Reviews}}: {{Common Threads}}},
 year = {2013}
}

@article{raadsen_continuous-time_2018,
 author = {Raadsen, Mark P.H. and Bliemer, Michiel C.J.},
 doi = {10.1016/j.trb.2018.01.003},
 file = {/home/matt/Zotero/storage/LMPTERGK/raadsen_ct_linktransmission_w_simplified_fanning_ii_2018.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 shorttitle = {Continuous-Time General Link Transmission Model with Simplified Fanning, {{Part II}}},
 title = {Continuous-Time General Link Transmission Model with Simplified Fanning, {{Part II}}: {{Event}}-Based Algorithm for Networks},
 year = {2018}
}

@article{raadsen_efficient_2016,
 author = {Raadsen, Mark P.H. and Bliemer, Michiel C.J. and Bell, Michael G.H.},
 doi = {10.1016/j.trb.2015.08.004},
 file = {/home/matt/Zotero/storage/8TDBRFK8/raadsen_2015_ct_networksim.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {191--210},
 title = {An Efficient and Exact Event-Based Algorithm for Solving Simplified First Order Dynamic Network Loading Problems in Continuous Time},
 volume = {92},
 year = {2016}
}

@techreport{radford_language_2018,
 abstract = {Natural language processing tasks, such as question answering, machine translation, reading comprehension, and summarization, are typically approached with supervised learning on taskspecific datasets. We demonstrate that language models begin to learn these tasks without any explicit supervision when trained on a new dataset of millions of webpages called WebText. When conditioned on a document plus questions, the answers generated by the language model reach 55 F1 on the CoQA dataset - matching or exceeding the performance of 3 out of 4 baseline systems without using the 127,000+ training examples. The capacity of the language model is essential to the success of zero-shot task transfer and increasing it improves performance in a log-linear fashion across tasks. Our largest model, GPT-2, is a 1.5B parameter Transformer that achieves state of the art results on 7 out of 8 tested language modeling datasets in a zero-shot setting but still underfits WebText. Samples from the model reflect these improvements and contain coherent paragraphs of text. These findings suggest a promising path towards building language processing systems which learn to perform tasks from their naturally occurring demonstrations.},
 author = {Radford, Alec and Wu, Jeffrey and Child, Rewon and Luan, David and Amodei, Dario and Sutskever, Ilya},
 file = {/home/matt/Zotero/storage/FGRKJQYA/Radford et al. - Language Models are Unsupervised Multitask Learner.pdf},
 institution = {{OpenAI}},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {24},
 title = {Language {{Models}} Are {{Unsupervised Multitask Learners}}},
 year = {2018}
}

@inproceedings{radford_unsupervised_2016,
 author = {Alec Radford and
Luke Metz and
Soumith Chintala},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/RadfordMC15.bib},
 booktitle = {4th International Conference on Learning Representations, {ICLR} 2016,
San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Unsupervised Representation Learning with Deep Convolutional Generative
Adversarial Networks},
 url = {http://arxiv.org/abs/1511.06434},
 year = {2016}
}

@article{raffel_exploring_2019,
 author = {Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J.},
 journal = {ArXiv preprint},
 title = {Exploring the {{Limits}} of {{Transfer Learning}} with a {{Unified Text}}-to-{{Text Transformer}}},
 url = {https://arxiv.org/abs/1910.10683},
 volume = {abs/1910.10683},
 year = {2019}
}

@article{rahtz_extensible_2019,
 author = {Rahtz, Matthew and Fang, James and Dragan, Anca D. and {Hadfield-Menell}, Dylan},
 journal = {ArXiv preprint},
 title = {An {{Extensible Interactive Interface}} for {{Agent Design}}},
 url = {https://arxiv.org/abs/1906.02641},
 volume = {abs/1906.02641},
 year = {2019}
}

@article{rajamani_complete_2001,
 author = {Rajamani, Rajesh and Howell, Adam S and Chen, Chieh and Hedrick, J Karl and Tomizuka, Masayoshi},
 journal = {Control Systems Technology, IEEE Transactions on},
 number = {4},
 pages = {553--564},
 title = {A Complete Fault Diagnostic System for Automated Vehicles Operating in a Platoon},
 volume = {9},
 year = {2001}
}

@article{rajamani_design_2000,
 author = {Rajamani, R and Choi, SB and Law, BK and Hedrick, JK and Prohaska, R and Kretz, P},
 journal = {Journal of dynamic systems, measurement, and control},
 number = {3},
 pages = {470--476},
 title = {Design and Experimental Implementation of Longitudinal Control for a Platoon of Automated Vehicles},
 volume = {122},
 year = {2000}
}

@inproceedings{rajkumar_cyber-physical_2010,
 abstract = {Cyber-physical systems (CPS) are physical and engineered systems whose operations are monitored, coordinated, controlled and integrated by a computing and communication core. Just as the internet transformed how humans interact with one another, cyber-physical systems will transform how we interact with the physical world around us. Many grand challenges await in the economically vital domains of transportation, health-care, manufacturing, agriculture, energy, defense, aerospace and buildings. The design, construction and verification of cyber-physical systems pose a multitude of technical challenges that must be addressed by a cross-disciplinary community of researchers and educators.},
 author = {Rajkumar, R. and Lee, I. and Sha, L. and Stankovic, J.},
 booktitle = {Design {{Automation Conference}}},
 doi = {10.1145/1837274.1837461},
 file = {/home/matt/Zotero/storage/99J8XDKV/Rajkumar et al. - 2010 - Cyber-physical systems The next computing revolut.pdf;/home/matt/Zotero/storage/C2YKJLXI/5523280.html},
 pages = {731--736},
 shorttitle = {Cyber-Physical Systems},
 title = {Cyber-Physical Systems: {{The}} next Computing Revolution},
 year = {2010}
}

@inproceedings{rakelly_efficient_2019,
 author = {Kate Rakelly and
Aurick Zhou and
Chelsea Finn and
Sergey Levine and
Deirdre Quillen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/RakellyZFLQ19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {5331--5340},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Efficient Off-Policy Meta-Reinforcement Learning via Probabilistic
Context Variables},
 url = {http://proceedings.mlr.press/v97/rakelly19a.html},
 volume = {97},
 year = {2019}
}

@inproceedings{rakelly_efficient_2019-1,
 author = {Kate Rakelly and
Aurick Zhou and
Chelsea Finn and
Sergey Levine and
Deirdre Quillen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/RakellyZFLQ19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {5331--5340},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {Efficient Off-Policy Meta-Reinforcement Learning via Probabilistic
Context Variables},
 url = {http://proceedings.mlr.press/v97/rakelly19a.html},
 volume = {97},
 year = {2019}
}

@article{rakkiyappan_existence_2015,
 abstract = {This paper deals with the problem of existence and uniform stability analysis of fractional-order complex-valued neural networks with constant time delays. Complex-valued recurrent neural networks is an extension of real-valued recurrent neural networks that includes complex-valued states, connection weights, or activation functions. This paper explains sufficient condition for the existence and uniform stability analysis of such networks. Three numerical simulations are delineated to substantiate the effectiveness of the theoretical results.},
 author = {Rakkiyappan, R. and Cao, Jinde and Velmurugan, G.},
 doi = {10.1109/TNNLS.2014.2311099},
 file = {/home/matt/Zotero/storage/CRFG5TSG/Rakkiyappan et al. - 2015 - Existence and Uniform Stability Analysis of Fracti.pdf;/home/matt/Zotero/storage/4V99C9AF/6781037.html},
 issn = {2162-2388},
 journal = {IEEE Transactions on Neural Networks and Learning Systems},
 number = {1},
 pages = {84--97},
 title = {Existence and {{Uniform Stability Analysis}} of {{Fractional}}-{{Order Complex}}-{{Valued Neural Networks With Time Delays}}},
 volume = {26},
 year = {2015}
}

@inproceedings{ramachandran_stand-alone_2019,
 author = {Niki Parmar and
Prajit Ramachandran and
Ashish Vaswani and
Irwan Bello and
Anselm Levskaya and
Jon Shlens},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/ParmarRVBLS19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {68--80},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Stand-Alone Self-Attention in Vision Models},
 url = {https://proceedings.neurips.cc/paper/2019/hash/3416a75f4cea9109507cacd8e2f2aefc-Abstract.html},
 year = {2019}
}

@inproceedings{rao_evaluating_2019,
 author = {Roshan Rao and
Nicholas Bhattacharya and
Neil Thomas and
Yan Duan and
Peter Chen and
John F. Canny and
Pieter Abbeel and
Yun S. Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/RaoBTDCCAS19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {9686--9698},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Evaluating Protein Transfer Learning with {TAPE}},
 url = {https://proceedings.neurips.cc/paper/2019/hash/37f65c068b7723cd7809ee2d31d7861c-Abstract.html},
 year = {2019}
}

@inproceedings{rashid_qmix_2018,
 author = {Tabish Rashid and
Mikayel Samvelyan and
Christian Schr{\"{o}}der de Witt and
Gregory Farquhar and
Jakob N. Foerster and
Shimon Whiteson},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/RashidSWFFW18.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {4292--4301},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {{QMIX:} Monotonic Value Function Factorisation for Deep Multi-Agent
Reinforcement Learning},
 url = {http://proceedings.mlr.press/v80/rashid18a.html},
 volume = {80},
 year = {2018}
}

@article{ratrout_comparative_2009,
 author = {Ratrout, Nedal T. and Rahman, Syed Masiur},
 file = {/home/matt/Zotero/storage/WJTP9ESV/A_comparative_analysis_of_currently_used_microscop.pdf},
 journal = {The Arabian Journal for Science and Engineering},
 number = {1B},
 pages = {121--133},
 title = {A Comparative Analysis of Currently Used Microscopic and Macroscopic Traffic Simulation Software},
 volume = {34},
 year = {2009}
}

@article{ravanbakhsh_real-time_2019,
 author = {Ravanbakhsh, Hadi and Laine, Forrest and Seshia, Sanjit A.},
 journal = {ArXiv preprint},
 title = {Real-Time {{Funnel Generation}} for {{Restricted Motion Planning}}},
 url = {https://arxiv.org/abs/1911.01532},
 volume = {abs/1911.01532},
 year = {2019}
}

@book{reaney_about_2012,
 annotation = {Published: Reuters},
 author = {Reaney, P.},
 title = {About One in Five Workers Worldwide Telecommute: Poll},
 year = {2012}
}

@inproceedings{reddi_convergence_2018,
 author = {Sashank J. Reddi and
Satyen Kale and
Sanjiv Kumar},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ReddiKK18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 04 Apr 2019 01:00:00 +0200},
 title = {On the Convergence of Adam and Beyond},
 url = {https://openreview.net/forum?id=ryQu7f-RZ},
 year = {2018}
}

@inproceedings{reddy_learning_2019,
 author = {Siddharth Reddy and
Anca D. Dragan and
Sergey Levine and
Shane Legg and
Jan Leike},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ReddyDLLL20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {8020--8029},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Learning Human Objectives by Evaluating Hypothetical Behavior},
 url = {http://proceedings.mlr.press/v119/reddy20a.html},
 volume = {119},
 year = {2020}
}

@inproceedings{reddy_sqil_2019,
 author = {Siddharth Reddy and
Anca D. Dragan and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ReddyDL20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {{SQIL:} Imitation Learning via Reinforcement Learning with Sparse
Rewards},
 url = {https://openreview.net/forum?id=S1xKd24twB},
 year = {2020}
}

@article{reilly_creating_2016,
 abstract = {This article presents a study on freeway networks instrumented with coordinated ramp metering and the ability of such control systems to produce arbitrarily complex congestion patterns within the dynamical limits of the traffic system. The developed method is used to evaluate the potential for an adversary with access to control infrastructure to enact high-level attacks on the underlying freeway system. The attacks are executed using a predictive, coordinated ramp metering controller based on finite-horizon optimal control and multi-objective optimization techniques. The efficacy of the control schemes in carrying out the prescribed attacks is determined via simulations of traffic network models based on the cell transmission model with onramps modeled as queue buffers. Freeway attacks with high-level objectives are presented on two illustrative examples: congestionon-demand, which aims to create precise, user-specified pockets of congestion, and catchme-if-you-can, which attempts to aid a fleeing vehicle from pursuant vehicles.},
 author = {Reilly, Jack and Martin, S{\'e}bastien and Payer, Mathias and Bayen, Alexandre M.},
 doi = {10.1016/j.trb.2016.05.017},
 file = {/home/matt/Zotero/storage/3XV4NRWN/Reilly et al. - 2016 - Creating complex congestion patterns via multi-obj.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {366--382},
 title = {Creating Complex Congestion Patterns via Multi-Objective Optimal Freeway Traffic Control with Application to Cyber-Security},
 volume = {91},
 year = {2016}
}

@misc{relax_california_department_of_transportation_caltrans_office_2015,
 author = {{\textbackslash relax California Department of Transportation (Caltrans)}},
 howpublished = {http://www.dot.ca.gov/hq/tpp/corridor-mobility/},
 title = {Office of {{System}}, {{Freight}}, \& {{Rail Planning}}},
 year = {2015}
}

@phdthesis{reynoso_mora_time-optimal_2013,
 abstract = {In this dissertation, we study two important subjects in robotics: (i) time-optimal trajectory planning, and (ii) optimal control synthesis methodologies for trajectory tracking. In the first subject, we concentrate on a rather specific sub-class of problems, the time-optimal trajectory planning along predetermined geometric paths. In this kind of problem, a purely geometric path is already known, and the task is to find out how to move along this path in the shortest time physically possible. In order to generate the true fastest solutions achievable by the actual robot manipulator, the complete nonlinear dynamic model should be incorporated into the problem formulation as a constraint that must be satisfied by the generated trajectories and feedforward torques. This important problem was studied in the 1980s, with many related methods for addressing it based on the so-called velocity limit curve and variational methods. Modern formulations directly discretize the problem and obtain a large-scale mathematical optimization problem, which is a prominent approach to tackle optimal control problems that has gained popularity over variational methods, mainly because it allows to obtain numerical solutions for harder problems.We contribute to the referred problem of time-optimal trajectory planning, by extending and improving the existing mathematical optimization formulations. We successfully incorporate the complete nonlinear dynamic model, including viscous friction because for the fastest motions it becomes even more significant than Coulomb friction; of course, Coulomb friction is likewise accommodated for in our formulation. We develop a framework that guarantees exact dynamic feasibility of the generated time-optimal trajectories and feedforward torques. Our initial formulation is carefully crafted in a rather specific manner, so that it allows to naturally propose a convex relaxation that solves exactly the original problem formulation, which is non-convex and therefore hard to solve. In order to numerically solve the proposed formulation, a discretization scheme is also developed. Unlike traditional and modern formulations, we motivate the incorporation of additional criteria to our original formulation, with simulation and experimental studies of three crucial variables for a 6-axis industrial manipulator. Namely, the resulting applied torques, the readings of a 3-axis accelerometer mounted at the manipulator end-effector, and the detrimental effects on the tracking errors induced by pure time-optimal solutions. We therefore emphasize the significance of penalizing a measure of total jerk and of imposing acceleration constraints. These two criteria are incorporated without destroying convexity. The final formulation generates near time-optimal trajectories and feedforward torques with traveling times that are slightly larger than those of pure time-optimal solutions. Nevertheless, the detrimental effects induced by pure time-optimality are eliminated. Experimental results on a 6-axis industrial manipulator confirm that our formulation generates the fastest solutions that can actually be implemented in the real robot manipulator.Following the work done on near time-optimal trajectories, we explore two controller synthesis methodologies for trajectory tracking, which are more suitable to achieve trajectory-tracking under such fast trajectories. In the first approach, we approximate the discrete-time nonlinear dynamics of robot manipulators, moving along the state-reference trajectory, as an affine time-varying (ATV) dynamical system in discrete-time. Therefore, the problem of trajectory tracking for robot manipulators is posed as a linear quadratic (LQ) optimal control problem for a class of discrete-time ATV dynamical systems. Then, an ATV control law to achieve trajectory tracking on the ATV system is developed, which uses LQ methods for linear time-varying (LTV) systems. Since the ATV dynamical system approximates the nonlinear robot dynamics along the state-reference trajectory, the resulting time-varying control law is suitable to achieve trajectory tracking on the robotmanipulator. The ATV control law is implemented in experiments for the 6-axis industrial manipulator, tracking the near time-optimal trajectory. Experimental results verify the better performance achieved with the ATV control law, but also expose its shortcomings.The second approach to address trajectory tracking is related in spirit, but different in crucial aspects, which ultimately endow this approach with its superior features. In this novel approach, the highly nonlinear dynamic model of robot manipulators, moving along a state-reference trajectory, is approximated as a class of piecewise affine (PWA) dynamical systems. We propose a framework to construct the referred PWA system, which consists in: (i) choosing strategic operating points on the state-reference trajectory with their respective (local) linearized system dynamics, (ii) constructing ellipsoidal regions centered at the operating points, whose purpose is to facilitate the scheduling strategy of controller gains designed for each local dynamics. Likewise, in order to switch controller gains as the robot state traverses in the direction of the state-reference trajectory, a simple scheduling strategy is proposed. The controller synthesis near each operating point is an LQR-type that takes into account the local coupled dynamics. The referred PWA control law is implemented in experiments for the 6-axis manipulator tracking the near time-optimal trajectory. The experimental results show the feasibility and superiority of the PWA control law over the typical PID controller and the ATV control law.},
 author = {Reynoso Mora, Pedro},
 file = {/home/matt/Zotero/storage/I96SSJPC/Reynoso Mora - 2013 - On the Time-optimal Trajectory Planning along Pred.pdf;/home/matt/Zotero/storage/DHCV55CP/58r3063m.html},
 language = {en},
 school = {UC Berkeley},
 title = {On the {{Time}}-Optimal {{Trajectory Planning}} along {{Predetermined Geometric Paths}} and {{Optimal Control Synthesis}} for {{Trajectory Tracking}} of {{Robot Manipulators}}},
 year = {2013}
}

@inproceedings{rhinehart_deep_2018,
 author = {Nicholas Rhinehart and
Rowan McAllister and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/RhinehartML20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Deep Imitative Models for Flexible Inference, Planning, and Control},
 url = {https://openreview.net/forum?id=Skl4mRNYDr},
 year = {2020}
}

@inproceedings{rhinehart_precog_2019,
 author = {Nicholas Rhinehart and
Rowan McAllister and
Kris Kitani and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/RhinehartMKL19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00291},
 pages = {2821--2830},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {{PRECOG:} PREdiction Conditioned on Goals in Visual Multi-Agent Settings},
 url = {https://doi.org/10.1109/ICCV.2019.00291},
 year = {2019}
}

@inproceedings{richard_neural_2021,
 author = {Alexander Richard and
Dejan Markovic and
Israel D. Gebru and
Steven Krenn and
Gladstone Alexander Butler and
Fernando De la Torre and
Yaser Sheikh},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/RichardMGKBTS21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Neural Synthesis of Binaural Speech From Mono Audio},
 url = {https://openreview.net/forum?id=uAX8q61EVRu},
 year = {2021}
}

@article{richards_shock_1956,
 author = {Richards, Paul F.},
 doi = {10.1287/opre.4.1.42},
 journal = {Operations Research},
 number = {1},
 pages = {42--51},
 title = {Shock Waves on the Highway},
 volume = {4},
 year = {1956}
}

@article{ristine_operation_2003,
 author = {Ristine, Jeff},
 journal = {The San Diego Union Tribune},
 title = {Operation: Bypass},
 year = {2003}
}

@techreport{ritchie_field_2002,
 address = {{Berkeley, California}},
 author = {Ritchie, S. G. and Park, S. and Oh, C. and Sun, C.},
 institution = {{Institute of Transportation Studies, University of California}},
 number = {PATH Research Report UCB-ITS-PRR-2002-15},
 title = {Field {{Investigation}} of {{Advanced Vehicle Reidentification Techniques}} and {{Detector Technologies}}-{{Phase}} 1},
 year = {2002}
}

@article{robertson_optimizing_1991,
 author = {Robertson, D. I. and Bretherton, R. D.},
 journal = {IEEE Transactions on Vehicular Technology},
 number = {1},
 pages = {11--15},
 title = {Optimizing {{Networks}} of {{Traffic Signals}} in {{Real Time}}-{{The SCOOT Method}}},
 volume = {40},
 year = {1991}
}

@article{roh_multimodal_2020,
 author = {Roh, Junha and Mavrogiannis, Christoforos and Madan, Rishabh and Fox, Dieter and Srinivasa, Siddhartha S.},
 journal = {ArXiv preprint},
 title = {Multimodal {{Trajectory Prediction}} via {{Topological Invariance}} for {{Navigation}} at {{Uncontrolled Intersections}}},
 url = {https://arxiv.org/abs/2011.03894},
 volume = {abs/2011.03894},
 year = {2020}
}

@inproceedings{rolf_post-estimation_2020,
 author = {Esther Rolf and
Michael I. Jordan and
Benjamin Recht},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aistats/RolfJR20.bib},
 booktitle = {The 23rd International Conference on Artificial Intelligence and Statistics,
{AISTATS} 2020, 26-28 August 2020, Online [Palermo, Sicily, Italy]},
 editor = {Silvia Chiappa and
Roberto Calandra},
 pages = {1759--1769},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Mon, 29 Jun 2020 01:00:00 +0200},
 title = {Post-Estimation Smoothing: {A} Simple Baseline for Learning with Side
Information},
 url = {http://proceedings.mlr.press/v108/rolf20a.html},
 volume = {108},
 year = {2020}
}

@article{rolnick_tackling_2019,
 author = {Rolnick, David and Donti, Priya L. and Kaack, Lynn H. and Kochanski, Kelly and Lacoste, Alexandre and Sankaran, Kris and Ross, Andrew Slavin and {Milojevic-Dupont}, Nikola and Jaques, Natasha and {Waldman-Brown}, Anna and Luccioni, Alexandra and Maharaj, Tegan and Sherwin, Evan D. and Mukkavilli, S. Karthik and Kording, Konrad P. and Gomes, Carla and Ng, Andrew Y. and Hassabis, Demis and Platt, John C. and Creutzig, Felix and Chayes, Jennifer and Bengio, Yoshua},
 journal = {ArXiv preprint},
 title = {Tackling {{Climate Change}} with {{Machine Learning}}},
 url = {https://arxiv.org/abs/1906.05433},
 volume = {abs/1906.05433},
 year = {2019}
}

@inproceedings{rong_dropedge_2019,
 author = {Yu Rong and
Wenbing Huang and
Tingyang Xu and
Junzhou Huang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/RongHXH20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {DropEdge: Towards Deep Graph Convolutional Networks on Node Classification},
 url = {https://openreview.net/forum?id=Hkx1qkrKPr},
 year = {2020}
}

@inproceedings{rong_dropedge_2020,
 author = {Yu Rong and
Wenbing Huang and
Tingyang Xu and
Junzhou Huang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/RongHXH20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {DropEdge: Towards Deep Graph Convolutional Networks on Node Classification},
 url = {https://openreview.net/forum?id=Hkx1qkrKPr},
 year = {2020}
}

@inproceedings{rong_self-supervised_2020,
 author = {Yu Rong and
Yatao Bian and
Tingyang Xu and
Weiyang Xie and
Ying Wei and
Wenbing Huang and
Junzhou Huang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/RongBXX0HH20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Thu, 29 Jul 2021 01:00:00 +0200},
 title = {Self-Supervised Graph Transformer on Large-Scale Molecular Data},
 url = {https://proceedings.neurips.cc/paper/2020/hash/94aef38441efa3380a3bed3faf1f9d5d-Abstract.html},
 year = {2020}
}

@article{rosasco_are_2004,
 abstract = {In this paper we investigate the impact of choosing different loss functions from the viewpoint of statistical learning theory. We introduce a convexity assumption - which is met by all loss functions commonly used in the literature, and study how the bound on the estimation error changes with the loss. We also derive a general result on the minimizer of the expected risk for a convex loss function in the case of classification. The main outcome of our analysis is that, for classification, the hinge loss appears to be the loss of choice. Other things being equal, the hinge loss leads to a convergence rate practically indistinguishable from the logistic loss rate and much better than the square loss rate. Furthermore, if the hypothesis space is sufficiently rich, the bounds obtained for the hinge loss are not loosened by the thresholding stage.},
 author = {Rosasco, Lorenzo and Vito, Ernesto De and Caponnetto, Andrea and Piana, Michele and Verri, Alessandro},
 doi = {10.1162/089976604773135104},
 file = {/home/matt/Zotero/storage/CFFVGP35/Rosasco et al. - 2004 - Are Loss Functions All the Same.pdf},
 issn = {0899-7667, 1530-888X},
 journal = {Neural Computation},
 language = {en},
 number = {5},
 pages = {1063--1076},
 title = {Are {{Loss Functions All}} the {{Same}}?},
 volume = {16},
 year = {2004}
}

@article{rosenbloom_stability_2019-1,
 abstract = {Instilling climate policy with stability has emerged as a central concern in both the academic literature and societal discourse around climate change. Societal actors have called for stable climate policy to enable lowcarbon investment; decisionmakers have sought to provide credible signals; and scholars have developed insights to inform ``stickier'' instrument design. However, given the sources of instability confronting climate policy and the transformative changes entailed by decarbonization, this paper argues that climate policy stability may not only be unattainable but also undesirable. Instead of striving for stability as an overriding feature of climate policy, we suggest attending to a broader aim: stabilizing the overarching orientation of climate policy as a transition towards a low greenhouse gas emission economy. We review the complementary concepts of path dependence, policy feedback, and transition pathways to distill strategies that may help in addressing this aim.},
 author = {Rosenbloom, Daniel and Meadowcroft, James and Cashore, Benjamin},
 doi = {10.1016/j.erss.2018.12.009},
 file = {/home/matt/Zotero/storage/RNJW6DWX/Rosenbloom et al. - 2019 - Stability and climate policy Harnessing insights .pdf},
 issn = {22146296},
 journal = {Energy Research \& Social Science},
 language = {en},
 pages = {168--178},
 shorttitle = {Stability and Climate Policy?},
 title = {Stability and Climate Policy? {{Harnessing}} Insights on Path Dependence, Policy Feedback, and Transition Pathways},
 volume = {50},
 year = {2019}
}

@article{rosolia_learning_2019,
 abstract = {We present a learning model predictive controller (LMPC) for autonomous racing. We model the autonomous racing problem as a minimum time iterative control task, where an iteration corresponds to a lap. The system trajectory and input sequence of each lap are stored and used to systematically update the controller for the next lap. In the proposed approach, the race time does not increase at each iteration. The first contribution is to propose a local LMPC which reduces the computational burden associated with existing LMPC strategies. In particular, we show how to construct a local safe set and approximation to the value function, using a subset of the stored data. The second contribution is to present a system identification strategy for the autonomous racing iterative control task. We use data from previous iterations and the vehicle's kinematic equations of motion to build an affine time-varying prediction model. The effectiveness of the proposed strategy is demonstrated by experimental results on the Berkeley Autonomous Race Car (BARC) platform.},
 author = {Rosolia, Ugo and Borrelli, Francesco},
 doi = {10.1109/TCST.2019.2948135},
 file = {/home/matt/Zotero/storage/UZHT76UX/Rosolia and Borrelli - 2019 - Learning How to Autonomously Race a Car A Predict.pdf},
 issn = {1063-6536, 1558-0865, 2374-0159},
 journal = {IEEE Transactions on Control Systems Technology},
 language = {en},
 pages = {1--7},
 shorttitle = {Learning {{How}} to {{Autonomously Race}} a {{Car}}},
 title = {Learning {{How}} to {{Autonomously Race}} a {{Car}}: {{A Predictive Control Approach}}},
 year = {2019}
}

@article{rosolia_minimum_2020,
 author = {Rosolia, Ugo and Borrelli, Francesco},
 journal = {ArXiv preprint},
 title = {Minimum {{Time Learning Model Predictive Control}}},
 url = {https://arxiv.org/abs/1911.09239},
 volume = {abs/1911.09239},
 year = {2019}
}

@article{rosolia_robust_2019,
 author = {Rosolia, Ugo and Zhang, Xiaojing and Borrelli, Francesco},
 journal = {ArXiv preprint},
 title = {Robust {{Learning Model Predictive Control}} for {{Linear Systems}}},
 url = {https://arxiv.org/abs/1911.09234},
 volume = {abs/1911.09234},
 year = {2019}
}

@article{rosolia_sample-based_2019,
 author = {Rosolia, Ugo and Borrelli, Francesco},
 journal = {ArXiv preprint},
 title = {Sample-{{Based Learning Model Predictive Control}} for {{Linear Uncertain Systems}}},
 url = {https://arxiv.org/abs/1904.06432},
 volume = {abs/1904.06432},
 year = {2019}
}

@inproceedings{rosolia_simple_2019,
 abstract = {A data-based policy for iterative control task is presented. The proposed strategy is model-free and can be applied whenever safe input and state trajectories of a system performing an iterative task are available. These trajectories, together with a user-defined cost function, are exploited to construct a piecewise affine approximation to the value function. The approximated value function is then used to evaluate the control policy by solving a linear program. We show that for linear system subject to convex cost and constraints, the proposed strategy guarantees closed-loop constraint satisfaction and performance bounds for the closed-loop trajectory. We evaluate the proposed strategy in simulations and experiments, the latter carried out on the Berkeley Autonomous Race Car (BARC) platform. We show that the proposed strategy is able to reduce the computation time by one order of magnitude while achieving the same performance as our model-based control algorithm.},
 author = {Rosolia, U. and Zhang, X. and Borrelli, F.},
 booktitle = {2019 {{American Control Conference}} ({{ACC}})},
 file = {/home/matt/Zotero/storage/2TCLL6B2/Rosolia et al_2019_Simple Policy Evaluation for Data-Rich Iterative Tasks.pdf;/home/matt/Zotero/storage/GFNIV3ZT/8814765.html},
 pages = {2855--2860},
 title = {Simple {{Policy Evaluation}} for {{Data}}-{{Rich Iterative Tasks}}},
 year = {2019}
}

@article{rosvall_networks_2005,
 abstract = {Traffic is constrained by the information involved in locating the receiver and the physical distance between sender and receiver. We here focus on the former, and investigate traffic in the perspective of information handling. We replot the road map of cities in terms of the information needed to locate specific addresses and create information city networks with roads mapped to nodes and intersections to links between nodes. These networks have the broad degree distribution found in many other complex networks. The mapping to an information city network makes it possible to quantify the information associated with locating specific addresses.},
 author = {Rosvall, M. and Trusina, A. and Minnhagen, P. and Sneppen, K.},
 doi = {10.1103/PhysRevLett.94.028701},
 file = {/home/matt/Zotero/storage/RL5TRCR6/Rosvall et al. - 2005 - Networks and Cities An Information Perspective.pdf;/home/matt/Zotero/storage/VPNAXIAM/PhysRevLett.94.html},
 journal = {Physical Review Letters},
 number = {2},
 pages = {028701},
 shorttitle = {Networks and {{Cities}}},
 title = {Networks and {{Cities}}: {{An Information Perspective}}},
 volume = {94},
 year = {2005}
}

@article{roth_optimal_2003,
 abstract = {For several major applications of data analysis, objects are often not represented as feature vectors in a vector space, but rather by a matrix gathering pairwise proximities. Such pairwise data often violates metricity and, therefore, cannot be naturally embedded in a vector space. Concerning the problem of unsupervised structure detection or clustering, in this paper, a new embedding method for pairwise data into Euclidean vector spaces is introduced. We show that all clustering methods, which are invariant under additive shifts of the pairwise proximities, can be reformulated as grouping problems in Euclidian spaces. The most prominent property of this constant shift embedding framework is the complete preservation of the cluster structure in the embedding space. Restating pairwise clustering problems in vector spaces has several important consequences, such as the statistical description of the clusters by way of cluster prototypes, the generic extension of the grouping procedure to a discriminative prediction rule, and the applicability of standard preprocessing methods like denoising or dimensionality reduction.},
 author = {Roth, V. and Laub, J. and Kawanabe, M. and Buhmann, J.M.},
 doi = {10.1109/TPAMI.2003.1251147},
 file = {/home/matt/Zotero/storage/ZLGGFYYC/Roth et al. - 2003 - Optimal cluster preserving embedding of nonmetric .pdf;/home/matt/Zotero/storage/8VS27FTB/1251147.html},
 issn = {1939-3539},
 journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
 number = {12},
 pages = {1540--1551},
 title = {Optimal Cluster Preserving Embedding of Nonmetric Proximity Data},
 volume = {25},
 year = {2003}
}

@article{rouwendal_basic_2006,
 author = {Rouwendal, Jan and Verhoef, Erik T.},
 doi = {10.1016/j.tranpol.2005.11.007},
 file = {/home/matt/Zotero/storage/2QP68PF9/RouwendalBasicEconomicRoadPricing.pdf},
 issn = {0967070X},
 journal = {Transport Policy},
 language = {en},
 number = {2},
 pages = {106--114},
 shorttitle = {Basic Economic Principles of Road Pricing},
 title = {Basic Economic Principles of Road Pricing: {{From}} Theory to Applications},
 volume = {13},
 year = {2006}
}

@inproceedings{rubanova_latent_2019,
 abstract = {Time series with non-uniform intervals occur in many applications, and are difficult to model using standard recurrent neural networks (RNNs). We generalize RNNs to have continuous-time hidden dynamics defined by ordinary differential equations (ODEs), a model we call ODE-RNNs. Furthermore, we use ODE-RNNs to replace the recognition network of the recently-proposed Latent ODE model. Both ODE-RNNs and Latent ODEs can naturally handle arbitrary time gaps between observations, and can explicitly model the probability of observation times using Poisson processes. We show experimentally that these ODE-based models outperform their RNN-based counterparts on irregularly-sampled data.},
 archiveprefix = {arXiv},
 author = {Rubanova, Yulia and Chen, Ricky T. Q. and Duvenaud, David},
 booktitle = {Advances in {{Neural Information Processing Systems}}},
 eprint = {1907.03907},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/RCZBH6AF/Rubanova et al. - 2019 - Latent ODEs for Irregularly-Sampled Time Series.pdf;/home/matt/Zotero/storage/A9RYDZJH/1907.html},
 title = {Latent {{ODEs}} for {{Irregularly}}-{{Sampled Time Series}}},
 volume = {33},
 year = {2019}
}

@inproceedings{ruch_amodeus_2018,
 abstract = {In an autonomous mobility-on-demand (AMoD) system, customers are transported by autonomously driving vehicles in an on-demand fashion. Although these AMoD systems will soon be introduced to cities, their quantitative analysis from a fleet operational and city planning viewpoint remains challenging due to the lack of dedicated analysis tools. In this paper, we introduce AMoDeus, an open-source software package for the accurate and quantitative analysis of autonomous mobility-on-demand systems. AMoDeus uses an agent-based transportation simulation framework to simulate arbitrarily configured AMoD systems with static or dynamic demand. It includes standard benchmark algorithms, fleet efficiency and service level analysis methods and a dedicated graphical viewer that allows in-depth insights into the system. Together with AMoDeus, we publish a typical simulation scenario based on taxi traces recorded in San Francisco. It can be used to test novel fleet control algorithms or as a basis to model more complex transportation research scenarios.},
 author = {Ruch, C. and H{\"o}rl, S. and Frazzoli, E.},
 booktitle = {2018 21st {{International Conference}} on {{Intelligent Transportation Systems}} ({{ITSC}})},
 doi = {10.1109/ITSC.2018.8569961},
 file = {/home/matt/Zotero/storage/TQBBKMB2/Ruch et al. - 2018 - AMoDeus, a Simulation-Based Testbed for Autonomous.pdf;/home/matt/Zotero/storage/ZBHFFPJD/8569961.html},
 pages = {3639--3644},
 title = {{{AMoDeus}}, a {{Simulation}}-{{Based Testbed}} for {{Autonomous Mobility}}-on-{{Demand Systems}}},
 year = {2018}
}

@article{s.g._shelby_overview_2008,
 author = {S.G. Shelby, D.M. Bullock, D. Gettman, R.S. Ghaman, Z.A. Sabra and Soyke, N.},
 journal = {87th Annual Meeting of the Transportation Research Board, Washington, D.C., USA},
 title = {An Overview and Performance Evaluation of {{ACS LITE}} - a Low Cost Adaptive Signal Control System},
 year = {2008}
}

@article{saberi_hysteresis_2013,
 author = {Saberi, Meead and Mahmassani, Hani},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 pages = {44--55},
 title = {Hysteresis and {{Capacity Drop Phenomena}} in {{Freeway Networks}}: {{Empirical Characterization}} and {{Interpretation}}},
 volume = {2391},
 year = {2013}
}

@inproceedings{sabour_dynamic_2017,
 author = {Sara Sabour and
Nicholas Frosst and
Geoffrey E. Hinton},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/SabourFH17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {3856--3866},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Dynamic Routing Between Capsules},
 url = {https://proceedings.neurips.cc/paper/2017/hash/2cad8fa47bbef282badbb8de5374b894-Abstract.html},
 year = {2017}
}

@inproceedings{sadigh_planning_2016,
 abstract = {Traditionally, autonomous cars make predictions about other drivers' future trajectories, and plan to stay out of their way. This tends to result in defensive and opaque behaviors. Our key insight is that an autonomous car's actions will actually affect what other cars will do in response, whether the car is aware of it or not. Our thesis is that we can leverage these responses to plan more efficient and communicative behaviors. We model the interaction between an autonomous car and a human driver as a dynamical system, in which the robot's actions have immediate consequences on the state of the car, but also on human actions. We model these consequences by approximating the human as an optimal planner, with a reward function that we acquire through Inverse Reinforcement Learning. When the robot plans with this reward function in this dynamical system, it comes up with actions that purposefully change human state: it merges in front of a human to get them to slow down or to reach its own goal faster; it blocks two lanes to get them to switch to a third lane; or it backs up slightly at an intersection to get them to proceed first. Such behaviors arise from the optimization, without relying on hand-coded signaling strategies and without ever explicitly modeling communication. Our user study results suggest that the robot is indeed capable of eliciting desired changes in human state by planning using this dynamical system.},
 author = {Sadigh, Dorsa and Sastry, Shankar and A. Seshia, Sanjit and D. Dragan, Anca},
 booktitle = {Robotics: {{Science}} and {{Systems XII}}},
 doi = {10.15607/RSS.2016.XII.029},
 file = {/home/matt/Zotero/storage/RXHW9KHN/Sadigh et al. - 2016 - Planning for Autonomous Cars that Leverage Effects.pdf},
 isbn = {978-0-9923747-2-3},
 language = {en},
 publisher = {{Robotics: Science and Systems Foundation}},
 title = {Planning for {{Autonomous Cars}} That {{Leverage Effects}} on {{Human Actions}}},
 year = {2016}
}

@article{saerens_methodology_2013,
 author = {Saerens, B. and Rakha, H.A. and Diehl, M. and {Van den Bulk}, E.},
 journal = {Transportation Research, Part D},
 pages = {20--27},
 title = {A Methodology for Assessing Eco-Cruise Control for Passanger Vehicles},
 volume = {19},
 year = {2013}
}

@inproceedings{saito_semi-supervised_2019,
 author = {Kuniaki Saito and
Donghyun Kim and
Stan Sclaroff and
Trevor Darrell and
Kate Saenko},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/SaitoKSDS19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00814},
 pages = {8049--8057},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Semi-Supervised Domain Adaptation via Minimax Entropy},
 url = {https://doi.org/10.1109/ICCV.2019.00814},
 year = {2019}
}

@article{sakiyama_eigendecomposition-free_2019,
 abstract = {This paper addresses the problem of selecting an optimal sampling set for signals on graphs. The proposed sampling set selection (SSS) is based on a localization operator that can consider both vertex domain and spectral domain localizations. We clarify the relationships among the proposed method, sensor position selection methods in machine learning, and existing SSS methods based on graph frequency. In contrast to the alternative graph signal processing-based approaches, the proposed method does not need to compute the eigendecomposition of a variation operator, while still considering (graph) frequency information. We evaluate the performance of our approach through comparisons of prediction errors and execution time.},
 author = {Sakiyama, Akie and Tanaka, Yuichi and Tanaka, Toshihisa and Ortega, Antonio},
 doi = {10.1109/TSP.2019.2908129},
 file = {/home/matt/Zotero/storage/RFMEJP7U/Sakiyama et al. - 2019 - Eigendecomposition-Free Sampling Set Selection for.pdf;/home/matt/Zotero/storage/LV4V9GLE/8676043.html},
 issn = {1941-0476},
 journal = {IEEE Transactions on Signal Processing},
 number = {10},
 pages = {2679--2692},
 title = {Eigendecomposition-{{Free Sampling Set Selection}} for {{Graph Signals}}},
 volume = {67},
 year = {2019}
}

@inproceedings{samanta_nevae_2019,
 author = {Bidisha Samanta and
Abir De and
Gourhari Jana and
Pratim Kumar Chattaraj and
Niloy Ganguly and
Manuel Gomez Rodriguez},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/SamantaDJCGR19.bib},
 booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
2019, The Thirty-First Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
USA, January 27 - February 1, 2019},
 doi = {10.1609/aaai.v33i01.33011110},
 pages = {1110--1117},
 publisher = {{AAAI} Press},
 timestamp = {Wed, 25 Sep 2019 01:00:00 +0200},
 title = {NeVAE: {A} Deep Generative Model for Molecular Graphs},
 url = {https://doi.org/10.1609/aaai.v33i01.33011110},
 year = {2019}
}

@phdthesis{samaranayake_routing_2014,
 abstract = {The research presented in this dissertation aims to develop computationally tractable models and algorithms for the reliable and efficient utilization of capacity restricted transportation networks via route selection and demand redistribution, motivated by the fact that traffic congestion in road networks is a major problem in urban communities. Three related topics are considered, 1) route planning with reliability guarantees, 2) system optimal dynamic traffic assignment, and 3) controlling user equilibrium departure times.Route planning can in many practical settings require finding a route that is both fast and reliable. However, in most operational settings, only deterministic shortest paths are considered, and even when the link travel-times are known to be stochastic the common approach is to simply minimize the expected travel-time. This approach does not account for the variance of the travel-time and gives no reliability guarantees. In many cases, travelers have hard deadlines or are willing to sacrifice some extra travel-time for increased travel-time reliability, such as in commercial routing applications where delivery guarantees need to be met and perishables need to be delivered on time. The research presented in this dissertation develops fast computation techniques for the reliable routing problem known as the stochastic on-time arrival (SOTA) problem, which provides a routing strategy that maximizes the probability of arriving at the destination within a fixed time budget. Selfish user optimal routing strategies can, however, lead to very inefficient traffic equilibria in congested traffic networks. This "Price of Anarchy" can be mitigated using system optimal coordinated routing algorithms. The dissertation considers the system optimal dynamic traffic assignment problem when only a subset of the network agents can be centrally coordinated. A road traffic dynamics model is developed based on the Lighthill-Williams-Richards partial differential equation and a corresponding multi-commodity junction solver. Full Lagrangian paths are assumed to be known for the controllable agents, while only the aggregate split ratios are required for the non-controllable (selfish) agents. The resulting non-linear optimal control problem is solved efficiently using the discrete adjoint method. Spill-back from under-capacitated off-ramps is one of the major causes of congestion during the morning commute. This spill-back induces a capacity drop on the freeway, which then creates a bottleneck for the mainline traffic that is passing by the off-ramp. Therefore, influencing the flow distribution of the vehicles that exit the freeway at the off-ramp can improve the throughput of freeway vehicles that pass this junction. The dissertation studies the generalized morning commute problem where vehicles exiting the freeway at the under-capacitated off-ramp have a fixed desired arrival time and a corresponding equilibrium departure time schedule, and presents strategies to manipulated this equilibrium to maximize throughput on the freeway via incentives or tolls.},
 author = {Samaranayake, Samitha},
 file = {/home/matt/Zotero/storage/ZF6RQXBM/Samaranayake - 2014 - Routing strategies for the reliable and efficient .pdf;/home/matt/Zotero/storage/6CWJPSLP/3r967409.html},
 language = {en},
 school = {UC Berkeley},
 title = {Routing Strategies for the Reliable and Efficient Utilization of Road Networks},
 year = {2014}
}

@article{samvelyan_starcraft_2019,
 author = {Samvelyan, Mikayel and Rashid, Tabish and {\noopsort{witt}}{de Witt}, Christian Schroeder and Farquhar, Gregory and Nardelli, Nantas and Rudner, Tim G. J. and Hung, Chia-Man and Torr, Philip H. S. and Foerster, Jakob and Whiteson, Shimon},
 journal = {ArXiv preprint},
 title = {The {{StarCraft Multi}}-{{Agent Challenge}}},
 url = {https://arxiv.org/abs/1902.04043},
 volume = {abs/1902.04043},
 year = {2019}
}

@article{sanchez_analysis_2011,
 author = {Sanchez, R. O. and Horowitz, R. and Varaiya, P.},
 journal = {Transportation Research Record},
 pages = {34--45},
 title = {Analysis of {{Queue Estimation Methods Using Wireless Magnetic Sensors}}},
 volume = {2229},
 year = {2011}
}

@phdthesis{sanchez_wireless_2012,
 abstract = {Intelligent Transportation Systems (ITS) are cost-effective measures to manage congestion due to increasing demand by improving the efficiency of existing transportation infrastructure. Traffic detection and surveillance play a pivotal role in deploying these technologies in the field. This dissertation continues the work that has been done in recent years in relation to the use of wireless magnetic sensor networks in transportation systems. As part of the effort to improve vehicle detection system technologies so that better management strategies can be implemented in the field, the work presented here focuses on advancing the use of wireless magnetic sensors in Intelligent Transportation Systems. This dissertation addresses improvements in algorithmic tools that advance the use of wireless magnetic sensors for both freeways and arterials. The applications addressed here include on-ramp queue estimation, arterial link vehicle-count, travel time estimation on heavily congested arterial streets, travel time and link vehicle-count in freeways, truck re-identification along long freeway segments, as well as cost-effective vehicle classification. The overall goal of this dissertation is to advance the use of these basic detection technologies to roles that extend beyond basic vehicle detection.A vehicle re-identification system, which relies on matching vehicle signatures from wireless magnetic sensors is modified to improve its performance for stop-and-go traffic conditions and is extended so that it can be used for truck re-identification along long freeway segments. The modifications to the algorithm address problems observed when vehicles stop or accelerate/decelerate as they go through the sensors. The modified system was tested to ensure that it overcame the deficiencies imposed by the original system. The extension of the vehicle re-identification system, presented as the iterative vehicle re-identification system, addresses traffic dynamics observed when vehicles travel along long road segments, in particular, vehicle overtaking. The system was tested extensively to ensure that it can be deployed for truck re-identification along long freeway segments, e.g., in between weigh-in-motion (WIM) stations.A link vehicle-count and a travel time estimator based on flow-measurements and vehicle re-identification data were studied at a freeway on-ramp, arterial segments as well as at freeway segments. The results show that the estimators are reliable and accurate, and are suitable for real-time traffic responsive management strategies that require precise link vehicle-count and/or vehicle travel time information, such as ramp metering, speed control and traffic intersection control.Vehicle classification, which utilizes a single wireless magnetic sensor installed in the middle of a freeway lane is also presented. The approach uses a two stage binary support vector machine (SVM) classifier based on features extracted from vehicle signatures. This is a cost effective classification system that uses a small subset of data efficiently extracted from the magnetic signal measured by the sensor. The results showed that vehicles can be reliably and accurately classified into passenger vehicles and trucks, and once trucks are extracted, this group can be further divided, with lower accuracy and consistency, into two groups: small trucks and large trucks.Finally, this dissertation presents a systematic tool for tuning vehicle re-identification parameters and evaluating performance. This tool uses different plots, metrics and algorithms to evaluate the output of the vehicle re-identification algorithm as well as estimates based on it, i.e., link vehicle-count and vehicle travel time.},
 author = {Sanchez, Rene Omar},
 file = {/home/matt/Zotero/storage/5IEEVBCQ/Sanchez - 2012 - Wireless Magnetic Sensor Applications in Transport.pdf;/home/matt/Zotero/storage/LC9K5EY9/5d2006gr.html},
 language = {en},
 school = {UC Berkeley},
 title = {Wireless {{Magnetic Sensor Applications}} in {{Transportation Infrastructure}}},
 year = {2012}
}

@inproceedings{sanh_movement_2020,
 author = {Victor Sanh and
Thomas Wolf and
Alexander M. Rush},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/Sanh0R20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Movement Pruning: Adaptive Sparsity by Fine-Tuning},
 url = {https://proceedings.neurips.cc/paper/2020/hash/eae15aabaa768ae4a5993a8a4f4fa6e4-Abstract.html},
 year = {2020}
}

@techreport{santero_virtual_2005,
 author = {Santero, N. and Nokes, W. and Harvey, J.},
 institution = {{California PATH, University of California, Berkeley}},
 number = {UCB-ITS-PWP-2005-05},
 title = {Virtual {{Weigh Stations}} in {{California}}: {{A Preliminary Cost}}-{{Effectiveness Analysis}}},
 year = {2005}
}

@article{santos_road_2006,
 author = {Santos, G. and Fraser, G.},
 journal = {Economic Policy},
 pages = {265--310},
 title = {Road Pricing: Lessons from {{London}}},
 year = {2006}
}

@inproceedings{sax_learning_2019,
 abstract = {How much does having visual priors about the world (e.g. the fact that the world is 3D) assist in learning to perform downstream motor tasks (e.g. navigating a complex environment)? What are the consequences of not utilizing such visual priors in learning? We study these questions by integrating a generic perceptual skill set (a distance estimator, an edge detector, etc.) within a reinforcement learning framework (see Fig. 1). This skill set (``mid-level vision'') provides the policy with a more processed state of the world compared to raw images.},
 archiveprefix = {arXiv},
 author = {Sax, Alexander and Zhang, Jeffrey O. and Emi, Bradley and Zamir, Amir and Savarese, Silvio and Guibas, Leonidas and Malik, Jitendra},
 booktitle = {3rd {{Conference}} on {{Robot Learning}} ({{CoRL}})},
 eprint = {1912.11121},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/3HF2V24B/Sax et al. - 2019 - Learning to Navigate Using Mid-Level Visual Priors.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Learning to {{Navigate Using Mid}}-{{Level Visual Priors}}},
 year = {2019}
}

@article{scarselli_graph_2009,
 author = {Scarselli, F. and Gori, M. and {Ah Chung Tsoi} and Hagenbuchner, M. and Monfardini, G.},
 doi = {10.1109/TNN.2008.2005605},
 file = {/home/matt/Zotero/storage/9I99YQJW/scarselli_graphnn.pdf},
 issn = {1045-9227, 1941-0093},
 journal = {IEEE Transactions on Neural Networks},
 number = {1},
 pages = {61--80},
 title = {The {{Graph Neural Network Model}}},
 volume = {20},
 year = {2009}
}

@article{schaller_new_2010,
 author = {Schaller, B.},
 journal = {Transportation Research Part C},
 pages = {266?273},
 title = {New {{York City}}?S Congestion Pricing Experience and Implications for Road Pricing Acceptance in the {{United States}}},
 volume = {17},
 year = {2010}
}

@article{schleif_indefinite_2015,
 author = {Schleif, Frank-Michael and Tino, Peter},
 doi = {10.1162/NECO_a_00770},
 file = {/home/matt/Zotero/storage/DV7KW9YQ/Schleif and Tino - 2015 - Indefinite Proximity Learning A Review.pdf},
 issn = {0899-7667, 1530-888X},
 journal = {Neural Computation},
 language = {en},
 number = {10},
 pages = {2039--2096},
 shorttitle = {Indefinite {{Proximity Learning}}},
 title = {Indefinite {{Proximity Learning}}: {{A Review}}},
 volume = {27},
 year = {2015}
}

@article{schleif_indefinite_2017,
 author = {Schleif, Frank-Michael and Tino, Peter},
 doi = {10.1016/j.patcog.2017.06.003},
 file = {/home/matt/Zotero/storage/SHMTQYLG/Schleif and Tino - 2017 - Indefinite Core Vector Machine.pdf},
 issn = {00313203},
 journal = {Pattern Recognition},
 language = {en},
 pages = {187--195},
 title = {Indefinite {{Core Vector Machine}}},
 volume = {71},
 year = {2017}
}

@inproceedings{schlichtkrull_interpreting_2021,
 author = {Michael Sejr Schlichtkrull and
Nicola De Cao and
Ivan Titov},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/SchlichtkrullCT21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Interpreting Graph Neural Networks for {NLP} With Differentiable Edge
Masking},
 url = {https://openreview.net/forum?id=WznmQa42ZAx},
 year = {2021}
}

@inproceedings{schlichtkrull_interpreting_2021-1,
 author = {Michael Sejr Schlichtkrull and
Nicola De Cao and
Ivan Titov},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/SchlichtkrullCT21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Interpreting Graph Neural Networks for {NLP} With Differentiable Edge
Masking},
 url = {https://openreview.net/forum?id=WznmQa42ZAx},
 year = {2021}
}

@article{schmeckpeper_learning_2019,
 author = {Schmeckpeper, Karl and Xie, Annie and Rybkin, Oleh and Tian, Stephen and Daniilidis, Kostas and Levine, Sergey and Finn, Chelsea},
 journal = {ArXiv preprint},
 title = {Learning {{Predictive Models From Observation}} and {{Interaction}}},
 url = {https://arxiv.org/abs/1912.12773},
 volume = {abs/1912.12773},
 year = {2019}
}

@inproceedings{schmerling_multimodal_2018,
 address = {{Brisbane, QLD}},
 author = {Schmerling, Edward and Leung, Karen and Vollprecht, Wolf and Pavone, Marco},
 booktitle = {2018 {{IEEE International Conference}} on {{Robotics}} and {{Automation}} ({{ICRA}})},
 doi = {10.1109/ICRA.2018.8460766},
 isbn = {978-1-5386-3081-5},
 pages = {3399--3406},
 publisher = {{IEEE}},
 title = {Multimodal {{Probabilistic Model}}-{{Based Planning}} for {{Human}}-{{Robot Interaction}}},
 year = {2018}
}

@article{schmidhuber_deep_2015,
 author = {Schmidhuber, J{\"u}rgen},
 doi = {10.1016/j.neunet.2014.09.003},
 file = {/home/matt/Documents/Papers/deepLearning.pdf},
 issn = {08936080},
 journal = {Neural Networks},
 language = {en},
 pages = {85--117},
 shorttitle = {Deep Learning in Neural Networks},
 title = {Deep Learning in Neural Networks: {{An}} Overview},
 volume = {61},
 year = {2015}
}

@article{schneider_null_2015,
 abstract = {Null hypothesis statistical significance tests (NHST) are widely used in quantitative research in the empirical sciences including scientometrics. Nevertheless, since their introduction nearly a century ago significance tests have been controversial. Many researchers are not aware of the numerous criticisms raised against NHST. As practiced, NHST has been characterized as a `null ritual' that is overused and too often misapplied and misinterpreted. NHST is in fact a patchwork of two fundamentally different classical statistical testing models, often blended with some wishful quasi-Bayesian interpretations. This is undoubtedly a major reason why NHST is very often misunderstood. But NHST also has intrinsic logical problems and the epistemic range of the information provided by such tests is much more limited than most researchers recognize. In this article we introduce to the scientometric community the theoretical origins of NHST, which is mostly absent from standard statistical textbooks, and we discuss some of the most prevalent problems relating to the practice of NHST and trace these problems back to the mix-up of the two different theoretical origins. Finally, we illustrate some of the misunderstandings with examples from the scientometric literature and bring forward some modest recommendations for a more sound practice in quantitative data analysis.},
 author = {Schneider, Jesper W.},
 doi = {10.1007/s11192-014-1251-5},
 file = {/home/matt/Zotero/storage/UHWAGY3H/Schneider - 2015 - Null hypothesis significance tests. A mix-up of tw.pdf},
 issn = {0138-9130, 1588-2861},
 journal = {Scientometrics},
 language = {en},
 number = {1},
 pages = {411--432},
 shorttitle = {Null Hypothesis Significance Tests. {{A}} Mix-up of Two Different Theories},
 title = {Null Hypothesis Significance Tests. {{A}} Mix-up of Two Different Theories: The Basis for Widespread Confusion and Numerous Misinterpretations},
 volume = {102},
 year = {2015}
}

@article{schoettler_deep_2019,
 author = {Schoettler, Gerrit and Nair, Ashvin and Luo, Jianlan and Bahl, Shikhar and Ojea, Juan Aparicio and Solowjow, Eugen and Levine, Sergey},
 journal = {ArXiv preprint},
 title = {Deep {{Reinforcement Learning}} for {{Industrial Insertion Tasks}} with {{Visual Inputs}} and {{Natural Rewards}}},
 url = {https://arxiv.org/abs/1906.05841},
 volume = {abs/1906.05841},
 year = {2019}
}

@book{scholkopf_learning_2002,
 author = {Sch{\"o}lkopf, Bernhard and Smola, Alexander J.},
 doi = {10.7551/mitpress/4175.001.0001},
 isbn = {978-0-262-25693-3},
 language = {en},
 publisher = {{The MIT Press}},
 shorttitle = {Learning with {{Kernels}}},
 title = {Learning with {{Kernels}}: {{Support Vector Machines}}, {{Regularization}}, {{Optimization}}, and {{Beyond}}},
 year = {2002}
}

@article{schreckenberg_discrete_1995,
 author = {Schreckenberg, M. and Schadschneider, A. and Nagel, K. and Ito, N.},
 doi = {10.1103/PhysRevE.51.2939},
 file = {/home/matt/Zotero/storage/UNZNFAV7/Schreckenberg et al. - 1995 - Discrete stochastic models for traffic flow.pdf},
 issn = {1063-651X, 1095-3787},
 journal = {Physical Review E},
 language = {en},
 number = {4},
 pages = {2939--2949},
 title = {Discrete Stochastic Models for Traffic Flow},
 volume = {51},
 year = {1995}
}

@inproceedings{schulman_high-dimensional_2016,
 author = {John Schulman and
Philipp Moritz and
Sergey Levine and
Michael I. Jordan and
Pieter Abbeel},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/SchulmanMLJA15.bib},
 booktitle = {4th International Conference on Learning Representations, {ICLR} 2016,
San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {High-Dimensional Continuous Control Using Generalized Advantage Estimation},
 url = {http://arxiv.org/abs/1506.02438},
 year = {2016}
}

@article{schulman_proximal_2017,
 author = {Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
 journal = {ArXiv preprint},
 title = {Proximal {{Policy Optimization Algorithms}}},
 url = {https://arxiv.org/abs/1707.06347},
 volume = {abs/1707.06347},
 year = {2017}
}

@inproceedings{schulman_trust_2015,
 author = {John Schulman and
Sergey Levine and
Pieter Abbeel and
Michael I. Jordan and
Philipp Moritz},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/SchulmanLAJM15.bib},
 booktitle = {Proceedings of the 32nd International Conference on Machine Learning,
{ICML} 2015, Lille, France, 6-11 July 2015},
 editor = {Francis R. Bach and
David M. Blei},
 pages = {1889--1897},
 publisher = {JMLR.org},
 series = {{JMLR} Workshop and Conference Proceedings},
 timestamp = {Wed, 29 May 2019 01:00:00 +0200},
 title = {Trust Region Policy Optimization},
 url = {http://proceedings.mlr.press/v37/schulman15.html},
 volume = {37},
 year = {2015}
}

@article{schwarting_planning_2018,
 author = {Schwarting, Wilko and {Alonso-Mora}, Javier and Rus, Daniela},
 journal = {ArXiv preprint},
 title = {Planning and {{Decision}}-{{Making}} for {{Autonomous Vehicles}}},
 url = {https://arxiv.org/abs/s},
 volume = {abs/s},
 year = {20s}
}

@article{schwartz_sous-espaces_1964,
 author = {Schwartz, Laurent},
 doi = {10.1007/BF02786620},
 file = {/home/matt/Zotero/storage/BKZAL828/BF02786620.pdf},
 journal = {Journal d'Analyse Math\'ematique},
 number = {1},
 pages = {115--256},
 title = {Sous-Espaces Hilbertiens d'espaces Vectoriels Topologiques et Noyaux Associ\'es ({{Noyaux}} Reproduisants)},
 volume = {13},
 year = {1964}
}

@inproceedings{sedghi_singular_2019,
 author = {Hanie Sedghi and
Vineet Gupta and
Philip M. Long},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/SedghiGL19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {The Singular Values of Convolutional Layers},
 url = {https://openreview.net/forum?id=rJevYoA9Fm},
 year = {2019}
}

@article{seely_non-symmetric_1919,
 author = {Seely, Dr. Caroline E.},
 doi = {10.2307/1967866},
 file = {/home/matt/Zotero/storage/2EEKDH3Q/Seely - 1919 - Non-Symmetric Kernels of Positive Type.pdf},
 issn = {0003486X},
 journal = {The Annals of Mathematics},
 language = {en},
 number = {3},
 pages = {172},
 title = {Non-{{Symmetric Kernels}} of {{Positive Type}}},
 volume = {20},
 year = {1919}
}

@article{seiler_disturbance_2004,
 author = {Seiler, Peter and Pant, Aniruddha and Hedrick, Karl},
 journal = {Automatic Control, IEEE Transactions on},
 number = {10},
 pages = {1835--1842},
 title = {Disturbance Propagation in Vehicle Strings},
 volume = {49},
 year = {2004}
}

@inproceedings{seita_zpd_2019,
 abstract = {Learning from demonstrations is a popular tool for accelerating and reducing the exploration requirements of reinforcement learning. When providing expert demonstrations to human students, we know that the demonstrations must fall within a particular range of difficulties called the ``Zone of Proximal Development (ZPD)'' [6, 33]. If they are too easy the student learns nothing, but if they are too difficult the student is unable to follow along. This raises the question: Given a set of potential demonstrators, which among them is best suited for teaching any particular learner? Prior work, such as the popular Deep Q-learning from Demonstrations (DQfD) algorithm has generally focused on single demonstrators. In this work we consider the problem of choosing among multiple demonstrators of varying skill levels. Our results align with intuition from human learners: it is not always the best policy to draw demonstrations from the best performing demonstrator (in terms of reward). We show that careful selection of teaching strategies can result in sample efficiency gains in the learner's environment across nine Atari games.},
 archiveprefix = {arXiv},
 author = {Seita, Daniel and Chan, David and Rao, Roshan and Tang, Chen and Zhao, Mandi and Canny, John},
 booktitle = {Deep {{Reinforcement Learning Workshop}} at {{NeurIPS}} 2019},
 eprint = {1910.12154},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/RTCNG5C6/Seita et al. - 2019 - ZPD Teaching Strategies for Deep Reinforcement Lea.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {{{ZPD Teaching Strategies}} for {{Deep Reinforcement Learning}} from {{Demonstrations}}},
 year = {2019}
}

@inproceedings{sennrich_neural_2016,
 address = {Berlin, Germany},
 author = {Sennrich, Rico  and
Haddow, Barry  and
Birch, Alexandra},
 booktitle = {Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)},
 doi = {10.18653/v1/P16-1162},
 pages = {1715--1725},
 publisher = {Association for Computational Linguistics},
 title = {Neural Machine Translation of Rare Words with Subword Units},
 url = {https://aclanthology.org/P16-1162},
 year = {2016}
}

@article{seo_structured_2016,
 author = {Seo, Youngjoo and Defferrard, Micha{\"e}l and Vandergheynst, Pierre and Bresson, Xavier},
 journal = {ArXiv preprint},
 title = {Structured {{Sequence Modeling}} with {{Graph Convolutional Recurrent Networks}}},
 url = {https://arxiv.org/abs/1612.07659},
 volume = {abs/1612.07659},
 year = {2016}
}

@article{seo_traffic_2017,
 abstract = {Traffic state estimation (TSE) refers to the process of the inference of traffic state variables (i.e., flow, density, speed and other equivalent variables) on road segments using partially observed traffic data. It is a key component of traffic control and operations, because traffic variables are measured not everywhere due to technological and financial limitations, and their measurement is noisy. Therefore, numerous studies have proposed TSE methods relying on various approaches, traffic flow models, and input data. In this review article, we conduct a survey of highway TSE methods, a topic which has gained great attention in the recent decades.},
 author = {Seo, Toru and Bayen, Alexandre M. and Kusakabe, Takahiko and Asakura, Yasuo},
 doi = {10.1016/j.arcontrol.2017.03.005},
 file = {/home/matt/Zotero/storage/BZ2I7YZ5/Seo et al. - 2017 - Traffic state estimation on highway A comprehensi.pdf},
 issn = {13675788},
 journal = {Annual Reviews in Control},
 language = {en},
 pages = {128--151},
 shorttitle = {Traffic State Estimation on Highway},
 title = {Traffic State Estimation on Highway: {{A}} Comprehensive Survey},
 volume = {43},
 year = {2017}
}

@article{seshia_semantic_2020,
 abstract = {Models produced by machine-learning (ML) algorithms, especially deep neural networks, are being used in diverse domains where trustworthiness is a concern. The field of adversarial machine learning investigates the generation of inputs, termed adversarial examples, that cause the ML model to produce incorrect output. However, most existing approaches to generating adversarial examples and devising robust ML algorithms mostly ignore the semantics and context of the overall system containing the ML component. In addition, one may want to prioritize the search for adversarial examples towards those that significantly modify the desired semantics of the overall system. Along the same lines, existing algorithms for constructing robust ML algorithms ignore the specification of the overall system. Such considerations are particularly relevant in resourceconstrained environments. In this paper, we present the paradigm of semantic adversarial machine learning, in which the semantics and specification of the overall system has a crucial role to play in this line of research. We present preliminary research results, and discuss directions for future work.},
 author = {Seshia, Sanjit A. and Jha, Somesh and Dreossi, Tommaso},
 doi = {10.1109/MDAT.2020.2968274},
 file = {/home/matt/Zotero/storage/VXTZKEI5/Seshia et al. - 2020 - Semantic Adversarial Deep Learning.pdf},
 issn = {2168-2356, 2168-2364},
 journal = {IEEE Design \& Test},
 language = {en},
 pages = {1--1},
 title = {Semantic {{Adversarial Deep Learning}}},
 year = {2020}
}

@techreport{shah_detroit_2001,
 author = {Shah, Vaishali P. and Wunderlich, Karl},
 institution = {{Federal Highway Administration}},
 number = {DTFH61-00-C-0001},
 title = {Detroit {{Freeway Corridor ITS Evaluation}}},
 year = {2001}
}

@inproceedings{shah_feasibility_2019,
 author = {Rohin Shah and
Noah Gundotra and
Pieter Abbeel and
Anca D. Dragan},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ShahGAD19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {5670--5679},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {On the Feasibility of Learning, Rather than Assuming, Human Biases
for Reward Inference},
 url = {http://proceedings.mlr.press/v97/shah19a.html},
 volume = {97},
 year = {2019}
}

@article{shahsavari_short-term_nodate,
 author = {Shahsavari, Behrooz and Abbeel, Pieter and Horowitz, Roberto},
 journal = {Transportation Research Part C},
 title = {Short-{{Term Traffic Forecasting Based}} on {{Learning Spatio}}-{{Temporal Dynamics}} of {{Network}} by {{Graph Neural Networks}}},
 year = {submitted}
}

@article{shalev-shwartz_safe_2016,
 author = {{Shalev-Shwartz}, Shai and Shammah, Shaked and Shashua, Amnon},
 journal = {ArXiv preprint},
 title = {Safe, {{Multi}}-{{Agent}}, {{Reinforcement Learning}} for {{Autonomous Driving}}},
 url = {https://arxiv.org/abs/1610.03295},
 volume = {abs/1610.03295},
 year = {2016}
}

@inproceedings{shankar_neural_2020,
 author = {Vaishaal Shankar and
Alex Fang and
Wenshuo Guo and
Sara Fridovich{-}Keil and
Jonathan Ragan{-}Kelley and
Ludwig Schmidt and
Benjamin Recht},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/ShankarFGFRSR20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {8614--8623},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Neural Kernels Without Tangents},
 url = {http://proceedings.mlr.press/v119/shankar20a.html},
 volume = {119},
 year = {2020}
}

@article{shankar_systematic_2019,
 author = {Shankar, Vaishaal and Dave, Achal and Roelofs, Rebecca and Ramanan, Deva and Recht, Benjamin and Schmidt, Ludwig},
 journal = {ArXiv preprint},
 title = {A Systematic Framework for Natural Perturbations from Videos},
 url = {https://arxiv.org/abs/1906.02168},
 volume = {abs/1906.02168},
 year = {2019}
}

@inproceedings{sharma_dynamics-aware_2020,
 author = {Archit Sharma and
Shixiang Gu and
Sergey Levine and
Vikash Kumar and
Karol Hausman},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/SharmaGLKH20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Dynamics-Aware Unsupervised Discovery of Skills},
 url = {https://openreview.net/forum?id=HJgLZR4KvH},
 year = {2020}
}

@article{sharma_input-output_2007,
 author = {Sharma, A. and Bullock, D. M. and Bonneson, J. A.},
 journal = {Transportation Research Record},
 pages = {69--80},
 title = {Input-output and Hybrid Techniques for Real-Time Prediction of Delay and Maximum Queue Length at Signalized Intersections},
 volume = {2035},
 year = {2007}
}

@article{sharman_driverless_2014,
 author = {Sharman, A.},
 journal = {The Financial Times},
 title = {Driverless Cars Wait for Green Light},
 year = {2014}
}

@inproceedings{shaw_self-attention_2018,
 address = {New Orleans, Louisiana},
 author = {Shaw, Peter  and
Uszkoreit, Jakob  and
Vaswani, Ashish},
 booktitle = {Proceedings of the 2018 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 2 (Short Papers)},
 doi = {10.18653/v1/N18-2074},
 pages = {464--468},
 publisher = {Association for Computational Linguistics},
 title = {Self-Attention with Relative Position Representations},
 url = {https://aclanthology.org/N18-2074},
 year = {2018}
}

@article{shchur_pitfalls_2019,
 author = {Shchur, Oleksandr and Mumme, Maximilian and Bojchevski, Aleksandar and G{\"u}nnemann, Stephan},
 journal = {ArXiv preprint},
 title = {Pitfalls of {{Graph Neural Network Evaluation}}},
 url = {https://arxiv.org/abs/1811.05868},
 volume = {abs/1811.05868},
 year = {2018}
}

@article{shelhamer_blurring_2019,
 author = {Shelhamer, Evan and Wang, Dequan and Darrell, Trevor},
 journal = {ArXiv preprint},
 title = {Blurring the {{Line Between Structure}} and {{Learning}} to {{Optimize}} and {{Adapt Receptive Fields}}},
 url = {https://arxiv.org/abs/1904.11487},
 volume = {abs/1904.11487},
 year = {2019}
}

@article{shen_detailed_2012,
 author = {Shen, Jingjing and Jin, Xiaogang},
 doi = {10.1016/j.gmod.2012.04.002},
 file = {/home/matt/Zotero/storage/7IX5LJIK/shen_jin_iidm_2012.pdf;/home/matt/Zotero/storage/YTZ9VQN6/shen_jin_iidm_2012.pdf},
 issn = {15240703},
 journal = {Graphical Models},
 language = {en},
 number = {5},
 pages = {265--282},
 title = {Detailed Traffic Animation for Urban Road Networks},
 volume = {74},
 year = {2012}
}

@inproceedings{shen_q-bert_2019,
 author = {Sheng Shen and
Zhen Dong and
Jiayu Ye and
Linjian Ma and
Zhewei Yao and
Amir Gholami and
Michael W. Mahoney and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/ShenDYMYGMK20.bib},
 booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
2020, The Thirty-Second Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
February 7-12, 2020},
 pages = {8815--8821},
 publisher = {{AAAI} Press},
 timestamp = {Tue, 02 Feb 2021 00:00:00 +0100},
 title = {{Q-BERT:} Hessian Based Ultra Low Precision Quantization of {BERT}},
 url = {https://aaai.org/ojs/index.php/AAAI/article/view/6409},
 year = {2020}
}

@article{shen_rethinking_2020,
 author = {Shen, Zhiqiang and Liu, Zechun and Liu, Zhuang and Savvides, Marios and Darrell, Trevor},
 journal = {ArXiv preprint},
 title = {Rethinking {{Image Mixture}} for {{Unsupervised Visual Representation Learning}}},
 url = {https://arxiv.org/abs/2003.05438},
 volume = {abs/2003.05438},
 year = {2020}
}

@article{shen_rethinking_2020-1,
 author = {Shen, Sheng and Yao, Zhewei and Gholami, Amir and Mahoney, Michael and Keutzer, Kurt},
 journal = {ArXiv preprint},
 title = {Rethinking {{Batch Normalization}} in {{Transformers}}},
 url = {https://arxiv.org/abs/2003.07845},
 volume = {abs/2003.07845},
 year = {2020}
}

@inproceedings{shen2019discovery,
 author = {Xi Shen and
Alexei A. Efros and
Mathieu Aubry},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/ShenEA19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00950},
 pages = {9278--9287},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Discovering Visual Patterns in Art Collections With Spatially-Consistent
Feature Learning},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Shen\_Discovering\_Visual\_Patterns\_in\_Art\_Collections\_With\_Spatially-Consistent\_Feature\_Learning\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{shepard_representation_2015,
 abstract = {Four representations and parametrizations of orthogonal matrices Q{$\in$}Rm \texttimes{} n in terms of the minimal number of essential parameters \{{$\varphi$}\} are discussed: the exponential representation, the Householder reflector representation, the Givens rotation representation, and the rational Cayley transform representation. Both square n = m and rectangular n {$<$} m situations are considered. Two separate kinds of parametrizations are considered: one in which the individual columns of Q are distinct, the Stiefel manifold, and the other in which only span(Q) is significant, the Grassmann manifold. The practical issues of numerical stability, continuity, and uniqueness are discussed. The computation of Q in terms of the essential parameters \{{$\varphi$}\}, and also the extraction of \{{$\varphi$}\} for a given Q are considered for all of the parametrizations. The transformation of gradient arrays between the Q and \{{$\varphi$}\} variables is discussed for all representations. It is our hope that developers of new methods will benefit from this comparative presentation of an important but rarely analyzed subject.},
 author = {Shepard, Ron and Brozell, Scott R. and Gidofalvi, Gergely},
 doi = {10.1021/acs.jpca.5b02015},
 file = {/home/matt/Zotero/storage/UPIIDTLS/Shepard et al. - 2015 - The Representation and Parametrization of Orthogon.pdf;/home/matt/Zotero/storage/MQM2Y8EX/acs.jpca.html},
 issn = {1089-5639},
 journal = {The Journal of Physical Chemistry A},
 number = {28},
 pages = {7924--7939},
 title = {The {{Representation}} and {{Parametrization}} of {{Orthogonal Matrices}}},
 volume = {119},
 year = {2015}
}

@article{sherali_estimation_2001,
 author = {Sherali, H. D. and Park, T.},
 journal = {Transportation Research B},
 pages = {217--235},
 title = {Estimation of Dynamic Origin{$\pm$}destination Trip Tables for a General Network},
 volume = {35},
 year = {2001}
}

@article{shi_driving_2019,
 author = {Shi, Tianyu and Wang, Pin and Cheng, Xuxin and Chan, Ching-Yao and Huang, Ding},
 journal = {ArXiv preprint},
 title = {Driving {{Decision}} and {{Control}} for {{Autonomous Lane Change}} Based on {{Deep Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1904.10171},
 volume = {abs/1904.10171},
 year = {2019}
}

@phdthesis{shi_flexible_2018,
 abstract = {Unlike conventional generators, the output of a renewable generator is only partially controlable and unpredictable. Consequently, its output level exhibits wide variability. The increasing amount of such kind of renewable resources in the generation mix of the electric power infrastructure poses new challenges to system operations. Due to the limitations of storage in current power systems, demand and supply of electricity must be matched instantaneously. Moreover, the flow of power is governed by Kirchhoff's laws and is prone to congestion. In order to serve load reliably in power systems with large-scale renewable integration, extreme ramping requirements on conventional generation resources will be imposed. The system operators could mitigate those requirements by deploying more reserves or increased amount of flexible generation resources which could undermine both the economic and environmental objectives of deploying renewable resources. Instead of utilizing the flexibility provided by conventional generation, we will focus on exploiting flexibility from the transmission system to mitigate the uncertainty and variability of renewable generation for power systems day-ahead scheduling.In this dissertation, we focus on harvesting flexibility from the transmission system to mitigate the uncertainty of renewable generation. There are two aspects of the such flexibility. First, we allow actively controlling the topology of the transmission network by switching on or off transmission lines as a recourse option. Second, the transmission lines can temporally adopt higher ratings to avoid the underutilization of the line capacity caused by the conventional conservativeness in line rating calculations. We adopt the two-stage stochastic unit commitment model for the power system day-ahead scheduling problem. Both transmission switching decisions and flexible line rating decisions are modeled as binary decisions in the second stage when renewable generation is realized. A scheme that decomposes an interconnected commercial system into zones is proposed to solve this large-scale stochastic mixed integer programming problem within a reasonable amount of time. In the sub-problem for each zone, conventional generators are separated into a set of slow-ramping generators and a set of fast-ramping generators. The commitment decisions of slow generators are first-stage decisions which are made before the realization of renewable generation. The commitment decisions of fast generators and the dispatch decisions are second-stage decisions. Topology control decisions through switching on/off transmission lines and flexible line rating decisions are modeled as recourse actions. Such recourse actions provide the possibility of actively control the transmission system in response to the variability and the uncertainty of renewable generations. Comparing with deploying more flexible conventional generators which are expensive, flexible transmission network recourse incurs no additional cost other than the cost associated with the abrasions of breakers. We provide demonstration studies based on the IEEE 118 system and a network representing the Central European system where there are over 650 conventional generators, 679 buses, and around 1000 transmission lines.We observe that the operating cost can be reduced by over 10\% for the IEEE 118 system with purely topology control recourse. The cost reduction for the Central European system is over 3\%, and substantial reduction is observed for some control areas with topology control recourse. The operating cost can be reduced if flexible line rating recourse is included.},
 author = {Shi, Jiaying},
 file = {/home/matt/Zotero/storage/D22LC234/Shi - 2018 - Flexible Transmission Networks for Renewables Inte.pdf;/home/matt/Zotero/storage/SW9QA9MG/5p5119rd.html},
 language = {en},
 school = {UC Berkeley},
 title = {Flexible {{Transmission Networks}} for {{Renewables Integration}}},
 year = {2018}
}

@inproceedings{shin_synthetic_2019,
 author = {Richard Shin and
Neel Kant and
Kavi Gupta and
Chris Bender and
Brandon Trabucco and
Rishabh Singh and
Dawn Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ShinKGBTSS19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Synthetic Datasets for Neural Program Synthesis},
 url = {https://openreview.net/forum?id=ryeOSnAqYm},
 year = {2019}
}

@article{shiomi_multilane_2015,
 author = {Shiomi, Yasuhiro and Taniguchi, Tomoki and Uno, Nobuhiro and Shimamoto, Hiroshi and Nakamura, Toshiyuki},
 doi = {10.1016/j.trc.2015.07.002},
 file = {/home/matt/Zotero/storage/7ZJTCVP8/2015_TRC_firstorder_multilane.pdf;/home/matt/Zotero/storage/BSA845JM/2015_TRC_firstorder_multilane.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {198--215},
 title = {Multilane First-Order Traffic Flow Model with Endogenous Representation of Lane-Flow Equilibrium},
 volume = {59},
 year = {2015}
}

@article{shladover_cooperative_2012,
 author = {Shladover, S. and Lu, X.-Y.},
 journal = {Transportation Research Record Journal of the Transportation Research Board},
 title = {Cooperative {{Adaptive Cruise Control Impact}} on Freeway Traffic Flow},
 volume = {1},
 year = {2012}
}

@article{shoup_free_2007,
 author = {Shoup, D.},
 journal = {Cruising for parking},
 title = {Free Parking or Free Markets},
 volume = {30},
 year = {2007}
}

@article{shoup_free_2011,
 author = {Shoup, D.},
 journal = {Access Magazine},
 title = {Free Parking or Free Markets},
 volume = {38},
 year = {2011}
}

@inproceedings{shrestha_approximating_2019,
 address = {{Knoxville TN USA}},
 author = {Shrestha, Amar and Fang, Haowen and Wu, Qing and Qiu, Qinru},
 booktitle = {Proceedings of the {{International Conference}} on {{Neuromorphic Systems}}},
 doi = {10.1145/3354265.3354275},
 file = {/home/matt/Zotero/storage/SEYICPUH/Shrestha et al. - 2019 - Approximating Back-propagation for a Biologically .pdf},
 isbn = {978-1-4503-7680-8},
 language = {en},
 pages = {1--8},
 publisher = {{ACM}},
 title = {Approximating {{Back}}-Propagation for a {{Biologically Plausible Local Learning Rule}} in {{Spiking Neural Networks}}},
 year = {2019}
}

@article{silver_mastering_2016,
 author = {Silver, David and Huang, Aja and Maddison, Chris J. and Guez, Arthur and Sifre, Laurent and {\noopsort{driessche}}{van den Driessche}, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and Dieleman, Sander and Grewe, Dominik and Nham, John and Kalchbrenner, Nal and Sutskever, Ilya and Lillicrap, Timothy and Leach, Madeleine and Kavukcuoglu, Koray and Graepel, Thore and Hassabis, Demis},
 doi = {10.1038/nature16961},
 file = {/home/matt/Zotero/storage/2AE58PRJ/Silver et al. - 2016 - Mastering the game of Go with deep neural networks.pdf},
 issn = {0028-0836, 1476-4687},
 journal = {Nature},
 language = {en},
 number = {7587},
 pages = {484--489},
 title = {Mastering the Game of {{Go}} with Deep Neural Networks and Tree Search},
 volume = {529},
 year = {2016}
}

@article{silver_mastering_2017,
 author = {Silver, David and Schrittwieser, Julian and Simonyan, Karen and Antonoglou, Ioannis and Huang, Aja and Guez, Arthur and Hubert, Thomas and Baker, Lucas and Lai, Matthew and Bolton, Adrian and Chen, Yutian and Lillicrap, Timothy and Hui, Fan and Sifre, Laurent and {\noopsort{driessche}}{van den Driessche}, George and Graepel, Thore and Hassabis, Demis},
 doi = {10.1038/nature24270},
 file = {/home/matt/Zotero/storage/3FE94G9W/Silver et al. - 2017 - Mastering the game of Go without human knowledge.pdf},
 issn = {0028-0836, 1476-4687},
 journal = {Nature},
 language = {en},
 number = {7676},
 pages = {354--359},
 title = {Mastering the Game of {{Go}} without Human Knowledge},
 volume = {550},
 year = {2017}
}

@article{simms_freeway_2003,
 author = {Simms, Julia A.},
 journal = {San Diego Source},
 title = {Freeway Widening to Begin Soon},
 year = {2003}
}

@inproceedings{simonovsky_dynamic_2017,
 author = {Martin Simonovsky and
Nikos Komodakis},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/SimonovskyK17.bib},
 booktitle = {2017 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2017, Honolulu, HI, USA, July 21-26, 2017},
 doi = {10.1109/CVPR.2017.11},
 pages = {29--38},
 publisher = {{IEEE} Computer Society},
 timestamp = {Tue, 14 Nov 2017 00:00:00 +0100},
 title = {Dynamic Edge-Conditioned Filters in Convolutional Neural Networks
on Graphs},
 url = {https://doi.org/10.1109/CVPR.2017.11},
 year = {2017}
}

@article{singh_end--end_2019,
 author = {Singh, Avi and Yang, Larry and Hartikainen, Kristian and Finn, Chelsea and Levine, Sergey},
 journal = {ArXiv preprint},
 title = {End-to-{{End Robotic Reinforcement Learning}} without {{Reward Engineering}}},
 url = {https://arxiv.org/abs/1904.07854},
 volume = {abs/1904.07854},
 year = {2019}
}

@inproceedings{singh_scalable_2020,
 abstract = {While robot learning has demonstrated promising results for enabling robots to automatically acquire new skills, a critical challenge in deploying learning-based systems is scale: acquiring enough data for the robot to effectively generalize broadly. Imitation learning, in particular, has remained a stable and powerful approach for robot learning, but critically relies on expert operators for data collection. In this work, we target this challenge, aiming to build an imitation learning system that can continuously improve through autonomous data collection, while simultaneously avoiding the explicit use of reinforcement learning, to maintain the stability, simplicity, and scalability of supervised imitation. To accomplish this, we cast the problem of imitation with autonomous improvement into a multi-task setting. We utilize the insight that, in a multi-task setting, a failed attempt at one task might represent a successful attempt at another task. This allows us to leverage the robot's own trials as demonstrations for tasks other than the one that the robot actually attempted. Using an initial dataset of multitask demonstration data, the robot autonomously collects trials which are only sparsely labeled with a binary indication of whether the trial accomplished any useful task or not. We then embed the trials into a learned latent space of tasks, trained using only the initial demonstration dataset, to draw similarities between various trials, enabling the robot to achieve one-shot generalization to new tasks. In contrast to prior imitation learning approaches, our method can autonomously collect data with sparse supervision for continuous improvement, and in contrast to reinforcement learning algorithms, our method can effectively improve from sparse, task-agnostic reward signals.},
 archiveprefix = {arXiv},
 author = {Singh, Avi and Jang, Eric and Irpan, Alexander and Kappler, Daniel and Dalal, Murtaza and Levine, Sergey and Khansari, Mohi and Finn, Chelsea},
 booktitle = {To Appear at {{ICRA}} 2020},
 eprint = {2003.02636},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/BHHQS466/Singh et al. - 2020 - Scalable Multi-Task Imitation Learning with Autono.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Scalable {{Multi}}-{{Task Imitation Learning}} with {{Autonomous Improvement}}},
 year = {2020}
}

@inproceedings{sinha_certifying_2018,
 author = {Aman Sinha and
Hongseok Namkoong and
John C. Duchi},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/SinhaND18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 04 Apr 2019 01:00:00 +0200},
 title = {Certifying Some Distributional Robustness with Principled Adversarial
Training},
 url = {https://openreview.net/forum?id=Hk6kPgZA-},
 year = {2018}
}

@inproceedings{sinha_variational_2019,
 author = {Samarth Sinha and
Sayna Ebrahimi and
Trevor Darrell},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/SinhaED19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00607},
 pages = {5971--5980},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Variational Adversarial Active Learning},
 url = {https://doi.org/10.1109/ICCV.2019.00607},
 year = {2019}
}

@article{sinopoli_kalman_2004,
 author = {Sinopoli, B. and Schenato, L. and Franceschetti, M. and Poolla, K. and Jordan, M.I. and Sastry, S.S.},
 doi = {10.1109/TAC.2004.834121},
 file = {/home/matt/Zotero/storage/UA73IFP2/kalman_filtering_intermittent.pdf},
 issn = {0018-9286},
 journal = {IEEE Transactions on Automatic Control},
 language = {en},
 number = {9},
 pages = {1453--1464},
 title = {Kalman {{Filtering With Intermittent Observations}}},
 volume = {49},
 year = {2004}
}

@article{sitawarin_minimum-norm_2020,
 author = {Sitawarin, Chawin and Wagner, David},
 journal = {ArXiv preprint},
 title = {Minimum-{{Norm Adversarial Examples}} on {{KNN}} and {{KNN}}-{{Based Models}}},
 url = {https://arxiv.org/abs/2003.06559},
 volume = {abs/2003.06559},
 year = {2020}
}

@techreport{skabardonis_evaluation_1998-1,
 address = {{Berkeley, California}},
 author = {Skabardonis, A. and Petty, K. and Varaiya, P.},
 institution = {{Institute of Transportation Studies, University of California}},
 number = {PATH Research Report UCB-ITS-PRR-98-13},
 title = {Evaluation of {{Freeway Service Patrol}} at a {{Los Angeles}} Freeway Site},
 year = {1998}
}

@article{skabardonis_real-time_2008,
 author = {Skabardonis, Alexander and Geroliminis, Nikolas},
 doi = {10.1080/15472450802023337},
 file = {/home/matt/Zotero/storage/UZXUAP7X/Real Time Monitoring and Control on Signalized Arterials.pdf},
 issn = {1547-2450},
 journal = {Journal of Intelligent Transportation Systems},
 language = {en},
 number = {2},
 pages = {64--74},
 title = {Real-{{Time Monitoring}} and {{Control}} on {{Signalized Arterials}}},
 volume = {12},
 year = {2008}
}

@article{small_differentiated_2006,
 author = {Small, K. A. and Winston, C. and Yan, J.},
 journal = {Brookings-Wharton Papers on Urban Affairs},
 pages = {53--96},
 title = {Differentiated {{Road Pricing}}, {{Express Lanes}}, and {{Carpools}}: {{Exploiting Heterogeneous Preferences}} in {{Policy Design}}},
 year = {2006}
}

@book{small_economics_2007,
 address = {{New York, NY, USA}},
 author = {Small, Kenneth A. and Verhoef, Erik T.},
 doi = {10.4324/9780203642306},
 edition = {Second},
 file = {/home/matt/Zotero/storage/C6L2CAHW/Small - 2007 - The Economics of Urban Transportation.pdf},
 isbn = {978-0-203-64230-6},
 language = {en},
 publisher = {{Routledge}},
 title = {The {{Economics}} of {{Urban Transportation}}},
 year = {2007}
}

@article{small_scheduling_1982,
 author = {Small, K. A.},
 journal = {American Economic Review},
 number = {3},
 pages = {467--479},
 title = {The {{Scheduling}} of {{Consumer Activities}}: {{Work Trips}}},
 volume = {72},
 year = {1982}
}

@techreport{small_valuation_1999,
 address = {{Washington DC}},
 author = {Small, K. and Noland, R. and Chu, X. and Lewis, D.},
 institution = {{National Cooperative Highway Research Program, TRB, National Research Council}},
 number = {431},
 title = {Valuation of {{Travel}}-{{Time Savings}} and {{Predictability}} in {{Congested Conditions}} for {{Highway User}}-{{Cost Estimation}}},
 year = {1999}
}

@article{small_value_2001,
 author = {Small, K. A. and Yan, J.},
 journal = {Journal of Urban Econormcs},
 pages = {310--336},
 title = {The {{Value}} of ``{{Value Pricing}}'' of {{Roads}}: {{Second}}-{{Best Pricing}} and {{Product Differentiation}}},
 volume = {49},
 year = {2001}
}

@article{smaragadis_series_2003,
 author = {Smaragadis, E. and Papageorgiou, M.},
 journal = {Transportation Research Record},
 number = {1856},
 pages = {74--86},
 title = {A Series of New Local Ramp Metering Strategies},
 year = {2003}
}

@inproceedings{smith_avid_2019,
 abstract = {Robotic reinforcement learning (RL) holds the promise of enabling robots to learn complex behaviors through experience. However, realizing this promise requires not only effective and scalable RL algorithms, but also mechanisms to reduce human burden in terms of defining the task and resetting the environment. In this paper, we study how these challenges can be alleviated with an automated robotic learning framework, in which multi-stage tasks are defined simply by providing videos of a human demonstrator and then learned autonomously by the robot from raw image observations. A central challenge in imitating human videos is the difference in morphology between the human and robot, which typically requires manual correspondence. We instead take an automated approach and perform pixel-level image translation via CycleGAN to convert the human demonstration into a video of a robot, which can then be used to construct a reward function for a model-based RL algorithm. The robot then learns the task one stage at a time, automatically learning how to reset each stage to retry it multiple times without human-provided resets. This makes the learning process largely automatic, from intuitive task specification via a video to automated training with minimal human intervention. We demonstrate that our approach is capable of learning complex tasks, such as operating a coffee machine, directly from raw image observations, requiring only 20 minutes to provide human demonstrations and about 180 minutes of robot interaction with the environment. A supplementary video depicting the experimental setup, learning process, and our method's final performance is available from https://sites.google.com/view/icra20avid},
 archiveprefix = {arXiv},
 author = {Smith, Laura and Dhawan, Nikita and Zhang, Marvin and Abbeel, Pieter and Levine, Sergey},
 booktitle = {Submitted to {{International Conference}} on {{Robotics}} and {{Animation}} ({{ICRA}}) 2020},
 eprint = {1912.04443},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/64SZ36DA/Smith et al. - 2019 - AVID Learning Multi-Stage Tasks via Pixel-Level T.pdf},
 shorttitle = {{{AVID}}},
 title = {{{AVID}}: {{Learning Multi}}-{{Stage Tasks}} via {{Pixel}}-{{Level Translation}} of {{Human Videos}}},
 year = {2019}
}

@article{smith_balancing_2019,
 author = {Smith, Stanley W. and Kim, Yeojun and Guanetti, Jacopo and Kurzhanskiy, Alexander A. and Arcak, Murat and Borrelli, Francesco},
 journal = {ArXiv preprint},
 title = {Balancing {{Safety}} and {{Traffic Throughput}} in {{Cooperative Vehicle Platooning}}},
 url = {https://arxiv.org/abs/1904.08557},
 volume = {abs/1904.08557},
 year = {2019}
}

@article{smith_existence_1979,
 author = {Smith, M. J.},
 journal = {Transportation Research},
 pages = {295--304},
 title = {The {{Existence}}, {{Uniqueness}} and {{Stability}} of {{Traffic Equilibira}}},
 volume = {13B},
 year = {1979}
}

@article{smith_impact_1994,
 author = {Smith, M. Theresa},
 journal = {Public Roads},
 number = {3},
 pages = {8--14},
 title = {The Impact of Highway Infrastructure on Economic Performance},
 volume = {57},
 year = {1994}
}

@book{smith_intellidrive_2011,
 annotation = {Published: University of Virginia},
 author = {Smith, B. L. and Venkatanarayana, R. and Park, H. and Goodall, N. and Datesh, J. and Skerrit, C.},
 title = {{{IntelliDrive Traffic Signal Control Algorithms}}},
 year = {2011}
}

@article{smith_new_1993,
 author = {Smith, M. J.},
 journal = {Transportation Research B},
 number = {1},
 pages = {49--63},
 title = {A New Dynamic Traffic Model and the Existence and Calculation of Dynamic User Equilibria on Congested Capacity-Constrained Road Networks},
 volume = {27},
 year = {1993}
}

@article{smith_splitting_2011,
 author = {Smith, M.J. and Mounce, R.},
 journal = {Transportation Research, Part B.},
 pages = {1389--1490},
 title = {A Splitting Rate Model of Traffic Re-Routing and Traffic Control},
 volume = {45},
 year = {2011}
}

@article{smith_traffic_2015,
 author = {Smith, M.J. and Liu, R. and Mounce, R.},
 journal = {Transportation Research, Part B. In Press.},
 title = {Traffic Control and Route Choice; Capacity Maximization and Stability},
 year = {2015}
}

@article{smits_family_2015,
 author = {Smits, Erik-Sander and Bliemer, Michiel C.J. and Pel, Adam J. and {\noopsort{arem}}{van Arem}, Bart},
 doi = {10.1016/j.trb.2015.01.002},
 file = {/home/matt/Zotero/storage/UJZ5W987/smits_2015_TRB_familyofnodemodels.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {20--39},
 title = {A Family of Macroscopic Node Models},
 volume = {74},
 year = {2015}
}

@article{smulders_control_1990,
 author = {Smulders, S.},
 journal = {Transportation Research, B},
 number = {2},
 pages = {111--132},
 title = {Control of Freeway Traffic Flow by Variable Speed Signs},
 volume = {24},
 year = {1990}
}

@inproceedings{socher_recursive_2013,
 address = {Seattle, Washington, USA},
 author = {Socher, Richard  and
Perelygin, Alex  and
Wu, Jean  and
Chuang, Jason  and
Manning, Christopher D.  and
Ng, Andrew  and
Potts, Christopher},
 booktitle = {Proceedings of the 2013 Conference on Empirical Methods in Natural Language Processing},
 pages = {1631--1642},
 publisher = {Association for Computational Linguistics},
 title = {Recursive Deep Models for Semantic Compositionality Over a Sentiment Treebank},
 url = {https://aclanthology.org/D13-1170},
 year = {2013}
}

@article{song_fault_2003,
 author = {Song, Bongsob and Hedrick, J Karl and Howell, Adam},
 journal = {Journal of dynamic systems, measurement, and control},
 number = {3},
 pages = {320--329},
 title = {Fault Tolerant Control and Classification for Longitudinal Vehicle Control},
 volume = {125},
 year = {2003}
}

@article{song_pip_2020,
 author = {Song, Haoran and Ding, Wenchao and Chen, Yuxuan and Shen, Shaojie and Wang, Michael Yu and Chen, Qifeng},
 journal = {ArXiv preprint},
 title = {{{PiP}}: {{Planning}}-Informed {{Trajectory Prediction}} for {{Autonomous Driving}}},
 url = {https://arxiv.org/abs/2003.11476},
 volume = {abs/2003.11476},
 year = {2020}
}

@article{song_reproducing_2013,
 abstract = {Targeting at sparse learning, we construct Banach spaces B of functions on an input space X with the following properties: (1) B possesses an {$\mathscr{l}$}1 norm in the sense that B is isometrically isomorphic to the Banach space of integrable functions on X with respect to the counting measure; (2) point evaluations are continuous linear functionals on B and are representable through a bilinear form with a kernel function; and (3) regularized learning schemes on B satisfy the linear representer theorem. Examples of kernel functions admissible for the construction of such spaces are given.},
 author = {Song, Guohui and Zhang, Haizhang and Hickernell, Fred J.},
 doi = {10.1016/j.acha.2012.03.009},
 file = {/home/matt/Zotero/storage/FI3PC9UM/Song et al. - 2013 - Reproducing kernel Banach spaces with the ℓ1 norm.pdf;/home/matt/Zotero/storage/ZYULPTW2/S1063520312000486.html},
 issn = {1063-5203},
 journal = {Applied and Computational Harmonic Analysis},
 language = {en},
 number = {1},
 pages = {96--116},
 title = {Reproducing Kernel {{Banach}} Spaces with the L1 Norm},
 volume = {34},
 year = {2013}
}

@inproceedings{souyris_formal_2009,
 abstract = {This paper relates an industrial experience in the field of formal verification of avionics software products. Ten years ago we presented our very first technological research results in [18]. What was just an idea plus some experimental results at that time is now an industrial reality. Indeed, since 2001, Airbus has been integrating several tool supported formal verification techniques into the development process of avionics software products. Just like all aspects of such processes, the use of formal verification techniques must comply with DO-178B [9] objectives and Airbus has been a pioneer in this domain.},
 address = {{Berlin, Heidelberg}},
 author = {Souyris, Jean and Wiels, Virginie and Delmas, David and Delseny, Herv{\'e}},
 booktitle = {{{FM}} 2009: {{Formal Methods}}},
 editor = {Cavalcanti, Ana and Dams, Dennis R.},
 isbn = {978-3-642-05089-3},
 pages = {532--546},
 publisher = {{Springer Berlin Heidelberg}},
 title = {Formal {{Verification}} of {{Avionics Software Products}}},
 year = {2009}
}

@article{srinivas_bottleneck_2021,
 author = {Srinivas, Aravind and Lin, Tsung-Yi and Parmar, Niki and Shlens, Jonathon and Abbeel, Pieter and Vaswani, Ashish},
 journal = {ArXiv preprint},
 title = {Bottleneck {{Transformers}} for {{Visual Recognition}}},
 url = {https://arxiv.org/abs/2101.11605},
 volume = {abs/2101.11605},
 year = {2021}
}

@article{srivastava_empirical_2013,
 author = {Srivastava, Anupam and Gerolimini, Nikolas},
 journal = {Transportation Research Part C: Emerging Technologies},
 pages = {161--177},
 title = {Empirical Observations of Capacity Drop in Freeway Merges with Ramp Control and Integration in a First-Order Model},
 volume = {30},
 year = {2013}
}

@article{steinwart_explicit_2006,
 abstract = {Although Gaussian radial basis function (RBF) kernels are one of the most often used kernels in modern machine learning methods such as support vector machines (SVMs), little is known about the structure of their reproducing kernel Hilbert spaces (RKHSs). In this work, two distinct explicit descriptions of the RKHSs corresponding to Gaussian RBF kernels are given and some consequences are discussed. Furthermore, an orthonormal basis for these spaces is presented. Finally, it is discussed how the results can be used for analyzing the learning performance of SVMs.},
 author = {Steinwart, I. and Hush, D. and Scovel, C.},
 doi = {10.1109/TIT.2006.881713},
 file = {/home/matt/Zotero/storage/CRJI8NE7/Steinwart et al. - 2006 - An Explicit Description of the Reproducing Kernel .pdf},
 issn = {0018-9448},
 journal = {IEEE Transactions on Information Theory},
 language = {en},
 number = {10},
 pages = {4635--4643},
 title = {An {{Explicit Description}} of the {{Reproducing Kernel Hilbert Spaces}} of {{Gaussian RBF Kernels}}},
 volume = {52},
 year = {2006}
}

@article{stern_dissipation_2018,
 abstract = {Traffic waves are phenomena that emerge when the vehicular density exceeds a critical threshold. Considering the presence of increasingly automated vehicles in the traffic stream, a number of research activities have focused on the influence of automated vehicles on the bulk traffic flow. In the present article, we demonstrate experimentally that intelligent control of an autonomous vehicle is able to dampen stop-and-go waves that can arise even in the absence of geometric or lane changing triggers. Precisely, our experiments on a circular track with more than 20 vehicles show that traffic waves emerge consistently, and that they can be dampened by controlling the velocity of a single vehicle in the flow. We compare metrics for velocity, braking events, and fuel economy across experiments. These experimental findings suggest a paradigm shift in traffic management: flow control will be possible via a few mobile actuators (less than 5\%) long before a majority of vehicles have autonomous capabilities.},
 author = {Stern, Raphael E. and Cui, Shumo and Delle Monache, Maria Laura and Bhadani, Rahul and Bunting, Matt and Churchill, Miles and Hamilton, Nathaniel and Haulcy, R'mani and Pohlmann, Hannah and Wu, Fangyu and Piccoli, Benedetto and Seibold, Benjamin and Sprinkle, Jonathan and Work, Daniel B.},
 doi = {10.1016/j.trc.2018.02.005},
 file = {/home/matt/Zotero/storage/G7B2ANLX/Stern et al. - 2018 - Dissipation of stop-and-go waves via control of au.pdf;/home/matt/Zotero/storage/QZWW6WWS/S0968090X18301517.html},
 issn = {0968-090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 pages = {205--221},
 shorttitle = {Dissipation of Stop-and-Go Waves via Control of Autonomous Vehicles},
 title = {Dissipation of Stop-and-Go Waves via Control of Autonomous Vehicles: {{Field}} Experiments},
 volume = {89},
 year = {2018}
}

@article{stoicescu_fuel-optimal_1995,
 author = {Stoicescu, A.P.},
 journal = {International Journal of Vehicle Design},
 pages = {229--256},
 title = {On Fuel-Optimal Velocity Control of a Motor Vehicle},
 volume = {17},
 year = {1995}
}

@techreport{stone_multiagent_1997,
 abstract = {Distributed Artificial Intelligence (DAI) has existed as a subfield of AI for less than two decades. DAI is concerned with systems that consist of multiple independent entities that interact in a domain. Traditionally, DAI has been divided into two sub-disciplines: Distributed Problem Solving (DPS) focuses on the information management aspects of systems with several components working together towards a common goal; Multiagent Systems (MAS) deals with behavior management in collections of several independent entities, or agents. This survey of MAS is intended to serve as an introduction to the field and as an organizational framework. A series of general multiagent scenarios are presented. For each scenario, the issues that arise are described along with a sampling of the techniques that exist to deal with them. The presented techniques are not exhaustive, but they highlight how multiagent systems can be and have been used to build complex systems. When options exist, the techniques presented are biased towards machine learning approaches. Additional opportunities for applying machine learning to MAS are highlighted and robotic soccer is presented as an appropriate test bed for MAS. This survey does not focus exclusively on robotic systems. However, we believe that much of the prior research in non-robotic MAS is relevant to robotic MAS, and we explicitly discuss several robotic MAS, including all of those presented in this issue.},
 address = {{Fort Belvoir, VA}},
 author = {Stone, Peter and Veloso, Manuela},
 doi = {10.21236/ADA333248},
 file = {/home/matt/Zotero/storage/Z9YALDYI/Stone and Veloso - 1997 - Multiagent Systems A Survey from a Machine Learni.pdf},
 institution = {{Defense Technical Information Center}},
 language = {en},
 shorttitle = {Multiagent {{Systems}}},
 title = {Multiagent {{Systems}}: {{A Survey}} from a {{Machine Learning Perspective}}:},
 year = {1997}
}

@article{stone_whats_2006,
 author = {Stone, Valerie E. and Gerrans, Philip},
 doi = {10.1080/17470910601029221},
 file = {/home/matt/Zotero/storage/JVHIZEAZ/Stone and Gerrans - 2006 - What's domain-specific about theory of mind.pdf},
 issn = {1747-0919, 1747-0927},
 journal = {Social Neuroscience},
 language = {en},
 number = {3-4},
 pages = {309--319},
 title = {What's Domain-Specific about Theory of Mind?},
 volume = {1},
 year = {2006}
}

@article{stooke_rlpyt_2019,
 author = {Stooke, Adam and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {Rlpyt: {{A Research Code Base}} for {{Deep Reinforcement Learning}} in {{PyTorch}}},
 url = {https://arxiv.org/abs/1909.01500},
 volume = {abs/1909.01500},
 year = {2019}
}

@article{straka_survey_2009,
 author = {Straka, Ond{\v r}ej and {\^S}imandl, Miroslav},
 doi = {10.3182/20090706-3-FR-2004.00226},
 file = {/home/matt/Documents/Papers/survey_of_adaptive_sample_size_for_pf.pdf},
 issn = {14746670},
 journal = {IFAC Proceedings Volumes},
 language = {en},
 number = {10},
 pages = {1358--1363},
 title = {A {{Survey}} of {{Sample Size Adaptation Techniques}} for {{Particle Filters}}},
 volume = {42},
 year = {2009}
}

@techreport{straus_estimating_2006,
 abstract = {Our best guess is that overweight vehicles impose somewhere between \$12 million and \$53 million per year in uncompensated damages to Arizona roadways. Arizona currently budgets about \$5.8 million per year for mobile enforcement efforts aimed at, among other things, penalizing and deterring overweight vehicle operations.},
 author = {Straus, S. H. and Semmens, J.},
 institution = {{Arizona Dept of Transportation}},
 number = {FHWA-AZ-06-528},
 title = {Estimating the {{Cost}} of {{Overweight Vehicle Travel}} on {{Arizona Highways}}},
 year = {2006}
}

@inproceedings{strubell_energy_2019,
 address = {Florence, Italy},
 author = {Strubell, Emma  and
Ganesh, Ananya  and
McCallum, Andrew},
 booktitle = {Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/P19-1355},
 pages = {3645--3650},
 publisher = {Association for Computational Linguistics},
 title = {Energy and Policy Considerations for Deep Learning in {NLP}},
 url = {https://aclanthology.org/P19-1355},
 year = {2019}
}

@inproceedings{su_affective_2021,
 abstract = {The success of deep learning has led to intense growth and interest in computer vision, along with concerns about its potential impact on society. Yet we know little about how these changes have affected the people that research and practice computer vision: we as a community spend so much effort trying to replicate the abilities of humans, but so little time considering the impact of this work on ourselves. In this paper, we report on a study in which we asked computer vision researchers and practitioners to write stories about emotionally-salient events that happened to them. Our analysis of over 50 responses found tremendous affective (emotional) strain in the computer vision community. While many describe excitement and success, we found strikingly frequent feelings of isolation, cynicism, apathy, and exasperation over the state of the field. This is especially true among people who do not share the unbridled enthusiasm for normative standards for computer vision research and who do not see themselves as part of the ``incrowd.'' Our findings suggest that these feelings are closely tied to the kinds of research and professional practices now expected in computer vision. We argue that as a community with significant stature, we need to work towards an inclusive culture that makes transparent and addresses the real emotional toil of its members.},
 author = {Su, Norman Makoto and Crandall, David J},
 booktitle = {{{CVPR}} 2021},
 file = {/home/matt/Zotero/storage/V72D2QIC/Su and Crandall - The Affective Growth of Computer Vision.pdf},
 language = {en},
 pages = {10},
 title = {The {{Affective Growth}} of {{Computer Vision}}},
 year = {2021}
}

@phdthesis{su_modeling_2014,
 abstract = {This dissertation studies a series of freeway and arterial traffic modeling, estimation and control methodologies. First, it investigates the Link-Node Cell Transmission Model's (LN-CTM's) ability to model arterial traffic. The LN-CTM is a modification of the cell transmission model developed by Daganzo. The investigation utilizes traffic data collected on an arterial segment in Los Angeles, California, and a link-node cell transmission model, with some adaptations to the arterial traffic, is constructed for the studied location. The simulated flow and the simulation travel time were compared with field measurements to evaluate the modeling accuracy.Second, an algorithm for estimating turning proportions is proposed in this dissertation. The knowledge about turning proportions at street intersections is a frequent input for traffic models, but it is often difficult to measure directly. Compared with previous estimation methods used to solve this problem, the proposed method can be used with only half the detectors employed in the conventional complete detector configuration. The proposed method formulates the estimation problem as a constrained least squares problem, and a recursive solving procedure is given. A simulation study was carried out to demonstrate the accuracy and efficiency of the proposed algorithm.In addition to addressing arterial traffic modeling and estimation problems, this dissertation also studies a freeway traffic control strategy and a freeway and arterial coordinated control strategy. It presents a coordinated control strategy of variable speed limits (VSL) and ramp metering to address freeway congestion caused by weaving effects. In this strategy, variable speed limits are designed to maximize the bottleneck flow, and ramp metering is designed to minimize travel time in a model predictive control frame work. A microscopic simulation based on the I-80 at Emeryville, California was built to evaluate the strategy, and the results showed that the traffic performance was significantly improved .Following the freeway control study, this dissertation discusses the coordinated control of freeways and arterials. In current practice, traffic controls on freeways and on arterials are independent. In order to coordinate these two systems for better performance, a control strategy covering the freeway ramp metering and the signal control at the adjacent intersection is developed. This control strategy uses upstream ALINEA, which is a well-known control algorithm, for ramp metering to locally maximize freeway throughput. For the intersection signal control, the proposed control strategy distributes green splits by taking into account both the available on-ramp space and the demands of all intersection movements. A microscopic simulation of traffic in an arterial intersection with flow discharge to a freeway on-ramp, which is calibrated using the data collected at San Jose, California, is created to evaluate the performance of the proposed control strategy. The results showed that the proposed strategy can reduce intersection delay by 8\%, compared to the current field-implemented control strategy.Transportation mobility can be improved not only by traffic management strategies, but also through the deployment of advanced vehicle technologies. This dissertation also investigates the impact of Adaptive Cruise Control (ACC) and Cooperative Adaptive Cruise Control (CACC) on highway capacity. A freeway microscopic traffic simulation model is constructed to evaluate how the freeway lane flow capacity change under different penetration rates of vehicles equipped with either ACC or CACC system. This simulation model is based on a calibrated driver behavioral model and the vehicle dynamics of the ACC and CACC systems. The model also utilizes data collected from a real experiment in which drivers' selections of time gaps are recorded. The simulation shows that highway capacity can be significantly increased when the CACC vehicles reach a moderate to high market penetration, as compared to both regular manually driven vehicles and vehicles equipped with only ACC.},
 author = {Su, Dongyan},
 file = {/home/matt/Zotero/storage/TIAMEY8E/Su - 2014 - Modeling, Estimation and Control of Traffic.pdf;/home/matt/Zotero/storage/7Y7JT84X/9570v0wj.html},
 language = {en},
 school = {UC Berkeley},
 title = {Modeling, {{Estimation}} and {{Control}} of {{Traffic}}},
 year = {2014}
}

@article{sucholutsky_less_2020,
 author = {Sucholutsky, Ilia and Schonlau, Matthias},
 journal = {ArXiv preprint},
 title = {'{{Less Than One}}'-{{Shot Learning}}: {{Learning N Classes From M}}},
 url = {https://arxiv.org/abs/2009.08449},
 volume = {abs/2009.08449},
 year = {2020}
}

@article{sucholutsky_less_2020-1,
 author = {Sucholutsky, Ilia and Schonlau, Matthias},
 journal = {ArXiv preprint},
 title = {'{{Less Than One}}'-{{Shot Learning}}: {{Learning N Classes From M}}},
 url = {https://arxiv.org/abs/2009.08449},
 volume = {abs/2009.08449},
 year = {2020}
}

@article{sugiyama_traffic_2008,
 abstract = {A traffic jam on a highway is a very familiar phenomenon. From the physical viewpoint, the system of vehicular flow is a non-equilibrium system of interacting particles (vehicles). The collective effect of the many-particle system induces the instability of a free flow state caused by the enhancement of fluctuations, and the transition to a jamming state occurs spontaneously if the average vehicle density exceeds a certain critical value. Thus, a bottleneck is only a trigger and not the essential origin of a traffic jam. In this paper, we present the first experimental evidence that the emergence of a traffic jam is a collective phenomenon like `dynamical' phase transitions and pattern formation in a non-equilibrium system. We have performed an experiment on a circuit to show the emergence of a jam with no bottleneck. In the initial condition, all the vehicles are moving, homogeneously distributed on the circular road, with the same velocity. The average density of the vehicles is prepared for the onset of the instability. Even a tiny fluctuation grows larger and then the homogeneous movement cannot be maintained. Finally, a jam cluster appears and propagates backward like a solitary wave with the same speed as that of a jam cluster on a highway.},
 author = {Sugiyama, Yuki and Fukui, Minoru and Kikuchi, Macoto and Hasebe, Katsuya and Nakayama, Akihiro and Nishinari, Katsuhiro and Tadaki, Shin-ichi and Yukawa, Satoshi},
 doi = {2008030504130900},
 file = {/home/matt/Zotero/storage/E82DPT6X/Sugiyama et al. - 2008 - Traffic jams without bottlenecks—experimental evid.pdf},
 issn = {1367-2630},
 journal = {New Journal of Physics},
 language = {en},
 number = {3},
 pages = {033001},
 title = {Traffic Jams without Bottlenecks\textemdash Experimental Evidence for the Physical Mechanism of the Formation of a Jam},
 volume = {10},
 year = {2008}
}

@article{suh_vision-based_2020,
 abstract = {This paper presents a novel approach for vision-based Simultaneous Localization and Mapping (SLAM) on a high curved track without pose-based landmarks. The proposed approach combines an Iterative Closest Points (ICP) method and Stochastic Gradient Descent (SGD) optimization and comprises four main steps. First, a Kalman filter with a simple circular lane model is used to estimate the road curvature using images from a front camera. Then, the vehicle position and orientation are reconstructed by using the yaw rate and longitudinal speed from inertial sensors. Drift and misalignment of the constructed map are corrected using ICP under the assumption that the vehicle continuously travels the same track. The final map is obtained using SGD optimization, which enforces curvature matching. We evaluate the performance of the proposed algorithm with an environment of the winding track of Hyundai-Kia California Proving Ground (CPG) located in Southern California and the customized ellipsoidal track. The experimental results show the effectiveness of the proposed approach.},
 author = {Suh, Jongsang and Choi, Eric Yongkeun and Borrelli, Francesco},
 doi = {10.1109/TVT.2019.2961516},
 file = {/home/matt/Zotero/storage/3KUE3HBU/Suh et al. - 2020 - Vision-Based Race Track SLAM Based Only on Lane Cu.pdf},
 issn = {0018-9545, 1939-9359},
 journal = {IEEE Transactions on Vehicular Technology},
 language = {en},
 number = {2},
 pages = {1495--1504},
 title = {Vision-{{Based Race Track SLAM Based Only}} on {{Lane Curvature}}},
 volume = {69},
 year = {2020}
}

@inproceedings{sukhbaatar_learning_2016,
 author = {Sainbayar Sukhbaatar and
Arthur Szlam and
Rob Fergus},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/SukhbaatarSF16.bib},
 booktitle = {Advances in Neural Information Processing Systems 29: Annual Conference
on Neural Information Processing Systems 2016, December 5-10, 2016,
Barcelona, Spain},
 editor = {Daniel D. Lee and
Masashi Sugiyama and
Ulrike von Luxburg and
Isabelle Guyon and
Roman Garnett},
 pages = {2244--2252},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Learning Multiagent Communication with Backpropagation},
 url = {https://proceedings.neurips.cc/paper/2016/hash/55b1927fdafef39c48e5b73b5d61ea60-Abstract.html},
 year = {2016}
}

@techreport{sulzer_regional_2000,
 author = {Sulzer, Kenneth E.},
 institution = {{San Diego Association of Governments}},
 number = {00-9-15 (Agenda Report)},
 title = {Regional Highway Project Evaluation - Final Results},
 year = {2000}
}

@article{sumalee_stochastic_2011,
 author = {Sumalee, A. and Zhong, R.X. and Pan, T.L. and Szeto, W.Y.},
 doi = {10.1016/j.trb.2010.09.006},
 file = {/home/matt/Zotero/storage/IC5AT9WA/sumalee_stochasticCTM.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {3},
 pages = {507--533},
 shorttitle = {Stochastic Cell Transmission Model ({{SCTM}})},
 title = {Stochastic Cell Transmission Model ({{SCTM}}): {{A}} Stochastic Dynamic Traffic Model for Traffic State Surveillance and Assignment},
 volume = {45},
 year = {2011}
}

@article{sun_behavior_2019,
 author = {Sun, Liting and Zhan, Wei and Chan, Ching-Yao and Tomizuka, Masayoshi},
 journal = {ArXiv preprint},
 title = {Behavior {{Planning}} of {{Autonomous Cars}} with {{Social Perception}}},
 url = {https://arxiv.org/abs/1905.00988},
 volume = {abs/1905.00988},
 year = {2019}
}

@article{sun_interpretable_2019,
 author = {Sun, Liting and Zhan, Wei and Hu, Yeping and Tomizuka, Masayoshi},
 journal = {ArXiv preprint},
 title = {Interpretable {{Modelling}} of {{Driving Behaviors}} in {{Interactive Driving Scenarios}} Based on {{Cumulative Prospect Theory}}},
 url = {https://arxiv.org/abs/1907.08707},
 volume = {abs/1907.08707},
 year = {2019}
}

@techreport{sun_investigation_2000,
 author = {Sun, C.},
 institution = {{California PATH, University of California, Berkeley}},
 number = {UCB-ITS-PRR-2000-04},
 title = {An Investigation in the Use of Inductive Loop Signatures for Vehicle Classification},
 year = {2000}
}

@inproceedings{sun_localized_2005,
 author = {Sun, X. and Horowitz, R.},
 booktitle = {Proceedings {{American Control Conference}}},
 title = {A Localized Switching Ramp-Metering Controller with a Queue Length Regulator for Congested Freeways},
 year = {2005}
}

@inproceedings{sun_mixture_2004,
 abstract = {We present our latest results on developing and implementing a traffic congestion mode and vehicle density estimator for a segment of Interstate 210 in Southern California. Using a mixture Kalman filtering (MKF) algorithm on the switching-mode traffic model, the estimator is able to provide estimated vehicle densities at unmeasured locations, as well as the congestion statuses (free-flow or congested), which are not directly observed. The program runs efficiently, thus making it possible to carry out estimation in real time.},
 author = {Sun, Xiaotian and Munoz, L. and Horowitz, R.},
 booktitle = {Proceedings of the 2004 {{American Control Conference}}},
 doi = {10.23919/ACC.2004.1383770},
 file = {/home/matt/Zotero/storage/CC9HBCEK/Xiaotian Sun et al. - 2004 - Mixture Kalman filter based highway congestion mod.pdf;/home/matt/Zotero/storage/WGJ3FYT5/1383770.html},
 pages = {2098-2103 vol.3},
 title = {Mixture {{Kalman}} Filter Based Highway Congestion Mode and Vehicle Density Estimator and Its Application},
 volume = {3},
 year = {2004}
}

@article{sun_network_2016,
 author = {Sun, Zhe and Jin, Wen-Long and Ng, ManWo},
 doi = {10.1016/j.trc.2016.04.015},
 file = {/home/matt/Zotero/storage/VTQL7EIY/sun_2016_network_sensor_health.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {300--310},
 title = {Network Sensor Health Problem},
 volume = {68},
 year = {2016}
}

@article{sun_optimal_2020,
 abstract = {This paper focuses on the speed planning problem for connected and automated vehicles (CAVs) communicating to traffic lights. The uncertainty of traffic signal timing for signalized intersections on the road is considered. The eco-driving problem is formulated as a data-driven chance constrained robust optimization problem. Effective red light duration (ERD) is defined as a random variable, and describes the feasible passing time through the signalized intersections. Usually, the true probability distribution for ERD is unknown. Consequently, a data-driven approach is adopted to formulate chance constraints based on empirical sample data. This incorporates robustness into the eco-driving control problem with respect to uncertain signal timing. Dynamic programming (DP) is employed to solve the optimization problem. Simulation results demonstrate that the proposed method can generate optimal speed reference trajectories with 40\% less vehicle fuel consumption, while maintaining the arrival time at a similar level compared to a modified intelligent driver model (IDM). The proposed control approach significantly improves the controller's robustness in the face of uncertain signal timing, without requiring to know the distribution of the random variable a priori.},
 author = {Sun, Chao and Guanetti, Jacopo and Borrelli, Francesco and Moura, Scott},
 doi = {10.1109/JIOT.2020.2968120},
 file = {/home/matt/Zotero/storage/CR8AEBA9/Sun et al. - 2020 - Optimal Eco-Driving Control of Connected and Auton.pdf},
 issn = {2327-4662, 2372-2541},
 journal = {IEEE Internet of Things Journal},
 language = {en},
 pages = {1--1},
 title = {Optimal {{Eco}}-{{Driving Control}} of {{Connected}} and {{Autonomous Vehicles Through Signalized Intersections}}},
 year = {2020}
}

@article{sun_scalable_2021,
 author = {Sun, Chuxiong and Wu, Guoshi},
 journal = {ArXiv preprint},
 title = {Scalable and {{Adaptive Graph Neural Networks}} with {{Self}}-{{Label}}-{{Enhanced}} Training},
 url = {https://arxiv.org/abs/2104.09376},
 volume = {abs/2104.09376},
 year = {2021}
}

@article{sun_set_2006,
 author = {Sun, X. and Horowitz, R.},
 journal = {Transportation Research Record},
 pages = {9--18},
 title = {Set of {{New Traffic}}-{{Responsive Ramp}}-{{Metering Algorithms}} and {{Microscopic Simulation Results}}},
 volume = {1959},
 year = {2006}
}

@article{sun_unsupervised_2019,
 author = {Sun, Yu and Tzeng, Eric and Darrell, Trevor and Efros, Alexei A.},
 journal = {ArXiv preprint},
 title = {Unsupervised {{Domain Adaptation}} through {{Self}}-{{Supervision}}},
 url = {https://arxiv.org/abs/1909.11825},
 volume = {abs/1909.11825},
 year = {2019}
}

@article{sun_use_1999,
 author = {Sun, C. and Ritchie, S. G. and Tsai, K. and Jayakrishnan, R.},
 journal = {Transportation Research, Part C},
 pages = {167--185},
 title = {Use of Vehicle Signature Analysis and Lexicographic Optimization for Vehicle Reidentification on Freeways},
 volume = {7},
 year = {1999}
}

@article{sun_vehicle_2004,
 author = {Sun, C. C. and Arr, G. S. and Ramachandram, R. P. and Ritchie, S. G.},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {3},
 pages = {155--164},
 title = {Vehicle {{Reidentification Using Multidetector Fusion}}},
 volume = {5},
 year = {2004}
}

@article{sundaresan_learning_2020,
 author = {Sundaresan, Priya and Grannen, Jennifer and Thananjeyan, Brijen and Balakrishna, Ashwin and Laskey, Michael and Stone, Kevin and Gonzalez, Joseph E. and Goldberg, Ken},
 journal = {ArXiv preprint},
 title = {Learning {{Rope Manipulation Policies Using Dense Object Descriptors Trained}} on {{Synthetic Depth Data}}},
 url = {https://arxiv.org/abs/2003.01835},
 volume = {abs/2003.01835},
 year = {2020}
}

@article{sunderhauf_limits_2018,
 abstract = {The application of deep learning in robotics leads to very specific problems and research questions that are typically not addressed by the computer vision and machine learning communities. In this paper we discuss a number of roboticsspecific learning, reasoning, and embodiment challenges for deep learning. We explain the need for better evaluation metrics, highlight the importance and unique challenges for deep robotic learning in simulation, and explore the spectrum between purely data-driven and model-driven approaches. We hope this paper provides a motivating overview of important research directions to overcome the current limitations, and helps to fulfill the promising potentials of deep learning in robotics.},
 author = {S{\"u}nderhauf, Niko and Brock, Oliver and Scheirer, Walter and Hadsell, Raia and Fox, Dieter and Leitner, J{\"u}rgen and Upcroft, Ben and Abbeel, Pieter and Burgard, Wolfram and Milford, Michael and Corke, Peter},
 doi = {10.1177/0278364918770733},
 file = {/home/matt/Zotero/storage/9FTAXENI/Sünderhauf et al. - 2018 - The limits and potentials of deep learning for rob.pdf},
 issn = {0278-3649, 1741-3176},
 journal = {The International Journal of Robotics Research},
 language = {en},
 number = {4-5},
 pages = {405--420},
 title = {The Limits and Potentials of Deep Learning for Robotics},
 volume = {37},
 year = {2018}
}

@article{sunehag_value-decomposition_2017,
 author = {Sunehag, Peter and Lever, Guy and Gruslys, Audrunas and Czarnecki, Wojciech Marian and Zambaldi, Vinicius and Jaderberg, Max and Lanctot, Marc and Sonnerat, Nicolas and Leibo, Joel Z. and Tuyls, Karl and Graepel, Thore},
 journal = {ArXiv preprint},
 title = {Value-{{Decomposition Networks For Cooperative Multi}}-{{Agent Learning}}},
 url = {https://arxiv.org/abs/1706.05296},
 volume = {abs/1706.05296},
 year = {2017}
}

@article{sunkari_benefits_2004,
 author = {Sunkari, S.},
 journal = {ITE Journal},
 pages = {26--29},
 title = {The {{Benefits}} of {{Retiming Traffic Signals}}},
 year = {2004}
}

@inproceedings{sutskever_sequence_2014,
 author = {Ilya Sutskever and
Oriol Vinyals and
Quoc V. Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/SutskeverVL14.bib},
 booktitle = {Advances in Neural Information Processing Systems 27: Annual Conference
on Neural Information Processing Systems 2014, December 8-13 2014,
Montreal, Quebec, Canada},
 editor = {Zoubin Ghahramani and
Max Welling and
Corinna Cortes and
Neil D. Lawrence and
Kilian Q. Weinberger},
 pages = {3104--3112},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Sequence to Sequence Learning with Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2014/hash/a14ac55a4f27472c5d894ec1c3c743d2-Abstract.html},
 year = {2014}
}

@article{swaroop_comparision_1994,
 author = {Swaroop, DVAHG and Hedrick, JK and Chien, CC and Ioannou, P},
 journal = {Vehicle System Dynamics},
 number = {1},
 pages = {597--625},
 title = {A Comparision of Spacing and Headway Control Laws for Automatically Controlled Vehicles1},
 volume = {23},
 year = {1994}
}

@article{swaroop_constant_1999,
 author = {Swaroop, DVAHG and Hedrick, JK},
 journal = {Journal of dynamic systems, measurement, and control},
 number = {3},
 pages = {462--470},
 title = {Constant Spacing Strategies for Platooning in Automated Highway Systems},
 volume = {121},
 year = {1999}
}

@article{swaroop_direct_2001,
 author = {Swaroop, Darbha and Hedrick, J Karl and Choi, SB},
 journal = {Vehicular Technology, IEEE Transactions on},
 number = {1},
 pages = {150--161},
 title = {Direct Adaptive Longitudinal Control of Vehicle Platoons},
 volume = {50},
 year = {2001}
}

@article{swaroop_string_1996,
 author = {Swaroop, D and Hedrick, JK},
 journal = {Automatic Control, IEEE Transactions on},
 number = {3},
 pages = {349--357},
 title = {String Stability of Interconnected Systems},
 volume = {41},
 year = {1996}
}

@book{system_metrics_group_inc._transportation_2003,
 author = {{System Metrics Group, Inc.}},
 title = {Transportation {{Management Systems Plan}}},
 year = {2003}
}

@inproceedings{szegedy_intriguing_2014,
 author = {Christian Szegedy and
Wojciech Zaremba and
Ilya Sutskever and
Joan Bruna and
Dumitru Erhan and
Ian J. Goodfellow and
Rob Fergus},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/SzegedyZSBEGF13.bib},
 booktitle = {2nd International Conference on Learning Representations, {ICLR} 2014,
Banff, AB, Canada, April 14-16, 2014, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Intriguing properties of neural networks},
 url = {http://arxiv.org/abs/1312.6199},
 year = {2014}
}

@inproceedings{tacchetti_relational_2018,
 author = {Andrea Tacchetti and
H. Francis Song and
Pedro A. M. Mediano and
Vin{\'{\i}}cius Flores Zambaldi and
J{\'{a}}nos Kram{\'{a}}r and
Neil C. Rabinowitz and
Thore Graepel and
Matthew Botvinick and
Peter W. Battaglia},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/TacchettiSMZKRG19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Relational Forward Models for Multi-Agent Learning},
 url = {https://openreview.net/forum?id=rJlEojAqFm},
 year = {2019}
}

@article{tadic_particle_2014,
 author = {Tadi{\textbackslash}'\{c\}, Predrag and {\DH}urovi{\textbackslash}'\{c\}, {\v Z}eljko},
 doi = {10.1016/j.jprocont.2014.02.009},
 file = {/home/matt/Zotero/storage/MTHT8ZN9/1-s2.0-S0959152414000602-main-1.pdf},
 issn = {09591524},
 journal = {Journal of Process Control},
 language = {en},
 number = {4},
 pages = {401--409},
 title = {Particle Filtering for Sensor Fault Diagnosis and Identification in Nonlinear Plants},
 volume = {24},
 year = {2014}
}

@book{taleb_antifragile_2012,
 author = {Taleb, Nassim Nicholas},
 isbn = {1-4000-6782-0},
 publisher = {{Random House}},
 title = {Antifragile: {{Things}} That {{Gain}} from {{Disorder}}},
 year = {2012}
}

@article{tampere_generic_2011,
 author = {Tamp{\`e}re, Chris M.J. and Corthout, Ruben and Cattrysse, Dirk and Immers, Lambertus H.},
 doi = {10.1016/j.trb.2010.06.004},
 file = {/home/matt/Zotero/storage/WET9C9NS/tempere_nodemodels.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {1},
 pages = {289--309},
 title = {A Generic Class of First Order Node Models for Dynamic Macroscopic Simulation of Traffic Flows},
 volume = {45},
 year = {2011}
}

@inproceedings{tan_efficientnet_2019,
 author = {Mingxing Tan and
Quoc V. Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/TanL19.bib},
 booktitle = {Proceedings of the 36th International Conference on Machine Learning,
{ICML} 2019, 9-15 June 2019, Long Beach, California, {USA}},
 editor = {Kamalika Chaudhuri and
Ruslan Salakhutdinov},
 pages = {6105--6114},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 11 Jun 2019 01:00:00 +0200},
 title = {EfficientNet: Rethinking Model Scaling for Convolutional Neural Networks},
 url = {http://proceedings.mlr.press/v97/tan19a.html},
 volume = {97},
 year = {2019}
}

@article{tanaka_generalized_2020,
 abstract = {We propose a framework for generalized sampling of graph signals that parallels sampling in shift invariant (SI) subspaces. This framework allows for arbitrary input signals which are not constrained to be bandlimited. Furthermore, the sampling and reconstruction filters may be different. We present design methods of the correction filter that compensate for these differences and lead to closed form expressions in the graph frequency domain. In this study, we consider two priors on graph signals: The first is a subspace prior, where the signal is assumed to lie in a periodic graph spectrum (PGS) subspace. The PGS subspace is proposed as a counterpart of the SI subspace used in standard sampling theory. The second is a smoothness prior that imposes a smoothness requirement on the graph signal. We suggest the use of recovery techniques when the recovery filter can be optimized and under a setting in which a predefined filter must be used. Sampling is performed in the graph frequency domain, which is a counterpart of ``sampling by modulation'' used in SI subspaces. We compare our approach with existing sampling techniques on graph signal processing. The effectiveness of the proposed generalized sampling approach is validated numerically through several experiments.},
 author = {Tanaka, Yuichi and Eldar, Yonina C.},
 doi = {10.1109/TSP.2020.2982325},
 file = {/home/matt/Zotero/storage/KJNMYSLF/Tanaka and Eldar - 2020 - Generalized Sampling on Graphs With Subspace and S.pdf;/home/matt/Zotero/storage/CRRWYYYV/9043719.html},
 issn = {1941-0476},
 journal = {IEEE Transactions on Signal Processing},
 pages = {2272--2286},
 title = {Generalized {{Sampling}} on {{Graphs With Subspace}} and {{Smoothness Priors}}},
 volume = {68},
 year = {2020}
}

@article{tanaka_spectral_2018,
 abstract = {Sampling methods for graph signals in the graph spectral domain are presented. Though the conventional sampling of graph signals can be regarded as sampling in the graph vertex domain, it does not have the desired characteristics in regard to the graph spectral domain. With the proposed methods, the down- and upsampled graph signals inherit the frequency-domain characteristics of the sampled signals defined in the time/spatial domain. The properties of the sampling effects were evaluated theoretically in comparison with those obtained with the conventional sampling method in the vertex domain. Various examples of signals on simple graphs enable precise understanding of the problem considered. Fractional sampling and Laplacian pyramid representation of graph signals are potential applications of these methods.},
 author = {Tanaka, Y.},
 doi = {10.1109/TSP.2018.2839620},
 file = {/home/matt/Zotero/storage/WLLAQHKK/Tanaka - 2018 - Spectral Domain Sampling of Graph Signals.pdf;/home/matt/Zotero/storage/W7LAGH5N/8362710.html},
 issn = {1053-587X},
 journal = {IEEE Transactions on Signal Processing},
 number = {14},
 pages = {3752--3767},
 title = {Spectral {{Domain Sampling}} of {{Graph Signals}}},
 volume = {66},
 year = {2018}
}

@inproceedings{tancik_fourier_2020,
 author = {Matthew Tancik and
Pratul P. Srinivasan and
Ben Mildenhall and
Sara Fridovich{-}Keil and
Nithin Raghavan and
Utkarsh Singhal and
Ravi Ramamoorthi and
Jonathan T. Barron and
Ren Ng},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/TancikSMFRSRBN20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Fourier Features Let Networks Learn High Frequency Functions in Low
Dimensional Domains},
 url = {https://proceedings.neurips.cc/paper/2020/hash/55053683268957697aa39fba6f231c68-Abstract.html},
 year = {2020}
}

@article{tang_disturbance-observer-based_2019,
 abstract = {The neural network policies are widely explored in the autonomous driving field, thanks to their capability of handling complicated driving tasks. However, the practical deployment of such policies is slowed down due to their lack of robustness against modeling gap and external disturbances. In our prior work, we proposed a planner-controller architecture and applied a disturbance-observer-based (DOB) robust tracking controller to reject the disturbances and achieved zero-shot policy transfer. In this paper, we present our latest progress on improving the policy transfer performance under this framework. Concretely, we applied adaptive DOB, so as to more accurately model the inverse system dynamics and increase the cut-off frequency of the Q-filter in the DOB. A closed-loop reference path smoothing algorithm is introduced to alleviate the step disturbance input imposed by the reference trajectory re-planning. On the neural network control policy side, we applied the parallel attribute networks, a hierarchical modular policy network to dynamically handle various driving tasks. We have carried out various simulations and experiments to validate the capability of our proposed method to achieve sim-to-sim and sim-to-real policy transfer. The proposed method achieves the most outstanding performance among a series of baseline control schemes.},
 author = {Tang, Chen and Xu, Zhuo and Tomizuka, Masayoshi},
 doi = {10.1109/TITS.2019.2951362},
 file = {/home/matt/Zotero/storage/LKFMP47Q/Tang et al. - 2019 - Disturbance-Observer-Based Tracking Controller for.pdf},
 issn = {1524-9050, 1558-0016},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 language = {en},
 pages = {1--12},
 title = {Disturbance-{{Observer}}-{{Based Tracking Controller}} for {{Neural Network Driving Policy Transfer}}},
 year = {2019}
}

@inproceedings{tang_graph-based_2021,
 author = {Binh Tang and
David S. Matteson},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/TangM21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Graph-Based Continual Learning},
 url = {https://openreview.net/forum?id=HHSEKOnPvaO},
 year = {2021}
}

@inproceedings{tang_local_2019,
 author = {Hao Tang and
Dan Xu and
Yan Yan and
Philip H. S. Torr and
Nicu Sebe},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/000500TS20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.00789},
 pages = {7867--7876},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {Local Class-Specific and Global Image-Level Generative Adversarial
Networks for Semantic-Guided Scene Generation},
 url = {https://doi.org/10.1109/CVPR42600.2020.00789},
 year = {2020}
}

@inproceedings{tang_multiple_2019,
 author = {Yichuan Charlie Tang and
Ruslan Salakhutdinov},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/TangS19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {15398--15408},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Multiple Futures Prediction},
 url = {https://proceedings.neurips.cc/paper/2019/hash/86a1fa88adb5c33bd7a68ac2f9f3f96b-Abstract.html},
 year = {2019}
}

@inproceedings{tao_supervised_2005,
 address = {{Houston, TX, USA}},
 author = {Tao, Dacheng and Li, Xuelong and Hu, Weiming and Maybank, Stephen and Wu, Xindong},
 booktitle = {Fifth {{IEEE International Conference}} on {{Data Mining}} ({{ICDM}}'05)},
 doi = {10.1109/ICDM.2005.139},
 file = {/home/matt/Zotero/storage/D46X99ZU/Tao et al. - 2005 - Supervised Tensor Learning.pdf},
 isbn = {978-0-7695-2278-4},
 pages = {450--457},
 publisher = {{IEEE}},
 title = {Supervised {{Tensor Learning}}},
 year = {2005}
}

@article{tassiulas_stability_1992,
 author = {Tassiulas, L. and Ephremides, A.},
 journal = {IEEE Trans. Auto. Control},
 number = {12},
 pages = {1936--1948},
 title = {Stability Properties of Constrained Queuing Systems and Scheduling Policies for Maximum Throughput in Multihop Radio Networks},
 volume = {37},
 year = {1992}
}

@techreport{teets_highway_1997,
 address = {{Washington, DC}},
 author = {Teets, Mary K.},
 institution = {{Federal Highway Administration}},
 number = {FHWA-PL-98-003},
 title = {Highway {{Statistics}} 1996},
 year = {1997}
}

@article{thananjeyan_abc-lmpc_2020,
 author = {Thananjeyan, Brijen and Balakrishna, Ashwin and Rosolia, Ugo and Gonzalez, Joseph E. and Ames, Aaron and Goldberg, Ken},
 journal = {ArXiv preprint},
 title = {{{ABC}}-{{LMPC}}: {{Safe Sample}}-{{Based Learning MPC}} for {{Stochastic Nonlinear Dynamical Systems}} with {{Adjustable Boundary Conditions}}},
 url = {https://arxiv.org/abs/2003.01410},
 volume = {abs/2003.01410},
 year = {2020}
}

@article{thananjeyan_extending_2019,
 author = {Thananjeyan, Brijen and Balakrishna, Ashwin and Rosolia, Ugo and Li, Felix and McAllister, Rowan and Gonzalez, Joseph E. and Levine, Sergey and Borrelli, Francesco and Goldberg, Ken},
 journal = {ArXiv preprint},
 title = {Extending {{Deep Model Predictive Control}} with {{Safety Augmented Value Estimation}} from {{Demonstrations}}},
 url = {https://arxiv.org/abs/1905.13402},
 volume = {abs/1905.13402},
 year = {2019}
}

@article{thananjeyan_extending_2019-1,
 author = {Thananjeyan, Brijen and Balakrishna, Ashwin and Rosolia, Ugo and Li, Felix and McAllister, Rowan and Gonzalez, Joseph E. and Levine, Sergey and Borrelli, Francesco and Goldberg, Ken},
 journal = {ArXiv preprint},
 title = {Extending {{Deep Model Predictive Control}} with {{Safety Augmented Value Estimation}} from {{Demonstrations}}},
 url = {https://arxiv.org/abs/1905.13402},
 volume = {abs/1905.13402},
 year = {2019}
}

@article{thananjeyan_safety_2019,
 abstract = {Reinforcement learning (RL) for robotics is challenging due to the difficulty in hand-engineering a dense cost function, which can lead to unintended behavior, and dynamical uncertainty, which makes exploration and constraint satisfaction challenging. We address these issues with a new modelbased reinforcement learning algorithm, Safety Augmented Value Estimation from Demonstrations (SAVED), which uses supervision that only identifies task completion and a modest set of suboptimal demonstrations to constrain exploration and learn efficiently while handling complex constraints. We derive iterative improvement guarantees for SAVED under known stochastic nonlinear systems. We then compare SAVED with 3 state-of-the-art model-based and model-free RL algorithms on 6 standard simulation benchmarks involving navigation and manipulation and a knot-tying task on the da Vinci surgical robot. Results suggest that SAVED outperforms prior methods in terms of success rate, constraint satisfaction, and sample efficiency, making it feasible to safely learn maneuvers directly on a real robot in less than an hour. For tasks on the robot, baselines succeed less than 5\% of the time while SAVED has a success rate of over 75\% in the first 50 training iterations. Code and supplementary material is available at https://tinyurl.com/saved-rl.},
 author = {Thananjeyan, Brijen and Balakrishna, Ashwin and Rosolia, Ugo and Li, Felix and McAllister, Rowan and Gonzalez, Joseph E and Levine, Sergey and Borrelli, Francesco and Goldberg, Ken},
 file = {/home/matt/Zotero/storage/RBXK3VJ2/Thananjeyan et al. - 2019 - Safety Augmented Value Estimation from Demonstrati.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Safety {{Augmented Value Estimation}} from {{Demonstrations}} ({{SAVED}}): {{Safe Deep Model}}-{{Based RL}} for {{Sparse Cost Robotic Tasks}}},
 year = {2019}
}

@article{thananjeyan_safety_2020,
 abstract = {Reinforcement learning (RL) for robotics is challenging due to the difficulty in hand-engineering a dense cost function, which can lead to unintended behavior, and dynamical uncertainty, which makes exploration and constraint satisfaction challenging. We address these issues with a new modelbased reinforcement learning algorithm, Safety Augmented Value Estimation from Demonstrations (SAVED), which uses supervision that only identifies task completion and a modest set of suboptimal demonstrations to constrain exploration and learn efficiently while handling complex constraints. We then compare SAVED with 3 state-of-the-art model-based and model-free RL algorithms on 6 standard simulation benchmarks involving navigation and manipulation and a physical knot-tying task on the da Vinci surgical robot. Results suggest that SAVED outperforms prior methods in terms of success rate, constraint satisfaction, and sample efficiency, making it feasible to safely learn a control policy directly on a real robot in less than an hour. For tasks on the robot, baselines succeed less than 5\% of the time while SAVED has a success rate of over 75\% in the first 50 training iterations. Code and supplementary material is available at https://tinyurl.com/saved-rl.},
 author = {Thananjeyan, Brijen and Balakrishna, Ashwin and Rosolia, Ugo and Li, Felix and McAllister, Rowan and Gonzalez, Joseph E. and Levine, Sergey and Borrelli, Francesco and Goldberg, Ken},
 doi = {10.1109/LRA.2020.2976272},
 file = {/home/matt/Zotero/storage/QU26X4LT/Thananjeyan et al. - 2020 - Safety Augmented Value Estimation from Demonstrati.pdf},
 issn = {2377-3766, 2377-3774},
 journal = {IEEE Robotics and Automation Letters},
 language = {en},
 pages = {1--1},
 shorttitle = {Safety {{Augmented Value Estimation}} from {{Demonstrations}} ({{SAVED}})},
 title = {Safety {{Augmented Value Estimation}} from {{Demonstrations}} ({{SAVED}}): {{Safe Deep Model}}-{{Based RL}} for {{Sparse Cost Robotic Tasks}}},
 year = {2020}
}

@book{the_pb_study_team_hov_2002,
 author = {{The PB Study Team}},
 title = {{{HOV Performance Program Evaluation Report}}. {{Los Angeles County Metropolitan Transportation Authority}}},
 year = {2002}
}

@article{thomson_operational_2012,
 author = {Thomson, Timothy and Liu, Xiaoyue Cathy and Wang, Yinhai and Schroeder, Bastian J. and Rouphail, Nagui M.},
 doi = {10.3141/2286-11},
 file = {/home/matt/Zotero/storage/6GVDTC6V/Thomson et al. - 2012 - Operational Performance and Speed–Flow Relationshi.pdf},
 issn = {0361-1981, 2169-4052},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 number = {1},
 pages = {94--104},
 title = {Operational {{Performance}} and {{Speed}}\textendash{{Flow Relationships}} for {{Basic Managed Lane Segments}}},
 volume = {2286},
 year = {2012}
}

@inproceedings{thost_directed_2021,
 author = {Veronika Thost and
Jie Chen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/Thost021.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {Directed Acyclic Graph Neural Networks},
 url = {https://openreview.net/forum?id=JbuYF437WB6},
 year = {2021}
}

@article{thrun_stanley_2006,
 author = {Thrun, Sebastian and Montemerlo, Mike and Dahlkamp, Hendrik and Stavens, David and Aron, Andrei and Diebel, James and Fong, Philip and Gale, John and Halpenny, Morgan and Hoffmann, Gabriel and Lau, Kenny and Oakley, Celia and Palatucci, Mark and Pratt, Vaughan and Stang, Pascal and Strohband, Sven and Dupont, Cedric and Jendrossek, Lars-Erik and Koelen, Christian and Markey, Charles and Rummel, Carlo and {\noopsort{niekerk}}van Niekerk, Joe and Jensen, Eric and Alessandrini, Philippe and Bradski, Gary and Davies, Bob and Ettinger, Scott and Kaehler, Adrian and Nefian, Ara and Mahoney, Pamela},
 journal = {ArXiv preprint},
 title = {Stanley: {{The}} Robot That Won the {{DARPA Grand Challenge}}},
 url = {https://arxiv.org/abs/10.1002},
 volume = {abs/10.1002},
 year = {2010}
}

@article{tian_rethinking_2020,
 author = {Tian, Yonglong and Wang, Yue and Krishnan, Dilip and Tenenbaum, Joshua B. and Isola, Phillip},
 journal = {ArXiv preprint},
 title = {Rethinking {{Few}}-{{Shot Image Classification}}: A {{Good Embedding Is All You Need}}?},
 url = {https://arxiv.org/abs/2003.11539},
 volume = {abs/2003.11539},
 year = {2020}
}

@book{tollroads_news_minnesota_2007,
 author = {{Tollroads News}},
 title = {Minnesota to Do Second Toll Express Lanes},
 year = {2007}
}

@book{topl_topl_2008,
 author = {{TOPL}},
 title = {{{TOPL}} Homepage},
 year = {2008}
}

@book{transportation_wim_2008,
 author = {{\noopsort{transportation}}of Transportation, California Department},
 title = {{{WIM Technical Overview}}},
 year = {2008}
}

@inproceedings{trautman_unfreezing_2010,
 address = {{Taipei}},
 author = {Trautman, Peter and Krause, Andreas},
 booktitle = {2010 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}}},
 doi = {10.1109/IROS.2010.5654369},
 isbn = {978-1-4244-6674-0},
 pages = {797--803},
 publisher = {{IEEE}},
 shorttitle = {Unfreezing the Robot},
 title = {Unfreezing the Robot: {{Navigation}} in Dense, Interacting Crowds},
 year = {2010}
}

@article{treiber_congested_2000,
 author = {Treiber, Martin and Hennecke, Ansgar and Helbing, Dirk},
 doi = {10.1103/PhysRevE.62.1805},
 file = {/home/matt/Zotero/storage/FZ8ID5TD/Treiber et al. - 2000 - Congested traffic states in empirical observations.pdf},
 issn = {1063-651X, 1095-3787},
 journal = {Physical Review E},
 language = {en},
 number = {2},
 pages = {1805--1824},
 title = {Congested Traffic States in Empirical Observations and Microscopic Simulations},
 volume = {62},
 year = {2000}
}

@article{treiber_derivation_1999,
 author = {Treiber, Martin and Hennecke, Ansgar and Helbing, Dirk},
 doi = {10.1103/PhysRevE.59.239},
 journal = {Physical Review E},
 number = {1},
 pages = {239--253},
 title = {Derivation, Properties, and Simulation of a Gas-Kinetic-Based, Nonlocal Traffic Model},
 volume = {59},
 year = {1999}
}

@book{treiber_traffic_2013,
 address = {{Berlin, Heidelberg}},
 author = {Treiber, Martin and Kesting, Arne},
 doi = {10.1007/978-3-642-32460-4},
 file = {/home/matt/Zotero/storage/CLWL2WTL/Treiber and Kesting - 2013 - Traffic Flow Dynamics.pdf},
 isbn = {978-3-642-32459-8 978-3-642-32460-4},
 language = {en},
 publisher = {{Springer Berlin Heidelberg}},
 title = {Traffic {{Flow Dynamics}}},
 year = {2013}
}

@inproceedings{trinh_learning_2018,
 author = {Trieu H. Trinh and
Andrew M. Dai and
Thang Luong and
Quoc V. Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/TrinhDLL18.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {4972--4981},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Learning Longer-term Dependencies in RNNs with Auxiliary Losses},
 url = {http://proceedings.mlr.press/v80/trinh18a.html},
 volume = {80},
 year = {2018}
}

@article{tsipras_there_2018,
 author = {Tsipras, Dimitris and Santurkar, Shibani and Engstrom, Logan and Turner, Alexander and Madry, Aleksander},
 file = {/home/matt/Zotero/storage/VAJ3X4XF/Tsipras et al. - 2018 - There Is No Free Lunch In Adversarial Robustness (.pdf;/home/matt/Zotero/storage/QPYNFRG4/1805.html},
 language = {en},
 title = {There {{Is No Free Lunch In Adversarial Robustness}} ({{But There Are Unexpected Benefits}})},
 year = {2018}
}

@inproceedings{tsuda_support_1999,
 address = {{Bruges}},
 author = {Tsuda, Koji},
 booktitle = {{{ESANN Proceedings}}},
 file = {/home/matt/Zotero/storage/95LIXG44/Tsuda - 1999 - Support Vector Classifier with Asymmetric Kernel F.pdf},
 pages = {183--188},
 title = {Support {{Vector Classifier}} with {{Asymmetric Kernel Functions}}},
 year = {1999}
}

@book{tsugawa_history_2008,
 annotation = {Published: IEEE International Conference on Vehicular Electronics and Safety (ICVES 2008)},
 author = {Tsugawa, S.},
 title = {A History of Automated Highway Systems in {{Japan}} and Future Issues},
 year = {2008}
}

@inproceedings{tucker_mirage_2018,
 author = {George Tucker and
Surya Bhupatiraju and
Shixiang Gu and
Richard E. Turner and
Zoubin Ghahramani and
Sergey Levine},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/TuckerBGTGL18.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {5022--5031},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {The Mirage of Action-Dependent Baselines in Reinforcement Learning},
 url = {http://proceedings.mlr.press/v80/tucker18a.html},
 volume = {80},
 year = {2018}
}

@techreport{turner_testing_2007,
 author = {Turner, S. and Middleton, D. and Longmire, R. and Brewer, M. and Eurek, R.},
 institution = {{Texas Transportation Institute}},
 number = {FHWA/TX-05/0-4422-2},
 title = {Testing and Evaluation of Pedestrian Sensors},
 year = {2007}
}

@techreport{turner_travel_1998,
 address = {{Washington, DC}},
 author = {Turner, Shawn M. and Eisele, William L. and Benz, Robert J. and Holdener, Douglas J.},
 institution = {{Federal Highway Administration}},
 number = {FHWA-PL-98-035},
 title = {Travel Time Collection Handbook},
 year = {1998}
}

@techreport{u.s._government_accountability_office_traffic_2012,
 author = {{U.S. Government Accountability Office}},
 institution = {{Report to the Subcommittee on Transportation, Housing, and Urban Development and Related Agencies, Committee on Appropriations, House of Representatives}},
 number = {GAO-12-119},
 title = {Traffic {{Congestion}}: {{Road Pricing Can Help Reduce Congestion}}, but {{Equity Concerns May Grow}}},
 year = {2012}
}

@techreport{unc_highway_safety_research_center_pedestrian_2010,
 author = {{UNC Highway Safety Research Center} and {Westat} and {VHB}},
 institution = {{Federal Highway Administration Office of Safety}},
 number = {FHWA-10-035},
 title = {Pedestrian {{Safety Strategic Plan}}: {{Recommendations}} for {{Research}} and {{Product Development}}},
 year = {2010}
}

@article{urakami_doorgym_2019,
 author = {Urakami, Yusuke and Hodgkinson, Alec and Carlin, Casey and Leu, Randall and Rigazio, Luca and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {{{DoorGym}}: {{A Scalable Door Opening Environment And Baseline Agent}}},
 url = {https://arxiv.org/abs/1908.01887},
 volume = {abs/1908.01887},
 year = {2019}
}

@article{van_lint_accurate_2005,
 author = {{\noopsort{lint}}{van Lint}, J.W.C. and Hoogendoorn, S.P. and {\noopsort{zuylen}}{van Zuylen}, H.J.},
 doi = {10.1016/j.trc.2005.03.001},
 file = {/home/matt/Zotero/storage/5N5IH8A9/vanlint_hoogendorn_neuralnetwork_2005.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 number = {5-6},
 pages = {347--369},
 title = {Accurate Freeway Travel Time Prediction with State-Space Neural Networks under Missing Data},
 volume = {13},
 year = {2005}
}

@article{van_lint_fastlane_2008,
 author = {{\noopsort{lint}}{van Lint}, J. and Hoogendoorn, Serge and Schreuder, Marco},
 doi = {10.3141/2088-19},
 file = {/home/matt/Zotero/storage/E72EWHSS/2008_TRR_FASTLANE.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {177--187},
 shorttitle = {Fastlane},
 title = {Fastlane: {{New Multiclass First}}-{{Order Traffic Flow Model}}},
 volume = {2088},
 year = {2008}
}

@article{van_vliet_saturn_1982,
 author = {Van Vliet, D.},
 journal = {Traffic Engineering and Control},
 number = {4},
 title = {{{SATURN}} - {{A}} Modern Traffic Assignment Model.},
 volume = {23},
 year = {1982}
}

@article{van_wageningen-kessels_lane_2015,
 abstract = {A new macroscopic steady state theory is proposed to explain how heterogeneous traffic distributes itself over the lanes of a congested highway. Firstly, a model is derived which predicts the speed of a given mixture of traffic within a single lane. The distribution over lanes is then phrased as an assignment problem, where it is assumed that individual drivers choose lanes so as to try to maximise their own speeds. Theory is derived which establishes circumstances in which the assignment matrix and consequent lane speeds can be solved for. Two examples are presented which demonstrate how the theory can be used to inform traffic management that employs either dynamic speed limits or mandatory lane policies. Future research and applications are then scoped.},
 author = {{\noopsort{wageningen-kessels}}{van Wageningen-Kessels}, Femke and Wilson, R. Eddie},
 doi = {10.1016/j.trpro.2015.09.051},
 file = {/home/matt/Zotero/storage/4HKZSUK6/van Wageningen-Kessels and Wilson - 2015 - Lane Distribution Estimation for Heterogeneous Tra.pdf},
 issn = {23521465},
 journal = {Transportation Research Procedia},
 language = {en},
 pages = {13--20},
 title = {Lane {{Distribution Estimation}} for {{Heterogeneous Traffic Flows}}},
 volume = {10},
 year = {2015}
}

@book{varaiya_counterexample_2007,
 author = {Varaiya, P.},
 title = {Counterexample to a {{Folk Theorem}} in {{Traffic Flow}}},
 year = {2007}
}

@unpublished{varaiya_dynamic_2007,
 author = {Varaiya, P.},
 title = {Dynamic Trip Assignment},
 year = {2007}
}

@article{varaiya_freeway_2008,
 author = {Varaiya, P.},
 journal = {Philosophical Trans. Royal Society A},
 pages = {1921--1930},
 title = {Freeway Congestion, Ramp Metering, and Tolls},
 volume = {366},
 year = {2008}
}

@book{varaiya_hot_2008,
 author = {Varaiya, P.},
 title = {{{HOT}} Tips},
 year = {2008}
}

@unpublished{varaiya_how_1997,
 author = {Varaiya, Pravin},
 title = {How to Measure Transportation System Performance},
 year = {1997}
}

@article{varaiya_max_2013,
 author = {Varaiya, Pravin},
 doi = {10.1016/j.trc.2013.08.014},
 file = {/home/matt/Zotero/storage/ULYCHFDC/varaiya_2013_maxpressure.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {177--195},
 title = {Max Pressure Control of a Network of Signalized Intersections},
 volume = {36},
 year = {2013}
}

@article{varaiya_reducing_2005,
 author = {Varaiya, P.},
 journal = {European Journal of Control},
 number = {4-5},
 pages = {301--309},
 title = {Reducing Highway Congestion: {{An}} Empirical Approach},
 volume = {11},
 year = {2005}
}

@book{varaiya_universal_2009,
 author = {Varaiya, P.},
 title = {A Universal Feedback Control Policy for Arbitrary Networks of Signalized Intersections},
 year = {2009}
}

@article{variya_smart_1993,
 author = {Variya, P.},
 journal = {IEEE Trans. Automatic Control},
 number = {2},
 pages = {195--207},
 title = {Smart Cars on Smart Roads: {{Problems}} of Control},
 volume = {38},
 year = {1993}
}

@inproceedings{vaswani_attention_2017,
 author = {Ashish Vaswani and
Noam Shazeer and
Niki Parmar and
Jakob Uszkoreit and
Llion Jones and
Aidan N. Gomez and
Lukasz Kaiser and
Illia Polosukhin},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/VaswaniSPUJGKP17.bib},
 booktitle = {Advances in Neural Information Processing Systems 30: Annual Conference
on Neural Information Processing Systems 2017, December 4-9, 2017,
Long Beach, CA, {USA}},
 editor = {Isabelle Guyon and
Ulrike von Luxburg and
Samy Bengio and
Hanna M. Wallach and
Rob Fergus and
S. V. N. Vishwanathan and
Roman Garnett},
 pages = {5998--6008},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Attention is All you Need},
 url = {https://proceedings.neurips.cc/paper/2017/hash/3f5ee243547dee91fbd053c1c4a845aa-Abstract.html},
 year = {2017}
}

@inproceedings{vaswani_tensor2tensor_2018,
 address = {Boston, MA},
 author = {Vaswani, Ashish  and
Bengio, Samy  and
Brevdo, Eugene  and
Chollet, Francois  and
Gomez, Aidan  and
Gouws, Stephan  and
Jones, Llion  and
Kaiser, {\L}ukasz  and
Kalchbrenner, Nal  and
Parmar, Niki  and
Sepassi, Ryan  and
Shazeer, Noam  and
Uszkoreit, Jakob},
 booktitle = {Proceedings of the 13th Conference of the Association for Machine Translation in the {A}mericas (Volume 1: Research Track)},
 pages = {193--199},
 publisher = {Association for Machine Translation in the Americas},
 title = {{T}ensor2{T}ensor for Neural Machine Translation},
 url = {https://aclanthology.org/W18-1819},
 year = {2018}
}

@article{vazquez-chanlatte_learning_2019,
 author = {{Vazquez-Chanlatte}, Marcell and Seshia, Sanjit A.},
 journal = {ArXiv preprint},
 title = {Learning {{Task Specifications}} from {{Demonstrations}} via the {{Principle}} of {{Maximum Causal Entropy}}},
 url = {https://arxiv.org/abs/1907.11792},
 volume = {abs/1907.11792},
 year = {2019}
}

@inproceedings{veerapaneni_entity_2019,
 abstract = {This paper tests the hypothesis that modeling a scene in terms of entities and their local interactions, as opposed to modeling the scene globally, provides a significant benefit in generalizing to physical tasks in a combinatorial space the learner has not encountered before. We present object-centric perception, prediction, and planning (OP3), which to the best of our knowledge is the first entity-centric dynamic latent variable framework for model-based reinforcement learning that acquires entity representations from raw visual observations without supervision and uses them to predict and plan. OP3 enforces entity-abstraction -- symmetric processing of each entity representation with the same locally-scoped function -- which enables it to scale to model different numbers and configurations of objects from those in training. Our approach to solving the key technical challenge of grounding these entity representations to actual objects in the environment is to frame this variable binding problem as an inference problem, and we developing an interactive inference algorithm that uses temporal continuity and interactive feedback to bind information about object properties to the entity variables. On block-stacking tasks, OP3 generalizes to novel block configurations and more objects than observed during training, outperforming an oracle model that assumes access to object supervision and achieving two to three times better accuracy than a state-of-the-art video prediction model.},
 archiveprefix = {arXiv},
 author = {Veerapaneni, Rishi and {Co-Reyes}, John D. and Chang, Michael and Janner, Michael and Finn, Chelsea and Wu, Jiajun and Tenenbaum, Joshua B. and Levine, Sergey},
 booktitle = {3rd {{Conference}} on {{Robot Learning}} ({{CoRL}} 2019)},
 eprint = {1910.12827},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/LHMMS6R3/Veerapaneni et al. - 2019 - Entity Abstraction in Visual Model-Based Reinforce.pdf;/home/matt/Zotero/storage/7EAIZ5QZ/1910.html},
 title = {Entity {{Abstraction}} in {{Visual Model}}-{{Based Reinforcement Learning}}},
 year = {2019}
}

@inproceedings{veerapaneni_entity_2019-1,
 abstract = {This paper tests the hypothesis that modeling a scene in terms of entities and their local interactions, as opposed to modeling the scene globally, provides a significant benefit in generalizing to physical tasks in a combinatorial space the learner has not encountered before. We present object-centric perception, prediction, and planning (OP3), which to the best of our knowledge is the first entity-centric probabilistic dynamic latent variable framework for model-based reinforcement learning that acquires entity representations from raw visual observations without supervision and uses them to predict and plan. OP3 enforces entity-abstraction \textendash{} symmetric processing of each entity representation with the same locally-scoped function \textendash{} which enables it to scale to model different numbers and configurations of objects from those in training. Our approach to solving the key technical challenge of grounding these entity representations to actual objects in the environment is to frame this variable binding problem as an inference problem, and we develop an interactive inference algorithm that uses temporal continuity and interactive feedback to bind information about object properties to the entity variables. On block-stacking tasks, OP3 generalizes to novel block configurations and more objects than observed during training, outperforming an oracle model that assumes access to object supervision and achieving two to three times better accuracy than a state-of-the-art video prediction model that does not exhibit entity abstraction.},
 archiveprefix = {arXiv},
 author = {Veerapaneni, Rishi and {Co-Reyes}, John D. and Chang, Michael and Janner, Michael and Finn, Chelsea and Wu, Jiajun and Tenenbaum, Joshua B. and Levine, Sergey},
 booktitle = {3rd {{Conference}} on {{Robot Learning}} ({{CoRL}} 2019)},
 eprint = {1910.12827},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/LPQ22RMG/Veerapaneni et al. - 2019 - Entity Abstraction in Visual Model-Based Reinforce.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Entity {{Abstraction}} in {{Visual Model}}-{{Based Reinforcement Learning}}},
 year = {2019}
}

@inproceedings{velickovic_graph_2018,
 author = {Petar Velickovic and
Guillem Cucurull and
Arantxa Casanova and
Adriana Romero and
Pietro Li{\`{o}} and
Yoshua Bengio},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/VelickovicCCRLB18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Graph Attention Networks},
 url = {https://openreview.net/forum?id=rJXMpikCZ},
 year = {2018}
}

@inproceedings{venugopalan_sequence_2015,
 author = {Subhashini Venugopalan and
Marcus Rohrbach and
Jeffrey Donahue and
Raymond J. Mooney and
Trevor Darrell and
Kate Saenko},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/VenugopalanRDMD15.bib},
 booktitle = {2015 {IEEE} International Conference on Computer Vision, {ICCV} 2015,
Santiago, Chile, December 7-13, 2015},
 doi = {10.1109/ICCV.2015.515},
 pages = {4534--4542},
 publisher = {{IEEE} Computer Society},
 timestamp = {Thu, 15 Jun 2017 01:00:00 +0200},
 title = {Sequence to Sequence - Video to Text},
 url = {https://doi.org/10.1109/ICCV.2015.515},
 year = {2015}
}

@article{verhoef_product_2007,
 author = {Verhoef, E. T. and Small, K. A.},
 journal = {Journal of Transport Economics and Policy},
 title = {Product Differentiation on Roads: Constrained Congestion Pricing with Heterogeneous Users},
 year = {2007}
}

@article{vespignani_complex_2010,
 abstract = {A study of failures in interconnected networks highlights the vulnerability of tightly coupled infrastructures and shows the need to consider mutually dependent network properties in designing resilient systems.},
 author = {Vespignani, Alessandro},
 copyright = {2010 Nature Publishing Group},
 doi = {10.1038/464984a},
 file = {/home/matt/Zotero/storage/X2L7CA56/Vespignani - 2010 - Complex networks The fragility of interdependency.pdf;/home/matt/Zotero/storage/UPM4SFGX/464984a.html},
 issn = {1476-4687},
 journal = {Nature},
 language = {en},
 number = {7291},
 pages = {984--985},
 shorttitle = {Complex Networks},
 title = {Complex Networks: {{The}} Fragility of Interdependency},
 volume = {464},
 year = {2010}
}

@article{vezzani_learning_2019,
 author = {Vezzani, Giulia and Gupta, Abhishek and Natale, Lorenzo and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {Learning Latent State Representation for Speeding up Exploration},
 url = {https://arxiv.org/abs/1905.12621},
 volume = {abs/1905.12621},
 year = {2019}
}

@article{vickery_congestion_1969,
 author = {Vickery, W. S.},
 journal = {American Economic Review},
 number = {2},
 pages = {251--260},
 title = {Congestion {{Theory}} and {{Transport Investment}}},
 volume = {59},
 year = {1969}
}

@article{vickery_pricing_1963,
 author = {Vickery, W. S.},
 journal = {American Economic Review},
 number = {2},
 pages = {452--465},
 title = {Pricing in {{Urban}} and {{Suburban Transport}}},
 volume = {53},
 year = {1963}
}

@article{vigos_real-time_2008,
 author = {Vigos, G. and Papageorgiou, M. and Wang, Y.},
 journal = {Transportation Research, Part C},
 pages = {18--35},
 title = {Real-Time Estimation of Vehicle-Count within Signalized Links},
 volume = {16},
 year = {2008}
}

@inproceedings{vinitsky_benchmarks_2018,
 abstract = {We release new benchmarks in the use of deep reinforcement learning (RL) to create controllers for mixed-autonomy traffic, where connected and autonomous vehicles (CAVs) interact with human drivers and infrastructure. Benchmarks, such as Mujoco or the Arcade Learning Environment, have spurred new research by enabling researchers to effectively compare their results so that they can focus on algorithmic improvements and control techniques rather than system design. To promote similar advances in traffic control via RL, we propose four benchmarks, based on three new traffic scenarios, illustrating distinct reinforcement learning problems with applications to mixed-autonomy traffic. We provide an introduction to each control problem, an overview of their MDP structures, and preliminary performance results from commonly used RL algorithms. For the purpose of reproducibility, the benchmarks, reference implementations, and tutorials are available at https://github.com/flow-project/flow.},
 address = {{Zurich, Switzerland}},
 author = {Vinitsky, Eugene and Kreidieh, Aboudy and Le Flem, Luc and Kheterpal, Nishant and Jang, Kathy and Wu, Cathy and Liaw, Richard and Liang, Eric and Bayen, Alexandre},
 booktitle = {Conference on {{Robot Learning}}},
 file = {/home/matt/Zotero/storage/2LU8U25J/Vinitsky and Kreidieh - Benchmarks for reinforcement learning in mixed-aut.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {399--409},
 title = {Benchmarks for Reinforcement Learning in Mixed-Autonomy Traffic},
 year = {2018}
}

@inproceedings{vinyals_pointer_2017,
 author = {Oriol Vinyals and
Meire Fortunato and
Navdeep Jaitly},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/VinyalsFJ15.bib},
 booktitle = {Advances in Neural Information Processing Systems 28: Annual Conference
on Neural Information Processing Systems 2015, December 7-12, 2015,
Montreal, Quebec, Canada},
 editor = {Corinna Cortes and
Neil D. Lawrence and
Daniel D. Lee and
Masashi Sugiyama and
Roman Garnett},
 pages = {2692--2700},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Pointer Networks},
 url = {https://proceedings.neurips.cc/paper/2015/hash/29921001f2f04bd3baee84a12e98098f-Abstract.html},
 year = {2015}
}

@article{virkler_field_2004,
 author = {Virkler, J. Tianand M. R. and Sun, C.},
 journal = {Transportation Research Record},
 pages = {210--216},
 title = {Field {{Testing}} for {{Automated Identification}} of {{Turning Movements}} at {{Signalized Intersections}}},
 volume = {1867},
 year = {2004}
}

@book{vong_monash-citylink-west_nodate,
 author = {Vong, V. and Gaffney, J.},
 title = {Monash-{{Citylink}}-{{West Gate}} Upgrade Project: {{Implementing}} Traffic Management Tools to Mitigate Freewy Congestion}
}

@inproceedings{wager_dropout_2013,
 author = {Stefan Wager and
Sida I. Wang and
Percy Liang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/WagerWL13.bib},
 booktitle = {Advances in Neural Information Processing Systems 26: 27th Annual
Conference on Neural Information Processing Systems 2013. Proceedings
of a meeting held December 5-8, 2013, Lake Tahoe, Nevada, United States},
 editor = {Christopher J. C. Burges and
L{\'{e}}on Bottou and
Zoubin Ghahramani and
Kilian Q. Weinberger},
 pages = {351--359},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Dropout Training as Adaptive Regularization},
 url = {https://proceedings.neurips.cc/paper/2013/hash/38db3aed920cf82ab059bfccbd02be6a-Abstract.html},
 year = {2013}
}

@article{waibel_phoneme_1989,
 abstract = {The authors present a time-delay neural network (TDNN) approach to phoneme recognition which is characterized by two important properties: (1) using a three-layer arrangement of simple computing units, a hierarchy can be constructed that allows for the formation of arbitrary nonlinear decision surfaces, which the TDNN learns automatically using error backpropagation; and (2) the time-delay arrangement enables the network to discover acoustic-phonetic features and the temporal relationships between them independently of position in time and therefore not blurred by temporal shifts in the input. As a recognition task, the speaker-dependent recognition of the phonemes B, D, and G in varying phonetic contexts was chosen. For comparison, several discrete hidden Markov models (HMM) were trained to perform the same task. Performance evaluation over 1946 testing tokens from three speakers showed that the TDNN achieves a recognition rate of 98.5\% correct while the rate obtained by the best of the HMMs was only 93.7\%.{$<>$}},
 author = {Waibel, A. and Hanazawa, T. and Hinton, G. and Shikano, K. and Lang, K.J.},
 doi = {10.1109/29.21701},
 file = {/home/matt/Zotero/storage/KTGUH3TN/Waibel et al. - 1989 - Phoneme recognition using time-delay neural networ.pdf;/home/matt/Zotero/storage/9Q5ARVWL/21701.html},
 issn = {0096-3518},
 journal = {IEEE Transactions on Acoustics, Speech, and Signal Processing},
 number = {3},
 pages = {328--339},
 title = {Phoneme Recognition Using Time-Delay Neural Networks},
 volume = {37},
 year = {1989}
}

@book{waldrop_complexity_1992,
 address = {{New York}},
 author = {Waldrop, M. Mitchell},
 isbn = {978-0-671-76789-1},
 lccn = {Q175 .W258 1992},
 publisher = {{Simon \& Schuster}},
 shorttitle = {Complexity},
 title = {Complexity: The Emerging Science at the Edge of Order and Chaos},
 year = {1992}
}

@inproceedings{wale_comparison_2006,
 abstract = {In recent years the development of computational techniques that build models to correctly assign chemical compounds to various classes or to retrieve potential drug-like compounds has been an active area of research. Many of the best-performing techniques for these tasks utilize a descriptor-based representation of the compound that captures various aspects of the underlying molecular graph's topology. In this paper we compare different set of descriptors that are currently used for chemical compound classification. In this process, we also introduce four different descriptors derived from all connected fragments present in the molecular graphs. In addition, we introduce an extension to existing vector-based kernel functions to take into account the length of the fragments present in the descriptors. We experimentally evaluate the performance of the previously introduced and the new descriptors in the context of SVM-based classification and ranked-retrieval on 28 classification and retrieval problems derived from 18 datasets. Our experiments show that for both these tasks, the new descriptors consistently and statistically outperform previously developed schemes based on the widely used fingerprint- and Maces keys-based descriptors, as well as recently introduced descriptors obtained by mining and analyzing the structure of the molecular graphs.},
 author = {Wale, Nikil and Karypis, George},
 booktitle = {Sixth {{International Conference}} on {{Data Mining}} ({{ICDM}}'06)},
 doi = {10.1109/ICDM.2006.39},
 file = {/home/matt/Zotero/storage/PQHDKR65/Wale and Karypis - 2006 - Comparison of Descriptor Spaces for Chemical Compo.pdf},
 issn = {2374-8486},
 pages = {678--689},
 title = {Comparison of {{Descriptor Spaces}} for {{Chemical Compound Retrieval}} and {{Classification}}},
 year = {2006}
}

@article{wallerberger_hypothesis_2017,
 author = {Wallerberger, Markus and Gull, Emanuel},
 doi = {10.1103/PhysRevE.96.053303},
 file = {/home/matt/Zotero/storage/LXTVJB75/Wallerberger and Gull - 2017 - Hypothesis testing of scientific Monte Carlo calcu.pdf},
 issn = {2470-0045, 2470-0053},
 journal = {Physical Review E},
 language = {en},
 number = {5},
 title = {Hypothesis Testing of Scientific {{Monte Carlo}} Calculations},
 volume = {96},
 year = {2017}
}

@article{walters_bottleneck_2002,
 author = {Walters, Carol},
 journal = {Texas Transportation Researcher},
 number = {2},
 pages = {8--9},
 title = {Do Bottleneck Improvements Really Reduce Congestion?},
 volume = {38},
 year = {2002}
}

@article{walters_theory_1961,
 author = {Walters, A. A.},
 journal = {Econometrica},
 number = {4},
 pages = {676--699},
 title = {The {{Theory}} and {{Measurement}} of {{Private}} and {{Social Cost}} of {{Highway Congestion}}},
 volume = {29},
 year = {1961}
}

@inproceedings{Wang_2019_CVPR,
 author = {Xin Wang and
Fisher Yu and
Ruth Wang and
Trevor Darrell and
Joseph E. Gonzalez},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/WangYWDG19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00193},
 pages = {1831--1840},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {TAFE-Net: Task-Aware Feature Embeddings for Low Shot Learning},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Wang\_TAFE-Net\_Task-Aware\_Feature\_Embeddings\_for\_Low\_Shot\_Learning\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{wang_cnn-generated_2019,
 author = {Sheng{-}Yu Wang and
Oliver Wang and
Richard Zhang and
Andrew Owens and
Alexei A. Efros},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/WangW0OE20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.00872},
 pages = {8692--8701},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {CNN-Generated Images Are Surprisingly Easy to Spot... for Now},
 url = {https://doi.org/10.1109/CVPR42600.2020.00872},
 year = {2020}
}

@article{wang_comparing_2017,
 author = {Wang, Ren and Li, Yanning and Work, Daniel B.},
 doi = {10.1016/j.trc.2017.02.011},
 file = {/home/matt/Documents/Papers/wang_work_state_estimation_avs.pdf},
 issn = {0968-090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {95--110},
 title = {Comparing Traffic State Estimators for Mixed Human and Automated Traffic Flows},
 volume = {78},
 year = {2017}
}

@article{wang_continuous_2019,
 author = {Wang, Pin and Li, Hanhan and Chan, Ching-Yao},
 journal = {ArXiv preprint},
 title = {Continuous {{Control}} for {{Automated Lane Change Behavior Based}} on {{Deep Deterministic Policy Gradient Algorithm}}},
 url = {https://arxiv.org/abs/1906.02275},
 volume = {abs/1906.02275},
 year = {2019}
}

@article{wang_cooperation_2020,
 author = {Wang, Rose E. and Kew, J. Chase and Lee, Dennis and Lee, Tsang-Wei Edward and Zhang, Tingnan and Ichter, Brian and Tan, Jie and Faust, Aleksandra},
 journal = {ArXiv preprint},
 title = {Cooperation without {{Coordination}}: {{Hierarchical Predictive Planning}} for {{Decentralized Multiagent Navigation}}},
 url = {https://arxiv.org/abs/2003.06906},
 volume = {abs/2003.06906},
 year = {2020}
}

@article{wang_data_2019,
 author = {Wang, Pin and Shi, Tianyu and Zou, Chonghao and Xin, Long and Chan, Ching-Yao},
 journal = {ArXiv preprint},
 title = {A {{Data Driven Method}} of {{Feedforward Compensator Optimization}} for {{Autonomous Vehicle Control}}},
 url = {https://arxiv.org/abs/1906.02277},
 volume = {abs/1906.02277},
 year = {2019}
}

@inproceedings{wang_deep_2019,
 abstract = {While learning visuomotor skills in an end-to-end manner is appealing, deep neural networks are often uninterpretable and fail in surprising ways. For robotics tasks, such as autonomous driving, models that explicitly represent objects may be more robust to new scenes and provide intuitive visualizations. We describe a taxonomy of ``object-centric'' models which leverage both object instances and end-to-end learning. In the Grand Theft Auto V simulator, we show that object-centric models outperform object-agnostic methods in scenes with other vehicles and pedestrians, even with an imperfect detector. We also demonstrate that our architectures perform well on real-world environments by evaluating on the Berkeley DeepDrive Video dataset, where an object-centric model outperforms object-agnostic models in the low-data regimes.},
 author = {Wang, D. and Devin, C. and Cai, Q. and Yu, F. and Darrell, T.},
 booktitle = {2019 {{International Conference}} on {{Robotics}} and {{Automation}} ({{ICRA}})},
 doi = {10.1109/ICRA.2019.8794224},
 file = {/home/matt/Zotero/storage/NUIBMAAX/8794224.html},
 pages = {8853--8859},
 title = {Deep {{Object}}-{{Centric Policies}} for {{Autonomous Driving}}},
 year = {2019}
}

@inproceedings{wang_deep_2019-1,
 abstract = {While learning visuomotor skills in an end-to-end manner is appealing, deep neural networks are often uninterpretable and fail in surprising ways. For robotics tasks, such as autonomous driving, models that explicitly represent objects may be more robust to new scenes and provide intuitive visualizations. We describe a taxonomy of ``object-centric'' models which leverage both object instances and end-to-end learning. In the Grand Theft Auto V simulator, we show that object-centric models outperform object-agnostic methods in scenes with other vehicles and pedestrians, even with an imperfect detector. We also demonstrate that our architectures perform well on real-world environments by evaluating on the Berkeley DeepDrive Video dataset, where an object-centric model outperforms object-agnostic models in the low-data regimes.},
 author = {Wang, D. and Devin, C. and Cai, Q. and Yu, F. and Darrell, T.},
 booktitle = {2019 {{International Conference}} on {{Robotics}} and {{Automation}} ({{ICRA}})},
 doi = {10.1109/ICRA.2019.8794224},
 file = {/home/matt/Zotero/storage/ALS8HMFF/Wang et al. - 2019 - Deep Object-Centric Policies for Autonomous Drivin.pdf;/home/matt/Zotero/storage/AELDI6IF/8794224.html},
 pages = {8853--8859},
 title = {Deep {{Object}}-{{Centric Policies}} for {{Autonomous Driving}}},
 year = {2019}
}

@inproceedings{wang_detecting_2019,
 author = {Sheng{-}Yu Wang and
Oliver Wang and
Richard Zhang and
Andrew Owens and
Alexei A. Efros},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/WangW0OE19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.01017},
 pages = {10071--10080},
 publisher = {{IEEE}},
 timestamp = {Thu, 05 Mar 2020 00:00:00 +0100},
 title = {Detecting Photoshopped Faces by Scripting Photoshop},
 url = {https://doi.org/10.1109/ICCV.2019.01017},
 year = {2019}
}

@article{wang_dynamic_2019,
 author = {Wang, Dequan and Shelhamer, Evan and Olshausen, Bruno and Darrell, Trevor},
 journal = {ArXiv preprint},
 title = {Dynamic {{Scale Inference}} by {{Entropy Minimization}}},
 url = {https://arxiv.org/abs/1908.03182},
 volume = {abs/1908.03182},
 year = {2019}
}

@article{wang_efficient_2016,
 author = {Wang, Ren and Fan, Shimao and Work, Daniel B.},
 doi = {10.1016/j.trc.2016.08.003},
 issn = {0968-090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 keywords = {Field implementation,Multiple model,Particle filter,Traffic estimation,Traffic incident detection},
 pages = {521--537},
 title = {Efficient Multiple Model Particle Filtering for Joint Traffic State Estimation and Incident Detection},
 volume = {71},
 year = {2016}
}

@inproceedings{wang_exploring_2019,
 author = {Tingwu Wang and
Jimmy Ba},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/WangB20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Exploring Model-based Planning with Policy Networks},
 url = {https://openreview.net/forum?id=H1exf64KwH},
 year = {2020}
}

@inproceedings{wang_fast_2019,
 author = {Qiang Wang and
Li Zhang and
Luca Bertinetto and
Weiming Hu and
Philip H. S. Torr},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/Wang0BHT19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00142},
 pages = {1328--1338},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Fast Online Object Tracking and Segmentation: {A} Unifying Approach},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Wang\_Fast\_Online\_Object\_Tracking\_and\_Segmentation\_A\_Unifying\_Approach\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{wang_frustratingly_2020,
 author = {Xin Wang and
Thomas E. Huang and
Joseph Gonzalez and
Trevor Darrell and
Fisher Yu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/WangH0DY20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {9919--9928},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Frustratingly Simple Few-Shot Object Detection},
 url = {http://proceedings.mlr.press/v119/wang20j.html},
 volume = {119},
 year = {2020}
}

@inproceedings{wang_glue_2019,
 author = {Alex Wang and
Amanpreet Singh and
Julian Michael and
Felix Hill and
Omer Levy and
Samuel R. Bowman},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/WangSMHLB19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {{GLUE:} {A} Multi-Task Benchmark and Analysis Platform for Natural
Language Understanding},
 url = {https://openreview.net/forum?id=rJ4km2R5t7},
 year = {2019}
}

@inproceedings{wang_idk_2018,
 author = {Xin Wang and
Yujia Luo and
Daniel Crankshaw and
Alexey Tumanov and
Fisher Yu and
Joseph E. Gonzalez},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/uai/WangLCTYG18.bib},
 booktitle = {Proceedings of the Thirty-Fourth Conference on Uncertainty in Artificial
Intelligence, {UAI} 2018, Monterey, California, USA, August 6-10,
2018},
 editor = {Amir Globerson and
Ricardo Silva},
 pages = {580--590},
 publisher = {{AUAI} Press},
 timestamp = {Thu, 12 Mar 2020 00:00:00 +0100},
 title = {{IDK} Cascades: Fast Deep Learning by Learning not to Overthink},
 url = {http://auai.org/uai2018/proceedings/papers/212.pdf},
 year = {2018}
}

@article{wang_inferring_2020,
 author = {Wang, Zining and Feng, Di and Zhou, Yiyang and Zhan, Wei and Rosenbaum, Lars and Timm, Fabian and Dietmayer, Klaus and Tomizuka, Masayoshi},
 journal = {ArXiv preprint},
 title = {Inferring {{Spatial Uncertainty}} in {{Object Detection}}},
 url = {https://arxiv.org/abs/2003.03644},
 volume = {abs/2003.03644},
 year = {2020}
}

@article{wang_language_2019,
 author = {Wang, Chenguang and Li, Mu and Smola, Alexander J.},
 journal = {ArXiv preprint},
 title = {Language {{Models}} with {{Transformers}}},
 url = {https://arxiv.org/abs/1904.09408},
 volume = {abs/1904.09408},
 year = {2019}
}

@article{wang_latte_2019,
 author = {Wang, Bernie and Wu, Virginia and Wu, Bichen and Keutzer, Kurt},
 journal = {ArXiv preprint},
 title = {{{LATTE}}: {{Accelerating LiDAR Point Cloud Annotation}} via {{Sensor Fusion}}, {{One}}-{{Click Annotation}}, and {{Tracking}}},
 url = {https://arxiv.org/abs/1904.09085},
 volume = {abs/1904.09085},
 year = {2019}
}

@article{wang_learning_2019,
 author = {Wang, Angelina and Kurutach, Thanard and Liu, Kara and Abbeel, Pieter and Tamar, Aviv},
 journal = {ArXiv preprint},
 title = {Learning {{Robotic Manipulation}} through {{Visual Planning}} and {{Acting}}},
 url = {https://arxiv.org/abs/1905.04411},
 volume = {abs/1905.04411},
 year = {2019}
}

@inproceedings{wang_learning_2019-1,
 address = {Florence, Italy},
 author = {Wang, Qiang  and
Li, Bei  and
Xiao, Tong  and
Zhu, Jingbo  and
Li, Changliang  and
Wong, Derek F.  and
Chao, Lidia S.},
 booktitle = {Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/P19-1176},
 pages = {1810--1822},
 publisher = {Association for Computational Linguistics},
 title = {Learning Deep Transformer Models for Machine Translation},
 url = {https://aclanthology.org/P19-1176},
 year = {2019}
}

@inproceedings{wang_learning_2020,
 author = {Linnan Wang and
Rodrigo Fonseca and
Yuandong Tian},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/WangFT20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Learning Search Space Partition for Black-box Optimization using Monte
Carlo Tree Search},
 url = {https://proceedings.neurips.cc/paper/2020/hash/e2ce14e81dba66dbff9cbc35ecfdb704-Abstract.html},
 year = {2020}
}

@article{wang_monocular_2019,
 author = {Wang, Dequan and Devin, Coline and Cai, Qi-Zhi and Kr{\"a}henb{\"u}hl, Philipp and Darrell, Trevor},
 journal = {ArXiv preprint},
 title = {Monocular {{Plan View Networks}} for {{Autonomous Driving}}},
 url = {https://arxiv.org/abs/1905.06937},
 volume = {abs/1905.06937},
 year = {2019}
}

@inproceedings{wang_precise_2019,
 abstract = {Robust 3D perception using LiDAR is of prime importance for robotics, and its fundamental core lies in precise object modelling resisting to noise and outliers. In this paper, a precise 3D object modelling algorithm is designed especially for the intelligent vehicles. The proposed algorithm is advantageous by leveraging the crucial traffic geometrical prior of road surface profile, and both the noise and outliers are elegantly handled by robust correntropy-based metric. More specifically, the road surface correction (RSC) method transforms each individual LiDAR measurement from its locally planar road surface to a globally ideal plane. This procedure essentially guarantees the reduction of vehicle's motion from arbitrary 3D motion to physically feasible 2D motion. To deal with the noise and outliers, a correntropy-based multi-frame matching (CorrMM) algorithm is proposed which has a robust objective function with respect to point-to-plane residual error. An efficient solver inspired by M-estimator and retraction technique on Lie group is developed, which elegantly converts the optimization of highly non-linear objective function into a simple quadratic programming (QP) problem. Extensive experimental results validate that the proposed algorithm attains more crisper 3D object models than several state-of-the-art algorithms on a challenging real traffic dataset.},
 address = {{Macau, China}},
 author = {Wang, Di and Xue, Jianru and Zhan, Wei and Jin, Yinghan and Zheng, Nanning and Tomizuka, Masayoshi},
 booktitle = {2019 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}} ({{IROS}})},
 doi = {10.1109/IROS40897.2019.8967589},
 file = {/home/matt/Zotero/storage/F882TEFD/Wang et al. - 2019 - Precise Correntropy-based 3D Object Modelling With.pdf},
 isbn = {978-1-72814-004-9},
 language = {en},
 pages = {2608--2613},
 publisher = {{IEEE}},
 title = {Precise {{Correntropy}}-Based {{3D Object Modelling With Geometrical Traffic Prior}}},
 year = {2019}
}

@inproceedings{wang_quadratic_2019,
 abstract = {Reinforcement Learning algorithms have recently been proposed to learn timesequential control policies in the field of autonomous driving. Direct applications of Reinforcement Learning algorithms with discrete action space will yield unsatisfactory results at the operational level of driving where continuous control actions are actually required. In addition, the design of neural networks often fails to incorporate the domain knowledge of the targeting problem such as the classical control theories in our case. In this paper, we propose a hybrid model by combining Q-learning and classic PID (Proportion Integration Differentiation) controller for handling continuous vehicle control problems under dynamic driving environment. Particularly, instead of using a big neural network as Q-function approximation, we design a Quadratic Q-function over actions with multiple simple neural networks for finding optimal values within a continuous space. We also build an action network based on the domain knowledge of the control mechanism of a PID controller to guide the agent to explore optimal actions more efficiently. We test our proposed approach in simulation under two common but challenging driving situations, the lane change scenario and ramp merge scenario. Results show that the autonomous vehicle agent can successfully learn a smooth and efficient driving behavior in both situations.},
 address = {{Vancouver, Canada}},
 archiveprefix = {arXiv},
 author = {Wang, Pin and Li, Hanhan and Chan, Ching-Yao},
 booktitle = {Machine {{Learning}} for {{Autonomous Driving Workshop}} at {{NeurIPS}} 2019},
 eprint = {1912.00074},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/MBYN5FKM/Wang et al. - 2019 - Quadratic Q-network for Learning Continuous Contro.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Quadratic {{Q}}-Network for {{Learning Continuous Control}} for {{Autonomous Vehicles}}},
 year = {2019}
}

@article{wang_real-time_2005,
 author = {Wang, Yibing and Papageorgiou, Markos},
 doi = {10.1016/j.trb.2004.03.003},
 file = {/home/matt/Zotero/storage/TGUBKX9X/wang_freeway_ekf.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {2},
 pages = {141--167},
 shorttitle = {Real-Time Freeway Traffic State Estimation Based on Extended {{Kalman}} Filter},
 title = {Real-Time Freeway Traffic State Estimation Based on Extended {{Kalman}} Filter: A General Approach},
 volume = {39},
 year = {2005}
}

@inproceedings{wang_review_2018,
 abstract = {Connected and automated vehicles (CAVs) have the potential to address the safety, mobility and sustainability issues of our current transportation systems. Cooperative adaptive cruise control (CACC), for example, is one promising technology to allow CAVs to be driven in a cooperative manner and introduces system-wide benefits. In this paper, we review the progress achieved by researchers worldwide regarding different aspects of CACC systems. Literature of CACC system architectures are reviewed, which explain how this system works from a higher level. Different control methodologies and their related issues are reviewed to introduce CACC systems from a lower level. Applications of CACC technology are demonstrated with detailed literature, which draw an overall landscape of CACC, point out current opportunities and challenges, and anticipate its development in the near future.},
 address = {{Maui, HI}},
 author = {Wang, Ziran and Wu, Guoyuan and Barth, Matthew J.},
 booktitle = {2018 21st {{International Conference}} on {{Intelligent Transportation Systems}} ({{ITSC}})},
 doi = {10.1109/ITSC.2018.8569947},
 file = {/home/matt/Zotero/storage/LF6SS3TQ/Wang et al. - 2018 - A Review on Cooperative Adaptive Cruise Control (C.pdf},
 isbn = {978-1-72810-321-1 978-1-72810-323-5},
 language = {en},
 pages = {2884--2891},
 publisher = {{IEEE}},
 shorttitle = {A {{Review}} on {{Cooperative Adaptive Cruise Control}} ({{CACC}}) {{Systems}}},
 title = {A {{Review}} on {{Cooperative Adaptive Cruise Control}} ({{CACC}}) {{Systems}}: {{Architectures}}, {{Controls}}, and {{Applications}}},
 year = {2018}
}

@techreport{wang_safety_2019,
 address = {{Institute of Transportation Studies}},
 author = {Wang, Peggy and Motamedi, Sanaz and Canas Bajo, Teresa and Zhou, Xiao and Qi, Shouming and Zhang, Tingting and Whitney, David and Chan, Ching-Yao},
 file = {/home/matt/Zotero/storage/N26BKBFF/Wang et al. - 2019 - Safety Implications of Automated Vehicle Providing.pdf},
 institution = {{University of California, Berkeley}},
 keywords = {⛔ No DOI found},
 language = {en},
 number = {UC-ITS-2019-12},
 pages = {45},
 title = {Safety {{Implications}} of {{Automated Vehicle Providing External Communication}} to {{Pedestrians}}},
 year = {2019}
}

@article{wang_tactical_2020,
 abstract = {In this study, a deep reinforcement learning approach is proposed to handle tactical driving in complex highway traffic environments for unmanned ground vehicles. Tactical driving is a challenging topic for unmanned ground vehicles because of its interplay with routing decisions as well as real-time traffic dynamics. The core of our deep reinforcement learning approach is a deep Q-network that takes dynamic traffic information as input and outputs typical tactical driving decisions as action. The reward is designed with the consideration of successful highway exit, average traveling speed, and driving safety and comfort. In order to endow an unmanned ground vehicle with situational traffic information that is critical for tactical driving, the vehicle's sensor information such as vehicle position and velocity are further augmented through the assessment of the ego-vehicle's collision risk, potential field, and kinematics and used as input for the deep Q-network model. A convolutional neural network is built and fine-tuned to extract traffic features which facilitate the decision-making process of Q-learning. For model training and testing, a highway simulation platform is constructed with realistic parameter settings obtained from a real-world highway traffic dataset. The performance of the deep Q-network model is validated with extensive simulation experiments under different parameter settings such as traffic density and risk level. The results exhibit the important potentials of our deep Q-network model in learning challenging tactical driving decisions given multiple objectives and complex traffic environment.},
 author = {Wang, Huanjie and Yuan, Shihua and Guo, Mengyu and Chan, Ching-Yao and Li, Xueyuan and Lan, Wei},
 doi = {10.1177/0954407019898009},
 file = {/home/matt/Zotero/storage/CSUA5JVK/Wang et al. - 2020 - Tactical driving decisions of unmanned ground vehi.pdf},
 issn = {0954-4070, 2041-2991},
 journal = {Proceedings of the Institution of Mechanical Engineers, Part D: Journal of Automobile Engineering},
 language = {en},
 pages = {095440701989800},
 shorttitle = {Tactical Driving Decisions of Unmanned Ground Vehicles in Complex Highway Environments},
 title = {Tactical Driving Decisions of Unmanned Ground Vehicles in Complex Highway Environments: {{A}} Deep Reinforcement Learning Approach},
 year = {2020}
}

@inproceedings{wang_tafe-net_nodate,
 author = {Xin Wang and
Fisher Yu and
Ruth Wang and
Trevor Darrell and
Joseph E. Gonzalez},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/WangYWDG19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00193},
 pages = {1831--1840},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {TAFE-Net: Task-Aware Feature Embeddings for Low Shot Learning},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Wang\_TAFE-Net\_Task-Aware\_Feature\_Embeddings\_for\_Low\_Shot\_Learning\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{wang_tafe-net_nodate-1,
 author = {Xin Wang and
Fisher Yu and
Ruth Wang and
Trevor Darrell and
Joseph E. Gonzalez},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/WangYWDG19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00193},
 pages = {1831--1840},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {TAFE-Net: Task-Aware Feature Embeddings for Low Shot Learning},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Wang\_TAFE-Net\_Task-Aware\_Feature\_Embeddings\_for\_Low\_Shot\_Learning\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{wang_task-aware_2019,
 author = {Wang, Xin and Yu, Fisher and Darrell, Trevor and Gonzalez, Joseph E.},
 journal = {ArXiv preprint},
 title = {Task-{{Aware Deep Sampling}} for {{Feature Generation}}},
 url = {https://arxiv.org/abs/1906.04854},
 volume = {abs/1906.04854},
 year = {2019}
}

@article{wang_temporal_2021,
 author = {Wang, Hao and Wang, Weining and Liu, Jing},
 journal = {ArXiv preprint},
 title = {Temporal {{Memory Attention}} for {{Video Semantic Segmentation}}},
 url = {https://arxiv.org/abs/2102.08643},
 volume = {abs/2102.08643},
 year = {2021}
}

@inproceedings{wang_weston-watkins_2020,
 author = {Yutong Wang and
Clayton Scott},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/WangS20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Weston-Watkins Hinge Loss and Ordered Partitions},
 url = {https://proceedings.neurips.cc/paper/2020/hash/e5e6851e7f7ffd3530e7389e183aa468-Abstract.html},
 year = {2020}
}

@article{wardrop_theoretical_1952,
 author = {Wardrop, J. G.},
 journal = {Proceedings of the Institute of Civil Engineers, Part II},
 pages = {325--378},
 title = {Some {{Theoretical Aspects}} of {{Road Traffic Research}}},
 volume = {1},
 year = {1952}
}

@article{wasson_real-time_2008,
 author = {Wasson, J. S. and Sturdevant, J. R. and James, R. and Bullock, D. M.},
 journal = {ITE Journal},
 number = {6},
 title = {Real-{{Time Travel Time Estimates Using Media Access Control Address Matching}}},
 volume = {78},
 year = {2008}
}

@article{waters_tesla_2013,
 author = {Waters, R.},
 journal = {The Financial Times},
 title = {Tesla Moves Ahead from {{Google}} in Race to Build Self-Driving Cars},
 year = {2013}
}

@article{wei_adaptive_2009,
 author = {Wei, Tao and Huang, Yufei and Chen, C. L. Philip},
 doi = {10.1109/TSMCC.2008.2006759},
 file = {/home/matt/Zotero/storage/QCAR3GGA/04787243.pdf},
 issn = {1094-6977},
 journal = {IEEE Transactions on Systems, Man, and Cybernetics, Part C (Applications and Reviews)},
 number = {2},
 pages = {201--213},
 title = {Adaptive {{Sensor Fault Detection}} and {{Identification Using Particle Filter Algorithms}}},
 volume = {39},
 year = {2009}
}

@inproceedings{wei_eda_2019,
 address = {Hong Kong, China},
 author = {Wei, Jason  and
Zou, Kai},
 booktitle = {Proceedings of the 2019 Conference on Empirical Methods in Natural Language Processing and the 9th International Joint Conference on Natural Language Processing (EMNLP-IJCNLP)},
 doi = {10.18653/v1/D19-1670},
 pages = {6382--6388},
 publisher = {Association for Computational Linguistics},
 title = {{EDA}: Easy Data Augmentation Techniques for Boosting Performance on Text Classification Tasks},
 url = {https://aclanthology.org/D19-1670},
 year = {2019}
}

@article{wen_online_2006,
 author = {Wen, Y. and Balakrishna, R. and {Ben-Akiva}, M.},
 journal = {IEE Proceedings on Intelligent Transportation Systems},
 number = {1},
 pages = {76--84},
 title = {Online Deployment of Dynamic Traffic Assignment: Architecture and Run-Time Management},
 volume = {153},
 year = {2006}
}

@inproceedings{wen_urbanloco_2019,
 abstract = {Mapping and localization is a critical module of autonomous driving, and significant achievements have been reached in this field. Beyond Global Navigation Satellite System (GNSS), research in point cloud registration, visual feature matching, and inertia navigation has greatly enhanced the accuracy and robustness of mapping and localization in different scenarios. However, highly urbanized scenes are still challenging: LIDAR- and camera-based methods perform poorly with numerous dynamic objects; the GNSS-based solutions experience signal loss and multipath problems; the inertia measurement units (IMU) suffer from drifting. Unfortunately, current public datasets either do not adequately address this urban challenge or do not provide enough sensor information related to mapping and localization. Here we present UrbanLoco: a mapping/localization dataset collected in highly-urbanized environments with a full sensor-suite. The dataset includes 13 trajectories collected in San Francisco and Hong Kong, covering a total length of over 40 kilometers. Our dataset includes a wide variety of urban terrains: urban canyons, bridges, tunnels, sharp turns, etc. More importantly, our dataset includes information from LIDAR, cameras, IMU, and GNSS receivers. Now the dataset is publicly available through the link in the footnote. Dataset Link: https://advdataset2019.wixsite.com/advlocalization.},
 archiveprefix = {arXiv},
 author = {Wen, Weisong and Zhou, Yiyang and Zhang, Guohao and {Fahandezh-Saadi}, Saman and Bai, Xiwei and Zhan, Wei and Tomizuka, Masayoshi and Hsu, Li-Ta},
 booktitle = {Submitted to {{International Conference}} on {{Robotics}} and {{Animation}} ({{ICRA}}) 2020},
 eprint = {1912.09513},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/DRLIH2C4/Wen et al. - 2019 - UrbanLoco A Full Sensor Suite Dataset for Mapping.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 shorttitle = {{{UrbanLoco}}},
 title = {{{UrbanLoco}}: {{A Full Sensor Suite Dataset}} for {{Mapping}} and {{Localization}} in {{Urban Scenes}}},
 year = {2019}
}

@article{westenbroek_feedback_2019,
 author = {Westenbroek, Tyler and {Fridovich-Keil}, David and Mazumdar, Eric and Arora, Shreyas and Prabhu, Valmik and Sastry, S. Shankar and Tomlin, Claire J.},
 journal = {ArXiv preprint},
 title = {Feedback {{Linearization}} for {{Unknown Systems}} via {{Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1910.13272},
 volume = {abs/1910.13272},
 year = {2019}
}

@article{white_nissan_2013,
 author = {White, J. B.},
 journal = {Wall Street Journal},
 title = {Nissan {{Expects}} to {{Market Self}}-{{Driving Cars}} by 2020},
 year = {2013}
}

@inproceedings{wiering_multi-agent_2000,
 author = {Wiering, MA},
 booktitle = {Proceedings of the {{Seventeenth International Conference}} on {{Machine Learning}} ({{ICML}} 2000)},
 file = {/home/matt/Documents/Papers/wiering_00_multi.pdf;/home/matt/Zotero/storage/W3K46ZV5/wiering_00_multi.pdf},
 pages = {1151--1158},
 title = {Multi-Agent Reinforcement Learning for Traffic Light Control},
 year = {2000}
}

@misc{wiering_wiering_00_multi.pdf_nodate,
 author = {Wiering, Marco},
 file = {/home/matt/Documents/Papers/wiering_00_multi.pdf},
 title = {Wiering\_00\_multi.Pdf}
}

@article{william_enhancement_2008,
 author = {William, S. N. Shoukry aand G. W. and Riad, M. Y. and Luo, Y.},
 journal = {Bridge Structures},
 number = {3-4},
 pages = {121--133},
 title = {Enhancement of Bridge Live Loads Based on {{West Virginia}} Weigh-in-Motion Data},
 volume = {4},
 year = {2008}
}

@inproceedings{williams_using_2001,
 author = {Christopher K. I. Williams and
Matthias W. Seeger},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/WilliamsS00.bib},
 booktitle = {Advances in Neural Information Processing Systems 13, Papers from
Neural Information Processing Systems {(NIPS)} 2000, Denver, CO, {USA}},
 editor = {Todd K. Leen and
Thomas G. Dietterich and
Volker Tresp},
 pages = {682--688},
 publisher = {{MIT} Press},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Using the Nystr{\"{o}}m Method to Speed Up Kernel Machines},
 url = {https://proceedings.neurips.cc/paper/2000/hash/19de10adbaa1b2ee13f77f679fa1483a-Abstract.html},
 year = {2000}
}

@article{willsey_egg_2020,
 author = {Willsey, Max and Nandi, Chandrakana and Wang, Yisu Remy and Flatt, Oliver and Tatlock, Zachary and Panchekha, Pavel},
 journal = {ArXiv preprint},
 title = {Egg: {{Fast}} and {{Extensible Equality Saturation}}},
 url = {https://arxiv.org/abs/2004.03082},
 volume = {abs/2004.03082},
 year = {2020}
}

@article{windover_observed_2001,
 author = {Windover, J. R. and Cassidy, M.},
 journal = {Transportation Research, Part A},
 pages = {881--894},
 title = {Some Observed Details of Freeway Traffic Evolution},
 volume = {35},
 year = {2001}
}

@article{wischik_making_2005,
 author = {Wischik, D. and McKeown, N.},
 journal = {ACM SIGCOMM Computer Communication Review},
 number = {3},
 pages = {73--78},
 title = {Making Router Buffers Much Smaller},
 volume = {35},
 year = {2005}
}

@article{wong_multi-class_2002,
 author = {Wong, G. C. K. and Wong, S. C.},
 doi = {10.1016/S0965-8564(01)00042-8},
 file = {/home/matt/Zotero/storage/USWK5F5K/2002_TRA_multiclass_multispeed.pdf},
 journal = {Transportation Research Part A: Policy and Practice},
 number = {9},
 pages = {827--841},
 title = {A Multi-Class Traffic Flow Model\textendash an Extension of {{LWR}} Model with Heterogeneous Drivers},
 volume = {36},
 year = {2002}
}

@article{wong_reserve_1997,
 abstract = {whole capacity of a road network is controlled by intersections whose capacity depends on traffic signal settings. We first define and formulate the reserve capacity of a whole signal-controlled road network, and then show how a b\&level programming method can be used to determine signal setting for maximization of the network reserve capacity.},
 author = {Wong, S. C. and Yang, H.},
 journal = {Transportation Research B},
 number = {5},
 pages = {397--402},
 title = {Reserve Capacity of a Signal-Controlled Road Network},
 volume = {31},
 year = {1997}
}

@book{wongpiromsarn_distributed_2012,
 author = {Wongpiromsarn, T. and Uthaicharoenpong, T. and Wang, Y. and Frazzoli, E. and Wang, D.},
 title = {Distributed {{Traffic Signal Control}} for {{Maximum Network Throughput}}},
 year = {2012}
}

@article{work_traffic_2010,
 author = {Work, D. B. and Blandin, S. and Tossavainen, O. P. and Piccoli, B. and Bayen, A. M.},
 doi = {10.1093/amrx/abq002},
 file = {/home/matt/Zotero/storage/MZIWVPI9/work_2010_vctm.pdf},
 issn = {1687-1200, 1687-1197},
 journal = {Applied Mathematics Research eXpress},
 language = {en},
 number = {1},
 pages = {1--35},
 title = {A {{Traffic Model}} for {{Velocity Data Assimilation}}},
 volume = {2010},
 year = {2010}
}

@article{wright_attentional_2019,
 author = {Wright, Matthew A. and Horowitz, Roberto},
 journal = {ArXiv preprint},
 title = {Attentional {{Policies}} for {{Cross}}-{{Context Multi}}-{{Agent Reinforcement Learning}}},
 url = {https://arxiv.org/abs/1905.13428},
 volume = {abs/1905.13428},
 year = {2019}
}

@inproceedings{wright_dynamic_2016,
 address = {{Monterey, CA}},
 author = {Wright, Matthew and Horowitz, Roberto and Kurzhanskiy, Alex A.},
 booktitle = {Proceedings of the 10th {{IFAC Symposium}} on {{Nonlinear Control Systems}}},
 doi = {10.1016/j.ifacol.2016.10.307},
 file = {/home/matt/Zotero/storage/55WLJ7N7/Wright et al. - 2016 - A dynamic system characterization of road network .pdf},
 language = {en},
 pages = {1054--1059},
 title = {A Dynamic System Characterization of Road Network Node Models},
 volume = {49},
 year = {2016}
}

@inproceedings{wright_dynamic-system-based_2018,
 abstract = {To help mitigate road congestion caused by the unrelenting growth of traffic demand, many transportation authorities have implemented managed lane policies, which restrict certain freeway lanes to certain types of vehicles. It was originally thought that managed lanes would improve the use of existing infrastructure through demand-management behaviors like carpooling, but implementations have often been characterized by unpredicted phenomena that are sometimes detrimental to system performance. The development of traffic models that can capture these sorts of behaviors is a key step for helping managed lanes deliver on their promised gains. Towards this goal, this paper presents an approach for solving for driver behavior of entering and exiting managed lanes at the macroscopic (i.e., fluid approximation of traffic) scale. Our method is inspired by recent work in extending a dynamic-system-based modeling framework from traffic behaviors on individual roads, to models at junctions, and can be considered a further extension of this dynamic-system paradigm to the route/lane choice problem. Unlike traditional route choice models that are often based on discrete-choice methods and often rely on computing and comparing drivers' estimated travel times from taking different routes, our method is agnostic to the particular choice of physical traffic model and is suited specifically towards making decisions at these interfaces using only local information. These features make it a natural drop-in component to extend existing dynamic traffic modeling methods.},
 author = {Wright, Matthew A. and Horowitz, Roberto and Kurzhanskiy, Alex A.},
 booktitle = {Proceedings of the {{ASME}} 2018 {{Dynamic Systems}} and {{Controls Conference}} ({{DSCC}})},
 doi = {10.1115/DSCC2018-9125},
 file = {/home/matt/Zotero/storage/WFYGN48K/Wright et al. - 2018 - A Dynamic-System-Based Approach to Modeling Driver.pdf},
 isbn = {978-0-7918-5190-6},
 pages = {V002T15A003},
 publisher = {{ASME}},
 title = {A {{Dynamic}}-{{System}}-{{Based Approach}} to {{Modeling Driver Movements Across General}}-{{Purpose}}/{{Managed Lane Interfaces}}},
 year = {2018}
}

@article{wright_framework_2020,
 abstract = {This article presents a model-based method for fusing data from multiple sensors with a hypothesis-test-based component for rejecting potentially faulty or otherwise malign data. Our framework is based on an extension of the classic particle filter algorithm for real-time state estimation of uncertain systems with nonlinear dynamics with partial and noisy observations. This extension, based on classical statistical theories, utilizes statistical tests against the system's observation model. We discuss the application of the two major statistical testing frameworks, Fisher significance testing and Neyman\textendash Pearson hypothesis testing, to the Monte Carlo and sensor fusion settings. The Monte Carlo Neyman\textendash Pearson test we develop is useful when one has a reliable model of faulty data, while the Fisher method is applicable when one does not have a model of faults, which may occur when dealing with third-party data, such as the Global Navigation Satellite System (GNSS) data of transportation system users. These statistical tests can be combined with a particle filter to obtain a Monte Carlo state estimation scheme that is robust to faulty or outlier data. We present a synthetic freeway-traffic state estimation problem where the filters are able to reject simulated faulty GNSS measurements. The fault-model-free Fisher filter underperforms the Neyman\textendash Pearson filter when the latter has an accurate fault model but outperforms it when the assumed fault model is incorrect.},
 author = {Wright, Matthew A. and Horowitz, Roberto},
 doi = {10.1109/MITS.2020.2994098},
 file = {/home/matt/Zotero/storage/G5FD4LWI/Wright and Horowitz - 2020 - A Framework for Robust Assimilation of Potentially.pdf},
 issn = {1939-1390, 1941-1197},
 journal = {IEEE Intelligent Transportation Systems Magazine},
 language = {en},
 pages = {XX3-XX3},
 title = {A {{Framework}} for {{Robust Assimilation}} of {{Potentially Malign Third}}-{{Party Data}}, and Its {{Statistical Meaning}}},
 year = {2020}
}

@article{wright_fusing_2016-1,
 abstract = {In an age of ever-increasing penetration of Global Positioning System-enabled mobile devices, the potential of real-time ``probe'' location information for estimating the state of transportation networks is receiving increasing attention. Much work has been done on using probe data to estimate the current speed of vehicle traffic (or, equivalently, trip travel time). While travel times are useful to individual drivers, the state variable for a large class of traffic models and control algorithms is vehicle density. Our goal is to use probe data to supplement traditional fixed-location loop detector data for density estimation. To this end, we derive a method based on Rao-Blackwellized particle filters, a sequential Monte Carlo scheme. We present a simulation where we obtain a 30\% reduction in density mean absolute percentage error from fusing loop and probe data versus using loop data alone. We also present results using real data from a 19-mi freeway section in Los Angeles, CA, where we obtain a 31\% reduction. In addition, our method's estimate when using only the real-world probe data and no loop data outperformed the estimate produced when only loop data were used (i.e., an 18\% reduction). These results demonstrate that probe data can be used for traffic density estimation.},
 author = {Wright, Matthew and Horowitz, Roberto},
 doi = {10.1109/TITS.2016.2565438},
 file = {/home/matt/Zotero/storage/6SN5PS2P/Wright and Horowitz - 2016 - Fusing Loop and GPS Probe Measurements to Estimate.pdf;/home/matt/Zotero/storage/UV3H43G8/7480389.html},
 issn = {1558-0016},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {12},
 pages = {3577--3590},
 title = {Fusing {{Loop}} and {{GPS Probe Measurements}} to {{Estimate Freeway Density}}},
 volume = {17},
 year = {2016}
}

@article{wright_generic_2017,
 author = {Wright, Matthew A. and Horowitz, Roberto},
 journal = {ArXiv preprint},
 title = {Generic Second-Order Macroscopic Traffic Node Model for General Multi-Input Multi-Output Road Junctions via a Dynamic System Approach},
 url = {https://arxiv.org/abs/1707.09346},
 volume = {abs/1707.09346},
 year = {2017}
}

@article{wright_macro-scale_2019,
 author = {Wright, Matthew A. and Horowitz, Roberto},
 journal = {In preparation},
 title = {Macro-{{Scale Lane}}-{{Changing}} and {{Overtaking Behaviors}} at {{Road Junctions}}: {{Continuous}}-{{Time}} and {{Optimization}}-{{Problem Formulations}}},
 year = {2019}
}

@article{wright_macroscopic_2019,
 author = {Wright, Matthew A. and Horowitz, Roberto and Kurzhanskiy, Alex A.},
 journal = {to be submitted to Transportation Research Part B: Methodological},
 title = {Macroscopic {{Modeling}}, {{Calibration}}, and {{Simulation}} of {{Managed Lane}}-{{Freeway Networks}}, {{Part I}}: {{Topological}} and {{Phenomenological Modeling}}},
 year = {2019}
}

@article{wright_macroscopic_2019_pt2,
 author = {Wright, Matthew A. and Horowitz, Roberto and Kurzhanskiy, Alex A.},
 journal = {to be submitted to Transportation Research Part B: Methodological},
 keywords = {⛔ No DOI found},
 title = {Macroscopic {{Modeling}}, {{Calibration}}, and {{Simulation}} of {{Managed Lane}}-{{Freeway Networks}}, {{Part II}}: {{Network}}-Scale {{Calibration Methods}} and {{Case Studies}}},
 year = {2019}
}

@inproceedings{wright_neural-attention-based_2019,
 abstract = {Deep neural networks can be powerful tools, but require careful application-specific design to ensure that the most informative relationships in the data are learnable. In this paper, we apply deep neural networks to the nonlinear spatiotemporal physics problem of vehicle traffic dynamics. We consider problems of estimating macroscopic quantities (e.g., the queue at an intersection) at a lane level. First-principles modeling at the lane scale has been a challenge due to complexities in modeling social behaviors like lane changes, and those behaviors' resultant macro-scale effects. Following domain knowledge that upstream/downstream lanes and neighboring lanes affect each others' traffic flows in distinct ways, we apply a form of neural attention that allows the neural network layers to aggregate information from different lanes in different manners. Using a microscopic traffic simulator as a testbed, we obtain results showing that an attentional neural network model can use information from nearby lanes to improve predictions, and, that explicitly encoding the lane-to-lane relationship types significantly improves performance. We also demonstrate the transfer of our learned neural network to a more complex road network, discuss how its performance degradation may be attributable to new traffic behaviors induced by increased topological complexity, and motivate learning dynamics models from many road network topologies.},
 author = {Wright, Matthew A. and Ehlers, Simon F. G. and Horowitz, Roberto},
 booktitle = {2019 {{IEEE Intelligent Transportation Systems Conference}} ({{ITSC}})},
 doi = {10.1109/ITSC.2019.8917174},
 file = {/home/matt/Zotero/storage/NB4A23KL/Wright et al. - 2019 - Neural-Attention-Based Deep Learning Architectures.pdf;/home/matt/Zotero/storage/ZI3EC245/8917174.html},
 issn = {null},
 pages = {3898--3905},
 title = {Neural-{{Attention}}-{{Based Deep Learning Architectures}} for {{Modeling Traffic Dynamics}} on {{Lane Graphs}}},
 year = {2019}
}

@inproceedings{wright_neural-attentional_2019,
 address = {{Long Beach, CA}},
 annotation = {In submission},
 author = {Wright, Matthew A. and Horowitz, Roberto},
 booktitle = {International {{Conference}} on {{Machine Learning}}, {{Workshop}} on {{RL}} for {{Real Life}}},
 title = {Neural-{{Attentional Architectures}} for {{Deep Multi}}-{{Agent Reinforcement Learning}} in {{Varying Environments}}},
 year = {2019}
}

@article{wright_node_2017,
 abstract = {Macroscopic traffic models are necessary for simulation and study of traffic's complex macro-scale dynamics, and are often used by practitioners for road network planning, integrated corridor management, and other applications. These models have two parts: a link model, which describes traffic flow behavior on individual roads, and a node model, which describes behavior at road junctions. As the road networks under study become larger and more complex \textemdash{} nowadays often including arterial networks \textemdash{} the node model becomes more important. Despite their great importance to macroscopic models, however, only recently have node models had similar levels of attention as link models in the literature. This paper focuses on the first order node model and has two main contributions. First, we formalize the multi-commodity flow distribution at a junction as an optimization problem with all the necessary constraints. Most interesting here is the formalization of input flow priorities. Then, we discuss a very common ``conservation of turning fractions'' or ``first-infirst-out'' (FIFO) constraint, and how it often produces unrealistic spillback. This spillback occurs when, at a diverge, a queue develops for a movement that only a few lanes service, but FIFO requires that all lanes experience spillback from this queue. As we show, avoiding this unrealistic spillback while retaining FIFO in the node model requires complicated network topologies. Our second contribution is a ``partial FIFO'' mechanism that avoids this unrealistic spillback, and a (first-order) node model and solution algorithm that incorporates this mechanism. The partial FIFO mechanism is parameterized through intervals that describe how individual movements influence each other, can be intuitively described from physical lane geometry and turning movement rules, and allows tuning to describe a link as having anything between full FIFO and no FIFO. Excepting the FIFO constraint, the present node model also fits within the well-established ``general class of first-order node models'' for multi-commodity flows. Several illustrative examples are presented.},
 author = {Wright, Matthew A. and Gomes, Gabriel and Horowitz, Roberto and Kurzhanskiy, Alex A.},
 doi = {10.1016/j.trb.2017.09.001},
 file = {/home/matt/Zotero/storage/PXGTKYMC/Wright et al. - 2017 - On node models for high-dimensional road networks.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {212--234},
 title = {On Node Models for High-Dimensional Road Networks},
 volume = {105},
 year = {2017}
}

@inproceedings{wright_particle-filter-enabled_2017,
 abstract = {We are experiencing an explosion in the amount of sensors measuring our activities and the world around us. These sensors are spread throughout the built environment and can help us perform state estimation and control of related systems, but they are often built and/or maintained by third parties or system users. As a result, by outsourcing system measurement to third parties, the controller must accept their measurements without being able to directly verify the sensors' correct operation. Instead, detection and rejection of measurements from faulty sensors must be done with the raw data only. Towards this goal, we present a method of detecting possibly faulty behavior of sensors. The method does not require that the control designer have any model of faulty sensor behavior. As we discuss, it turns out that the widely-used particle filter state estimation algorithm provides the ingredients necessary for a hypothesis test against all ranges of correct operating behavior, obviating the need for a fault model to compare measurements. We demonstrate the applicability of our method by showing its ability to reject faulty measurements and accuracy in state estimation of a nonlinear vehicle traffic model, without information of generated faulty measurements' characteristics. In our test, we correctly identify nearly 90\% of measurements as faulty or non-faulty without having any fault model. This leads to only a 3\% increase in state estimation error over a theoretical 100\%-accurate fault detector.},
 author = {Wright, M. A. and Horowitz, R.},
 booktitle = {2017 {{IEEE}} 56th {{Annual Conference}} on {{Decision}} and {{Control}} ({{CDC}})},
 doi = {10.1109/CDC.2017.8264529},
 file = {/home/matt/Zotero/storage/UKQCXUZR/Wright and Horowitz - 2017 - Particle-filter-enabled real-time sensor fault det.pdf;/home/matt/Zotero/storage/P8XMGQUD/8264529.html},
 pages = {5757--5763},
 title = {Particle-Filter-Enabled Real-Time Sensor Fault Detection without a Model of Faults},
 year = {2017}
}

@article{wright_road_nodate,
 author = {Wright, Matthew A. and Ehlers, Simon and Horowitz, Roberto},
 title = {Road {{Network State Estimation}} via {{Geometric Deep Learning}}, {{Neural Attention}}, and {{PDE Dynamics}}},
 year = {In preparation}
}

@article{wu_-flight_2020,
 author = {Wu, Xiangyu and Mueller, Mark W.},
 journal = {ArXiv preprint},
 title = {In-Flight Range Optimization of Multicopters Using Multivariable Extremum Seeking with Adaptive Step Size},
 url = {https://arxiv.org/abs/2003.02907},
 volume = {abs/2003.02907},
 year = {2020}
}

@inproceedings{wu_ace_2019,
 author = {Zuxuan Wu and
Xin Wang and
Joseph Gonzalez and
Tom Goldstein and
Larry Davis},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/Wu0GG019.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00221},
 pages = {2121--2130},
 publisher = {{IEEE}},
 timestamp = {Thu, 30 Apr 2020 01:00:00 +0200},
 title = {{ACE:} Adapting to Changing Environments for Semantic Segmentation},
 url = {https://doi.org/10.1109/ICCV.2019.00221},
 year = {2019}
}

@techreport{wu_analysis_2005,
 abstract = {Many emerging applications formulate nonpositive semidefinite similarity matrices, and hence cannot fit into the framework of kernel machines. A popular approach to this problem is to transform the spectrum of the similarity matrix so as to generate a positive semidefinite kernel matrix. In this paper, we present an analytical framework to explore four representative transformation methods: denoise, flip, diffusion, and shift. Theoretically, we interpret each transformation and analyze its influence on classification using kernel machines. Moreover, when situations arise where the test data are not available during transformation, we propose an efficient algorithm to address the problem of updating the cross-similarity matrix between test and training data. Extensive experiments have been conducted to evaluate the performance of these methods on several realworld (dis)similarity matrices with semantic meanings.},
 author = {Wu, Gang and Chang, Edward Y and Zhang, Zhihua},
 file = {/home/matt/Zotero/storage/8JDLUMUW/Wu et al. - An Analysis of Transformation on Non-Positive Semi.pdf},
 institution = {{University of California, Santa Barbara}},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {9},
 title = {An {{Analysis}} of {{Transformation}} on {{Non}}-{{Positive Semidefinite Similarity Matrix}} for {{Kernel Machines}}},
 year = {2005}
}

@techreport{wu_asymmetric_2010,
 abstract = {This paper addresses a new kernel learning problem, referred to as `asymmetric kernel learning' (AKL). First, we give the definition of asymmetric kernel and point out that many `similarity functions' in real applications can be viewed as asymmetric kernels, for example, VSM, BM25, and LMIR in search. Then, we formalize AKL as an optimization problem whose objective function is a regularized loss function on supervised training data. Next, we propose an approach to AKL, which conducts AKL by using kernel methods. In the approach, the space of asymmetric kernels is assumed to be a reproducing kernel Hilbert space (RKHS), and thus existing kernel methods can be employed to learn the optimal asymmetric kernel. We also show that such an RKHS (i.e., space of asymmetric kernels) exists and refer to the kernel generating the RKHS as `hyper asymmetric kernel' (HAK). We present examples of HAK as well as theoretical basis for constructing HAKs. The proposed approach is applied to search to learn a relevance model from click-through data. Experimental results on web search and enterprise search data show that the model, named `Robust BM25' can work better than BM25 because it can effectively deal with the term mismatch problem which plagues BM25.},
 author = {Wu, Wei and Xu, Jun and Li, Hang and Oyama, Satoshi},
 file = {/home/matt/Zotero/storage/6EWKFBWD/Wu et al. - Asymmetric Kernel Learning.pdf},
 institution = {{Microsoft Research}},
 keywords = {⛔ No DOI found},
 language = {en},
 pages = {23},
 title = {Asymmetric {{Kernel Learning}}},
 year = {2010}
}

@article{wu_block_2019,
 abstract = {This paper presents the problem of block simplex constrained signal recovery, which has been demonstrated to be a suitable formulation for estimation problems in networks such as route flow estimation in traffic. There are several natural approaches to this problem: compressed sensing, Bayesian inference, and convex optimization. This paper presents new methods within each framework and assesses their respective abilities to reconstruct signals, with the particular emphasis on sparse recovery, ability to incorporate prior information, and scalability. We then apply these methods to route flow estimation in traffic networks of various sizes and network topologies. We find that both compressed sensing and Bayesian inference approaches are appropriate for structured recovery but have scalability limitations. The convex optimization approach does not directly incorporate prior information, but scales well and has been shown to achieve 90\% route flow accuracy on a full-scale network of over 10,000 links and 280,000 routes on a synthetic benchmark based on the I-210 corridor near Los Angeles, CA, USA.},
 author = {Wu, C. and Pozdnukhov, A. and Bayen, A. M.},
 doi = {10.1109/TITS.2019.2914174},
 file = {/home/matt/Zotero/storage/8CBBRWHB/Wu et al_2019_Block Simplex Signal Recovery.pdf;/home/matt/Zotero/storage/GMX2G9IG/8710616.html},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 pages = {1--13},
 shorttitle = {Block {{Simplex Signal Recovery}}},
 title = {Block {{Simplex Signal Recovery}}: {{Methods}}, {{Trade}}-{{Offs}}, and an {{Application}} to {{Routing}}},
 year = {2019}
}

@article{wu_flow_2017,
 author = {Wu, Cathy and Kreidieh, Aboudy and Parvate, Kanaad and Vinitsky, Eugene and Bayen, Alexandre M.},
 journal = {ArXiv preprint},
 title = {Flow: {{Architecture}} and {{Benchmarking}} for {{Reinforcement Learning}} in {{Traffic Control}}},
 url = {https://arxiv.org/abs/1710.05465},
 volume = {abs/1710.05465},
 year = {2017}
}

@article{wu_identification_2010,
 author = {Wu, X. and Liu, H. X. and Gettman, D.},
 journal = {Transportation Research, Part C},
 pages = {626--638},
 title = {Identification of Oversaturated Intersections Using High-Resolution Traffic Signal Data},
 volume = {18},
 year = {2010}
}

@phdthesis{wu_learning_2018,
 abstract = {Mixed autonomy characterizes problems surrounding the gradual and complex integration of automation and AI into existing systems. In the context of mobility, we consider: how will the gradual introduction of self-driving cars change urban mobility? In this dissertation, we develop machine learning and optimization techniques to address three key challenges: 1) quantifying the behavior of such complex systems, 2) addressing inherent sensing limitations, and 3) mitigating negative effects of introducing the automation.We demonstrate that deep reinforcement learning (RL) can serve as a unifying framework for studying the behavior of disparate and complex scenarios common in mixed autonomy systems. In particular, using deep RL, we find that automating a small fraction of vehicles in various traffic scenarios can result in a significant system-level velocity increase and numerous emergent driving behaviors. We demonstrate through the development of variance reduction techniques for policy gradient methods, that deep RL has the potential to scale to high-dimensional control systems, such as traffic networks and other mixed autonomy systems. We additionally present Flow, an open source RL platform with the goal of easing the design and study of disparate traffic scenarios. To address sensing limitations inherent when only parts of a system are automated, sensor fusion is explored. In particular, we introduce a convex optimization method for cellular network measurements from AT\&amp;T at the scale of the Greater Los Angeles Area, to address a flow estimation problem previously believed to be intractable. Finally, when automation reduces the cost of the activity (of transport), anticipated negative effects include induced demand and increased energy consumption. We study how the design of the mobility system itself can mitigate these effects. In particular, joint work with Microsoft Research provides insight into how high-occupancy vehicle lanes can simultaneously satisfy comfort and time preferences of users, and provide system benefits. We introduce combinatorial optimization methods based on clustering and local search for the resulting ridesharing problem. Together, these learning and optimization methods demonstrate that a small number of vehicles and sensors can be harnessed for significant impact on urban mobility, and shed light into the future study of mixed autonomy systems.},
 author = {Wu, Cathy},
 file = {/home/matt/Zotero/storage/B29VS7S9/Wu - 2018 - Learning and Optimization for Mixed Autonomy Syste.pdf;/home/matt/Zotero/storage/ANPNE4FG/3d93t6xq.html},
 language = {en},
 school = {UC Berkeley},
 title = {Learning and {{Optimization}} for {{Mixed Autonomy Systems}} - {{A Mobility Context}}},
 year = {2018}
}

@article{wu_learning_2020,
 author = {Wu, Yilin and Yan, Wilson and Kurutach, Thanard and Pinto, Lerrel and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {Learning to {{Manipulate Deformable Objects}} without {{Demonstrations}}},
 url = {https://arxiv.org/abs/1910.13439},
 volume = {abs/1910.13439},
 year = {2019}
}

@inproceedings{wu_pay_2019,
 author = {Felix Wu and
Angela Fan and
Alexei Baevski and
Yann N. Dauphin and
Michael Auli},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/WuFBDA19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Pay Less Attention with Lightweight and Dynamic Convolutions},
 url = {https://openreview.net/forum?id=SkVhlh09tX},
 year = {2019}
}

@article{wu_regularization_2013,
 abstract = {Learning with indefinite kernels attracted considerable attention in recent years due to their success in various learning scenarios. In this paper we study the asymptotic properties of the regularization kernel networks where the kernels are assumed to be indefinite, without the usual restrictions of symmetry and positive semi-definiteness as in the traditional study of kernel methods. The kernels are characterized in terms of the singular value decomposition of the corresponding kernel integrals. Two reproducing kernel Hilbert spaces are induced to characterize the approximation ability. Capacity independent error bounds are proved. Fast convergence rates are obtained both in reproducing kernel Hilbert spaces and in L2 sense.},
 author = {Wu, Qiang},
 doi = {10.1016/j.jat.2012.10.001},
 file = {/home/matt/Zotero/storage/BEGGLRV7/Wu - 2013 - Regularization networks with indefinite kernels.pdf;/home/matt/Zotero/storage/ZBK283C6/S0021904512001736.html},
 issn = {0021-9045},
 journal = {Journal of Approximation Theory},
 language = {en},
 pages = {1--18},
 title = {Regularization Networks with Indefinite Kernels},
 volume = {166},
 year = {2013}
}

@article{wu_self-supervised_2021,
 author = {Wu, Jiancan and Wang, Xiang and Feng, Fuli and He, Xiangnan and Chen, Liang and Lian, Jianxun and Xie, Xing},
 journal = {ArXiv preprint},
 title = {Self-Supervised {{Graph Learning}} for {{Recommendation}}},
 url = {https://arxiv.org/abs/2010.10783},
 volume = {abs/2010.10783},
 year = {2020}
}

@article{wu_squeezesegv2_2018,
 author = {Wu, Bichen and Zhou, Xuanyu and Zhao, Sicheng and Yue, Xiangyu and Keutzer, Kurt},
 journal = {ArXiv preprint},
 title = {{{SqueezeSegV2}}: {{Improved Model Structure}} and {{Unsupervised Domain Adaptation}} for {{Road}}-{{Object Segmentation}} from a {{LiDAR Point Cloud}}},
 url = {https://arxiv.org/abs/1809.08495},
 volume = {abs/1809.08495},
 year = {2018}
}

@inproceedings{xhonneux_continuous_2020,
 author = {Louis{-}Pascal A. C. Xhonneux and
Meng Qu and
Jian Tang},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/XhonneuxQT20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {10432--10441},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {Continuous Graph Neural Networks},
 url = {http://proceedings.mlr.press/v119/xhonneux20a.html},
 volume = {119},
 year = {2020}
}

@article{xia_periphery-fovea_2019,
 author = {Xia, Ye and Kim, Jinkyu and Canny, John and Zipser, Karl and Whitney, David},
 journal = {ArXiv preprint},
 title = {Periphery-{{Fovea Multi}}-{{Resolution Driving Model}} Guided by {{Human Attention}}},
 url = {https://arxiv.org/abs/1903.09950},
 volume = {abs/1903.09950},
 year = {2019}
}

@inproceedings{xia_periphery-fovea_2020,
 address = {{Aspen, CO}},
 author = {Xia, Ye and Kim, Jinkyu and Canny, John and Zipser, Karl and {Canas-Bajo}, Teresa and Whitney, David},
 booktitle = {The {{IEEE}} Winter Conference on Applications of Computer Vision ({{WACV}})},
 file = {/home/matt/Zotero/storage/FDJNWV9Q/Xia et al. - Periphery-Fovea Multi-Resolution Driving Model Gui.pdf},
 pages = {1767--1775},
 title = {Periphery-Fovea Multi-Resolution Driving Model Guided by Human Attention},
 year = {2020}
}

@article{xie_schedule-driven_2012,
 author = {Xie, X.-F. and Smith, S. F. and Lu, L. and Barlow, G. J.},
 journal = {Transportation Research, Part C},
 pages = {168--189},
 title = {Schedule-Driven Intersection Control},
 year = {2012}
}

@article{xie_unified_2014,
 author = {Xie, Xiao-Feng and Feng, Yiheng and Smith, Stephen and Head, K.},
 doi = {10.3141/2466-12},
 file = {/home/matt/Zotero/storage/E7CPGIZ4/TRB14RCTC.pdf},
 issn = {0361-1981},
 journal = {Transportation Research Record: Journal of the Transportation Research Board},
 language = {en},
 pages = {105--113},
 shorttitle = {Unified {{Route Choice Framework}}},
 title = {Unified {{Route Choice Framework}}: {{Specification}} and {{Application}} to {{Urban Traffic Control}}},
 volume = {2466},
 year = {2014}
}

@inproceedings{xin_accelerated_2019,
 author = {Xin, Long and Li, Shengbo Eben and Wang, Pin and Wang, Yulin and Nie, Bingbing and Chan, Ching-Yao and Cheng, Bo},
 booktitle = {{{IEEE}} Intelligent {{Transportation Systems Conference Proceedings}}},
 file = {/home/matt/Zotero/storage/XCHMSRS7/Xin et al. - 2019 - Accelerated Inverse Reinforcement Learning with Ra.pdf},
 title = {Accelerated {{Inverse Reinforcement Learning}} with {{Randomly Pre}}-Sampled {{Policies}} for {{Autonomous Driving Reward Design}}},
 year = {2019}
}

@inproceedings{xin_accelerated_2019-1,
 abstract = {To learn a reward function that a driver adheres to is of importance to the human-like design of autonomous driving systems. Inverse reinforcement learning (IRL) is one of the recent advances that can achieve this objective, but it often suffers from the low efficiency of generating optimal policy by reinforcement learning (RL) each time when updating reward weights. This paper presents an accelerated IRL method by approaching the optimal policy among randomly pre-sampled policies in designed sub-space instead of finding it through RL in the whole policy space. The corresponding trajectories are targeted via an optimal trajectory selector in the candidate trajectory library generated by pre-sampled policies. The weights then are updated by comparing the selected trajectories and the expert ones. The proposed method is very suitable for improving learning efficiency for low-dimensional problems like autonomous driving, whose expert policies are nearly tractable. Results with simulated driving data show that it only took 11 iterations to converge, while the average longitudinal RMS error of the recovered trajectories based on the learned reward function was only 2.14m.},
 address = {{Auckland, New Zealand}},
 author = {Xin, Long and Li, Shengbo Eben and Wang, Pin and Cao, Wenhan and Nie, Bingbing and Chan, Ching-Yao and Cheng, Bo},
 booktitle = {2019 {{IEEE Intelligent Transportation Systems Conference}} ({{ITSC}})},
 doi = {10.1109/ITSC.2019.8916952},
 file = {/home/matt/Zotero/storage/I97MS2W2/Xin et al. - 2019 - Accelerated Inverse Reinforcement Learning with Ra.pdf},
 isbn = {978-1-5386-7024-8},
 language = {en},
 pages = {2757--2764},
 publisher = {{IEEE}},
 title = {Accelerated {{Inverse Reinforcement Learning}} with {{Randomly Pre}}-Sampled {{Policies}} for {{Autonomous Driving Reward Design}}},
 year = {2019}
}

@article{xu_autoscale_2019,
 author = {Xu, Chenfeng and Liang, Dingkang and Xu, Yongchao and Bai, Song and Zhan, Wei and Tomizuka, Masayoshi and Bai, Xiang},
 journal = {ArXiv preprint},
 title = {{{AutoScale}}: {{Learning}} to {{Scale}} for {{Crowd Counting}}},
 url = {https://arxiv.org/abs/1912.09632},
 volume = {abs/1912.09632},
 year = {2019}
}

@inproceedings{xu_how_2019,
 author = {Keyulu Xu and
Weihua Hu and
Jure Leskovec and
Stefanie Jegelka},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/XuHLJ19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {How Powerful are Graph Neural Networks?},
 url = {https://openreview.net/forum?id=ryGs6iA5Km},
 year = {2019}
}

@inproceedings{xu_how_2021,
 author = {Keyulu Xu and
Mozhi Zhang and
Jingling Li and
Simon Shaolei Du and
Ken{-}ichi Kawarabayashi and
Stefanie Jegelka},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/XuZLDKJ21.bib},
 booktitle = {9th International Conference on Learning Representations, {ICLR} 2021,
Virtual Event, Austria, May 3-7, 2021},
 publisher = {OpenReview.net},
 timestamp = {Wed, 23 Jun 2021 01:00:00 +0200},
 title = {How Neural Networks Extrapolate: From Feedforward to Graph Neural
Networks},
 url = {https://openreview.net/forum?id=UH-cmocLJC},
 year = {2021}
}

@article{xu_minimal_2019,
 author = {Xu, Jingyi and Danielczuk, Michael and Ichnowski, Jeff and Mahler, Jeffrey and Steinbach, Eckehard and Goldberg, Ken},
 journal = {ArXiv preprint},
 title = {Minimal {{Work}}: {{A Grasp Quality Metric}} for {{Deformable Hollow Objects}}},
 url = {https://arxiv.org/abs/1909.11226},
 volume = {abs/1909.11226},
 year = {2019}
}

@inproceedings{xu_motion_2014,
 abstract = {We present a motion planning framework for autonomous on-road driving considering both the uncertainty caused by an autonomous vehicle and other traffic participants. The future motion of traffic participants is predicted using a local planner, and the uncertainty along the predicted trajectory is computed based on Gaussian propagation. For the autonomous vehicle, the uncertainty from localization and control is estimated based on a Linear-Quadratic Gaussian (LQG) framework. Compared with other safety assessment methods, our framework allows the planner to avoid unsafe situations more efficiently, thanks to the direct uncertainty information feedback to the planner. We also demonstrate our planner's ability to generate safer trajectories compared to planning only with a LQG framework.},
 author = {Xu, Wenda and Pan, Jia and Wei, Junqing and Dolan, John M.},
 booktitle = {2014 {{IEEE International Conference}} on {{Robotics}} and {{Automation}} ({{ICRA}})},
 doi = {10.1109/ICRA.2014.6907209},
 file = {/home/matt/Zotero/storage/GQUW739E/Xu et al. - 2014 - Motion planning under uncertainty for on-road auto.pdf;/home/matt/Zotero/storage/TR4WH5FA/6907209.html},
 issn = {1050-4729},
 pages = {2507--2512},
 title = {Motion Planning under Uncertainty for On-Road Autonomous Driving},
 year = {2014}
}

@inproceedings{xu_pointfusion_2018,
 author = {Danfei Xu and
Dragomir Anguelov and
Ashesh Jain},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/XuAJ18.bib},
 booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
 doi = {10.1109/CVPR.2018.00033},
 pages = {244--253},
 publisher = {{IEEE} Computer Society},
 timestamp = {Wed, 06 Feb 2019 00:00:00 +0100},
 title = {PointFusion: Deep Sensor Fusion for 3D Bounding Box Estimation},
 url = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Xu\_PointFusion\_Deep\_Sensor\_CVPR\_2018\_paper.html},
 year = {2018}
}

@inproceedings{xu_representation_2018,
 author = {Keyulu Xu and
Chengtao Li and
Yonglong Tian and
Tomohiro Sonobe and
Ken{-}ichi Kawarabayashi and
Stefanie Jegelka},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/XuLTSKJ18.bib},
 booktitle = {Proceedings of the 35th International Conference on Machine Learning,
{ICML} 2018, Stockholmsm{\"{a}}ssan, Stockholm, Sweden, July 10-15,
2018},
 editor = {Jennifer G. Dy and
Andreas Krause},
 pages = {5449--5458},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Wed, 03 Apr 2019 01:00:00 +0200},
 title = {Representation Learning on Graphs with Jumping Knowledge Networks},
 url = {http://proceedings.mlr.press/v80/xu18c.html},
 volume = {80},
 year = {2018}
}

@inproceedings{xu_show_2015,
 author = {Kelvin Xu and
Jimmy Ba and
Ryan Kiros and
Kyunghyun Cho and
Aaron C. Courville and
Ruslan Salakhutdinov and
Richard S. Zemel and
Yoshua Bengio},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/XuBKCCSZB15.bib},
 booktitle = {Proceedings of the 32nd International Conference on Machine Learning,
{ICML} 2015, Lille, France, 6-11 July 2015},
 editor = {Francis R. Bach and
David M. Blei},
 pages = {2048--2057},
 publisher = {JMLR.org},
 series = {{JMLR} Workshop and Conference Proceedings},
 timestamp = {Wed, 29 May 2019 01:00:00 +0200},
 title = {Show, Attend and Tell: Neural Image Caption Generation with Visual
Attention},
 url = {http://proceedings.mlr.press/v37/xuc15.html},
 volume = {37},
 year = {2015}
}

@inproceedings{xu_toward_2019,
 abstract = {Neural network autonomous driving policies are widely explored. However, no matter using imitation learning or reinforcement learning, the network policies are generally hard to train, and the learned knowledge encoded in neural network policies are hard to transfer. We propose to modularize the complicated driving policies in terms of the driving attributes, and present the parallel attribute networks (PAN), which can learn to fullfill the requirements of the attributes in the driving tasks separately, and later assemble their knowledge together. Concretely, we first train a policy network that accomplish the base lane tracking attribute. The modules for the add-on attributes such as avoiding obstacles and obeying traffic rules are then trained to map the corresponding state to a satisfactory set of the vehicle action space. Finally the reference action given by the base policy is projected into the satisfactory sets so as to satisfy the requirements of all the attributes. Using the PAN, many complicated tasks that are hard to train from scratch can be easily trained; also unseen driving tasks can be solved in a zero-shot manner by assembling the pretrained attribute modules. We have validated the capability of our model on a class of autonomous driving problems with attributes of obstacle avoidance, traffic light and speed limit in simulation. Experimental results based on an obstacle avoidance task are also presented.},
 author = {Xu, Z. and Chang, H. and Tang, C. and Liu, C. and Tomizuka, M.},
 booktitle = {2019 {{IEEE Intelligent Vehicles Symposium}} ({{IV}})},
 doi = {10.1109/IVS.2019.8813861},
 file = {/home/matt/Zotero/storage/WJ42BGWP/Xu et al_2019_Toward Modularization of Neural Network Autonomous Driving Policy Using.pdf;/home/matt/Zotero/storage/A39QESX3/8813861.html},
 pages = {1400--1407},
 title = {Toward {{Modularization}} of {{Neural Network Autonomous Driving Policy Using Parallel Attribute Networks}}},
 year = {2019}
}

@inproceedings{xu_what_2020,
 author = {Keyulu Xu and
Jingling Li and
Mozhi Zhang and
Simon S. Du and
Ken{-}ichi Kawarabayashi and
Stefanie Jegelka},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/XuLZDKJ20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {What Can Neural Networks Reason About?},
 url = {https://openreview.net/forum?id=rJxbJeHFPS},
 year = {2020}
}

@article{xue_primal_2019,
 abstract = {Kernel methods have been widely applied in machine learning to solve complex nonlinear problems. Kernel selection is one of the key issues in kernel methods, since it is vital for improving generalization performance. Traditionally, the selection of kernel is restricted to be positive definite which makes their applicability partially limited. Actually, in many real applications such as gene identification and object recognition, indefinite kernels frequently emerge and can achieve better performance. However, compared to positive definite ones, indefinite kernels are more complicated due to the non-convexity of the subsequent optimization problems, which leads to the incapability of most existing kernel algorithms. Some indefinite kernel methods have been proposed based on the dual of support vector machine (SVM), which mostly emphasize on how to transform the non-convex optimization to be convex by using positive definite kernels to approximate indefinite ones. In fact, the duality gap in SVM usually exists in the case of indefinite kernels and therefore these algorithms do not indeed solve the indefinite kernel problems themselves. In this paper, we present a novel framework for indefinite kernel learning derived directly from the primal of SVM, which establishes several new models not only for single indefinite kernel but also extends to multiple indefinite kernel scenarios. Several algorithms are developed to handle the non-convex optimization problems in these models. We further provide a constructive approach for kernel selection in the algorithms by using the theory of similarity functions. Experiments on real world datasets demonstrate the superiority of our models.},
 author = {Xue, Hui and Wang, Lin and Chen, Songcan and Wang, Yunyun},
 doi = {10.1007/s11063-019-10019-7},
 file = {/home/matt/Zotero/storage/P9G859QM/Xue et al. - 2019 - A Primal Framework for Indefinite Kernel Learning.pdf},
 issn = {1573-773X},
 journal = {Neural Processing Letters},
 language = {en},
 number = {1},
 pages = {165--188},
 title = {A {{Primal Framework}} for {{Indefinite Kernel Learning}}},
 volume = {50},
 year = {2019}
}

@inproceedings{y._gao_spatial_2012,
 author = {Y. Gao, A. Gray, J. V. Frasch, T. Lin, E. Tseng, J. K. Hedrick, F. Borrelli},
 booktitle = {Proceedings of the 2012 {{International Symposium}} on {{Advanced Vehicle Control}}},
 title = {Spatial {{Predictive Control}} for {{Agile Semi}}-{{Autonomous Ground Vehicles}}},
 year = {2012}
}

@article{yan_learning_2020,
 author = {Yan, Wilson and Vangipuram, Ashwin and Abbeel, Pieter and Pinto, Lerrel},
 journal = {ArXiv preprint},
 title = {Learning {{Predictive Representations}} for {{Deformable Objects Using Contrastive Estimation}}},
 url = {https://arxiv.org/abs/2003.05436},
 volume = {abs/2003.05436},
 year = {2020}
}

@article{yang_cellular_2015,
 abstract = {To better understand the characteristics of car\textendash truck heterogeneous traffic flow that is very common on freeway, a cellular automata-based traffic flow model is proposed for single lane traffic in this paper. The proposed model discriminates the four types of car\textendash truck following combination, car-following-car (CC), car-following-truck (CT), truck-following-car (TC) and truck-following-truck (TT). The four combinations are considered in terms of the safety distance, reaction time and randomization probability. The parameter values in the proposed model are derived from NGSIM data. Simulations are conducted based on the new model and some new conclusions about the characteristics of the car\textendash truck traffic flow are drawn. First, in the density range of (23\textendash 36) vehs/km, the fundamental diagram mainly depends on the car\textendash truck following combination, especially, on the proportion of CC combination. In this range, the fundamental diagram curves with the same proportion of CC gather into a cluster, and the flow rate increases with the increment of the proportion of CC for the same traffic density. Second, traffic congestion can be effectively reduced up to 6.3\% by increasing the proportion of TC or CT combination. This finding provides a possible way to alleviate traffic congestion on freeway. Third, reducing randomization probability of the four combinations can effectively increase traffic capacity and alleviate traffic congestion.},
 author = {Yang, Da and Qiu, Xiaoping and Yu, Dan and Sun, Ruoxiao and Pu, Yun},
 doi = {10.1016/j.physa.2014.12.020},
 file = {/home/matt/Zotero/storage/CTFPC5DE/Yang et al. - 2015 - A cellular automata model for car–truck heterogene.pdf;/home/matt/Zotero/storage/R3Z4IR8C/S0378437114010553.html},
 issn = {0378-4371},
 journal = {Physica A: Statistical Mechanics and its Applications},
 pages = {62--72},
 title = {A Cellular Automata Model for Car\textendash Truck Heterogeneous Traffic Flow Considering the Car\textendash Truck Following Combination Effect},
 volume = {424},
 year = {2015}
}

@article{yang_deep_2019,
 abstract = {Cardinality estimation has long been grounded in statistical tools for density estimation. To capture the rich multivariate distributions of relational tables, we propose the use of a new type of high-capacity statistical model: deep autoregressive models. However, direct application of these models leads to a limited estimator that is prohibitively expensive to evaluate for range or wildcard predicates. To produce a truly usable estimator, we develop a Monte Carlo integration scheme on top of autoregressive models that can efficiently handle range queries with dozens of dimensions or more.},
 author = {Yang, Zongheng and Liang, Eric and Kamsetty, Amog and Wu, Chenggang and Duan, Yan and Chen, Xi and Abbeel, Pieter and Hellerstein, Joseph M and Krishnan, Sanjay and Stoica, Ion},
 doi = {10.14778/3368289.3368294},
 file = {/home/matt/Zotero/storage/QNPWHMUE/Yang et al. - Deep Unsupervised Cardinality Estimation.pdf},
 journal = {Proceedings of the VLDB Endowment},
 keywords = {⛔ No DOI found},
 language = {en},
 number = {3},
 pages = {279--292},
 title = {Deep {{Unsupervised Cardinality Estimation}}},
 volume = {13},
 year = {2019}
}

@article{yang_morphology-agnostic_2020,
 abstract = {Existing approaches for visuomotor robotic control typically require characterizing the robot in advance by calibrating the camera or performing system identification. We propose MAVRIC, an approach that works with minimal prior knowledge of the robot's morphology, and requires only a camera view containing the robot and its environment and an unknown control interface. MAVRIC revolves around a mutual information-based method for self-recognition, which discovers visual ``control points'' on the robot body within a few seconds of exploratory interaction, and these control points in turn are then used for visual servoing. MAVRIC can control robots with imprecise actuation, no proprioceptive feedback, unknown morphologies including novel tools, unknown camera poses, and even unsteady handheld cameras. We demonstrate our method on visually-guided 3D point reaching, trajectory following, and robot-to-robot imitation.},
 author = {Yang, Brian and Jayaraman, Dinesh and Berseth, Glen and Efros, Alexei and Levine, Sergey},
 doi = {10.1109/LRA.2019.2963824},
 file = {/home/matt/Zotero/storage/7NSADC3D/Yang et al. - 2020 - Morphology-Agnostic Visual Robotic Control.pdf},
 issn = {2377-3766, 2377-3774},
 journal = {IEEE Robotics and Automation Letters},
 language = {en},
 number = {2},
 pages = {766--773},
 title = {Morphology-{{Agnostic Visual Robotic Control}}},
 volume = {5},
 year = {2020}
}

@article{yang_multivariable_2016,
 abstract = {This paper presents the multivariable extension of the feedback particle filter (FPF) algorithm for the nonlinear filtering problem in continuous-time. The FPF is a control-oriented approach to particle filtering. The approach does not require importance sampling or resampling and offers significant variance improvements; in particular, the algorithm can be applied to systems that are not stable. This paper describes new representations and algorithms for the FPF in the general multivariable nonlinear non-Gaussian setting. Theory surrounding the FPF is improved: Exactness of the FPF is established in the general setting, as well as well-posedness of the associated boundary value problem to obtain the filter gain. A Galerkin finite-element algorithm is proposed for approximation of the gain. Its performance is illustrated in numerical experiments.},
 author = {Yang, Tao and Laugesen, Richard S. and Mehta, Prashant G. and Meyn, Sean P.},
 doi = {10.1016/j.automatica.2016.04.019},
 file = {/home/matt/Zotero/storage/5PZ72HG7/Yang et al. - 2016 - Multivariable feedback particle filter.pdf;/home/matt/Zotero/storage/2UYRP9IV/S000510981630142X.html},
 issn = {0005-1098},
 journal = {Automatica},
 pages = {10--23},
 title = {Multivariable Feedback Particle Filter},
 volume = {71},
 year = {2016}
}

@article{yang_replab_2019,
 author = {Yang, Brian and Zhang, Jesse and Pong, Vitchyr and Levine, Sergey and Jayaraman, Dinesh},
 journal = {ArXiv preprint},
 title = {{{REPLAB}}: {{A Reproducible Low}}-{{Cost Arm Benchmark Platform}} for {{Robotic Learning}}},
 url = {https://arxiv.org/abs/1905.07447},
 volume = {abs/1905.07447},
 year = {2019}
}

@article{yang_selectivity_2019,
 author = {Yang, Zongheng and Liang, Eric and Kamsetty, Amog and Wu, Chenggang and Duan, Yan and Chen, Xi and Abbeel, Pieter and Hellerstein, Joseph M. and Krishnan, Sanjay and Stoica, Ion},
 journal = {ArXiv preprint},
 title = {Selectivity {{Estimation}} with {{Deep Likelihood Models}}},
 url = {https://arxiv.org/abs/1905.04278},
 volume = {abs/1905.04278},
 year = {2019}
}

@article{yang_tppo_2020,
 author = {Yang, Biao and Yan, Guocheng and Wang, Pin and Chan, Ching-yao and Liu, Xiaofeng and Chen, Yang},
 journal = {ArXiv preprint},
 title = {{{TPPO}}: {{A Novel Trajectory Predictor}} with {{Pseudo Oracle}}},
 url = {https://arxiv.org/abs/2002.01852},
 volume = {abs/2002.01852},
 year = {2020}
}

@inproceedings{yang_xlnet_2019,
 author = {Zhilin Yang and
Zihang Dai and
Yiming Yang and
Jaime G. Carbonell and
Ruslan Salakhutdinov and
Quoc V. Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/YangDYCSL19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {5754--5764},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {XLNet: Generalized Autoregressive Pretraining for Language Understanding},
 url = {https://proceedings.neurips.cc/paper/2019/hash/dc6a7e655d7e5840e66733e9ee67cc69-Abstract.html},
 year = {2019}
}

@article{yao_pyhessian_2020,
 author = {Yao, Zhewei and Gholami, Amir and Keutzer, Kurt and Mahoney, Michael},
 journal = {ArXiv preprint},
 title = {{{PyHessian}}: {{Neural Networks Through}} the {{Lens}} of the {{Hessian}}},
 url = {https://arxiv.org/abs/1912.07145},
 volume = {abs/1912.07145},
 year = {2019}
}

@inproceedings{yao_revisiting_2018,
 author = {Huaxiu Yao and
Xianfeng Tang and
Hua Wei and
Guanjie Zheng and
Zhenhui Li},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/YaoTWZL19.bib},
 booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
2019, The Thirty-First Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
USA, January 27 - February 1, 2019},
 doi = {10.1609/aaai.v33i01.33015668},
 pages = {5668--5675},
 publisher = {{AAAI} Press},
 timestamp = {Tue, 02 Feb 2021 00:00:00 +0100},
 title = {Revisiting Spatial-Temporal Similarity: {A} Deep Learning Framework
for Traffic Prediction},
 url = {https://doi.org/10.1609/aaai.v33i01.33015668},
 year = {2019}
}

@article{ye_automated_2020,
 author = {Ye, Fei and Cheng, Xuxin and Wang, Pin and Chan, Ching-Yao},
 journal = {ArXiv preprint},
 title = {Automated {{Lane Change Strategy}} Using {{Proximal Policy Optimization}}-Based {{Deep Reinforcement Learning}}},
 url = {https://arxiv.org/abs/2002.02667},
 volume = {abs/2002.02667},
 year = {2020}
}

@article{ye_sketch-driven_2020,
 author = {Ye, Xi  and
Chen, Qiaochu  and
Wang, Xinyu  and
Dillig, Isil  and
Durrett, Greg},
 doi = {10.1162/tacl_a_00339},
 journal = {Transactions of the Association for Computational Linguistics},
 pages = {679--694},
 title = {Sketch-Driven Regular Expression Generation from Natural Language and Examples},
 url = {https://aclanthology.org/2020.tacl-1.44},
 volume = {8},
 year = {2020}
}

@article{yen_finding_1971,
 author = {Yen, Jin Y.},
 journal = {Management Science},
 number = {11},
 pages = {712--716},
 title = {Finding the \textbackslash em {{K Shortest Loopless Paths}} in a {{Neetwork}}},
 volume = {17},
 year = {1971}
}

@article{yerra_emergence_2005,
 abstract = {A transportation network is a complex system that exhibits the properties of self-organization and emergence. Previous research in dynamics related to transportation networks focuses on traffic assignment or traffic management. This research concentrates on the dynamics of the orientation of major roads in a network and abstractly models these dynamics to understand the basic properties of transportation networks. A model is developed to capture the dynamics that leads to a hierarchical arrangement of roads for a given network structure and land use distribution. Localized investment rules, wherein revenue produced by traffic on a link is invested for that link's own development, are employed. Under reasonable parameters, these investment rules, coupled with traveler behavior, and underlying network topology result in the emergence of a hierarchical pattern. Hypothetical networks subject to certain conditions are tested with this model to explore their network properties. Though hierarchies seem to be designed by planners and engineers, the results show that they are intrinsic properties of networks. Also, the results show that roads, specific routes with continuous attributes, are emergent properties of transportation networks.},
 author = {Yerra, Bhanu M. and Levinson, David M.},
 doi = {10.1007/s00168-005-0230-4},
 issn = {1432-0592},
 journal = {The Annals of Regional Science},
 language = {en},
 number = {3},
 pages = {541--553},
 title = {The Emergence of Hierarchy in Transportation Networks},
 volume = {39},
 year = {2005}
}

@book{yi_development_2010,
 annotation = {Published: University of Akron},
 author = {Yi, P. and Shao, C. and Mao, J.},
 title = {Development and Testing of an Automatic Turn Movements Identification System},
 year = {2010}
}

@article{yin__2017,
 author = {Yin, Penghang and Sun, Zhe and Jin, Wen-Long and Xin, Jack},
 doi = {10.1016/j.trb.2017.08.006},
 file = {/home/matt/Zotero/storage/NUDTSXMY/l1_minimization_for_link_flow_correction.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {398--408},
 title = {{$\mathscr{l}$} 1 -Minimization Method for Link Flow Correction},
 volume = {104},
 year = {2017}
}

@inproceedings{Yin_2019_CVPR,
 author = {Zhichao Yin and
Trevor Darrell and
Fisher Yu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/YinDY19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00620},
 pages = {6044--6053},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Hierarchical Discrete Distribution Decomposition for Match Density
Estimation},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Yin\_Hierarchical\_Discrete\_Distribution\_Decomposition\_for\_Match\_Density\_Estimation\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{yin_hierarchical_nodate,
 author = {Zhichao Yin and
Trevor Darrell and
Fisher Yu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/YinDY19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00620},
 pages = {6044--6053},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Hierarchical Discrete Distribution Decomposition for Match Density
Estimation},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Yin\_Hierarchical\_Discrete\_Distribution\_Decomposition\_for\_Match\_Density\_Estimation\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{yin_meta-learning_2020,
 author = {Mingzhang Yin and
George Tucker and
Mingyuan Zhou and
Sergey Levine and
Chelsea Finn},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/YinTZLF20.bib},
 booktitle = {8th International Conference on Learning Representations, {ICLR} 2020,
Addis Ababa, Ethiopia, April 26-30, 2020},
 publisher = {OpenReview.net},
 timestamp = {Thu, 07 May 2020 01:00:00 +0200},
 title = {Meta-Learning without Memorization},
 url = {https://openreview.net/forum?id=BklEFpEYwS},
 year = {2020}
}

@inproceedings{ying_hierarchical_2018,
 author = {Zhitao Ying and
Jiaxuan You and
Christopher Morris and
Xiang Ren and
William L. Hamilton and
Jure Leskovec},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/YingY0RHL18.bib},
 booktitle = {Advances in Neural Information Processing Systems 31: Annual Conference
on Neural Information Processing Systems 2018, NeurIPS 2018, December
3-8, 2018, Montr{\'{e}}al, Canada},
 editor = {Samy Bengio and
Hanna M. Wallach and
Hugo Larochelle and
Kristen Grauman and
Nicol{\`{o}} Cesa{-}Bianchi and
Roman Garnett},
 pages = {4805--4815},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Hierarchical Graph Representation Learning with Differentiable Pooling},
 url = {https://proceedings.neurips.cc/paper/2018/hash/e77dbaf6759253c7c6d0efc5690369c7-Abstract.html},
 year = {2018}
}

@book{yoon_surface_2007,
 author = {Yoon, J. and Noble, B. and Liu, M.},
 title = {Surface {{Street Traffic Estimation}}},
 year = {2007}
}

@inproceedings{you_design_2020,
 author = {Jiaxuan You and
Zhitao Ying and
Jure Leskovec},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/YouYL20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Design Space for Graph Neural Networks},
 url = {https://proceedings.neurips.cc/paper/2020/hash/c5c3d4fe6b2cc463c7d7ecba17cc9de7-Abstract.html},
 year = {2020}
}

@inproceedings{you_graph_2020,
 author = {Yuning You and
Tianlong Chen and
Yongduo Sui and
Ting Chen and
Zhangyang Wang and
Yang Shen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/YouCSCWS20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Graph Contrastive Learning with Augmentations},
 url = {https://proceedings.neurips.cc/paper/2020/hash/3fe230348e9a12c13120749e3f9fa4cd-Abstract.html},
 year = {2020}
}

@article{you_large-batch_2019,
 author = {You, Yang and Hseu, Jonathan and Ying, Chris and Demmel, James and Keutzer, Kurt and Hsieh, Cho-Jui},
 journal = {ArXiv preprint},
 title = {Large-{{Batch Training}} for {{LSTM}} and {{Beyond}}},
 url = {https://arxiv.org/abs/1901.08256},
 volume = {abs/1901.08256},
 year = {2019}
}

@inproceedings{you_large-batch_2019-1,
 abstract = {Large-batch training approaches have enabled researchers to utilize distributed processing and greatly accelerate deep neural networks training. However, there are three problems in current large-batch research: (1) Although RNN approaches like LSTM have been widely used in many applications, current large-batch research is principally focused on CNNs. (2) Even for CNNs, there is no automated technique for extending the batch size beyond 8K. (3) To keep the variance in the gradient expectation constant, theory suggests that a Sqrt Scaling scheme should be used in large-batch training. Unfortunately, there are not many successful applications. In this paper, we propose Dynamic Adaptive-Tuning Engine (DATE) for better large-batch training. DATE achieves a 5.3x average speedup over the baselines for four LSTM-based applications on the same hardware. We finish the ImageNet training with ResNet-50 in two minutes on 1024 v3 TPUs (76.7\% top-1 accuracy), which is the fastest version as of June of 2019.},
 address = {{Denver Colorado}},
 author = {You, Yang and Hseu, Jonathan and Ying, Chris and Demmel, James and Keutzer, Kurt and Hsieh, Cho-Jui},
 booktitle = {Proceedings of the {{International Conference}} for {{High Performance Computing}}, {{Networking}}, {{Storage}} and {{Analysis}}},
 doi = {10.1145/3295500.3356137},
 file = {/home/matt/Zotero/storage/3WZTVULM/You et al. - 2019 - Large-batch training for LSTM and beyond.pdf},
 isbn = {978-1-4503-6229-0},
 language = {en},
 pages = {1--16},
 publisher = {{ACM}},
 title = {Large-Batch Training for {{LSTM}} and Beyond},
 year = {2019}
}

@inproceedings{you_when_2020,
 author = {Yuning You and
Tianlong Chen and
Zhangyang Wang and
Yang Shen},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/icml/YouCWS20.bib},
 booktitle = {Proceedings of the 37th International Conference on Machine Learning,
{ICML} 2020, 13-18 July 2020, Virtual Event},
 pages = {10871--10880},
 publisher = {{PMLR}},
 series = {Proceedings of Machine Learning Research},
 timestamp = {Tue, 15 Dec 2020 00:00:00 +0100},
 title = {When Does Self-Supervision Help Graph Convolutional Networks?},
 url = {http://proceedings.mlr.press/v119/you20a.html},
 volume = {119},
 year = {2020}
}

@article{youse_local_2018,
 abstract = {We show a Talagrand-type concentration inequality for Multi-Task Learning (MTL), with which we establish sharp excess risk bounds for MTL in terms of the Local Rademacher Complexity (LRC). We also give a new bound on the LRC for any norm regularized hypothesis classes, which applies not only to MTL, but also to the standard Single-Task Learning (STL) setting. By combining both results, one can easily derive fast-rate bounds on the excess risk for many prominent MTL methods, including\textemdash as we demonstrate\textemdash Schatten norm, group norm, and graph regularized MTL. The derived bounds reflect a relationship akin to a conservation law of asymptotic convergence rates. When compared to the rates obtained via a traditional, global Rademacher analysis, this very relationship allows for trading off slower rates with respect to the number of tasks for faster rates with respect to the number of available samples per task.},
 author = {Yousefi, Niloofar and Lei, Yunwen and Kloft, Marius and Mollaghasemi, Mansooreh and Anagnostopoulos, Georgios C},
 file = {/home/matt/Zotero/storage/SH7EJLVC/Youseﬁ et al. - Local Rademacher Complexity-based Learning Guarant.pdf},
 journal = {Journal of Machine Learning Research},
 keywords = {⛔ No DOI found},
 language = {en},
 number = {1},
 pages = {1385--1431},
 title = {Local {{Rademacher Complexity}}-Based {{Learning Guarantees}} for {{Multi}}-{{Task Learning}}},
 volume = {19},
 year = {2018}
}

@article{yousefpour_failout_2020,
 author = {Yousefpour, Ashkan and Nguyen, Brian Q. and Devic, Siddartha and Wang, Guanhua and Kreidieh, Aboudy and Lobel, Hans and Bayen, Alexandre M. and Jue, Jason P.},
 journal = {ArXiv preprint},
 title = {Failout: {{Achieving Failure}}-{{Resilient Inference}} in {{Distributed Neural Networks}}},
 url = {https://arxiv.org/abs/2002.07386},
 volume = {abs/2002.07386},
 year = {2020}
}

@article{yousefpour_guardians_2019,
 author = {Yousefpour, Ashkan and Devic, Siddartha and Nguyen, Brian Q. and Kreidieh, Aboudy and Liao, Alan and Bayen, Alexandre M. and Jue, Jason P.},
 journal = {ArXiv preprint},
 title = {Guardians of the {{Deep Fog}}: {{Failure}}-{{Resilient DNN Inference}} from {{Edge}} to {{Cloud}}},
 url = {https://arxiv.org/abs/1909.00995},
 volume = {abs/1909.00995},
 year = {2019}
}

@article{yousefpour_guardians_2019-1,
 abstract = {Partitioning and distributing deep neural networks (DNNs) over physical nodes such as edge, fog, or cloud nodes, could enhance sensor fusion, and reduce bandwidth and inference latency. However, when a DNN is distributed over physical nodes, failure of the physical nodes causes the failure of the DNN units that are placed on these nodes. The performance of the inference task will be unpredictable, and most likely, poor, if the distributed DNN is not specifically designed and properly trained for failures. Motivated by this, we introduce deepFogGuard, a DNN architecture augmentation scheme for making the distributed DNN inference task failure-resilient. To articulate deepFogGuard, we introduce the elements and a model for the resiliency of distributed DNN inference. Inspired by the concept of residual connections in DNNs, we introduce skip hyperconnections in distributed DNNs, which are the basis of deepFogGuard's design to provide resiliency. Next, our extensive experiments using two existing datasets for the sensing and vision applications confirm the ability of deepFogGuard to provide resiliency for distributed DNNs in edge-cloud networks.},
 archiveprefix = {arXiv},
 author = {Yousefpour, Ashkan and Devic, Siddartha and Nguyen, Brian Q. and Kreidieh, Aboudy and Liao, Alan and Bayen, Alexandre M. and Jue, Jason P.},
 doi = {10.1145/3363347.3363366},
 eprint = {1909.00995},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/JX5FCUBL/Yousefpour et al. - 2019 - Guardians of the Deep Fog Failure-Resilient DNN I.pdf},
 journal = {Proceedings of the First International Workshop on Challenges in Artificial Intelligence and Machine Learning for Internet of Things  - AIChallengeIoT'19},
 language = {en},
 pages = {25--31},
 shorttitle = {Guardians of the {{Deep Fog}}},
 title = {Guardians of the {{Deep Fog}}: {{Failure}}-{{Resilient DNN Inference}} from {{Edge}} to {{Cloud}}},
 year = {2019}
}

@inproceedings{yperman_link_2005,
 address = {{Poznan, Poland}},
 author = {Yperman, Isaak and Logghe, Steven and Immers, Ben},
 booktitle = {Proceedings of the 10th {{EWGT Meeting}}, {{Poznan}}, {{Poland}}},
 file = {/home/matt/Zotero/storage/PIN8P8QX/The_link_transmission_model_An_efficient_implement.pdf},
 keywords = {⛔ No DOI found},
 pages = {122--127},
 shorttitle = {The Link Transmission Model},
 title = {The Link Transmission Model: {{An}} Efficient Implementation of the Kinematic Wave Theory in Traffic Networks},
 year = {2005}
}

@inproceedings{yu_c2fnas_2020,
 author = {Qihang Yu and
Dong Yang and
Holger Roth and
Yutong Bai and
Yixiao Zhang and
Alan L. Yuille and
Daguang Xu},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/YuYRBZYX20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.00418},
 pages = {4125--4134},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {{C2FNAS:} Coarse-to-Fine Neural Architecture Search for 3D Medical
Image Segmentation},
 url = {https://doi.org/10.1109/CVPR42600.2020.00418},
 year = {2020}
}

@inproceedings{yu_deep_2017,
 author = {Fisher Yu and
Dequan Wang and
Evan Shelhamer and
Trevor Darrell},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/YuWSD18.bib},
 booktitle = {2018 {IEEE} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2018, Salt Lake City, UT, USA, June 18-22, 2018},
 doi = {10.1109/CVPR.2018.00255},
 pages = {2403--2412},
 publisher = {{IEEE} Computer Society},
 timestamp = {Wed, 06 Feb 2019 00:00:00 +0100},
 title = {Deep Layer Aggregation},
 url = {http://openaccess.thecvf.com/content\_cvpr\_2018/html/Yu\_Deep\_Layer\_Aggregation\_CVPR\_2018\_paper.html},
 year = {2018}
}

@article{yu_forecasting_2020-1,
 author = {Yu, Byeonghyeop and Lee, Yongjin and Sohn, Keemin},
 doi = {10.1016/j.trc.2020.02.013},
 file = {/home/matt/Zotero/storage/HJYUKGKA/Yu et al. - 2020 - Forecasting road traffic speeds by considering are.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {189--204},
 title = {Forecasting Road Traffic Speeds by Considering Area-Wide Spatio-Temporal Dependencies Based on a Graph Convolutional Neural Network ({{GCN}})},
 volume = {114},
 year = {2020}
}

@inproceedings{yu_gradient_2020,
 author = {Tianhe Yu and
Saurabh Kumar and
Abhishek Gupta and
Sergey Levine and
Karol Hausman and
Chelsea Finn},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/YuK0LHF20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Gradient Surgery for Multi-Task Learning},
 url = {https://proceedings.neurips.cc/paper/2020/hash/3fe78a8acf5fda99de95303940a2420c-Abstract.html},
 year = {2020}
}

@inproceedings{yu_meta-world_2019,
 abstract = {Meta-reinforcement learning algorithms can enable robots to acquire new skills much more quickly, by leveraging prior experience to learn how to learn. However, much of the current research on meta-reinforcement learning focuses on task distributions that are very narrow. For example, a commonly used meta-reinforcement learning benchmark uses different running velocities for a simulated robot as different tasks. When policies are meta-trained on such narrow task distributions, they cannot possibly generalize to more quickly acquire entirely new tasks. Therefore, if the aim of these methods is to enable faster acquisition of entirely new behaviors, we must evaluate them on task distributions that are sufficiently broad to enable generalization to new behaviors. In this paper, we propose an open-source simulated benchmark for meta-reinforcement learning and multi-task learning consisting of 50 distinct robotic manipulation tasks. Our aim is to make it possible to develop algorithms that generalize to accelerate the acquisition of entirely new, held-out tasks. We evaluate 6 state-of-the-art metareinforcement learning and multi-task learning algorithms on these tasks. Surprisingly, while each task and its variations (e.g., with different object positions) can be learned with reasonable success, these algorithms struggle to learn with multiple tasks at the same time, even with as few as ten distinct training tasks. Our analysis and open-source environments pave the way for future research in multi-task learning and meta-learning that can enable meaningful generalization, thereby unlocking the full potential of these methods.1.},
 archiveprefix = {arXiv},
 author = {Yu, Tianhe and Quillen, Deirdre and He, Zhanpeng and Julian, Ryan and Hausman, Karol and Finn, Chelsea and Levine, Sergey},
 booktitle = {3rd {{Conference}} on {{Robot Learning}} ({{CoRL}} 2019)},
 eprint = {1910.10897},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/S48G6UUX/Yu et al. - 2019 - Meta-World A Benchmark and Evaluation for Multi-T.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 shorttitle = {Meta-{{World}}},
 title = {Meta-{{World}}: {{A Benchmark}} and {{Evaluation}} for {{Multi}}-{{Task}} and {{Meta Reinforcement Learning}}},
 year = {2019}
}

@article{yu_motivation_2017,
 abstract = {The `One Belt, One Road' (OBOR) initiatives form the centerpiece of the Chinese leadership's new foreign policy. The OBOR initiatives are a reflection of China's ascendance in the global arena, economically, politically, and strategically. Developing inter-connectivity of infrastructure development forms a central part of China's OBOR initiatives. The Asian Infrastructure Investment Bank (AIIB) aims to facilitate and accelerate infrastructure improvement in the region by providing capital loans and technical services. The AIIB will serve as the spearhead of China's OBOR initiatives. The AIIB and OBOR initiatives have put China at the center of geoeconomics and geopolitics in the region and beyond, a position from which it hopes to strengthen its economic ties with other Asian countries. The new Silk Road initiatives also provide a channel for Chinese companies and capital to invest in other countries by leveraging China's strengths in infrastructure development, financial power and manufacturing capacity. The OBOR initiatives and the AIIB could change the economic and political landscape of Asia, the most dynamic and economically vibrant region of the twenty-first century. However, China faces serious challenges, both internally and externally, in implementing these initiatives.},
 author = {Yu, Hong},
 doi = {10.1080/10670564.2016.1245894},
 file = {/home/matt/Zotero/storage/5385WZ66/Yu - 2017 - Motivation behind China’s ‘One Belt, One Road’ Ini.pdf},
 issn = {1067-0564},
 journal = {Journal of Contemporary China},
 number = {105},
 pages = {353--368},
 title = {Motivation behind {{China}}'s `{{One Belt}}, {{One Road}}' {{Initiatives}} and {{Establishment}} of the {{Asian Infrastructure Investment Bank}}},
 volume = {26},
 year = {2017}
}

@inproceedings{yu_multi-scale_2016,
 author = {Fisher Yu and
Vladlen Koltun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/journals/corr/YuK15.bib},
 booktitle = {4th International Conference on Learning Representations, {ICLR} 2016,
San Juan, Puerto Rico, May 2-4, 2016, Conference Track Proceedings},
 editor = {Yoshua Bengio and
Yann LeCun},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Multi-Scale Context Aggregation by Dilated Convolutions},
 url = {http://arxiv.org/abs/1511.07122},
 year = {2016}
}

@inproceedings{yu_one-shot_2019,
 abstract = {We consider the problem of learning multi-stage vision-based tasks on a real robot from a single video of a human performing the task, while leveraging demonstration data of subtasks with other objects. This problem presents a number of major challenges. Video demonstrations without teleoperation are easy for humans to provide, but do not provide any direct supervision. Learning policies from raw pixels enables full generality but calls for large function approximators with many parameters to be learned. Finally, compound tasks can require impractical amounts of demonstration data, when treated as a monolithic skill. To address these challenges, we propose a method that learns both how to learn primitive behaviors from video demonstrations and how to dynamically compose these behaviors to perform multi-stage tasks by ``watching'' a human demonstrator. Our results on a simulated Sawyer robot and real PR2 robot illustrate our method for learning a variety of order fulfillment and kitchen serving tasks with novel objects and raw pixel inputs. Video results are linked at https://sites.google.com/view/one-shot-hil.},
 address = {{Macau, China}},
 author = {Yu, Tianhe and Abbeel, Pieter and Levine, Sergey and Finn, Chelsea},
 booktitle = {2019 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}} ({{IROS}})},
 doi = {10.1109/IROS40897.2019.8967745},
 file = {/home/matt/Zotero/storage/HPUU2VNT/Yu et al. - 2019 - One-Shot Composition of Vision-Based Skills from D.pdf},
 isbn = {978-1-72814-004-9},
 language = {en},
 pages = {2643--2650},
 publisher = {{IEEE}},
 title = {One-{{Shot Composition}} of {{Vision}}-{{Based Skills}} from {{Demonstration}}},
 year = {2019}
}

@inproceedings{yu_qanet_2018,
 author = {Adams Wei Yu and
David Dohan and
Minh{-}Thang Luong and
Rui Zhao and
Kai Chen and
Mohammad Norouzi and
Quoc V. Le},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/YuDLZ00L18.bib},
 booktitle = {6th International Conference on Learning Representations, {ICLR} 2018,
Vancouver, BC, Canada, April 30 - May 3, 2018, Conference Track Proceedings},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {QANet: Combining Local Convolution with Global Self-Attention for
Reading Comprehension},
 url = {https://openreview.net/forum?id=B14TlG-RW},
 year = {2018}
}

@article{yu_reinforcement_2019,
 author = {Yu, Huan and Park, Saehong and Moura, Scott and Bayen, Alexandre and Krstic, Miroslav},
 journal = {ArXiv preprint},
 title = {Reinforcement {{Learning}} vs. {{Backstepping Control}} of {{Stop}}-and-{{Go Traffic}}},
 url = {https://arxiv.org/abs/1904.12957},
 volume = {abs/1904.12957},
 year = {2019}
}

@article{yu_salvaging_2020,
 author = {Yu, Tao and Bagdasaryan, Eugene and Shmatikov, Vitaly},
 journal = {ArXiv preprint},
 title = {Salvaging {{Federated Learning}} by {{Local Adaptation}}},
 url = {https://arxiv.org/abs/2002.04758},
 volume = {abs/2002.04758},
 year = {2020}
}

@article{yuan_real-time_2012,
 author = {Yuan, Yufei and {\noopsort{lint}}{van Lint}, J. W. C. and Wilson, R. Eddie and {\noopsort{wageningen-kessels}}{van Wageningen-Kessels}, Femke and Hoogendoorn, Serge P.},
 doi = {10.1109/TITS.2011.2178837},
 file = {/home/matt/Zotero/storage/MRCGMTQI/YuanEtAl_LagrangianEstimator.pdf},
 issn = {1524-9050, 1558-0016},
 journal = {IEEE Transactions on Intelligent Transportation Systems},
 number = {1},
 pages = {59--70},
 title = {Real-{{Time Lagrangian Traffic State Estimator}} for {{Freeways}}},
 volume = {13},
 year = {2012}
}

@inproceedings{yue_domain_2019,
 author = {Xiangyu Yue and
Yang Zhang and
Sicheng Zhao and
Alberto L. Sangiovanni{-}Vincentelli and
Kurt Keutzer and
Boqing Gong},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/YueZZSKG19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00219},
 pages = {2100--2110},
 publisher = {{IEEE}},
 timestamp = {Fri, 06 Mar 2020 00:00:00 +0100},
 title = {Domain Randomization and Pyramid Consistency: Simulation-to-Real Generalization
Without Accessing Target Domain Data},
 url = {https://doi.org/10.1109/ICCV.2019.00219},
 year = {2019}
}

@inproceedings{yun_graph_2020,
 author = {Seongjun Yun and
Minbyul Jeong and
Raehyun Kim and
Jaewoo Kang and
Hyunwoo J. Kim},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/YunJKKK19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {11960--11970},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Graph Transformer Networks},
 url = {https://proceedings.neurips.cc/paper/2019/hash/9d63484abb477c97640154d40595a3bb-Abstract.html},
 year = {2019}
}

@article{zaharia_apache_2016,
 author = {Zaharia, Matei and Xin, Reynold S. and Wendell, Patrick and Das, Tathagata and Armbrust, Michael and Dave, Ankur and Meng, Xiangrui and Rosen, Josh and Venkataraman, Shivaram and Franklin, Michael J. and Ghodsi, Ali and Gonzalez, Joseph and Shenker, Scott and Stoica, Ion},
 doi = {10.1145/2934664},
 file = {/home/matt/Zotero/storage/D7EFAPR5/Zaharia et al. - 2016 - Apache Spark a unified engine for big data proces.pdf},
 issn = {0001-0782, 1557-7317},
 journal = {Communications of the ACM},
 language = {en},
 number = {11},
 pages = {56--65},
 shorttitle = {Apache {{Spark}}},
 title = {Apache {{Spark}}: A Unified Engine for Big Data Processing},
 volume = {59},
 year = {2016}
}

@article{zanella_internet_2014,
 abstract = {The Internet of Things (IoT) shall be able to incorporate transparently and seamlessly a large number of different and heterogeneous end systems, while providing open access to selected subsets of data for the development of a plethora of digital services. Building a general architecture for the IoT is hence a very complex task, mainly because of the extremely large variety of devices, link layer technologies, and services that may be involved in such a system. In this paper, we focus specifically to an urban IoT system that, while still being quite a broad category, are characterized by their specific application domain. Urban IoTs, in fact, are designed to support the Smart City vision, which aims at exploiting the most advanced communication technologies to support added-value services for the administration of the city and for the citizens. This paper hence provides a comprehensive survey of the enabling technologies, protocols, and architecture for an urban IoT. Furthermore, the paper will present and discuss the technical solutions and best-practice guidelines adopted in the Padova Smart City project, a proof-of-concept deployment of an IoT island in the city of Padova, Italy, performed in collaboration with the city municipality.},
 author = {Zanella, A. and Bui, N. and Castellani, A. and Vangelista, L. and Zorzi, M.},
 doi = {10.1109/JIOT.2014.2306328},
 file = {/home/matt/Zotero/storage/XAHECDPX/Zanella et al. - 2014 - Internet of Things for Smart Cities.pdf;/home/matt/Zotero/storage/55HI34SS/6740844.html},
 issn = {2327-4662},
 journal = {IEEE Internet of Things Journal},
 number = {1},
 pages = {22--32},
 title = {Internet of {{Things}} for {{Smart Cities}}},
 volume = {1},
 year = {2014}
}

@phdthesis{zareei_transformation_2018,
 abstract = {The method of Transformation Optics, which is based on transformation solutions, was originally developed in optics community for creating passive invisibility cloaks. This method uses the subtle idea of coordinate transformation and form-invariance of Maxwell equations and offers an unprecedented way of steering optical waves through architecting the constitutive parameters (i.e. permittivity and permeability) of a dielectric.In this thesis, we present the method transformation media, inspired by transformation optics, as a general mathematical framework for an arbitrary steering of mechanical waves including surface gravity waves in fluids and also flexural waves in thin plates. Particularly, we prove that surface gravity wave equation in shallow water (long-wave limit) is form-invariant and therefore permits transformation solutions. We further formulate a general coordinate free equation that determines spatial variations required for water depth and gravitational acceleration as constitutive parameters for an arbitrary steering of long surface gravity waves. This general equation provides transformation media scheme for water waves. Additionally, since one of the constitutive parameters is gravitational acceleration and is actually a physical constant, we formulate a nonlinear transformation to keep the gravitational acceleration intact and with only sea-bed variations, we design and numerically validate a broadband invisibility cloak for surface gravity waves as the benchmark of transformation media method. In order to fully enable various applications of transformation media for surface gravity waves, a variable gravitational acceleration is required. We show that an altered effective gravitational acceleration is possible through a visco-elastic sea-bed, where the effective gravity depends on viscosity and elasticity of the bottom carpet. The visco-elastic sea bed itself provides a new mechanism to control oceanic wave energy through variations in the effective gravitational acceleration. Based on this idea, we present a theoretical design for an equivalent of graded-index optical fibers for water-waves which defies the spreading loss of water waves and can transmit wave energy over long distances in a broad range of frequencies and without a need for side-walls. Since the effect of sea-bed variation decreases exponentially as the water depth increases, a whole new approach is required for controlling waves in finite/deep water. We propose a flexural buoyant carpet, with an engineered rigidity and mass, floating on the free surface to affect and control waves. We further design a cloaking carpet for water waves in finite/deep water waves to prove the efficacy of the proposed method.In the case of flexural waves, the governing equation for elastic waves in thin plates is not form invariant, and hence transformation based solution does not apply to such waves. Applying a transformation to the flexural wave equation, most of the terms in the transformed equation do not match with the exact orthotropic and inhomogeneous flexural wave equation, and therefore the governing equation is not form-invariant. We show that by carefully designing the transformation and also assuming a pre-stressed material with body forces, all of the terms in the transformed equation match with the exact inhomogeneous and orthotropic equation, and a perfect broadband flexural cloak can be designed. For a readily achievable flexural cloak in a physical setting, we further present an approximate adoption of our perfect cloak under more restrictive physical constraints. Through direct simulation of the governing equations, we show that this cloak maintains a consistently high cloaking efficiency over a broad range of frequencies. The methodology developed here may be used for steering waves and designing cloaks in other physical systems with non form-invariant governing equations. Lastly, we show the relation between flexural rigidity in thin plates and the equivalent of refractive index for flexural waves. We design a flexural GRIN lens in a thin plate by smoothly varying the plate's rigidity, and thus its refractive index. We show that the proposed lens is broadband, has a fixed focal point over a wide range of frequencies, and is theoretically capable of zero-aberration focusing. We numerically explore our Continuous Profile GRIN lens (CP-GRIN lens) and further experimentally validate an implemented design.},
 author = {Zareei, Ahmad},
 file = {/home/matt/Zotero/storage/PQRSC3PZ/Zareei - 2018 - Transformation Based Wave Control.pdf;/home/matt/Zotero/storage/HW5552SJ/21d6c40m.html},
 language = {en},
 school = {UC Berkeley},
 title = {Transformation {{Based Wave Control}}},
 year = {2018}
}

@inproceedings{zellers_hellaswag_2019,
 address = {Florence, Italy},
 author = {Zellers, Rowan  and
Holtzman, Ari  and
Bisk, Yonatan  and
Farhadi, Ali  and
Choi, Yejin},
 booktitle = {Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/P19-1472},
 pages = {4791--4800},
 publisher = {Association for Computational Linguistics},
 title = {{H}ella{S}wag: Can a Machine Really Finish Your Sentence?},
 url = {https://aclanthology.org/P19-1472},
 year = {2019}
}

@article{zeng_differential_2020,
 abstract = {Generating agile maneuvers for a quadrotor with a cable-suspended load is a challenging problem. State-of-theart approaches often need significant computation time and complex parameter tuning. We use a coordinate-free geometric formulation and exploit a differential flatness based hybrid model of a quadrotor with a cable-suspended payload. We perform direct collocation on the differentially-flat hybrid system, and use complementarity constraints to avoid specifying hybrid mode sequences. The non-differentiable obstacle avoidance constraints are reformulated using dual variables, resulting in smooth constraints. We show that our approach has lower computational time than the state-of-the-art and guarantees feasibility of the trajectory with respect to both the system dynamics and input constraints without the need to tune lots of parameters. We validate our approach on a variety of tasks in both simulations and experiments, including navigation through waypoints and obstacle avoidance.},
 author = {Zeng, Jun and Kotaru, Prasanth and Mueller, Mark W. and Sreenath, Koushil},
 doi = {10.1109/LRA.2020.2972845},
 file = {/home/matt/Zotero/storage/SJP7A4UR/Zeng et al. - 2020 - Differential Flatness Based Path Planning With Dir.pdf},
 issn = {2377-3766, 2377-3774},
 journal = {IEEE Robotics and Automation Letters},
 language = {en},
 number = {2},
 pages = {3074--3081},
 title = {Differential {{Flatness Based Path Planning With Direct Collocation}} on {{Hybrid Modes}} for a {{Quadrotor With}} a {{Cable}}-{{Suspended Payload}}},
 volume = {5},
 year = {2020}
}

@inproceedings{zeng_end--end_2019,
 author = {Wenyuan Zeng and
Wenjie Luo and
Simon Suo and
Abbas Sadat and
Bin Yang and
Sergio Casas and
Raquel Urtasun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/ZengLSSYCU19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00886},
 pages = {8660--8669},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Wed, 25 Nov 2020 00:00:00 +0100},
 title = {End-To-End Interpretable Neural Motion Planner},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Zeng\_End-To-End\_Interpretable\_Neural\_Motion\_Planner\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{zha_collision-resilient_2020,
 author = {Zha, Jiaming and Wu, Xiangyu and Kroeger, Joseph and Perez, Natalia and Mueller, Mark W.},
 journal = {ArXiv preprint},
 title = {A Collision-Resilient Aerial Vehicle with Icosahedron Tensegrity Structure},
 url = {https://arxiv.org/abs/2003.03417},
 volume = {abs/2003.03417},
 year = {2020}
}

@article{zha_economic_2016,
 author = {Zha, Liteng and Yin, Yafeng and Yang, Hai},
 doi = {10.1016/j.trc.2016.07.010},
 file = {/home/matt/Documents/Papers/zha_yin_yang_2016_ridesourcing.pdf},
 issn = {0968090X},
 journal = {Transportation Research Part C: Emerging Technologies},
 language = {en},
 pages = {249--266},
 title = {Economic Analysis of Ride-Sourcing Markets},
 volume = {71},
 year = {2016}
}

@article{zhai_squeezewave_2020,
 author = {Zhai, Bohan and Gao, Tianren and Xue, Flora and Rothchild, Daniel and Wu, Bichen and Gonzalez, Joseph E. and Keutzer, Kurt},
 journal = {ArXiv preprint},
 title = {{{SqueezeWave}}: {{Extremely Lightweight Vocoders}} for {{On}}-Device {{Speech Synthesis}}},
 url = {https://arxiv.org/abs/2001.05685},
 volume = {abs/2001.05685},
 year = {2020}
}

@inproceedings{zhan_constructing_2019,
 abstract = {Research in the areas related to driving behavior, e.g., behavior modeling and prediction, requires datasets with highly interactive vehicle motions. Existing public vehicle motion datasets emphasize increasing the number of vehicles and time duration, but behavior-related researchers are suffering from two factors. First, strong interactions among vehicles are not well addressed and datasets are of relatively lowdensity to observe meaningful interactions. Second, most of the existing datasets are missing the map information with reference paths which is essential for driving-behavior-related research. To address this issue, a dataset with highly interactive vehicle motions is constructed in this paper. A variety of challenging driving scenarios such as unsignalized intersections and roundabouts are included. Reference paths are also constructed from motion data along with high-definition maps so that key features can be generated for both prediction and planning algorithms. Moreover, we propose a set of metrics to extract the interactive motions in different maps, including the minimum difference of time to collision point (MDTTC) and duration of waiting period. Such metrics are used to quantify the interaction density of the dataset. We also give several representative results on prediction and motion generation utilizing the constructed dataset to demonstrate how the dataset can facilitate research in the area of driving behavior.},
 address = {{Macau, China}},
 author = {Zhan, Wei and Sun, Liting and Wang, Di and Jin, Yinghan and Tomizuka, Masayoshi},
 booktitle = {2019 {{IEEE}}/{{RSJ International Conference}} on {{Intelligent Robots}} and {{Systems}} ({{IROS}})},
 doi = {10.1109/IROS40897.2019.8967724},
 file = {/home/matt/Zotero/storage/QCD8Q5I7/Zhan et al. - 2019 - Constructing a Highly Interactive Vehicle Motion D.pdf},
 isbn = {978-1-72814-004-9},
 language = {en},
 pages = {6415--6420},
 publisher = {{IEEE}},
 title = {Constructing a {{Highly Interactive Vehicle Motion Dataset}}},
 year = {2019}
}

@inproceedings{zhan_non-conservatively_2016,
 abstract = {From the driving strategy point of view, a major challenge for autonomous vehicles in urban environment is to behave defensively to potential dangers, yet to not overreact to threats with low probability. As it is overwhelming to program the action rules case-by-case, a unified planning framework under uncertainty is proposed in this paper, which achieves a non-conservatively defensive strategy (NCDS) in various kinds of scenarios for urban autonomous driving. First, uncertainties in urban scenarios are simplified to two probabilistic cases, namely passing and yielding. Two-way-stop intersection is used as an exemplar scenario to illustrate the derivation of probabilities for different intentions of others via a logistic regression model. Then a deterministic planner is designed as the baseline. Also, a safe set is defined, which considers both current and preview safety. The planning framework under uncertainty is then proposed, in which safety is guaranteed and overcautious behavior is prevented. Finally, the proposed planning framework is tested by simulation in the exemplar scenario, which demonstrates that an NCDS can be realistically achieved by employing the proposed framework.},
 author = {Zhan, Wei and Liu, Changliu and Chan, Ching-Yao and Tomizuka, Masayoshi},
 booktitle = {2016 {{IEEE}} 19th {{International Conference}} on {{Intelligent Transportation Systems}} ({{ITSC}})},
 doi = {10.1109/ITSC.2016.7795595},
 file = {/home/matt/Zotero/storage/AHWFE8V3/7795595.html},
 issn = {2153-0017},
 pages = {459--464},
 title = {A Non-Conservatively Defensive Strategy for Urban Autonomous Driving},
 year = {2016}
}

@inproceedings{Zhang_2019_CVPR,
 author = {Xuaner Zhang and
Qifeng Chen and
Ren Ng and
Vladlen Koltun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/ZhangCNK19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00388},
 pages = {3762--3770},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Zoom to Learn, Learn to Zoom},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Zhang\_Zoom\_to\_Learn\_Learn\_to\_Zoom\_CVPR\_2019\_paper.html},
 year = {2019}
}

@article{zhang_anodev2_2019,
 author = {Zhang, Tianjun and Yao, Zhewei and Gholami, Amir and Keutzer, Kurt and Gonzalez, Joseph and Biros, George and Mahoney, Michael},
 journal = {ArXiv preprint},
 title = {{{ANODEV2}}: {{A Coupled Neural ODE Evolution Framework}}},
 url = {https://arxiv.org/abs/1906.04596},
 volume = {abs/1906.04596},
 year = {2019}
}

@inproceedings{zhang_asynchronous_2019,
 abstract = {Significant progress has been made in the area of model-based reinforcement learning. State-of-the-art algorithms are now able to match the asymptotic performance of model-free methods while being significantly more data efficient. However, this success has come at a price: state-of-the-art model-based methods require significant computation interleaved with data collection, resulting in run times that take days, even if the amount of agent interaction might be just hours or even minutes. When considering the goal of learning in real-time on real robots, this means these state-of-the-art model-based algorithms still remain impractical. In this work, we propose an asynchronous framework for model-based reinforcement learning methods that brings down the run time of these algorithms to be just the data collection time. We evaluate our asynchronous framework on a range of standard MuJoCo benchmarks. We also evaluate our asynchronous framework on three real-world robotic manipulation tasks. We show how asynchronous learning not only speeds up learning w.r.t wall-clock time through parallelization, but also further reduces the sample complexity of model-based approaches by means of improving the exploration and by means of effectively avoiding the policy overfitting to the deficiencies of learned dynamics models.},
 archiveprefix = {arXiv},
 author = {Zhang, Yunzhi and Clavera, Ignasi and Tsai, Boren and Abbeel, Pieter},
 booktitle = {3rd {{Conference}} on {{Robot Learning}} ({{CoRL}} 2019)},
 eprint = {1910.12453},
 eprinttype = {arxiv},
 file = {/home/matt/Zotero/storage/A8KLRLU2/Zhang et al. - 2019 - Asynchronous Methods for Model-Based Reinforcement.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Asynchronous {{Methods}} for {{Model}}-{{Based Reinforcement Learning}}},
 year = {2019}
}

@inproceedings{zhang_fixup_2019,
 author = {Hongyi Zhang and
Yann N. Dauphin and
Tengyu Ma},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iclr/ZhangDM19.bib},
 booktitle = {7th International Conference on Learning Representations, {ICLR} 2019,
New Orleans, LA, USA, May 6-9, 2019},
 publisher = {OpenReview.net},
 timestamp = {Thu, 25 Jul 2019 01:00:00 +0200},
 title = {Fixup Initialization: Residual Learning Without Normalization},
 url = {https://openreview.net/forum?id=H1gsz30cKX},
 year = {2019}
}

@article{zhang_frames_2011,
 abstract = {Frames in a Banach space B were defined as a sequence in its dual space B⁎ in some recent references. We propose to define them as a collection of elements in B by making use of semi-inner products. Classical theory on frames and Riesz bases is generalized under this new perspective. We then aim at establishing the Shannon sampling theorem in Banach spaces. The existence of such expansions in translation invariant reproducing kernel Hilbert and Banach spaces is discussed.},
 author = {Zhang, Haizhang and Zhang, Jun},
 doi = {10.1016/j.acha.2010.09.007},
 file = {/home/matt/Zotero/storage/QKMFHA5H/Zhang and Zhang - 2011 - Frames, Riesz bases, and sampling expansions in Ba.pdf;/home/matt/Zotero/storage/SMUEA9RF/S1063520310001120.html},
 issn = {1063-5203},
 journal = {Applied and Computational Harmonic Analysis},
 language = {en},
 number = {1},
 pages = {1--25},
 title = {Frames, {{Riesz}} Bases, and Sampling Expansions in {{Banach}} Spaces via Semi-Inner Products},
 volume = {31},
 year = {2011}
}

@article{zhang_general_1996,
 author = {Zhang, M. and Ritchie, S. G. and Recker, W. W.},
 journal = {Transportation Research, Part C},
 number = {2},
 pages = {51--69},
 title = {Some General Results on the Optimal Ramp Control Problem},
 volume = {4},
 year = {1996}
}

@article{zhang_graph-bert_2020,
 author = {Zhang, Jiawei and Zhang, Haopeng and Xia, Congying and Sun, Li},
 journal = {ArXiv preprint},
 title = {Graph-{{Bert}}: {{Only Attention}} Is {{Needed}} for {{Learning Graph Representations}}},
 url = {https://arxiv.org/abs/2001.05140},
 volume = {abs/2001.05140},
 year = {2020}
}

@article{zhang_link-journey-speed_1999,
 author = {Zhang, H. M.},
 journal = {Transportation Research Record},
 number = {1676},
 pages = {109--115},
 title = {Link-Journey-Speed Model for Arterial Traffic},
 year = {1999}
}

@article{zhang_mathematical_1999,
 author = {Zhang, H.M.},
 doi = {10.1016/S0191-2615(98)00022-8},
 file = {/home/matt/Documents/Papers/HOV-HOT/HOVmodeling/zhang_1999_hysteresis.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {1},
 pages = {1--23},
 title = {A Mathematical Theory of Traffic Hysteresis},
 volume = {33},
 year = {1999}
}

@article{zhang_near-optimal_2019,
 author = {Zhang, Xiaojing and Bujarbaruah, Monimoy and Borrelli, Francesco},
 journal = {ArXiv preprint},
 title = {Near-{{Optimal Rapid MPC}} Using {{Neural Networks}}: {{A Primal}}-{{Dual Policy Learning Framework}}},
 url = {https://arxiv.org/abs/1912.04744},
 volume = {abs/1912.04744},
 year = {2019}
}

@article{zhang_non-equilibrium_2002,
 author = {Zhang, H.M.},
 doi = {10.1016/S0191-2615(00)00050-3},
 file = {/home/matt/Documents/Papers/zhang_nonequilibrium_traffic.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 number = {3},
 pages = {275--290},
 title = {A Non-Equilibrium Traffic Model Devoid of Gas-like Behavior},
 volume = {36},
 year = {2002}
}

@inproceedings{zhang_predicting_2019,
 author = {Jason Y. Zhang and
Panna Felsen and
Angjoo Kanazawa and
Jitendra Malik},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/iccv/ZhangFKM19.bib},
 booktitle = {2019 {IEEE/CVF} International Conference on Computer Vision, {ICCV}
2019, Seoul, Korea (South), October 27 - November 2, 2019},
 doi = {10.1109/ICCV.2019.00721},
 pages = {7113--7122},
 publisher = {{IEEE}},
 timestamp = {Wed, 10 Jun 2020 01:00:00 +0200},
 title = {Predicting 3D Human Dynamics From Video},
 url = {https://doi.org/10.1109/ICCV.2019.00721},
 year = {2019}
}

@article{zhang_regularized_2012,
 abstract = {We view regularized learning of a function in a Banach space from its finite samples as an optimization problem. Within the framework of reproducing kernel Banach spaces, we prove the representer theorem for the minimizer of regularized learning schemes with a general loss function and a nondecreasing regularizer. When the loss function and the regularizer are differentiable, a characterization equation for the minimizer is also established.},
 author = {Zhang, Haizhang and Zhang, Jun},
 doi = {10.1007/s10898-010-9575-z},
 file = {/home/matt/Zotero/storage/P6IMETKC/Zhang and Zhang - 2012 - Regularized learning in Banach spaces as an optimi.pdf},
 issn = {1573-2916},
 journal = {Journal of Global Optimization},
 language = {en},
 number = {2},
 pages = {235--250},
 shorttitle = {Regularized Learning in {{Banach}} Spaces as an Optimization Problem},
 title = {Regularized Learning in {{Banach}} Spaces as an Optimization Problem: Representer Theorems},
 volume = {54},
 year = {2012}
}

@article{zhang_reproducing_2009,
 abstract = {We introduce the notion of reproducing kernel Banach spaces (RKBS) and study special semiinner-product RKBS by making use of semi-inner-products and the duality mapping. Properties of an RKBS and its reproducing kernel are investigated. As applications, we develop in the framework of RKBS standard learning schemes including minimal norm interpolation, regularization network, support vector machines, and kernel principal component analysis. In particular, existence, uniqueness and representer theorems are established.},
 author = {Zhang, Haizhang and Xu, Yuesheng and Zhang, Jun},
 file = {/home/matt/Zotero/storage/W3BVEJY7/Zhang et al. - 2009 - Reproducing kernel Banach spaces for machine learn.pdf},
 journal = {Journal of Machine Learning Research},
 language = {en},
 pages = {2741--2775},
 title = {Reproducing Kernel {{Banach}} Spaces for Machine Learning},
 volume = {10},
 year = {2009}
}

@article{zhang_safe_2019,
 author = {Zhang, Xiaojing and Bujarbaruah, Monimoy and Borrelli, Francesco},
 journal = {ArXiv preprint},
 title = {Safe and {{Near}}-{{Optimal Policy Learning}} for {{Model Predictive Control}} Using {{Primal}}-{{Dual Neural Networks}}},
 url = {https://arxiv.org/abs/1906.08257},
 volume = {abs/1906.08257},
 year = {2019}
}

@article{zhang_safe_2021,
 author = {Zhang, Zixu and Fisac, Jaime F.},
 journal = {ArXiv preprint},
 title = {Safe {{Occlusion}}-Aware {{Autonomous Driving}} via {{Game}}-{{Theoretic Active Perception}}},
 url = {https://arxiv.org/abs/2105.08169},
 volume = {abs/2105.08169},
 year = {2021}
}

@inproceedings{zhang_secret_2020,
 author = {Yuheng Zhang and
Ruoxi Jia and
Hengzhi Pei and
Wenxiao Wang and
Bo Li and
Dawn Song},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/ZhangJP0LS20.bib},
 booktitle = {2020 {IEEE/CVF} Conference on Computer Vision and Pattern Recognition,
{CVPR} 2020, Seattle, WA, USA, June 13-19, 2020},
 doi = {10.1109/CVPR42600.2020.00033},
 pages = {250--258},
 publisher = {{IEEE}},
 timestamp = {Tue, 11 Aug 2020 01:00:00 +0200},
 title = {The Secret Revealer: Generative Model-Inversion Attacks Against Deep
Neural Networks},
 url = {https://doi.org/10.1109/CVPR42600.2020.00033},
 year = {2020}
}

@article{zhang_side-tuning_2019,
 author = {Zhang, Jeffrey O. and Sax, Alexander and Zamir, Amir and Guibas, Leonidas and Malik, Jitendra},
 journal = {ArXiv preprint},
 title = {Side-{{Tuning}}: {{Network Adaptation}} via {{Additive Side Networks}}},
 url = {https://arxiv.org/abs/1912.13503},
 volume = {abs/1912.13503},
 year = {2019}
}

@inproceedings{zhang_zoom_nodate,
 author = {Xuaner Zhang and
Qifeng Chen and
Ren Ng and
Vladlen Koltun},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/cvpr/ZhangCNK19.bib},
 booktitle = {{IEEE} Conference on Computer Vision and Pattern Recognition, {CVPR}
2019, Long Beach, CA, USA, June 16-20, 2019},
 doi = {10.1109/CVPR.2019.00388},
 pages = {3762--3770},
 publisher = {Computer Vision Foundation / {IEEE}},
 timestamp = {Mon, 20 Jan 2020 00:00:00 +0100},
 title = {Zoom to Learn, Learn to Zoom},
 url = {http://openaccess.thecvf.com/content\_CVPR\_2019/html/Zhang\_Zoom\_to\_Learn\_Learn\_to\_Zoom\_CVPR\_2019\_paper.html},
 year = {2019}
}

@inproceedings{zhao_cycleemotiongan_2019,
 author = {Sicheng Zhao and
Chuang Lin and
Pengfei Xu and
Sendong Zhao and
Yuchen Guo and
Ravi Krishna and
Guiguang Ding and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/ZhaoLXZGKDK19.bib},
 booktitle = {The Thirty-Third {AAAI} Conference on Artificial Intelligence, {AAAI}
2019, The Thirty-First Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2019, The Ninth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2019, Honolulu, Hawaii,
USA, January 27 - February 1, 2019},
 doi = {10.1609/aaai.v33i01.33012620},
 pages = {2620--2627},
 publisher = {{AAAI} Press},
 timestamp = {Tue, 02 Feb 2021 00:00:00 +0100},
 title = {CycleEmotionGAN: Emotional Semantic Consistency Preserved CycleGAN
for Adapting Image Emotions},
 url = {https://doi.org/10.1609/aaai.v33i01.33012620},
 year = {2019}
}

@article{zhao_data_2020,
 author = {Zhao, Tong and Liu, Yozen and Neves, Leonardo and Woodford, Oliver and Jiang, Meng and Shah, Neil},
 journal = {ArXiv preprint},
 title = {Data {{Augmentation}} for {{Graph Neural Networks}}},
 url = {https://arxiv.org/abs/2006.06830},
 volume = {abs/2006.06830},
 year = {2020}
}

@inproceedings{zhao_end--end_2020,
 author = {Sicheng Zhao and
Yunsheng Ma and
Yang Gu and
Jufeng Yang and
Tengfei Xing and
Pengfei Xu and
Runbo Hu and
Hua Chai and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/ZhaoMGYXXHCK20.bib},
 booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
2020, The Thirty-Second Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
February 7-12, 2020},
 pages = {303--311},
 publisher = {{AAAI} Press},
 timestamp = {Tue, 02 Feb 2021 00:00:00 +0100},
 title = {An End-to-End Visual-Audio Attention Network for Emotion Recognition
in User-Generated Videos},
 url = {https://aaai.org/ojs/index.php/AAAI/article/view/5364},
 year = {2020}
}

@article{zhao_experimental_2020,
 author = {Zhao, Weiye and Sun, Liting and Liu, Changliu and Tomizuka, Masayoshi},
 journal = {ArXiv preprint},
 title = {Experimental {{Evaluation}} of {{Human Motion Prediction}}: {{Toward Safe}} and {{Efficient Human Robot Collaboration}}},
 url = {https://arxiv.org/abs/2001.09550},
 volume = {abs/2001.09550},
 year = {2020}
}

@article{zhao_learning_2019,
 author = {Zhao, Ruihan and Tiomkin, Stas and Abbeel, Pieter},
 journal = {ArXiv preprint},
 title = {Learning {{Efficient Representation}} for {{Intrinsic Motivation}}},
 url = {https://arxiv.org/abs/1912.02624},
 volume = {abs/1912.02624},
 year = {2019}
}

@article{zhao_madan_2020,
 author = {Zhao, Sicheng and Li, Bo and Yue, Xiangyu and Xu, Pengfei and Keutzer, Kurt},
 journal = {ArXiv preprint},
 title = {{{MADAN}}: {{Multi}}-Source {{Adversarial Domain Aggregation Network}} for {{Domain Adaptation}}},
 url = {https://arxiv.org/abs/2003.00820},
 volume = {abs/2003.00820},
 year = {2020}
}

@inproceedings{zhao_multi-source_2019,
 author = {Sicheng Zhao and
Bo Li and
Xiangyu Yue and
Yang Gu and
Pengfei Xu and
Runbo Hu and
Hua Chai and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/ZhaoLYG0HCK19.bib},
 booktitle = {Advances in Neural Information Processing Systems 32: Annual Conference
on Neural Information Processing Systems 2019, NeurIPS 2019, December
8-14, 2019, Vancouver, BC, Canada},
 editor = {Hanna M. Wallach and
Hugo Larochelle and
Alina Beygelzimer and
Florence d'Alch{\'{e}}{-}Buc and
Emily B. Fox and
Roman Garnett},
 pages = {7285--7298},
 timestamp = {Thu, 21 Jan 2021 00:00:00 +0100},
 title = {Multi-source Domain Adaptation for Semantic Segmentation},
 url = {https://proceedings.neurips.cc/paper/2019/hash/db9ad56c71619aeed9723314d1456037-Abstract.html},
 year = {2019}
}

@article{zhao_multi-source_2020,
 author = {Zhao, Sicheng and Li, Bo and Reed, Colorado and Xu, Pengfei and Keutzer, Kurt},
 journal = {ArXiv preprint},
 title = {Multi-Source {{Domain Adaptation}} in the {{Deep Learning Era}}: {{A Systematic Survey}}},
 url = {https://arxiv.org/abs/2002.12169},
 volume = {abs/2002.12169},
 year = {2020}
}

@inproceedings{zhao_multi-source_2020-1,
 author = {Sicheng Zhao and
Guangzhi Wang and
Shanghang Zhang and
Yang Gu and
Yaxian Li and
Zhichao Song and
Pengfei Xu and
Runbo Hu and
Hua Chai and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/aaai/ZhaoWZGLS0HCK20.bib},
 booktitle = {The Thirty-Fourth {AAAI} Conference on Artificial Intelligence, {AAAI}
2020, The Thirty-Second Innovative Applications of Artificial Intelligence
Conference, {IAAI} 2020, The Tenth {AAAI} Symposium on Educational
Advances in Artificial Intelligence, {EAAI} 2020, New York, NY, USA,
February 7-12, 2020},
 pages = {12975--12983},
 publisher = {{AAAI} Press},
 timestamp = {Tue, 02 Feb 2021 00:00:00 +0100},
 title = {Multi-Source Distilling Domain Adaptation},
 url = {https://aaai.org/ojs/index.php/AAAI/article/view/6997},
 year = {2020}
}

@article{zhao_particle_2014,
 author = {Zhao, Bo and Skjetne, Roger and Blanke, Mogens and Dukan, Fredrik},
 doi = {10.1109/TCST.2014.2300815},
 file = {/home/matt/Zotero/storage/3VMJT9D5/06736066.pdf},
 issn = {1063-6536, 1558-0865},
 journal = {IEEE Transactions on Control Systems Technology},
 number = {6},
 pages = {2399--2407},
 title = {Particle {{Filter}} for {{Fault Diagnosis}} and {{Robust Navigation}} of {{Underwater Robot}}},
 volume = {22},
 year = {2014}
}

@inproceedings{zhao_pdanet_2019,
 author = {Sicheng Zhao and
Zizhou Jia and
Hui Chen and
Leida Li and
Guiguang Ding and
Kurt Keutzer},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/mm/ZhaoJCLDK19.bib},
 booktitle = {Proceedings of the 27th {ACM} International Conference on Multimedia,
{MM} 2019, Nice, France, October 21-25, 2019},
 crossref = {DBLP:conf/mm/2019},
 doi = {10.1145/3343031.3351062},
 pages = {192--201},
 timestamp = {Wed, 20 Jan 2021 00:00:00 +0100},
 title = {PDANet: Polarity-consistent Deep Attention Network for Fine-grained
Visual Emotion Regression},
 url = {https://doi.org/10.1145/3343031.3351062},
 year = {2019}
}

@article{zheng_detecting_2006,
 author = {Zheng, J. and Wang, Y. and Nihan, N. L.},
 journal = {Computer-Aided Civil and Infrastructure Engineering},
 pages = {425--435},
 title = {Detecting {{Cycle Failures}} at {{Signalized Intersections Using Video Image Processing}}},
 volume = {21},
 year = {2006}
}

@article{zheng_recent_2014,
 abstract = {This paper comprehensively reviews recent developments in modeling lane-changing behavior. The major lane changing models in the literature are categorized into two groups: models that aim to capture the lane changing decision-making process, and models that aim to quantify the impact of lane changing behavior on surrounding vehicles. The methodologies and important features (including their limitations) of representative models in each category are outlined and discussed. Future research needs are determined.},
 author = {Zheng, Zuduo},
 doi = {10.1016/j.trb.2013.11.009},
 file = {/home/matt/Zotero/storage/K4UPYUP2/Zheng - 2014 - Recent developments and research needs in modeling.pdf},
 issn = {01912615},
 journal = {Transportation Research Part B: Methodological},
 language = {en},
 pages = {16--32},
 title = {Recent Developments and Research Needs in Modeling Lane Changing},
 volume = {60},
 year = {2014}
}

@article{zhou_graph_2019,
 author = {Zhou, Jie and Cui, Ganqu and Zhang, Zhengyan and Yang, Cheng and Liu, Zhiyuan and Wang, Lifeng and Li, Changcheng and Sun, Maosong},
 journal = {ArXiv preprint},
 title = {Graph {{Neural Networks}}: {{A Review}} of {{Methods}} and {{Applications}}},
 url = {https://arxiv.org/abs/1812.08434},
 volume = {abs/1812.08434},
 year = {2018}
}

@article{zhou_plug-electric_2015,
 author = {Zhou, Yan and Wang, Michael and Hao, Han and Johnson, Larry and Wang, Hewu and Hao, Han},
 doi = {10.1007/s11027-014-9611-2},
 file = {/home/matt/Zotero/storage/D7WD2DNJ/s11027-014-9611-2.pdf},
 issn = {1381-2386, 1573-1596},
 journal = {Mitigation and Adaptation Strategies for Global Change},
 language = {en},
 number = {5},
 pages = {777--795},
 shorttitle = {Plug-in Electric Vehicle Market Penetration and Incentives},
 title = {Plug-in Electric Vehicle Market Penetration and Incentives: A Global Review},
 volume = {20},
 year = {2015}
}

@inproceedings{zhu_beyond_2020,
 author = {Jiong Zhu and
Yujun Yan and
Lingxiao Zhao and
Mark Heimann and
Leman Akoglu and
Danai Koutra},
 bibsource = {dblp computer science bibliography, https://dblp.org},
 biburl = {https://dblp.org/rec/conf/nips/ZhuYZHAK20.bib},
 booktitle = {Advances in Neural Information Processing Systems 33: Annual Conference
on Neural Information Processing Systems 2020, NeurIPS 2020, December
6-12, 2020, virtual},
 editor = {Hugo Larochelle and
Marc'Aurelio Ranzato and
Raia Hadsell and
Maria{-}Florina Balcan and
Hsuan{-}Tien Lin},
 timestamp = {Tue, 19 Jan 2021 00:00:00 +0100},
 title = {Beyond Homophily in Graph Neural Networks: Current Limitations and
Effective Designs},
 url = {https://proceedings.neurips.cc/paper/2020/hash/58ae23d878a47004366189884c2f8440-Abstract.html},
 year = {2020}
}

@inproceedings{ziebart_maximum_2008,
 abstract = {Recent research has shown the benefit of framing problems of imitation learning as solutions to Markov Decision Problems. This approach reduces learning to the problem of recovering a utility function that makes the behavior induced by a near-optimal policy closely mimic demonstrated behavior. In this work, we develop a probabilistic approach based on the principle of maximum entropy. Our approach provides a well-defined, globally normalized distribution over decision sequences, while providing the same performance guarantees as existing methods.},
 author = {Ziebart, Brian D and Maas, Andrew and Bagnell, J Andrew and Dey, Anind K},
 booktitle = {Proceedings of the {{Twenty}}-{{Third AAAI Conference}} on {{Artificial Intelligence}}},
 file = {/home/matt/Zotero/storage/4TU5LXSD/Ziebart et al. - Maximum Entropy Inverse Reinforcement Learning.pdf},
 keywords = {⛔ No DOI found},
 language = {en},
 title = {Maximum {{Entropy Inverse Reinforcement Learning}}},
 year = {2008}
}

@article{ziliaskopoulos_cell_1997,
 author = {Ziliaskopoulos, A. K. and Lee, S.},
 journal = {Transportation Research Record},
 number = {1701},
 pages = {12--23},
 title = {A Cell Transmission Based Assignment-Simulation Model for Integrated Freeway/Surface Street Systems.},
 year = {1997}
}

@article{ziliaskopoulos_linear_2000,
 author = {Ziliaskopoulos, A. K.},
 journal = {Transportation Science},
 number = {1},
 pages = {37--49},
 title = {A {{Linear Programming Model}} for the {{Single Destination System Optimum Dynamic Traffic Assignment Problem}}},
 volume = {34},
 year = {2000}
}

@inproceedings{zohdy_game_2012,
 author = {Zohdy, I.H. and Rakha, H.},
 booktitle = {Intelligent {{Transportation Systems}} ({{ITSC}}), 2012 15th {{International IEEE Conference}} On},
 doi = {10.1109/ITSC.2012.6338644},
 keywords = {Acceleration,adaptive control,automated vehicle,CACC system,Control systems,cooperative systems,Delay,delay systems,four-way stop control,game theory,Game theory,Games,heuristic optimization algorithm,intersection controller,intersection-based cooperative adaptive cruise control,manager agent,Monte Carlo methods,Monte Carlo simulation,optimisation,Optimization,reactive agent,road traffic control,road vehicles,total delay,Vehicles},
 pages = {1097--1102},
 title = {Game Theory Algorithm for Intersection-Based Cooperative Adaptive Cruise Control ({{CACC}}) Systems},
 year = {2012}
}

@article{zohdy_intersection_2014,
 author = {Zohdy, Ismail H. and Rakha, Hesham A.},
 doi = {10.1080/15472450.2014.889918},
 journal = {Journal of Intelligent Transportation Systems},
 pages = {1--16},
 title = {Intersection {{Management}} via {{Vehicle Connectivity}}: {{The Intersection Cooperative Adaptive Cruise Control System Concept}}},
 year = {2014}
}

@inproceedings{wang-etal-2020-hat,
 address = {Online},
 author = {Wang, Hanrui  and
Wu, Zhanghao  and
Liu, Zhijian  and
Cai, Han  and
Zhu, Ligeng  and
Gan, Chuang  and
Han, Song},
 booktitle = {Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics},
 doi = {10.18653/v1/2020.acl-main.686},
 pages = {7675--7688},
 publisher = {Association for Computational Linguistics},
 title = {{HAT}: Hardware-Aware Transformers for Efficient Natural Language Processing},
 url = {https://aclanthology.org/2020.acl-main.686},
 year = {2020}
}



==> figTex/counter-example.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{figures/gnn-weak-counter-example.png}
    \caption{GNN cannot capture the similar components in the graph. \zhanghao{Some figure like this}}
    \label{fig:counter-example}
\end{figure}

==> figTex/overview.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\textwidth]{example-image-a}
    \caption{Overview figure TBD}
    \label{fig:overview}
\end{figure}

==> sections/07_checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The main potentially negative societal impact of our work is potentially raising the barrier to entry for GNN research. It is well-known that state-of-the-art Transformer models are among the largest and most costly deep neural networks that exist today. If future results confirm that all-to-all Transformer modules are necessary for top performance on graph datasets, this could potentially make state-of-the-art GNNs as inaccessible to the general public as state-of-the-art NLP models like GPT-3.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report standard deviations for small datasets. For the large datasets, accuracy results are quite stable.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See supplementary material.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Code is included}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
